Classifier Calibration: A survey on how to assess and improve predicted class probabilities

This paper provides both an introduction to and a detailed overview of the principles and practice of classifier calibration. A well-calibrated classifier correctly quantifies the level of uncertainty or confidence associated with its instance-wise predictions. This is essential for critical applications, optimal decision making, cost-sensitive classification, and for some types of context change. Calibration research has a rich history which predates the birth of machine learning as an academic field by decades. However, a recent increase in the interest on calibration has led to new methods and the extension from binary to the multiclass setting. The space of options and issues to consider is large, and navigating it requires the right set of concepts and tools. We provide both introductory material and up-to-date technical details of the main concepts and methods, including proper scoring rules and other evaluation metrics, visualisation approaches, a comprehensive account of post-hoc calibration methods for binary and multiclass classification, and several advanced topics.

==> 01_intro.tex <==
\section{Introduction and motivation}
\label{sec:intro}


A $K$-class probabilistic classifier is \emph{well-calibrated} if among test instances receiving a predicted $K$-dimensional probability vector $\mathbf{s}$, the class distribution is (approximately) distributed as $\mathbf{s}$.  
This property is of fundamental importance when using a classifier for cost-sensitive classification, for human decision making, or within an autonomous system.
It means that the classifier correctly quantifies the level of uncertainty or confidence associated with its predictions. 
In a binary setting, scores given by a sufficiently calibrated classifier can be simply thresholded to minimise expected misclassification cost. Thresholds can also be derived to optimally adapt to a change in class prior, or to a combination of both. In contrast, for a poorly calibrated classifier the optimal thresholds cannot be obtained without optimisation.

Many machine learning algorithms are known to produce over-confident models, unless dedicated procedures are applied during training. 
%(e.g., Laplace smoothing in decision trees \cite{ferri2003improving}).
The goal of \emph{(post-hoc) calibration methods} is to use hold-out validation data to learn a \emph{calibration map} for a previously trained model that transforms the model's predictions to be better calibrated.
Many calibration methods for binary classifiers have been introduced, including
logistic calibration (also known as `Platt scaling'), 
various binning methods including isotonic calibration (also known as the ROC convex hull method), 
as well as more recent methods including beta calibration and Bayesian methods. 

When we have more than two classes, calibration is generally more involved, as is often the case with multiclass classification. 
Multiclass calibration has mostly been approached by decomposing the problem into $K$ one-vs-rest binary calibration tasks, one for each class. The predictions of these $K$ calibration models form unnormalised probability vectors, which, after normalisation, may not be calibrated in a multiclass sense. 
Native multiclass calibration methods were introduced recently focusing on neural networks. These methods constitute various multiclass extensions of Platt scaling, adding a calibration layer between the logits of the neural network and the softmax layer. 

The literature on post-hoc classifier calibration in machine learning is now sufficiently rich that it is no longer straightforward to obtain or maintain a good overview of the area, which was the main motivation for writing this survey. It grew out of a tutorial we presented at the 2020 European Conference on Machine Learning and Principles and Practice of Knowledge Discovery in Databases (see \url{https://classifier-calibration.github.io}). Our aim then and now is to provide both introductory material and up-to-date technical details of the main concepts and methods. \newtext{Our focus is on the classical setup where the classifier is deployed in the same setting where it was calibrated, except for potential changes in class prior or misclassification costs. We do not cover methods to achieve robustness under conditions of other distributional shifts or out-of-distribution inputs \cite{ovadia2019can}.} We try to do justice to historical developments and pay attention to important topics that are not as widely known as they deserve to be, such as proper scoring rules. 

We also try to identify and clarify possible sources for confusion. 
The multiclass setting in particular introduces numerous subtleties that have not always been recognised or correctly dealt with in previous work. 
For example, some authors use the weaker notion of \emph{confidence calibration}, which requires only that the classifier's predicted probability for what it considers the most likely class is calibrated. 
While this is perfectly valid in its own right, it isn't always appreciated by subsequent authors that this is a much weaker notion of calibration than the one defined informally in the first sentence of this survey. 
One can also observe variations in the evaluation metric used and in the way calibrated probabilities are visualised. 
Our main aim in this survey is hence to provide a unified perspective on the different methods and metrics for binary and multiclass calibration, giving each variation its proper place. 

For the purpose of this survey we have developed a Python library which includes most of the functionalities presented in the following sections.
PyCalib~\footnote{https://classifier-calibration.github.io/PyCalib/} implements several calibration metrics (eg. confidence and classwise ECE, and their MCE counterparts), common calibration methods (eg. Isotonic Calibration, Platt's Scaling, Binning calibration), a method to combine arbitrary classifiers and calibrators into a unified training and deployment pipeline, a one-vs-the-rest implementation to adapt any binary calibration method to the multiclass setting, and multiple visualisation tools to inspect visually the calibration quality as well as tools to get better insights about the learned calibration maps.
As an illustration of the library's capabilities, most of the figures and results reported in this paper have been generated using PyCalib.

%Given the lack of a unified code distribution for calibration, we have created a Python library called .
%which includes most of the functionalities presented in this paper to assess calibration.
%This library implements several calibration metrics (eg. confidence-ECE, classwise-ECE, confidence-MCE), common calibration methods (eg. Isotonic Calibration, Platt's Scaling, Binning calibration), a one-vs-the-rest implementation to adapt any binary calibration method for the multiclass setting, and multiple visualisation tools to assess calibration (eg. binary and multiclass reliability diagrams, calibration maps for two and three classes, and other functions to explore three class classification problems). Most of the reliability diagrams and other common calibration metrics in this survey have been generated using this library.

The survey is structured as follows. 
The next section will cover important notions and intuitions related to calibration. \newtext{It aims to be at a more introductory level}, leaving technical detail for later sections. 
Section \ref{sec:psr} discusses proper scoring rules, an important general framework for evaluation of probability estimates. In Section \ref{sec:metrics} we present systematic overview of visualisation approaches and evaluation metrics for classifier calibration. 
Section \ref{sec:calibrators} is devoted to a comprehensive account of post-hoc calibration methods for both the binary and multiclass scenarios. 
Section \ref{sec:hyp} covers hypothesis tests for calibration, and Section \ref{sec:conclusion} concludes with a summary and outlook. 

==> 02_highlevel_intro.tex <==
\section{A brief introduction to classifier calibration}
\label{sec:intro:high:level}

\newtext{
The origins of classifier calibration can be traced back to weather forecasting and meteorology. 
Here is what the UK Met Office website used to say about what their forecast probabilities mean: 

\begin{quote}
    ``[S]uppose the Met Office says that the probability of rain tomorrow in your region is 80\%. They aren't saying that it will rain in 80\% of the land area of your region, and not rain in the other 20\%. Nor are they saying it will rain for 80\% of the time. What they are saying is there is an 80\% chance of rain occurring at any one place in the region, such as in your garden.
[...]
[A] forecast of 80\% chance of rain in your region should broadly mean that, on about 80\% of days when the weather conditions are like tomorrow's, you will experience rain where you are. 
%But there is still some expert judgement involved, and different forecasting organisations with different experts and different technology might well give different probabilities.
[...]
If it doesn't rain in your garden tomorrow, then the 80\% forecast wasn't wrong, because it didn't say rain was certain. But if you look at a long run of days, on which the Met Office said the probability of rain was 80\%, you'd expect it to have rained on about 80\% of them. '' %
%(\url{https://www.metoffice.gov.uk/about-us/what/accuracy-and-trust})
(\url{https://web.archive.org/web/20210928235732/https://www.metoffice.gov.uk/about-us/what/accuracy-and-trust/probability})
%\todo[inline]{The link is broken now. I found an archived version from Sept. 28, 2021 in the Internet Archive.}
\end{quote}
\noindent
Note the phrase ``a long run of days'': determining the degree to which a forecaster is well-calibrated cannot be done on a per-forecast basis, but rather requires looking at a sufficiently large and diverse set of forecasts. 

\begin{table}[!t]
        \centering
        \includegraphics[width=\linewidth]{hallenbeck1920_tab1}
        \caption{Reproduced from \citet{hallenbeck1920}.}
        \label{tab:eval:hallenbeck1920}
\end{table}

\begin{figure}[!b]
    \centering
%    \includegraphics[width=0.6\linewidth]{Hallenbeck.pdf}\\
    \begin{subfigure}[b]{0.45\linewidth}
    \includegraphics[width=\linewidth]{Hallenbeck.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{0.40\linewidth}
    \includegraphics[width=\linewidth]{hallenbeck_alt.pdf}
    \end{subfigure}
    \caption{Two different graphical representations of the forecasts in Table~\ref{tab:eval:hallenbeck1920}.
\textbf{(Left)} The bottom graph gives a histogram of the probability forecasts. 
The top graph compares the forecast probabilities with the proportion of actual rain events in that bin. 
The red bars indicate to what extent these proportions are higher or lower than predicted. 
\textbf{(Right)} A simplified visualisation, only showing the proportion of rain events in a bin (y-axis) against the average prediction in the bin (x-axis).
    }\label{fig:hallenbeck-rel}
\end{figure}


Table~\ref{tab:eval:hallenbeck1920}, reproduced from \citet{hallenbeck1920}, groups 123 weather forecasts in 10 equal-width bins, and compares each bin with the actual empirical percentage of rain events. 
Figure~\ref{fig:hallenbeck-rel} shows two possibilities of displaying this information graphically, comparing the predicted probabilities on the $x$-axis to empirical probabilities on the $y$-axis. 
A variety of such graphical representations can be found in the literature; they are generally known as \emph{reliability diagrams}, `reliability' being one of many terms used to denote goodness of calibration \cite{murphy1977reliability}.
We can see that most of the forecasts are slight under-estimates: for example, of the 15 forecasts in the 40-49\% bin, $8/15=53\%$ were actual rain events. 
In the left graph this is shown by the vertical red line, which indicates how much the top of the blue bar extends above the diagonal (meaning that the actual proportion of rain events was higher than estimated). 
On the right graph this can be seen directly from how much the respective point is higher than the diagonal.
Similarly, we see that two of the bins (20-29\% and 30-39\%) are very slight over-estimates: on the left graph the top of the blue bar is below the diagonal, which means that the actual proportion of rain events was lower than estimated. 

\begin{figure}[!t]
    \centering
    \begin{subfigure}{0.45\linewidth}
    \includegraphics[width=\linewidth]{Hallenbeck2.pdf}
    \end{subfigure}
    \begin{subfigure}{0.45\linewidth}
    \includegraphics[width=\linewidth]{Hallenbeck3.pdf}
    \end{subfigure}
    \caption{Dividing the forecasts in Table~\ref{tab:eval:hallenbeck1920} in five (left figure) and two (right figure) equal-width bins.}\label{fig:hallenbeck2-rel}
\end{figure}

The choice of ten equal-width bins is somewhat arbitrary, and it is informative to consider different choices. 
Merging pairs of adjacent bins results in five equal-width bins, as depicted in Figure~\ref{fig:hallenbeck2-rel} (left). 
We see that all but the right-most bin averages are now slightly off-centre (we assumed that within each original bin all forecast probabilities are the same and equal to the bin centre: e.g., 25\% in the 20-29\% bin). Again, the pattern is that the higher forecast probabilities are about 10\% too low. 
Figure~\ref{fig:hallenbeck2-rel} (right) shows what we get with only two bins. 
We have lost a bit too much information here, so bins shouldn't be taken too wide. 
On the other hand they shouldn't be taken too narrow either, in order to be able to measure the true proportion of rain events with sufficient resolution. 

Taking the forecast event as a binary variable means that the calibration concept is directly applicable to binary classification. Here is an example from the typical machine learning task of learning a classifier for distinguishing `junk' or `spam' emails from regular ones: 

\begin{quote}
    A prediction `70\% chance of spam' should be spam 70\% of the time.
\end{quote}
\noindent
And a generalisation to categorical variables with more than two values is equally straightforward, as this example from Fisher's famous Iris dataset shows: 

\begin{quote}
    A prediction `70\% chance of setosa, 10\% chance of versicolor and 20\% chance of virginica' should be setosa/versicolor/virginica 70/10/20\% of the time.
\end{quote}
\noindent
So, to sum up: \emph{A predicted probability (vector) should match empirical (observed) probabilities.}
\newtext{
In the language of predictive machine learning, given an instance space $\mathbb{X}$, a binary target space $\mathbb{Y} = \{+, -\}$, and a binary probabilistic classifier $\mathsf{f}:\mathbb{X}\rightarrow [0, 1]$, the binary classifier is \emph{calibrated} if $\forall s \in[0,1]$:
\begin{align*} 
\mathsf{P}(Y=+ \: | \: \mathsf{f}(\mathbf{X}) = s)=s
\end{align*}}




% \subsection{A closer look at calibration, and why it matters}
% \label{sec:2:1}

% % \paragraph{Why are we interested in calibration?}
% In general, to calibrate means \emph{to employ a known scale with known properties}. 
% % \bb{E.g., additive scale with a well-defined zero, so that ratios are meaningful.}
% For example, we can calibrate a thermometer to Celsius or Fahrenheit scales; 
% or a weighing device to kilograms or pounds. 
% If a measuring device is calibrated to one scale but we need the measurement in another, there are usually simple conversion formulas: 
% for example, $\text{F}=\text{C}\cdot 9/5+32$ for Celsius to Fahrenheit, and $\text{Lb}=2.2\cdot \text{Kg}$ for kilograms to pounds. 
% Notice that the temperature conversion shifts the zero point 
% (0 degrees Celsius is 32 degrees Fahrenheit, and 0 degrees Fahrenheit is $-17.8$ degrees Celsius) 
% as it is essentially arbitrarily chosen for either scale. 

% The weight conversion, in contrast, has an absolute zero which is the same for all scales. 
% Such scales are called \textit{ratio scales}, because the ratio of two measurements is meaningful: e.g., if one object is twice as heavy as another in kilograms then it will be so regardless of the scale. Such ratios are not meaningful for Celsius and Fahrenheit, but temperature \textit{differences} are.  
% For example, we could say that this person's change from morning to evening body temperature today is twice that of yesterday, without specifying the temperature scale. 
% It follows that ratios of differences (or intervals) are meaningful in this case, which is why Celsius and Fahrenheit are called \textit{interval scales}. 

% For classifiers we want to use the probability scale. Probabilities have an absolute zero like any other ratio scale, and so it is meaningful to say that one event is twice as probable as another. Probabilities also have a fixed maximum, so that taking the complement with respect to the maximum gives another ratio scale: for example, the probability of this event \textbf{not} happening might be twice the probability of another event \textbf{not} happening. This essentially fixes the scale: we don't have pounds vs.\ kilograms dilemmas for probabilities. 

% % Q: Is the probability scale additive?
% Are probabilities additive? In certain situations it is indeed valid to sum probabilities, for example to obtain the probability of any one of a number of mutually exclusive events happening, as might occur when joining classes in a multiclass classification setting. 
% But multiplication and division of probabilities are more common basic operations, for example to obtain the joint probability of independent events, or to derive a conditional probability from joint and marginal probabilities. This makes the probability scale \textit{multiplicative} for typical usage. We could obtain an additive scale by taking logarithms, giving log-likelihoods, logits as differences of log-likelihoods, etc. A couple of observations are worth making: 
% \begin{itemize}
% \item Such transformations are fundamentally different from scale conversions such as Celsius to Fahrenheit, because probabilities and log-likelihoods measure different things -- physicists might say they represent different \textit{dimensions}. Nevertheless, the transformations are invertible and hence the dimensions convey the same information. 
% \item While some ratios or products of probabilities again yield probabilities, in other cases they may derive another dimension, such as \textit{odds}, which are not expressed on a probability scale.
% \end{itemize}

\subsection{Why calibration matters}
\label{sec:int:why}

What are the benefits of using well-defined calibrated scales in general, and well-calibrated probabilities in particular? One obvious benefit of calibrated scales is that we can easily combine measurements that are expressed on the same scale without comparing apples and oranges. Another is that we can use standardised decision rules, e.g., defining a fever as a body temperature exceeding 100 degrees Fahrenheit. These benefits
% \footnote{As for combining multiple probability estimates as might happen in ensemble methods in machine learning, note that the argument of probabilities being multiplicative leads to favouring the \textit{geometric mean} (or the arithmetic mean on log-probabilities). Using the arithmetic mean directly on probabilities means that the members of the ensemble are treated as classifiers scoring on some arbitrary but fixed and additive scale, disregarding their probabilistic nature.}
directly carry over to the class probability scenario, justifying decision rules such as predicting the class whose estimated probability exceeds $0.5$ in binary classification, or the class with the highest predicted probability for multiclass classification. Importantly, there is a further benefit to using calibrated probabilities as it means we can adjust these decision rules in a straightforward way to account for different class priors or misclassification costs, as we will briefly discuss presently.

% %Q: What issues might arise when applying MAP decisions to poorly calibrated classifiers such as naive Bayes? 

% % PF: UNTIL HERE (27 JAN 9.30 GMT)

% % \paragraph{Optimal decisions}
% Denote the cost of predicting class $j$ for an instance of true class $i$ as ${\mathsf{C}(\hat{Y}=j|Y=i)}$. 
% % Since we don't know the true class of an unlabelled instance, we need to base our prediction on an assessment of the expected cost over all possible true classes. 
% The expected cost of predicting class $j$ for instance $\mathbf{x}$ is then
% %
% \begin{align}\label{eq::expected-cost}
% \mathsf{C}(\hat{Y}=j|\mathbf{X}=\mathbf{x}) &= \sum_i \mathsf{P}(Y=i|\mathbf{X}=\mathbf{x})\mathsf{C}(\hat{Y}=j|Y=i)
% \end{align}
% %
% where $\mathsf{P}(Y=i|\mathbf{X}=\mathbf{x})$ is the (true) probability of instance $\mathbf{x}$ having true class $i$
% (as would be given by the Bayes-optimal classifier). 
% %
% The optimal decision is to predict the class with lowest expected cost:
% \begin{align*}
% \hat{Y}^* = \argmin_j \mathsf{C}(\hat{Y}=j|\mathbf{X}=\mathbf{x}) = \argmin_j \sum_i \mathsf{P}(Y=i|\mathbf{X}=\mathbf{x})\mathsf{C}(\hat{Y}=j|Y=i)
% \end{align*}
% %
% % In the special case that all misclassifications have equal cost we can assume without loss of generality that $C(\hat{Y}=j|Y=i)=1$ for $i\neq j$ and $C(\hat{Y}=j|Y=i)=0$ for $i=j$, which gives
% % \begin{align*}
% % C(\hat{Y}=j|X=x) &= \sum_{i\neq j} P(Y=i|X=x) = 1-P(Y=j|X=x) \\
% % %\end{align*}
% % %and so
% % %\begin{align*}
% % \hat{Y}^* &= \arg\min_j [1-P(Y=j|X=x)] = \argmax_j P(Y=j|X=x)
% % \end{align*}
% In binary classification (with a positive, $+$, and and negative class, $-$) we have one predicted probability and four cost parameters, and we can rewrite Equation~(\ref{eq::expected-cost}) as
% %
% \begin{align*}
% \mathsf{C}(\hat{Y}=+|\mathbf{X}=\mathbf{x}) &= \mathsf{P}(+|\mathbf{x})\mathsf{C}(+|+) + \big(1-\mathsf{P}(+|\mathbf{x})\big)\mathsf{C}(+|-) \\
% \mathsf{C}(\hat{Y}=-|\mathbf{X}=\mathbf{x}) &= \mathsf{P}(+|\mathbf{x})\mathsf{C}(-|+) + \big(1-\mathsf{P}(+|\mathbf{x})\big)\mathsf{C}(-|-)
% \end{align*}
% %
% where $\mathsf{P}(+|\mathbf{x})$ is shorthand for $\mathsf{P}(Y=+|\mathbf{X}=\mathbf{x})$ and $\mathsf{C}(j|i)$ for $\mathsf{C}(\hat{Y}=j|Y=i)$.
% %
% On the optimal decision boundary these two expected costs are equal, 
% which gives
% \begin{align*}
% \mathsf{P}(+|\mathbf{x})\mathsf{C}(+|+) + (1-\mathsf{P}(+|\mathbf{x}))\mathsf{C}(+|-) = \mathsf{P}(+|\mathbf{x})\mathsf{C}(-|+) + (1-\mathsf{P}(+|\mathbf{x}))\mathsf{C}(-|-)
% \end{align*}
% which can be rearranged to give the posterior odds
% \begin{align*}
% \frac{\mathsf{P}(+|\mathbf{x})}{1-\mathsf{P}(+|\mathbf{x})} = \frac{\mathsf{C}(+|-)-\mathsf{C}(-|-)}{\mathsf{C}(-|+)-\mathsf{C}(+|+)}
% \end{align*}
% as well as the posterior probability
% \begin{align*}%\label{eq::cost-threshold}
% \mathsf{P}(+|\mathbf{x})  = \frac{{\mathsf{C}(+|-)-\mathsf{C}(-|-)}}{{\mathsf{C}(+|-)-\mathsf{C}(-|-)}+{\mathsf{C}(-|+)-\mathsf{C}(+|+)}} \triangleq c
% \end{align*}
% %
% $c$ thus gives the optimal threshold on the hypothetical Bayes-optimal probabilities. 
% It is also the best thing to do in practice, as long as the probabilities are well-calibrated (this is discussed in more detail in Section~\ref{sec:out:conc}). 

% Under reasonable assumptions (e.g., changing the prediction from correct to incorrect cannot decrease the incurred cost) we can set the cost of true positives and true negatives to zero \cite{elkan2001}; 

Let
$c = \frac{\mathsf{C}(+|-)}{\mathsf{C}(+|-) + \mathsf{C}(-|+)}$ be the cost of a false positive in proportion to the combined cost of one false positive and one false negative. 
With these cost parameters the Bayes-optimal decision rule is to set the decision threshold to $c$.
For instance, if false positives are 4 times as costly as false negatives then we set the decision threshold to $4/(4+1)=0.8$ in order to only make positive predictions if we are sufficiently certain.
%
Similar reasoning applies to changes in class priors: 
\begin{itemize}
    \item if we trained on balanced classes but want to deploy with 4 times as many positives compared to negatives, we lower the decision threshold to $0.2$; 
    \item more generally, if we trained for class ratio $r$ and deploy for class ratio $r'$ we set the decision threshold to $r/(r+r')$. 
\end{itemize}
Cost and class prior changes can be combined in the obvious way; see  \citet{flach2014classification} for details.

In summary, an important reason to be interested in calibrating our classifiers is that default decision rules such as predicting the class with the highest predicted probability are fully justified from a decision-theoretic point of view, and can easily be adapted to changes in class and cost distributions. In contrast, poorly calibrated classifiers such as naive Bayes will often perform sub-optimally with default decision rules. It is possible to learn a better decision rule for a given cost and class skew using, e.g., ROC analysis \cite{lachiche2003improving} but this would have to be repeated each time the skew changes. The great advantage of post-calibration is that it only needs to be done once -- in a sense, it optimises all possible decision rules in one go.

%\todo{mention fairness and explainability?}

%\subsection{Challenges in evaluating calibration}
%Impact of binning for reliability diagrams}



\subsection{Common forms of miscalibration, and how to fix them}

There are many reasons why a probabilistic classifier might produce miscalibrated scores, and hence many ways in which miscalibration manifests itself, but two main types stand out: underconfidence and overconfidence. In this section we look at some examples and introduce two mitigation techniques. 

 
Figure~\ref{fig:under-over}, taken from \citet{niculescu-mizil2005}, shows two typical examples. In both cases the points in the reliability diagram are far from the diagonal, although the effect is smaller in the figure on the right. 

\begin{figure}[!t]
    \centering
    \begin{subfigure}{0.4\linewidth}
        \includegraphics[width=\linewidth]{caruana_fig_1.pdf}
        \caption{Underconfidence}
    \end{subfigure}%\hfill
    \hspace{1cm}
    \begin{subfigure}{0.4\linewidth}
        \includegraphics[width=\linewidth]{caruana_fig_2.pdf}
        \caption{Overconfidence}
    \end{subfigure}
    \caption{Examples of under- and overconfident classifiers. The axes are the same as for the previous figures: x-axis shows predicted probabilities and y-axis shows empirical probabilities. The dots represent the reliability diagram, and the lines show the best-fit logistic curve and beta curve.
    %To correct the underconfident scores on the left we would have to pull the points away from the midpoint on the $x$-axis, whereas to deal with the overconfidence on the right we would push them toward the midpoint. 
    Note that the logistic sigmoid is a good fit for underconfident scores but not for overconfidence.
    The figure has been adapted from \citet{niculescu-mizil2005}, and the beta curves have been added.}
    \label{fig:under-over}
\end{figure}


% \begin{figure}[!t]
%     \centering
%     \begin{subfigure}{0.3\linewidth}
%         \includegraphics[width=\linewidth]{Underconfidence.pdf}
%         \caption{Underconfidence, logistic curve}
%     \end{subfigure}\hfill
%     \begin{subfigure}{0.3\linewidth}
%         \includegraphics[width=\linewidth]{Overconfidence.pdf}
%         \caption{Overconfidence, logistic curve}
%     \end{subfigure}
%     \begin{subfigure}{0.35\linewidth}
%         \includegraphics[width=\linewidth]{betafig.pdf}
%         \caption{Overconfidence, beta curve}
%     \end{subfigure}
%     \caption{Examples of under- and overconfident classifiers. The axes are the same as for the previous figures: x-axis shows predicted probabilities and y-axis shows empirical probabilities. The dots represent the reliability diagram, and the line shows the best-fit logistic curve (a,b) or beta curve (c).
%     %To correct the underconfident scores on the left we would have to pull the points away from the midpoint on the $x$-axis, whereas to deal with the overconfidence on the right we would push them toward the midpoint. 
%     Note that the logistic sigmoid is a good fit for underconfident scores but not for overconfidence.
%     Figures (a,b) are reproduced from \citet{niculescu-mizil2005}.}
%     \label{fig:under-over}
% \end{figure}

What do we see in the left figure? It is quite natural to give precedence to vertical information in such graphs, so you might be inclined to say ``The points on the left are too low, and the points on the right are too high''. But keeping in mind that the predicted probabilities on the $x$-axis are under our control but not the empirical probabilities on the $y$-axis, a more `actionable' way to express this is

\begin{quote}
    The lower points are too far to the right, and the higher points are too far to the left. In other words, the points have a tendency to sit too close to the midpoint on the $x$-axis. 
\end{quote}
\noindent
This is the typical pattern displayed by an \textit{underconfident} classifier, which thinks it's {worse} at separating classes than it actually is. 

Hence, to mitigate this, we need to {pull predicted probabilities away from the centre}. As the left plot in Figure \ref{fig:under-over} shows, this can be neatly modelled by a sigmoidal logistic curve, which can be defined in parametric form as
%
\begin{align*}
    \mathsf{c}(s; w, m) &= \frac{1}{1+\exp(-w(s-m))}%\\
    % w &= (\mu_{\textit{pos}}-\mu_{\textit{neg}})/\sigma^2, 
    % m = (\mu_{\textit{pos}}+\mu_{\textit{neg}})/2
\end{align*}
%
Here, $s$ is the uncalibrated score produced by the classifier and $\mathsf{c}$ gives the logistically calibrated score. 
$m$ and $w$ are the two parameters of the logistic family, which determine the point where $\mathsf{c}(s)=0.5$ and the slope at that point, respectively. They can be estimated from the points in the reliability diagram in order to find the best fit. In this case they can be obtained analytically as the mean of the classwise average scores, and the difference between those two means in proportion to the score variance \cite{flach2012machine}.
%(which is assumed to be the same for both classes). 

The fitted logistic curve thus establishes a \textit{calibration map} which transforms uncalibrated scores $s$ into calibrated scores $\mathsf{c}(s)$. 
Even though the calibration map doesn't map to empirical probabilities, plotting it over the reliability diagram allows us to see clearly that if we project each point in the reliability diagram vertically onto the calibration map, and replace its $x$-value with the corresponding $y$-value of the projection, we end up with points on or very close to the diagonal, and hence near-perfectly calibrated scores (Figure~\ref{fig:under-cal}).

\begin{figure}[!t]
    \centering
        \includegraphics[width=0.5\linewidth]{caruana_fig_3.pdf}
    \caption{Graphical illustration of how a well-fitted calibration map leads to near-perfect calibration. From left to right, the dotted arrows show (1) using a point's uncalibrated score $s$ on the $x$-axis as input to the calibration map, (2) mapping the resulting output $\mathsf{c}(s)$ back to the diagonal, and (3) combine with the empirical probability of the point we started from. The closer the original point is to the fitted calibration map, the closer the calibrated point (in red) will be to the diagonal. }
    \label{fig:under-cal}
\end{figure}

The logistic curve is widely used as a `squashing function', compressing values on a possibly unbounded scale into the $[0,1]$ interval. 
Following \citet{platt2000} it is often used as a way to convert scores from a Support Vector Machine into probabilities. 
Technically this isn't calibration as SVM scores are not probabilities but (signed) geometric distances from the decision boundary -- this is also called \textit{scaling} to emphasise the difference \newtext{(hence the popular name `Platt scaling`)}. 
The parametric form of the logistic map can be derived from first principles by assuming that within each class the uncalibrated scores are normally distributed with the same variance. % (Figure~\ref{fig:logistic}). 
\label{page:platt}

% \begin{figure}[!b]
%     \centering
%     \includegraphics[width=0.6\textwidth]{Logistic.pdf}\vfill
%     \caption{Assuming normally distributed scores within each class (left) leads to a logistic calibration map (right).}\label{fig:logistic}
% \end{figure}

The other common form of miscalibration is overconfidence, as exemplified in Figure~\ref{fig:under-over}(b,c). 
% Here, we see that
%
% \begin{quote}
%     The lower points are too far to the left, and the higher points are too far to the right. In other words, the points have a tendency to be too far from the midpoint on the $x$-axis. 
% \end{quote}
% \noindent
An \textit{overconfident} classifier thinks it's {better} at separating classes than it actually is. 
Hence we need to {make predicted probabilities less extreme by pushing them toward the centre}. 
The paper we took this figure from \cite{niculescu-mizil2005} also fitted a logistic curve to this reliability diagram Figure~\ref{fig:under-over}(b), because they were investigating the effect of Platt scaling in a wide range of scenarios. But we see clearly that the fit is rather poor, and using this logistic curve as a calibration map is likely to make matters worse. In this particular case we would be looking for something that can produce an inverse sigmoidal curve. What would be a principled way to achieve this? 

%\begin{figure}[!b]
%    \centering
%    \includegraphics[width=0.9\textwidth]{Beta.pdf}
%    \caption{An example of Beta calibration where overconfident scores (left) lead to an inverse-sigmoidal calibration map (right).}\label{fig:beta}
%\end{figure}

One approach that works well is to model the classwise scores with Beta distributions \cite{pmlr-v54-kull17a,kull2017beyond}.
These assume random variables bounded in $[0,1]$ which is exactly what we need for post-hoc calibration. 
Beta distributions can easily model the skewed distributions resulting from overconfident classifiers, as demonstrated in Figure~\ref{fig:under-over}(b).%Figure~\ref{fig:beta}. 
Mathematically, these curves have three parameters: 
%
    \begin{align*}
        \mathsf{c}(s; a, b, c) &= \frac{1}{1+\exp(-a \ln s + b \ln (1-s) - c)}
        % a &= \alpha_{\textit{pos}}-\alpha_{\textit{neg}}, 
        % b = \beta_{\textit{neg}}-\beta_{\textit{pos}}
    \end{align*}
%
This additional degree of freedom allows Beta calibration to produce both sigmoidal and inverse-sigmoidal calibration maps. 
It can even fit the identity map ($a=b=1$, $c=0$), which means that Beta calibration can recognise that scores are already calibrated. 
In contrast, applying logistic calibration to a calibrated classifier will decalibrate it. 
While Beta calibration can achieve many shapes of calibration maps, it is still a limited parametric family.
Methods to fit richer calibration map families will be discussed in Section~\ref{sec:calibrators}.

%PF: UNTIL HERE (28 JAN 18.00 GMT)

% So far we have seen two calibration techniques: 
% \begin{itemize}
%     \item logistic calibration, which -- although technically a scaling technique, mapping real-valued scores into probabilities -- can adjust for underconfident scores; 
%     \item Beta calibration, which assumes a classifier already scores on a probability scale, and which can adjust for both over- and underconfident scores. 
% \end{itemize}
% We will now take a first look at 
%%% A third calibration technique
%%% % quite different from these two because it 
%%% derives a calibration map from the \textit{ranks} of a set of scores, and hence works for classifiers scoring on arbitrary scales. It is also different from logistic and Beta calibration because it doesn't attempt to model the classwise score distributions, and is hence \textit{non-parametric}. 
%%% %
%%% The technique in question is called \textit{isotonic regression}, belying its origin as an alternative to linear regression which learns a piecewise constant, monotonically increasing or decreasing function. There are several algorithms for isotonic regression, one of which is called \textit{pooled adjacent violators}, which in turn is also used for constructing the convex hull of an ROC curve \cite{zadrozny2001obtaining,fawcett2007}. Figure~\ref{fig:isotonic} demonstrates this graphically. 
%%% 
%%% \begin{figure}[!t]
%%%     \centering
%%%     \begin{subfigure}{0.44\linewidth}
%%%     \includegraphics[width=\linewidth]{ROCCH.pdf}
%%%     \caption{ROC curve and convex hull.}
%%%     \end{subfigure}
%%%     \begin{subfigure}{0.55\linewidth}
%%%     \includegraphics[width=\linewidth]{ROCcal2.pdf}
%%%     \caption{Isotonic calibration map.}
%%%     \end{subfigure}
%%%     \caption{An example of isotonic calibration which derives a piece-wise constant calibration map from the ROC convex hull (Source: \cite{flach2016roc}).}\label{fig:isotonic}
%%% \end{figure}
%%% 
%%% The technique starts from a list of test instances, ranked on their scores; this might give a list of class labels like that depicted at the top of the right figure in Figure~\ref{fig:isotonic}. We then proceed to segment this ranking such that, in each adjacent pair of segments, the right neighbour has a larger proportion of positives than the left neighbour. This defines a unique set of segments, which is depicted on the right of the right figure. Each segment defines an interval on the original classifier scores, as well as an empirical probability of positives in that segment which is taken as the calibrated score for all instances whose score falls in that interval. The calibration map is thus piece-wise constant and increasing. 
%%% 
%%% As a non-parametric method, isotonic regression avoids problems of misspecification which can plague parametric models. For example, a perfectly calibrated classifier has classwise scores which are far from normally distributed, so applying logistic calibration will make matters worse. The downside is that isotonic regression tends to need more labelled data to reliably estimate the segment boundaries and the empirical probabilities within each segment, and is more liable to overfitting if data is not plentiful. 
%%% 

%----------------------------------------------------%
\subsection{Multiclass calibration}
%----------------------------------------------------%

The examples we have seen so far all relate to binary classification. Is it straightforward to generalise calibration concepts and methods to more than two classes? 
The answer to this question is somewhat involved. Some ideas do generalise quite easily: for example, we can model per-class scores by multivariate distributions such as Dirichlet distributions \cite{kull2019}. Some other ideas don't generalise easily at all: for example, a multiclass generalisation of isotonic regression is not straightforward because rankings are inherently bipartite. Such approaches therefore need to be approximated by considering classes in a pairwise or one-versus-rest manner. 

This helps to explain why there is divergence even at a definitional level. 
There are at least three different ways of \emph{defining} what it means to be calibrated in a multiclass setting. 
They are equivalent for binary classification but increasingly stronger for more than two classes,%
\footnote{In rare cases it is possible for a multiclass classifier to be classwise calibrated but not confidence calibrated.
% Example due to Meelis
Here is an example with 40 instances in four groups:
10 instances with predicted probabilities (0.3,0.3,0.4) and actual class distribution (4,2,4);
another 10 with probabilities (0.4,0.3,0.3) and classes (3,4,3);
another 10 with probabilities (0.4,0.6,0.0) and classes (5,5,0);
and the remaining 10 instances with probabilities (0.3,0.6,0.1) and classes (2,7,1).
This classifier is classwise-calibrated but not confidence-calibrated. There are 20 instances with confidence level 0.6 and accuracy 0.6 (5+7=12 out of 20), but the remaining 20 instances have confidence 0.4 and accuracy 0.35 (4+3=7 out of 20). The key idea of this construction is that classwise calibration considers the instances with 0.4 predicted for class 1 as a single group, but confidence calibration looks among them only at those instances for which 0.4 is the highest probability -- e.g., it does consider (0.4,0.3,0.3) but not (0.4,0.6,0.0).}
and can be summarised as follows: 
    \begin{itemize}
        \item {Confidence calibration}: only consider the highest predicted probability. 
        \item {Classwise calibration}: only consider marginal probabilities.
        \item {Multiclass calibration}: consider the entire vector of predicted probabilities.
    \end{itemize}
We will use this terminology throughout the paper to avoid confusion. 

%\renewcommand{\vph}{\hat{\mathbf{p}}}

\textit{Confidence calibration} was proposed by \citet{guo2017}, although not under that name. It requires that among all instances where the probability of \emph{the most likely class} is predicted to be $\alpha$, the expected accuracy is $\alpha$. 
Let $\mathbb{X}$ denote the instance space and $\mathbb{P}_{\mathbb{Y}}$ the probability $K$-simplex, then a probabilistic classifier $\mathsf{f}:\mathbb{X}\rightarrow\mathbb{P}_{\mathbb{Y}}$ is \emph{confidence-calibrated}, if for any confidence level $\alpha\in[0,1]$, 
the actual proportion of the predicted class, among all possible instances $\mathbf{x}$ being predicted this class with confidence $\alpha$, is equal to $\alpha$:  
\begin{align*} 
\mathsf{P}(Y=\hat{Y} \: | \: S_{\hat{Y}}=\alpha)=\alpha\qquad\text{where }\ \hat{Y}=\argmax_j S_j.
%P\Big(Y=\argmax\big(\vph(X)\big) \: \Big| \: \max\big(\vph(X)\big)=c\Big)=c.
\end{align*}
Here, $S_j$ denotes the $j$-th dimension of $\mathsf{f}(\mathbf{X})$.

\textit{Classwise calibration}, proposed by \citet{zadrozny2002}, requires that all \emph{one-vs-rest} probability estimators obtained from the original multiclass model are calibrated. 
Formally, a probabilistic classifier $\mathsf{f}:\mathbb{X}\rightarrow\mathbb{P}_{\mathbb{Y}}$ is \emph{classwise-calibrated}, if for any class $i \in \{1, \dots, K\}$ and any predicted probability value $s \in [0, 1]$ for this class, 
the actual proportion of class $i$, among all possible instances on the random variable $\mathbf{X}$ getting the same prediction on class i, is equal to $s$:  
\begin{align*} 
\mathsf{P}(Y=i\mid S_i=s)=s
\end{align*}

\textit{Multiclass calibration}, also called \textit{calibration in the strong sense} \cite{widmann2019calibration}, is the {strongest form of calibration} for more than two classes, subsuming the previous two definitions. 
A probabilistic classifier $\mathsf{f}:\mathbb{X}\rightarrow\mathbb{P}_{\mathbb{Y}}$ is \emph{multiclass-calibrated} if for any prediction vector $\mathbf{s}=[s_1,\dots,s_K]\in\mathbb{P}_{\mathbb{Y}}$, the proportions of classes among all possible instances on the random variable $\mathbf{X}$ getting the same prediction $\mathsf{f}(\mathbf{X})=\mathbf{s}$ are equal to the prediction vector $\mathbf{s}$:  
\begin{align*} %\label{eq:calib}
\mathsf{P}(Y=i\mid \mathsf{f}(\mathbf{X})=\mathbf{s})=s_i\qquad\text{for }\ i=1,\dots,K.
\end{align*}
%
%Here $\mathbf{s}=[s_1, \dots, s_K]$ denotes the $K$-dimensional probability vector instance.

For practical purposes, the conditions in these definitions need to be relaxed. This is where {binning} comes in. 
Once we define the bins, we can draw a {reliability diagram} as in the two-class case. For classwise calibration, we can show per-class reliability diagrams or a single averaged one. 
One way to assess the degree of calibration is by means of the {gaps} in the reliability diagram. 
These topics will be explored in Section \ref{sec:metrics}. 
We will first take a closer look at the important concept of \emph{proper scoring rules} in the next section. Proper scoring rules are instance-wise evaluation measures for probability estimates that avoid the need for score binning. As a result they cannot measure the degree of calibration directly, but through decomposition results, we will show how the scores can be decomposed into various components, including the calibration loss. 

}


==> 03_evaluation.tex <==
\section{From proper scoring rules to calibration}
\label{sec:psr}




%----------------------------------------------------%
% \subsection{Proper scoring rules}
% \label{sec:met:psr}
%----------------------------------------------------%

% {\color{red}(TODO: Mention this \cite{savage1971}.)}
    
As early as 1950 researchers were interested in scoring functions that would evaluate probabilistic forecasts without influencing the forecaster into making undesirable predictions \cite{brier1950}, thus keeping the forecaster ``honest'' while encouraging useful forecasts. In the late 1960s the term \emph{proper scoring rule} was already in use for score functions whose computation was based on a forecaster's probabilities and the actual occurrence or not of the corresponding events \cite{winkler1969scoring}. Informally, a scoring rule is said to be proper if optimal values are obtained by the forecaster predicting the true probabilities of the events. %At the same time, proper scoring rules were shown to be useful not only to evaluate predicted probabilities but also to help in training better forecasters \cite{winkler1969scoring}.
% In addition to machine learning evaluation and to the seminal works in meteorology, 
Proper scoring rules and their ability to induce useful and accurate forecasts also lend themselves to game-theoretic interpretations, as discussed in the seminal work of \citet{savage1971}.

Before diving into details, let us introduce the notation. In a multiclass classification task with $K$ classes, let the true class of an instance be a vector $\dot{\mathbf{y}}=[y_1,\ldots,y_K]$, where $y_j = 1$ when the true class is $j$, otherwise $y_j = 0$. Additionally, let $\mathbf{s}=[s_1,\ldots,s_K]$ be a class probability vector obtained from a classification model for an instance, i.e. $s_j \geq 0$, $j=1,\ldots,K$ and $\sum^K_{j=1} s_j = 1$. A scoring rule $\phi(\mathbf{s}, \dot{\mathbf{y}})$ is a non-negative measure of how well the estimated probability vector $\mathbf{s}$ matches the true class vector $\mathbf{\dot{y}}$. We assume that lower values of $\phi(\mathbf{s}, \dot{\mathbf{y}})$ are better.% 
\footnote{Some authors \cite{winkler1969scoring,gneiting2007} use scoring rules in the opposite way, i.e. higher is better, sometimes calling them utility or payoff functions, in the sense that a forecaster is rewarded for giving better predictions. If a scoring rule was proposed as a payoff function, we can typically negate its values such that lower values are better.} 

Popular scoring rules include Brier score $\phi_{\text{BS}}$ and log-loss $\phi_{\text{LL}}$, which are defined as follows:
%
\begin{equation}
    \label{eq:evaluation:brier}
    \phi_{\text{BS}}(\mathbf{s}, \mathbf{\dot{y}})  = \sum_{j=1}^{K} (s_j - y_j)^2.
\end{equation}

  \begin{equation}
    \label{eq:evaluation:logloss}
    \phi_{\text{LL}}(\mathbf{s}, \mathbf{\dot{y}}) = - \sum_{j=1}^{K} y_j \log s_j.
\end{equation}
%
Our Brier score definition ranges between $0$ and $2$, agreeing with Brier's original definition \cite{brier1950}, although it is now common for half this quantity to be called Brier score. While scoring rules evaluate the loss incurred by the class probability estimates for a single instance, we are usually interested in evaluating the performance of a model on test data. Thus, given a test dataset, we can calculate the empirical loss as the average instance-wise loss across the data. % Going back to our example from Table \ref{tab:evaluation:toy}, we have 



% \begin{align*}
%     \bar{\phi}_{\text{BS}} &= \frac{1}{30}\sum_{i=1}^{30} \sum_{j=1}^{3} (p_{ij} - y_{ij})^2, \\ &= \frac{1}{30}\left[(1 -1)^2 + (0 - 0)^2 + (0 - 0)^2 + \ldots  + (0.3 - 0)^2 + (0.7 - 1)^2\right], \\ &= XXX,
% \end{align*}

% \noindent and

% \begin{align*}
%     \bar{\phi}_{\text{LL}} &= -\frac{1}{30}\sum_{i=1}^{30} \sum_{j=1}^{3} y_{ij} \log p_{ij}, \\ &= -\frac{1}{30}\left(1\log 1 + 0\log 0 + 0\log 0 + \ldots + 0\log 0 + 0\log 0.3 + 1\log 0.7\right), \\ &= XXX.
% \end{align*}

Suppose the class labels $\mathbf{\dot{y}}$ are drawn from the true distribution $\mathbf{q}$ over classes. A scoring rule $\phi$ is proper if its expected value on probability vector $\mathbf{s}$ and $\mathbf{\dot{y}}$ is higher than (i.e., worse) or the same as its expected value on $\mathbf{q}$ and $\mathbf{\dot{y}}$, that is if

% In this section we cover loss measures ($\breve{\phi}$) that prefer Bayes-optimal classifiers over other classifiers, i.e. for any given $P(\mathbf{X}, Y)$, $\mathbf{x} \in \mathcal{X}$, the following is satisfied:

\begin{align*}
\mathsf{E}_{\mathbf{\dot{y}} \sim \mathbf{q}} \Big[ \phi\big(\mathbf{s}, \mathbf{\dot{y}}\big)  \Big] \geq \mathsf{E}_{\mathbf{\dot{y}} \sim \mathbf{q}} \Big[ \phi\big(\mathbf{q}, \mathbf{\dot{y}}\big)  \Big], 
\end{align*}
and it is strictly proper if and only if both sides of the expression being equal implies $\mathbf{s} = \mathbf{q}$. % and $P(Y \mid \mathbf{X}=\mathbf{x})$ is a vector with elements $P(Y=j \mid \mathbf{X}=\mathbf{x})$.
Both Brier score and log-loss are strictly proper scoring rules.
     
%  Proper scoring rules are calculated as expectations over probability distributions, while ECE measures are averages across bins. If proper scoring rules are approximated empirically, they can be interpreted as putting each item in its separate bin, which would look like the example in Figure \ref{fig:rel4}, then computing the average of some loss for each predicted probability and its corresponding observed label. Instead of the absolute difference, as in ECE, this loss can be the quadratic error or the Kullback–Leibler divergence, which have better mathematical properties. The best-known proper scoring rules include Brier score and log-loss, which are given by Equations (\ref{eq:evaluation:brier}) and (\ref{eq:evaluation:logloss}), respectively, where $\mathbb{I}(\cdot)$ is an indicator function, such that $\mathbb{I}(y_n=j) = 1$, if $y_n=j$, otherwise $\mathbb{I}(y_n=j) = 0$.
    
    % \begin{figure}
    %     \centering
    %     \includegraphics[width=0.7\textwidth]{figures/evaluation/Forecaster4.png}
    %     \caption{Binary reliability diagram with one bin per instance.}
    %     \label{fig:eval:forecaster4}
    % \end{figure}
    


    % \begin{equation}
    %     \label{eq:evaluation:brier}
    %     \breve{\phi}_{\text{BS}}\Big(\mathbf{Q}, \mathbf{y}\Big)  = \frac{1}{N}\sum_{n=1}^{N}\sum_{j=1}^{K} \Big(\mathbb{I}(y_n=j) - q_{n,j} \Big)^2.
    % \end{equation}
    
    %   \begin{equation}
    %     \label{eq:evaluation:logloss}
    %     \breve{\phi}_{\text{LL}}\Big(\mathbf{Q}, \mathbf{y}\Big) = -\frac{1}{N}\sum_{n=1}^{N} \sum_{j=1}^{K} \mathbb{I}(y_n=j) \cdot \text{log} (q_{n,j}).
    % \end{equation}
    
% TSF proposed text
%    Among proper scoring rules, log-loss in particular is frequently used as the training loss of machine learning methods such as neural networks, often under the name of cross-entropy. At the instance level, log-loss only depends on the predicted class probability for the true class (as all other classes $y_j$ are zero) and it might not be obvious why it is a proper scoring function. However, properness is defined as an expectation over a population. For instance, suppose that, for a population of instances, the true probability is $[0.8, 0.2, 0.0]$. In this case, the expected log-loss will be $-(0.8 \log(s_1) + 0.2 \log(s_2))$, which can only be minimised by predicting the probability vector $[0.8, 0.2, 0.0]$, satisfying the properness condition.
    
% MPN merged TSF and MK and PF feedback
Among proper scoring rules, log-loss in particular is frequently used as the training loss of machine learning methods such as neural networks, often under the name of cross-entropy. \newtext{It is also the loss function used by most of the calibration methods discussed in Section \ref{sec:calibrators}, including Platt scaling, temperature scaling and its variations (vector and matrix), beta calibration and Dirichlet calibration. A notable exception is isotonic calibration, which optimised Brier score.}

At the instance level, log-loss only depends on the predicted class probability for the true class (as all other classes $y_j$ are zero) and it might not be obvious why it is a proper scoring function.
For example, one could argue that it does not matter whether the model predicts $[0.8, 0.2, 0.0]$ or $[0.8, 0.1, 0.1]$ on an instance of class $1$, as log-loss would be $-\ln(0.8)$ in both cases.
However, one needs to keep in mind that properness is defined as an expectation over a population. 
For instance, suppose that, for a population of instances, the true probability is $[0.8, 0.2, 0.0]$.
In this case, the expected log-loss will be $-(0.8 \log(s_1) + 0.2 \log(s_2))$, which can only be minimised by predicting the probability vector $[0.8, 0.2, 0.0]$, satisfying the properness condition.
Note that log-loss can be dominated by cases where the true class is predicted with low probability: in the extreme case of a single instance with zero probability for the true class the loss is infinite. 

    %, as it only penalises the probability given to the true class, which can be useful if one is only interested in maximising the probability given to the true class of an instance.
   %Log-loss only depends on the predicted class probability for the true class (as all other $y_j$ are zero) and it might not be obvious why it is a proper scoring function. %, i.e. why this loss has a unique minimum achieved by the Bayes-optimal model. 
   %For example, one could argue that it does not matter whether the model would predict $[0.7,0.1,0.1,0.1]$ or $[0.7,0.3,0.0,0.0]$ on an instance of class $1$, as log-loss would be $-\ln(0.7)$ in both cases. However, one needs to keep in mind that at the time of making the prediction the model does not know the true class of the instance and has no way of knowing which of the values in the predicted probability vector will be `probed' by the loss and will thus eventually matter. Therefore, the model should only predict $[0.7,0.3,0.0,0.0]$ when it is absolutely sure that the instance cannot belong to classes 3 and 4, because otherwise the evaluation on test set might catch it with an infinite loss of $-\ln(0)$ with a predicted probability $0$ for the true class $3$ or $4$.

    % We can easily see that Brier score and log-loss are not minimised by constantly predicting the class distribution, as in ECE. In fact, if a classifier predicts $0.5$ positive probability for two different instances, one positive and another negative, Equations (\ref{eq:evaluation:brier}) and (\ref{eq:evaluation:logloss}) result in $\breve{\phi}_{\text{BS}}\Big(\mathbf{Q}, \mathbf{y}\Big) = 0.5$ and $\breve{\phi}_{\text{LL}}\Big(\mathbf{Q}, \mathbf{y}\Big) = 0.6931$, respectively.
        
    
  
    
    


\subsection{Decompositions of proper scoring rules}\label{sec:decomp}

When proposing the forecast evaluation that would later be known as Brier score, Brier mentioned that it could not be ``gamed'', i.e. in order to obtain low scores, the forecaster has to produce honest, useful and correct predictions. Later research focused on why this was true for Brier score and other proper scoring rules.

\citet{sanders1963} showed that Brier score corresponds to the sum of two aspects of probability evaluation: validity and sharpness, terms introduced by \citet{miller1962statistical} and \citet{bross1953design}, respectively. Validity, later known as reliability \cite{murphy1977reliability}, is now often called \emph{calibration loss} \cite{kull2015novel}. It refers to the fit between the forecasts and the frequency of occurrence of the event, which means that it is a joint property of the predictions and the events. Sharpness, which is now commonly called \emph{refinement loss} and was also known as resolution \cite{murphy1977reliability}, is the loss due to predicting the same probability for instances from different classes.
% and is a property of predicted probabilities only. 
\citet{degroot1983} %comparison}
showed that these two terms make up proper scoring rules in general, and that probabilistic predictions should minimise refinement loss subject to calibration.

We now formally introduce such proper scoring rule decompositions. Let $\mathbf{X}$ and $\mathbf{\dot{Y}}=[Y_1,\ldots,Y_K]$ be multivariate random variables, respectively corresponding to the features and the class of a randomly picked instance, where $Y_j=1$ if the instance is of class $j$, otherwise $Y_j= 0$, for $j=1,2,\ldots,k$. Given a scoring classifier, class probability estimator or probability forecaster $\mathsf{f}$, we denote by $\mathbf{S}=[S_1,S_2,...,S_k]=\mathsf{f}(\mathbf{X})$ the vector output of $\mathsf{f}$ for random feature $\mathbf{X}$, where $\mathbf{S}$ is a random vector due to its dependence on $\mathbf{X}$. The expected value of proper scoring rule $\phi$ with respect to $\mathbf{S}$ and $\mathbf{\dot{Y}}$ is then $\mathsf{E} \Big[ \phi\big(\mathbf{S}, \mathbf{\dot{Y}}\big)  \Big]$.

\begin{table}[h]
\centering
\begin{tabular}{cccccc}
\hline
\textbf{$i$} & \textbf{$X^{(i)}$} & \textbf{$Y^{(i)}$} & $Q^{(i)}$         & $S^{(i)}$       & $C^{(i)}$          \\ \hline
$1$          & $(3,1,3)$          & $(1,0,0)$          & $(0.75,0.25,0.0)$ & $(0.9,0.1,0.0)$ & $(0.75,0.25,0.0)$  \\
$2$          & $(3,1,3)$          & $(1,0,0)$          & $(0.75,0.25,0.0)$ & $(0.9,0.1,0.0)$ & $(0.75,0.25,0.0)$  \\
$3$          & $(3,1,3)$          & $(1,0,0)$          & $(0.75,0.25,0.0)$ & $(0.9,0.1,0.0)$ & $(0.75,0.25,0.0)$  \\
$4$          & $(3,1,3)$          & $(0,1,0)$          & $(0.75,0.25,0.0)$ & $(0.9,0.1,0.0)$ & $(0.75,0.25,0.0)$  \\
$5$          & $(2,2,2)$          & $(1,0,0)$          & $(0.50,0.50,0.0)$ & $(0.6,0.2,0.2)$ & $(0.17,0.50,0.33)$ \\
$6$          & $(2,2,2)$          & $(0,1,0)$          & $(0.50,0.50,0.0)$ & $(0.6,0.2,0.2)$ & $(0.17,0.50,0.33)$ \\
$7$          & $(0,2,2)$          & $(0,1,0)$          & $(0.0,0.50,0.50)$ & $(0.6,0.2,0.2)$ & $(0.17,0.50,0.33)$ \\
$8$          & $(0,2,2)$          & $(0,1,0)$          & $(0.0,0.50,0.50)$ & $(0.6,0.2,0.2)$ & $(0.17,0.50,0.33)$ \\
$9$          & $(0,2,2)$          & $(0,0,1)$          & $(0.0,0.50,0.50)$ & $(0.6,0.2,0.2)$ & $(0.17,0.50,0.33)$ \\
$10$         & $(0,2,2)$          & $(0,0,1)$          & $(0.0,0.50,0.50)$ & $(0.6,0.2,0.2)$ & $(0.17,0.50,0.33)$ \\ \hline
\end{tabular}
        \caption{Example dataset with three classes and three features. Column $Q^{(i)}$ shows class posteriors given by the optimal model with $Q_1 = 0.25X_1$, $Q_2 = 0.25X_2$ and $Q_3 = 1 - (Q_1 + Q_2)$. Column $S^{(i)}$ corresponds to estimated class posteriors $S=f(X)$, which are given by $S_1 = 0.3X_3$, $S_2 = 0.1X_2$ and $S_3 = 1 - (S_1 + S_2)$. Finally, column $C$ represents calibrated probabilities.
        %calculated with $X|Y_1 \sim \mathcal{N}(4.375,1)$, $X|Y_2 \sim \mathcal{N}(1.875,2)$ and $X|Y_3 \sim \mathcal{N}(0,1)$. The class posteriors $S=f(X)$ are estimated by a trained model $f$ with $X|Y_1 \sim \mathcal{N}(4.5,1)$, $X|Y_2 \sim \mathcal{N}(3,1)$ and $X|Y_3 \sim \mathcal{N}(0.5,1)$. For the optimal model, the class priors are $\pi_1 = 4/10$,  $\pi_2 = 4/10$ and  $\pi_3 = 2/10$, while for model $f$, $\pi_1 = \pi_2 = \pi_3 = 1/3$, i.e. the classes are considered equally probable. Column $C$ represents calibrated probabilities.
        }
        \label{tab:evaluation:toy:psr}
\end{table}

Consider a classification test set of $10$ instances belonging to three classes ($K=3$) and described by $3$ features, as shown in column $\mathbf{X}^{(i)}$ of Table \ref{tab:evaluation:toy:psr}. Suppose instances  $1$, $2$, $3$ and $5$ belong to class $1$, i.e. $Y_1=1$, instances $4$, $6$, $7$, $8$ belong to class $2$ and the rest belong to class $3$. Note that in this example, the optimal class posteriors $\mathbf{Q}^{(i)}$ are given, however this is not generally the case. Additionally, the sample is representative by design, with average $\mathbf{Y}^{(i)}$, among instances with the same feature values, exactly agreeing with $\mathbf{Q}^{(i)}$. Given columns $\mathbf{S}^{(i)}$ and $\mathbf{Y}^{(i)}$ from Table \ref{tab:evaluation:toy:psr}, and using Equations (\ref{eq:evaluation:brier}) and (\ref{eq:evaluation:logloss}), by averaging over the 10 instances, we get a mean Brier score of $0.71$ and mean log-loss of $1.12$.

% \begin{align*}
%     \bar{\phi}_{\text{BS}} &= \frac{1}{10}\sum_{i=1}^{10} \sum_{j=1}^{3} (p_{ij} - y_{ij})^2, \\ &= \frac{1}{10}\left[(1 -0.9)^2 + (0 - 0.1)^2 + (0 - 0)^2 + \ldots  + (0.3 - 0)^2 + (0.7 - 1)^2\right], \\ &= XXX,
% \end{align*}

% \noindent and

% \begin{align*}
%     \bar{\phi}_{\text{LL}} &= -\frac{1}{10}\sum_{i=1}^{10} \sum_{j=1}^{3} y_{ij} \log p_{ij}, \\ &= -\frac{1}{30}\left(1\log 1 + 0\log 0 + 0\log 0 + \ldots + 0\log 0 + 0\log 0.3 + 1\log 0.7\right), \\ &= XXX.
% \end{align*}


% \todo[inline]{Meelis Kull: I think it is better to first state that suppose Q is given. Because then C can be calculated from it. Otherwise it is not clear how the expectation of E[Y|S] has been obtained. Note that by a lucky chance (well,.. by our design) the average Y exactly agrees with Q, i.e. Y are a representative sample.  This makes average[Y|S]=average[Q|S], which does not have to be the case in general. So somehow we need to be a bit careful to distinguish what is a coincidence here and what is exactly equal always. One possibility is to make the data generating process to pick lines from this table uniformly randomly, but not sure it is the best way to explain.}
Now let $\mathbf{C}=[C_1,C_2,\ldots,C_K]$ be yet another random vector, where $C_j=\mathsf{E}[Y_j| \mathbf{S}]$, i.e. $C_j$ represents the actual proportion of class $j$ given all instances which received the same estimate $\mathbf{S}$ from model $\mathsf{f}$. The decomposition of proper scoring rule $\phi$ into calibration loss and refinement loss is then the sum of expected loss between $\mathbf{S}$ and $\mathbf{C}$ and expected loss between $\mathbf{C}$ and $\mathbf{Y}$ \cite{brocker2007,kull2015novel}:
\begin{align*}
    \mathsf{E} \Big[ \mathsf{d}\big(\mathbf{S}, \mathbf{\dot{Y}}\big)  \Big] = \mathsf{E} \Big[ \mathsf{d}\big(\mathbf{S}, \mathbf{C}\big)\Big] + \mathsf{E} \Big[ \mathsf{d}\big(\mathbf{C}, \mathbf{\dot{Y}}\big)  \Big],
\end{align*}

\noindent where $\mathsf{d}: \mathbb{P}_{\mathbb{Y}} \times \mathbb{P}_{\mathbb{Y}} \rightarrow \mathbb{R}$ is the divergence associated to proper scoring rule $\phi$. For log-loss and Brier score, $\mathsf{d}$ has been shown to correspond to the Kullback-Leibler divergence and the mean squared difference, respectively \cite{kull2015novel}.

The definition above is given based on expected population loss. In practice, we would be calculating these quantities on test data, as we generally do not have access to the whole population. Thus, we actually calculate an empirical loss. But assuming that test data is representative of the whole population and that there is a uniform distribution over the test instances and zero probability elsewhere, empirical loss can be interpreted as a special case of expected loss and all decompositions derived for expected loss also apply to empirical loss \cite{kull2015novel}. 

In our example in Table \ref{tab:evaluation:toy:psr}, the first four instances share the same model scores $\mathbf{S}=[0.9,0.1,0.0]$, with the first three instances belonging to class $1$ and the fourth to class $2$. Thus, for these instances, $\mathbf{C}=[0.75,0.25,0.0]$. The other six instances also share a score vector, with $1$ instance from class $1$, three from class $2$ and 2 instances from class $3$. As a result, they share the same calibrated probabilities $\mathbf{C}=[1/6, 3/6, 2/6]$. Given these values and considering Brier score, calibration loss is $0.19$ and refinement loss is $0.52$, which sum up to the Brier score of $0.71$, as expected. For log-loss the decomposition is $1.12 = 0.29 + 0.83$.

% {\color{red}(TODO: Calculate using toy example.)}

It is easy to see that a function that maps $\mathbf{S}$ to $\mathbf{C}$, known as a calibrator in Section \ref{sec:calibrators}, could potentially reduce calibration loss to $0$, consequently decreasing proper scoring rule loss. Refinement loss, on the other hand, is only zero if there are no ties between instances of different classes, i.e. they do not share the same value for $\mathbf{S}$. If that is the case, it is possible to map $\mathbf{S}$ to $\mathbf{C}$ such that it is perfectly confident and correct, i.e. $C_j = Y_j$.

Now suppose we knew the optimal model that outputs the true posterior class probabilities $\mathbf{Q}=[Q_1,Q_2,\ldots,Q_K]$, where $Q_j=\mathsf{E}[Y_j|\mathbf{X}]$, i.e. $Q_j$ is the true proportion of class $j$ among instances with feature values $\mathbf{X}$. Then the expected loss according to proper scoring rule $\phi$ can be decomposed into the sum of expected divergences between $\mathbf{S}$ and $\mathbf{Q}$ and $\mathbf{Q}$ and $\mathbf{Y}$:

\begin{align*}
    \mathsf{E} \Big[ \mathsf{d}\big(\mathbf{S}, \mathbf{\dot{Y}}\big)  \Big] = \mathsf{E} \Big[ \mathsf{d}\big(\mathbf{S}, \mathbf{Q}\big)\Big] + \mathsf{E} \Big[ \mathsf{d}\big(\mathbf{Q}, \mathbf{\dot{Y}}\big)  \Big],
\end{align*}
The first term in the sum is called epistemic loss \cite{senge2014reliable} and is the loss due to our model $\mathsf{f}(\mathbf{X})$ not being optimal. The second term is called irreducible or aleatoric loss \cite{senge2014reliable} and is the loss of the optimal model. Going back to the example in Table \ref{tab:evaluation:toy:psr}, for Brier score, epistemic loss is $0.26$ and irreducible loss is $0.45$. For log-loss the decomposition is $1.12 = 0.48 + 0.64$. The irreducible loss is only zero if the attributes of every instance $\mathbf{X}$ carry enough information to uniquely define the label $\mathbf{\dot{Y}}$. It is thus not possible to come up with a procedure to reduce the overall loss based on it. Additionally it would be unrealistic to do so based on epistemic loss. We are then naturally drawn to calibration loss as it is simple to interpret (we want our predicted probabilities of occurrence of an event to match the actual frequencies of occurrence) and also because we can easily estimate it with enough data. Thus, as discussed in the following section, visualisation and estimation of miscalibration have received considerable attention in the literature of probability evaluation and machine learning.


% {\color{red}(TODO: Connect to reliability diagrams (depends on the section's position).)}


% {\color{red}(TODO: Epistemic-irreducible.)}
%Other decompositions and why they're important


%  Let us once again return to our example from Table \ref{tab:evaluation:toy}. As mentioned before, a model that always outputs the class proportion will have a perfect ECE of 0, and that is what happens if we take class 1 as the positive class and constantly predict class probabilities equal to the class proportions. But while this gives $\text{binary-ECE}=0$ for class 1, the resulting log-loss is $0.6365$.
% % 
%  On the other hand, a different model which always outputs $0.9$ probability to the instances' true classes gets the reliability diagram shown in Figure \ref{fig:eval:reliability0.9}, with $\text{binary-ECE}=0.1$ for class 1, and $0.1054$ log-loss.
% %
% From the first to the second model, ECE increases (0 to 0.1), but log-loss decreases (0.6365 to 0.1054). This happens because proper scoring rules do not measure only calibration. In fact, they can be decomposed into terms with distinct interpretations \cite{kull2015}. 




%     \begin{figure}
%         \centering
%         \includegraphics[width=0.7\textwidth]{figures/evaluation/reliability-0.9-v2.pdf}
%         \caption{Binary reliability diagram of a model that always outputs $0.9$ probability for the true class of the instances in Table \ref{tab:evaluation:toy}.}
%         \label{fig:eval:reliability0.9}
%     \end{figure}



% An intuitive way to decompose proper scoring rules is into refinement (RL) and calibration losses (CL): $\mathsf{E}\left[\breve{\phi}\right] = \text{RL} + \text{CL}$. Refinement loss is the loss due to producing the same probability for instances from different classes (the second model reduces this loss), while calibration loss is the loss due to the difference between
% the probabilities predicted by the model and the observed class proportions among instances with the same output (the second model increases this loss).

% Since we don't usually know the real score distribution, we would need to once again rely on binning if we wanted to actually estimate refinement and calibration losses. Additionally, the terms are calculated (estimated) differently, depending on the proper scoring rule. Finally, the loss of the optimal classifier is not necessarily 0. This is due to irreducible loss, which is only 0 if the attributes provide enough information to uniquely determine the instances' right label Y, with probability 1 \cite{kull2015}.


%\subsection{Calibration metrics}
%    \subsubsection{First attempts to evaluate calibration}
%    \subsubsection{Binary}
%    \subsubsection{ECE}


\newpage

\section{Evaluation and visualisation of classifier calibration}
\label{sec:metrics}

In this section we present a range of approaches to evaluate and visualise calibration, and discuss the advantages and disadvantages of each.
In Section \ref{sec:met:1st} we explore the first steps towards measuring miscalibration, starting from the early work on weather forecast calibration, and discuss various approaches to visually inspect miscalibration.
Some of those early approaches have been later adapted and proposed as new calibration metrics which are discussed in the following sections.
We start with binary calibration in Section \ref{sec:met:bin} which will serve as a building block for the two multiclass calibration measures discussed in Sections \ref{sec:met:clw:ece} and \ref{sec:met:con:ece}.
% We finish this section discussing hypothesis tests for calibration in Section \ref{sec:met:hyp}.



%----------------------------------------------------%
%\subsection{First attempts to evaluate calibration}
\subsection{Visualising calibration}
\label{sec:met:1st}
%----------------------------------------------------%

% Calibration metrics and proper scoring rules can provide evidence of the quality of a model's calibration.
Several visualisation techniques have been proposed for easier inspection of the reliability of predictions at different score ranges.
In this section we summarise a range of approaches that have been proposed in the literature, from simple tabular inspection to the more recent reliability diagrams (see \citet{brocker2007} for an extended discussion of reliability diagrams).

Starting from the binary case, the basic idea has been to show the relation between a particular predicted score $\hat{s} \in [0, 1]$ for the positive class of a probabilistic classifier and the respective observed proportion of positives, which we denote by $\mathsf{\bar{y}}(\hat{s})$.
In order to compute a observed proportion of positives we require multiple samples with the same score $\hat{s}$. However, given that the scores are continuous variables, the probability of getting multiple samples with the same score is almost zero.
For that reason, the score space is commonly discretised into $M$ bins $\{\mathbb{B}_1, \dots, \mathbb{B}_M\}$, thus increasing the probability of having multiple samples per estimation range (perhaps by forcing each bin to have a minimum number of samples).
Then, we can obtain $M$ observed proportions of positives $\mathsf{\bar{y}}(\mathbb{B}_m)$ instead of one per score value $\hat{s}$.
% If we have an indicator variable for every bin with the indices of the scores that fall into it $\mathbb{I}_m \in \{i; \hat{s}_i \in \mathbb{B}_m\}$ we can compute the \emph{observed proportion of positives} in each bin as
% %
% \begin{equation}
%     \mathsf{\bar{y}}(\mathbb{B}_m) = \frac{\sum_{i \in \mathbb{I}_m} y_i}{\text{count}(\mathbb{I}_m)}.
% \end{equation}
% %
% Some of the first uses of \emph{observed proportion of positives} appeared in the context of weather forecast evaluation in the form of tabular data \cite{hallenbeck1920, brier1950}.
%\citet{hallenbeck1920} showed ten equally distributed bin boundaries with their respective number of forecasts, number of rains and percentage (See Figure \ref{tab:eval:hallenbeck1920:1}). 
See Table \ref{tab:eval:hallenbeck1920} for an early use of observed proportions of positives using equal-width bins of predicted probabilities. 

\begin{figure}
    % \begin{subfigure}{0.48\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{figures/evaluation/hallenbeck1920_tab1}
    %     \caption{Hallenbeck 1920}
    %     \label{tab:eval:hallenbeck1920:1}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}{0.48\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{figures/evaluation/brier1950_tab2}
    %     \caption{Brier 1950}
    %     \label{tab:eval:brier1950:2}
    % \end{subfigure}
    
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{sanders1963_fig1}
        \caption{\citep[Fig.~1]{sanders1963}}
        \label{fig:eval:sanders1963:1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{lichtenstein1976_fig6.jpg}
        \caption{\citep[Fig.~2]{lichtenstein1977calibration}}
        \label{fig:eval:lichtenstein1977:6}
    \end{subfigure}
    
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{brocker_2007_fig1}
        \caption{\citep[Fig.~1]{brocker2007}}
        \label{fig:eval:brocker2007:1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{brocker_2007_fig4}
        \caption{\citep[Fig.~4]{brocker2007}}
        \label{fig:eval:brocker2007:4}
    \end{subfigure}
    \caption{Different graphical representations of calibration-related information found in the literature.}
    \label{fig:eval:rd}
\end{figure}
    
Later work showed line plots instead of tabular data, with markers at the centre of each bin~\cite{sanders1963, lichtenstein1977calibration, lichtenstein1982, murphy1977reliability}; occasionally including the number of samples in each bin next to the markers (See Figure \ref{fig:eval:sanders1963:1}). Other authors showed the markers with size relative to the sample size~\cite{hagedorn2005}, or as a separate histogram next to the reliability diagram~\cite{niculescu-mizil2005}.
Line plots facilitate visual inspection of the discrepancy of the observed proportions of positives against a perfectly calibrated model, which corresponds to the diagonal.
However, positioning the markers at the centre of the bins can be misleading, as even perfectly calibrated scores may result in a \emph{visually} non-calibrated reliability diagram with a deviation of up to half the bin width from the diagonal~\cite{brocker2007} (See Figure \ref{fig:mean:vs:centre} for an example).
This may happen in cases in which the scores are not evenly distributed in each bin.
%
\begin{figure}
    \centering
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=1.0\linewidth]{rd_mean_score_vs_bin_centre_not_calibrated.pdf}
        \caption{Not calibrated example. $4$ samples with score $0$ from which $25\%$ are positive, and $4$ samples with score $1$ from which $75\%$ are positive.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=1.0\linewidth]{rd_mean_score_vs_bin_centre_calibrated.pdf}
        \caption{Calibrated example. $1$ sample with score $0$ from negative class, and $1$ sample with score $1$ from positive class.}
    \end{subfigure}
    \caption{
Simple example showing the maximum discrepancy in calibration error when using the centre of the bin for the marker instead of the average score of the bin. Both examples show only two bins $[0, 0.5)$ and $[0.5, 1]$.
\textbf{(a)} shows a model not calibrated, but using the centre of the bin (green dashed line) visually seems calibrated. The gap between the centre of the bin and the average score is maximum, which corresponds to half of the bin size with respect to the average score (red line).
\textbf{(b)} shows a calibrated model which seems uncalibrated if using the centre of the bin. The gap is again half of the bin size.
}
    \label{fig:mean:vs:centre}
\end{figure}
%
In order to alleviate this problem, later work centred the markers on the average predicted scores $\mathsf{\bar{s}}(\mathbb{B}_m)$ in each bin instead. % where
% %
% \begin{equation}
%     \mathsf{\bar{s}}(\mathbb{B}_m) = \frac{\sum_{i \in \mathbb{I}_m}\hat{s_i}}{\text{count}(\mathbb{I}_m)}.
% \end{equation}
% %

There are two main methods to group the predicted scores into bins to build reliability diagrams. The first one, commonly called \emph{width binning}, distributes scores into a number of  bins of the same width, choosing bin edges accordingly (e.g., 10 bins $[0, 0.1], (0.1, 0.2], \ldots, $ $(0.9, 1.0]$). Another method, called \emph{frequency binning} (also equal size or equal mass binning) groups the scores by keeping the same number of samples in each bin. Frequency binning can and will normally result in bins with different widths, but it ensures that all bins have the same ``weight'' when assessing the model's miscalibration.

Bin estimations have varying reliability, e.g., depending on the number of samples in the bin. 
One way to show this visually is by incorporating confidence intervals.
%If previous work showed the counts in text form (eg. in a table or next to the markers \cite{brier1950, sanders1963, murphy1977reliability}), later work also incorporated in the visualisation confidence intervals in the reliability diagram.
One of the simplest methods is to assume that each bin is sampled from a binomial distribution, and compute the corresponding confidence intervals of the observed proportion of positives (see Figure~\ref{fig:eval:pycalib:lines}).
However, making the assumption of fixed bins, score averages and proportion of positives is unrealistic; unless the score distribution is uniform (see \cite{brocker2007} for a detailed discussion).
More accurate intervals can be obtained by using the \emph{consistency resampling} method proposed by \citet{brocker2007}, which consists on sampling the scores with replacement several times in order to obtain multiple surrogate forecasts and observations and their respective quantiles.

More recently, binary reliability diagrams have been extended to the multiclass setting.
One method to show multiclass scores in a binary fashion consists in plotting only the \emph{confidence} of the model for each sample (the highest score among all possible classes). 
% and consider a positive prediction if the predicted class is correct, and negative otherwise.
%.showing only the highest score per sample and its corresponding class as the positive; which could still be  a wrong or right prediction.
This approach was already used for binary classification by
\citet{lichtenstein1977calibration}, reproduced here as Figure \ref{fig:eval:lichtenstein1977:6}. 
The figure shows a binary reliability diagram with scores in the range $[0.5,1]$
(with $K$ classes the confidence is never lower than $1/K$).
% and refers back to the work of \citet{Hazard1973}. {\color{red}(TODO: I can not find the pdf of Hazard1973, may need to check it.)}
% The specific score of the winning class is commonly referred as the \emph{confidence} value of the prediction.
%
Another example of the use of confidences in multiclass problems is the recent work of \citet{guo2017}, which shows the confidence for multiclass problems in the form of bar plots and the ECE and MCE metrics discussed below. 
% (which in this work we refer as confidence ECE and MCE).
%In this case, bins with probabilities lower than $1/K$ are always empty, where $K$ is the number of classes.
% \citet{guo2017} also show the deviations from the diagonal as red bars, which is a good way to highlight the mis-calibration but could be somewhat misleading as the area of such bars is not informative.
% Showing bars instead of lines is helpful to visually inspect the miscalibration, however, it is difficult to compare multiple models.
%
Finally, instead of collapsing all classes into a single diagram one could construct one reliability diagram per class as line plots or bars in a one-vs-rest manner \cite{kull2019} (see Figure \ref{fig:eval:pycalib:ter}).

\begin{figure}
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{pycalib_rd_bars.pdf}
        \caption{Reliability diagram with bars for each bin and red error gaps with regards to a perfectly calibrated model, and a histogram of the scores at the bottom.}
        \label{fig:eval:pycalib:bars}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{pycalib_rd_lines.pdf}
        \caption{Comparison of multiple calibration methods, with Clopper–Pearson binomial confidence intervals of 95\% in each observed proportion of positives.}
        \label{fig:eval:pycalib:lines}
    \end{subfigure}
    
    \begin{subfigure}{1.0\linewidth}
        \centering
        \includegraphics[width=\linewidth]{pycalib_rd_ternary.pdf}
        \caption{Multiple classes can be shown as one-vs-rest reliability diagrams.}
        \label{fig:eval:pycalib:ter}
    \end{subfigure}
    \caption{Examples of reliability diagrams using the Python library PyCalib}
    \label{fig:eval:pycal}
\end{figure}

%It is often also useful to show the number of samples in each bin in the form of a histogram next (or below) the reliability diagram in the form of a small histogram at the bottom of the reliability diagram, sharing the x-axis (as seen in {\color{red}[add references]}).\todo{MPN: fix}
%
%{\color{blue}
%MPN: We possibly need to reference the reliability diagram analysis of \cite{vaicenavicius2019evaluating} and their proposed one. And mention \cite{brocker2007} as the original idea? \cite{brocker2007} indicates that \cite{wilks2011statistical} has a great explanation of reliability diagrams.
%}
%

% All the following text in blue are notes
%\cite{Hallenbeck1920} shows a table with 10 bins and the number of rains, forecasts and actual percentage \ref{tab:eval:hallenbeck1920:1}
%
%\cite{brier1950} already used reliability diagrams in form of a table as it was enough to show 5 bins with their corresponding observed proportion of rain cases \ref{tab:eval:brier1950:2}
%
%\cite{sanders1963} is one of the first articles that show a reliability diagram depicting forecast probabilities agains observed relative frequencty of occurrence. However, the forecast probabilities always fall into a one decimal point, including zero and one (11 bins). Other figures show what it seems to be 21 bins but the first and last bins are empty.
%{\color{red} Need to understand what is the range of every bin, given that the boundaries may contain a smaller bin width.}. 
%The author also included the number of forecasts in every bin. Find out what are the numbers on the right y-axis in \ref{fig:eval:sanders1963:1}. Altough a reliability diagram is first presented, the rest of the article chooses to show departure from expectancy vs observed departure of relative frequency of occurrence \ref{fig:eval:sanders1963:2}.

%----------------------------------------------------%
% \subsection{Expected/Maximum calibration error}
%----------------------------------------------------%
    % \begin{itemize}
    %     \item As seen in the previous Section, each notion of calibration is related to a reliability diagram
    %     \begin{itemize}
    %         \item This can be used to visualise miscalibration on binned scores
    %     \end{itemize}
    %     \item We will now see how these bins can be used to measure miscalibration
    % \end{itemize}


    % \begin{itemize}
    %     \item We start by introducing a toy example:
    % \end{itemize}
    
    \begin{table}[!b]
        \begin{tabular}{lrrrr}
            \toprule
            {id} &  $\hat{s}_1$ &  $\hat{s}_2$ &  $\hat{s}_3$ &  $y$ \\
            \midrule
            1  &     1.0 &     0.0 &     0.0 &    1 \\
            2  &     0.9 &     0.1 &     0.0 &    1 \\
            3  &     0.8 &     0.1 &     0.1 &    1 \\
            4  &     0.7 &     0.1 &     0.2 &    1 \\
            5  &     0.6 &     0.3 &     0.1 &    1 \\
            6  &     0.4 &     0.1 &     0.5 &    1 \\
            7  &     1/3 &     1/3 &     1/3 &    1 \\
            8  &     1/3 &     1/3 &     1/3 &    1 \\
            9  &     0.2 &     0.4 &     0.4 &    1 \\
            10 &     0.1 &     0.5 &     0.4 &    1 \\
            \bottomrule
        \end{tabular}
        \hfill
        \begin{tabular}{lrrrr}
            \toprule
            {id} &  $\hat{s}_1$ &  $\hat{s}_2$ &  $\hat{s}_3$ &  $y$ \\
            \midrule
            11 &          0.8 &          0.2 &          0.0 &    2 \\
            12 &          0.7 &          0.0 &          0.3 &    2 \\
            13 &          0.5 &          0.2 &          0.3 &    2 \\
            14 &          0.4 &          0.4 &          0.2 &    2 \\
            15 &          0.4 &          0.2 &          0.4 &    2 \\
            16 &          0.3 &          0.4 &          0.3 &    2 \\
            17 &          0.2 &          0.3 &          0.5 &    2 \\
            18 &          0.1 &          0.6 &          0.3 &    2 \\
            19 &          0.1 &          0.3 &          0.6 &    2 \\
            20 &          0.0 &          0.2 &          0.8 &    2 \\
            \bottomrule
        \end{tabular}
        \hfill
        \begin{tabular}{lrrrr}
            \toprule
            {id} &  $\hat{s}_1$ &  $\hat{s}_2$ &  $\hat{s}_3$ &  $y$ \\
            \midrule
            21 &          0.8 &          0.2 &          0.0 &    3 \\
            22 &          0.8 &          0.1 &          0.1 &    3 \\
            23 &          0.8 &          0.0 &          0.2 &    3 \\
            24 &          0.6 &          0.0 &          0.4 &    3 \\
            25 &          0.3 &          0.0 &          0.7 &    3 \\
            26 &          0.2 &          0.6 &          0.2 &    3 \\
            27 &          0.2 &          0.4 &          0.4 &    3 \\
            28 &          0.0 &          0.4 &          0.6 &    3 \\
            29 &          0.0 &          0.3 &          0.7 &    3 \\
            30 &          0.0 &          0.3 &          0.7 &    3 \\
            \bottomrule
        \end{tabular}
        \caption{Class probabilities given by a classifier to 30 instances belonging to three different classes.}
        \label{tab:evaluation:toy}
    \end{table}

%----------------------------------------------------%
\subsection{Evaluating calibration error: the binary case}
\label{sec:met:bin}
%----------------------------------------------------%

% We define the binary \textit{estimated calibration error} \citep{roelofs2021mitigating}, also commonly called \textit{expected calibration error}, or binary-ECE \citep{naeini2015}, as the average gap across all bins in a reliability diagram, weighted by the number of instances in each bin, as given by Equation (\ref{eq:binaryECE}).


% In the past, most of the research on the calibration of probabilities has focused on binary classification problems. However, more recently multiclass calibration has got some attention and new metrics and visualisation tools have been proposed.
We now proceed with discussing how to measure calibration error. 
We will use the three-class toy problem in Table \ref{tab:evaluation:toy} throughout. 
In this section we convert it to a binary classification problem by taking class 1 as positive and classes 2 and 3 as negative. 
We then apply equal-width binning to the class 1 probabilities. 
% in order to separate class 1 probabilities and their corresponding labels into 5 bins, corresponding to intervals $[0, 0.2]$, $(0.2, 0.4]$, $(0.4, 0.6]$, $(0.6, 0.8]$, and $(0.8, 1.0]$. 
Table \ref{tab:evaluation:binary:bins} shows the resulting bins $\mathbb{B}_m$, $m \in \{1, \ldots, 5\}$, from which we calculate the number of instances in the bin denoted as $|\mathbb{B}_{m}|$, the average probability $\Bar{\mathsf{s}}(\mathbb{B}_{m})$, the proportion of positives $\Bar{\mathsf{y}}(\mathbb{B}_{m})$, and the absolute gap between them $|\Bar{\mathsf{y}}(\mathbb{B}_m) - \Bar{\mathsf{s}}(\mathbb{B}_m)|$. 


        \begin{table}[!b]
            \centering
            \small
            \begin{tabular}{lrllllc}
                \toprule
                 $\mathbb{B}_m$ &  $|\mathbb{B}_{m}|$ &  $\mathsf{s}(\mathbb{B}_{m})$ & $\Bar{\mathsf{s}}(\mathbb{B}_{m})$ & $\mathsf{y}(\mathbb{B}_{m})$                             & $\Bar{\mathsf{y}}(\mathbb{B}_{m})$ & $|\Bar{\mathsf{y}}(\mathbb{B}_m) - \Bar{\mathsf{s}}(\mathbb{B}_m)|$ \\
                \midrule
                 %$\mathbb{B}_1$ &         11 &  0.0, 0.0, 0.0, 0.0, 0.1, 0.1, 0.1,  \ldots &           0.10 &  0 (9), 1 (2) &             0.18 & 0.08\\
                 $\mathbb{B}_1$ &         11 &  $0.0^{(4)}$, $0.1^{(3)}$,  $0.2^{(4)}$ &           0.10 &  $0^{(9)}$, $1^{(2)}$ &             $0.18$ & 0.08\\
                 $\mathbb{B}_2$ &          7 &              $0.3^{(2)}$, $1/3^{(2)}$, $0.4^{(3)}$ &            0.35 &              $0^{(4)}$, $1^{(3)}$ &              0.43 & 0.08\\
                 %$\mathbb{B}_3$ &          3 &                                    0.5, 0.6, 0.6 &            0.57 &                          0 (2), 1 (1) &              $0.\arc{33}$ & 0.24\\
                 $\mathbb{B}_3$ &          3 &                                    0.5, 0.6, 0.6 &            0.57 &                          0, 0, 1 &              $0.33$ & 0.24\\
                 $\mathbb{B}_4$ &          7 &                $0.7^{(2)}$, $0.8^{(5)}$ &            0.77 &              $0^{(5)}$, $1^{(2)}$ &              0.29 & 0.48 \\
                 %$\mathbb{B}_5$ &          2 &                                         0.9, 1.0 &            0.95 &                             1 (2) &              1.00 & 0.05\\
                 $\mathbb{B}_5$ &          2 &                                         0.9, 1.0 &            0.95 &                             1, 1 &              1.00 & 0.05\\
                \bottomrule
            \end{tabular}
            
        \caption{Positive probabilities and corresponding instance labels separated into 5 bins. The probabilities were obtained by taking class 1 as the positive class in the multiclass problem in Table \ref{tab:evaluation:toy}. To reduce the width of the table, a number followed by a superscript parenthesis $X^{(Y)}$ indicates a list of number $X$ repeated $Y$ times.}
        \label{tab:evaluation:binary:bins}
    \end{table}
    
The values of $\Bar{\mathsf{p}}(\mathbb{B}_{m})$, $\Bar{\mathsf{y}}(\mathbb{B}_{m})$ and $|\Bar{\mathsf{y}}(\mathbb{B}_m) - \Bar{\mathsf{s}}(\mathbb{B}_m)|$ in Table \ref{tab:evaluation:binary:bins} can be used to draw the reliability diagram shown in Figure \ref{fig:eval:rel_diagram}, where we can see the red bars representing the calibration error at each bin.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.7\textwidth]{binary-reliability-v2.pdf}
    \caption{Reliability diagram corresponding to the 5 bins presented in Table \ref{tab:evaluation:binary:bins}.}
    \label{fig:eval:rel_diagram}
\end{figure}

Given the information about the bins in Table \ref{tab:evaluation:binary:bins} we could calculate an average of the bin-wise calibration error, which leads us to  binary estimated calibration error, as defined in  Definition \ref{def:binary:ece}.
%
\begin{definition}[Binary-ECE]
\label{def:binary:ece}
Binary \textit{estimated calibration error} \citep{roelofs2021mitigating}, or binary-ECE \citep{naeini2015}, is the average gap across all bins in a reliability diagram, weighted by the number of instances in each bin:
$$\mathsf{ECE}_{\text{binary}}  = \sum_{m=1}^M \frac{|\mathbb{B}_{m}|}{N} |\Bar{\mathsf{y}}(\mathbb{B}_{m}) - \Bar{\mathsf{s}}(\mathbb{B}_{m})|,$$
where $M$ and $N$ are the number of bins and instances, respectively. 
% $\mathbb{B}_{m}$ is the $m$-th probability bin, $|\mathbb{B}_{m}|$ denotes the size of the bin, and $\Bar{\mathsf{s}}(\mathbb{B}_{m})$ and $\Bar{\mathsf{y}}(\mathbb{B}_{m})$ are the average predicted probability and the proportion of positives in bin $\mathbb{B}_{m}$. 
Binary-ECE is also commonly called binary \textit{expected calibration error}, however this quantity is empirically estimated on a validation or test sample, which is why we prefer to call it binary \textit{estimated calibration error}.
\end{definition}
%
Binary-ECE aggregates part of the visual information about calibration error in Figure  \ref{fig:eval:rel_diagram} by taking the weighted mean of the sizes of these gaps. In this example, $\mathsf{ECE}_{\text{binary}} =0.1873$. 

Binary-ECE ranges from $0$ to $1$, with particular values including $\mathsf{ECE}_{\text{binary}} =\pi_1$ (proportion of positives) for a classifier that randomly outputs probability $1$ for one of the classes, $\mathsf{ECE}_{\text{binary}} =0$ for a perfect classifier that always predicts probability $1$ for the correct class or for a classifier that constantly outputs positive probability equal to $\pi_1$, and $\mathsf{ECE}_{\text{binary}} =1$ for a classifier that always assigns probability $1$ to the wrong class.

% \begin{equation}
% \label{eq:binaryECE}
%     \text{binary-ECE}  = \sum_{i=1}^M \frac{|B_{i}|}{N} |\Bar{y}(B_{i}) - \Bar{p}(B_{i})|,
% \end{equation}

% \noindent where $M$ and $N$ are the number of bins and instances, respectively, $B_{i}$ is the $i$-th probability bin, $|B_{i}|$ denotes the size of the bin, and $\Bar{p}(B_{i})$ and $\Bar{y}(B_{i})$ are the average predicted probability and the proportion of positives in bin $B_{i}$.

Instead of measuring how miscalibrated the model is on average, one might be interested in the worst case, in other words ``how maximally miscalibrated is the model''? In this case, one might use the binary maximum calibration error \citep{naeini2015}.
%
\begin{definition}[Binary-MCE]
\label{def:binary:mce}
Binary maximum calibration error (binary-MCE) is the maximum gap across all bins in a reliability diagram: $$\mathsf{MCE}_{\text{binary}} = \max_{m \in \{1, \ldots, M\}} |\Bar{\mathsf{y}}(\mathbb{B}_m) - \Bar{\mathsf{s}}(\mathbb{B}_m)|.$$
\end{definition}
%
In our example, Table \ref{tab:evaluation:binary:bins} and Figure \ref{fig:eval:rel_diagram} show that the fourth bin has the largest gap, with its size corresponding to $\mathsf{MCE}_{\text{binary}} = 0.48$. 

Binary-MCE can be very sensitive to bins with few instances, where the values of $\Bar{\mathsf{y}}(\mathbb{B}_m)$ and $\Bar{\mathsf{s}}(\mathbb{B}_m)$ are calculated based on very little information. In extreme cases with only a single instance in a bin, $\Bar{\mathsf{y}}(\mathbb{B}_m)$ will be the instance's actual label (1 or 0), potentially resulting in a large gap that would have a small weight in binary-ECE, while being the whole value of binary-MCE, meaning that the model would be evaluated based on its performance for a single instance.

% We can similarly define the maximum calibration error (binary-MCE) as the maximum gap across all bins in a reliability diagram, or

% \begin{equation}
% \label{eq:binaryMCE}
%     \text{binary-MCE} = \max_{i \in \{1, \ldots, M\}} |\Bar{y}(B_i) - \Bar{p}(B_i)|.
% \end{equation}


%----------------------------------------------------%
\subsection{Classwise calibration error}
\label{sec:met:clw:ece}
%----------------------------------------------------%

We now proceed to settings with more than two classes and start by defining the estimated calibration error corresponding to a single class $j$ in a multiclass task.

\begin{definition}[Class-$j$-ECE]
\label{def:class:j:ece}
Given a multiclass task with $K$ classes, class-$j$-ECE corresponds to the binary-ECE calculated by taking class $j$ as positive and the other $K-1$ classes together as a new negative class:
$$\mathsf{ECE}_{j}  = \sum_{m=1}^M \frac{|\mathbb{B}_{m,j}|}{N} |\Bar{\mathsf{y}}_j(\mathbb{B}_{m,j}) - \Bar{\mathsf{s}}_j(\mathbb{B}_{m,j})|,$$
where $\mathbb{B}_{m,j}$ is the $m$-th bin of class $j$.
\end{definition}

Once again we turn to our example in Table \ref{tab:evaluation:toy}. Following Definition \ref{def:class:j:ece}, we have already calculated class-$1$-ECE ($0.1873$) in our binary-ECE example. Now we need to calculate class-$2$-ECE and class-$3$-ECE. Tables \ref{tab:evaluation:binary2:bins} and \ref{tab:evaluation:binary3:bins} show the binary bins for classes $2$ and $3$, respectively, while the binary reliability diagrams of the three classes can be seen in Figure \ref{fig:eval:clas_rel_diagram}.

%\begin{table}[!b]
%    \centering
%    \small
%    \begin{tabular}{lrllllc}
%        \toprule
%         $\mathbb{B}_{m,2}$ &  $|\mathbb{B}_{m,2}|$ &                                              & $\Bar{\mathsf{s}}(\mathbb{B}_{m,2})$ &                                          & $\Bar{\mathsf{y}}(\mathbb{B}_{m,2})$ & $|\Bar{\mathsf{y}}(\mathbb{B}_m) - \Bar{\mathsf{s}}(\mathbb{B}_m)|$  \\
%        \midrule
%         $\mathbb{B}_{1,2}$ &         15 &  0.0$\times$(5), 0.1$\times$(5), 0.2$\times$(5) &           0.10 &  0$\times$(10), 1$\times$(5) &             0.33 & 0.23\\
%         $\mathbb{B}_{2,2}$ &         12 &  0.3$\times$(5), 1/3$\times$(2),  0.4$\times$(5) &           0.35 &           0$\times$(8), 1$\times$(4) &             0.33 & 0.02\\
%         $\mathbb{B}_{3,2}$ &          3 &                                    0.5, 0.6, 0.6 &            0.57 &                                      0, 0, 1 &              0.33 & 0.24\\
%         $\mathbb{B}_{4,2}$ &          0 &                                                  &             &                                              &             \\
%         $\mathbb{B}_{5,2}$ &          0 &                                                  &             &                                              &             \\
%        \bottomrule
%    \end{tabular}
%    \caption{Positive probabilities and corresponding instance labels separated into 5 bins. The probabilities were obtained by taking class 2 as the positive class in the multiclass problem in Table \ref{tab:evaluation:toy}.}
%        \label{tab:evaluation:binary2:bins}
%\end{table}

\begin{table}[!b]
    \setlength{\tabcolsep}{5pt}
    \centering
    \small
    \begin{tabular}{lrllllc}
        \toprule
         $\mathbb{B}_{m,2}$ &
         $|\mathbb{B}_{m,2}|$ &
         $\mathsf{s}(\mathbb{B}_{m,2})$&
         $\Bar{\mathsf{s}}(\mathbb{B}_{m,2})$&
         $\mathsf{y}(\mathbb{B}_{m,2})$ &
         $\Bar{\mathsf{y}}(\mathbb{B}_{m,2})$ &
         {\footnotesize $|\Bar{\mathsf{y}}(\mathbb{B}_m) - \Bar{\mathsf{s}}(\mathbb{B}_m)|$}  \\
        \midrule
         $\mathbb{B}_{1,2}$ &         15 &  $0^{(5)}$, $0.1^{(5)}$, $0.2^{(5)}$ &           0.10 &  $0^{(10)}$, $1^{(5)}$ &             0.33 & 0.23\\
         $\mathbb{B}_{2,2}$ &         12 &  $0.3^{(5)}$, $1/3^{(2)}$,  $0.4^{(5)}$ &           0.35 &           $0^{(8)}$, $1^{(4)}$ &             0.33 & 0.02\\
         $\mathbb{B}_{3,2}$ &          3 &                                    0.5, 0.6, 0.6 &            0.57 &                                      0, 0, 1 &              0.33 & 0.24\\
         $\mathbb{B}_{4,2}$ &          0 &                                                  &             &                                              &             \\
         $\mathbb{B}_{5,2}$ &          0 &                                                  &             &                                              &             \\
        \bottomrule
    \end{tabular}
    \caption{Positive probabilities and corresponding instance labels separated into 5 bins. The probabilities were obtained by taking class 2 as the positive class in the multiclass problem in Table \ref{tab:evaluation:toy}.}
        \label{tab:evaluation:binary2:bins}
\end{table}

\begin{table}[ht]
    \setlength{\tabcolsep}{5pt}
    \centering
    \small
    \begin{tabular}{lrllllc}
        \toprule
         $\mathbb{B}_{m,3}$ & 
         $|\mathbb{B}_{m,3}|$ &
         $\mathsf{s}(\mathbb{B}_{m,3})$ &
         $\Bar{\mathsf{s}}(\mathbb{B}_{m,3})$ &
         $\mathsf{y}(\mathbb{B}_{m,3})$ &
         $\Bar{\mathsf{y}}(\mathbb{B}_{m,3})$ &
         {\footnotesize
         $|\Bar{y}(\mathbb{B}_m) - \Bar{p}(\mathbb{B}_m)|$}\\
        \midrule
         $\mathbb{B}_{1,3}$ &         11 &  $0.0^{(4)}$, $0.1^{(3)}$, $0.2^{(4)}$ &           0.10 &  $0^{(7)}$, $1^{(4)}$ &             0.36 & 0.26\\
         $\mathbb{B}_{2,3}$ &         11 &  $0.3^{(4)}$, $1/3^{(2)}$, $0.4^{(5)}$ &           0.35 &  $0^{(9)}$, $1^{(2)}$ &             0.18 & 0.17\\
         $\mathbb{B}_{3,3}$ &          4 &                               0.5, 0.5, 0.6, 0.6 &            0.55 &                       0, 0, 0, 1 &              0.25 & 0.3\\
         $\mathbb{B}_{4,3}$ &          4 &                               0.7, 0.7, 0.7, 0.8 &            0.72 &                       0, 1, 1, 1 &              0.75 & 0.03\\
         $\mathbb{B}_{5,3}$ &          0 &                                                  &             &                                  &             \\
        \bottomrule
    \end{tabular}
    \caption{Positive probabilities and corresponding instance labels separated into 5 bins. The probabilities were obtained by taking class 3 as the positive class in the multiclass problem in Table \ref{tab:evaluation:toy}.}
        \label{tab:evaluation:binary3:bins}
\end{table}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth,trim=0 0 0 0, clip]{classwise-reliability-v2.pdf}
    \caption{Binary reliability diagram of each class in our running example. Note the empty bins in the second and third reliability diagrams, showing that the classifier never outputs high probabilities for these classes.}
    \label{fig:eval:clas_rel_diagram}
\end{figure}

\noindent From the values in Tables \ref{tab:evaluation:binary2:bins} and \ref{tab:evaluation:binary3:bins} and following Definition \ref{def:class:j:ece}, we get $\text{class-$2$-ECE} = 0.147$ and $\text{class-$3$-ECE} = 0.2017$. 

We can now define classwise-ECE \cite{kull2019}. 
%
\begin{definition}[Classwise-ECE]
\label{def:classwise:ece}
The estimated classwise calibration error (classwise-ECE) is the average class-$j$-ECE across all classes:
$$\mathsf{ECE}_{\text{classwise}}  = \frac{1}{K}\sum_{j=1}^K \mathsf{ECE}_{j}.$$
\end{definition}
%
According to Definition \ref{def:classwise:ece}, in our example $\text{classwise-ECE} = (0.1873 + 0.147 + 0.2017)/3 = 0.1787$.

% Confidence-ECE only cares about the calibration error associated with the winning class. In order to measure miscalibration for all classes, we can take the average binary-ECE across all classes, which gives the expected classwise calibration error (classwise-ECE) \cite{kull2019}. Formally, classwise-ECE is defined as the average gap across all classwise reliability diagrams, weighted by the number of instances in each bin, as shown in Equation (\ref{eq:classwiseECE}).

% \begin{equation}
%     \label{eq:classwiseECE}
%     \text{classwise-ECE}  = \frac{1}{K}\sum_{j=1}^K \sum_{i=1}^M \frac{|B_{i,j}|}{N} |\Bar{y}_j(B_{i,j}) - \Bar{p}_j(B_{i,j})|,
% \end{equation}

% \noindent where $B_{i,j}$ is the $i$-th bin of the $j$-th class, $|B_{i,j}|$ denotes the size of the bin, and  $\Bar{p}_j(B_{i,j})$ and $\Bar{y}_j(B_{i,j})$ denote the average prediction of class $j$ probability and the actual proportion of class $j$ in the bin $B_{i,j}$. The contribution of a single class $j$ to classwise-ECE is called class-$j$-ECE.

\begin{definition}[Classwise-MCE]
\label{def:classwise:mce}
The maximum classwise calibration error (classwise-MCE) \cite{kull2019} is defined as the maximum gap across all bins and all classwise-reliability diagrams:
$$
    \mathsf{MCE}_{\text{classwise}}  = \max_{j \in \{1, \ldots, K\}\, m \in \{1, \ldots, M\}}  |\Bar{\mathsf{y}}_j(B_{m,j}) - \Bar{\mathsf{s}}_j(B_{m,j})|.
$$
\end{definition}
%
% Equation (\ref{eq:classwiseMCE}) presents the maximum classwise calibration error (classwise-MCE), which is defined as the maximum gap across all bins and all classwise-reliability diagrams.
%
% \begin{equation}
%     \label{eq:classwiseMCE}
%     \text{classwise-MCE}  = \max_{j \in \{1, \ldots, K\}\, i \in \{1, \ldots, M\}}  |\Bar{y}_j(B_{i,j}) - \Bar{p}_j(B_{i,j})|.
% \end{equation}
%
In our running example, $\mathsf{MCE}_{\text{classwise}} = 0.48$. 

Note that this is not the only way to define classwise-MCE. For example, one could be interested in the average maximum gap across classes, i.e. an average class-$j$-MCE, which in our example would be $(0.48 + 0.24 + 0.3)/3 = 0.34$. As another variation, one could take the maximum class-$j$-ECE, which would then indicate the most miscalibrated class on average. In our example, this variation corresponds to class-$3$-ECE ($0.2017$).





% \begin{figure}
%     \centering
%     \includegraphics[width=0.7\textwidth]{figures/evaluation/perfect-reliability.png}
%     \caption{Reliability diagram of a classifier that predicts the  overall class distribution ($0.5$ in this case). The corresponding binary-ECE here is zero.}
%     \label{fig:eval:optim_ece}
% \end{figure}

Although classwise-ECE and MCE measure calibration error over all classes, they do not take into account the miscalibration that arises from every possible relationship between classes. For a true multiclass-ECE, we could bin the probability vectors in simplex space and then calculate the gaps between the average probability vector and the vector of class proportions in each bin. Although this seems like the right thing to do when evaluating multiclass calibration, it might not be efficiently computable with large numbers of classes, as the number of bins can be prohibitively high and most bins would likely be empty.

Similarly to binary-ECE, a value of $\text{classwise-ECE} = 0$ can be obtained by a classifier that constantly outputs the class proportions. For example, if a classifier always predicts $1/3$ setosa, $1/3$ versicolor and $1/3$ virginica for Fisher's Iris dataset, the resulting classwise-ECE will be $0$.
% Another limitation of all ECE/MCE measures is that optimising them can be as simple as predicting the overall class distribution, regardless of the given instance, as shown in Figure \ref{fig:eval:optim_ece}.



%----------------------------------------------------%
\subsection{Confidence calibration error}
\label{sec:met:con:ece}
%----------------------------------------------------%

As already mentioned, some calibration measures only consider a model's confidence, defined as
the maximum value in the predicted probability vector, i.e. the probability given to the winning class. Prediction confidence is not a new idea and has been around since at least the 1970s. \citet{lichtenstein1977calibration} called it the half-range method in the binary case (referred to as ``two alternatives'' in the paper) and it was also mentioned as one of the variations of the multiclass task, which the authors called ``three or more alternatives''. 
More recently it has been popularised by \citet{guo2017}.
    
    To calculate confidence-ECE, we first bin the confidence values and, for each instance of each bin, we produce a binary value indicating if the classifier predicted correctly or not.
    Recalling the example from Table \ref{tab:evaluation:toy}, the resulting confidence bins are presented in Table \ref{tab:evaluation:confidence:bins}, where $\Bar{\mathsf{p}}(\mathbb{B}_{m})$ and $\mathsf{acc}(\mathbb{B}_{m})$ are respectively the average confidence and prediction accuracy in bin $\mathbb{B}_{m}$, with the corresponding reliability diagram in Figure \ref{fig:eval:rel_diagram2}.
    Note that bin $\mathbb{B}_1$ is empty, which demonstrates that confidence-ECE and confidence reliability diagrams are different from binary-ECE even on two-class problems. 
        
        \begin{table}[ht]
        \centering
        \small
        \begin{tabular}{lrllllc}
            \toprule
             $\mathbb{B}_m$ &
             $|\mathbb{B}_{m}|$ &
             $\mathsf{s}(\mathbb{B}_{m})$ &
             $\Bar{\mathsf{s}}(\mathbb{B}_{m})$ &
             $\mathsf{y}(\mathbb{B}_{m})$ &
             $\mathsf{acc}(\mathbb{B}_{m})$ &
             $|\mathsf{acc}(\mathbb{B}_m) - \Bar{\mathsf{p}}(\mathbb{B}_m)|$ \\
            \midrule
             $\mathbb{B}_1$ &          0 &                                                  &             &                                  &             \\
             $\mathbb{B}_2$ &          7 &              $1/3^{(2)}$, $0.4^{(5)}$ &            0.38 &              $0^{(4)}$, $1^{(3)}$ &              0.43 & 0.05\\
             $\mathbb{B}_3$ &         10 &  $0.5^{(4)}$, $0.6^{(6)}$ &           0.56 &     $0^{(7)}$, $1^{(3)}$ &             0.30 & 0.26\\
             $\mathbb{B}_4$ &         11 &  $0.7^{(5)}$, $0.8^{(6)}$ &           0.75 &  $0^{(6)}$, $1^{(5)}$ &             0.45 & 0.3\\
             $\mathbb{B}_5$ &          2 &                                         0.9, 1.0 &            0.95 &                             1, 1 &              1.00 & 0.05\\
            \bottomrule
        \end{tabular}\caption{Confidence bins corresponding to the toy example from Table \ref{tab:evaluation:toy}. The binary values in the fifth column indicate if the classifier correctly classified each instance. }
        \label{tab:evaluation:confidence:bins}
        \end{table}
        
   

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.7\textwidth]{confidence-reliability-v2.pdf}
    \caption{Confidence reliability diagram corresponding to the bins in Table \ref{tab:evaluation:confidence:bins}.}
    \label{fig:eval:rel_diagram2}
\end{figure}

\begin{definition}[Confidence-ECE]
    \label{def:confidence:ece}
    Confidence-ECE is the average difference between accuracy and average confidence across all bins in a confidence reliability diagram, weighted by the number of instances in each bin: $$\mathsf{ECE}_{\text{confidence}}  = \sum_{m=1}^M \frac{|\mathbb{B}_{m}|}{N} |\mathsf{acc}(\mathbb{B}_{m}) - \Bar{\mathsf{p}}(\mathbb{B}_{m})|.$$
    \end{definition}
    %
    We then calculate confidence-ECE as the weighted mean of the gaps between average confidence and prediction accuracy at each bin, thus $\mathsf{ECE}_{\text{confidence}}=0.2117$, while the maximum confidence calibration error (confidence-MCE) corresponds to the largest gap, i.e. $\mathsf{MCE}_{\text{confidence}}=0.3$. As with binary-ECE and for the same reasons, confidence-MCE is very sensitive to small bins, but in this particular example, its value corresponds to the gap of the largest bin.
    


%\todo{TSF: please add concluding paragraph}

As we show in Section \ref{sec:calibrators}, there is a wide range of post-hoc calibration techniques in the literature, each one capable of handling different miscalibration patterns. Thus, it can be useful to first analyse a model's reliability diagram, as it allows us to diagnose model miscalibration, i.e. in what probability ranges it is underconfident or overconfident, and this can help choose an appropriate calibration method. In addition, any of the ECE measures discussed in this Section  can be used to decide if a classifier actually needs to be calibrated, by testing the hypothesis that the model is already calibrated, as shown in Section \ref{sec:hyp}. \newtext{Finally, it is important to consider that all ECE/MCE measures can provide very different values given different number of bins, as shown in Figs. \ref{fig:hallenbeck-rel} and \ref{fig:hallenbeck2-rel}, and they can be minimised by predicting the overall class distribution, regardless of the given instance. Thus, it is good practice to use them together with the proper scoring rules presented in Section \ref{sec:psr}, to get a full evaluation of the probabilities produced by a model.}





%----------------------------------------------------%




==> 04_calibrators.tex <==
\section{Calibration methods}
\label{sec:calibrators}

In this section we provide a systematic review of standard approaches to calibrating classifiers through the construction of calibration maps.
In particular, we focus on post-hoc calibration methods for classification, which can be used to adjust probability outputs separately from the initial training process.
For each method, we cover the mathematical formulation, the objective function for learning the map, and the predictive function to calculate the class probabilities for a new instance.
We include a few test cases to empirically analyse each method, and discuss their advantages and disadvantages.
General guidance on each method's implementation is also discussed, addressing issues such as overfitting and computational effort.
At the end of the section, we briefly describe some related work to classifier calibration, such as methods that can improve the calibration level during training time, methods that are designed for getting well-calibrated probability for other predictive tasks, and approaches that are designed for specific tasks in areas such as computer vision and natural language processing. 

\subsection{Preliminaries}

We denote a calibration map as a function $\mathsf{g}: \mathbb{S}_{\mathbb{Y}} \rightarrow \mathbb{P}_{\mathbb{Y}}$. 
Here $\mathbb{Y} =\{1, \dots, K\}$ is the discrete space with $K$ classes of the target variable.
$\mathbb{P}_{\mathbb{Y}}$ denotes the probability vector space on $\mathbb{Y}$, that is: $\mathbb{P}_{\mathbb{Y}} = \{ [s_1, \dots, s_K] \mid s_j \geq 0, \sum_{j=1}^{K} s_j = 1\}$.  
$\mathbb{S}_{\mathbb{Y}}$ represents the original output space of the (uncalibrated) classifier, which can take various forms depending on the formalisation of the classifier.
For instance, for a typical probabilistic classifier, we have $\mathbb{S}_{\mathbb{Y}} = \mathbb{P}_{\mathbb{Y}}$.
A one-vs-rest SVM might produce $K$-dimensional vectors in $\mathbb{S}_{\mathbb{Y}} = \mathbb{R}^{K}$.
Deep neural networks can also provide unnormalised vector outputs before the softmax is performed at the final layer. 
Calibration maps that work with such vector spaces are referred to as scaling approaches.
The name suggests these approaches are used to scale the vector output into a probability output, which is quite useful for models like SVMs, as the hinge loss does not optimise probability estimates by default.
However, other than the name and historical motivation, in modern applications, probability calibrators and scaling approaches can be used interchangeably, as the probability space and vector space can be transformed into each other by using the link function (e.g. softmax) and inverse link function (e.g. logit transform ). 

In general, to obtain a calibration map, we will have a calibration set with uncalibrated probabilities and labels, denoted as $\mathbb{C} = \{(\mathbf{s}_1, y_1), \dots, (\mathbf{s}_N, y_N)\}$, and an objective function $\mathsf{L}(\mathbb{C})$ to optimise.
Typically, the objective function is constructed using proper scoring rules, that is, $\mathsf{L}(\mathbb{C}) = \sum_{i=1}^{N} \phi(\mathbf{s}_i, y_i)$, and it can be optimised via various gradient descent algorithms.


\newtext{
\textbf{Training Schemes}: While the above notation suggested that the calibration map can be obtained by fitting a calibrator on a given hold-out calibration set, in practice a small training set and calibration set might lead to over-fitting thus limiting the performance of the calibrated model.
A typical solution here is to introduce multi-fold dataset splits as introduced in \cite{platt99probabilisticoutputs}.
The author proposes to divide the training sets into three different folds and fit the model and calibration map in cross-validation.
Two folds are used to train the uncalibrated model, and the model predictions on the last fold are collected and used to fit the calibration map.
This training process thus ends up with three pairs of models and calibration maps.
At test time each instance will be predicted with all three pairs, and resulting probabilities are averaged to give the final estimate.
Alternatively, people have also used applied label smoothing \cite{muller2019does} to reduce the level of overfitting and over-confidence.
The idea is to have a weighted average between the original probability vector (either from the uncalibrated model or after a calibration method has been applied) and a uniform probability vector.
Therefore, the final probability vector will be pushed somewhat towards the uniform probability vector, which avoids overly high confidence for unsuitable cases.}


\subsection{Two-Class Test Cases}

We designed some test cases to illustrate each calibration map's characteristics empirically.
These test cases are designed with a known distribution and allow us to directly sample the instances.
For ease of understanding, we consider a scenario with a univariate feature ($ \mathbf{x} \in \mathbb{R}$), so that we can inspect the fitted functions and reliability diagrams by means of $x$-$y$ plots.

% \subsubsection*{Binary Test Cases}
Figure~\ref{fig:test_dataset} depicts the probability density functions for the synthetic two-class dataset, as well as the posterior class probabilities when predicting any new instances.
%The density functions are constructed with a mixture of Gaussian distributions, and the class prior is set to be equal to construct the joint dataset distribution.
The generative model is equally likely to produce a positive and a negative, and the distribution of the feature values are mixtures of two normal distributions within each class. 
% is a mixture of Gaussian distributions N(-4,960) and N(64,1280) for positives and a mixture of Gaussian distributions N(4,980) and N(-72,1024) for negatives. 
Denoting the mixture components as $H=1$ and $H=2$, our generative model can be formally written down as:
%
\begin{align*}
    Y &\sim \text{Bernoulli}(0.5) \\
    H &\sim \text{Bernoulli}(0.5) \\
    X \mid Y=1, H=1 &\sim \text{Gaussian}(-4, 960) \\
    X \mid Y=1, H=2 & \sim \text{Gaussian}(64, 1280) \\
    X \mid Y=2, H=1 & \sim \text{Gaussian}(4, 980) \\
    X \mid Y=2, H=2 & \sim \text{Gaussian}(-72, 1024) \\
\end{align*}


\begin{figure}[!tbp]
    \centering
    %\includegraphics[width=0.6\textwidth]{figures/calibrators/data_distribution.png}
    %\includegraphics[width=0.273\textwidth]{figures/calibrators/data_prediction.png}
    \includegraphics[width=0.61\textwidth, valign=t]{data_distribution.png}
    \includegraphics[width=0.33\textwidth, valign=t]{data_prediction.png}
    \caption{The synthetic dataset used in the test cases. The left two figures shows the data distribution for each class respectively. The figure on the right gives the Bayes-optimal posterior probability for class 1.}
    \label{fig:test_dataset}
\end{figure}

%\todo[inline]{MPN: I have modified the images in Figure \ref{fig:test_dataset}. Should I put the previous figures back?}

\noindent
This generative assumption allows us to approximate the `true' reliability diagram closely for every test case and provides better insights into each calibration map. Specifically, we generate a large number of random samples and use small bin sizes to approximate a smooth reliability diagram.

We consider three cases for binary classification, each of which may occur in practice. 
The first two cases are hypothetical over/under-confident scenarios using a logistic regression model of the form 
    $\hat{\mathsf{f}}(x) = (1 + \exp(-a\cdot x))^{-1}$.
Such a model puts the decision boundary at $x=0$, which is nearly Bayes-optimal for the synthetic data. 
The model confidence can be moderated with the parameter $a$, and we will use the following two cases: 
%
\begin{align*}
    \hat{\mathsf{f}}_{\text{under}}(x) = \frac{1}{1 + \exp(-0.01\cdot x)} \\
    \hat{\mathsf{f}}_{\text{over}}(x) = \frac{1}{1 + \exp(-0.05\cdot x)}
\end{align*}
%
The third case is obtained with an MLP classifier as implemented by the scikit-learn Python package.
The model is specified with a two layer structure with 128 hidden units per layer.
The activation is selected as the ReLU function.
The remaining settings are left at their default values.
$10,000$ instances are sampled to train the model.

The smoothed reliability diagrams for these three cases are shown in Figure~\ref{fig:binary_test_cases}.
In the under-confident case the output probabilities barely reach the outside of the interval $[0.1, 0.9]$.
The reliability diagram shows a higher slope compared with the perfectly calibrated  one (the diagonal).
In contrast, the over-confident case has a shallower slope around the middle compared with the diagonal.
It further causes the reliability diagram to have sharp transitions while approaching the extremes. 
For the MLP case, we can observe both under-confident and over-confident regions throughout the reliability diagram.
%As we have seen with the previous two test cases, before the 0.5 on the horizontal axis, if the reliability diagram falls below the diagonal, it indicates under-confident, and vice versa.
%After the 0.5 on the horizontal axis, having the reliability diagram above the diagonal becomes the sign of under-confident, and vice verse.
This specific MLP classifier tends to be under-confident around $s \in [0, 0.1]$ and $s \in [0.65, 1]$, and mostly over-confident elsewhere.

\begin{figure}[!tbp]
    \centering
    %\includegraphics[width=0.28\textwidth]{figures/calibrators/test_case_1.png}
    %\includegraphics[width=0.28\textwidth]{figures/calibrators/test_case_2.png}
    \includegraphics[width=0.3\textwidth, valign=t]{test_case_1.png}
    \includegraphics[width=0.3\textwidth, valign=t]{test_case_2.png}
    %\includegraphics[width=0.28\textwidth]{figures/calibrators/test_case_3.png}
    \includegraphics[width=0.3\textwidth, valign=t]{test_case_3.png}
    \caption{The reliability diagrams of the three uncalibrated classifiers. The left figure shows the $\hat{\mathsf{f}}_{\text{under}}$ case, where the classifier predicts a probability closer to 0.5 compared with the Bayes-optimal case (Fig.~\ref{fig:test_dataset}, right), resulting in a reliability diagram with steeper slope. The middle figure shows the $\hat{\mathsf{f}}_{\text{over}}$  case, where the predicted probabilities are pushed towards $0$ and $1$ respectively, resulting in a shallower reliability curve. The right figure is obtained with a MLP classifier ($\hat{\mathsf{f}}_{\text{MLP}}$), where the reliability diagram shows over-confident and under-confident predictions around different regions. 
    }
    \label{fig:binary_test_cases}
\end{figure}

%\todo[inline]{MPN: Decide if should increase the font size of all figures (I have changed Fig. 12 Test Case 1, 2 and 3 as an example).}

\subsection{Calibration for Binary Classification}

We start with methods that can learn calibration maps for binary problems.
In binary classification, probability estimates are scalars, so the calibration maps are functions mapping from $[0, 1]$ to $[0, 1]$.
Here we describe four widely applied methods in detail: empirical binning, isotonic regression, logistic calibration and Beta calibration.  
Other approaches will be be briefly mentioned at the end of this section.

\subsubsection*{Empirical Binning}

Empirical binning \newtext{\cite{zadrozny2001obtaining,naeini2015}} is one of the simplest methods to build a calibration map.
It directly connects to the previously introduced ECE measure, which evaluates the calibration level by calculating the empirical frequencies within a set of score intervals. 
Therefore, binning approaches can directly optimise a variant of ECE depending on how the binning scheme is selected.

\begin{figure}[!tbp]
    \centering
    \begin{subfigure}{\textwidth}
    \centering
    %\includegraphics[width=0.28\textwidth]{figures/calibrators/Case1_EMP10_prediction.png}
    \includegraphics[width=0.28\textwidth]{Case1_EMP10_calibration.png}
    \includegraphics[width=0.28\textwidth]{Case1_EMP10_reliability.png}
    \caption{Test case 1: under-confidence}
    \end{subfigure}
    
    
    \begin{subfigure}{\textwidth}
    \centering
    %\includegraphics[width=0.28\textwidth]{figures/calibrators/Case2_EMP10_prediction.png}
    \includegraphics[width=0.28\textwidth]{Case2_EMP10_calibration.png}
    \includegraphics[width=0.28\textwidth]{Case2_EMP10_reliability.png}
    \caption{Test case 2: over-confidence}
    \end{subfigure}
    
    \begin{subfigure}{\textwidth}
    \centering
    % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case3_EMP10_prediction.png}
    \includegraphics[width=0.28\textwidth]{Case3_EMP10_calibration.png}
    \includegraphics[width=0.28\textwidth]{Case3_EMP10_reliability.png}
    \caption{Test case 3: MLP classifier}
    \end{subfigure}
    
    \caption{Examples of empirical binning calibration with 10 equal-width bins. As the binning approach can only give discrete outputs, we can observe the probabilities after calibration are no longer continuous and are only presented with 10 values or less (the under-confidence case has fewer values as there are no observations in bins closer to the extremes. The reliability diagrams show that the calibration method works well with all three test case, with most points being close to the calibrated diagonal.  }
    \label{fig:test_emp10}
\end{figure}

% \begin{figure}[!tbp]
%     \centering
%     \begin{subfigure}{\textwidth}
%     \centering
%     %\includegraphics[width=0.28\textwidth]{figures/calibrators/Case1_EMP32_prediction.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/Case1_EMP32_calibration.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/Case1_EMP32_reliability.png}
%     \caption{Test case 1: under-confidence}
%     \end{subfigure}
    
    
%     \begin{subfigure}{\textwidth}
%     \centering
%     %\includegraphics[width=0.28\textwidth]{figures/calibrators/Case2_EMP32_prediction.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/Case2_EMP32_calibration.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/Case2_EMP32_reliability.png}
%     \caption{Test case 2: over-confidence}
%     \end{subfigure}
    
%     \begin{subfigure}{\textwidth}
%     \centering
%     % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case3_EMP32_prediction.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/Case3_EMP32_calibration.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/Case3_EMP32_reliability.png}
%     \caption{Test case 3: MLP classifier}
%     \end{subfigure}
    
%     \caption{Examples of empirical binning calibration with 32 equal-width bins. With a higher number of bins, the discrete probabilities appear to be denser, and the predictions fits the ground-truth better. On the other hand, as we have less samples within each bin, some bins might have a poorer estimates than the 10-bins case. This is more observable with the over-confidence case, where we have less observations around the middle region.}
%     \label{fig:test_emp32}
% \end{figure}

For a typical setting, the empirical binning approach comes with the following parameters. 
(1) Bins: $\{\mathbb{B}_1, \dots, \mathbb{B}_M \}$, where each bin $\mathbb{B}_m \subset [0, 1]$ is an interval of probability range, and $\cup_{m=1}^{M} \mathbb{B}_m = [0, 1]$.
(2) Probability estimates in the bins:  $\mathbf{a}=\{a_1,\dots,a_{M}\}$, where $a_m \in [0, 1]$ specifies the calibrated probability value in each bin.
We usually assume that these bins do not overlap with each other. 
To make a prediction based on an uncalibrated probability $s$, empirical binning uses the following functional form:
%
\begin{align}
% \mathsf{c}(p; B_1, \dots, B_M, \mathbf{a}) = \sum_{j=1}^{M} \mathbb{I}(p\in \mathbb{B}_j) \cdot a_j
\mathsf{g}(s; \mathbb{B}_1, \dots, \mathbb{B}_M, \mathbf{a}) = a_m \quad \quad \quad \text{if}\ s \in \mathbb{B}_m
\end{align}
%
Here $ s \in \mathbb{B}_m$ means that the uncalibrated probability $s$ falls within $\mathbb{B}_m$.

Fitting a binning calibration map can be done by optimising $\mathbf{a}$ using ECE as a loss function: 
%
\begin{align}
%\mathbb{L}(\mathbf{a}) = \sum_{j=1}^{M} \Big | \frac{\sum_{i=1}^{N} \mathbb{I}(p_i \in B_j) \cdot y_i}{|B_j|} - a_j \Big|
\mathbf{a}^* &
= \arg\min_{\mathbf{a}} \mathsf{L}(\mathbf{a}) \\
\mathsf{L}(\mathbf{a}) &= \mathsf{ECE}(\mathbf{a}) 
                       = \sum_{m=1}^{M} \Big | \bar{\mathsf{y}}(\mathbb{B}_m) - a_m \Big|
\end{align}
%
Here $\bar{\mathsf{y}}(\mathbb{B}_m)$ represents the empirical frequency within $\mathbb{B}_m$ as defined in the previous section.  
The equation hence indicates that we want to assign each $a_m$ according to the empirical frequency of the labels within each bin $\mathbb{B}_m$.

We empirically analyse the binning approach with a simple setting of $M=10$ equal-width bins.  
The results with the three test cases are shown in Figure~\ref{fig:test_emp10}.
The binning approach performs well on most points, as the reliability diagram are close to the diagonal  after calibration.
However, it should be noted that the output probabilities can only take $M$ different values.
Therefore, while the final probabilities are calibrated,  we can no longer distinguish instances that receive different predictions from the uncalibrated model.
In other words, binning approaches can reduce the calibration loss at the cost of a higher grouping loss \cite{kull2015novel}.
% According to the data points pictured at the bottom of the figure, we can see this poor performance is mainly caused by the lower amounts of data points around these regions.
% As the test case 2 is designed to be an over-confident example, predictions are more pushed towards either $0$ or $1$ depending on their actual classes, causing the regions around $0.2$ and $0.8$to be emptier than the rest, further causing the bin estimates to be worse for these regions. 

While here we illustrated the binning approach with equal-width bins, it is possible to use other binning schemes such as equal-frequency binning.
For example, \cite{naeini2015} propose a Bayesian binning approach.

To summarise, the main advantages of binning approaches are as follows:
(1) They can be used to directly minimise a specific variant of ECE, hence are useful when calibration loss is of primary concern.
(2) Training is reasonably fast and straightforward. 
(3) Given its non-parametric nature, it does not have any constraint on the form of the calibration maps and therefore can capture arbitrary shapes according to the given bins.
In addition, other binning strategies can also be applied to deal with different datasets and uncalibrated models. %such as equal-frequency binning and Bayesian binning \cite{naeini2015}.



\subsubsection*{Isotonic Calibration}

Calibration by means of isotonic regression is another widely used non-parametric approach \newtext{\cite{barlow1972isotonic,niculescu-mizil2005,naeini2016}}.
The isotonic approach was originally proposed to solve univariate regression tasks where the function were required to be monotonic.
In the case of probability calibration, if we assume the uncalibrated model has a monotonic reliability diagram, then isotonic regression is a suitable approach to achieve a better level of calibration. 

Isotonic regression achieves a monotonic fit by estimating a set of non-decreasing constant segments, corresponding to a set of bins of varying width.  
Isotonic regression can therefore be described with the following parameters:
(1) Bin boundaries: $\mathbf{b}=(b_1,\dots,b_M)$, $b_j \in [0, 1], b_j < b_{j+1}$, and  (2) Edge values:  $\mathbf{v}=(v_1,\dots,v_{M})$, $ v_j \in [0, 1], v_j \leq v_{j+1}$.
As indicated by the parameters, isotonic regression is quite close to an empirical binning approach.
The main difference is that instead of having a pre-defined set of bin edges, isotonic regression learns these bin boundaries from the data.
As a result, isotonic regression can have an variable number of bins depending on the training set.
To calibrate a probability $s$, isotonic regression uses the following predictive function: 
%
\begin{align}
%c(p; \mathbf{b}, \mathbf{v}) = & \frac{1}{\sum_{j=1}^{M-1} \mathbb{I}(p\geq b_j)\cdot\mathbb{I}(p\leq b_{j+1})} \\ \nonumber
%&\sum_{j=1}^{M-1} \mathbb{I}(p\geq b_j)\cdot\mathbb{I}(p<b_{j+1}) \cdot \Big(v_j + \frac{p-b_j}{b_{j+1}-b_j}(v_{j+1} - v_j)\Big) 
\mathsf{g}(s; \mathbf{b}, \mathbf{v}) = \sum_{m=1}^{M-1} \mathsf{I}(s\geq b_m)\cdot\mathsf{I}(s<b_{m+1}) \cdot m_j 
\end{align}
%

\begin{figure}[!tbp]
    \centering
    \begin{subfigure}{\textwidth}
    \centering
    %\includegraphics[width=0.28\textwidth]{figures/calibrators/Case1_ISO_L_prediction.png}
    \includegraphics[width=0.28\textwidth]{Case1_ISO_L_calibration.png}
    \includegraphics[width=0.28\textwidth]{Case1_ISO_L_reliability.png}
    \caption{Test case 1: under-confidence}
    \end{subfigure}
    
    
    \begin{subfigure}{\textwidth}
    \centering
    % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case2_ISO_L_prediction.png}
    \includegraphics[width=0.28\textwidth]{Case2_ISO_L_calibration.png}
    \includegraphics[width=0.28\textwidth]{Case2_ISO_L_reliability.png}
    \caption{Test case 2: over-confidence}
    \end{subfigure}
    
    \begin{subfigure}{\textwidth}
    \centering
    % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case3_ISO_L_prediction.png}
    \includegraphics[width=0.28\textwidth]{Case3_ISO_L_calibration.png}
    \includegraphics[width=0.28\textwidth]{Case3_ISO_L_reliability.png}
    \caption{Test case 3: MLP classifier}
    \end{subfigure}
    
    \caption{Examples of isotonic calibration trained with 10,000 samples. Compared with empirical binning, we can see the isotonic approach can provide a larger variety of outputs in the continuous interval of $[0, 1]$, and different bins can be automatically learnt according to the observations. The calibration method works reasonably well on all three test cases. The over-confidence case still has some errors around around the middle-left and middle-right boundaries, due to the lack of training points within these areas. }
    \label{fig:test_iso_L}
\end{figure}


% \begin{figure}[!tbp]
%     \centering
%     \begin{subfigure}{\textwidth}
%     \centering
%     % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case1_ISO_S_prediction.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/Case1_ISO_S_calibration.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/Case1_ISO_S_reliability.png}
%     \caption{Test case 1: under-confidence}
%     \end{subfigure}
    
    
%     \begin{subfigure}{\textwidth}
%     \centering
%     % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case2_ISO_S_prediction.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/Case2_ISO_S_calibration.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/Case2_ISO_S_reliability.png}
%     \caption{Test case 2: over-confidence}
%     \end{subfigure}
    
%     \begin{subfigure}{\textwidth}
%     \centering
%     % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case3_ISO_S_prediction.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/Case3_ISO_S_calibration.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/Case3_ISO_S_reliability.png}
%     \caption{Test case 3: MLP classifier}
%     \end{subfigure}
    
%     \caption{Examples of isotonic calibration trained with 1,000 samples. We can see from the reliability diagram that the calibration performance is significantly worse than the previous example with 10,000 samples. Being a non-parametric approach, the isotonic calibration is more suitable on larger datasets.}
%     \label{fig:test_iso_S}
% \end{figure}

The three test cases on istonic regression are shown in Figure~\ref{fig:test_iso_L}.
To compare with the empirical binning approach again, while in the empirical case we have a constant prediction within each bin, we can see the prediction of the isotonic approach depends on the two values on the bin edges.
In the case where the two bin edges do not share the same value, isotonic regression performs linear interpolation to calculate the predicted value. 
This behaviour is due to the way that the isotonic approach is estimated. 
To ensure the estimated function is monotonically increasing, the learning algorithm starts with the first bin edge as the minimal feature value ($0$ in the case of an isotonic calibration) and extends the following bin edges until it sees a higher target value (this is also referred to as `pooling adjacent violators' \cite{fawcett2007}).
It can be proven that, with monotonic sets of $\mathbf{b}$ and $\mathbf{s}$, the learning algorithm is equivalent to optimising the following loss \cite{ayer1955empirical}: 
%
\begin{align}
\mathsf{L}(\mathbf{b}, \mathbf{v}) = \frac{1}{N} \sum_{i=1}^{N}\Big( \mathsf{g}(s_i; \mathbf{b}, \mathbf{v}) - y_i\Big)^2
\end{align}
%
Therefore, when used as a probability calibration map, isotonic regression minimises the Brier score on the training set.
Instead of applying isotonic regression directly, \cite{naeini2016} also consider building an ensemble calibration map by combining a set of near-isotonic functions.  
Recently, \cite{allikivi2019} propose a Bayesian approach to improve isotonic regression, with demonstrated improvements on binary tasks.

Isotonic regression is a compelling approach for probability calibration, with the following advantages:
(1) When the monotonic assumption is suitable, isotonic regression can find the optimal bin edges for Brier score on the training sets, which is also known to give the convex hull in ROC analysis.
(2) The non-parametric nature avoids catastrophic model misfit.
On the other hand, isotonic regression has some drawbacks also:
(1) By predicting constant values within bins, it inevitably increases grouping loss. 
(2) When the uncalibrated model has a non-monotonic reliability diagram, isotonic regression can only give sub-optimal results (i.e. large grouping loss).
(3) While it performs well on large datasets, isotonic regression's training time and memory consumption are also high on large datasets.
(4) Isotonic regression can result in the first and last bins having full confidence (0 and 1), which can be problematic for certain datasets and evaluation metrics (e.g. log-loss). 
It is therefore common to clip the outputs from isotonic regression with a small $\epsilon$ (i.e., $0$ to $\epsilon$ and $1$ to $1 - \epsilon$).

\subsubsection*{Platt Scaling}

Platt scaling is probably one of the most widely known approaches for probability calibration, partly due to the popularity of SVMs around the year 2000 \newtext{\cite{platt2000}}.
As SVMs are optimised with hinge loss, they can only output scores on the samples based on the estimated margins.
Given that the margins are real scalars by definition, John Platt proposed to transform the scores into probability estimates with logistic regression.
Platt scaling hence has the same parameters as a univariate logistic regression model: 
a shape parameter $w \in \mathbb{R}$, and  
a location parameter $b \in \mathbb{R}$.
The predictive function is then: 
%
\begin{align}
\mathsf{g}(s; w, b) = \frac{1}{1+\exp(-w \cdot s-b)}
\end{align}
%
The parameters can be estimated by optimising the log-likelihood on the training set, so Platt scaling can be seen as optimising log-loss in the calibration context:
%
\begin{align}
\mathsf{L}(w, b) = \frac{1}{N} \sum_{i=1}^{N} \ln \Big(\sum_{j=1}^{2} - \mathsf{I}(y_i=j) \cdot \mathsf{g}(s; w, b)\Big) 
\end{align}
%

\begin{figure}[!tbp]
    \centering
    \begin{subfigure}{\textwidth}
    \centering
    % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case1_PLATT_prediction.png}
    \includegraphics[width=0.28\textwidth]{Case1_PLATT_calibration.png}
    \includegraphics[width=0.28\textwidth]{Case1_PLATT_reliability.png}
    \caption{Test case 1: under-confidence}
    \end{subfigure}
    
    
    \begin{subfigure}{\textwidth}
    \centering
    % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case2_PLATT_prediction.png}
    \includegraphics[width=0.28\textwidth]{Case2_PLATT_calibration.png}
    \includegraphics[width=0.28\textwidth]{Case2_PLATT_reliability.png}
    \caption{Test case 2: over-confidence}
    \end{subfigure}
    
    \begin{subfigure}{\textwidth}
    \centering
    % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case3_PLATT_prediction.png}
    \includegraphics[width=0.28\textwidth]{Case3_PLATT_calibration.png}
    \includegraphics[width=0.28\textwidth]{Case3_PLATT_reliability.png}
    \caption{Test case 3: MLP classifier}
    \end{subfigure}
    
    \caption{Examples of the Platt scaling approach. While it improves the under-confidence case well, it fails to do much with the over-confidence case. This is due to the fact that the sigmoid shape can not push the probabilities towards the middle hence can not fix over-confidence. Such result can also be observed with the MLP test case, where Platt scaling actually makes the level of calibration worse around several regions.}
    \label{fig:test_platt}
\end{figure}


% In addition, as ordinary logistic regression with log-loss can easily overfit to small datasets, 
Platt also included a technique to prevent overfitting and improve the generalisation of calibration, \newtext{which is introduced as one of the training schemes at the beginning of this section.}
The test results are shown in Figure~\ref{fig:test_platt}.

In general, Platt scaling is a practical calibration approach with the following advantages:
(1) As it is based on logistic regression, implementation is straightforward.
(2) The standard logistic regression has a convex loss.
The overall training process can, therefore be quite fast.
On the negative side, Platt scaling has two main drawbacks:
(1) The calibration map is restricted to a sigmoid shape, which effectively pushes probabilities away from the centre and may lead to over-confidence.
(2) By definition, the logistic regression model considers the input space to be a real scalar space. 
While such an assumption is suitable for the margins obtained from an SVM, it is less appropriate for probabilistic classifiers, as the input is bounded by the interval $[0, 1]$. 
Hence, certain transformations are required when applying Platt scaling to calibrate probabilistic classifiers, such as the logit transform.

\subsubsection*{Beta Calibration}

Beta calibration is specifically designed for probabilistic classifiers \newtext{and alleviates both drawbacks of Platt scaling \cite{pmlr-v54-kull17a,kull2017beyond}}.
While the latter can be derived from first principles by assuming that within each class the scores are normally distributed with the same variance, Beta calibration instead assumes two Beta distributions.
This gives a richer family of calibration functions with three parameters: two shape parameters $a, b \in \mathbb{R}$, and a location parameter $c \in \mathbb{R}$. 
The calibration function is then given as:
%
\begin{align}
\mathsf{g}(s; a, b, c) = \frac{1}{1+\exp \big(-a \cdot \ln s + b \cdot \ln(1-s) - c \big)}
\end{align}
%
In comparison with Platt scaling, Beta calibration is a bivariate logistic regression model, where the two features are $\ln s$ and $\ln(1-s)$ respectively.
Similar cross-validation training is also adopted as proposed in \cite{pmlr-v54-kull17a}. 

Given its close relationship to logistic regression, Beta calibration also optimises the log-loss and the objective function can be given with the log-likelihood:
%
\begin{align}
\mathsf{L}(a, b, c) = \frac{1}{N} \sum_{i=1}^{N} \ln \Big(\sum_{j=1}^{2} - \mathsf{I}(y_i=j) \cdot \mathsf{g}(s; a, b, c)\Big)
\end{align}

\begin{figure}[!htbp]
    \centering
    \begin{subfigure}{\textwidth}
    \centering
    % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case1_BETA_prediction.png}
    \includegraphics[width=0.28\textwidth]{Case1_BETA_calibration.png}
    \includegraphics[width=0.28\textwidth]{Case1_BETA_reliability.png}
    \caption{Test case 1: under-confidence}
    \end{subfigure}
    
    
    \begin{subfigure}{\textwidth}
    \centering
    % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case2_BETA_prediction.png}
    \includegraphics[width=0.28\textwidth]{Case2_BETA_calibration.png}
    \includegraphics[width=0.28\textwidth]{Case2_BETA_reliability.png}
    \caption{Test case 2: over-confidence}
    \end{subfigure}
    
    \begin{subfigure}{\textwidth}
    \centering
    % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case3_BETA_prediction.png}
    \includegraphics[width=0.28\textwidth]{Case3_BETA_calibration.png}
    \includegraphics[width=0.28\textwidth]{Case3_BETA_reliability.png}
    \caption{Test case 3: MLP classifier}
    \end{subfigure}
    
    \caption{Examples of Beta calibration. The Beta approach deals with the under-confident case fairly well, as the reliability diagram follows the diagonal closely after calibration. Regarding the over-confident case, Beta calibration manages to put more corrections than the Platt scaling around the $[0, 0.5]$ region, as it pushes the reliability diagram towards the diagonal. However, it doesn't help much in $[0.5, 1.0]$ region. On the MLP case, Beta provides some improvements around the $[0.6, 1.0]$ region, and matches the reliability diagram to the diagonal. Here we can see that the reliability diagrams after calibration are almost identical for the over-confidence and under-confidence test cases. This observation is because the Beta calibration method fits the map on the logarithm of the uncalibrated probabilities, and therefore reverts the sigmoid functions of the pseudo-models in both test cases. The calibration method then finds similar solutions as the pre-sigmoid parts are both linear models on the feature. This result suggests that the Beta calibration method can effectively fix the over/under-confidence caused by a sub-optimal linear-sigmoid operation. }
    \label{fig:test_beta}
    % \todo{Hao: add two sentences why the top two reliability diagrams are the same in Fig. \ref{fig:test_beta}.}
\end{figure}

Figure~\ref{fig:test_beta} demonstrates Beta calibration on the three test cases.
The advantages of Beta calibration include:
(1) Compared with Platt scaling, it allows a richer family of calibration maps including inverse sigmoids and the identity map. 
The latter is particularly useful to prevent over-calibration and apply unnecessary adjustments to already calibrated probabilities.
(2) Like with Platt scaling, implementation is straightforward. 
(3) With the Beta assumption, the calibration map supports any two-class probabilistic classifiers, and the calibration map is  learnt from a set of functions that map from $[0, 1]$ to $[0, 1]$. 
However, Beta calibration's main drawback is that it can only model specific calibration maps, so if the original classifier is severely uncalibrated and requires a complicated calibration map, it might be preferable to choose non-parametric methods instead. %and it can obtain ill-posed results (e.g. non-monotonic calibration map) around the boundaries if no constraint is applied to the parameters.
% \todo{Hao: please reformulate last two sentences as they are cryptic to me (PF) how about now.}

\subsection{Calibration for Multi-class Classification}

We now proceed with calibration maps that can work natively with a multi-class classification task, without the need for binarisation.
%
% % \subsubsection*{Uncalibrated Classifier for a 3-class Problem}
% In this section, we only focus on the test case with the MLP classifier, since both the concepts of over-confident and under-confident are considered in a two-class setting.
%
We define a three-class test case for the purpose of examining multi-class calibration with a multi-layer perceptron (MLP).
% In this case we only consider the MLP classifier, as the concepts of under-confidence and over-confidence can be examined with two-class calibration methods.
We modify the previous synthetic dataset to add an additional class, such that all classes are equi-probable and the distribution of the feature for the instances of class 3 is Gaussian also:
\begin{align*}
    Y &\sim \text{Categorical}([\frac{1}{3}, \frac{1}{3}, \frac{1}{3}]) \\
    H &\sim \text{Categorical}(0.5) \\
    X \mid Y=1, H=1 &\sim \text{Gaussian}(-4, 960) \\
    X \mid Y=1, H=2 & \sim \text{Gaussian}(64, 1280) \\
    X \mid Y=2, H=1 & \sim \text{Gaussian}(4, 980) \\
    X \mid Y=2, H=2 & \sim \text{Gaussian}(-72, 1024) \\
    X \mid Y=3 &\sim \text{Gaussian}(0, 8) \\
\end{align*}

% On the visualisation side, because the calibration map is no longer a $1D$ function, we consider to visualise them in a class-wise simplex.
We visualise the calibration maps in the probability simplex (one for each class). 
An example can be seen in the top row of Figure~\ref{fig:TS}, where the heat maps indicate the change of probability for each class after calibration.
For the figure on the left, each point within the simplex represents an uncalibrated probability vector, a positive value (i.e., red colour) on that point indicates that the calibration map increases the probability value of class 1 in the vector and a negative value (i.e., blue colour) shows that the probability value on class 1 is reduced.
The white line indicates where the probability values for class 1 remain (almost) unchanged.
Class 2 and class 3 calibration maps are also depicted.
% Regarding the reliability diagram, we select the class-wise reliability diagram, and examples can be seen at the bottom of Figure~\ref{fig:TS}.
The bottom row of each figure shows the class-wise reliability diagrams. 

\subsubsection*{Temperature Scaling}

\begin{figure}[!tbp]
    \centering
    %\includegraphics[width=0.85\textwidth]{figures/calibrators/TS_prediction.png}
    \includegraphics[width=0.95\textwidth]{TS_calibration.png}
    \includegraphics[width=0.85\textwidth]{TS_reliability.png}
    \caption{MLP classifier with Temperature scaling (top: class-wise calibration map, bottom: class-wise reliability diagram). While Temperature scaling manages to improve the reliability diagram around the $[0.1, 0.4]$ region for classes 1 and 2, we can see it actually makes things worse elsewhere. As the calibration maps show, Temperature scaling applies the same calibration map to all three classes despite them having different class-wise reliability diagrams, which is the main reason for the sub-optimal results.}
    \label{fig:TS}
\end{figure}

Temperature scaling has become one of the default approaches to provide better-calibrated probabilities, \newtext{particularly in deep learning research \cite{hinton2015distilling,guo2017}}.  
Instead of simply applying the softmax operation at the last layer to obtain a probability vector on the classes, Temperature scaling assumes a single temperature parameter $t \in \mathbb{R}$ and applies a linear operation before the softmax.
Denoting $\mathbf{z} = [z_1, \dots, z_K] \in \mathbb{R}^K$ as the $K$-dimensional real vector before softmax, the probability output after Temperature scaling is given as:
%
\begin{align}
\mathsf{c}_{j}(\mathbf{z}; t) = \frac{\exp\big(-z_j / t\big)}{\sum_{j=1}^{K}\exp\big(-z_j / t\big)}
\end{align}
%
Therefore, conventional softmax can be seen as the case of scaling with a fixed temperature of $t=1$.

If we want to apply Temperature scaling to a generic probabilistic model where $z$ is not accessible, we can also use the $\mathsf{logit}$ transform on the uncalibrated probability vector to obtain a real vector:
%
\begin{align*}
    z_j &= \mathsf{logit}_j (\mathbf{s}) \\
        &= \ln\frac{s_j}{s_K}
\end{align*}
%
Here, $K$ is selected as the reference class to compute the probability ratio with other classes.
The parameter is also normally estimated with the log-loss, and the objective function is given as:
%
\begin{align}
\mathsf{L}(t) = \frac{1}{N} \sum_{i=1}^{N} \ln \Big(\sum_{j=1}^{K} - \mathsf{I}(y_i=j) \cdot \mathsf{g}_{j}(\mathbf{z}_i; t)\Big)   
\end{align}

Figure~\ref{fig:TS} gives the results on the MLP test case.
The most distinctive characteristic of Temperature scaling is that it only has a single parameter, which can be seen as both an advantage and a disadvantage.
On the positive side, a single parameter restricts the space of calibration maps and can prevent overfitting for small datasets with many classes. 
On the negative side, Temperature scaling can be sub-optimal when the function space of the calibration maps does not include the right reliability diagram.  

\subsubsection*{Vector Scaling}

\begin{figure}[!tbp]
    \centering
    % \includegraphics[width=0.85\textwidth]{figures/calibrators/VS_prediction.png}
    \includegraphics[width=0.95\textwidth]{VS_calibration.png}
    \includegraphics[width=0.85\textwidth]{VS_reliability.png}
    \caption{Class-wise calibration maps and reliability diagrams for the MLP classifier with Vector scaling. The most obvious change from Temperature scaling is that now the calibration maps are different for each class. However, the calibration maps still have a circular shape as Vector scaling only adjusts one dimension of the logit vector for each class. As a result, the reliability diagram is close to the ones of Temperature scaling. Some minor improvements can be seen with class 3, where Vector scaling does not make it quite as bad as for Temperature scaling. }
    \label{fig:VS}
\end{figure}

Where Temperature scaling only has a single parameter across all classes, it is natural to extend the parameters to support a richer form of calibration maps.
Vector scaling \newtext{\cite{guo2017}} allows a different temperature for each class, denoted as $\mathbf{w} \in \mathbb{R}^{K}$, as well as adding a set of intercept parameters $\mathbf{b} \in \mathbb{R}^{K}$ for the $K$ classes.
The predictive function is given as ($\mathbf{z}$ can also be obtained with the logit transform for generic probability classifier, as in Temperature scaling):
%
\begin{align}
\mathsf{c}_{j}(\mathbf{z}; \mathbf{w}) = \frac{\exp\big(-w_j \cdot z_j -b_j\big)}{\sum_{j=1}^{K}\exp\big(-w_j \cdot z_j - b_j\big)}
\end{align}
%
And the objective function to optimise log-likelihood is similar to the one for Temperature scaling, but with more parameters:
%
\begin{align}
\mathsf{L}(\mathbf{w}, \mathbf{b})= \frac{1}{N} \sum_{i=1}^{N} \ln \Big(\sum_{j=1}^{K} - \mathsf{I}(y_i=j) \cdot \mathsf{g}_{j}(\mathbf{z}_i; \mathbf{w}, \mathbf{b})\Big)
\end{align}

The test result is given in Figure~\ref{fig:VS}.
Vector scaling can be seen as a middle point between the quite restrictive Temperature scaling and the general approach of Matrix scaling discussed below. 
Hence it balances the risk of overfitting and the richness of available calibration maps. 

\subsubsection*{Matrix Scaling}

Matrix scaling \newtext{\cite{guo2017}} removes all the parameter constraints on Temperature scaling and Vector scaling.
Similar to a fully connected layer, it has a matrix parameter $(\mathbf{w}_1, \cdots, \mathbf{w}_K), \mathbf{w}_j \in \mathbb{R}^K$ together with the intercept parameter $\mathbf{b} \in \mathbb{R}^{K}$.
The predictive function is ($\mathbf{z}$ can also be obtained with the logit transform, as in Temperature scaling):
%
\begin{align}
\mathsf{c}_{j}(\mathbf{z}; \mathbf{w}_1, \dots, \mathbf{w}_{K}, \mathbf{b}) = \frac{\exp\big(-\mathbf{w}_j^T \mathbf{z} - b_j\big)}{\sum_{j=1}^{K}\exp\big(-\mathbf{w}_j^T \mathbf{z} - b_j\big)}
\end{align}
%
and the objective function is:
%
\begin{align}
\mathsf{L}(\mathbf{w}_1, \dots, \mathbf{w}_K, \mathbf{b})= \frac{1}{N} \sum_{i=1}^{N} \ln \Big(\sum_{j=1}^{K} - \mathsf{I}(y_i=j) \cdot \mathsf{g}_{j}(\mathbf{z}_i; \mathbf{w}_1, \dots, \mathbf{w}_K, \mathbf{b})\Big)
\end{align}

As indicated in Figure~\ref{fig:MS}, Matrix scaling can support a broader family of calibration maps than Vector scaling and Temperature scaling, but may be vulnerable to overfitting as it can be seen as another fully connected layer.  

\begin{figure}[!tbp]
    \centering
    % \includegraphics[width=0.85\textwidth]{figures/calibrators/MS_prediction.png}
    \includegraphics[width=0.95\textwidth]{MS_calibration.png}
    \includegraphics[width=0.85\textwidth]{MS_reliability.png}
    \caption{Class-wise calibration maps and reliability diagrams for the MLP classifier with Matrix scaling. As Matrix scaling is capable of providing fully linear adjustments on the logits for each class, we can see the class-wise calibration map no longer has the circular shape. While there are still minor improvements on the reliability diagram of class 1 and class 2, class 3 has gained a significant improvement.}
    \label{fig:MS}
\end{figure}

\subsubsection*{Dirichlet Calibration}

Dirichlet calibration is the multi-class extension of Beta calibration \cite{kull2019}.
Assuming Dirichlet distributions for the predicted probability vectors within each class, Dirichlet calibration is determined by a set of coefficient vectors $(\mathbf{w}_1, \cdots, \mathbf{w}_K), \mathbf{w}_j \in \mathbb{R}^K$, and a set of intercepts $\mathbf{b} \in \mathbb{R}^{K}$. 
The calibrated probability on the $j\text{-th}$ class is obtained as:
%
\begin{align}
\mathsf{g}_{j}(\mathbf{s}; \mathbf{w}_1, \dots, \mathbf{w}_{K}, \mathbf{b}) = \frac{\exp(-b_j - \mathbf{w}_j^T \ln \mathbf{s})}{\sum_{j=1}^{K}\exp(-b_j-\mathbf{w}_j^T \ln \mathbf{s})}
\end{align}
%
This function can be seen as a $K$-dimensional logistic regression on the log-probabilities (i.e., the sufficient statistics of the Dirichlet distribution). 
Therefore, to apply Dirichlet calibration to a deep neural network, one can first obtain a probability vector using the softmax function, then apply Dirichlet calibration as with other probabilistic classifiers.
%
The objective function is:
%
\begin{align}
\mathsf{L}(\mathbf{w}_1, \dots, \mathbf{w}_K, \mathbf{b})= \frac{1}{N} \sum_{i=1}^{N} \ln \Big(\sum_{j=1}^{K} - \mathsf{I}(y_i=j) \cdot \mathsf{g}_{j}(\mathbf{s}_i; \mathbf{w}_1, \dots, \mathbf{w}_K, \mathbf{b})\Big)
\end{align}

The test results are given in Figure~\ref{fig:Dcal}.
Similar to Beta calibration, one of the advantages of Dirichlet calibration is that it also supports the identity map, so it can also prevent over-adjusting calibrated results.
% Following the derivation, the Dirichlet can also be written with an interpretable canonical parameter form.
As the number of parameters is similar to that of Matrix scaling, the Dirichlet calibration can also overfit on small datasets.
The authors propose the ODIR (Off-Diagonal and Intercept Regularisation) approach to address this issue further and report various performance improvements in their experiments.



\begin{figure}[!tbp]
    \centering
    % \includegraphics[width=0.85\textwidth]{figures/calibrators/DIR_prediction.png}
    \includegraphics[width=0.95\textwidth]{DIR_calibration.png}
    \includegraphics[width=0.85\textwidth]{DIR_reliability.png}
    \caption{Class-wise calibration maps and reliability diagrams for the MLP classifier with Dirichlet calibration. The overall results on the class-wise reliability diagrams are close to those obtained with Matrix scaling. 
    % This is understandable considering the similarity on their mathematical forms. 
    The major differences are seen in the calibration maps, where we can clearly observe a local region for the changes on class 3. Importantly, this region for the Dirichlet calibration approach doesn't cover the area where the predicted probability of class 3 is close to 1. This is more reasonable compared with Matrix scaling, as both the Bayes-optimal predictions and the MLP predictions for class 3 are capped around 0.8.}
    \label{fig:Dcal}
\end{figure}

% \begin{figure}[!tbp]
%     \centering
%     \includegraphics[width=0.85\textwidth]{figures/calibrators/all_prediction.png}
%     \includegraphics[width=0.85\textwidth]{figures/calibrators/all_reliability.png}
%     \caption{A comparison of all calibrators on the binary synthetic dataset.}
%    \label{fig:all}
%\end{figure}

%\begin{figure}[!tbp]
%    \centering
%    \includegraphics[width=0.85\textwidth]{figures/calibrators/all3_prediction.png}
%    \includegraphics[width=0.85\textwidth]{figures/calibrators/all3_reliability.png}
%    \caption{A comparison of all calibrators on the ternary synthetic dataset.}
%    \label{fig:all_3}
%\end{figure}

% \subsection{Calibration methods by extension}

% At the end of this section we briefly mention related approaches that can improve the level of probability calibration in a classification setting, as well as specific applications in areas such as computer vision and natural language processing.
% While we have demonstrated generic post-hoc calibrators that can work with any probabilistic classifier without extensive training setup and specific domain knowledge (i.e. DNN architecture), in this section we will address some methods that come with such additional requirements.
% The methods covered in this section can be described with the following categories: (1) methods that can improve calibration during training time, (2) methods that require a composite training scheme, and (3) methods that work on uncertainty quantification tasks related to classifier probability calibration. 

% \subsubsection{Binary probability calibration, class-wise calibration and confidence calibration}
% Being one of most basic and interpretable definition of calibration, 
\newtext{
\subsection{Extended methods for post-hoc classifier calibration}
\label{sec:cal:extension}
%While some standard binary and multi-class post-hoc calibration methods are introduced above, the research area has recently drawn more attention as the industry is adopting ML systems into production.
In this section we discuss more recent work extending the standard calibration methods discussed above. 

\citet{leathart2017} aim to build calibration maps locally instead of a global calibration map and proposes using modified logistic model trees to build an ensemble calibration method. A decision tree is learnt to separate the original feature space into multiple regions, where a local calibrator can then be estimated using the corresponding outputs and labels.
\citet{kumar2019} propose a combined approach of scaling and binning methods to achieve better calibration with smaller calibration sets. Instead of calculating the label frequency in binning methods, the authors show that using the average value of a pre-fit continuous calibration map gives better calibration. The authors also indicate that a debiased estimator can provide better calibration error in sample complexity.
\citet{wang2019calibrating} discuss how to build flexible univariate non-decreasing calibration maps from shape-restricted polynomial regression models. The resulting method provides a useful alternative when methods like Plat scaling and Beta calibration cannot approximate the actual reliability diagram.
\citet{wenger2020} investigate non-parametric post-hoc approaches that can support richer forms of calibration map for a multi-class setting.
The idea is to employ the framework of Gaussian processes and model the calibration map as latent distribution of functions.
The family of calibration maps can thus be richer with the selection of suitable kernels.
\citet{zhang2020mix} propose an approach to build an ensemble of base calibrators, which can improve the capacity of the calibration maps while preserving the accuracy.
The authors also adapt kernel density estimation as an alternative approach to evaluating calibration error. 
\citet{ma2021meta} consider the confidence calibration setting and propose to improve a calibration map with a ranking model. The authors demonstrate that the ranking model can be used to maintain the performance of the uncalibrated classifier in terms of precision and false positive rate.
\citet{patel2021multiclass} tackle the issue of applying class-wise binning calibrators to a multi-class setting. An iterative update method is provided to adjust the bin edges to better calibration, and a sample-sharing approach among similar classes is also introduced for better sample efficiency. 

\subsection{Methods that can improve calibration during training time}
\label{sec:cal:training}

%So far, we have been mainly focusing on post-hoc calibration approaches.
While post-hoc calibration can be applied to most existing classifiers, it is of practical interest to train well-calibrated models in the first place.
Here we briefly mention some training-time calibration methods.

\citet{kumar2018} consider a regularisation approach with kernel mean embedding.
The idea is to add a differentiable regularisation term concerning the goodness of calibration, where the kernel mean of the scores is calculated as an approximation of the calibration error. 
The overall objective function allows the model to achieve better calibration during the training phase.
\citet{thulasidasan2019mixup} show that the Mixup strategy can improve the calibration level when introduced during the training phase.
Vicinal points are created by combining existing data points and labels, and then added to the training set.
The authors suggest that the improvement in calibration is due to the augmentation effect and label smoothing effect, both from the mixup process and act as a form of regularisation.
\citet{kristiadi2020being} consider a Bayesian approach where a Gaussian approximation distribution is fitted to the last layer's weights of a ReLu network.
The authors demonstrated that the method could reduce the over-confidence problem in a classification setting, particularly on data points not commonly seen in the original training set.
\citet{wen2020batchensemble} propose an efficient ensemble approach that can train multiple deep networks with lower computational and memory costs.
The authors show that the obtained ensemble achieves better calibration on out-of-distribution samples at test time.

Other than deep networks, some recent work achieves better calibration on Bayesian nonparametric methods.
\citet{milios2018} propose an alternative approach to train Gaussian Processes for classification tasks.
While the traditional GP classifier relies on sigmoid or probit link functions and requires suitable approximated inference schemes to ensure good performance, the authors propose a modified Dirichlet link function to ensure the level of calibration as well as scalability.
\citet{tran2019calibrating} demonstrate that convolution Gaussian process classifiers can be miscalibrated, and propose a solution to mitigate the issue.

% \subsubsection{Methods that require a composite fitting procedure}

% While we have introduced some general calibration methods in detail, some recent work has introduced methods that can improve calibration in a certain sense (i.e. from a binary, class-wise or confidence perspective), with the cost of a more composite fitting procedure.
% Given the diversity of these fitting procedures, here we provide a brief introduction to some of the methods so the readers can further refer to the papers for implementation details. 


\subsection{Methods for probability calibration for other predictive settings}
\label{sec:cal:other}

% Although we have discussed probability calibration in a classification setting, 
The concept of calibration can be naturally generalised to predictive settings other than classification.
The most straightforward extension is the calibration of regression outputs.
As in the classification scenario, there are multiple definitions of calibration for regression models.
The standard definition of calibration comes from the field of quantile regression \cite{koenker2001quantile}, where being calibrated means that the predicted quantile matches the marginal distribution of the target variable.
As in the case of classification, there are methods designed for training calibrated quantile regression as well as post-hoc approaches that calibrate pre-trained models.
\citet{fasiolo2020fast} provide an approach to train generalised additive regression models with calibrated quantiles.
\citet{cui2020calibrated} propose an approach to train deep regression models with better-calibrated quantiles, where the model parameter is first fit with log-loss and then updated with a loss based on the maximal mean discrepancy \cite{gretton2012kernel}.
For the post-hoc setting, \citet{kuleshov2018} point out that deep regression models' quantiles can be calibrated with binary calibrators such as isotonic regression and yield better performance on downstream tasks such as reinforcement learning.
\citet{chung2021beyond} introduce some modified loss functions to train quantile calibrators with specific emphases, such as balancing between calibration and sharpness. 

Regarding the definition of calibration, \citet{pmlr-v97-song19a} propose a stronger notion of calibration in regression, where the local conditional distribution is required to be calibrated instead of the global quantile. 
The authors 
% refer to this definition as distribution-calibrated for regression models and 
show that being distribution-calibrated in this sense implies being quantile-calibrated.
A post-hoc approach based on the Gaussian process is also introduced, where the GP models a distribution of Beta calibrators conditioning on the original regression outputs.
\citet{kuleshov2022calibrated} consider achieving post-hoc distribution calibration by learning a lower dimensional representation of the (uncalibrated) local distributions, and the post-hoc calibrators can then be built with density estimators on these representations and the target values, which avoids the costs of distributional kernels and sparse variational inference.
\citet{sahoo3reliable} propose the definition of threshold calibration for regression models, which is a stronger notion of calibration than being quantile-calibrated and weaker than the distribution-calibrated definition.
Instead of asking for calibration on a marginal quantile or local distribution level, the proposed definition requires the model to be calibrated on a group of distributions that satisfy a given threshold condition, which ensures optimal decision-making when a threshold is put on the regression outputs.

Calibration of structured outputs, such as sequential outputs, is also of interest for application domains such as natural language processing and time-series modelling. 
\citet{kuleshov2015calibrated} propose approaches to simplify the structured output to a two-class problem and employ a well-calibrated binary classifier to improve the calibration level.
On the information-retrieval side, the traditional precision-recall curve is not sufficiently similar to a ROC curve to allow a similar calibration property.
In contrast, the precision-recall-gain curve proposed by \citet{flach2015} can be seen as a proper generalisation of ROC curve obtained by replacing weighted accuracy with F-score.


Conformal prediction \cite{vovk2005algorithmic,romano2019conformalized,angelopoulos2021gentle} is another area closely related to the topic of probability calibration.
For classification, conformal prediction aims to predict a set of labels that has a probability of $1 - \alpha$ that includes the true label, where $\alpha$ is a user-defined significance level.
Therefore, we can see the conformal prediction for classifiers as an alternative definition of calibration to label probability calibration. That is, instead of requiring the probability to be accurate on the label distributions, conformal prediction wants to ensure the calibration on a variable set of labels that are exactly calibrated on the given significance level.
One of the approaches to construct a conformal classifier is to use a Venn predictor \cite{vovk2003self,vovk2012venn,johansson2018}.
The framework makes use of the Venn taxonomy to define subsets of the original label space, and requires a classifier to make predictions about each element in the subset.
The final conformal prediction can then be calculated using these predictions.

\subsection{Methods designed for other research fields and applications}
\label{sec:cal:app}

The notion of calibration can also be generalised to other areas where uncertainty quantification is of interest. rRecent work has started to explore other topics in statistics, machine learning and artificial intelligence related to calibration.
Here we briefly introduce some of them. 
A comprehensive analysis of these works is left as future work.
\citet{pleiss2017fairness} draw a link between the level of calibration and the evaluation of classifier fairness.
\citet{CobbGal2018Loss} propose an approach to modify the lower bound of approximate Bayesian inference so that the final objective function can be calibrated according to a given decision loss. 
\citet{liu2018generalized} adopt calibrated deep models to improve zero-shot learning.
\citet{menon2018loss} consider the calibration problem for an anomaly detection setup.
\citet{ghandeharioun2019characterizing} consider uncertainty and calibration as a tool to improve explainability for computer vision tasks. 
And \citet{liu2019accurate} adopt a calibration procedure to achieve better posterior distributions for a Bayesian non-parametric ensemble model.
\citet{ding2021local} consider the problem of improving calibration for semantic segmentation.
\citet{guillory2021predicting,jiang2021assessing} show that calibrated classifier can be used to estimate the model performance on OOD test sets. 
}


% \cite{kuleshov2018} focus on the calibration of quantile regression approaches, and propose to use binary post-hoc calibrators to improve various deep regression models.

%\cite{song2019} proposes a stronger definition of calibration for regression tasks, which requires the output to be calibrated on a distribution level instead of a quantile level, a GP-based approach is also given to improve such calibration.

% \cite{widmann2019} gives a statistical test framework for calibration in a multi-class setting.

% {\color{red}
% I will add some citations here that may be useful as well

% \cite{Krishnan2020}
% \begin{itemize}
%     \item Uncertainty under distribution shift between training and test
%     \item Propose a new differentiable accuracy versus uncertainty calibration (AvUC) loss function
%     \item Can be applied as a post-hoc calibration method
%     \item Intended to deal with out-of-distribution in the training data manifold
%     \item Categorise calibration methods into: (1) post-processing calibration (eg. Temperature scaling and dirichlet calibration), (2) training with data augmentation, (3) probabilistic methods with respect to the model parameters.
%     \item Contribution: (1) differentiable proxy for Accuracy versus Uncertainty measure (not sure if this measure is also a contribution), (2) evaluation of results under distribution shift, (3) propose post-hoc calibration with Temperature scaling, (4) comparison with stae-of-the-art methods (need to see this yet).
%     \item Evaluation metrics: conf-ECE, expected uncertainty calibration error (UCE) [41], NLL, Brier score, conditional probabilities $p(accurate|certain)$ and $p(uncertain|inaccurate)$ [39], AUROC, and AUPR (not gain curves).
%     \item Accuracy vs uncertainty (AvU) uses a confusion matrix to compute the "accuracy" of "certainty". Basically, constructing a confusion matrix of correctly predicted vs certain predictions if a threshold is well defined, and then computing the Accuracy on that confusion matrix.
%     \item Accuracy vs uncertainty calibration (AvUC) loss: In order to make the previous metric differentiable, a surrogate function is defined by defining a fixed threshold to determine what is considered certain, and an hyperbolic tangent of the certainty is used to approximate a similar behaviour than AvU in ideal conditions.
%     \item AvUC loss is used as an additional term to the original loss, and intended to be used as a regularization factor.
%     \item In the example with loss-calibrated evidence lower bound (ELBO), the first epochs are trained ONLY with ELBO, later the AvUC term is introduced with an scaling hyperparameter Beta. The required uncertainty "threshold is obtained from the average of predictive uncertainty mean for accurate and inaccurate predictions on the training data from initial epochs".
%     \item Question: The method is trying to calibrate the probabilistic outputs, but uses a fixed threshold to define what is certain, and what is not... This is very simplistic in my view, and it should show signs of poor classwise calibration.
%     \item Experiments compare several sota networks with Temperature scaling, deep-ensembles, Monte Carlo dropout, Mean-field stochastic variational inference, Temperature scaling on SVI, and Radial Bayesian neural network.
%     \item All methods evaluated in 16 types of image corruption at 5 level of intensities (80 variations).
% \end{itemize}
% }

% \subsection{The toy dataset (feature space, generative view)}
% For better illustration, we adopt a dataset and a set of visualisations.
% \begin{figure}
%     \centering
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/toy.png}\hfill
%     \includegraphics[width=0.62\textwidth]{figures/calibrators/toy_conditional.png}
% \end{figure}

% \subsection{The toy dataset (feature space, discriminative view)}

% As we know the data distribution, we can calculate the Bayes-optimal scoring model, that is: 
% \begin{align*}
% s(x) = P(Y=1 | X=x)
% \end{align*}

% \subsection{The distribution of predictions}
% We can further calculate the distribution of $s(x)$.
% \begin{figure}
%     \centering
%     \includegraphics[width=0.33\textwidth]{figures/calibrators/bayes_opt.png}
%     \caption{Distribution of scores }
% \end{figure}

% \begin{figure}
% \centering
% \includegraphics[width=0.62\textwidth]{figures/calibrators/bo_conditional.png}
% \caption{Probability distribution of scores per class}
% \end{figure}


% \subsection{Reliability diagram}
% As well as $P\Big(Y=1 | s(x)\Big)$ (reliability diagram).
% Since the model is Bayes-optimal, we have a perfect reliability diagram.
% \begin{figure}
%     \centering
%     \includegraphics[width=0.33\textwidth]{figures/calibrators/bo_score.png}
%     \includegraphics[width=0.27\textwidth]{figures/calibrators/bo_rg.png}
%     \caption{Joint probability distribution of the scores, and correspoinding reliability diagram.}
% \end{figure}

% \subsection{With a classifier}
% Now if we train a neural network with some samples.
% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/mlp.png}
% \includegraphics[width=0.28\textwidth]{figures/calibrators/mlp_rel.png}
% \caption{Neural network's predicted scores in the input space, and corresponding reliability diagram.}
% \end{figure}

% \subsection{Post-hoc calibrators}
% This is where we need post-hoc calibrators.

% \subsection{Post-hoc calibrators (scaling view)}

% \begin{itemize}
%     \item It is also common to re-scale a real vector output into calibrated probability vector space.  (e.g. SVM margins, final layer of a neural network) 
    
%     \item Since a real vector and a probability vector can be transformed into each other through link function and inverse link function (e.g. soft-max and logit transform), for later slides we will use the probability vector view by default. 

% \end{itemize}



% \begin{figure}
%     \centering
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/mlp_map.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/mlp_map_sca.png}
%     \caption{Example of original and scaled scores.}
% \end{figure}

% \section{Scaling v.s. Probability calibrator}

% \subsection{Scaling v.s. Probability calibrator}{
% \textbf{Scaling}: designed to re-scale a function output into probability vector space and match with target observations. (e.g. SVM margins, final layer of a neural network, latent functions modelled by a Gaussian process)

%   \begin{figure}
%       \centering
%       \includegraphics[width=0.28\textwidth]{figures/calibrators/svm_margin.png}
%       \includegraphics[width=0.1\textwidth]{figures/calibrators/right_arrow.png}
%       \includegraphics[width=0.28\textwidth]{figures/calibrators/svm_after.png}
%   \end{figure}

%}

% \subsection{Scaling v.s. Probability calibrator}{
% \textbf{Probability calibrator}: designed to match a probability output with target observations.

 %   \begin{figure}
   %    \centering
  %     \includegraphics[width=0.65\textwidth]{figures/calibrators/p_x_g_y_model.png} 
    %   \includegraphics[width=0.05\textwidth]{figures/calibrators/down_arrow.png}
   %    \includegraphics[width=0.65\textwidth]{figures/calibrators/p_x_g_y_hat.png}
  % \end{figure}

%}

% \subsection{Scaling v.s. Probability calibrator}{
% \textbf{Probability calibrator}: designed to match a probability output with target observations.

%    \begin{figure}
%        \centering
%        \includegraphics[width=0.65\textwidth]{figures/calibrators/simplex_model.png} 
%        \includegraphics[width=0.05\textwidth]{figures/calibrators/down_arrow.png}
%        \includegraphics[width=0.65\textwidth]{figures/calibrators/simplex_hat.png}
%    \end{figure}

% }

%\section{Categories of Calibrators}

%\subsection{Categories of Calibrators}{
%     Scaling approaches v.s. probability calibrator 
%     Parametric approaches v.s. non-parametric approaches 
%     Generative approaches v.s. discriminative approaches 
%}

%\subsection{Scaling approaches v.s. probability calibrator}{
%    \textbf{Scaling approaches}: designed to re-scale a function output into probability vector space and match with target observations.
    
%    \begin{figure}
%        \centering
%        \includegraphics[width=0.5\textwidth]{figures/calibrators/f_x.png} 
%        \includegraphics[width=0.15\textwidth]{figures/calibrators/down_arrow.png}
%        \includegraphics[width=0.5\textwidth]{figures/calibrators/p_x.png}
%    \end{figure}
%}

%\subsection{Scaling approaches v.s. probability calibrator}{
%    \textbf{Probability calibrator}: designed to match a probability output with target observations.
    
%    \begin{figure}
%        \centering
%        \includegraphics[width=0.5\textwidth]{figures/calibrators/p_x.png} 
%        \includegraphics[width=0.15\textwidth]{figures/calibrators/down_arrow.png}
%        \includegraphics[width=0.5\textwidth]{figures/calibrators/p_hat_x.png}
%    \end{figure}
%}

%\subsection{Scaling approaches v.s. probability calibrator}{
%The differences between scaling approaches and probability calibrators mainly come from their motivations.
%For instance, some scaling approaches are proposed for non-probabilistic models such as SVM.
%In practice, the application of both types are exchangeable. 
%We can re-scale a function value into probability estimation, and apply probability calibrators.
%We can also use inverse link function to turn a probability estimation into a real number, and apply scaling approaches.
%}

% \subsection{Parametric approaches v.s. non-parametric approaches}{}

% \subsection{Generative approaches v.s. discriminative approaches}{}

% \section{Calibrators}

% \subsection{Binary approaches}

% \begin{itemize}
%     \item \cite{naeini2016}
%     \item \cite{platt2000}
%     \item \cite{kull2017}
% \end{itemize}

% \subsubsection{Empirical Binning}

% While being simple and effective, binning approaches can only give discrete outputs.

% you can trust the probabilities, but it doesn't give many.

% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/emp_map_1000_10.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/emp_rel_1000_10.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/emp_1000_10.png}
% \caption{Empirical binning with 10 bins}
% \end{figure}

% A suitable number of bins / binning algorithm is important to get good results. 

% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/emp_map_1000_100.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/emp_rel_1000_100.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/emp_1000_100.png}
% \caption{Empirical binning with 100 bins}
% \end{figure}

% \textbf{Parameters:} 
% \hspace{24pt}Bins: $\{\mathbb{B}_1, \dots, \mathbb{B}_M \}, \mathbb{B}_j \subset [0, 1]$  
% \hspace{24pt}Bin averages:  $\mathbf{a}=(a_1,\dots,a_{M})$, $a_j \in \{0, 1\}$
% \vspace{12pt}
% \textbf{Predictive Function:} 
% \hspace{24pt}$c(p; \mathbb{B}_1, \dots, \mathbb{B}_M, \mathbf{a}) = \sum_{j=1}^{M} \mathbb{I}(p\in \mathbb{B}_j) \cdot a_j$ 
% \vspace{12pt}
% \textbf{Objective Function:} 
% \hspace{24pt} $\mathbb{L}(\mathbf{a}) = \sum_{j=1}^{M} \Big | \frac{\sum_{i=1}^{N} \mathbb{I}(p_i \in B_j) \cdot y_i}{|\mathbb{B}_j|} - a_j \Big|$ 


% \subsubsection{Isotonic Regression}

% With the ROC-convex hull method, isotonic regression can give good calibration performance with automatic binning and interpolation.
% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/iso_map_100.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/iso_rel_100.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/iso_100.png}
% \caption{Isotonic regression with 100 data points}
% \end{figure}

% More data points are beneficial for isotonic regression, but the monotonicity assumption might not be suitable for certain datasets / base models.
% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/iso_map_10000.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/iso_rel_10000.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/iso_10000.png}
% \caption{Isotonic regression with 10,000 data points}
% \end{figure}

% \textbf{Parameters:} 
% \hspace{24pt}Bin edges: $\mathbf{b}=(b_1,\dots,b_M)$, $b_j \in \{0, 1\}, b_j < b_{j+1}$  
% \hspace{24pt}Edge values:  $\mathbf{v}=(v_1,\dots,v_{M})$, $ v_j \in [0, 1], v_j \leq v_{j+1}$
% \vspace{12pt}
% \textbf{Predictive Function:} 
% \hspace{24pt}$c(p; \mathbf{b}, \mathbf{v}) = \frac{1}{\sum_{j=1}^{M-1} \mathbb{I}(p\geq b_j)\cdot\mathbb{I}(p\leq b_{j+1})}\sum_{j=1}^{M-1} \mathbb{I}(p\geq b_j)\cdot\mathbb{I}(p<b_{j+1}) \cdot \Big(v_j + \frac{p-b_j}{b_{j+1}-b_j}(v_{j+1} - v_j)\Big) $ 
% \vspace{12pt}
% \textbf{Objective Function:} 
% \hspace{24pt} $\mathbb{L}(\mathbf{b}, \mathbf{v}) = \frac{1}{N} \sum_{i=1}^{N}\Big( c(p_i; \mathbf{b}, \mathbf{v}) - y_i\Big)^2$ 

% \subsubsection{Platt Scaling}

% The ONE that allows SVMs to output probabilities.

% \begin{figure}
%        \centering
%        \includegraphics[width=0.4\textwidth]{figures/calibrators/svm_margin.png}\hfill
%        \includegraphics[width=0.1\textwidth]{figures/calibrators/right_arrow.png}\hfill
%        \includegraphics[width=0.4\textwidth]{figures/calibrators/svm_after.png}
%    \end{figure}

% We can also use it to calibrate from the final layer of the MLP classifier.
% \begin{figure}
%        \centering
%        \includegraphics[width=0.28\textwidth]{figures/calibrators/platt_map.png}\hfill
%        \includegraphics[width=0.28\textwidth]{figures/calibrators/platt_rel.png}\hfill
%        \includegraphics[width=0.28\textwidth]{figures/calibrators/platt.png}
% \end{figure}

% \textbf{Parameters:} 
% \hspace{24pt}Slope: $w \in \mathbb{R}$  
% \hspace{24pt}Intercept: $b \in \mathbb{R}$ 
% \vspace{12pt}
% \textbf{Predictive Function:} 
% \hspace{24pt}$c(p; w, b) = \frac{1}{1+\exp(-w \cdot p-b)}$ 
% \vspace{12pt}
% \textbf{Objective Function:} 
% \hspace{24pt} $\mathbb{L}(w, b) = \frac{1}{N} \sum_{i=1}^{N} \ln \Big(\sum_{j=1}^{2} - \mathbb{I}(y_i=j) \cdot c(p; w, b)\Big) $ 

% \subsubsection{Beta Calibration}

% While Platt scaling can be derived with conditional Gaussian distribution with shared variance, probabilities are on a finite support hence Gaussian is less suitable.

% With a Beta assumption, we can get calibration maps that get beyond sigmoid.
% \begin{figure}
% \centering
% \includegraphics[width=0.45\textwidth]{figures/calibrators/beta_list.png}
%\end{figure}

% As well as a identity map if the original model is already calibrated, or no better calibration map can be modelled.
% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/beta_3_map.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/beta_3_rel.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/beta_3.png}
% \end{figure}

% \textbf{Parameters:} 
% \hspace{24pt}Slope 1: $a \in \mathbb{R}$ 
% \hspace{24pt}Slope 2: $b \in \mathbb{R}$ 
% \hspace{24pt}Intercept: $c \in \mathbb{R}$ 
% \vspace{12pt}
% \textbf{Predictive Function:} 
% \hspace{24pt}$c(p; a, b, c) = \frac{1}{1+\exp\big(-a \cdot \ln p - b \cdot \ln (1-p) - c \big)}$ 
% \vspace{12pt}
% \textbf{Objective Function:} 
% \hspace{24pt} $\mathbb{L}(a, b, c) = \frac{1}{N} \sum_{i=1}^{N} \ln \Big(\sum_{j=1}^{2} - % \mathbb{I}(y_i=j) \cdot c(p; a, b, c)\Big) $ 

% \subsection{Multi-class approaches}


% \begin{table}[htpb!]
%     \centering
%     \begin{tabularx}{\linewidth}{L|l|l}
%         \toprule
%         \textbf{Calibration method} & \textbf{Details} & \textbf{} \\
%         \midrule
%         Platt's scaling \cite{platt1999}       &  Multiclass & Scaling \\
%         \midrule
%         Isotonic regression \cite{chakravarti1989}   &  & Non-parametric\\
%         \midrule
%         Nearly-Isotonic regression \cite{chakravarti1989}   &  & Non-parametric\\
%         \midrule
%         Size binning     & & \\
%         \midrule
%         Width binning     & & \\
%         \midrule
%         Binning averaging \cite{zadrozny2001}     & & \\
%         \midrule
%         Similarity binning averaging \cite{bella2009} & & \\
%         \midrule
%         Bayesian binning into quantiles \cite{naeini2015} & & \\
%         \midrule
%         Probability Calibration Trees \cite{leathart2017} & & \\
%         \midrule
%         Calibration of nested dichotomies \cite{leathart2018} & & \\
%         \midrule
%         Temporal probability calibration \cite{leathart2020} & & \\
%         \midrule
%         Venn predictors for probability estimation trees \cite{johansson2018} & &  \\
%         \midrule
%         Ensemble of Near Isotonic Regression \cite{Naeini2017} & Binary & \\
%         \midrule
%         Temperature scaling \cite{guo2017}  & Multiclass & \\
%         \midrule
%         Vector scaling \cite{guo2017}       & Multiclass & \\
%         \midrule
%         Matrix scaling \cite{guo2017}       & Multiclass &  \\
%         \midrule
%         Dirichlet calibration \cite{kull2019} & Multiclass & \\
%         \midrule
%         Accuracy versus uncertainty calibration (AvUC) loss \cite{Krishnan2020}   & Multiclass confidence & %  \\
%         \midrule
%         \cite{milios2018}   & &  \\
%         \midrule
%         \cite{allikivi2019} & &  \\
%         \midrule
%         \cite{Kumar2018}    & &  \\
%         \midrule
%         \cite{Wenger2020}   & &  \\
%         \midrule
%         \cite{Kuleshov2018} & &  \\
%         \midrule
%         \cite{song2019}     & &  \\
%         \midrule
%         \cite{widmann2019}  & &  \\
%          \bottomrule
%     \end{tabularx}
%     \caption{Caption}
% \end{table}

% \subsubsection{Start with adding one more class}

% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/ternary_1.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/ternary_2.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/ternary_3.png}
% \end{figure}


% \subsubsection{Temperature Scaling}

% \textbf{Parameters:} 
% \hspace{24pt}Temperature: $t \in \mathbb{R}$  
% \vspace{12pt}
% \textbf{Predictive Function:} 
% \hspace{24pt}$c_{j}(\mathbf{p}; t) = \frac{\exp\big(-t \cdot \text{logit}_j (p)\big)}{\sum_{j=1}^{K}\exp\big(-t \cdot \text{logit}_j (p)\big)}$ 
% \vspace{12pt}
% \textbf{Objective Function:} 
% \hspace{24pt} $\mathbb{L}(t) = \frac{1}{N} \sum_{i=1}^{N} \ln \Big(\sum_{j=1}^{K} - \mathbb{I}(y_i=j) \cdot c_{j}(\mathbf{p}_i; t)\Big)$


% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/ts_c1.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/ts_c2.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/ts_c3.png}
% \end{figure}
% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/ts_map_c1.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/ts_map_c2.png}\hfill
% \includegraphics[width=0.33\textwidth]{figures/calibrators/ts_map_c3.png}
% \end{figure}

% \subsubsection{Vector Scaling}

% \textbf{Parameters:} 
% \hspace{24pt}Vector: $\mathbf{w} \in \mathbb{R}^{K}$  
% \hspace{24pt}Intercept: $\mathbf{b} \in \mathbb{R}^{K}$ 
% \vspace{12pt}
% \textbf{Predictive Function:} 
% \hspace{24pt}$c_{j}(\mathbf{p}; \mathbf{w}) = \frac{\exp\big(-w_j \cdot \text{logit}_j (p) -b_j\big)}{\sum_{j=1}^{K}\exp\big(-w_j \cdot \text{logit}_j (p) - b_j\big)}$ 
%\vspace{12pt}
% \textbf{Objective Function:} 
% \hspace{24pt} $\mathbb{L}(\mathbf{w}, \mathbf{b})= \frac{1}{N} \sum_{i=1}^{N} \ln \Big(\sum_{j=1}^{K} - \mathbb{I}(y_i=j) \cdot c_{j}(\mathbf{p}_i; \mathbf{w}, \mathbf{b})\Big)$


% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/vs_c1.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/vs_c2.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/vs_c3.png}
% \end{figure}
% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/vs_map_c1.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/vs_map_c2.png}\hfill
% \includegraphics[width=0.33\textwidth]{figures/calibrators/vs_map_c3.png}
% \end{figure}


% \subsubsection{Matrix Scaling}

% \textbf{Parameters:} 
% \hspace{24pt}Matrix: $(\mathbf{w}_1, \cdots, \mathbf{w}_K), \mathbf{w}_j \in \mathbb{R}^K$   
% \hspace{24pt}Intercept: $\mathbf{b} \in \mathbb{R}^{K}$
% \vspace{12pt}
% \textbf{Predictive Function:} 
% \hspace{24pt}$c_{j}(\mathbf{p}; \mathbf{w}_1, \dots, \mathbf{w}_{K}, \mathbf{b}) = \frac{\exp\big(-\mathbf{w}_j^T \text{logit}( \mathbf{p}) - b_j\big)}{\sum_{j=1}^{K}\exp\big(-\mathbf{w}_j^T \text{logit}( \mathbf{p}) - b_j\big)}$ 
% \vspace{12pt}
% \textbf{Objective Function:} 
% \hspace{24pt} $\mathbb{L}(\mathbf{w}_1, \dots, \mathbf{w}_K, \mathbf{b})= \frac{1}{N} \sum_{i=1}^{N} \ln \Big(\sum_{j=1}^{K} - \mathbb{I}(y_i=j) \cdot c_{j}(\mathbf{p}_i; \mathbf{w}_1, \dots, \mathbf{w}_K, \mathbf{b})\Big)$

% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/ms_c1.png}\hfill
% \includegraphics[width=0.28\t\extwidth]{figures/calibrators/ms_c2.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/ms_c3.png}
% \end{figure}

% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/ms_map_c1.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/ms_map_c2.png}\hfill
% \includegraphics[width=0.33\textwidth]{figures/calibrators/ms_map_c3.png}
% \end{figure}

% \subsubsection{Dirichlet Calibration}

% \textbf{Parameters:} 
% \hspace{24pt}Coefficients: $(\mathbf{w}_1, \cdots, \mathbf{w}_K), \mathbf{w}_j \in \mathbb{R}^K$  
% \hspace{24pt}Intercept: $\mathbf{b} \in \mathbb{R}^{K}$ 
% \vspace{12pt}
% \textbf{Predictive Function:} 
% \hspace{24pt}$c_{j}(\mathbf{p}; \mathbf{w}_1, \dots, \mathbf{w}_{K}, \mathbf{b}) = \frac{\exp(-b_j - \mathbf{w}_j^T \ln \mathbf{p})}{\sum_{j=1}^{K}\exp(-b_j-\mathbf{w}_j^T \ln \mathbf{p})}$
% \vspace{12pt}
% \textbf{Objective Function:} 
% \hspace{24pt} $\mathbb{L}(\mathbf{w}_1, \dots, \mathbf{w}_K, \mathbf{b})= \frac{1}{N} \sum_{i=1}^{N} \ln \Big(\sum_{j=1}^{K} - \mathbb{I}(y_i=j) \cdot c_{j}(\mathbf{p}_i; \mathbf{w}_1, \dots, \mathbf{w}_K, \mathbf{b})\Big)$

% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/dir_c1.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/dir_c2.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/dir_c3.png}
% \end{figure}
% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/dir_map_c1.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/dir_map_c2.png}\hfill
% \includegraphics[width=0.33\textwidth]{figures/calibrators/dir_map_c3.png}
% \end{figure}

% \subsection{Notable Mentions}

% \begin{itemize}
% \item \cite{naeini2015}
% \item \cite{milios2018}
% \item \cite{allikivi2019}
% \item \cite{Kumar2018}
% \item \cite{Wenger2020}
% \item \cite{Kuleshov2018}
% \item \cite{song2019}
% \item \cite{widmann2019}
% \end{itemize}

% \subsection{Regularisation and Bayesian Treatments}

% \begin{itemize}
%     \item Typical approaches are generally easy to adopt: $L_{0}$, $L_{1}$, $L_2$, lasso, ridge, as well as common Bayesian inference with certain priors on the parameters. 
    
%     \item In Dirichlet calibration, the authors proposed an off-diagonal L2 regularisation approach for Dirichlet calibration, which improves the generalisation of calibration for deep nets by limiting the pair-wise interaction among different classes.
% \end{itemize}


% \subsection{Implementation}

% There are also some common practices when implementing a calibration approach:
% \begin{itemize}
% \item Have multiple inner folds to train the base model and calibrators separately
% \item Approaches including Beta, Dirichlet, and matrix scaling can be easily trained with existing logistic regression implementations.  
% \item For calibrators with a convex loss, when the number of data points and classes is manageable, explicit Newton approaches is generally better than stochastic optimisation.
% \end{itemize}

% \subsection{Wrap Up}

% \subsubsection{Lessons learned}

% To select a suitable calibrator, consider the following:
% \begin{itemize}
% \item Do you care about the entire probability vector or just about a single class? (the latter $\rightarrow$ binary approaches)
% \item Do you have a large calibration set? (yes $\rightarrow$ non-parametric approaches)
% \item Do you have a small calibration set? (yes $\rightarrow$ consider regularisation)
% \item Are you only interested in certain probability values? (yes $\rightarrow$ binning approaches)
% \end{itemize}


==> 05_advanced_topics.tex <==
% \section{Advanced topics}
% \label{sec:out:conc}

% Now that we are nearing the end of this survey we will briefly discuss some more advanced topics related to post-hoc calibration.
% Section~\ref{sec:hyp} gives an introduction to statistical tests for calibration.
% Section~\ref{sec:costs} provides an alternative, cost-based view of the problem of classifier calibration, and discusses the need of calibration from the point of decision theory.
% In Section~\ref{sec:regcal} we consider what it means to calibrate in regression.
% Finally, section~\ref{sec:conclusion} concludes the paper.

\section{Hypothesis tests for calibration}
\label{sec:hyp}
%----------------------------------------------------%

Even if a classifier is perfectly calibrated, it almost always slightly deviates from calibration on any finite dataset due to sampling effects.
Here we consider a method of testing whether the dataset provides sufficient evidence that the classifier is uncalibrated. 

\newtext{A common way to test for calibration is to apply goodness-of-fit tests that were originally proposed for logistic regression models, but can be extended to any model that predicts probabilities. For example, one could apply the Pearson chi-squared goodness-of-fit test, which works by grouping instances sharing the same value of the independent variable $X$ and then applying a chi-squared test under the null hypothesis that the observed number of positives in the target variable is equal to the predicted number of positives for each unique value of $X$.}

\newtext{The issue with this approach is that the higher the number of unique values of $X$ or the higher the number of combinations of values of multiple independent variables, the lower the probability that each group of instances will be well-represented enough for the calculation of the Pearson chi-squared statistic to be reliable. A possible solution to this problem is to group instances into $M$ bins based on percentiles of the predicted probabilities for the positive class (equal-frequency binning) and then apply the Hosmer-Lemeshow (HL) test, which involves calculating the statistic $H$ given by Equation (\ref{eq:hosmer-lemeshow}) \cite{Hosmer2003applied}.} 

\newtext{
\begin{equation}
\label{eq:hosmer-lemeshow}
H = \sum_{m=1}^{M} \left(\frac{\left(O_{m+} - E_{m+}\right)^2}{E_{m+}}+\frac{\left(O_{m-} - E_{m-}\right)^2}{E_{m-}} \right),
\end{equation}
}
\newtext{
\noindent where $O_{m+}$ and $O_{m-}$ are the observed counts of positives and negatives in bin $\mathbb{B}_{m}$ and $E_{m+}$ and $E_{m-}$ are the expected counts of positives and negatives in bin $\mathbb{B}_{m}$, calculated as the sums of positive and negative probabilities in the bin, respectively.
}

\newtext{The HL test was later extended to evaluate the goodness-of-fit of multinomial logistic regression models, by binning instances based on the percentiles of $\sum_{j=2}^K s_{ij} = 1 - s_{i1}$, i.e. the complement of the probabilities assigned to the reference class \cite{fagerland2008multinomial}. Then, similarly to the binary case, once the instances are binned, we calculate $O_{mj}$ and $E_{mj}$, respectively the observed and expected counts for each class $j$ and bin $m$. Finally we calculate the $C$ statistic, given by Equation (\ref{eq:hosmer-lemeshow:C}), which is expected to follow a chi-squared distribution with $(M-2)(K-1)$ degrees of freedom.}

\newtext{
\begin{equation}
\label{eq:hosmer-lemeshow:C}
C = \sum_{m=1}^{M}\sum_{j=1}^{K} \left(\frac{\left(O_{mj} - E_{mj}\right)^2}{E_{mj}}+\frac{\left(O_{mj} - E_{mj}\right)^2}{E_{mj}} \right).
\end{equation}
}

\newtext{Table \ref{tab:hosmer:lemeshow} shows $M=5$ bins based on the toy example of Table \ref{tab:evaluation:toy}. By applying Equation (\ref{eq:hosmer-lemeshow:C}) to these values, we get $C = 25.3$. Finally, to complete the HL test under the null hypothesis that the observed and expected proportions are the same, we compare $C$ to a chi-squared distribution with $(M-2)(K-1) = 6$ degrees of freedom, obtaining a p-value of $0.0003$, rejecting the null hypothesis with $\alpha=0.05$.}

\begin{table}[ht]
    \centering
    \small

    \begin{tabular}{llrrrrrr}
    \toprule
    $\mathbb{B}_{m}$ &    $\mathsf{s}(\mathbb{B}_{m})$ &  $O_{m1}$ &       $E_{m1}$ &  $O_{m2}$ &       $E_{m2}$ &  $O_{m3}$ &     $E_{m3}$ \\
    \midrule
    $\mathbb{B}_{1}$ &  $[0.0, 0.2]$ &  $3.0$ &  $5.9$ &  $1.0$ &  $0.7$ &  $3.0$ &  $0.4$ \\
    $\mathbb{B}_{2}$ &  $(0.2, 0.56]$&  $2.0$ &  $3.1$ &  $2.0$ &  $0.6$ &  $1.0$ &  $1.3$ \\
    $\mathbb{B}_{3}$ &  $(0.56, 0.7]$&  $3.0$ &  $2.47$ &  $3.0$ &  $1.77$ &  $1.0$ &  $2.77$ \\
    $\mathbb{B}_{4}$ &  $(0.7, 0.9]$ &  $2.0$ &  $1.1$ &  $3.0$ &  $3.1$ &  $2.0$ &  $2.8$ \\
    $\mathbb{B}_{5}$ &  $(0.9, 1.0]$ &  $0.0$ &  $0.0$ &  $1.0$ &  $1.2$ &  $3.0$ &  $2.8$ \\
    \bottomrule
    \end{tabular}
    \caption{\newtext{Instances grouped into 5 bins using equal-frequency binning on the complement of the probabilities predicted for class 1. Column $\mathsf{s}(\mathbb{B}_{m})$ shows the probability intervals corresponding to each bin. The probabilities were obtained by considering the multiclass toy problem in Table \ref{tab:evaluation:toy}.}}
        \label{tab:hosmer:lemeshow}
\end{table}

\newtext{This example is of course simply illustrative, as the HL test is not recommended for such small samples, as experiments have shown that it has satisfactory power for samples of over 400 instances \cite{fagerland2008multinomial}. There are several other goodness-of-fit tests, most of them using some sort of binning to calculate a statistic that is assumed to follow a chi-squared distribution. Additionally, as the multiclass HL test, they usually test for classwise calibration. Testing for multiclass calibration is a more complex task and has recently been investigated by \citet{widmann2019calibration}, by using kernel-based measures. These measures were later adapted for regression calibration \cite{widmann2022calibration}. For  details on how these measures can be interpreted as test statistics, we refer the reader to their original papers.}

\newtext{Another approach, proposed by \citet{vaicenavicius2019evaluating}, is to test the classifier's probabilities according to an arbitrary measure of calibration.}
Given a classifier $\mathsf{f}$, we can check if its predictions for a test set $\{(\boldsymbol{x}_1, y_1), \dots, (\boldsymbol{x}_N, y_N)\}$ are calibrated according to a chosen calibration measure $\phi(\mathsf{f}(\mathbf{X}_{\text{test}}),\mathbf{\dot{Y}}_{\text{test}})$, such as ECE, log-loss or Brier score. We discuss a simple resampling-based hypothesis test under the null hypothesis that the classifier's outputs are calibrated \cite{vaicenavicius2019evaluating}. Algorithm \ref{alg:test:steps} details the steps of the hypothesis test procedure.

\begin{algorithm}[H]
		\caption{Hypothesis test for calibration}
		\label{alg:test:steps}
		\begin{algorithmic}[1]
			\Require Test predictions $\mathsf{f}(\mathbf{X}_{\text{test}})$; test set labels $\mathbf{\dot{Y}}_{\text{test}}$, Calibration measure $\phi$; Number of resampled label sets $L$; Significance level $\alpha$;
			
			\For { l=1:L}
			\State Sample $\boldsymbol{y}_l$, $l \in \{1, \ldots, L\}$, such that each $y_{l,i} \sim \mathsf{Cat}(\mathsf{f}(\mathbf{\hat{x}}_i))$;
			\State $\phi_s \leftarrow \phi\left(\mathsf{f}(\mathbf{X}_{\text{test}}),\mathbf{\dot{Y}}_l\right)$;
			\EndFor
		
			\State $\text{p-value} \leftarrow \text{proportion of $\phi_l$ among $\phi_1,\dots,\phi_L$ with}\ \phi_l > \phi\left(\mathsf{f}(\mathbf{X}_{\text{test}}),\mathbf{\dot{Y}}_{\text{test}}\right)$;
			
			\If {$\text{p-value} < \alpha$}
			\State Reject the null hypothesis and conclude that the classifier is not calibrated;
			\Else
			\State Accept the null hypothesis, i.e. there is not enough evidence that the classifier is not calibrated.
			\EndIf
		\end{algorithmic}
\end{algorithm}

Let us return to our toy example (Table \ref{tab:evaluation:toy}). If we follow Algorithm \ref{alg:test:steps} and choose $\mathsf{ECE}_{\text{classwise}}$ as the calibration measure and $L=1,000$, we obtain a distribution such as the one in Figure \ref{fig:eval:loss-distribution}. 

% First, we generate $S$ bootstrapped label sets $\boldsymbol{y}_s$, $s \in \{1, \ldots, S\}$, such that each $y_{s,i}$ is sampled from $\boldsymbol{\hat{p}}(\boldsymbol{\hat{x}}_i)$. Then we calculate $\phi(\boldsymbol{\hat{p}}(X_{\text{test}}), \boldsymbol{y}_s)$ for each label set $\boldsymbol{y}_s$, which gives us a distribution such as the one in Figure \ref{fig:eval:loss-distribution:a}.

% \begin{figure}
%         \centering
%         \includegraphics[width=0.7\textwidth]{figures/evaluation/loss-distribution.png}
%         \caption{Distribution of $\text{classwise-ECE}$ values calculated for every bootstrapped label set $\boldsymbol{y}_s$ with $s \in \{1, \ldots, S\}$, following the procedure described in Algorithm \ref{alg:test:steps}.}
%         \label{fig:eval:loss-distribution}
%     \end{figure}

\begin{figure}[!t]
    \centering
%    \begin{subfigure}{0.45\linewidth}
%    \includegraphics[width=\linewidth]{figures/evaluation/loss-distribution.png}
%    \caption{Distribution of loss values.}
%    \label{fig:eval:loss-distribution:a}
%    \end{subfigure}
%    \begin{subfigure}{0.45\linewidth}
%    \includegraphics[width=\linewidth]{figures/evaluation/loss-distribution-p-value.png}
%    \caption{Red bars represent $\phi_l >  0.1787$.}
%    \label{fig:eval:loss-distribution:b}
%    \end{subfigure}    
    \includegraphics[width=0.6\linewidth]{loss-distribution-p-value.png}
    \caption{Distribution of $\mathsf{ECE}_{\text{classwise}}$ values $\phi_1,\dots,\phi_L$ calculated for every resampled label set $\mathbf{\dot{Y}}_l$ with $l \in \{1, \ldots, L\}$, following the procedure described in Algorithm \ref{alg:test:steps}. The red bars represent the region where $\phi_l >  0.1787$.}\label{fig:eval:loss-distribution}
\end{figure}


Recall that in our example $\mathsf{ECE}_{\text{classwise}} = 0.1787$. The p-value for this test is then $\mathsf{P}\Big(\phi_l >  0.1787\Big) \approx 0.016$, which means we can reject the null hypothesis that the classifier is calibrated according to $\mathsf{ECE}_{\text{classwise}}$. Note that we keep the scores fixed and only resample the labels to perform this test. This means that instances will stay in the same bins and small bins will have low weights for all $L$ resampled $\mathsf{ECE}_{\text{classwise}}$ values.




% Now let the value of the arbitrary loss measure for the test set be $\phi(\boldsymbol{\hat{p}}(X_{\text{test}}), \boldsymbol{y}_{\text{test}}) = 0.32$. We calculate the p-value for the test as $P\Big(\phi(\boldsymbol{\hat{p}}(X_{\text{test}}), \boldsymbol{y}_s) > 0.32\Big) \approx 0.26$, which is equivalent to the red area in Figure \ref{fig:eval:loss-distribution:b}. Thus, we cannot reject the null hypothesis in this example, and this classifier would be considered calibrated.


% \subsection{A cost-based view of classifier calibration}
% \label{sec:costs}
%So far we have framed calibration as aiming to get as close as possible to the Bayes-optimal classifier, predicting the `true' $\mathsf{P}(y|x)$.
%That is, we want the probabilities estimated by a predictive model to match the observed frequencies as closely as possible. 
% One of the scenarios where calibrated probabilities are particularly required is cost-sensitive decision making, where the aim is to minimise the expected cost of misclassifications, given the cost matrix specifying the cost of predicting class $i$ for an instance of class $j$ for any classes $i$ and $j$.
% In Section~\ref{sec:2:1} \todo[inline]{Fix reference to sec:2:1. A closer look at calibration, and why it matters}, we saw that in binary classification the optimal threshold for the Bayes-optimal model $\mathsf{P}(+|\mathbf{x})$ is equal to $c=\frac{\mathsf{C}(+|-)}{\mathsf{C}(+|-)+\mathsf{C}(-|+)}$, where $\mathsf{C}(+|-)$ and $\mathsf{C}(-|+)$ are the costs of a false positive and a false negative, respectively.
% We will refer to $c \in [0, 1]$ as the cost proportion.
%It is also possible to justify the need of calibration from a decision-theoretic point of view.
% Let us now investigate what the optimal threshold is for non-optimal classifiers. 
%In the context of binary classification, we need to decide which class to predict for any score $s$, and our aim is to minimise some given objective on the dataset.
% Among all the possible values of predicted positive class probability $s$, the optimal threshold $s_{\text{dec}}$ is such that the expected misclassification cost is the same regardless of which class is predicted:
%
%When the evaluation metric is accuracy, an intuitive location for the decision boundary is where both classes are equally likely on the particular score.
%This condition explicitly suggests the calibrated probability of $0.5$.
%
%Now we move to a more comprehensive setting.
%Let $c_{FP}$ denote the instance-wise cost for making a false positive prediction, and $c_{FN}$ the instance-wise cost for a false negative prediction.
%Denoting the Recall that the decision boundary $s_{\text{dec}}$ is where it makes no difference to predict either class, which suggests:
%
% \begin{align}
% \label{eq:samecost}
%     P(Y=+ \mid s_{\text{dec}}) \mathsf{C}(-|+) = P(Y=- \mid s_{\text{dec}})  \mathsf{C}(+|-)
% \end{align}
% but additionally, we also need to require that scores higher than $s_{\text{dec}}$ would be more likely positives and scores lower than $s_{\text{dec}}$ would be less likely positives (known as the requirement of being classification-calibrated at $s_{\text{dec}}$ \citep{nguyen2009surrogate}):
% \begin{align*}
%     \label{eq:dec}
%     P(Y=+ \mid s') &> P(Y=+ \mid s_{\text{dec}}) \quad \forall s' > s_{\text{dec}} \\
%     P(Y=+ \mid s') &< P(Y=+ \mid s_{\text{dec}}) \quad \forall s' < s_{\text{dec}} \nonumber
% \end{align*}
% The requirement (\ref{eq:samecost}) that the expected misclassification cost is the same regardless of which class is predicted can be rewritten as
% \begin{align*}
%     P(Y=+ \mid s_{\text{dec}}) \mathsf{C}(-|+) = \Big(1 - P(Y=+ \mid s_{\text{dec}}) \Big) \mathsf{C}(+|-)
% \end{align*}
% leading to
% \begin{align*}
%     \quad P(Y=+ \mid s_{\text{dec}}) = \frac{\mathsf{C}(+|-)}{\mathsf{C}(+|-) + \mathsf{C}(-|+)}=c
% \end{align*}
%
%Since both costs can be assumed to be positive, we can normalise it as the relative misclassification cost:
%
%\begin{align*}
%    c = \frac{c_{FP}}{c_{FP} + c_{FN}}
%\end{align*}
%
% The corresponding decision threshold $s_{\text{dec}}$ for a given $c$ is then such that:
%
% \begin{align*}
%    P(Y=+ \mid s_{\text{dec}}) = c
% \end{align*}
% If the scoring classifier is perfectly calibrated, then $P(Y=+ \mid s_{\text{dec}})=s_{\text{dec}}$. From this we can conclude that for calibrated classifiers the optimal 
% decision threshold is $s_{\text{dec}}=c$, which is the same optimal threshold as for the Bayes-optimal classifier.

%Next, we will continue on binary classification and cover the definitions of classification-calibrated and ranking-calibrated, which are both weaker concepts than class probability calibration.
%While the decision boundary only suggests that it makes no difference to predict either class given the particular score, it can help us to determine the predictions for other scores when the following conditions are met (referred to as being classification-calibrated on $s_{\text{dec}}$ by \citet{nguyen2009surrogate}):
%
%\begin{align}
%    \label{eq:dec}
%    P(Y=+ \mid s') &> P(Y=+ \mid s_{\text{dec}}) \quad \forall s' > s_{\text{dec}} \\
%    P(Y=+ \mid s') &< P(Y=+ \mid s_{\text{dec}}) \quad \forall s' < s_{\text{dec}} \nonumber
%\end{align}
%
%That is, given any other score $s'$, the probability of $P(Y=+ \mid s')$ will be larger than $P(Y=+ \mid s_{\text{dec}})$ is $s' > s_{\text{dec}}$, and vice versa.
%In this case, we can simply predict positives for every score that is larger than $s'$, and predict negative otherwise. 
%Therefore, if we have a cost proportion $c$, and the two conditions in Equation~(\ref{eq:dec}) are met, then the optimal threshold $s_{dec}$ is the score that has a calibrated probability of $c$.


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.35\textwidth]{figures/conclusion/rel.png}\hfill
%     \includegraphics[width=0.5\textwidth]{figures/conclusion/brier_curve.png}
%     \caption{({Left}) The reliability diagrams of the same logistic classifier that are respectively uncalibrated and perfectly post-calibrated. ({Right}): The corresponding Brier curves. The area under the blue curve is the refinement loss of both classifiers, and the area between the red and blue curves is the calibration loss of the uncalibrated model.}
%     \label{fig:brier_curve}
% \end{figure}


% At first sight, calculating misclassification cost based on costs of false positives and false negatives is quite a different way of evaluating a classifier than proper scoring rules.
% Interestingly though, connections can be made between them.
% Suppose we consider different cost scenarios with different values of the cost proportion $c$, but only such that the cost of a false positive and a false negative add up to $2$, that is $\mathsf{C}(+|-)+\mathsf{C}(-|+)=2$.
% Here requiring the sum to be equal to $2$ ensures that the error rate is among the considered scenarios, as then $\mathsf{C}(+|-)=\mathsf{C}(-|+)=1$.
% Let us always pick the decision threshold assuming that the scoring classifier is perfectly calibrated, i.e. $s_{\text{dec}}=c$, even if actually the classifier is not calibrated.
% Then the \emph{Brier curve} is the result of plotting average misclassification cost per instance denoted as $L(c)$ against the cost proportion $c$ 
%  \cite{hernandez-orallo2011}, where $L(c)$ is defined as: 
% \begin{align*}
% L(c)=\frac{1}{n}\sum_{i=1}^n \mathsf{C}(+|-)\mathsf{I}(\hat{y}_i=+,y_i=-)+\mathsf{C}(-|+)\mathsf{I}(\hat{y}_i=-,y_i=+)
% \end{align*}
% and $\mathsf{C}(+|-)=2c$, $\mathsf{C}(-|+)=2(1-c)$. 
% Denote $\pi$ as the marginal probability for the positive class, $\mathit{fpr}(s_{dec})$ and $\mathit{tpr}(s_{dec})$ as the false positive rate and true positive rate at threshold $s_{dec}$. 
% The normalised optimal cost can then be derived as \cite{hernandez-orallo2012}:
% %
% \begin{align*}
%     L_c(s_{dec}) = 2c(1-\pi)\mathit{fpr}(s_{dec}) + 2(1-c)\pi(1 - \mathit{tpr}(s_{dec}))
% \end{align*}
% %
% Denote $\hat{Y}$ as the predicted label, here $(1-\pi)\mathit{fpr}(s_{dec})$ is the probability of false positive $P(Y=-, \hat{Y}=+)$, and $\pi(1 - \mathit{tpr}(s_{dec}))$ is the probability of false negative $P(Y=+, \hat{Y}=-)$. 
% A factor of $2$ is added to mimic the common definition of error rate, which corresponds to the case of $c = 0.5$ (i.e. a false positive has the same cost as a false negative).
% 
% While the above threshold $s_{\text{dec}}$ and cost are only optimised for the specific cost proportion $c$, it would be desirable if the classifier can provide scores that can be optimised with any potential cost proportion $c \in [0, 1]$.
% In this case, we want the conditions in Equation~(\ref{eq:dec}) to be met with any $s_{dec} $ (hence $c$), leading to the following definition.
% %
% \textit{Ranking calibration}: Denote a scoring binary classifier as $\mathsf{f}: \mathbb{X} \rightarrow \mathbb{R}$, $s_1, s_2 \in \mathbb{R}$ are two independent model output values, the classifier is ranking-calibrated if the following condition is met:
% %
% \begin{align}
%     P(Y=+ \mid s_1) \geq P(Y=+ \mid s_2)  \quad \forall s_1 \geq s_2
% \end{align}
% %
% With a ranking-calibrated classifier, we can simply find the $s_{\text{dec}}$ with any given cost proportion $c$.
% 
% This procedure can be further simplified by assuming $s$ are probability-calibrated scores, which is a sufficient condition to be ranking-calibrated:
% %
% \begin{align*}
%     P(Y=+ \mid s) = s  \quad \forall s \in [0, 1]
% \end{align*}
% %
% With calibrated scores, given any cost proportion $c$, we always have $s_{\text{dec}}=c$, and the optimal cost is hence:
% %
% \begin{align*}
%     L_c(c) = 2c(1-\pi)\mathit{fpr}(c) + 2(1-c)\pi(1 - \mathit{tpr}(c))
% \end{align*}
% 
% 
% Since the cost now only depends on $c$, it is possible to plot $L(c)$ as a scalar function of $c$, and such a visualisation is known as cost curves.
% The Brier curve plots $L(c)$ against $c$ \cite{hernandez-orallo2011}. 
% Brier curves are a particular kind of cost curve \cite{drummond2006}.
% These Brier curves have several useful properties:
% (1) The area under the Brier curve (i.e., the expected loss over uniform $c$) is equal to the Brier score, making a connection between the cost perspective and the proper scoring rule perspective; 
% (2) Among all possible score transformations, a perfectly calibrated classifier has the lowest possible Brier curve (lower envelope);
% (3) The areas between and under the Brier curves before and after perfectly calibrating are corresponding to the decomposition of Brier score into refinement loss and calibration loss. 

% Example Brier curves are given in Figure~\ref{fig:brier_curve}.
% We again consider a synthetic dataset where we can have as many data points as necessary to ensure a classifier can be nearly calibrated everywhere.
% As indicated by the left figure, we have a logistic classifier trained on the synthetic dataset, resulting in uncalibrated probabilities as depicted by the red reliability diagram.
% With unlimited data points, we then calibrate the classifier to be close to perfectly calibrated, and the corresponding blue reliability diagram follows the ascending diagonal.
% For the right figure, we see that the blue curve has a smaller area under it, which indicates a smaller Brier score.
% Since the blue curve is from a perfectly calibrated model, this area is also equivalent to the refinement loss of the model as calculated by the Brier score.
% The area between the two curves is therefore the calibration loss of the uncalibrated model.
% \citet{flach2015lmce} demonstrates that this construction carries over to other proper scoring rules. 



% \subsection{Beyond the calibration of label probabilities}
% \label{sec:beyond}
% 
% While we have been mainly addressing calibration of label probabilities in the classification context, the notion of calibration can be generalised to various tasks beyond standard probabilistic classification.
% 
% \subsubsection*{Probability calibration for optimal decisions with F-score}
% 
% When we discussed the cost-sensitive view of calibration in the previous section, we saw that the decision boundary under a standard accuracy setting (equal misclassification cost) is the calibrated probability of $0.5$.
% Furthermore, if we have a classifier that is calibrated for a specific probability value of $p$, it will be the corresponding decision boundary if we assume the negatives are $\frac{p}{1-p}$ times more important than positives.
% This assumption leads to a modified version of the accuracy measure, known as the weighted accuracy:
% %
% \begin{align*}
%     \mathit{acc}_{p}(t) = 2p(1 - \pi)\mathit{tnr}(t) + 2(1-p)\pi \mathit{tpr}(t)
% \end{align*}
% 
% By varying the value of $p$, we provide a cost-sensitive trade-off between true positives and true negatives, which further implies a trade-off between precision and recall.  
% In the extreme case, if we only care about the positives, that is, we can have $p$ getting close to $0$, and it means negatives are $\frac{p}{1-p} \rightarrow 0$ times more important than positives.
% With this setting, we can see the decision boundary will be the calibrated probability of $0$ and we will have a weighted accuracy of $1$.
% As a result, this decision boundary will lead to a recall of $1$ and a precision of $\pi$, which corresponds to a always-positive classifier.
% 
% Since the results above indicate a specific trade-off between precision and recall, it is more interpretable to use the $F_{\beta}$ score as a evaluation metric, as it includes both the precision and recall terms:
% %
% \begin{align*}
%     F_{\beta}(t) &= \frac{1}{\fracii{\frac{1}{1+\beta^2}}{\text{prec(t)}} + \fracii{\frac{\beta^2}{1+\beta^2}}{\text{rec(t)}}} \\
%     &= \frac{(1+\beta^2)\text{TP}(t)}{(1+\beta^2)\text{TP}(t) + \text{FP}(t) + \beta^2 \text{FN}(t)}
% \end{align*}
% %
% While $F_{\beta}$ is the standard form of the F-score, it is often more convenient to have a $[0, 1]$ weight $d = \frac{1}{1 + \beta^2}$, leading to the following re-parameterised version:
% %
% \begin{align*}
%     F_{d}(t) &= \frac{1}{d\frac{1}{\text{prec}(t)} + (1-d)\frac{1}{\text{rec}(t)}} \\
%     &= \frac{\text{TP}(t)}{\text{TP}(t) + d \text{FP}(t) + (1-d)\text{FN}(t) }
% \end{align*}
% 
% \begin{figure}[!b]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/conclusion/fig2-left.pdf}
%     \includegraphics[width=0.45\textwidth]{figures/conclusion/fig2-right.png}
%     \caption{({Left}): precision-recall curve, ({Right}) precision-recall-gain curve.}
%     \label{fig:pr_prg}
% \end{figure}
% 
% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/conclusion/PRG2.png}
%     \includegraphics[width=0.45\textwidth]{figures/conclusion/PRG3.png}
%     \caption{({Left}) Calibration for weighted accuracy with ROC curve, ({Right}) Calibration for $F_{\beta}$-score with precision-recall-gain curve.}
%     \label{fig:prg}
% \end{figure}
% 
% The question is now: how to calibrate a probabilistic classifier so that instances with a score value of $d$ will be on the $F_{d}$ decision boundary? 
% \citet{flach2015} address this problem by means of a non-linear transformation of the measures involved.
% We have seen that the conventional ROC curve can be used for calibrating probabilities by constructing the ROC convex hull, which is equivalent to isotonic regression.
% However, the traditional precision-recall curve is not sufficiently similar to a ROC curve to allow a similar calibration property.
% In contrast, the precision-recall-gain curve proposed by \citet{flach2015} can be seen as a proper generalisation of ROC curve obtained by replacing weighted accuracy with F-score.
% Figure~\ref{fig:pr_prg} gives a comparison between the precision-recall curve and the precision-recall-gain curve.
% Figure~\ref{fig:prg} exemplifies the calibration procedure for both the ROC curve and the precision-recall-gain curve.
% As indicated by the figures, unlike the traditional precision-recall curve, precision-recall-gain curve can be used together with the convex hull method to achieve calibration on any given $F_{\beta}$ score, as with the ROC curve with weighted accuracy.  

% \subsection{Calibration for regression}
% \label{sec:regcal}

% While in this survey we have focused on the cases where the target variable is discrete, the notion of calibration is also applicable to the continuous regression case.
% As in the classification scenario, there are multiple definitions of calibration for regression models.

% We first introduce the concept of quantile calibration.
% We denote a quantile regression model as $g: \mathbb{X} \times [0, 1] \rightarrow \mathbb{R}$, which takes a feature vector $\mathbf{x}$ and a value $\tau \in [0, 1]$, and outputs the estimated $\tau$-quantile value $\hat{y}$ so that $P(Y \leq \hat{y} \mid \mathbf{X}=\mathbf{x}) = \tau$. 
% The quantile regression model is defined as \emph{quantile-calibrated}, if and only if
% for $\forall \tau \in [0, 1]$, the following is satisfied: 
% %
% \begin{align*}
%     P\Big(Y \leq g(\mathbf{X}, \tau) \Big) = \tau \qquad \text{for } \forall \tau \in [0, 1]
% \end{align*}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.95\textwidth]{figures/conclusion/quantile_example.png}
%     \caption{An example of quantile calibration, calibrating the quantiles corresponding to $\tau=0.05,0.75,0.9$ (left plot) using a calibration map (middle plot) into quantiles corresponding to $\tau=0.1,0.5,0.8$ (right plot). }
%     \label{fig:quanitle}
% \end{figure}

% Following this definition, we can investigate how to calibrate a quantile regression model within a post-hoc setting.
% Since all possible quantiles are in the interval of $[0, 1]$, \citet{kuleshov2018} propose to adopt existing binary calibrators to adjust the quantiles.
% This procedure is demonstrated in Figure~\ref{fig:quanitle}.

% \subsubsection*{Distribution calibration for regression}

% Unlike calibration as defined for classifiers, quantile calibration for regression is defined globally across all predictions, and has no requirements on the individual prediction produced by the regression model.   
%
% To mimic the same level of calibration as in classification, \citet{pmlr-v97-song19a} introduce a stronger definition known as distribution calibration for regression. 
% If we denote a regression model (or conditional density estimator) as $$f: \mathbb{X} \rightarrow \{s \mid s:\mathbb{R} \rightarrow [0, \infty), \int s(y)dy = 1 \}$$ then this model is defined as \emph{distribution-calibrated}, if and only if
% for $\forall s :\mathbb{R} \rightarrow [0, \infty), \int s(y)dy = 1$, the following holds: 
%
% \begin{align*}
%     P\Big(Y=y \mid f(\mathbf{X}) = s) \Big) = s(y) \qquad \text{for } \forall s :\mathbb{R} \rightarrow [0, \infty), \int s(y)dy = 1
% \end{align*}
%
% Being distribution-calibrated is a sufficient but not necessary condition for being quantile-calibrated \citep[][Theorem 1]{pmlr-v97-song19a}.

% Figure~\ref{fig:dist} gives an illustration of the differences between quantile calibration and distribution calibration.
% Quantile-calibrated regression considers the global quantiles, and distribution-calibrated regression further models local distributions.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.65\textwidth]{figures/conclusion/regression_example.png}
%     \caption{The difference between distribution calibration and quantile calibration.}
%     \label{fig:dist}
% \end{figure}

% Alternative concepts of regression calibration also exist, including conformal prediction \cite{romano2019conformalized} and threshold calibration \cite{sahoo3reliable}. 
%\todo{This citation is incomplete (missing year)}




% \newtext{Will work on this in a few hours \begin{itemize}
%         \item There are various ways to visualise and quantify calibration
%         \item ECE measures aim at producing an aggregate measure of the visual information provided in reliability diagrams
%         \begin{itemize}
%             \item Thus, their optimisation is not guaranteed to produce desirable classifiers
%         \end{itemize}
%         \item Proper scoring rules measure different aspects of probability correctness
%         \begin{itemize}
%             \item They have been used as training losses in classifier training for a while
%             \item But they cannot tell ``where'' the model is more miscalibrated
%         \end{itemize}
%         \item Finally, the hypothesis test for calibration can help determine if a particular loss value means that the classifier is calibrated or not
%     \end{itemize}}


==> 06_conclusion.tex <==
\section{Concluding remarks}
\label{sec:conclusion}

In this survey we have given a detailed overview of the principles and practice of classifier calibration.
We discussed the motivation, definition, evaluation and related approaches for the calibration of probabilistic classifiers, and touched upon topics beyond the standard classification setting.
With the recent proliferation of predictive machine learning, it is becoming more and more important that models are carefully evaluated and if possibly improved on multiple criteria to ensure the overall system robustness.
Classifier calibration relates to the criterion of uncertainty quantification, investigating the statistical relationships between model predictions and observed target variables.
There are other levels of uncertainty in the overall modelling procedure, including uncertainty pertaining to model parameters when the training set is limited, uncertainty brought about by model mismatch, or uncertainty regarding whether the model should abstain when there might be novel target values that were not seen in the training set -- see \cite{hullermeier2021aleatoric} for a recent survey on uncertainty in machine learning. 
% With all of these interesting challenges in mind, we hope this paper can provide a useful reference for researchers and practitioner that are interested in bring predictive machine learning to the next steps.

As we hopefully have made clear in this survey, calibration research has a rich history which predates the birth of machine learning as an academic field by decades. It is important to take full advantage of that history, which perhaps isn't always fully acknowledged in recent literature on classifier calibration (e.g., of deep neural networks, which are often over-confident). Recent proposals such as confidence calibration, temperature scaling and expected calibration error have value but are far from the only options and may not be suitable for a particular application. As is often the case in machine learning, the space of options and things to consider is large, and navigating this space requires the right set of concepts and tools, many of which we have discussed in detail in this survey. 

It is perhaps useful to point out that, naturally, there are also concepts that are less than helpful when thinking about classifier calibration. One of the most prominent of these is the concept of a decision boundary, which is like describing Mount Everest with a single contour line, halfway up. To faithfully characterise the mountain -- which is what is needed for optimal decision making -- one needs many contour lines at different elevations. The only case in which the decision boundary is useful is when the class prior (and misclassification costs, if any) won't change after training, in which case only the decision threshold needs calibrating. In all other cases context change is expected and needs to be anticipated with a proper calibration analysis. 

\newtext{If a trained classifier $f$ is going to be used for a task for which it is good enough to be accurate, precise or to perform well according to any contingency matrix-based measure, then there is no particular need to consider calibration in the model's development pipeline. However, if calibrated probabilities are important for any decisions supported by $f$, the following steps can be taken to implement what was discussed in this paper:}
\newtext{
    \begin{enumerate}
        \item If possible, any classifiers considered for a task should be trained using a proper scoring rule as loss function;
        \begin{itemize}
            \item The resulting models are likely to produce better probabilities than if a non-proper loss function is used, as probability refinement and calibration will be encouraged during training (recall Section \ref{sec:psr});
            \item An alternative is to use a method that encourages calibration during training time, as discussed in Section \ref{sec:cal:training};
        \end{itemize}
        \item With the trained classifiers and, preferably a held-out calibration dataset, the calibration of the probabilities produced by the models can be evaluated using classwise reliability diagrams, to understand the miscalibration patterns, and/or ECE measures (recall Section \ref{sec:metrics});
        \item To help define which models are uncalibrated, a hypothesis test for calibration can be applied (recall Section \ref{sec:hyp});
        \item If any models produce uncalibrated probabilities, post-hoc calibrators should be used to fix them;
        \begin{itemize}
            \item The resulting calibrators should also be evaluated using reliability diagrams, ECE measures and hypothesis tests to find out which ones work best for the particular miscalibration patterns found during step 2.
        \end{itemize}
    \end{enumerate}
}

\newtext{
In order to help with the aforementioned steps, we have developed an open-source Python library called PyCalib \cite{pycalib} \footnote{The documentation of the library can be found at https://classifier-calibration.github.io/PyCalib/}. This library provides tools to measure the calibration quality of a classifier, multiple visualisation functions to better understand how calibrated is a model, and some calibration methods and pipelines to directly train arbitrary calibrated classifiers.
}

\newtext{We close this survey with some open problems. First, although binning is such an important concept in calibration, there is no standard method to decide which type of binning, e.g. equal frequency or equal width, or what number of bins to use. Recent work \cite{kangsepp2022usefulness} has investigated cross-validation to tune the number of bins used to evaluate a model on a calibration set. Second, a recurrent topic of interest is the fact that post-hoc calibration does not improve robustness against out-of-distribution inputs and what can be done to improve calibration in this context \cite{ovadia2019can}. Finally, and somewhat related to the previous point, even though calibrated probabilities provide estimations of the uncertainty regarding an instance's class given its feature values (aleatoric or first-order uncertainty), classifiers could also be made to predict their uncertainty about the predicted probabilities, which comes from not knowing the true probabilities (epistemic uncertainty). This type of prediction, a distribution of distributions, also called second-order uncertainty \cite{hullermeier2022quantifying,bengs2022pitfalls}, has been recently treated using inference based on Bayesian methods and credal sets, which are convex sets of probability distributions \cite{shaker2021ensemble}.}

% Ensure that after lessons learned we add some discussion of current open problems: second-level uncertainty, aleatoric/epistemic uncertainty, out of distribution, better metrics, better binning

%----------------------------------------------------%
% \subsection{Concluding remarks}

% \paragraph{{The myth of the decision boundary}}
%  \begin{itemize}
%     \item \highlighted{red}{Resist} thinking in terms of decision boundaries.
%     \begin{itemize}
%         \item {That is like describing Mount Everest with a single contour line, halfway up.}
%         \item {To faithfully characterise the mountain you need many contour lines at different elevations.}
%     \end{itemize}
%     \item[]
%     \item The \highlighted{red}{only case} in which the decision boundary is useful is when the class prior (and misclassification costs, if any) won't change after training. 
%         \bb{In that case you don't need to calibrate the entire probability range, only the decision threshold.}
% \end{itemize}

% \paragraph{{The long history of classifier calibration}}
%\begin{itemize}
%\item Contrary what recent machine learning literature may lead you to believe, \highlighted{red}{calibration research predates machine learning} and has been studied for three-quarters of a century.
%\item{Make sure you take full advantage of that history, and don't just follow the citations in the latest NeurIPS paper on DNN calibration.}
%\item[]
%\item Recent proposals such as confidence calibration, temperature scaling and expected calibration error have their value, but are far from the only options and may not be suitable for your particular application. 
%\item{Which leads me to\ldots}
% \end{itemize}

% \paragraph{{Calibration is an art as well as a science}}
% Many practical questions don't have \textit{a priori} answers:
%\begin{itemize}
%    \item Which calibration method? 
%    \item How many bins? 
%    \item What evaluation metric? 
%    \item Do I use a validation set? How large? 
%    \item \ldots
% \end{itemize}

%\begin{description}
%    \item[]
%    \item[We hope this tutorial has given you the tools to navigate this space!]
%\end{description}

==> 07_declarations.tex <==
\subsection*{Declarations}

\paragraph{Funding} 
The work of PF, RSR and MPN was supported by the SPHERE Next Steps Project funded by the UK Engineering and Physical Sciences Research Council (EPSRC) [grant EP/R005273/1]. The work of RSR was funded by the UKRI Turing AI Fellowship [grant EP/V024817/1].
The work of PF and HS was supported by The Alan Turing Institute under EPSRC [grant EP/N510129/1].
The work of MK was supported by Estonian Research Council [grant PRG1604].

\paragraph{Conflicts of interest/Competing interests} Not applicable.
\paragraph{Ethics approval} Not applicable.
\paragraph{Consent to participate} Not applicable.
\paragraph{Consent for publication} Not applicable.
\paragraph{Availability of data and material} The availability of data and material used in this survey can be found at \href{https://github.com/classifier-calibration/additional_material}{https://github.com/classifier-calibration/additional\_material}. Further information is available at \href{ https://classifier-calibration.github.io/survey/}{ https://classifier-calibration.github.io/survey/}.
\paragraph{Code availability} The code to generate measurements, visualisation and results is part of \href{https://pypi.org/project/pycalib/}{PyCalib}. Further information can be found in the documentation of the library
\url{https://classifier-calibration.github.io/PyCalib/}.
\paragraph{Authors' contributions}
TSF: conceptualisation, formal analysis, methodology, software, writing (original draft, and review and editing). 
HS: conceptualisation, formal analysis, methodology, software,  writing (original draft, and review and editing). 
MPN: formal analysis, methodology, software, visualisation, writing (original draft, and review and editing). 
RSR: formal analysis, writing (review and editing). 
MK: conceptualisation, formal analysis, methodology, writing (review and editing). 
PF: conceptualisation, formal analysis, methodology, supervision, writing (original draft, and review and editing).
\footnote{The categories follow the CRediT taxonomy: http://credit.niso.org/}


==> Makefile <==
SHELL := /bin/bash

build:
	latexmk -pdf main.tex

autobuild:
	latexmk -pdf -pvc main.tex

showwordcount:
	texcount main.tex chapters/0*.tex frontmatter/*.tex

totalwordcount:
	texcount -sum -1 main.tex chapters/0*.tex frontmatter/*.tex

generatecounttext:
	numwords=$(shell texcount -sum -1 main.tex chapters/0*.tex frontmatter/*.tex); \
	echo Number of words $$numwords; \
	number_to_words $$numwords > frontmatter/word_count.tex;

clean:
	latexmk -c


==> definitions.tex <==
\newcommand{\bb}[1]{
    \begin{itemize}
        \item {#1}
    \end{itemize}
}

% MPN: I am currently ignoring the color
\newcommand{\highlighted}[2]{\textcolor{red}{\textbf{#2}}}
%\setbeamercolor{emph}{fg=ecmlred}
\renewcommand{\cite}[1]{\citep{#1}}

\newcolumntype{L}{>{\raggedright\arraybackslash}X}

% MPN: Allows to align figures
\usepackage[export]{adjustbox}% http://ctan.org/pkg/adjustbox

% MPN: Review modifications
%\newcommand{\newtext}[1]{{
%\leavevmode\color{red}{#1}}}
\newcommand{\newtext}[1]{{#1}}
\newcommand{\done}{\textcolor{green}{\checkmark}}
% Opinion of a reviewer that does not need response
\newcommand{\opinion}[1]{{\fontfamily{qhv}\selectfont
\leavevmode\color{gray}{#1}}}
% Suggestion of a reviewer that requires changes
\newcommand{\suggestion}[1]{{\fontfamily{qhv}\selectfont
\leavevmode\color{black}{#1}}}
% Our response to a suggestion
\newcommand{\response}[1]{{\fontfamily{cmr}\selectfont
\leavevmode\color{green!60!blue}{#1}}}


==> mlj_files/01_intro.tex <==
\section{Introduction and motivation}
\label{sec:intro}


A $K$-class probabilistic classifier is \emph{well-calibrated} if among test instances receiving a predicted $K$-dimensional probability vector $\mathbf{s}$, the class distribution is (approximately) distributed as $\mathbf{s}$.  
This property is of fundamental importance when using a classifier for cost-sensitive classification, for human decision making, or within an autonomous system.
It means that the classifier correctly quantifies the level of uncertainty or confidence associated with its predictions. 
In a binary setting, scores given by a sufficiently calibrated classifier can be simply thresholded to minimise expected misclassification cost. Thresholds can also be derived to optimally adapt to a change in class prior, or to a combination of both. In contrast, for a poorly calibrated classifier the optimal thresholds cannot be obtained without optimisation.

Many machine learning algorithms are known to produce over-confident models, unless dedicated procedures are applied during training. 
%(e.g., Laplace smoothing in decision trees \cite{ferri2003improving}).
The goal of \emph{(post-hoc) calibration methods} is to use hold-out validation data to learn a \emph{calibration map} for a previously trained model that transforms the model's predictions to be better calibrated.
Many calibration methods for binary classifiers have been introduced, including
logistic calibration (also known as `Platt scaling'), 
various binning methods including isotonic calibration (also known as the ROC convex hull method), 
as well as more recent methods including beta calibration and Bayesian methods. 

When we have more than two classes, calibration is generally more involved, as is often the case with multiclass classification. 
Multiclass calibration has mostly been approached by decomposing the problem into $K$ one-vs-rest binary calibration tasks, one for each class. The predictions of these $K$ calibration models form unnormalised probability vectors, which, after normalisation, may not be calibrated in a multiclass sense. 
Native multiclass calibration methods were introduced recently focusing on neural networks. These methods constitute various multiclass extensions of Platt scaling, adding a calibration layer between the logits of the neural network and the softmax layer. 

The literature on post-hoc classifier calibration in machine learning is now sufficiently rich that it is no longer straightforward to obtain or maintain a good overview of the area, which was the main motivation for writing this survey. It grew out of a tutorial we presented at the 2020 European Conference on Machine Learning and Principles and Practice of Knowledge Discovery in Databases (see \url{https://classifier-calibration.github.io}). Our aim then and now is to provide both introductory material and up-to-date technical details of the main concepts and methods. \newtext{Our focus is on the classical setup where the classifier is deployed in the same setting where it was calibrated, except for potential changes in class prior or misclassification costs. We do not cover methods to achieve robustness under conditions of other distributional shifts or out-of-distribution inputs \cite{ovadia2019can}.} We try to do justice to historical developments and pay attention to important topics that are not as widely known as they deserve to be, such as proper scoring rules. 

We also try to identify and clarify possible sources for confusion. 
The multiclass setting in particular introduces numerous subtleties that have not always been recognised or correctly dealt with in previous work. 
For example, some authors use the weaker notion of \emph{confidence calibration}, which requires only that the classifier's predicted probability for what it considers the most likely class is calibrated. 
While this is perfectly valid in its own right, it isn't always appreciated by subsequent authors that this is a much weaker notion of calibration than the one defined informally in the first sentence of this survey. 
One can also observe variations in the evaluation metric used and in the way calibrated probabilities are visualised. 
Our main aim in this survey is hence to provide a unified perspective on the different methods and metrics for binary and multiclass calibration, giving each variation its proper place. 

For the purpose of this survey we have developed a Python library which includes most of the functionalities presented in the following sections.
PyCalib~\footnote{https://classifier-calibration.github.io/PyCalib/} implements several calibration metrics (eg. confidence and classwise ECE, and their MCE counterparts), common calibration methods (eg. Isotonic Calibration, Platt's Scaling, Binning calibration), a method to combine arbitrary classifiers and calibrators into a unified training and deployment pipeline, a one-vs-the-rest implementation to adapt any binary calibration method to the multiclass setting, and multiple visualisation tools to inspect visually the calibration quality as well as tools to get better insights about the learned calibration maps.
As an illustration of the library's capabilities, most of the figures and results reported in this paper have been generated using PyCalib.

%Given the lack of a unified code distribution for calibration, we have created a Python library called .
%which includes most of the functionalities presented in this paper to assess calibration.
%This library implements several calibration metrics (eg. confidence-ECE, classwise-ECE, confidence-MCE), common calibration methods (eg. Isotonic Calibration, Platt's Scaling, Binning calibration), a one-vs-the-rest implementation to adapt any binary calibration method for the multiclass setting, and multiple visualisation tools to assess calibration (eg. binary and multiclass reliability diagrams, calibration maps for two and three classes, and other functions to explore three class classification problems). Most of the reliability diagrams and other common calibration metrics in this survey have been generated using this library.

The survey is structured as follows. 
The next section will cover important notions and intuitions related to calibration. \newtext{It aims to be at a more introductory level}, leaving technical detail for later sections. 
Section \ref{sec:psr} discusses proper scoring rules, an important general framework for evaluation of probability estimates. In Section \ref{sec:metrics} we present systematic overview of visualisation approaches and evaluation metrics for classifier calibration. 
Section \ref{sec:calibrators} is devoted to a comprehensive account of post-hoc calibration methods for both the binary and multiclass scenarios. 
Section \ref{sec:hyp} covers hypothesis tests for calibration, and Section \ref{sec:conclusion} concludes with a summary and outlook. 

==> mlj_files/02_highlevel_intro.tex <==
\section{A brief introduction to classifier calibration}
\label{sec:intro:high:level}

\newtext{
The origins of classifier calibration can be traced back to weather forecasting and meteorology. 
Here is what the UK Met Office website used to say about what their forecast probabilities mean: 

\begin{quote}
    ``[S]uppose the Met Office says that the probability of rain tomorrow in your region is 80\%. They aren't saying that it will rain in 80\% of the land area of your region, and not rain in the other 20\%. Nor are they saying it will rain for 80\% of the time. What they are saying is there is an 80\% chance of rain occurring at any one place in the region, such as in your garden.
[...]
[A] forecast of 80\% chance of rain in your region should broadly mean that, on about 80\% of days when the weather conditions are like tomorrow's, you will experience rain where you are. 
%But there is still some expert judgement involved, and different forecasting organisations with different experts and different technology might well give different probabilities.
[...]
If it doesn't rain in your garden tomorrow, then the 80\% forecast wasn't wrong, because it didn't say rain was certain. But if you look at a long run of days, on which the Met Office said the probability of rain was 80\%, you'd expect it to have rained on about 80\% of them. '' %
%(\url{https://www.metoffice.gov.uk/about-us/what/accuracy-and-trust})
(\url{https://web.archive.org/web/20210928235732/https://www.metoffice.gov.uk/about-us/what/accuracy-and-trust/probability})
%\todo[inline]{The link is broken now. I found an archived version from Sept. 28, 2021 in the Internet Archive.}
\end{quote}
\noindent
Note the phrase ``a long run of days'': determining the degree to which a forecaster is well-calibrated cannot be done on a per-forecast basis, but rather requires looking at a sufficiently large and diverse set of forecasts. 

\begin{table}[!t]
        \centering
        \includegraphics[width=\linewidth]{hallenbeck1920_tab1}
        \caption{Reproduced from \citet{hallenbeck1920}.}
        \label{tab:eval:hallenbeck1920}
\end{table}

\begin{figure}[!b]
    \centering
%    \includegraphics[width=0.6\linewidth]{Hallenbeck.pdf}\\
    \begin{subfigure}[b]{0.45\linewidth}
    \includegraphics[width=\linewidth]{Hallenbeck.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{0.40\linewidth}
    \includegraphics[width=\linewidth]{hallenbeck_alt.pdf}
    \end{subfigure}
    \caption{Two different graphical representations of the forecasts in Table~\ref{tab:eval:hallenbeck1920}.
\textbf{(Left)} The bottom graph gives a histogram of the probability forecasts. 
The top graph compares the forecast probabilities with the proportion of actual rain events in that bin. 
The red bars indicate to what extent these proportions are higher or lower than predicted. 
\textbf{(Right)} A simplified visualisation, only showing the proportion of rain events in a bin (y-axis) against the average prediction in the bin (x-axis).
    }\label{fig:hallenbeck-rel}
\end{figure}


Table~\ref{tab:eval:hallenbeck1920}, reproduced from \citet{hallenbeck1920}, groups 123 weather forecasts in 10 equal-width bins, and compares each bin with the actual empirical percentage of rain events. 
Figure~\ref{fig:hallenbeck-rel} shows two possibilities of displaying this information graphically, comparing the predicted probabilities on the $x$-axis to empirical probabilities on the $y$-axis. 
A variety of such graphical representations can be found in the literature; they are generally known as \emph{reliability diagrams}, `reliability' being one of many terms used to denote goodness of calibration \cite{murphy1977reliability}.
We can see that most of the forecasts are slight under-estimates: for example, of the 15 forecasts in the 40-49\% bin, $8/15=53\%$ were actual rain events. 
In the left graph this is shown by the vertical red line, which indicates how much the top of the blue bar extends above the diagonal (meaning that the actual proportion of rain events was higher than estimated). 
On the right graph this can be seen directly from how much the respective point is higher than the diagonal.
Similarly, we see that two of the bins (20-29\% and 30-39\%) are very slight over-estimates: on the left graph the top of the blue bar is below the diagonal, which means that the actual proportion of rain events was lower than estimated. 

\begin{figure}[!t]
    \centering
    \begin{subfigure}{0.45\linewidth}
    \includegraphics[width=\linewidth]{Hallenbeck2.pdf}
    \end{subfigure}
    \begin{subfigure}{0.45\linewidth}
    \includegraphics[width=\linewidth]{Hallenbeck3.pdf}
    \end{subfigure}
    \caption{Dividing the forecasts in Table~\ref{tab:eval:hallenbeck1920} in five (left figure) and two (right figure) equal-width bins.}\label{fig:hallenbeck2-rel}
\end{figure}

The choice of ten equal-width bins is somewhat arbitrary, and it is informative to consider different choices. 
Merging pairs of adjacent bins results in five equal-width bins, as depicted in Figure~\ref{fig:hallenbeck2-rel} (left). 
We see that all but the right-most bin averages are now slightly off-centre (we assumed that within each original bin all forecast probabilities are the same and equal to the bin centre: e.g., 25\% in the 20-29\% bin). Again, the pattern is that the higher forecast probabilities are about 10\% too low. 
Figure~\ref{fig:hallenbeck2-rel} (right) shows what we get with only two bins. 
We have lost a bit too much information here, so bins shouldn't be taken too wide. 
On the other hand they shouldn't be taken too narrow either, in order to be able to measure the true proportion of rain events with sufficient resolution. 

Taking the forecast event as a binary variable means that the calibration concept is directly applicable to binary classification. Here is an example from the typical machine learning task of learning a classifier for distinguishing `junk' or `spam' emails from regular ones: 

\begin{quote}
    A prediction `70\% chance of spam' should be spam 70\% of the time.
\end{quote}
\noindent
And a generalisation to categorical variables with more than two values is equally straightforward, as this example from Fisher's famous Iris dataset shows: 

\begin{quote}
    A prediction `70\% chance of setosa, 10\% chance of versicolor and 20\% chance of virginica' should be setosa/versicolor/virginica 70/10/20\% of the time.
\end{quote}
\noindent
So, to sum up: \emph{A predicted probability (vector) should match empirical (observed) probabilities.}
\newtext{
In the language of predictive machine learning, given an instance space $\mathbb{X}$, a binary target space $\mathbb{Y} = \{+, -\}$, and a binary probabilistic classifier $\mathsf{f}:\mathbb{X}\rightarrow [0, 1]$, the binary classifier is \emph{calibrated} if $\forall s \in[0,1]$:
\begin{align*} 
\mathsf{P}(Y=+ \: | \: \mathsf{f}(\mathbf{X}) = s)=s
\end{align*}}




% \subsection{A closer look at calibration, and why it matters}
% \label{sec:2:1}

% % \paragraph{Why are we interested in calibration?}
% In general, to calibrate means \emph{to employ a known scale with known properties}. 
% % \bb{E.g., additive scale with a well-defined zero, so that ratios are meaningful.}
% For example, we can calibrate a thermometer to Celsius or Fahrenheit scales; 
% or a weighing device to kilograms or pounds. 
% If a measuring device is calibrated to one scale but we need the measurement in another, there are usually simple conversion formulas: 
% for example, $\text{F}=\text{C}\cdot 9/5+32$ for Celsius to Fahrenheit, and $\text{Lb}=2.2\cdot \text{Kg}$ for kilograms to pounds. 
% Notice that the temperature conversion shifts the zero point 
% (0 degrees Celsius is 32 degrees Fahrenheit, and 0 degrees Fahrenheit is $-17.8$ degrees Celsius) 
% as it is essentially arbitrarily chosen for either scale. 

% The weight conversion, in contrast, has an absolute zero which is the same for all scales. 
% Such scales are called \textit{ratio scales}, because the ratio of two measurements is meaningful: e.g., if one object is twice as heavy as another in kilograms then it will be so regardless of the scale. Such ratios are not meaningful for Celsius and Fahrenheit, but temperature \textit{differences} are.  
% For example, we could say that this person's change from morning to evening body temperature today is twice that of yesterday, without specifying the temperature scale. 
% It follows that ratios of differences (or intervals) are meaningful in this case, which is why Celsius and Fahrenheit are called \textit{interval scales}. 

% For classifiers we want to use the probability scale. Probabilities have an absolute zero like any other ratio scale, and so it is meaningful to say that one event is twice as probable as another. Probabilities also have a fixed maximum, so that taking the complement with respect to the maximum gives another ratio scale: for example, the probability of this event \textbf{not} happening might be twice the probability of another event \textbf{not} happening. This essentially fixes the scale: we don't have pounds vs.\ kilograms dilemmas for probabilities. 

% % Q: Is the probability scale additive?
% Are probabilities additive? In certain situations it is indeed valid to sum probabilities, for example to obtain the probability of any one of a number of mutually exclusive events happening, as might occur when joining classes in a multiclass classification setting. 
% But multiplication and division of probabilities are more common basic operations, for example to obtain the joint probability of independent events, or to derive a conditional probability from joint and marginal probabilities. This makes the probability scale \textit{multiplicative} for typical usage. We could obtain an additive scale by taking logarithms, giving log-likelihoods, logits as differences of log-likelihoods, etc. A couple of observations are worth making: 
% \begin{itemize}
% \item Such transformations are fundamentally different from scale conversions such as Celsius to Fahrenheit, because probabilities and log-likelihoods measure different things -- physicists might say they represent different \textit{dimensions}. Nevertheless, the transformations are invertible and hence the dimensions convey the same information. 
% \item While some ratios or products of probabilities again yield probabilities, in other cases they may derive another dimension, such as \textit{odds}, which are not expressed on a probability scale.
% \end{itemize}

\subsection{Why calibration matters}
\label{sec:int:why}

What are the benefits of using well-defined calibrated scales in general, and well-calibrated probabilities in particular? One obvious benefit of calibrated scales is that we can easily combine measurements that are expressed on the same scale without comparing apples and oranges. Another is that we can use standardised decision rules, e.g., defining a fever as a body temperature exceeding 100 degrees Fahrenheit. These benefits
% \footnote{As for combining multiple probability estimates as might happen in ensemble methods in machine learning, note that the argument of probabilities being multiplicative leads to favouring the \textit{geometric mean} (or the arithmetic mean on log-probabilities). Using the arithmetic mean directly on probabilities means that the members of the ensemble are treated as classifiers scoring on some arbitrary but fixed and additive scale, disregarding their probabilistic nature.}
directly carry over to the class probability scenario, justifying decision rules such as predicting the class whose estimated probability exceeds $0.5$ in binary classification, or the class with the highest predicted probability for multiclass classification. Importantly, there is a further benefit to using calibrated probabilities as it means we can adjust these decision rules in a straightforward way to account for different class priors or misclassification costs, as we will briefly discuss presently.

% %Q: What issues might arise when applying MAP decisions to poorly calibrated classifiers such as naive Bayes? 

% % PF: UNTIL HERE (27 JAN 9.30 GMT)

% % \paragraph{Optimal decisions}
% Denote the cost of predicting class $j$ for an instance of true class $i$ as ${\mathsf{C}(\hat{Y}=j|Y=i)}$. 
% % Since we don't know the true class of an unlabelled instance, we need to base our prediction on an assessment of the expected cost over all possible true classes. 
% The expected cost of predicting class $j$ for instance $\mathbf{x}$ is then
% %
% \begin{align}\label{eq::expected-cost}
% \mathsf{C}(\hat{Y}=j|\mathbf{X}=\mathbf{x}) &= \sum_i \mathsf{P}(Y=i|\mathbf{X}=\mathbf{x})\mathsf{C}(\hat{Y}=j|Y=i)
% \end{align}
% %
% where $\mathsf{P}(Y=i|\mathbf{X}=\mathbf{x})$ is the (true) probability of instance $\mathbf{x}$ having true class $i$
% (as would be given by the Bayes-optimal classifier). 
% %
% The optimal decision is to predict the class with lowest expected cost:
% \begin{align*}
% \hat{Y}^* = \argmin_j \mathsf{C}(\hat{Y}=j|\mathbf{X}=\mathbf{x}) = \argmin_j \sum_i \mathsf{P}(Y=i|\mathbf{X}=\mathbf{x})\mathsf{C}(\hat{Y}=j|Y=i)
% \end{align*}
% %
% % In the special case that all misclassifications have equal cost we can assume without loss of generality that $C(\hat{Y}=j|Y=i)=1$ for $i\neq j$ and $C(\hat{Y}=j|Y=i)=0$ for $i=j$, which gives
% % \begin{align*}
% % C(\hat{Y}=j|X=x) &= \sum_{i\neq j} P(Y=i|X=x) = 1-P(Y=j|X=x) \\
% % %\end{align*}
% % %and so
% % %\begin{align*}
% % \hat{Y}^* &= \arg\min_j [1-P(Y=j|X=x)] = \argmax_j P(Y=j|X=x)
% % \end{align*}
% In binary classification (with a positive, $+$, and and negative class, $-$) we have one predicted probability and four cost parameters, and we can rewrite Equation~(\ref{eq::expected-cost}) as
% %
% \begin{align*}
% \mathsf{C}(\hat{Y}=+|\mathbf{X}=\mathbf{x}) &= \mathsf{P}(+|\mathbf{x})\mathsf{C}(+|+) + \big(1-\mathsf{P}(+|\mathbf{x})\big)\mathsf{C}(+|-) \\
% \mathsf{C}(\hat{Y}=-|\mathbf{X}=\mathbf{x}) &= \mathsf{P}(+|\mathbf{x})\mathsf{C}(-|+) + \big(1-\mathsf{P}(+|\mathbf{x})\big)\mathsf{C}(-|-)
% \end{align*}
% %
% where $\mathsf{P}(+|\mathbf{x})$ is shorthand for $\mathsf{P}(Y=+|\mathbf{X}=\mathbf{x})$ and $\mathsf{C}(j|i)$ for $\mathsf{C}(\hat{Y}=j|Y=i)$.
% %
% On the optimal decision boundary these two expected costs are equal, 
% which gives
% \begin{align*}
% \mathsf{P}(+|\mathbf{x})\mathsf{C}(+|+) + (1-\mathsf{P}(+|\mathbf{x}))\mathsf{C}(+|-) = \mathsf{P}(+|\mathbf{x})\mathsf{C}(-|+) + (1-\mathsf{P}(+|\mathbf{x}))\mathsf{C}(-|-)
% \end{align*}
% which can be rearranged to give the posterior odds
% \begin{align*}
% \frac{\mathsf{P}(+|\mathbf{x})}{1-\mathsf{P}(+|\mathbf{x})} = \frac{\mathsf{C}(+|-)-\mathsf{C}(-|-)}{\mathsf{C}(-|+)-\mathsf{C}(+|+)}
% \end{align*}
% as well as the posterior probability
% \begin{align*}%\label{eq::cost-threshold}
% \mathsf{P}(+|\mathbf{x})  = \frac{{\mathsf{C}(+|-)-\mathsf{C}(-|-)}}{{\mathsf{C}(+|-)-\mathsf{C}(-|-)}+{\mathsf{C}(-|+)-\mathsf{C}(+|+)}} \triangleq c
% \end{align*}
% %
% $c$ thus gives the optimal threshold on the hypothetical Bayes-optimal probabilities. 
% It is also the best thing to do in practice, as long as the probabilities are well-calibrated (this is discussed in more detail in Section~\ref{sec:out:conc}). 

% Under reasonable assumptions (e.g., changing the prediction from correct to incorrect cannot decrease the incurred cost) we can set the cost of true positives and true negatives to zero \cite{elkan2001}; 

Let
$c = \frac{\mathsf{C}(+|-)}{\mathsf{C}(+|-) + \mathsf{C}(-|+)}$ be the cost of a false positive in proportion to the combined cost of one false positive and one false negative. 
With these cost parameters the Bayes-optimal decision rule is to set the decision threshold to $c$.
For instance, if false positives are 4 times as costly as false negatives then we set the decision threshold to $4/(4+1)=0.8$ in order to only make positive predictions if we are sufficiently certain.
%
Similar reasoning applies to changes in class priors: 
\begin{itemize}
    \item if we trained on balanced classes but want to deploy with 4 times as many positives compared to negatives, we lower the decision threshold to $0.2$; 
    \item more generally, if we trained for class ratio $r$ and deploy for class ratio $r'$ we set the decision threshold to $r/(r+r')$. 
\end{itemize}
Cost and class prior changes can be combined in the obvious way; see  \citet{flach2014classification} for details.

In summary, an important reason to be interested in calibrating our classifiers is that default decision rules such as predicting the class with the highest predicted probability are fully justified from a decision-theoretic point of view, and can easily be adapted to changes in class and cost distributions. In contrast, poorly calibrated classifiers such as naive Bayes will often perform sub-optimally with default decision rules. It is possible to learn a better decision rule for a given cost and class skew using, e.g., ROC analysis \cite{lachiche2003improving} but this would have to be repeated each time the skew changes. The great advantage of post-calibration is that it only needs to be done once -- in a sense, it optimises all possible decision rules in one go.

%\todo{mention fairness and explainability?}

%\subsection{Challenges in evaluating calibration}
%Impact of binning for reliability diagrams}



\subsection{Common forms of miscalibration, and how to fix them}

There are many reasons why a probabilistic classifier might produce miscalibrated scores, and hence many ways in which miscalibration manifests itself, but two main types stand out: underconfidence and overconfidence. In this section we look at some examples and introduce two mitigation techniques. 

 
Figure~\ref{fig:under-over}, taken from \citet{niculescu-mizil2005}, shows two typical examples. In both cases the points in the reliability diagram are far from the diagonal, although the effect is smaller in the figure on the right. 

\begin{figure}[!t]
    \centering
    \begin{subfigure}{0.4\linewidth}
        \includegraphics[width=\linewidth]{caruana_fig_1.pdf}
        \caption{Underconfidence}
    \end{subfigure}%\hfill
    \hspace{1cm}
    \begin{subfigure}{0.4\linewidth}
        \includegraphics[width=\linewidth]{caruana_fig_2.pdf}
        \caption{Overconfidence}
    \end{subfigure}
    \caption{Examples of under- and overconfident classifiers. The axes are the same as for the previous figures: x-axis shows predicted probabilities and y-axis shows empirical probabilities. The dots represent the reliability diagram, and the lines show the best-fit logistic curve and beta curve.
    %To correct the underconfident scores on the left we would have to pull the points away from the midpoint on the $x$-axis, whereas to deal with the overconfidence on the right we would push them toward the midpoint. 
    Note that the logistic sigmoid is a good fit for underconfident scores but not for overconfidence.
    The figure has been adapted from \citet{niculescu-mizil2005}, and the beta curves have been added.}
    \label{fig:under-over}
\end{figure}


% \begin{figure}[!t]
%     \centering
%     \begin{subfigure}{0.3\linewidth}
%         \includegraphics[width=\linewidth]{Underconfidence.pdf}
%         \caption{Underconfidence, logistic curve}
%     \end{subfigure}\hfill
%     \begin{subfigure}{0.3\linewidth}
%         \includegraphics[width=\linewidth]{Overconfidence.pdf}
%         \caption{Overconfidence, logistic curve}
%     \end{subfigure}
%     \begin{subfigure}{0.35\linewidth}
%         \includegraphics[width=\linewidth]{betafig.pdf}
%         \caption{Overconfidence, beta curve}
%     \end{subfigure}
%     \caption{Examples of under- and overconfident classifiers. The axes are the same as for the previous figures: x-axis shows predicted probabilities and y-axis shows empirical probabilities. The dots represent the reliability diagram, and the line shows the best-fit logistic curve (a,b) or beta curve (c).
%     %To correct the underconfident scores on the left we would have to pull the points away from the midpoint on the $x$-axis, whereas to deal with the overconfidence on the right we would push them toward the midpoint. 
%     Note that the logistic sigmoid is a good fit for underconfident scores but not for overconfidence.
%     Figures (a,b) are reproduced from \citet{niculescu-mizil2005}.}
%     \label{fig:under-over}
% \end{figure}

What do we see in the left figure? It is quite natural to give precedence to vertical information in such graphs, so you might be inclined to say ``The points on the left are too low, and the points on the right are too high''. But keeping in mind that the predicted probabilities on the $x$-axis are under our control but not the empirical probabilities on the $y$-axis, a more `actionable' way to express this is

\begin{quote}
    The lower points are too far to the right, and the higher points are too far to the left. In other words, the points have a tendency to sit too close to the midpoint on the $x$-axis. 
\end{quote}
\noindent
This is the typical pattern displayed by an \textit{underconfident} classifier, which thinks it's {worse} at separating classes than it actually is. 

Hence, to mitigate this, we need to {pull predicted probabilities away from the centre}. As the left plot in Figure \ref{fig:under-over} shows, this can be neatly modelled by a sigmoidal logistic curve, which can be defined in parametric form as
%
\begin{align*}
    \mathsf{c}(s; w, m) &= \frac{1}{1+\exp(-w(s-m))}%\\
    % w &= (\mu_{\textit{pos}}-\mu_{\textit{neg}})/\sigma^2, 
    % m = (\mu_{\textit{pos}}+\mu_{\textit{neg}})/2
\end{align*}
%
Here, $s$ is the uncalibrated score produced by the classifier and $\mathsf{c}$ gives the logistically calibrated score. 
$m$ and $w$ are the two parameters of the logistic family, which determine the point where $\mathsf{c}(s)=0.5$ and the slope at that point, respectively. They can be estimated from the points in the reliability diagram in order to find the best fit. In this case they can be obtained analytically as the mean of the classwise average scores, and the difference between those two means in proportion to the score variance \cite{flach2012machine}.
%(which is assumed to be the same for both classes). 

The fitted logistic curve thus establishes a \textit{calibration map} which transforms uncalibrated scores $s$ into calibrated scores $\mathsf{c}(s)$. 
Even though the calibration map doesn't map to empirical probabilities, plotting it over the reliability diagram allows us to see clearly that if we project each point in the reliability diagram vertically onto the calibration map, and replace its $x$-value with the corresponding $y$-value of the projection, we end up with points on or very close to the diagonal, and hence near-perfectly calibrated scores (Figure~\ref{fig:under-cal}).

\begin{figure}[!t]
    \centering
        \includegraphics[width=0.5\linewidth]{caruana_fig_3.pdf}
    \caption{Graphical illustration of how a well-fitted calibration map leads to near-perfect calibration. From left to right, the dotted arrows show (1) using a point's uncalibrated score $s$ on the $x$-axis as input to the calibration map, (2) mapping the resulting output $\mathsf{c}(s)$ back to the diagonal, and (3) combine with the empirical probability of the point we started from. The closer the original point is to the fitted calibration map, the closer the calibrated point (in red) will be to the diagonal. }
    \label{fig:under-cal}
\end{figure}

The logistic curve is widely used as a `squashing function', compressing values on a possibly unbounded scale into the $[0,1]$ interval. 
Following \citet{platt2000} it is often used as a way to convert scores from a Support Vector Machine into probabilities. 
Technically this isn't calibration as SVM scores are not probabilities but (signed) geometric distances from the decision boundary -- this is also called \textit{scaling} to emphasise the difference \newtext{(hence the popular name `Platt scaling`)}. 
The parametric form of the logistic map can be derived from first principles by assuming that within each class the uncalibrated scores are normally distributed with the same variance. % (Figure~\ref{fig:logistic}). 
\label{page:platt}

% \begin{figure}[!b]
%     \centering
%     \includegraphics[width=0.6\textwidth]{Logistic.pdf}\vfill
%     \caption{Assuming normally distributed scores within each class (left) leads to a logistic calibration map (right).}\label{fig:logistic}
% \end{figure}

The other common form of miscalibration is overconfidence, as exemplified in Figure~\ref{fig:under-over}(b,c). 
% Here, we see that
%
% \begin{quote}
%     The lower points are too far to the left, and the higher points are too far to the right. In other words, the points have a tendency to be too far from the midpoint on the $x$-axis. 
% \end{quote}
% \noindent
An \textit{overconfident} classifier thinks it's {better} at separating classes than it actually is. 
Hence we need to {make predicted probabilities less extreme by pushing them toward the centre}. 
The paper we took this figure from \cite{niculescu-mizil2005} also fitted a logistic curve to this reliability diagram Figure~\ref{fig:under-over}(b), because they were investigating the effect of Platt scaling in a wide range of scenarios. But we see clearly that the fit is rather poor, and using this logistic curve as a calibration map is likely to make matters worse. In this particular case we would be looking for something that can produce an inverse sigmoidal curve. What would be a principled way to achieve this? 

%\begin{figure}[!b]
%    \centering
%    \includegraphics[width=0.9\textwidth]{Beta.pdf}
%    \caption{An example of Beta calibration where overconfident scores (left) lead to an inverse-sigmoidal calibration map (right).}\label{fig:beta}
%\end{figure}

One approach that works well is to model the classwise scores with Beta distributions \cite{pmlr-v54-kull17a,kull2017beyond}.
These assume random variables bounded in $[0,1]$ which is exactly what we need for post-hoc calibration. 
Beta distributions can easily model the skewed distributions resulting from overconfident classifiers, as demonstrated in Figure~\ref{fig:under-over}(b).%Figure~\ref{fig:beta}. 
Mathematically, these curves have three parameters: 
%
    \begin{align*}
        \mathsf{c}(s; a, b, c) &= \frac{1}{1+\exp(-a \ln s + b \ln (1-s) - c)}
        % a &= \alpha_{\textit{pos}}-\alpha_{\textit{neg}}, 
        % b = \beta_{\textit{neg}}-\beta_{\textit{pos}}
    \end{align*}
%
This additional degree of freedom allows Beta calibration to produce both sigmoidal and inverse-sigmoidal calibration maps. 
It can even fit the identity map ($a=b=1$, $c=0$), which means that Beta calibration can recognise that scores are already calibrated. 
In contrast, applying logistic calibration to a calibrated classifier will decalibrate it. 
While Beta calibration can achieve many shapes of calibration maps, it is still a limited parametric family.
Methods to fit richer calibration map families will be discussed in Section~\ref{sec:calibrators}.

%PF: UNTIL HERE (28 JAN 18.00 GMT)

% So far we have seen two calibration techniques: 
% \begin{itemize}
%     \item logistic calibration, which -- although technically a scaling technique, mapping real-valued scores into probabilities -- can adjust for underconfident scores; 
%     \item Beta calibration, which assumes a classifier already scores on a probability scale, and which can adjust for both over- and underconfident scores. 
% \end{itemize}
% We will now take a first look at 
%%% A third calibration technique
%%% % quite different from these two because it 
%%% derives a calibration map from the \textit{ranks} of a set of scores, and hence works for classifiers scoring on arbitrary scales. It is also different from logistic and Beta calibration because it doesn't attempt to model the classwise score distributions, and is hence \textit{non-parametric}. 
%%% %
%%% The technique in question is called \textit{isotonic regression}, belying its origin as an alternative to linear regression which learns a piecewise constant, monotonically increasing or decreasing function. There are several algorithms for isotonic regression, one of which is called \textit{pooled adjacent violators}, which in turn is also used for constructing the convex hull of an ROC curve \cite{zadrozny2001obtaining,fawcett2007}. Figure~\ref{fig:isotonic} demonstrates this graphically. 
%%% 
%%% \begin{figure}[!t]
%%%     \centering
%%%     \begin{subfigure}{0.44\linewidth}
%%%     \includegraphics[width=\linewidth]{ROCCH.pdf}
%%%     \caption{ROC curve and convex hull.}
%%%     \end{subfigure}
%%%     \begin{subfigure}{0.55\linewidth}
%%%     \includegraphics[width=\linewidth]{ROCcal2.pdf}
%%%     \caption{Isotonic calibration map.}
%%%     \end{subfigure}
%%%     \caption{An example of isotonic calibration which derives a piece-wise constant calibration map from the ROC convex hull (Source: \cite{flach2016roc}).}\label{fig:isotonic}
%%% \end{figure}
%%% 
%%% The technique starts from a list of test instances, ranked on their scores; this might give a list of class labels like that depicted at the top of the right figure in Figure~\ref{fig:isotonic}. We then proceed to segment this ranking such that, in each adjacent pair of segments, the right neighbour has a larger proportion of positives than the left neighbour. This defines a unique set of segments, which is depicted on the right of the right figure. Each segment defines an interval on the original classifier scores, as well as an empirical probability of positives in that segment which is taken as the calibrated score for all instances whose score falls in that interval. The calibration map is thus piece-wise constant and increasing. 
%%% 
%%% As a non-parametric method, isotonic regression avoids problems of misspecification which can plague parametric models. For example, a perfectly calibrated classifier has classwise scores which are far from normally distributed, so applying logistic calibration will make matters worse. The downside is that isotonic regression tends to need more labelled data to reliably estimate the segment boundaries and the empirical probabilities within each segment, and is more liable to overfitting if data is not plentiful. 
%%% 

%----------------------------------------------------%
\subsection{Multiclass calibration}
%----------------------------------------------------%

The examples we have seen so far all relate to binary classification. Is it straightforward to generalise calibration concepts and methods to more than two classes? 
The answer to this question is somewhat involved. Some ideas do generalise quite easily: for example, we can model per-class scores by multivariate distributions such as Dirichlet distributions \cite{kull2019}. Some other ideas don't generalise easily at all: for example, a multiclass generalisation of isotonic regression is not straightforward because rankings are inherently bipartite. Such approaches therefore need to be approximated by considering classes in a pairwise or one-versus-rest manner. 

This helps to explain why there is divergence even at a definitional level. 
There are at least three different ways of \emph{defining} what it means to be calibrated in a multiclass setting. 
They are equivalent for binary classification but increasingly stronger for more than two classes,%
\footnote{In rare cases it is possible for a multiclass classifier to be classwise calibrated but not confidence calibrated.
% Example due to Meelis
Here is an example with 40 instances in four groups:
10 instances with predicted probabilities (0.3,0.3,0.4) and actual class distribution (4,2,4);
another 10 with probabilities (0.4,0.3,0.3) and classes (3,4,3);
another 10 with probabilities (0.4,0.6,0.0) and classes (5,5,0);
and the remaining 10 instances with probabilities (0.3,0.6,0.1) and classes (2,7,1).
This classifier is classwise-calibrated but not confidence-calibrated. There are 20 instances with confidence level 0.6 and accuracy 0.6 (5+7=12 out of 20), but the remaining 20 instances have confidence 0.4 and accuracy 0.35 (4+3=7 out of 20). The key idea of this construction is that classwise calibration considers the instances with 0.4 predicted for class 1 as a single group, but confidence calibration looks among them only at those instances for which 0.4 is the highest probability -- e.g., it does consider (0.4,0.3,0.3) but not (0.4,0.6,0.0).}
and can be summarised as follows: 
    \begin{itemize}
        \item {Confidence calibration}: only consider the highest predicted probability. 
        \item {Classwise calibration}: only consider marginal probabilities.
        \item {Multiclass calibration}: consider the entire vector of predicted probabilities.
    \end{itemize}
We will use this terminology throughout the paper to avoid confusion. 

%\renewcommand{\vph}{\hat{\mathbf{p}}}

\textit{Confidence calibration} was proposed by \citet{guo2017}, although not under that name. It requires that among all instances where the probability of \emph{the most likely class} is predicted to be $\alpha$, the expected accuracy is $\alpha$. 
Let $\mathbb{X}$ denote the instance space and $\mathbb{P}_{\mathbb{Y}}$ the probability $K$-simplex, then a probabilistic classifier $\mathsf{f}:\mathbb{X}\rightarrow\mathbb{P}_{\mathbb{Y}}$ is \emph{confidence-calibrated}, if for any confidence level $\alpha\in[0,1]$, 
the actual proportion of the predicted class, among all possible instances $\mathbf{x}$ being predicted this class with confidence $\alpha$, is equal to $\alpha$:  
\begin{align*} 
\mathsf{P}(Y=\hat{Y} \: | \: S_{\hat{Y}}=\alpha)=\alpha\qquad\text{where }\ \hat{Y}=\argmax_j S_j.
%P\Big(Y=\argmax\big(\vph(X)\big) \: \Big| \: \max\big(\vph(X)\big)=c\Big)=c.
\end{align*}
Here, $S_j$ denotes the $j$-th dimension of $\mathsf{f}(\mathbf{X})$.

\textit{Classwise calibration}, proposed by \citet{zadrozny2002}, requires that all \emph{one-vs-rest} probability estimators obtained from the original multiclass model are calibrated. 
Formally, a probabilistic classifier $\mathsf{f}:\mathbb{X}\rightarrow\mathbb{P}_{\mathbb{Y}}$ is \emph{classwise-calibrated}, if for any class $i \in \{1, \dots, K\}$ and any predicted probability value $s \in [0, 1]$ for this class, 
the actual proportion of class $i$, among all possible instances on the random variable $\mathbf{X}$ getting the same prediction on class i, is equal to $s$:  
\begin{align*} 
\mathsf{P}(Y=i\mid S_i=s)=s
\end{align*}

\textit{Multiclass calibration}, also called \textit{calibration in the strong sense} \cite{widmann2019calibration}, is the {strongest form of calibration} for more than two classes, subsuming the previous two definitions. 
A probabilistic classifier $\mathsf{f}:\mathbb{X}\rightarrow\mathbb{P}_{\mathbb{Y}}$ is \emph{multiclass-calibrated} if for any prediction vector $\mathbf{s}=[s_1,\dots,s_K]\in\mathbb{P}_{\mathbb{Y}}$, the proportions of classes among all possible instances on the random variable $\mathbf{X}$ getting the same prediction $\mathsf{f}(\mathbf{X})=\mathbf{s}$ are equal to the prediction vector $\mathbf{s}$:  
\begin{align*} %\label{eq:calib}
\mathsf{P}(Y=i\mid \mathsf{f}(\mathbf{X})=\mathbf{s})=s_i\qquad\text{for }\ i=1,\dots,K.
\end{align*}
%
%Here $\mathbf{s}=[s_1, \dots, s_K]$ denotes the $K$-dimensional probability vector instance.

For practical purposes, the conditions in these definitions need to be relaxed. This is where {binning} comes in. 
Once we define the bins, we can draw a {reliability diagram} as in the two-class case. For classwise calibration, we can show per-class reliability diagrams or a single averaged one. 
One way to assess the degree of calibration is by means of the {gaps} in the reliability diagram. 
These topics will be explored in Section \ref{sec:metrics}. 
We will first take a closer look at the important concept of \emph{proper scoring rules} in the next section. Proper scoring rules are instance-wise evaluation measures for probability estimates that avoid the need for score binning. As a result they cannot measure the degree of calibration directly, but through decomposition results, we will show how the scores can be decomposed into various components, including the calibration loss. 

}


==> mlj_files/03_evaluation.tex <==
\section{From proper scoring rules to calibration}
\label{sec:psr}




%----------------------------------------------------%
% \subsection{Proper scoring rules}
% \label{sec:met:psr}
%----------------------------------------------------%

% {\color{red}(TODO: Mention this \cite{savage1971}.)}
    
As early as 1950 researchers were interested in scoring functions that would evaluate probabilistic forecasts without influencing the forecaster into making undesirable predictions \cite{brier1950}, thus keeping the forecaster ``honest'' while encouraging useful forecasts. In the late 1960s the term \emph{proper scoring rule} was already in use for score functions whose computation was based on a forecaster's probabilities and the actual occurrence or not of the corresponding events \cite{winkler1969scoring}. Informally, a scoring rule is said to be proper if optimal values are obtained by the forecaster predicting the true probabilities of the events. %At the same time, proper scoring rules were shown to be useful not only to evaluate predicted probabilities but also to help in training better forecasters \cite{winkler1969scoring}.
% In addition to machine learning evaluation and to the seminal works in meteorology, 
Proper scoring rules and their ability to induce useful and accurate forecasts also lend themselves to game-theoretic interpretations, as discussed in the seminal work of \citet{savage1971}.

Before diving into details, let us introduce the notation. In a multiclass classification task with $K$ classes, let the true class of an instance be a vector $\dot{\mathbf{y}}=[y_1,\ldots,y_K]$, where $y_j = 1$ when the true class is $j$, otherwise $y_j = 0$. Additionally, let $\mathbf{s}=[s_1,\ldots,s_K]$ be a class probability vector obtained from a classification model for an instance, i.e. $s_j \geq 0$, $j=1,\ldots,K$ and $\sum^K_{j=1} s_j = 1$. A scoring rule $\phi(\mathbf{s}, \dot{\mathbf{y}})$ is a non-negative measure of how well the estimated probability vector $\mathbf{s}$ matches the true class vector $\mathbf{\dot{y}}$. We assume that lower values of $\phi(\mathbf{s}, \dot{\mathbf{y}})$ are better.% 
\footnote{Some authors \cite{winkler1969scoring,gneiting2007} use scoring rules in the opposite way, i.e. higher is better, sometimes calling them utility or payoff functions, in the sense that a forecaster is rewarded for giving better predictions. If a scoring rule was proposed as a payoff function, we can typically negate its values such that lower values are better.} 

Popular scoring rules include Brier score $\phi_{\text{BS}}$ and log-loss $\phi_{\text{LL}}$, which are defined as follows:
%
\begin{equation}
    \label{eq:evaluation:brier}
    \phi_{\text{BS}}(\mathbf{s}, \mathbf{\dot{y}})  = \sum_{j=1}^{K} (s_j - y_j)^2.
\end{equation}

  \begin{equation}
    \label{eq:evaluation:logloss}
    \phi_{\text{LL}}(\mathbf{s}, \mathbf{\dot{y}}) = - \sum_{j=1}^{K} y_j \log s_j.
\end{equation}
%
Our Brier score definition ranges between $0$ and $2$, agreeing with Brier's original definition \cite{brier1950}, although it is now common for half this quantity to be called Brier score. While scoring rules evaluate the loss incurred by the class probability estimates for a single instance, we are usually interested in evaluating the performance of a model on test data. Thus, given a test dataset, we can calculate the empirical loss as the average instance-wise loss across the data. % Going back to our example from Table \ref{tab:evaluation:toy}, we have 



% \begin{align*}
%     \bar{\phi}_{\text{BS}} &= \frac{1}{30}\sum_{i=1}^{30} \sum_{j=1}^{3} (p_{ij} - y_{ij})^2, \\ &= \frac{1}{30}\left[(1 -1)^2 + (0 - 0)^2 + (0 - 0)^2 + \ldots  + (0.3 - 0)^2 + (0.7 - 1)^2\right], \\ &= XXX,
% \end{align*}

% \noindent and

% \begin{align*}
%     \bar{\phi}_{\text{LL}} &= -\frac{1}{30}\sum_{i=1}^{30} \sum_{j=1}^{3} y_{ij} \log p_{ij}, \\ &= -\frac{1}{30}\left(1\log 1 + 0\log 0 + 0\log 0 + \ldots + 0\log 0 + 0\log 0.3 + 1\log 0.7\right), \\ &= XXX.
% \end{align*}

Suppose the class labels $\mathbf{\dot{y}}$ are drawn from the true distribution $\mathbf{q}$ over classes. A scoring rule $\phi$ is proper if its expected value on probability vector $\mathbf{s}$ and $\mathbf{\dot{y}}$ is higher than (i.e., worse) or the same as its expected value on $\mathbf{q}$ and $\mathbf{\dot{y}}$, that is if

% In this section we cover loss measures ($\breve{\phi}$) that prefer Bayes-optimal classifiers over other classifiers, i.e. for any given $P(\mathbf{X}, Y)$, $\mathbf{x} \in \mathcal{X}$, the following is satisfied:

\begin{align*}
\mathsf{E}_{\mathbf{\dot{y}} \sim \mathbf{q}} \Big[ \phi\big(\mathbf{s}, \mathbf{\dot{y}}\big)  \Big] \geq \mathsf{E}_{\mathbf{\dot{y}} \sim \mathbf{q}} \Big[ \phi\big(\mathbf{q}, \mathbf{\dot{y}}\big)  \Big], 
\end{align*}
and it is strictly proper if and only if both sides of the expression being equal implies $\mathbf{s} = \mathbf{q}$. % and $P(Y \mid \mathbf{X}=\mathbf{x})$ is a vector with elements $P(Y=j \mid \mathbf{X}=\mathbf{x})$.
Both Brier score and log-loss are strictly proper scoring rules.
     
%  Proper scoring rules are calculated as expectations over probability distributions, while ECE measures are averages across bins. If proper scoring rules are approximated empirically, they can be interpreted as putting each item in its separate bin, which would look like the example in Figure \ref{fig:rel4}, then computing the average of some loss for each predicted probability and its corresponding observed label. Instead of the absolute difference, as in ECE, this loss can be the quadratic error or the Kullback–Leibler divergence, which have better mathematical properties. The best-known proper scoring rules include Brier score and log-loss, which are given by Equations (\ref{eq:evaluation:brier}) and (\ref{eq:evaluation:logloss}), respectively, where $\mathbb{I}(\cdot)$ is an indicator function, such that $\mathbb{I}(y_n=j) = 1$, if $y_n=j$, otherwise $\mathbb{I}(y_n=j) = 0$.
    
    % \begin{figure}
    %     \centering
    %     \includegraphics[width=0.7\textwidth]{figures/evaluation/Forecaster4.png}
    %     \caption{Binary reliability diagram with one bin per instance.}
    %     \label{fig:eval:forecaster4}
    % \end{figure}
    


    % \begin{equation}
    %     \label{eq:evaluation:brier}
    %     \breve{\phi}_{\text{BS}}\Big(\mathbf{Q}, \mathbf{y}\Big)  = \frac{1}{N}\sum_{n=1}^{N}\sum_{j=1}^{K} \Big(\mathbb{I}(y_n=j) - q_{n,j} \Big)^2.
    % \end{equation}
    
    %   \begin{equation}
    %     \label{eq:evaluation:logloss}
    %     \breve{\phi}_{\text{LL}}\Big(\mathbf{Q}, \mathbf{y}\Big) = -\frac{1}{N}\sum_{n=1}^{N} \sum_{j=1}^{K} \mathbb{I}(y_n=j) \cdot \text{log} (q_{n,j}).
    % \end{equation}
    
% TSF proposed text
%    Among proper scoring rules, log-loss in particular is frequently used as the training loss of machine learning methods such as neural networks, often under the name of cross-entropy. At the instance level, log-loss only depends on the predicted class probability for the true class (as all other classes $y_j$ are zero) and it might not be obvious why it is a proper scoring function. However, properness is defined as an expectation over a population. For instance, suppose that, for a population of instances, the true probability is $[0.8, 0.2, 0.0]$. In this case, the expected log-loss will be $-(0.8 \log(s_1) + 0.2 \log(s_2))$, which can only be minimised by predicting the probability vector $[0.8, 0.2, 0.0]$, satisfying the properness condition.
    
% MPN merged TSF and MK and PF feedback
Among proper scoring rules, log-loss in particular is frequently used as the training loss of machine learning methods such as neural networks, often under the name of cross-entropy. \newtext{It is also the loss function used by most of the calibration methods discussed in Section \ref{sec:calibrators}, including Platt scaling, temperature scaling and its variations (vector and matrix), beta calibration and Dirichlet calibration. A notable exception is isotonic calibration, which optimised Brier score.}

At the instance level, log-loss only depends on the predicted class probability for the true class (as all other classes $y_j$ are zero) and it might not be obvious why it is a proper scoring function.
For example, one could argue that it does not matter whether the model predicts $[0.8, 0.2, 0.0]$ or $[0.8, 0.1, 0.1]$ on an instance of class $1$, as log-loss would be $-\ln(0.8)$ in both cases.
However, one needs to keep in mind that properness is defined as an expectation over a population. 
For instance, suppose that, for a population of instances, the true probability is $[0.8, 0.2, 0.0]$.
In this case, the expected log-loss will be $-(0.8 \log(s_1) + 0.2 \log(s_2))$, which can only be minimised by predicting the probability vector $[0.8, 0.2, 0.0]$, satisfying the properness condition.
Note that log-loss can be dominated by cases where the true class is predicted with low probability: in the extreme case of a single instance with zero probability for the true class the loss is infinite. 

    %, as it only penalises the probability given to the true class, which can be useful if one is only interested in maximising the probability given to the true class of an instance.
   %Log-loss only depends on the predicted class probability for the true class (as all other $y_j$ are zero) and it might not be obvious why it is a proper scoring function. %, i.e. why this loss has a unique minimum achieved by the Bayes-optimal model. 
   %For example, one could argue that it does not matter whether the model would predict $[0.7,0.1,0.1,0.1]$ or $[0.7,0.3,0.0,0.0]$ on an instance of class $1$, as log-loss would be $-\ln(0.7)$ in both cases. However, one needs to keep in mind that at the time of making the prediction the model does not know the true class of the instance and has no way of knowing which of the values in the predicted probability vector will be `probed' by the loss and will thus eventually matter. Therefore, the model should only predict $[0.7,0.3,0.0,0.0]$ when it is absolutely sure that the instance cannot belong to classes 3 and 4, because otherwise the evaluation on test set might catch it with an infinite loss of $-\ln(0)$ with a predicted probability $0$ for the true class $3$ or $4$.

    % We can easily see that Brier score and log-loss are not minimised by constantly predicting the class distribution, as in ECE. In fact, if a classifier predicts $0.5$ positive probability for two different instances, one positive and another negative, Equations (\ref{eq:evaluation:brier}) and (\ref{eq:evaluation:logloss}) result in $\breve{\phi}_{\text{BS}}\Big(\mathbf{Q}, \mathbf{y}\Big) = 0.5$ and $\breve{\phi}_{\text{LL}}\Big(\mathbf{Q}, \mathbf{y}\Big) = 0.6931$, respectively.
        
    
  
    
    


\subsection{Decompositions of proper scoring rules}\label{sec:decomp}

When proposing the forecast evaluation that would later be known as Brier score, Brier mentioned that it could not be ``gamed'', i.e. in order to obtain low scores, the forecaster has to produce honest, useful and correct predictions. Later research focused on why this was true for Brier score and other proper scoring rules.

\citet{sanders1963} showed that Brier score corresponds to the sum of two aspects of probability evaluation: validity and sharpness, terms introduced by \citet{miller1962statistical} and \citet{bross1953design}, respectively. Validity, later known as reliability \cite{murphy1977reliability}, is now often called \emph{calibration loss} \cite{kull2015novel}. It refers to the fit between the forecasts and the frequency of occurrence of the event, which means that it is a joint property of the predictions and the events. Sharpness, which is now commonly called \emph{refinement loss} and was also known as resolution \cite{murphy1977reliability}, is the loss due to predicting the same probability for instances from different classes.
% and is a property of predicted probabilities only. 
\citet{degroot1983} %comparison}
showed that these two terms make up proper scoring rules in general, and that probabilistic predictions should minimise refinement loss subject to calibration.

We now formally introduce such proper scoring rule decompositions. Let $\mathbf{X}$ and $\mathbf{\dot{Y}}=[Y_1,\ldots,Y_K]$ be multivariate random variables, respectively corresponding to the features and the class of a randomly picked instance, where $Y_j=1$ if the instance is of class $j$, otherwise $Y_j= 0$, for $j=1,2,\ldots,k$. Given a scoring classifier, class probability estimator or probability forecaster $\mathsf{f}$, we denote by $\mathbf{S}=[S_1,S_2,...,S_k]=\mathsf{f}(\mathbf{X})$ the vector output of $\mathsf{f}$ for random feature $\mathbf{X}$, where $\mathbf{S}$ is a random vector due to its dependence on $\mathbf{X}$. The expected value of proper scoring rule $\phi$ with respect to $\mathbf{S}$ and $\mathbf{\dot{Y}}$ is then $\mathsf{E} \Big[ \phi\big(\mathbf{S}, \mathbf{\dot{Y}}\big)  \Big]$.

\begin{table}[h]
\centering
\begin{tabular}{cccccc}
\hline
\textbf{$i$} & \textbf{$X^{(i)}$} & \textbf{$Y^{(i)}$} & $Q^{(i)}$         & $S^{(i)}$       & $C^{(i)}$          \\ \hline
$1$          & $(3,1,3)$          & $(1,0,0)$          & $(0.75,0.25,0.0)$ & $(0.9,0.1,0.0)$ & $(0.75,0.25,0.0)$  \\
$2$          & $(3,1,3)$          & $(1,0,0)$          & $(0.75,0.25,0.0)$ & $(0.9,0.1,0.0)$ & $(0.75,0.25,0.0)$  \\
$3$          & $(3,1,3)$          & $(1,0,0)$          & $(0.75,0.25,0.0)$ & $(0.9,0.1,0.0)$ & $(0.75,0.25,0.0)$  \\
$4$          & $(3,1,3)$          & $(0,1,0)$          & $(0.75,0.25,0.0)$ & $(0.9,0.1,0.0)$ & $(0.75,0.25,0.0)$  \\
$5$          & $(2,2,2)$          & $(1,0,0)$          & $(0.50,0.50,0.0)$ & $(0.6,0.2,0.2)$ & $(0.17,0.50,0.33)$ \\
$6$          & $(2,2,2)$          & $(0,1,0)$          & $(0.50,0.50,0.0)$ & $(0.6,0.2,0.2)$ & $(0.17,0.50,0.33)$ \\
$7$          & $(0,2,2)$          & $(0,1,0)$          & $(0.0,0.50,0.50)$ & $(0.6,0.2,0.2)$ & $(0.17,0.50,0.33)$ \\
$8$          & $(0,2,2)$          & $(0,1,0)$          & $(0.0,0.50,0.50)$ & $(0.6,0.2,0.2)$ & $(0.17,0.50,0.33)$ \\
$9$          & $(0,2,2)$          & $(0,0,1)$          & $(0.0,0.50,0.50)$ & $(0.6,0.2,0.2)$ & $(0.17,0.50,0.33)$ \\
$10$         & $(0,2,2)$          & $(0,0,1)$          & $(0.0,0.50,0.50)$ & $(0.6,0.2,0.2)$ & $(0.17,0.50,0.33)$ \\ \hline
\end{tabular}
        \caption{Example dataset with three classes and three features. Column $Q^{(i)}$ shows class posteriors given by the optimal model with $Q_1 = 0.25X_1$, $Q_2 = 0.25X_2$ and $Q_3 = 1 - (Q_1 + Q_2)$. Column $S^{(i)}$ corresponds to estimated class posteriors $S=f(X)$, which are given by $S_1 = 0.3X_3$, $S_2 = 0.1X_2$ and $S_3 = 1 - (S_1 + S_2)$. Finally, column $C$ represents calibrated probabilities.
        %calculated with $X|Y_1 \sim \mathcal{N}(4.375,1)$, $X|Y_2 \sim \mathcal{N}(1.875,2)$ and $X|Y_3 \sim \mathcal{N}(0,1)$. The class posteriors $S=f(X)$ are estimated by a trained model $f$ with $X|Y_1 \sim \mathcal{N}(4.5,1)$, $X|Y_2 \sim \mathcal{N}(3,1)$ and $X|Y_3 \sim \mathcal{N}(0.5,1)$. For the optimal model, the class priors are $\pi_1 = 4/10$,  $\pi_2 = 4/10$ and  $\pi_3 = 2/10$, while for model $f$, $\pi_1 = \pi_2 = \pi_3 = 1/3$, i.e. the classes are considered equally probable. Column $C$ represents calibrated probabilities.
        }
        \label{tab:evaluation:toy:psr}
\end{table}

Consider a classification test set of $10$ instances belonging to three classes ($K=3$) and described by $3$ features, as shown in column $\mathbf{X}^{(i)}$ of Table \ref{tab:evaluation:toy:psr}. Suppose instances  $1$, $2$, $3$ and $5$ belong to class $1$, i.e. $Y_1=1$, instances $4$, $6$, $7$, $8$ belong to class $2$ and the rest belong to class $3$. Note that in this example, the optimal class posteriors $\mathbf{Q}^{(i)}$ are given, however this is not generally the case. Additionally, the sample is representative by design, with average $\mathbf{Y}^{(i)}$, among instances with the same feature values, exactly agreeing with $\mathbf{Q}^{(i)}$. Given columns $\mathbf{S}^{(i)}$ and $\mathbf{Y}^{(i)}$ from Table \ref{tab:evaluation:toy:psr}, and using Equations (\ref{eq:evaluation:brier}) and (\ref{eq:evaluation:logloss}), by averaging over the 10 instances, we get a mean Brier score of $0.71$ and mean log-loss of $1.12$.

% \begin{align*}
%     \bar{\phi}_{\text{BS}} &= \frac{1}{10}\sum_{i=1}^{10} \sum_{j=1}^{3} (p_{ij} - y_{ij})^2, \\ &= \frac{1}{10}\left[(1 -0.9)^2 + (0 - 0.1)^2 + (0 - 0)^2 + \ldots  + (0.3 - 0)^2 + (0.7 - 1)^2\right], \\ &= XXX,
% \end{align*}

% \noindent and

% \begin{align*}
%     \bar{\phi}_{\text{LL}} &= -\frac{1}{10}\sum_{i=1}^{10} \sum_{j=1}^{3} y_{ij} \log p_{ij}, \\ &= -\frac{1}{30}\left(1\log 1 + 0\log 0 + 0\log 0 + \ldots + 0\log 0 + 0\log 0.3 + 1\log 0.7\right), \\ &= XXX.
% \end{align*}


% \todo[inline]{Meelis Kull: I think it is better to first state that suppose Q is given. Because then C can be calculated from it. Otherwise it is not clear how the expectation of E[Y|S] has been obtained. Note that by a lucky chance (well,.. by our design) the average Y exactly agrees with Q, i.e. Y are a representative sample.  This makes average[Y|S]=average[Q|S], which does not have to be the case in general. So somehow we need to be a bit careful to distinguish what is a coincidence here and what is exactly equal always. One possibility is to make the data generating process to pick lines from this table uniformly randomly, but not sure it is the best way to explain.}
Now let $\mathbf{C}=[C_1,C_2,\ldots,C_K]$ be yet another random vector, where $C_j=\mathsf{E}[Y_j| \mathbf{S}]$, i.e. $C_j$ represents the actual proportion of class $j$ given all instances which received the same estimate $\mathbf{S}$ from model $\mathsf{f}$. The decomposition of proper scoring rule $\phi$ into calibration loss and refinement loss is then the sum of expected loss between $\mathbf{S}$ and $\mathbf{C}$ and expected loss between $\mathbf{C}$ and $\mathbf{Y}$ \cite{brocker2007,kull2015novel}:
\begin{align*}
    \mathsf{E} \Big[ \mathsf{d}\big(\mathbf{S}, \mathbf{\dot{Y}}\big)  \Big] = \mathsf{E} \Big[ \mathsf{d}\big(\mathbf{S}, \mathbf{C}\big)\Big] + \mathsf{E} \Big[ \mathsf{d}\big(\mathbf{C}, \mathbf{\dot{Y}}\big)  \Big],
\end{align*}

\noindent where $\mathsf{d}: \mathbb{P}_{\mathbb{Y}} \times \mathbb{P}_{\mathbb{Y}} \rightarrow \mathbb{R}$ is the divergence associated to proper scoring rule $\phi$. For log-loss and Brier score, $\mathsf{d}$ has been shown to correspond to the Kullback-Leibler divergence and the mean squared difference, respectively \cite{kull2015novel}.

The definition above is given based on expected population loss. In practice, we would be calculating these quantities on test data, as we generally do not have access to the whole population. Thus, we actually calculate an empirical loss. But assuming that test data is representative of the whole population and that there is a uniform distribution over the test instances and zero probability elsewhere, empirical loss can be interpreted as a special case of expected loss and all decompositions derived for expected loss also apply to empirical loss \cite{kull2015novel}. 

In our example in Table \ref{tab:evaluation:toy:psr}, the first four instances share the same model scores $\mathbf{S}=[0.9,0.1,0.0]$, with the first three instances belonging to class $1$ and the fourth to class $2$. Thus, for these instances, $\mathbf{C}=[0.75,0.25,0.0]$. The other six instances also share a score vector, with $1$ instance from class $1$, three from class $2$ and 2 instances from class $3$. As a result, they share the same calibrated probabilities $\mathbf{C}=[1/6, 3/6, 2/6]$. Given these values and considering Brier score, calibration loss is $0.19$ and refinement loss is $0.52$, which sum up to the Brier score of $0.71$, as expected. For log-loss the decomposition is $1.12 = 0.29 + 0.83$.

% {\color{red}(TODO: Calculate using toy example.)}

It is easy to see that a function that maps $\mathbf{S}$ to $\mathbf{C}$, known as a calibrator in Section \ref{sec:calibrators}, could potentially reduce calibration loss to $0$, consequently decreasing proper scoring rule loss. Refinement loss, on the other hand, is only zero if there are no ties between instances of different classes, i.e. they do not share the same value for $\mathbf{S}$. If that is the case, it is possible to map $\mathbf{S}$ to $\mathbf{C}$ such that it is perfectly confident and correct, i.e. $C_j = Y_j$.

Now suppose we knew the optimal model that outputs the true posterior class probabilities $\mathbf{Q}=[Q_1,Q_2,\ldots,Q_K]$, where $Q_j=\mathsf{E}[Y_j|\mathbf{X}]$, i.e. $Q_j$ is the true proportion of class $j$ among instances with feature values $\mathbf{X}$. Then the expected loss according to proper scoring rule $\phi$ can be decomposed into the sum of expected divergences between $\mathbf{S}$ and $\mathbf{Q}$ and $\mathbf{Q}$ and $\mathbf{Y}$:

\begin{align*}
    \mathsf{E} \Big[ \mathsf{d}\big(\mathbf{S}, \mathbf{\dot{Y}}\big)  \Big] = \mathsf{E} \Big[ \mathsf{d}\big(\mathbf{S}, \mathbf{Q}\big)\Big] + \mathsf{E} \Big[ \mathsf{d}\big(\mathbf{Q}, \mathbf{\dot{Y}}\big)  \Big],
\end{align*}
The first term in the sum is called epistemic loss \cite{senge2014reliable} and is the loss due to our model $\mathsf{f}(\mathbf{X})$ not being optimal. The second term is called irreducible or aleatoric loss \cite{senge2014reliable} and is the loss of the optimal model. Going back to the example in Table \ref{tab:evaluation:toy:psr}, for Brier score, epistemic loss is $0.26$ and irreducible loss is $0.45$. For log-loss the decomposition is $1.12 = 0.48 + 0.64$. The irreducible loss is only zero if the attributes of every instance $\mathbf{X}$ carry enough information to uniquely define the label $\mathbf{\dot{Y}}$. It is thus not possible to come up with a procedure to reduce the overall loss based on it. Additionally it would be unrealistic to do so based on epistemic loss. We are then naturally drawn to calibration loss as it is simple to interpret (we want our predicted probabilities of occurrence of an event to match the actual frequencies of occurrence) and also because we can easily estimate it with enough data. Thus, as discussed in the following section, visualisation and estimation of miscalibration have received considerable attention in the literature of probability evaluation and machine learning.


% {\color{red}(TODO: Connect to reliability diagrams (depends on the section's position).)}


% {\color{red}(TODO: Epistemic-irreducible.)}
%Other decompositions and why they're important


%  Let us once again return to our example from Table \ref{tab:evaluation:toy}. As mentioned before, a model that always outputs the class proportion will have a perfect ECE of 0, and that is what happens if we take class 1 as the positive class and constantly predict class probabilities equal to the class proportions. But while this gives $\text{binary-ECE}=0$ for class 1, the resulting log-loss is $0.6365$.
% % 
%  On the other hand, a different model which always outputs $0.9$ probability to the instances' true classes gets the reliability diagram shown in Figure \ref{fig:eval:reliability0.9}, with $\text{binary-ECE}=0.1$ for class 1, and $0.1054$ log-loss.
% %
% From the first to the second model, ECE increases (0 to 0.1), but log-loss decreases (0.6365 to 0.1054). This happens because proper scoring rules do not measure only calibration. In fact, they can be decomposed into terms with distinct interpretations \cite{kull2015}. 




%     \begin{figure}
%         \centering
%         \includegraphics[width=0.7\textwidth]{figures/evaluation/reliability-0.9-v2.pdf}
%         \caption{Binary reliability diagram of a model that always outputs $0.9$ probability for the true class of the instances in Table \ref{tab:evaluation:toy}.}
%         \label{fig:eval:reliability0.9}
%     \end{figure}



% An intuitive way to decompose proper scoring rules is into refinement (RL) and calibration losses (CL): $\mathsf{E}\left[\breve{\phi}\right] = \text{RL} + \text{CL}$. Refinement loss is the loss due to producing the same probability for instances from different classes (the second model reduces this loss), while calibration loss is the loss due to the difference between
% the probabilities predicted by the model and the observed class proportions among instances with the same output (the second model increases this loss).

% Since we don't usually know the real score distribution, we would need to once again rely on binning if we wanted to actually estimate refinement and calibration losses. Additionally, the terms are calculated (estimated) differently, depending on the proper scoring rule. Finally, the loss of the optimal classifier is not necessarily 0. This is due to irreducible loss, which is only 0 if the attributes provide enough information to uniquely determine the instances' right label Y, with probability 1 \cite{kull2015}.


%\subsection{Calibration metrics}
%    \subsubsection{First attempts to evaluate calibration}
%    \subsubsection{Binary}
%    \subsubsection{ECE}


\newpage

\section{Evaluation and visualisation of classifier calibration}
\label{sec:metrics}

In this section we present a range of approaches to evaluate and visualise calibration, and discuss the advantages and disadvantages of each.
In Section \ref{sec:met:1st} we explore the first steps towards measuring miscalibration, starting from the early work on weather forecast calibration, and discuss various approaches to visually inspect miscalibration.
Some of those early approaches have been later adapted and proposed as new calibration metrics which are discussed in the following sections.
We start with binary calibration in Section \ref{sec:met:bin} which will serve as a building block for the two multiclass calibration measures discussed in Sections \ref{sec:met:clw:ece} and \ref{sec:met:con:ece}.
% We finish this section discussing hypothesis tests for calibration in Section \ref{sec:met:hyp}.



%----------------------------------------------------%
%\subsection{First attempts to evaluate calibration}
\subsection{Visualising calibration}
\label{sec:met:1st}
%----------------------------------------------------%

% Calibration metrics and proper scoring rules can provide evidence of the quality of a model's calibration.
Several visualisation techniques have been proposed for easier inspection of the reliability of predictions at different score ranges.
In this section we summarise a range of approaches that have been proposed in the literature, from simple tabular inspection to the more recent reliability diagrams (see \citet{brocker2007} for an extended discussion of reliability diagrams).

Starting from the binary case, the basic idea has been to show the relation between a particular predicted score $\hat{s} \in [0, 1]$ for the positive class of a probabilistic classifier and the respective observed proportion of positives, which we denote by $\mathsf{\bar{y}}(\hat{s})$.
In order to compute a observed proportion of positives we require multiple samples with the same score $\hat{s}$. However, given that the scores are continuous variables, the probability of getting multiple samples with the same score is almost zero.
For that reason, the score space is commonly discretised into $M$ bins $\{\mathbb{B}_1, \dots, \mathbb{B}_M\}$, thus increasing the probability of having multiple samples per estimation range (perhaps by forcing each bin to have a minimum number of samples).
Then, we can obtain $M$ observed proportions of positives $\mathsf{\bar{y}}(\mathbb{B}_m)$ instead of one per score value $\hat{s}$.
% If we have an indicator variable for every bin with the indices of the scores that fall into it $\mathbb{I}_m \in \{i; \hat{s}_i \in \mathbb{B}_m\}$ we can compute the \emph{observed proportion of positives} in each bin as
% %
% \begin{equation}
%     \mathsf{\bar{y}}(\mathbb{B}_m) = \frac{\sum_{i \in \mathbb{I}_m} y_i}{\text{count}(\mathbb{I}_m)}.
% \end{equation}
% %
% Some of the first uses of \emph{observed proportion of positives} appeared in the context of weather forecast evaluation in the form of tabular data \cite{hallenbeck1920, brier1950}.
%\citet{hallenbeck1920} showed ten equally distributed bin boundaries with their respective number of forecasts, number of rains and percentage (See Figure \ref{tab:eval:hallenbeck1920:1}). 
See Table \ref{tab:eval:hallenbeck1920} for an early use of observed proportions of positives using equal-width bins of predicted probabilities. 

\begin{figure}
    % \begin{subfigure}{0.48\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{figures/evaluation/hallenbeck1920_tab1}
    %     \caption{Hallenbeck 1920}
    %     \label{tab:eval:hallenbeck1920:1}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}{0.48\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{figures/evaluation/brier1950_tab2}
    %     \caption{Brier 1950}
    %     \label{tab:eval:brier1950:2}
    % \end{subfigure}
    
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{sanders1963_fig1}
        \caption{\citep[Fig.~1]{sanders1963}}
        \label{fig:eval:sanders1963:1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{lichtenstein1976_fig6.jpg}
        \caption{\citep[Fig.~2]{lichtenstein1977calibration}}
        \label{fig:eval:lichtenstein1977:6}
    \end{subfigure}
    
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{brocker_2007_fig1}
        \caption{\citep[Fig.~1]{brocker2007}}
        \label{fig:eval:brocker2007:1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{brocker_2007_fig4}
        \caption{\citep[Fig.~4]{brocker2007}}
        \label{fig:eval:brocker2007:4}
    \end{subfigure}
    \caption{Different graphical representations of calibration-related information found in the literature.}
    \label{fig:eval:rd}
\end{figure}
    
Later work showed line plots instead of tabular data, with markers at the centre of each bin~\cite{sanders1963, lichtenstein1977calibration, lichtenstein1982, murphy1977reliability}; occasionally including the number of samples in each bin next to the markers (See Figure \ref{fig:eval:sanders1963:1}). Other authors showed the markers with size relative to the sample size~\cite{hagedorn2005}, or as a separate histogram next to the reliability diagram~\cite{niculescu-mizil2005}.
Line plots facilitate visual inspection of the discrepancy of the observed proportions of positives against a perfectly calibrated model, which corresponds to the diagonal.
However, positioning the markers at the centre of the bins can be misleading, as even perfectly calibrated scores may result in a \emph{visually} non-calibrated reliability diagram with a deviation of up to half the bin width from the diagonal~\cite{brocker2007} (See Figure \ref{fig:mean:vs:centre} for an example).
This may happen in cases in which the scores are not evenly distributed in each bin.
%
\begin{figure}
    \centering
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=1.0\linewidth]{rd_mean_score_vs_bin_centre_not_calibrated.pdf}
        \caption{Not calibrated example. $4$ samples with score $0$ from which $25\%$ are positive, and $4$ samples with score $1$ from which $75\%$ are positive.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=1.0\linewidth]{rd_mean_score_vs_bin_centre_calibrated.pdf}
        \caption{Calibrated example. $1$ sample with score $0$ from negative class, and $1$ sample with score $1$ from positive class.}
    \end{subfigure}
    \caption{
Simple example showing the maximum discrepancy in calibration error when using the centre of the bin for the marker instead of the average score of the bin. Both examples show only two bins $[0, 0.5)$ and $[0.5, 1]$.
\textbf{(a)} shows a model not calibrated, but using the centre of the bin (green dashed line) visually seems calibrated. The gap between the centre of the bin and the average score is maximum, which corresponds to half of the bin size with respect to the average score (red line).
\textbf{(b)} shows a calibrated model which seems uncalibrated if using the centre of the bin. The gap is again half of the bin size.
}
    \label{fig:mean:vs:centre}
\end{figure}
%
In order to alleviate this problem, later work centred the markers on the average predicted scores $\mathsf{\bar{s}}(\mathbb{B}_m)$ in each bin instead. % where
% %
% \begin{equation}
%     \mathsf{\bar{s}}(\mathbb{B}_m) = \frac{\sum_{i \in \mathbb{I}_m}\hat{s_i}}{\text{count}(\mathbb{I}_m)}.
% \end{equation}
% %

There are two main methods to group the predicted scores into bins to build reliability diagrams. The first one, commonly called \emph{width binning}, distributes scores into a number of  bins of the same width, choosing bin edges accordingly (e.g., 10 bins $[0, 0.1], (0.1, 0.2], \ldots, $ $(0.9, 1.0]$). Another method, called \emph{frequency binning} (also equal size or equal mass binning) groups the scores by keeping the same number of samples in each bin. Frequency binning can and will normally result in bins with different widths, but it ensures that all bins have the same ``weight'' when assessing the model's miscalibration.

Bin estimations have varying reliability, e.g., depending on the number of samples in the bin. 
One way to show this visually is by incorporating confidence intervals.
%If previous work showed the counts in text form (eg. in a table or next to the markers \cite{brier1950, sanders1963, murphy1977reliability}), later work also incorporated in the visualisation confidence intervals in the reliability diagram.
One of the simplest methods is to assume that each bin is sampled from a binomial distribution, and compute the corresponding confidence intervals of the observed proportion of positives (see Figure~\ref{fig:eval:pycalib:lines}).
However, making the assumption of fixed bins, score averages and proportion of positives is unrealistic; unless the score distribution is uniform (see \cite{brocker2007} for a detailed discussion).
More accurate intervals can be obtained by using the \emph{consistency resampling} method proposed by \citet{brocker2007}, which consists on sampling the scores with replacement several times in order to obtain multiple surrogate forecasts and observations and their respective quantiles.

More recently, binary reliability diagrams have been extended to the multiclass setting.
One method to show multiclass scores in a binary fashion consists in plotting only the \emph{confidence} of the model for each sample (the highest score among all possible classes). 
% and consider a positive prediction if the predicted class is correct, and negative otherwise.
%.showing only the highest score per sample and its corresponding class as the positive; which could still be  a wrong or right prediction.
This approach was already used for binary classification by
\citet{lichtenstein1977calibration}, reproduced here as Figure \ref{fig:eval:lichtenstein1977:6}. 
The figure shows a binary reliability diagram with scores in the range $[0.5,1]$
(with $K$ classes the confidence is never lower than $1/K$).
% and refers back to the work of \citet{Hazard1973}. {\color{red}(TODO: I can not find the pdf of Hazard1973, may need to check it.)}
% The specific score of the winning class is commonly referred as the \emph{confidence} value of the prediction.
%
Another example of the use of confidences in multiclass problems is the recent work of \citet{guo2017}, which shows the confidence for multiclass problems in the form of bar plots and the ECE and MCE metrics discussed below. 
% (which in this work we refer as confidence ECE and MCE).
%In this case, bins with probabilities lower than $1/K$ are always empty, where $K$ is the number of classes.
% \citet{guo2017} also show the deviations from the diagonal as red bars, which is a good way to highlight the mis-calibration but could be somewhat misleading as the area of such bars is not informative.
% Showing bars instead of lines is helpful to visually inspect the miscalibration, however, it is difficult to compare multiple models.
%
Finally, instead of collapsing all classes into a single diagram one could construct one reliability diagram per class as line plots or bars in a one-vs-rest manner \cite{kull2019} (see Figure \ref{fig:eval:pycalib:ter}).

\begin{figure}
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{pycalib_rd_bars.pdf}
        \caption{Reliability diagram with bars for each bin and red error gaps with regards to a perfectly calibrated model, and a histogram of the scores at the bottom.}
        \label{fig:eval:pycalib:bars}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{pycalib_rd_lines.pdf}
        \caption{Comparison of multiple calibration methods, with Clopper–Pearson binomial confidence intervals of 95\% in each observed proportion of positives.}
        \label{fig:eval:pycalib:lines}
    \end{subfigure}
    
    \begin{subfigure}{1.0\linewidth}
        \centering
        \includegraphics[width=\linewidth]{pycalib_rd_ternary.pdf}
        \caption{Multiple classes can be shown as one-vs-rest reliability diagrams.}
        \label{fig:eval:pycalib:ter}
    \end{subfigure}
    \caption{Examples of reliability diagrams using the Python library PyCalib}
    \label{fig:eval:pycal}
\end{figure}

%It is often also useful to show the number of samples in each bin in the form of a histogram next (or below) the reliability diagram in the form of a small histogram at the bottom of the reliability diagram, sharing the x-axis (as seen in {\color{red}[add references]}).\todo{MPN: fix}
%
%{\color{blue}
%MPN: We possibly need to reference the reliability diagram analysis of \cite{vaicenavicius2019evaluating} and their proposed one. And mention \cite{brocker2007} as the original idea? \cite{brocker2007} indicates that \cite{wilks2011statistical} has a great explanation of reliability diagrams.
%}
%

% All the following text in blue are notes
%\cite{Hallenbeck1920} shows a table with 10 bins and the number of rains, forecasts and actual percentage \ref{tab:eval:hallenbeck1920:1}
%
%\cite{brier1950} already used reliability diagrams in form of a table as it was enough to show 5 bins with their corresponding observed proportion of rain cases \ref{tab:eval:brier1950:2}
%
%\cite{sanders1963} is one of the first articles that show a reliability diagram depicting forecast probabilities agains observed relative frequencty of occurrence. However, the forecast probabilities always fall into a one decimal point, including zero and one (11 bins). Other figures show what it seems to be 21 bins but the first and last bins are empty.
%{\color{red} Need to understand what is the range of every bin, given that the boundaries may contain a smaller bin width.}. 
%The author also included the number of forecasts in every bin. Find out what are the numbers on the right y-axis in \ref{fig:eval:sanders1963:1}. Altough a reliability diagram is first presented, the rest of the article chooses to show departure from expectancy vs observed departure of relative frequency of occurrence \ref{fig:eval:sanders1963:2}.

%----------------------------------------------------%
% \subsection{Expected/Maximum calibration error}
%----------------------------------------------------%
    % \begin{itemize}
    %     \item As seen in the previous Section, each notion of calibration is related to a reliability diagram
    %     \begin{itemize}
    %         \item This can be used to visualise miscalibration on binned scores
    %     \end{itemize}
    %     \item We will now see how these bins can be used to measure miscalibration
    % \end{itemize}


    % \begin{itemize}
    %     \item We start by introducing a toy example:
    % \end{itemize}
    
    \begin{table}[!b]
        \begin{tabular}{lrrrr}
            \toprule
            {id} &  $\hat{s}_1$ &  $\hat{s}_2$ &  $\hat{s}_3$ &  $y$ \\
            \midrule
            1  &     1.0 &     0.0 &     0.0 &    1 \\
            2  &     0.9 &     0.1 &     0.0 &    1 \\
            3  &     0.8 &     0.1 &     0.1 &    1 \\
            4  &     0.7 &     0.1 &     0.2 &    1 \\
            5  &     0.6 &     0.3 &     0.1 &    1 \\
            6  &     0.4 &     0.1 &     0.5 &    1 \\
            7  &     1/3 &     1/3 &     1/3 &    1 \\
            8  &     1/3 &     1/3 &     1/3 &    1 \\
            9  &     0.2 &     0.4 &     0.4 &    1 \\
            10 &     0.1 &     0.5 &     0.4 &    1 \\
            \bottomrule
        \end{tabular}
        \hfill
        \begin{tabular}{lrrrr}
            \toprule
            {id} &  $\hat{s}_1$ &  $\hat{s}_2$ &  $\hat{s}_3$ &  $y$ \\
            \midrule
            11 &          0.8 &          0.2 &          0.0 &    2 \\
            12 &          0.7 &          0.0 &          0.3 &    2 \\
            13 &          0.5 &          0.2 &          0.3 &    2 \\
            14 &          0.4 &          0.4 &          0.2 &    2 \\
            15 &          0.4 &          0.2 &          0.4 &    2 \\
            16 &          0.3 &          0.4 &          0.3 &    2 \\
            17 &          0.2 &          0.3 &          0.5 &    2 \\
            18 &          0.1 &          0.6 &          0.3 &    2 \\
            19 &          0.1 &          0.3 &          0.6 &    2 \\
            20 &          0.0 &          0.2 &          0.8 &    2 \\
            \bottomrule
        \end{tabular}
        \hfill
        \begin{tabular}{lrrrr}
            \toprule
            {id} &  $\hat{s}_1$ &  $\hat{s}_2$ &  $\hat{s}_3$ &  $y$ \\
            \midrule
            21 &          0.8 &          0.2 &          0.0 &    3 \\
            22 &          0.8 &          0.1 &          0.1 &    3 \\
            23 &          0.8 &          0.0 &          0.2 &    3 \\
            24 &          0.6 &          0.0 &          0.4 &    3 \\
            25 &          0.3 &          0.0 &          0.7 &    3 \\
            26 &          0.2 &          0.6 &          0.2 &    3 \\
            27 &          0.2 &          0.4 &          0.4 &    3 \\
            28 &          0.0 &          0.4 &          0.6 &    3 \\
            29 &          0.0 &          0.3 &          0.7 &    3 \\
            30 &          0.0 &          0.3 &          0.7 &    3 \\
            \bottomrule
        \end{tabular}
        \caption{Class probabilities given by a classifier to 30 instances belonging to three different classes.}
        \label{tab:evaluation:toy}
    \end{table}

%----------------------------------------------------%
\subsection{Evaluating calibration error: the binary case}
\label{sec:met:bin}
%----------------------------------------------------%

% We define the binary \textit{estimated calibration error} \citep{roelofs2021mitigating}, also commonly called \textit{expected calibration error}, or binary-ECE \citep{naeini2015}, as the average gap across all bins in a reliability diagram, weighted by the number of instances in each bin, as given by Equation (\ref{eq:binaryECE}).


% In the past, most of the research on the calibration of probabilities has focused on binary classification problems. However, more recently multiclass calibration has got some attention and new metrics and visualisation tools have been proposed.
We now proceed with discussing how to measure calibration error. 
We will use the three-class toy problem in Table \ref{tab:evaluation:toy} throughout. 
In this section we convert it to a binary classification problem by taking class 1 as positive and classes 2 and 3 as negative. 
We then apply equal-width binning to the class 1 probabilities. 
% in order to separate class 1 probabilities and their corresponding labels into 5 bins, corresponding to intervals $[0, 0.2]$, $(0.2, 0.4]$, $(0.4, 0.6]$, $(0.6, 0.8]$, and $(0.8, 1.0]$. 
Table \ref{tab:evaluation:binary:bins} shows the resulting bins $\mathbb{B}_m$, $m \in \{1, \ldots, 5\}$, from which we calculate the number of instances in the bin denoted as $|\mathbb{B}_{m}|$, the average probability $\Bar{\mathsf{s}}(\mathbb{B}_{m})$, the proportion of positives $\Bar{\mathsf{y}}(\mathbb{B}_{m})$, and the absolute gap between them $|\Bar{\mathsf{y}}(\mathbb{B}_m) - \Bar{\mathsf{s}}(\mathbb{B}_m)|$. 


        \begin{table}[!b]
            \centering
            \small
            \begin{tabular}{lrllllc}
                \toprule
                 $\mathbb{B}_m$ &  $|\mathbb{B}_{m}|$ &  $\mathsf{s}(\mathbb{B}_{m})$ & $\Bar{\mathsf{s}}(\mathbb{B}_{m})$ & $\mathsf{y}(\mathbb{B}_{m})$                             & $\Bar{\mathsf{y}}(\mathbb{B}_{m})$ & $|\Bar{\mathsf{y}}(\mathbb{B}_m) - \Bar{\mathsf{s}}(\mathbb{B}_m)|$ \\
                \midrule
                 %$\mathbb{B}_1$ &         11 &  0.0, 0.0, 0.0, 0.0, 0.1, 0.1, 0.1,  \ldots &           0.10 &  0 (9), 1 (2) &             0.18 & 0.08\\
                 $\mathbb{B}_1$ &         11 &  $0.0^{(4)}$, $0.1^{(3)}$,  $0.2^{(4)}$ &           0.10 &  $0^{(9)}$, $1^{(2)}$ &             $0.18$ & 0.08\\
                 $\mathbb{B}_2$ &          7 &              $0.3^{(2)}$, $1/3^{(2)}$, $0.4^{(3)}$ &            0.35 &              $0^{(4)}$, $1^{(3)}$ &              0.43 & 0.08\\
                 %$\mathbb{B}_3$ &          3 &                                    0.5, 0.6, 0.6 &            0.57 &                          0 (2), 1 (1) &              $0.\arc{33}$ & 0.24\\
                 $\mathbb{B}_3$ &          3 &                                    0.5, 0.6, 0.6 &            0.57 &                          0, 0, 1 &              $0.33$ & 0.24\\
                 $\mathbb{B}_4$ &          7 &                $0.7^{(2)}$, $0.8^{(5)}$ &            0.77 &              $0^{(5)}$, $1^{(2)}$ &              0.29 & 0.48 \\
                 %$\mathbb{B}_5$ &          2 &                                         0.9, 1.0 &            0.95 &                             1 (2) &              1.00 & 0.05\\
                 $\mathbb{B}_5$ &          2 &                                         0.9, 1.0 &            0.95 &                             1, 1 &              1.00 & 0.05\\
                \bottomrule
            \end{tabular}
            
        \caption{Positive probabilities and corresponding instance labels separated into 5 bins. The probabilities were obtained by taking class 1 as the positive class in the multiclass problem in Table \ref{tab:evaluation:toy}. To reduce the width of the table, a number followed by a superscript parenthesis $X^{(Y)}$ indicates a list of number $X$ repeated $Y$ times.}
        \label{tab:evaluation:binary:bins}
    \end{table}
    
The values of $\Bar{\mathsf{p}}(\mathbb{B}_{m})$, $\Bar{\mathsf{y}}(\mathbb{B}_{m})$ and $|\Bar{\mathsf{y}}(\mathbb{B}_m) - \Bar{\mathsf{s}}(\mathbb{B}_m)|$ in Table \ref{tab:evaluation:binary:bins} can be used to draw the reliability diagram shown in Figure \ref{fig:eval:rel_diagram}, where we can see the red bars representing the calibration error at each bin.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.7\textwidth]{binary-reliability-v2.pdf}
    \caption{Reliability diagram corresponding to the 5 bins presented in Table \ref{tab:evaluation:binary:bins}.}
    \label{fig:eval:rel_diagram}
\end{figure}

Given the information about the bins in Table \ref{tab:evaluation:binary:bins} we could calculate an average of the bin-wise calibration error, which leads us to  binary estimated calibration error, as defined in  Definition \ref{def:binary:ece}.
%
\begin{definition}[Binary-ECE]
\label{def:binary:ece}
Binary \textit{estimated calibration error} \citep{roelofs2021mitigating}, or binary-ECE \citep{naeini2015}, is the average gap across all bins in a reliability diagram, weighted by the number of instances in each bin:
$$\mathsf{ECE}_{\text{binary}}  = \sum_{m=1}^M \frac{|\mathbb{B}_{m}|}{N} |\Bar{\mathsf{y}}(\mathbb{B}_{m}) - \Bar{\mathsf{s}}(\mathbb{B}_{m})|,$$
where $M$ and $N$ are the number of bins and instances, respectively. 
% $\mathbb{B}_{m}$ is the $m$-th probability bin, $|\mathbb{B}_{m}|$ denotes the size of the bin, and $\Bar{\mathsf{s}}(\mathbb{B}_{m})$ and $\Bar{\mathsf{y}}(\mathbb{B}_{m})$ are the average predicted probability and the proportion of positives in bin $\mathbb{B}_{m}$. 
Binary-ECE is also commonly called binary \textit{expected calibration error}, however this quantity is empirically estimated on a validation or test sample, which is why we prefer to call it binary \textit{estimated calibration error}.
\end{definition}
%
Binary-ECE aggregates part of the visual information about calibration error in Figure  \ref{fig:eval:rel_diagram} by taking the weighted mean of the sizes of these gaps. In this example, $\mathsf{ECE}_{\text{binary}} =0.1873$. 

Binary-ECE ranges from $0$ to $1$, with particular values including $\mathsf{ECE}_{\text{binary}} =\pi_1$ (proportion of positives) for a classifier that randomly outputs probability $1$ for one of the classes, $\mathsf{ECE}_{\text{binary}} =0$ for a perfect classifier that always predicts probability $1$ for the correct class or for a classifier that constantly outputs positive probability equal to $\pi_1$, and $\mathsf{ECE}_{\text{binary}} =1$ for a classifier that always assigns probability $1$ to the wrong class.

% \begin{equation}
% \label{eq:binaryECE}
%     \text{binary-ECE}  = \sum_{i=1}^M \frac{|B_{i}|}{N} |\Bar{y}(B_{i}) - \Bar{p}(B_{i})|,
% \end{equation}

% \noindent where $M$ and $N$ are the number of bins and instances, respectively, $B_{i}$ is the $i$-th probability bin, $|B_{i}|$ denotes the size of the bin, and $\Bar{p}(B_{i})$ and $\Bar{y}(B_{i})$ are the average predicted probability and the proportion of positives in bin $B_{i}$.

Instead of measuring how miscalibrated the model is on average, one might be interested in the worst case, in other words ``how maximally miscalibrated is the model''? In this case, one might use the binary maximum calibration error \citep{naeini2015}.
%
\begin{definition}[Binary-MCE]
\label{def:binary:mce}
Binary maximum calibration error (binary-MCE) is the maximum gap across all bins in a reliability diagram: $$\mathsf{MCE}_{\text{binary}} = \max_{m \in \{1, \ldots, M\}} |\Bar{\mathsf{y}}(\mathbb{B}_m) - \Bar{\mathsf{s}}(\mathbb{B}_m)|.$$
\end{definition}
%
In our example, Table \ref{tab:evaluation:binary:bins} and Figure \ref{fig:eval:rel_diagram} show that the fourth bin has the largest gap, with its size corresponding to $\mathsf{MCE}_{\text{binary}} = 0.48$. 

Binary-MCE can be very sensitive to bins with few instances, where the values of $\Bar{\mathsf{y}}(\mathbb{B}_m)$ and $\Bar{\mathsf{s}}(\mathbb{B}_m)$ are calculated based on very little information. In extreme cases with only a single instance in a bin, $\Bar{\mathsf{y}}(\mathbb{B}_m)$ will be the instance's actual label (1 or 0), potentially resulting in a large gap that would have a small weight in binary-ECE, while being the whole value of binary-MCE, meaning that the model would be evaluated based on its performance for a single instance.

% We can similarly define the maximum calibration error (binary-MCE) as the maximum gap across all bins in a reliability diagram, or

% \begin{equation}
% \label{eq:binaryMCE}
%     \text{binary-MCE} = \max_{i \in \{1, \ldots, M\}} |\Bar{y}(B_i) - \Bar{p}(B_i)|.
% \end{equation}


%----------------------------------------------------%
\subsection{Classwise calibration error}
\label{sec:met:clw:ece}
%----------------------------------------------------%

We now proceed to settings with more than two classes and start by defining the estimated calibration error corresponding to a single class $j$ in a multiclass task.

\begin{definition}[Class-$j$-ECE]
\label{def:class:j:ece}
Given a multiclass task with $K$ classes, class-$j$-ECE corresponds to the binary-ECE calculated by taking class $j$ as positive and the other $K-1$ classes together as a new negative class:
$$\mathsf{ECE}_{j}  = \sum_{m=1}^M \frac{|\mathbb{B}_{m,j}|}{N} |\Bar{\mathsf{y}}_j(\mathbb{B}_{m,j}) - \Bar{\mathsf{s}}_j(\mathbb{B}_{m,j})|,$$
where $\mathbb{B}_{m,j}$ is the $m$-th bin of class $j$.
\end{definition}

Once again we turn to our example in Table \ref{tab:evaluation:toy}. Following Definition \ref{def:class:j:ece}, we have already calculated class-$1$-ECE ($0.1873$) in our binary-ECE example. Now we need to calculate class-$2$-ECE and class-$3$-ECE. Tables \ref{tab:evaluation:binary2:bins} and \ref{tab:evaluation:binary3:bins} show the binary bins for classes $2$ and $3$, respectively, while the binary reliability diagrams of the three classes can be seen in Figure \ref{fig:eval:clas_rel_diagram}.

%\begin{table}[!b]
%    \centering
%    \small
%    \begin{tabular}{lrllllc}
%        \toprule
%         $\mathbb{B}_{m,2}$ &  $|\mathbb{B}_{m,2}|$ &                                              & $\Bar{\mathsf{s}}(\mathbb{B}_{m,2})$ &                                          & $\Bar{\mathsf{y}}(\mathbb{B}_{m,2})$ & $|\Bar{\mathsf{y}}(\mathbb{B}_m) - \Bar{\mathsf{s}}(\mathbb{B}_m)|$  \\
%        \midrule
%         $\mathbb{B}_{1,2}$ &         15 &  0.0$\times$(5), 0.1$\times$(5), 0.2$\times$(5) &           0.10 &  0$\times$(10), 1$\times$(5) &             0.33 & 0.23\\
%         $\mathbb{B}_{2,2}$ &         12 &  0.3$\times$(5), 1/3$\times$(2),  0.4$\times$(5) &           0.35 &           0$\times$(8), 1$\times$(4) &             0.33 & 0.02\\
%         $\mathbb{B}_{3,2}$ &          3 &                                    0.5, 0.6, 0.6 &            0.57 &                                      0, 0, 1 &              0.33 & 0.24\\
%         $\mathbb{B}_{4,2}$ &          0 &                                                  &             &                                              &             \\
%         $\mathbb{B}_{5,2}$ &          0 &                                                  &             &                                              &             \\
%        \bottomrule
%    \end{tabular}
%    \caption{Positive probabilities and corresponding instance labels separated into 5 bins. The probabilities were obtained by taking class 2 as the positive class in the multiclass problem in Table \ref{tab:evaluation:toy}.}
%        \label{tab:evaluation:binary2:bins}
%\end{table}

\begin{table}[!b]
    \setlength{\tabcolsep}{5pt}
    \centering
    \small
    \begin{tabular}{lrllllc}
        \toprule
         $\mathbb{B}_{m,2}$ &
         $|\mathbb{B}_{m,2}|$ &
         $\mathsf{s}(\mathbb{B}_{m,2})$&
         $\Bar{\mathsf{s}}(\mathbb{B}_{m,2})$&
         $\mathsf{y}(\mathbb{B}_{m,2})$ &
         $\Bar{\mathsf{y}}(\mathbb{B}_{m,2})$ &
         {\footnotesize $|\Bar{\mathsf{y}}(\mathbb{B}_m) - \Bar{\mathsf{s}}(\mathbb{B}_m)|$}  \\
        \midrule
         $\mathbb{B}_{1,2}$ &         15 &  $0^{(5)}$, $0.1^{(5)}$, $0.2^{(5)}$ &           0.10 &  $0^{(10)}$, $1^{(5)}$ &             0.33 & 0.23\\
         $\mathbb{B}_{2,2}$ &         12 &  $0.3^{(5)}$, $1/3^{(2)}$,  $0.4^{(5)}$ &           0.35 &           $0^{(8)}$, $1^{(4)}$ &             0.33 & 0.02\\
         $\mathbb{B}_{3,2}$ &          3 &                                    0.5, 0.6, 0.6 &            0.57 &                                      0, 0, 1 &              0.33 & 0.24\\
         $\mathbb{B}_{4,2}$ &          0 &                                                  &             &                                              &             \\
         $\mathbb{B}_{5,2}$ &          0 &                                                  &             &                                              &             \\
        \bottomrule
    \end{tabular}
    \caption{Positive probabilities and corresponding instance labels separated into 5 bins. The probabilities were obtained by taking class 2 as the positive class in the multiclass problem in Table \ref{tab:evaluation:toy}.}
        \label{tab:evaluation:binary2:bins}
\end{table}

\begin{table}[ht]
    \setlength{\tabcolsep}{5pt}
    \centering
    \small
    \begin{tabular}{lrllllc}
        \toprule
         $\mathbb{B}_{m,3}$ & 
         $|\mathbb{B}_{m,3}|$ &
         $\mathsf{s}(\mathbb{B}_{m,3})$ &
         $\Bar{\mathsf{s}}(\mathbb{B}_{m,3})$ &
         $\mathsf{y}(\mathbb{B}_{m,3})$ &
         $\Bar{\mathsf{y}}(\mathbb{B}_{m,3})$ &
         {\footnotesize
         $|\Bar{y}(\mathbb{B}_m) - \Bar{p}(\mathbb{B}_m)|$}\\
        \midrule
         $\mathbb{B}_{1,3}$ &         11 &  $0.0^{(4)}$, $0.1^{(3)}$, $0.2^{(4)}$ &           0.10 &  $0^{(7)}$, $1^{(4)}$ &             0.36 & 0.26\\
         $\mathbb{B}_{2,3}$ &         11 &  $0.3^{(4)}$, $1/3^{(2)}$, $0.4^{(5)}$ &           0.35 &  $0^{(9)}$, $1^{(2)}$ &             0.18 & 0.17\\
         $\mathbb{B}_{3,3}$ &          4 &                               0.5, 0.5, 0.6, 0.6 &            0.55 &                       0, 0, 0, 1 &              0.25 & 0.3\\
         $\mathbb{B}_{4,3}$ &          4 &                               0.7, 0.7, 0.7, 0.8 &            0.72 &                       0, 1, 1, 1 &              0.75 & 0.03\\
         $\mathbb{B}_{5,3}$ &          0 &                                                  &             &                                  &             \\
        \bottomrule
    \end{tabular}
    \caption{Positive probabilities and corresponding instance labels separated into 5 bins. The probabilities were obtained by taking class 3 as the positive class in the multiclass problem in Table \ref{tab:evaluation:toy}.}
        \label{tab:evaluation:binary3:bins}
\end{table}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth,trim=0 0 0 0, clip]{classwise-reliability-v2.pdf}
    \caption{Binary reliability diagram of each class in our running example. Note the empty bins in the second and third reliability diagrams, showing that the classifier never outputs high probabilities for these classes.}
    \label{fig:eval:clas_rel_diagram}
\end{figure}

\noindent From the values in Tables \ref{tab:evaluation:binary2:bins} and \ref{tab:evaluation:binary3:bins} and following Definition \ref{def:class:j:ece}, we get $\text{class-$2$-ECE} = 0.147$ and $\text{class-$3$-ECE} = 0.2017$. 

We can now define classwise-ECE \cite{kull2019}. 
%
\begin{definition}[Classwise-ECE]
\label{def:classwise:ece}
The estimated classwise calibration error (classwise-ECE) is the average class-$j$-ECE across all classes:
$$\mathsf{ECE}_{\text{classwise}}  = \frac{1}{K}\sum_{j=1}^K \mathsf{ECE}_{j}.$$
\end{definition}
%
According to Definition \ref{def:classwise:ece}, in our example $\text{classwise-ECE} = (0.1873 + 0.147 + 0.2017)/3 = 0.1787$.

% Confidence-ECE only cares about the calibration error associated with the winning class. In order to measure miscalibration for all classes, we can take the average binary-ECE across all classes, which gives the expected classwise calibration error (classwise-ECE) \cite{kull2019}. Formally, classwise-ECE is defined as the average gap across all classwise reliability diagrams, weighted by the number of instances in each bin, as shown in Equation (\ref{eq:classwiseECE}).

% \begin{equation}
%     \label{eq:classwiseECE}
%     \text{classwise-ECE}  = \frac{1}{K}\sum_{j=1}^K \sum_{i=1}^M \frac{|B_{i,j}|}{N} |\Bar{y}_j(B_{i,j}) - \Bar{p}_j(B_{i,j})|,
% \end{equation}

% \noindent where $B_{i,j}$ is the $i$-th bin of the $j$-th class, $|B_{i,j}|$ denotes the size of the bin, and  $\Bar{p}_j(B_{i,j})$ and $\Bar{y}_j(B_{i,j})$ denote the average prediction of class $j$ probability and the actual proportion of class $j$ in the bin $B_{i,j}$. The contribution of a single class $j$ to classwise-ECE is called class-$j$-ECE.

\begin{definition}[Classwise-MCE]
\label{def:classwise:mce}
The maximum classwise calibration error (classwise-MCE) \cite{kull2019} is defined as the maximum gap across all bins and all classwise-reliability diagrams:
$$
    \mathsf{MCE}_{\text{classwise}}  = \max_{j \in \{1, \ldots, K\}\, m \in \{1, \ldots, M\}}  |\Bar{\mathsf{y}}_j(B_{m,j}) - \Bar{\mathsf{s}}_j(B_{m,j})|.
$$
\end{definition}
%
% Equation (\ref{eq:classwiseMCE}) presents the maximum classwise calibration error (classwise-MCE), which is defined as the maximum gap across all bins and all classwise-reliability diagrams.
%
% \begin{equation}
%     \label{eq:classwiseMCE}
%     \text{classwise-MCE}  = \max_{j \in \{1, \ldots, K\}\, i \in \{1, \ldots, M\}}  |\Bar{y}_j(B_{i,j}) - \Bar{p}_j(B_{i,j})|.
% \end{equation}
%
In our running example, $\mathsf{MCE}_{\text{classwise}} = 0.48$. 

Note that this is not the only way to define classwise-MCE. For example, one could be interested in the average maximum gap across classes, i.e. an average class-$j$-MCE, which in our example would be $(0.48 + 0.24 + 0.3)/3 = 0.34$. As another variation, one could take the maximum class-$j$-ECE, which would then indicate the most miscalibrated class on average. In our example, this variation corresponds to class-$3$-ECE ($0.2017$).





% \begin{figure}
%     \centering
%     \includegraphics[width=0.7\textwidth]{figures/evaluation/perfect-reliability.png}
%     \caption{Reliability diagram of a classifier that predicts the  overall class distribution ($0.5$ in this case). The corresponding binary-ECE here is zero.}
%     \label{fig:eval:optim_ece}
% \end{figure}

Although classwise-ECE and MCE measure calibration error over all classes, they do not take into account the miscalibration that arises from every possible relationship between classes. For a true multiclass-ECE, we could bin the probability vectors in simplex space and then calculate the gaps between the average probability vector and the vector of class proportions in each bin. Although this seems like the right thing to do when evaluating multiclass calibration, it might not be efficiently computable with large numbers of classes, as the number of bins can be prohibitively high and most bins would likely be empty.

Similarly to binary-ECE, a value of $\text{classwise-ECE} = 0$ can be obtained by a classifier that constantly outputs the class proportions. For example, if a classifier always predicts $1/3$ setosa, $1/3$ versicolor and $1/3$ virginica for Fisher's Iris dataset, the resulting classwise-ECE will be $0$.
% Another limitation of all ECE/MCE measures is that optimising them can be as simple as predicting the overall class distribution, regardless of the given instance, as shown in Figure \ref{fig:eval:optim_ece}.



%----------------------------------------------------%
\subsection{Confidence calibration error}
\label{sec:met:con:ece}
%----------------------------------------------------%

As already mentioned, some calibration measures only consider a model's confidence, defined as
the maximum value in the predicted probability vector, i.e. the probability given to the winning class. Prediction confidence is not a new idea and has been around since at least the 1970s. \citet{lichtenstein1977calibration} called it the half-range method in the binary case (referred to as ``two alternatives'' in the paper) and it was also mentioned as one of the variations of the multiclass task, which the authors called ``three or more alternatives''. 
More recently it has been popularised by \citet{guo2017}.
    
    To calculate confidence-ECE, we first bin the confidence values and, for each instance of each bin, we produce a binary value indicating if the classifier predicted correctly or not.
    Recalling the example from Table \ref{tab:evaluation:toy}, the resulting confidence bins are presented in Table \ref{tab:evaluation:confidence:bins}, where $\Bar{\mathsf{p}}(\mathbb{B}_{m})$ and $\mathsf{acc}(\mathbb{B}_{m})$ are respectively the average confidence and prediction accuracy in bin $\mathbb{B}_{m}$, with the corresponding reliability diagram in Figure \ref{fig:eval:rel_diagram2}.
    Note that bin $\mathbb{B}_1$ is empty, which demonstrates that confidence-ECE and confidence reliability diagrams are different from binary-ECE even on two-class problems. 
        
        \begin{table}[ht]
        \centering
        \small
        \begin{tabular}{lrllllc}
            \toprule
             $\mathbb{B}_m$ &
             $|\mathbb{B}_{m}|$ &
             $\mathsf{s}(\mathbb{B}_{m})$ &
             $\Bar{\mathsf{s}}(\mathbb{B}_{m})$ &
             $\mathsf{y}(\mathbb{B}_{m})$ &
             $\mathsf{acc}(\mathbb{B}_{m})$ &
             $|\mathsf{acc}(\mathbb{B}_m) - \Bar{\mathsf{p}}(\mathbb{B}_m)|$ \\
            \midrule
             $\mathbb{B}_1$ &          0 &                                                  &             &                                  &             \\
             $\mathbb{B}_2$ &          7 &              $1/3^{(2)}$, $0.4^{(5)}$ &            0.38 &              $0^{(4)}$, $1^{(3)}$ &              0.43 & 0.05\\
             $\mathbb{B}_3$ &         10 &  $0.5^{(4)}$, $0.6^{(6)}$ &           0.56 &     $0^{(7)}$, $1^{(3)}$ &             0.30 & 0.26\\
             $\mathbb{B}_4$ &         11 &  $0.7^{(5)}$, $0.8^{(6)}$ &           0.75 &  $0^{(6)}$, $1^{(5)}$ &             0.45 & 0.3\\
             $\mathbb{B}_5$ &          2 &                                         0.9, 1.0 &            0.95 &                             1, 1 &              1.00 & 0.05\\
            \bottomrule
        \end{tabular}\caption{Confidence bins corresponding to the toy example from Table \ref{tab:evaluation:toy}. The binary values in the fifth column indicate if the classifier correctly classified each instance. }
        \label{tab:evaluation:confidence:bins}
        \end{table}
        
   

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.7\textwidth]{confidence-reliability-v2.pdf}
    \caption{Confidence reliability diagram corresponding to the bins in Table \ref{tab:evaluation:confidence:bins}.}
    \label{fig:eval:rel_diagram2}
\end{figure}

\begin{definition}[Confidence-ECE]
    \label{def:confidence:ece}
    Confidence-ECE is the average difference between accuracy and average confidence across all bins in a confidence reliability diagram, weighted by the number of instances in each bin: $$\mathsf{ECE}_{\text{confidence}}  = \sum_{m=1}^M \frac{|\mathbb{B}_{m}|}{N} |\mathsf{acc}(\mathbb{B}_{m}) - \Bar{\mathsf{p}}(\mathbb{B}_{m})|.$$
    \end{definition}
    %
    We then calculate confidence-ECE as the weighted mean of the gaps between average confidence and prediction accuracy at each bin, thus $\mathsf{ECE}_{\text{confidence}}=0.2117$, while the maximum confidence calibration error (confidence-MCE) corresponds to the largest gap, i.e. $\mathsf{MCE}_{\text{confidence}}=0.3$. As with binary-ECE and for the same reasons, confidence-MCE is very sensitive to small bins, but in this particular example, its value corresponds to the gap of the largest bin.
    


%\todo{TSF: please add concluding paragraph}

As we show in Section \ref{sec:calibrators}, there is a wide range of post-hoc calibration techniques in the literature, each one capable of handling different miscalibration patterns. Thus, it can be useful to first analyse a model's reliability diagram, as it allows us to diagnose model miscalibration, i.e. in what probability ranges it is underconfident or overconfident, and this can help choose an appropriate calibration method. In addition, any of the ECE measures discussed in this Section  can be used to decide if a classifier actually needs to be calibrated, by testing the hypothesis that the model is already calibrated, as shown in Section \ref{sec:hyp}. \newtext{Finally, it is important to consider that all ECE/MCE measures can provide very different values given different number of bins, as shown in Figs. \ref{fig:hallenbeck-rel} and \ref{fig:hallenbeck2-rel}, and they can be minimised by predicting the overall class distribution, regardless of the given instance. Thus, it is good practice to use them together with the proper scoring rules presented in Section \ref{sec:psr}, to get a full evaluation of the probabilities produced by a model.}





%----------------------------------------------------%




==> mlj_files/04_calibrators.tex <==
\section{Calibration methods}
\label{sec:calibrators}

In this section we provide a systematic review of standard approaches to calibrating classifiers through the construction of calibration maps.
In particular, we focus on post-hoc calibration methods for classification, which can be used to adjust probability outputs separately from the initial training process.
For each method, we cover the mathematical formulation, the objective function for learning the map, and the predictive function to calculate the class probabilities for a new instance.
We include a few test cases to empirically analyse each method, and discuss their advantages and disadvantages.
General guidance on each method's implementation is also discussed, addressing issues such as overfitting and computational effort.
At the end of the section, we briefly describe some related work to classifier calibration, such as methods that can improve the calibration level during training time, methods that are designed for getting well-calibrated probability for other predictive tasks, and approaches that are designed for specific tasks in areas such as computer vision and natural language processing. 

\subsection{Preliminaries}

We denote a calibration map as a function $\mathsf{g}: \mathbb{S}_{\mathbb{Y}} \rightarrow \mathbb{P}_{\mathbb{Y}}$. 
Here $\mathbb{Y} =\{1, \dots, K\}$ is the discrete space with $K$ classes of the target variable.
$\mathbb{P}_{\mathbb{Y}}$ denotes the probability vector space on $\mathbb{Y}$, that is: $\mathbb{P}_{\mathbb{Y}} = \{ [s_1, \dots, s_K] \mid s_j \geq 0, \sum_{j=1}^{K} s_j = 1\}$.  
$\mathbb{S}_{\mathbb{Y}}$ represents the original output space of the (uncalibrated) classifier, which can take various forms depending on the formalisation of the classifier.
For instance, for a typical probabilistic classifier, we have $\mathbb{S}_{\mathbb{Y}} = \mathbb{P}_{\mathbb{Y}}$.
A one-vs-rest SVM might produce $K$-dimensional vectors in $\mathbb{S}_{\mathbb{Y}} = \mathbb{R}^{K}$.
Deep neural networks can also provide unnormalised vector outputs before the softmax is performed at the final layer. 
Calibration maps that work with such vector spaces are referred to as scaling approaches.
The name suggests these approaches are used to scale the vector output into a probability output, which is quite useful for models like SVMs, as the hinge loss does not optimise probability estimates by default.
However, other than the name and historical motivation, in modern applications, probability calibrators and scaling approaches can be used interchangeably, as the probability space and vector space can be transformed into each other by using the link function (e.g. softmax) and inverse link function (e.g. logit transform ). 

In general, to obtain a calibration map, we will have a calibration set with uncalibrated probabilities and labels, denoted as $\mathbb{C} = \{(\mathbf{s}_1, y_1), \dots, (\mathbf{s}_N, y_N)\}$, and an objective function $\mathsf{L}(\mathbb{C})$ to optimise.
Typically, the objective function is constructed using proper scoring rules, that is, $\mathsf{L}(\mathbb{C}) = \sum_{i=1}^{N} \phi(\mathbf{s}_i, y_i)$, and it can be optimised via various gradient descent algorithms.


\newtext{
\textbf{Training Schemes}: While the above notation suggested that the calibration map can be obtained by fitting a calibrator on a given hold-out calibration set, in practice a small training set and calibration set might lead to over-fitting thus limiting the performance of the calibrated model.
A typical solution here is to introduce multi-fold dataset splits as introduced in \cite{platt99probabilisticoutputs}.
The author proposes to divide the training sets into three different folds and fit the model and calibration map in cross-validation.
Two folds are used to train the uncalibrated model, and the model predictions on the last fold are collected and used to fit the calibration map.
This training process thus ends up with three pairs of models and calibration maps.
At test time each instance will be predicted with all three pairs, and resulting probabilities are averaged to give the final estimate.
Alternatively, people have also used applied label smoothing \cite{muller2019does} to reduce the level of overfitting and over-confidence.
The idea is to have a weighted average between the original probability vector (either from the uncalibrated model or after a calibration method has been applied) and a uniform probability vector.
Therefore, the final probability vector will be pushed somewhat towards the uniform probability vector, which avoids overly high confidence for unsuitable cases.}


\subsection{Two-Class Test Cases}

We designed some test cases to illustrate each calibration map's characteristics empirically.
These test cases are designed with a known distribution and allow us to directly sample the instances.
For ease of understanding, we consider a scenario with a univariate feature ($ \mathbf{x} \in \mathbb{R}$), so that we can inspect the fitted functions and reliability diagrams by means of $x$-$y$ plots.

% \subsubsection*{Binary Test Cases}
Figure~\ref{fig:test_dataset} depicts the probability density functions for the synthetic two-class dataset, as well as the posterior class probabilities when predicting any new instances.
%The density functions are constructed with a mixture of Gaussian distributions, and the class prior is set to be equal to construct the joint dataset distribution.
The generative model is equally likely to produce a positive and a negative, and the distribution of the feature values are mixtures of two normal distributions within each class. 
% is a mixture of Gaussian distributions N(-4,960) and N(64,1280) for positives and a mixture of Gaussian distributions N(4,980) and N(-72,1024) for negatives. 
Denoting the mixture components as $H=1$ and $H=2$, our generative model can be formally written down as:
%
\begin{align*}
    Y &\sim \text{Bernoulli}(0.5) \\
    H &\sim \text{Bernoulli}(0.5) \\
    X \mid Y=1, H=1 &\sim \text{Gaussian}(-4, 960) \\
    X \mid Y=1, H=2 & \sim \text{Gaussian}(64, 1280) \\
    X \mid Y=2, H=1 & \sim \text{Gaussian}(4, 980) \\
    X \mid Y=2, H=2 & \sim \text{Gaussian}(-72, 1024) \\
\end{align*}


\begin{figure}[!tbp]
    \centering
    %\includegraphics[width=0.6\textwidth]{figures/calibrators/data_distribution.png}
    %\includegraphics[width=0.273\textwidth]{figures/calibrators/data_prediction.png}
    \includegraphics[width=0.61\textwidth, valign=t]{data_distribution.png}
    \includegraphics[width=0.33\textwidth, valign=t]{data_prediction.png}
    \caption{The synthetic dataset used in the test cases. The left two figures shows the data distribution for each class respectively. The figure on the right gives the Bayes-optimal posterior probability for class 1.}
    \label{fig:test_dataset}
\end{figure}

%\todo[inline]{MPN: I have modified the images in Figure \ref{fig:test_dataset}. Should I put the previous figures back?}

\noindent
This generative assumption allows us to approximate the `true' reliability diagram closely for every test case and provides better insights into each calibration map. Specifically, we generate a large number of random samples and use small bin sizes to approximate a smooth reliability diagram.

We consider three cases for binary classification, each of which may occur in practice. 
The first two cases are hypothetical over/under-confident scenarios using a logistic regression model of the form 
    $\hat{\mathsf{f}}(x) = (1 + \exp(-a\cdot x))^{-1}$.
Such a model puts the decision boundary at $x=0$, which is nearly Bayes-optimal for the synthetic data. 
The model confidence can be moderated with the parameter $a$, and we will use the following two cases: 
%
\begin{align*}
    \hat{\mathsf{f}}_{\text{under}}(x) = \frac{1}{1 + \exp(-0.01\cdot x)} \\
    \hat{\mathsf{f}}_{\text{over}}(x) = \frac{1}{1 + \exp(-0.05\cdot x)}
\end{align*}
%
The third case is obtained with an MLP classifier as implemented by the scikit-learn Python package.
The model is specified with a two layer structure with 128 hidden units per layer.
The activation is selected as the ReLU function.
The remaining settings are left at their default values.
$10,000$ instances are sampled to train the model.

The smoothed reliability diagrams for these three cases are shown in Figure~\ref{fig:binary_test_cases}.
In the under-confident case the output probabilities barely reach the outside of the interval $[0.1, 0.9]$.
The reliability diagram shows a higher slope compared with the perfectly calibrated  one (the diagonal).
In contrast, the over-confident case has a shallower slope around the middle compared with the diagonal.
It further causes the reliability diagram to have sharp transitions while approaching the extremes. 
For the MLP case, we can observe both under-confident and over-confident regions throughout the reliability diagram.
%As we have seen with the previous two test cases, before the 0.5 on the horizontal axis, if the reliability diagram falls below the diagonal, it indicates under-confident, and vice versa.
%After the 0.5 on the horizontal axis, having the reliability diagram above the diagonal becomes the sign of under-confident, and vice verse.
This specific MLP classifier tends to be under-confident around $s \in [0, 0.1]$ and $s \in [0.65, 1]$, and mostly over-confident elsewhere.

\begin{figure}[!tbp]
    \centering
    %\includegraphics[width=0.28\textwidth]{figures/calibrators/test_case_1.png}
    %\includegraphics[width=0.28\textwidth]{figures/calibrators/test_case_2.png}
    \includegraphics[width=0.3\textwidth, valign=t]{test_case_1.png}
    \includegraphics[width=0.3\textwidth, valign=t]{test_case_2.png}
    %\includegraphics[width=0.28\textwidth]{figures/calibrators/test_case_3.png}
    \includegraphics[width=0.3\textwidth, valign=t]{test_case_3.png}
    \caption{The reliability diagrams of the three uncalibrated classifiers. The left figure shows the $\hat{\mathsf{f}}_{\text{under}}$ case, where the classifier predicts a probability closer to 0.5 compared with the Bayes-optimal case (Fig.~\ref{fig:test_dataset}, right), resulting in a reliability diagram with steeper slope. The middle figure shows the $\hat{\mathsf{f}}_{\text{over}}$  case, where the predicted probabilities are pushed towards $0$ and $1$ respectively, resulting in a shallower reliability curve. The right figure is obtained with a MLP classifier ($\hat{\mathsf{f}}_{\text{MLP}}$), where the reliability diagram shows over-confident and under-confident predictions around different regions. 
    }
    \label{fig:binary_test_cases}
\end{figure}

%\todo[inline]{MPN: Decide if should increase the font size of all figures (I have changed Fig. 12 Test Case 1, 2 and 3 as an example).}

\subsection{Calibration for Binary Classification}

We start with methods that can learn calibration maps for binary problems.
In binary classification, probability estimates are scalars, so the calibration maps are functions mapping from $[0, 1]$ to $[0, 1]$.
Here we describe four widely applied methods in detail: empirical binning, isotonic regression, logistic calibration and Beta calibration.  
Other approaches will be be briefly mentioned at the end of this section.

\subsubsection*{Empirical Binning}

Empirical binning \newtext{\cite{zadrozny2001obtaining,naeini2015}} is one of the simplest methods to build a calibration map.
It directly connects to the previously introduced ECE measure, which evaluates the calibration level by calculating the empirical frequencies within a set of score intervals. 
Therefore, binning approaches can directly optimise a variant of ECE depending on how the binning scheme is selected.

\begin{figure}[!tbp]
    \centering
    \begin{subfigure}{\textwidth}
    \centering
    %\includegraphics[width=0.28\textwidth]{figures/calibrators/Case1_EMP10_prediction.png}
    \includegraphics[width=0.28\textwidth]{Case1_EMP10_calibration.png}
    \includegraphics[width=0.28\textwidth]{Case1_EMP10_reliability.png}
    \caption{Test case 1: under-confidence}
    \end{subfigure}
    
    
    \begin{subfigure}{\textwidth}
    \centering
    %\includegraphics[width=0.28\textwidth]{figures/calibrators/Case2_EMP10_prediction.png}
    \includegraphics[width=0.28\textwidth]{Case2_EMP10_calibration.png}
    \includegraphics[width=0.28\textwidth]{Case2_EMP10_reliability.png}
    \caption{Test case 2: over-confidence}
    \end{subfigure}
    
    \begin{subfigure}{\textwidth}
    \centering
    % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case3_EMP10_prediction.png}
    \includegraphics[width=0.28\textwidth]{Case3_EMP10_calibration.png}
    \includegraphics[width=0.28\textwidth]{Case3_EMP10_reliability.png}
    \caption{Test case 3: MLP classifier}
    \end{subfigure}
    
    \caption{Examples of empirical binning calibration with 10 equal-width bins. As the binning approach can only give discrete outputs, we can observe the probabilities after calibration are no longer continuous and are only presented with 10 values or less (the under-confidence case has fewer values as there are no observations in bins closer to the extremes. The reliability diagrams show that the calibration method works well with all three test case, with most points being close to the calibrated diagonal.  }
    \label{fig:test_emp10}
\end{figure}

% \begin{figure}[!tbp]
%     \centering
%     \begin{subfigure}{\textwidth}
%     \centering
%     %\includegraphics[width=0.28\textwidth]{figures/calibrators/Case1_EMP32_prediction.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/Case1_EMP32_calibration.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/Case1_EMP32_reliability.png}
%     \caption{Test case 1: under-confidence}
%     \end{subfigure}
    
    
%     \begin{subfigure}{\textwidth}
%     \centering
%     %\includegraphics[width=0.28\textwidth]{figures/calibrators/Case2_EMP32_prediction.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/Case2_EMP32_calibration.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/Case2_EMP32_reliability.png}
%     \caption{Test case 2: over-confidence}
%     \end{subfigure}
    
%     \begin{subfigure}{\textwidth}
%     \centering
%     % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case3_EMP32_prediction.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/Case3_EMP32_calibration.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/Case3_EMP32_reliability.png}
%     \caption{Test case 3: MLP classifier}
%     \end{subfigure}
    
%     \caption{Examples of empirical binning calibration with 32 equal-width bins. With a higher number of bins, the discrete probabilities appear to be denser, and the predictions fits the ground-truth better. On the other hand, as we have less samples within each bin, some bins might have a poorer estimates than the 10-bins case. This is more observable with the over-confidence case, where we have less observations around the middle region.}
%     \label{fig:test_emp32}
% \end{figure}

For a typical setting, the empirical binning approach comes with the following parameters. 
(1) Bins: $\{\mathbb{B}_1, \dots, \mathbb{B}_M \}$, where each bin $\mathbb{B}_m \subset [0, 1]$ is an interval of probability range, and $\cup_{m=1}^{M} \mathbb{B}_m = [0, 1]$.
(2) Probability estimates in the bins:  $\mathbf{a}=\{a_1,\dots,a_{M}\}$, where $a_m \in [0, 1]$ specifies the calibrated probability value in each bin.
We usually assume that these bins do not overlap with each other. 
To make a prediction based on an uncalibrated probability $s$, empirical binning uses the following functional form:
%
\begin{align}
% \mathsf{c}(p; B_1, \dots, B_M, \mathbf{a}) = \sum_{j=1}^{M} \mathbb{I}(p\in \mathbb{B}_j) \cdot a_j
\mathsf{g}(s; \mathbb{B}_1, \dots, \mathbb{B}_M, \mathbf{a}) = a_m \quad \quad \quad \text{if}\ s \in \mathbb{B}_m
\end{align}
%
Here $ s \in \mathbb{B}_m$ means that the uncalibrated probability $s$ falls within $\mathbb{B}_m$.

Fitting a binning calibration map can be done by optimising $\mathbf{a}$ using ECE as a loss function: 
%
\begin{align}
%\mathbb{L}(\mathbf{a}) = \sum_{j=1}^{M} \Big | \frac{\sum_{i=1}^{N} \mathbb{I}(p_i \in B_j) \cdot y_i}{|B_j|} - a_j \Big|
\mathbf{a}^* &
= \arg\min_{\mathbf{a}} \mathsf{L}(\mathbf{a}) \\
\mathsf{L}(\mathbf{a}) &= \mathsf{ECE}(\mathbf{a}) 
                       = \sum_{m=1}^{M} \Big | \bar{\mathsf{y}}(\mathbb{B}_m) - a_m \Big|
\end{align}
%
Here $\bar{\mathsf{y}}(\mathbb{B}_m)$ represents the empirical frequency within $\mathbb{B}_m$ as defined in the previous section.  
The equation hence indicates that we want to assign each $a_m$ according to the empirical frequency of the labels within each bin $\mathbb{B}_m$.

We empirically analyse the binning approach with a simple setting of $M=10$ equal-width bins.  
The results with the three test cases are shown in Figure~\ref{fig:test_emp10}.
The binning approach performs well on most points, as the reliability diagram are close to the diagonal  after calibration.
However, it should be noted that the output probabilities can only take $M$ different values.
Therefore, while the final probabilities are calibrated,  we can no longer distinguish instances that receive different predictions from the uncalibrated model.
In other words, binning approaches can reduce the calibration loss at the cost of a higher grouping loss \cite{kull2015novel}.
% According to the data points pictured at the bottom of the figure, we can see this poor performance is mainly caused by the lower amounts of data points around these regions.
% As the test case 2 is designed to be an over-confident example, predictions are more pushed towards either $0$ or $1$ depending on their actual classes, causing the regions around $0.2$ and $0.8$to be emptier than the rest, further causing the bin estimates to be worse for these regions. 

While here we illustrated the binning approach with equal-width bins, it is possible to use other binning schemes such as equal-frequency binning.
For example, \cite{naeini2015} propose a Bayesian binning approach.

To summarise, the main advantages of binning approaches are as follows:
(1) They can be used to directly minimise a specific variant of ECE, hence are useful when calibration loss is of primary concern.
(2) Training is reasonably fast and straightforward. 
(3) Given its non-parametric nature, it does not have any constraint on the form of the calibration maps and therefore can capture arbitrary shapes according to the given bins.
In addition, other binning strategies can also be applied to deal with different datasets and uncalibrated models. %such as equal-frequency binning and Bayesian binning \cite{naeini2015}.



\subsubsection*{Isotonic Calibration}

Calibration by means of isotonic regression is another widely used non-parametric approach \newtext{\cite{barlow1972isotonic,niculescu-mizil2005,naeini2016}}.
The isotonic approach was originally proposed to solve univariate regression tasks where the function were required to be monotonic.
In the case of probability calibration, if we assume the uncalibrated model has a monotonic reliability diagram, then isotonic regression is a suitable approach to achieve a better level of calibration. 

Isotonic regression achieves a monotonic fit by estimating a set of non-decreasing constant segments, corresponding to a set of bins of varying width.  
Isotonic regression can therefore be described with the following parameters:
(1) Bin boundaries: $\mathbf{b}=(b_1,\dots,b_M)$, $b_j \in [0, 1], b_j < b_{j+1}$, and  (2) Edge values:  $\mathbf{v}=(v_1,\dots,v_{M})$, $ v_j \in [0, 1], v_j \leq v_{j+1}$.
As indicated by the parameters, isotonic regression is quite close to an empirical binning approach.
The main difference is that instead of having a pre-defined set of bin edges, isotonic regression learns these bin boundaries from the data.
As a result, isotonic regression can have an variable number of bins depending on the training set.
To calibrate a probability $s$, isotonic regression uses the following predictive function: 
%
\begin{align}
%c(p; \mathbf{b}, \mathbf{v}) = & \frac{1}{\sum_{j=1}^{M-1} \mathbb{I}(p\geq b_j)\cdot\mathbb{I}(p\leq b_{j+1})} \\ \nonumber
%&\sum_{j=1}^{M-1} \mathbb{I}(p\geq b_j)\cdot\mathbb{I}(p<b_{j+1}) \cdot \Big(v_j + \frac{p-b_j}{b_{j+1}-b_j}(v_{j+1} - v_j)\Big) 
\mathsf{g}(s; \mathbf{b}, \mathbf{v}) = \sum_{m=1}^{M-1} \mathsf{I}(s\geq b_m)\cdot\mathsf{I}(s<b_{m+1}) \cdot m_j 
\end{align}
%

\begin{figure}[!tbp]
    \centering
    \begin{subfigure}{\textwidth}
    \centering
    %\includegraphics[width=0.28\textwidth]{figures/calibrators/Case1_ISO_L_prediction.png}
    \includegraphics[width=0.28\textwidth]{Case1_ISO_L_calibration.png}
    \includegraphics[width=0.28\textwidth]{Case1_ISO_L_reliability.png}
    \caption{Test case 1: under-confidence}
    \end{subfigure}
    
    
    \begin{subfigure}{\textwidth}
    \centering
    % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case2_ISO_L_prediction.png}
    \includegraphics[width=0.28\textwidth]{Case2_ISO_L_calibration.png}
    \includegraphics[width=0.28\textwidth]{Case2_ISO_L_reliability.png}
    \caption{Test case 2: over-confidence}
    \end{subfigure}
    
    \begin{subfigure}{\textwidth}
    \centering
    % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case3_ISO_L_prediction.png}
    \includegraphics[width=0.28\textwidth]{Case3_ISO_L_calibration.png}
    \includegraphics[width=0.28\textwidth]{Case3_ISO_L_reliability.png}
    \caption{Test case 3: MLP classifier}
    \end{subfigure}
    
    \caption{Examples of isotonic calibration trained with 10,000 samples. Compared with empirical binning, we can see the isotonic approach can provide a larger variety of outputs in the continuous interval of $[0, 1]$, and different bins can be automatically learnt according to the observations. The calibration method works reasonably well on all three test cases. The over-confidence case still has some errors around around the middle-left and middle-right boundaries, due to the lack of training points within these areas. }
    \label{fig:test_iso_L}
\end{figure}


% \begin{figure}[!tbp]
%     \centering
%     \begin{subfigure}{\textwidth}
%     \centering
%     % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case1_ISO_S_prediction.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/Case1_ISO_S_calibration.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/Case1_ISO_S_reliability.png}
%     \caption{Test case 1: under-confidence}
%     \end{subfigure}
    
    
%     \begin{subfigure}{\textwidth}
%     \centering
%     % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case2_ISO_S_prediction.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/Case2_ISO_S_calibration.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/Case2_ISO_S_reliability.png}
%     \caption{Test case 2: over-confidence}
%     \end{subfigure}
    
%     \begin{subfigure}{\textwidth}
%     \centering
%     % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case3_ISO_S_prediction.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/Case3_ISO_S_calibration.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/Case3_ISO_S_reliability.png}
%     \caption{Test case 3: MLP classifier}
%     \end{subfigure}
    
%     \caption{Examples of isotonic calibration trained with 1,000 samples. We can see from the reliability diagram that the calibration performance is significantly worse than the previous example with 10,000 samples. Being a non-parametric approach, the isotonic calibration is more suitable on larger datasets.}
%     \label{fig:test_iso_S}
% \end{figure}

The three test cases on istonic regression are shown in Figure~\ref{fig:test_iso_L}.
To compare with the empirical binning approach again, while in the empirical case we have a constant prediction within each bin, we can see the prediction of the isotonic approach depends on the two values on the bin edges.
In the case where the two bin edges do not share the same value, isotonic regression performs linear interpolation to calculate the predicted value. 
This behaviour is due to the way that the isotonic approach is estimated. 
To ensure the estimated function is monotonically increasing, the learning algorithm starts with the first bin edge as the minimal feature value ($0$ in the case of an isotonic calibration) and extends the following bin edges until it sees a higher target value (this is also referred to as `pooling adjacent violators' \cite{fawcett2007}).
It can be proven that, with monotonic sets of $\mathbf{b}$ and $\mathbf{s}$, the learning algorithm is equivalent to optimising the following loss \cite{ayer1955empirical}: 
%
\begin{align}
\mathsf{L}(\mathbf{b}, \mathbf{v}) = \frac{1}{N} \sum_{i=1}^{N}\Big( \mathsf{g}(s_i; \mathbf{b}, \mathbf{v}) - y_i\Big)^2
\end{align}
%
Therefore, when used as a probability calibration map, isotonic regression minimises the Brier score on the training set.
Instead of applying isotonic regression directly, \cite{naeini2016} also consider building an ensemble calibration map by combining a set of near-isotonic functions.  
Recently, \cite{allikivi2019} propose a Bayesian approach to improve isotonic regression, with demonstrated improvements on binary tasks.

Isotonic regression is a compelling approach for probability calibration, with the following advantages:
(1) When the monotonic assumption is suitable, isotonic regression can find the optimal bin edges for Brier score on the training sets, which is also known to give the convex hull in ROC analysis.
(2) The non-parametric nature avoids catastrophic model misfit.
On the other hand, isotonic regression has some drawbacks also:
(1) By predicting constant values within bins, it inevitably increases grouping loss. 
(2) When the uncalibrated model has a non-monotonic reliability diagram, isotonic regression can only give sub-optimal results (i.e. large grouping loss).
(3) While it performs well on large datasets, isotonic regression's training time and memory consumption are also high on large datasets.
(4) Isotonic regression can result in the first and last bins having full confidence (0 and 1), which can be problematic for certain datasets and evaluation metrics (e.g. log-loss). 
It is therefore common to clip the outputs from isotonic regression with a small $\epsilon$ (i.e., $0$ to $\epsilon$ and $1$ to $1 - \epsilon$).

\subsubsection*{Platt Scaling}

Platt scaling is probably one of the most widely known approaches for probability calibration, partly due to the popularity of SVMs around the year 2000 \newtext{\cite{platt2000}}.
As SVMs are optimised with hinge loss, they can only output scores on the samples based on the estimated margins.
Given that the margins are real scalars by definition, John Platt proposed to transform the scores into probability estimates with logistic regression.
Platt scaling hence has the same parameters as a univariate logistic regression model: 
a shape parameter $w \in \mathbb{R}$, and  
a location parameter $b \in \mathbb{R}$.
The predictive function is then: 
%
\begin{align}
\mathsf{g}(s; w, b) = \frac{1}{1+\exp(-w \cdot s-b)}
\end{align}
%
The parameters can be estimated by optimising the log-likelihood on the training set, so Platt scaling can be seen as optimising log-loss in the calibration context:
%
\begin{align}
\mathsf{L}(w, b) = \frac{1}{N} \sum_{i=1}^{N} \ln \Big(\sum_{j=1}^{2} - \mathsf{I}(y_i=j) \cdot \mathsf{g}(s; w, b)\Big) 
\end{align}
%

\begin{figure}[!tbp]
    \centering
    \begin{subfigure}{\textwidth}
    \centering
    % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case1_PLATT_prediction.png}
    \includegraphics[width=0.28\textwidth]{Case1_PLATT_calibration.png}
    \includegraphics[width=0.28\textwidth]{Case1_PLATT_reliability.png}
    \caption{Test case 1: under-confidence}
    \end{subfigure}
    
    
    \begin{subfigure}{\textwidth}
    \centering
    % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case2_PLATT_prediction.png}
    \includegraphics[width=0.28\textwidth]{Case2_PLATT_calibration.png}
    \includegraphics[width=0.28\textwidth]{Case2_PLATT_reliability.png}
    \caption{Test case 2: over-confidence}
    \end{subfigure}
    
    \begin{subfigure}{\textwidth}
    \centering
    % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case3_PLATT_prediction.png}
    \includegraphics[width=0.28\textwidth]{Case3_PLATT_calibration.png}
    \includegraphics[width=0.28\textwidth]{Case3_PLATT_reliability.png}
    \caption{Test case 3: MLP classifier}
    \end{subfigure}
    
    \caption{Examples of the Platt scaling approach. While it improves the under-confidence case well, it fails to do much with the over-confidence case. This is due to the fact that the sigmoid shape can not push the probabilities towards the middle hence can not fix over-confidence. Such result can also be observed with the MLP test case, where Platt scaling actually makes the level of calibration worse around several regions.}
    \label{fig:test_platt}
\end{figure}


% In addition, as ordinary logistic regression with log-loss can easily overfit to small datasets, 
Platt also included a technique to prevent overfitting and improve the generalisation of calibration, \newtext{which is introduced as one of the training schemes at the beginning of this section.}
The test results are shown in Figure~\ref{fig:test_platt}.

In general, Platt scaling is a practical calibration approach with the following advantages:
(1) As it is based on logistic regression, implementation is straightforward.
(2) The standard logistic regression has a convex loss.
The overall training process can, therefore be quite fast.
On the negative side, Platt scaling has two main drawbacks:
(1) The calibration map is restricted to a sigmoid shape, which effectively pushes probabilities away from the centre and may lead to over-confidence.
(2) By definition, the logistic regression model considers the input space to be a real scalar space. 
While such an assumption is suitable for the margins obtained from an SVM, it is less appropriate for probabilistic classifiers, as the input is bounded by the interval $[0, 1]$. 
Hence, certain transformations are required when applying Platt scaling to calibrate probabilistic classifiers, such as the logit transform.

\subsubsection*{Beta Calibration}

Beta calibration is specifically designed for probabilistic classifiers \newtext{and alleviates both drawbacks of Platt scaling \cite{pmlr-v54-kull17a,kull2017beyond}}.
While the latter can be derived from first principles by assuming that within each class the scores are normally distributed with the same variance, Beta calibration instead assumes two Beta distributions.
This gives a richer family of calibration functions with three parameters: two shape parameters $a, b \in \mathbb{R}$, and a location parameter $c \in \mathbb{R}$. 
The calibration function is then given as:
%
\begin{align}
\mathsf{g}(s; a, b, c) = \frac{1}{1+\exp \big(-a \cdot \ln s + b \cdot \ln(1-s) - c \big)}
\end{align}
%
In comparison with Platt scaling, Beta calibration is a bivariate logistic regression model, where the two features are $\ln s$ and $\ln(1-s)$ respectively.
Similar cross-validation training is also adopted as proposed in \cite{pmlr-v54-kull17a}. 

Given its close relationship to logistic regression, Beta calibration also optimises the log-loss and the objective function can be given with the log-likelihood:
%
\begin{align}
\mathsf{L}(a, b, c) = \frac{1}{N} \sum_{i=1}^{N} \ln \Big(\sum_{j=1}^{2} - \mathsf{I}(y_i=j) \cdot \mathsf{g}(s; a, b, c)\Big)
\end{align}

\begin{figure}[!htbp]
    \centering
    \begin{subfigure}{\textwidth}
    \centering
    % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case1_BETA_prediction.png}
    \includegraphics[width=0.28\textwidth]{Case1_BETA_calibration.png}
    \includegraphics[width=0.28\textwidth]{Case1_BETA_reliability.png}
    \caption{Test case 1: under-confidence}
    \end{subfigure}
    
    
    \begin{subfigure}{\textwidth}
    \centering
    % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case2_BETA_prediction.png}
    \includegraphics[width=0.28\textwidth]{Case2_BETA_calibration.png}
    \includegraphics[width=0.28\textwidth]{Case2_BETA_reliability.png}
    \caption{Test case 2: over-confidence}
    \end{subfigure}
    
    \begin{subfigure}{\textwidth}
    \centering
    % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case3_BETA_prediction.png}
    \includegraphics[width=0.28\textwidth]{Case3_BETA_calibration.png}
    \includegraphics[width=0.28\textwidth]{Case3_BETA_reliability.png}
    \caption{Test case 3: MLP classifier}
    \end{subfigure}
    
    \caption{Examples of Beta calibration. The Beta approach deals with the under-confident case fairly well, as the reliability diagram follows the diagonal closely after calibration. Regarding the over-confident case, Beta calibration manages to put more corrections than the Platt scaling around the $[0, 0.5]$ region, as it pushes the reliability diagram towards the diagonal. However, it doesn't help much in $[0.5, 1.0]$ region. On the MLP case, Beta provides some improvements around the $[0.6, 1.0]$ region, and matches the reliability diagram to the diagonal. Here we can see that the reliability diagrams after calibration are almost identical for the over-confidence and under-confidence test cases. This observation is because the Beta calibration method fits the map on the logarithm of the uncalibrated probabilities, and therefore reverts the sigmoid functions of the pseudo-models in both test cases. The calibration method then finds similar solutions as the pre-sigmoid parts are both linear models on the feature. This result suggests that the Beta calibration method can effectively fix the over/under-confidence caused by a sub-optimal linear-sigmoid operation. }
    \label{fig:test_beta}
    % \todo{Hao: add two sentences why the top two reliability diagrams are the same in Fig. \ref{fig:test_beta}.}
\end{figure}

Figure~\ref{fig:test_beta} demonstrates Beta calibration on the three test cases.
The advantages of Beta calibration include:
(1) Compared with Platt scaling, it allows a richer family of calibration maps including inverse sigmoids and the identity map. 
The latter is particularly useful to prevent over-calibration and apply unnecessary adjustments to already calibrated probabilities.
(2) Like with Platt scaling, implementation is straightforward. 
(3) With the Beta assumption, the calibration map supports any two-class probabilistic classifiers, and the calibration map is  learnt from a set of functions that map from $[0, 1]$ to $[0, 1]$. 
However, Beta calibration's main drawback is that it can only model specific calibration maps, so if the original classifier is severely uncalibrated and requires a complicated calibration map, it might be preferable to choose non-parametric methods instead. %and it can obtain ill-posed results (e.g. non-monotonic calibration map) around the boundaries if no constraint is applied to the parameters.
% \todo{Hao: please reformulate last two sentences as they are cryptic to me (PF) how about now.}

\subsection{Calibration for Multi-class Classification}

We now proceed with calibration maps that can work natively with a multi-class classification task, without the need for binarisation.
%
% % \subsubsection*{Uncalibrated Classifier for a 3-class Problem}
% In this section, we only focus on the test case with the MLP classifier, since both the concepts of over-confident and under-confident are considered in a two-class setting.
%
We define a three-class test case for the purpose of examining multi-class calibration with a multi-layer perceptron (MLP).
% In this case we only consider the MLP classifier, as the concepts of under-confidence and over-confidence can be examined with two-class calibration methods.
We modify the previous synthetic dataset to add an additional class, such that all classes are equi-probable and the distribution of the feature for the instances of class 3 is Gaussian also:
\begin{align*}
    Y &\sim \text{Categorical}([\frac{1}{3}, \frac{1}{3}, \frac{1}{3}]) \\
    H &\sim \text{Categorical}(0.5) \\
    X \mid Y=1, H=1 &\sim \text{Gaussian}(-4, 960) \\
    X \mid Y=1, H=2 & \sim \text{Gaussian}(64, 1280) \\
    X \mid Y=2, H=1 & \sim \text{Gaussian}(4, 980) \\
    X \mid Y=2, H=2 & \sim \text{Gaussian}(-72, 1024) \\
    X \mid Y=3 &\sim \text{Gaussian}(0, 8) \\
\end{align*}

% On the visualisation side, because the calibration map is no longer a $1D$ function, we consider to visualise them in a class-wise simplex.
We visualise the calibration maps in the probability simplex (one for each class). 
An example can be seen in the top row of Figure~\ref{fig:TS}, where the heat maps indicate the change of probability for each class after calibration.
For the figure on the left, each point within the simplex represents an uncalibrated probability vector, a positive value (i.e., red colour) on that point indicates that the calibration map increases the probability value of class 1 in the vector and a negative value (i.e., blue colour) shows that the probability value on class 1 is reduced.
The white line indicates where the probability values for class 1 remain (almost) unchanged.
Class 2 and class 3 calibration maps are also depicted.
% Regarding the reliability diagram, we select the class-wise reliability diagram, and examples can be seen at the bottom of Figure~\ref{fig:TS}.
The bottom row of each figure shows the class-wise reliability diagrams. 

\subsubsection*{Temperature Scaling}

\begin{figure}[!tbp]
    \centering
    %\includegraphics[width=0.85\textwidth]{figures/calibrators/TS_prediction.png}
    \includegraphics[width=0.95\textwidth]{TS_calibration.png}
    \includegraphics[width=0.85\textwidth]{TS_reliability.png}
    \caption{MLP classifier with Temperature scaling (top: class-wise calibration map, bottom: class-wise reliability diagram). While Temperature scaling manages to improve the reliability diagram around the $[0.1, 0.4]$ region for classes 1 and 2, we can see it actually makes things worse elsewhere. As the calibration maps show, Temperature scaling applies the same calibration map to all three classes despite them having different class-wise reliability diagrams, which is the main reason for the sub-optimal results.}
    \label{fig:TS}
\end{figure}

Temperature scaling has become one of the default approaches to provide better-calibrated probabilities, \newtext{particularly in deep learning research \cite{hinton2015distilling,guo2017}}.  
Instead of simply applying the softmax operation at the last layer to obtain a probability vector on the classes, Temperature scaling assumes a single temperature parameter $t \in \mathbb{R}$ and applies a linear operation before the softmax.
Denoting $\mathbf{z} = [z_1, \dots, z_K] \in \mathbb{R}^K$ as the $K$-dimensional real vector before softmax, the probability output after Temperature scaling is given as:
%
\begin{align}
\mathsf{c}_{j}(\mathbf{z}; t) = \frac{\exp\big(-z_j / t\big)}{\sum_{j=1}^{K}\exp\big(-z_j / t\big)}
\end{align}
%
Therefore, conventional softmax can be seen as the case of scaling with a fixed temperature of $t=1$.

If we want to apply Temperature scaling to a generic probabilistic model where $z$ is not accessible, we can also use the $\mathsf{logit}$ transform on the uncalibrated probability vector to obtain a real vector:
%
\begin{align*}
    z_j &= \mathsf{logit}_j (\mathbf{s}) \\
        &= \ln\frac{s_j}{s_K}
\end{align*}
%
Here, $K$ is selected as the reference class to compute the probability ratio with other classes.
The parameter is also normally estimated with the log-loss, and the objective function is given as:
%
\begin{align}
\mathsf{L}(t) = \frac{1}{N} \sum_{i=1}^{N} \ln \Big(\sum_{j=1}^{K} - \mathsf{I}(y_i=j) \cdot \mathsf{g}_{j}(\mathbf{z}_i; t)\Big)   
\end{align}

Figure~\ref{fig:TS} gives the results on the MLP test case.
The most distinctive characteristic of Temperature scaling is that it only has a single parameter, which can be seen as both an advantage and a disadvantage.
On the positive side, a single parameter restricts the space of calibration maps and can prevent overfitting for small datasets with many classes. 
On the negative side, Temperature scaling can be sub-optimal when the function space of the calibration maps does not include the right reliability diagram.  

\subsubsection*{Vector Scaling}

\begin{figure}[!tbp]
    \centering
    % \includegraphics[width=0.85\textwidth]{figures/calibrators/VS_prediction.png}
    \includegraphics[width=0.95\textwidth]{VS_calibration.png}
    \includegraphics[width=0.85\textwidth]{VS_reliability.png}
    \caption{Class-wise calibration maps and reliability diagrams for the MLP classifier with Vector scaling. The most obvious change from Temperature scaling is that now the calibration maps are different for each class. However, the calibration maps still have a circular shape as Vector scaling only adjusts one dimension of the logit vector for each class. As a result, the reliability diagram is close to the ones of Temperature scaling. Some minor improvements can be seen with class 3, where Vector scaling does not make it quite as bad as for Temperature scaling. }
    \label{fig:VS}
\end{figure}

Where Temperature scaling only has a single parameter across all classes, it is natural to extend the parameters to support a richer form of calibration maps.
Vector scaling \newtext{\cite{guo2017}} allows a different temperature for each class, denoted as $\mathbf{w} \in \mathbb{R}^{K}$, as well as adding a set of intercept parameters $\mathbf{b} \in \mathbb{R}^{K}$ for the $K$ classes.
The predictive function is given as ($\mathbf{z}$ can also be obtained with the logit transform for generic probability classifier, as in Temperature scaling):
%
\begin{align}
\mathsf{c}_{j}(\mathbf{z}; \mathbf{w}) = \frac{\exp\big(-w_j \cdot z_j -b_j\big)}{\sum_{j=1}^{K}\exp\big(-w_j \cdot z_j - b_j\big)}
\end{align}
%
And the objective function to optimise log-likelihood is similar to the one for Temperature scaling, but with more parameters:
%
\begin{align}
\mathsf{L}(\mathbf{w}, \mathbf{b})= \frac{1}{N} \sum_{i=1}^{N} \ln \Big(\sum_{j=1}^{K} - \mathsf{I}(y_i=j) \cdot \mathsf{g}_{j}(\mathbf{z}_i; \mathbf{w}, \mathbf{b})\Big)
\end{align}

The test result is given in Figure~\ref{fig:VS}.
Vector scaling can be seen as a middle point between the quite restrictive Temperature scaling and the general approach of Matrix scaling discussed below. 
Hence it balances the risk of overfitting and the richness of available calibration maps. 

\subsubsection*{Matrix Scaling}

Matrix scaling \newtext{\cite{guo2017}} removes all the parameter constraints on Temperature scaling and Vector scaling.
Similar to a fully connected layer, it has a matrix parameter $(\mathbf{w}_1, \cdots, \mathbf{w}_K), \mathbf{w}_j \in \mathbb{R}^K$ together with the intercept parameter $\mathbf{b} \in \mathbb{R}^{K}$.
The predictive function is ($\mathbf{z}$ can also be obtained with the logit transform, as in Temperature scaling):
%
\begin{align}
\mathsf{c}_{j}(\mathbf{z}; \mathbf{w}_1, \dots, \mathbf{w}_{K}, \mathbf{b}) = \frac{\exp\big(-\mathbf{w}_j^T \mathbf{z} - b_j\big)}{\sum_{j=1}^{K}\exp\big(-\mathbf{w}_j^T \mathbf{z} - b_j\big)}
\end{align}
%
and the objective function is:
%
\begin{align}
\mathsf{L}(\mathbf{w}_1, \dots, \mathbf{w}_K, \mathbf{b})= \frac{1}{N} \sum_{i=1}^{N} \ln \Big(\sum_{j=1}^{K} - \mathsf{I}(y_i=j) \cdot \mathsf{g}_{j}(\mathbf{z}_i; \mathbf{w}_1, \dots, \mathbf{w}_K, \mathbf{b})\Big)
\end{align}

As indicated in Figure~\ref{fig:MS}, Matrix scaling can support a broader family of calibration maps than Vector scaling and Temperature scaling, but may be vulnerable to overfitting as it can be seen as another fully connected layer.  

\begin{figure}[!tbp]
    \centering
    % \includegraphics[width=0.85\textwidth]{figures/calibrators/MS_prediction.png}
    \includegraphics[width=0.95\textwidth]{MS_calibration.png}
    \includegraphics[width=0.85\textwidth]{MS_reliability.png}
    \caption{Class-wise calibration maps and reliability diagrams for the MLP classifier with Matrix scaling. As Matrix scaling is capable of providing fully linear adjustments on the logits for each class, we can see the class-wise calibration map no longer has the circular shape. While there are still minor improvements on the reliability diagram of class 1 and class 2, class 3 has gained a significant improvement.}
    \label{fig:MS}
\end{figure}

\subsubsection*{Dirichlet Calibration}

Dirichlet calibration is the multi-class extension of Beta calibration \cite{kull2019}.
Assuming Dirichlet distributions for the predicted probability vectors within each class, Dirichlet calibration is determined by a set of coefficient vectors $(\mathbf{w}_1, \cdots, \mathbf{w}_K), \mathbf{w}_j \in \mathbb{R}^K$, and a set of intercepts $\mathbf{b} \in \mathbb{R}^{K}$. 
The calibrated probability on the $j\text{-th}$ class is obtained as:
%
\begin{align}
\mathsf{g}_{j}(\mathbf{s}; \mathbf{w}_1, \dots, \mathbf{w}_{K}, \mathbf{b}) = \frac{\exp(-b_j - \mathbf{w}_j^T \ln \mathbf{s})}{\sum_{j=1}^{K}\exp(-b_j-\mathbf{w}_j^T \ln \mathbf{s})}
\end{align}
%
This function can be seen as a $K$-dimensional logistic regression on the log-probabilities (i.e., the sufficient statistics of the Dirichlet distribution). 
Therefore, to apply Dirichlet calibration to a deep neural network, one can first obtain a probability vector using the softmax function, then apply Dirichlet calibration as with other probabilistic classifiers.
%
The objective function is:
%
\begin{align}
\mathsf{L}(\mathbf{w}_1, \dots, \mathbf{w}_K, \mathbf{b})= \frac{1}{N} \sum_{i=1}^{N} \ln \Big(\sum_{j=1}^{K} - \mathsf{I}(y_i=j) \cdot \mathsf{g}_{j}(\mathbf{s}_i; \mathbf{w}_1, \dots, \mathbf{w}_K, \mathbf{b})\Big)
\end{align}

The test results are given in Figure~\ref{fig:Dcal}.
Similar to Beta calibration, one of the advantages of Dirichlet calibration is that it also supports the identity map, so it can also prevent over-adjusting calibrated results.
% Following the derivation, the Dirichlet can also be written with an interpretable canonical parameter form.
As the number of parameters is similar to that of Matrix scaling, the Dirichlet calibration can also overfit on small datasets.
The authors propose the ODIR (Off-Diagonal and Intercept Regularisation) approach to address this issue further and report various performance improvements in their experiments.



\begin{figure}[!tbp]
    \centering
    % \includegraphics[width=0.85\textwidth]{figures/calibrators/DIR_prediction.png}
    \includegraphics[width=0.95\textwidth]{DIR_calibration.png}
    \includegraphics[width=0.85\textwidth]{DIR_reliability.png}
    \caption{Class-wise calibration maps and reliability diagrams for the MLP classifier with Dirichlet calibration. The overall results on the class-wise reliability diagrams are close to those obtained with Matrix scaling. 
    % This is understandable considering the similarity on their mathematical forms. 
    The major differences are seen in the calibration maps, where we can clearly observe a local region for the changes on class 3. Importantly, this region for the Dirichlet calibration approach doesn't cover the area where the predicted probability of class 3 is close to 1. This is more reasonable compared with Matrix scaling, as both the Bayes-optimal predictions and the MLP predictions for class 3 are capped around 0.8.}
    \label{fig:Dcal}
\end{figure}

% \begin{figure}[!tbp]
%     \centering
%     \includegraphics[width=0.85\textwidth]{figures/calibrators/all_prediction.png}
%     \includegraphics[width=0.85\textwidth]{figures/calibrators/all_reliability.png}
%     \caption{A comparison of all calibrators on the binary synthetic dataset.}
%    \label{fig:all}
%\end{figure}

%\begin{figure}[!tbp]
%    \centering
%    \includegraphics[width=0.85\textwidth]{figures/calibrators/all3_prediction.png}
%    \includegraphics[width=0.85\textwidth]{figures/calibrators/all3_reliability.png}
%    \caption{A comparison of all calibrators on the ternary synthetic dataset.}
%    \label{fig:all_3}
%\end{figure}

% \subsection{Calibration methods by extension}

% At the end of this section we briefly mention related approaches that can improve the level of probability calibration in a classification setting, as well as specific applications in areas such as computer vision and natural language processing.
% While we have demonstrated generic post-hoc calibrators that can work with any probabilistic classifier without extensive training setup and specific domain knowledge (i.e. DNN architecture), in this section we will address some methods that come with such additional requirements.
% The methods covered in this section can be described with the following categories: (1) methods that can improve calibration during training time, (2) methods that require a composite training scheme, and (3) methods that work on uncertainty quantification tasks related to classifier probability calibration. 

% \subsubsection{Binary probability calibration, class-wise calibration and confidence calibration}
% Being one of most basic and interpretable definition of calibration, 
\newtext{
\subsection{Extended methods for post-hoc classifier calibration}
\label{sec:cal:extension}
%While some standard binary and multi-class post-hoc calibration methods are introduced above, the research area has recently drawn more attention as the industry is adopting ML systems into production.
In this section we discuss more recent work extending the standard calibration methods discussed above. 

\citet{leathart2017} aim to build calibration maps locally instead of a global calibration map and proposes using modified logistic model trees to build an ensemble calibration method. A decision tree is learnt to separate the original feature space into multiple regions, where a local calibrator can then be estimated using the corresponding outputs and labels.
\citet{kumar2019} propose a combined approach of scaling and binning methods to achieve better calibration with smaller calibration sets. Instead of calculating the label frequency in binning methods, the authors show that using the average value of a pre-fit continuous calibration map gives better calibration. The authors also indicate that a debiased estimator can provide better calibration error in sample complexity.
\citet{wang2019calibrating} discuss how to build flexible univariate non-decreasing calibration maps from shape-restricted polynomial regression models. The resulting method provides a useful alternative when methods like Plat scaling and Beta calibration cannot approximate the actual reliability diagram.
\citet{wenger2020} investigate non-parametric post-hoc approaches that can support richer forms of calibration map for a multi-class setting.
The idea is to employ the framework of Gaussian processes and model the calibration map as latent distribution of functions.
The family of calibration maps can thus be richer with the selection of suitable kernels.
\citet{zhang2020mix} propose an approach to build an ensemble of base calibrators, which can improve the capacity of the calibration maps while preserving the accuracy.
The authors also adapt kernel density estimation as an alternative approach to evaluating calibration error. 
\citet{ma2021meta} consider the confidence calibration setting and propose to improve a calibration map with a ranking model. The authors demonstrate that the ranking model can be used to maintain the performance of the uncalibrated classifier in terms of precision and false positive rate.
\citet{patel2021multiclass} tackle the issue of applying class-wise binning calibrators to a multi-class setting. An iterative update method is provided to adjust the bin edges to better calibration, and a sample-sharing approach among similar classes is also introduced for better sample efficiency. 

\subsection{Methods that can improve calibration during training time}
\label{sec:cal:training}

%So far, we have been mainly focusing on post-hoc calibration approaches.
While post-hoc calibration can be applied to most existing classifiers, it is of practical interest to train well-calibrated models in the first place.
Here we briefly mention some training-time calibration methods.

\citet{kumar2018} consider a regularisation approach with kernel mean embedding.
The idea is to add a differentiable regularisation term concerning the goodness of calibration, where the kernel mean of the scores is calculated as an approximation of the calibration error. 
The overall objective function allows the model to achieve better calibration during the training phase.
\citet{thulasidasan2019mixup} show that the Mixup strategy can improve the calibration level when introduced during the training phase.
Vicinal points are created by combining existing data points and labels, and then added to the training set.
The authors suggest that the improvement in calibration is due to the augmentation effect and label smoothing effect, both from the mixup process and act as a form of regularisation.
\citet{kristiadi2020being} consider a Bayesian approach where a Gaussian approximation distribution is fitted to the last layer's weights of a ReLu network.
The authors demonstrated that the method could reduce the over-confidence problem in a classification setting, particularly on data points not commonly seen in the original training set.
\citet{wen2020batchensemble} propose an efficient ensemble approach that can train multiple deep networks with lower computational and memory costs.
The authors show that the obtained ensemble achieves better calibration on out-of-distribution samples at test time.

Other than deep networks, some recent work achieves better calibration on Bayesian nonparametric methods.
\citet{milios2018} propose an alternative approach to train Gaussian Processes for classification tasks.
While the traditional GP classifier relies on sigmoid or probit link functions and requires suitable approximated inference schemes to ensure good performance, the authors propose a modified Dirichlet link function to ensure the level of calibration as well as scalability.
\citet{tran2019calibrating} demonstrate that convolution Gaussian process classifiers can be miscalibrated, and propose a solution to mitigate the issue.

% \subsubsection{Methods that require a composite fitting procedure}

% While we have introduced some general calibration methods in detail, some recent work has introduced methods that can improve calibration in a certain sense (i.e. from a binary, class-wise or confidence perspective), with the cost of a more composite fitting procedure.
% Given the diversity of these fitting procedures, here we provide a brief introduction to some of the methods so the readers can further refer to the papers for implementation details. 


\subsection{Methods for probability calibration for other predictive settings}
\label{sec:cal:other}

% Although we have discussed probability calibration in a classification setting, 
The concept of calibration can be naturally generalised to predictive settings other than classification.
The most straightforward extension is the calibration of regression outputs.
As in the classification scenario, there are multiple definitions of calibration for regression models.
The standard definition of calibration comes from the field of quantile regression \cite{koenker2001quantile}, where being calibrated means that the predicted quantile matches the marginal distribution of the target variable.
As in the case of classification, there are methods designed for training calibrated quantile regression as well as post-hoc approaches that calibrate pre-trained models.
\citet{fasiolo2020fast} provide an approach to train generalised additive regression models with calibrated quantiles.
\citet{cui2020calibrated} propose an approach to train deep regression models with better-calibrated quantiles, where the model parameter is first fit with log-loss and then updated with a loss based on the maximal mean discrepancy \cite{gretton2012kernel}.
For the post-hoc setting, \citet{kuleshov2018} point out that deep regression models' quantiles can be calibrated with binary calibrators such as isotonic regression and yield better performance on downstream tasks such as reinforcement learning.
\citet{chung2021beyond} introduce some modified loss functions to train quantile calibrators with specific emphases, such as balancing between calibration and sharpness. 

Regarding the definition of calibration, \citet{pmlr-v97-song19a} propose a stronger notion of calibration in regression, where the local conditional distribution is required to be calibrated instead of the global quantile. 
The authors 
% refer to this definition as distribution-calibrated for regression models and 
show that being distribution-calibrated in this sense implies being quantile-calibrated.
A post-hoc approach based on the Gaussian process is also introduced, where the GP models a distribution of Beta calibrators conditioning on the original regression outputs.
\citet{kuleshov2022calibrated} consider achieving post-hoc distribution calibration by learning a lower dimensional representation of the (uncalibrated) local distributions, and the post-hoc calibrators can then be built with density estimators on these representations and the target values, which avoids the costs of distributional kernels and sparse variational inference.
\citet{sahoo3reliable} propose the definition of threshold calibration for regression models, which is a stronger notion of calibration than being quantile-calibrated and weaker than the distribution-calibrated definition.
Instead of asking for calibration on a marginal quantile or local distribution level, the proposed definition requires the model to be calibrated on a group of distributions that satisfy a given threshold condition, which ensures optimal decision-making when a threshold is put on the regression outputs.

Calibration of structured outputs, such as sequential outputs, is also of interest for application domains such as natural language processing and time-series modelling. 
\citet{kuleshov2015calibrated} propose approaches to simplify the structured output to a two-class problem and employ a well-calibrated binary classifier to improve the calibration level.
On the information-retrieval side, the traditional precision-recall curve is not sufficiently similar to a ROC curve to allow a similar calibration property.
In contrast, the precision-recall-gain curve proposed by \citet{flach2015} can be seen as a proper generalisation of ROC curve obtained by replacing weighted accuracy with F-score.


Conformal prediction \cite{vovk2005algorithmic,romano2019conformalized,angelopoulos2021gentle} is another area closely related to the topic of probability calibration.
For classification, conformal prediction aims to predict a set of labels that has a probability of $1 - \alpha$ that includes the true label, where $\alpha$ is a user-defined significance level.
Therefore, we can see the conformal prediction for classifiers as an alternative definition of calibration to label probability calibration. That is, instead of requiring the probability to be accurate on the label distributions, conformal prediction wants to ensure the calibration on a variable set of labels that are exactly calibrated on the given significance level.
One of the approaches to construct a conformal classifier is to use a Venn predictor \cite{vovk2003self,vovk2012venn,johansson2018}.
The framework makes use of the Venn taxonomy to define subsets of the original label space, and requires a classifier to make predictions about each element in the subset.
The final conformal prediction can then be calculated using these predictions.

\subsection{Methods designed for other research fields and applications}
\label{sec:cal:app}

The notion of calibration can also be generalised to other areas where uncertainty quantification is of interest. rRecent work has started to explore other topics in statistics, machine learning and artificial intelligence related to calibration.
Here we briefly introduce some of them. 
A comprehensive analysis of these works is left as future work.
\citet{pleiss2017fairness} draw a link between the level of calibration and the evaluation of classifier fairness.
\citet{CobbGal2018Loss} propose an approach to modify the lower bound of approximate Bayesian inference so that the final objective function can be calibrated according to a given decision loss. 
\citet{liu2018generalized} adopt calibrated deep models to improve zero-shot learning.
\citet{menon2018loss} consider the calibration problem for an anomaly detection setup.
\citet{ghandeharioun2019characterizing} consider uncertainty and calibration as a tool to improve explainability for computer vision tasks. 
And \citet{liu2019accurate} adopt a calibration procedure to achieve better posterior distributions for a Bayesian non-parametric ensemble model.
\citet{ding2021local} consider the problem of improving calibration for semantic segmentation.
\citet{guillory2021predicting,jiang2021assessing} show that calibrated classifier can be used to estimate the model performance on OOD test sets. 
}


% \cite{kuleshov2018} focus on the calibration of quantile regression approaches, and propose to use binary post-hoc calibrators to improve various deep regression models.

%\cite{song2019} proposes a stronger definition of calibration for regression tasks, which requires the output to be calibrated on a distribution level instead of a quantile level, a GP-based approach is also given to improve such calibration.

% \cite{widmann2019} gives a statistical test framework for calibration in a multi-class setting.

% {\color{red}
% I will add some citations here that may be useful as well

% \cite{Krishnan2020}
% \begin{itemize}
%     \item Uncertainty under distribution shift between training and test
%     \item Propose a new differentiable accuracy versus uncertainty calibration (AvUC) loss function
%     \item Can be applied as a post-hoc calibration method
%     \item Intended to deal with out-of-distribution in the training data manifold
%     \item Categorise calibration methods into: (1) post-processing calibration (eg. Temperature scaling and dirichlet calibration), (2) training with data augmentation, (3) probabilistic methods with respect to the model parameters.
%     \item Contribution: (1) differentiable proxy for Accuracy versus Uncertainty measure (not sure if this measure is also a contribution), (2) evaluation of results under distribution shift, (3) propose post-hoc calibration with Temperature scaling, (4) comparison with stae-of-the-art methods (need to see this yet).
%     \item Evaluation metrics: conf-ECE, expected uncertainty calibration error (UCE) [41], NLL, Brier score, conditional probabilities $p(accurate|certain)$ and $p(uncertain|inaccurate)$ [39], AUROC, and AUPR (not gain curves).
%     \item Accuracy vs uncertainty (AvU) uses a confusion matrix to compute the "accuracy" of "certainty". Basically, constructing a confusion matrix of correctly predicted vs certain predictions if a threshold is well defined, and then computing the Accuracy on that confusion matrix.
%     \item Accuracy vs uncertainty calibration (AvUC) loss: In order to make the previous metric differentiable, a surrogate function is defined by defining a fixed threshold to determine what is considered certain, and an hyperbolic tangent of the certainty is used to approximate a similar behaviour than AvU in ideal conditions.
%     \item AvUC loss is used as an additional term to the original loss, and intended to be used as a regularization factor.
%     \item In the example with loss-calibrated evidence lower bound (ELBO), the first epochs are trained ONLY with ELBO, later the AvUC term is introduced with an scaling hyperparameter Beta. The required uncertainty "threshold is obtained from the average of predictive uncertainty mean for accurate and inaccurate predictions on the training data from initial epochs".
%     \item Question: The method is trying to calibrate the probabilistic outputs, but uses a fixed threshold to define what is certain, and what is not... This is very simplistic in my view, and it should show signs of poor classwise calibration.
%     \item Experiments compare several sota networks with Temperature scaling, deep-ensembles, Monte Carlo dropout, Mean-field stochastic variational inference, Temperature scaling on SVI, and Radial Bayesian neural network.
%     \item All methods evaluated in 16 types of image corruption at 5 level of intensities (80 variations).
% \end{itemize}
% }

% \subsection{The toy dataset (feature space, generative view)}
% For better illustration, we adopt a dataset and a set of visualisations.
% \begin{figure}
%     \centering
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/toy.png}\hfill
%     \includegraphics[width=0.62\textwidth]{figures/calibrators/toy_conditional.png}
% \end{figure}

% \subsection{The toy dataset (feature space, discriminative view)}

% As we know the data distribution, we can calculate the Bayes-optimal scoring model, that is: 
% \begin{align*}
% s(x) = P(Y=1 | X=x)
% \end{align*}

% \subsection{The distribution of predictions}
% We can further calculate the distribution of $s(x)$.
% \begin{figure}
%     \centering
%     \includegraphics[width=0.33\textwidth]{figures/calibrators/bayes_opt.png}
%     \caption{Distribution of scores }
% \end{figure}

% \begin{figure}
% \centering
% \includegraphics[width=0.62\textwidth]{figures/calibrators/bo_conditional.png}
% \caption{Probability distribution of scores per class}
% \end{figure}


% \subsection{Reliability diagram}
% As well as $P\Big(Y=1 | s(x)\Big)$ (reliability diagram).
% Since the model is Bayes-optimal, we have a perfect reliability diagram.
% \begin{figure}
%     \centering
%     \includegraphics[width=0.33\textwidth]{figures/calibrators/bo_score.png}
%     \includegraphics[width=0.27\textwidth]{figures/calibrators/bo_rg.png}
%     \caption{Joint probability distribution of the scores, and correspoinding reliability diagram.}
% \end{figure}

% \subsection{With a classifier}
% Now if we train a neural network with some samples.
% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/mlp.png}
% \includegraphics[width=0.28\textwidth]{figures/calibrators/mlp_rel.png}
% \caption{Neural network's predicted scores in the input space, and corresponding reliability diagram.}
% \end{figure}

% \subsection{Post-hoc calibrators}
% This is where we need post-hoc calibrators.

% \subsection{Post-hoc calibrators (scaling view)}

% \begin{itemize}
%     \item It is also common to re-scale a real vector output into calibrated probability vector space.  (e.g. SVM margins, final layer of a neural network) 
    
%     \item Since a real vector and a probability vector can be transformed into each other through link function and inverse link function (e.g. soft-max and logit transform), for later slides we will use the probability vector view by default. 

% \end{itemize}



% \begin{figure}
%     \centering
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/mlp_map.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/mlp_map_sca.png}
%     \caption{Example of original and scaled scores.}
% \end{figure}

% \section{Scaling v.s. Probability calibrator}

% \subsection{Scaling v.s. Probability calibrator}{
% \textbf{Scaling}: designed to re-scale a function output into probability vector space and match with target observations. (e.g. SVM margins, final layer of a neural network, latent functions modelled by a Gaussian process)

%   \begin{figure}
%       \centering
%       \includegraphics[width=0.28\textwidth]{figures/calibrators/svm_margin.png}
%       \includegraphics[width=0.1\textwidth]{figures/calibrators/right_arrow.png}
%       \includegraphics[width=0.28\textwidth]{figures/calibrators/svm_after.png}
%   \end{figure}

%}

% \subsection{Scaling v.s. Probability calibrator}{
% \textbf{Probability calibrator}: designed to match a probability output with target observations.

 %   \begin{figure}
   %    \centering
  %     \includegraphics[width=0.65\textwidth]{figures/calibrators/p_x_g_y_model.png} 
    %   \includegraphics[width=0.05\textwidth]{figures/calibrators/down_arrow.png}
   %    \includegraphics[width=0.65\textwidth]{figures/calibrators/p_x_g_y_hat.png}
  % \end{figure}

%}

% \subsection{Scaling v.s. Probability calibrator}{
% \textbf{Probability calibrator}: designed to match a probability output with target observations.

%    \begin{figure}
%        \centering
%        \includegraphics[width=0.65\textwidth]{figures/calibrators/simplex_model.png} 
%        \includegraphics[width=0.05\textwidth]{figures/calibrators/down_arrow.png}
%        \includegraphics[width=0.65\textwidth]{figures/calibrators/simplex_hat.png}
%    \end{figure}

% }

%\section{Categories of Calibrators}

%\subsection{Categories of Calibrators}{
%     Scaling approaches v.s. probability calibrator 
%     Parametric approaches v.s. non-parametric approaches 
%     Generative approaches v.s. discriminative approaches 
%}

%\subsection{Scaling approaches v.s. probability calibrator}{
%    \textbf{Scaling approaches}: designed to re-scale a function output into probability vector space and match with target observations.
    
%    \begin{figure}
%        \centering
%        \includegraphics[width=0.5\textwidth]{figures/calibrators/f_x.png} 
%        \includegraphics[width=0.15\textwidth]{figures/calibrators/down_arrow.png}
%        \includegraphics[width=0.5\textwidth]{figures/calibrators/p_x.png}
%    \end{figure}
%}

%\subsection{Scaling approaches v.s. probability calibrator}{
%    \textbf{Probability calibrator}: designed to match a probability output with target observations.
    
%    \begin{figure}
%        \centering
%        \includegraphics[width=0.5\textwidth]{figures/calibrators/p_x.png} 
%        \includegraphics[width=0.15\textwidth]{figures/calibrators/down_arrow.png}
%        \includegraphics[width=0.5\textwidth]{figures/calibrators/p_hat_x.png}
%    \end{figure}
%}

%\subsection{Scaling approaches v.s. probability calibrator}{
%The differences between scaling approaches and probability calibrators mainly come from their motivations.
%For instance, some scaling approaches are proposed for non-probabilistic models such as SVM.
%In practice, the application of both types are exchangeable. 
%We can re-scale a function value into probability estimation, and apply probability calibrators.
%We can also use inverse link function to turn a probability estimation into a real number, and apply scaling approaches.
%}

% \subsection{Parametric approaches v.s. non-parametric approaches}{}

% \subsection{Generative approaches v.s. discriminative approaches}{}

% \section{Calibrators}

% \subsection{Binary approaches}

% \begin{itemize}
%     \item \cite{naeini2016}
%     \item \cite{platt2000}
%     \item \cite{kull2017}
% \end{itemize}

% \subsubsection{Empirical Binning}

% While being simple and effective, binning approaches can only give discrete outputs.

% you can trust the probabilities, but it doesn't give many.

% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/emp_map_1000_10.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/emp_rel_1000_10.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/emp_1000_10.png}
% \caption{Empirical binning with 10 bins}
% \end{figure}

% A suitable number of bins / binning algorithm is important to get good results. 

% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/emp_map_1000_100.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/emp_rel_1000_100.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/emp_1000_100.png}
% \caption{Empirical binning with 100 bins}
% \end{figure}

% \textbf{Parameters:} 
% \hspace{24pt}Bins: $\{\mathbb{B}_1, \dots, \mathbb{B}_M \}, \mathbb{B}_j \subset [0, 1]$  
% \hspace{24pt}Bin averages:  $\mathbf{a}=(a_1,\dots,a_{M})$, $a_j \in \{0, 1\}$
% \vspace{12pt}
% \textbf{Predictive Function:} 
% \hspace{24pt}$c(p; \mathbb{B}_1, \dots, \mathbb{B}_M, \mathbf{a}) = \sum_{j=1}^{M} \mathbb{I}(p\in \mathbb{B}_j) \cdot a_j$ 
% \vspace{12pt}
% \textbf{Objective Function:} 
% \hspace{24pt} $\mathbb{L}(\mathbf{a}) = \sum_{j=1}^{M} \Big | \frac{\sum_{i=1}^{N} \mathbb{I}(p_i \in B_j) \cdot y_i}{|\mathbb{B}_j|} - a_j \Big|$ 


% \subsubsection{Isotonic Regression}

% With the ROC-convex hull method, isotonic regression can give good calibration performance with automatic binning and interpolation.
% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/iso_map_100.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/iso_rel_100.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/iso_100.png}
% \caption{Isotonic regression with 100 data points}
% \end{figure}

% More data points are beneficial for isotonic regression, but the monotonicity assumption might not be suitable for certain datasets / base models.
% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/iso_map_10000.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/iso_rel_10000.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/iso_10000.png}
% \caption{Isotonic regression with 10,000 data points}
% \end{figure}

% \textbf{Parameters:} 
% \hspace{24pt}Bin edges: $\mathbf{b}=(b_1,\dots,b_M)$, $b_j \in \{0, 1\}, b_j < b_{j+1}$  
% \hspace{24pt}Edge values:  $\mathbf{v}=(v_1,\dots,v_{M})$, $ v_j \in [0, 1], v_j \leq v_{j+1}$
% \vspace{12pt}
% \textbf{Predictive Function:} 
% \hspace{24pt}$c(p; \mathbf{b}, \mathbf{v}) = \frac{1}{\sum_{j=1}^{M-1} \mathbb{I}(p\geq b_j)\cdot\mathbb{I}(p\leq b_{j+1})}\sum_{j=1}^{M-1} \mathbb{I}(p\geq b_j)\cdot\mathbb{I}(p<b_{j+1}) \cdot \Big(v_j + \frac{p-b_j}{b_{j+1}-b_j}(v_{j+1} - v_j)\Big) $ 
% \vspace{12pt}
% \textbf{Objective Function:} 
% \hspace{24pt} $\mathbb{L}(\mathbf{b}, \mathbf{v}) = \frac{1}{N} \sum_{i=1}^{N}\Big( c(p_i; \mathbf{b}, \mathbf{v}) - y_i\Big)^2$ 

% \subsubsection{Platt Scaling}

% The ONE that allows SVMs to output probabilities.

% \begin{figure}
%        \centering
%        \includegraphics[width=0.4\textwidth]{figures/calibrators/svm_margin.png}\hfill
%        \includegraphics[width=0.1\textwidth]{figures/calibrators/right_arrow.png}\hfill
%        \includegraphics[width=0.4\textwidth]{figures/calibrators/svm_after.png}
%    \end{figure}

% We can also use it to calibrate from the final layer of the MLP classifier.
% \begin{figure}
%        \centering
%        \includegraphics[width=0.28\textwidth]{figures/calibrators/platt_map.png}\hfill
%        \includegraphics[width=0.28\textwidth]{figures/calibrators/platt_rel.png}\hfill
%        \includegraphics[width=0.28\textwidth]{figures/calibrators/platt.png}
% \end{figure}

% \textbf{Parameters:} 
% \hspace{24pt}Slope: $w \in \mathbb{R}$  
% \hspace{24pt}Intercept: $b \in \mathbb{R}$ 
% \vspace{12pt}
% \textbf{Predictive Function:} 
% \hspace{24pt}$c(p; w, b) = \frac{1}{1+\exp(-w \cdot p-b)}$ 
% \vspace{12pt}
% \textbf{Objective Function:} 
% \hspace{24pt} $\mathbb{L}(w, b) = \frac{1}{N} \sum_{i=1}^{N} \ln \Big(\sum_{j=1}^{2} - \mathbb{I}(y_i=j) \cdot c(p; w, b)\Big) $ 

% \subsubsection{Beta Calibration}

% While Platt scaling can be derived with conditional Gaussian distribution with shared variance, probabilities are on a finite support hence Gaussian is less suitable.

% With a Beta assumption, we can get calibration maps that get beyond sigmoid.
% \begin{figure}
% \centering
% \includegraphics[width=0.45\textwidth]{figures/calibrators/beta_list.png}
%\end{figure}

% As well as a identity map if the original model is already calibrated, or no better calibration map can be modelled.
% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/beta_3_map.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/beta_3_rel.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/beta_3.png}
% \end{figure}

% \textbf{Parameters:} 
% \hspace{24pt}Slope 1: $a \in \mathbb{R}$ 
% \hspace{24pt}Slope 2: $b \in \mathbb{R}$ 
% \hspace{24pt}Intercept: $c \in \mathbb{R}$ 
% \vspace{12pt}
% \textbf{Predictive Function:} 
% \hspace{24pt}$c(p; a, b, c) = \frac{1}{1+\exp\big(-a \cdot \ln p - b \cdot \ln (1-p) - c \big)}$ 
% \vspace{12pt}
% \textbf{Objective Function:} 
% \hspace{24pt} $\mathbb{L}(a, b, c) = \frac{1}{N} \sum_{i=1}^{N} \ln \Big(\sum_{j=1}^{2} - % \mathbb{I}(y_i=j) \cdot c(p; a, b, c)\Big) $ 

% \subsection{Multi-class approaches}


% \begin{table}[htpb!]
%     \centering
%     \begin{tabularx}{\linewidth}{L|l|l}
%         \toprule
%         \textbf{Calibration method} & \textbf{Details} & \textbf{} \\
%         \midrule
%         Platt's scaling \cite{platt1999}       &  Multiclass & Scaling \\
%         \midrule
%         Isotonic regression \cite{chakravarti1989}   &  & Non-parametric\\
%         \midrule
%         Nearly-Isotonic regression \cite{chakravarti1989}   &  & Non-parametric\\
%         \midrule
%         Size binning     & & \\
%         \midrule
%         Width binning     & & \\
%         \midrule
%         Binning averaging \cite{zadrozny2001}     & & \\
%         \midrule
%         Similarity binning averaging \cite{bella2009} & & \\
%         \midrule
%         Bayesian binning into quantiles \cite{naeini2015} & & \\
%         \midrule
%         Probability Calibration Trees \cite{leathart2017} & & \\
%         \midrule
%         Calibration of nested dichotomies \cite{leathart2018} & & \\
%         \midrule
%         Temporal probability calibration \cite{leathart2020} & & \\
%         \midrule
%         Venn predictors for probability estimation trees \cite{johansson2018} & &  \\
%         \midrule
%         Ensemble of Near Isotonic Regression \cite{Naeini2017} & Binary & \\
%         \midrule
%         Temperature scaling \cite{guo2017}  & Multiclass & \\
%         \midrule
%         Vector scaling \cite{guo2017}       & Multiclass & \\
%         \midrule
%         Matrix scaling \cite{guo2017}       & Multiclass &  \\
%         \midrule
%         Dirichlet calibration \cite{kull2019} & Multiclass & \\
%         \midrule
%         Accuracy versus uncertainty calibration (AvUC) loss \cite{Krishnan2020}   & Multiclass confidence & %  \\
%         \midrule
%         \cite{milios2018}   & &  \\
%         \midrule
%         \cite{allikivi2019} & &  \\
%         \midrule
%         \cite{Kumar2018}    & &  \\
%         \midrule
%         \cite{Wenger2020}   & &  \\
%         \midrule
%         \cite{Kuleshov2018} & &  \\
%         \midrule
%         \cite{song2019}     & &  \\
%         \midrule
%         \cite{widmann2019}  & &  \\
%          \bottomrule
%     \end{tabularx}
%     \caption{Caption}
% \end{table}

% \subsubsection{Start with adding one more class}

% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/ternary_1.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/ternary_2.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/ternary_3.png}
% \end{figure}


% \subsubsection{Temperature Scaling}

% \textbf{Parameters:} 
% \hspace{24pt}Temperature: $t \in \mathbb{R}$  
% \vspace{12pt}
% \textbf{Predictive Function:} 
% \hspace{24pt}$c_{j}(\mathbf{p}; t) = \frac{\exp\big(-t \cdot \text{logit}_j (p)\big)}{\sum_{j=1}^{K}\exp\big(-t \cdot \text{logit}_j (p)\big)}$ 
% \vspace{12pt}
% \textbf{Objective Function:} 
% \hspace{24pt} $\mathbb{L}(t) = \frac{1}{N} \sum_{i=1}^{N} \ln \Big(\sum_{j=1}^{K} - \mathbb{I}(y_i=j) \cdot c_{j}(\mathbf{p}_i; t)\Big)$


% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/ts_c1.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/ts_c2.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/ts_c3.png}
% \end{figure}
% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/ts_map_c1.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/ts_map_c2.png}\hfill
% \includegraphics[width=0.33\textwidth]{figures/calibrators/ts_map_c3.png}
% \end{figure}

% \subsubsection{Vector Scaling}

% \textbf{Parameters:} 
% \hspace{24pt}Vector: $\mathbf{w} \in \mathbb{R}^{K}$  
% \hspace{24pt}Intercept: $\mathbf{b} \in \mathbb{R}^{K}$ 
% \vspace{12pt}
% \textbf{Predictive Function:} 
% \hspace{24pt}$c_{j}(\mathbf{p}; \mathbf{w}) = \frac{\exp\big(-w_j \cdot \text{logit}_j (p) -b_j\big)}{\sum_{j=1}^{K}\exp\big(-w_j \cdot \text{logit}_j (p) - b_j\big)}$ 
%\vspace{12pt}
% \textbf{Objective Function:} 
% \hspace{24pt} $\mathbb{L}(\mathbf{w}, \mathbf{b})= \frac{1}{N} \sum_{i=1}^{N} \ln \Big(\sum_{j=1}^{K} - \mathbb{I}(y_i=j) \cdot c_{j}(\mathbf{p}_i; \mathbf{w}, \mathbf{b})\Big)$


% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/vs_c1.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/vs_c2.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/vs_c3.png}
% \end{figure}
% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/vs_map_c1.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/vs_map_c2.png}\hfill
% \includegraphics[width=0.33\textwidth]{figures/calibrators/vs_map_c3.png}
% \end{figure}


% \subsubsection{Matrix Scaling}

% \textbf{Parameters:} 
% \hspace{24pt}Matrix: $(\mathbf{w}_1, \cdots, \mathbf{w}_K), \mathbf{w}_j \in \mathbb{R}^K$   
% \hspace{24pt}Intercept: $\mathbf{b} \in \mathbb{R}^{K}$
% \vspace{12pt}
% \textbf{Predictive Function:} 
% \hspace{24pt}$c_{j}(\mathbf{p}; \mathbf{w}_1, \dots, \mathbf{w}_{K}, \mathbf{b}) = \frac{\exp\big(-\mathbf{w}_j^T \text{logit}( \mathbf{p}) - b_j\big)}{\sum_{j=1}^{K}\exp\big(-\mathbf{w}_j^T \text{logit}( \mathbf{p}) - b_j\big)}$ 
% \vspace{12pt}
% \textbf{Objective Function:} 
% \hspace{24pt} $\mathbb{L}(\mathbf{w}_1, \dots, \mathbf{w}_K, \mathbf{b})= \frac{1}{N} \sum_{i=1}^{N} \ln \Big(\sum_{j=1}^{K} - \mathbb{I}(y_i=j) \cdot c_{j}(\mathbf{p}_i; \mathbf{w}_1, \dots, \mathbf{w}_K, \mathbf{b})\Big)$

% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/ms_c1.png}\hfill
% \includegraphics[width=0.28\t\extwidth]{figures/calibrators/ms_c2.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/ms_c3.png}
% \end{figure}

% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/ms_map_c1.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/ms_map_c2.png}\hfill
% \includegraphics[width=0.33\textwidth]{figures/calibrators/ms_map_c3.png}
% \end{figure}

% \subsubsection{Dirichlet Calibration}

% \textbf{Parameters:} 
% \hspace{24pt}Coefficients: $(\mathbf{w}_1, \cdots, \mathbf{w}_K), \mathbf{w}_j \in \mathbb{R}^K$  
% \hspace{24pt}Intercept: $\mathbf{b} \in \mathbb{R}^{K}$ 
% \vspace{12pt}
% \textbf{Predictive Function:} 
% \hspace{24pt}$c_{j}(\mathbf{p}; \mathbf{w}_1, \dots, \mathbf{w}_{K}, \mathbf{b}) = \frac{\exp(-b_j - \mathbf{w}_j^T \ln \mathbf{p})}{\sum_{j=1}^{K}\exp(-b_j-\mathbf{w}_j^T \ln \mathbf{p})}$
% \vspace{12pt}
% \textbf{Objective Function:} 
% \hspace{24pt} $\mathbb{L}(\mathbf{w}_1, \dots, \mathbf{w}_K, \mathbf{b})= \frac{1}{N} \sum_{i=1}^{N} \ln \Big(\sum_{j=1}^{K} - \mathbb{I}(y_i=j) \cdot c_{j}(\mathbf{p}_i; \mathbf{w}_1, \dots, \mathbf{w}_K, \mathbf{b})\Big)$

% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/dir_c1.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/dir_c2.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/dir_c3.png}
% \end{figure}
% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/dir_map_c1.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/dir_map_c2.png}\hfill
% \includegraphics[width=0.33\textwidth]{figures/calibrators/dir_map_c3.png}
% \end{figure}

% \subsection{Notable Mentions}

% \begin{itemize}
% \item \cite{naeini2015}
% \item \cite{milios2018}
% \item \cite{allikivi2019}
% \item \cite{Kumar2018}
% \item \cite{Wenger2020}
% \item \cite{Kuleshov2018}
% \item \cite{song2019}
% \item \cite{widmann2019}
% \end{itemize}

% \subsection{Regularisation and Bayesian Treatments}

% \begin{itemize}
%     \item Typical approaches are generally easy to adopt: $L_{0}$, $L_{1}$, $L_2$, lasso, ridge, as well as common Bayesian inference with certain priors on the parameters. 
    
%     \item In Dirichlet calibration, the authors proposed an off-diagonal L2 regularisation approach for Dirichlet calibration, which improves the generalisation of calibration for deep nets by limiting the pair-wise interaction among different classes.
% \end{itemize}


% \subsection{Implementation}

% There are also some common practices when implementing a calibration approach:
% \begin{itemize}
% \item Have multiple inner folds to train the base model and calibrators separately
% \item Approaches including Beta, Dirichlet, and matrix scaling can be easily trained with existing logistic regression implementations.  
% \item For calibrators with a convex loss, when the number of data points and classes is manageable, explicit Newton approaches is generally better than stochastic optimisation.
% \end{itemize}

% \subsection{Wrap Up}

% \subsubsection{Lessons learned}

% To select a suitable calibrator, consider the following:
% \begin{itemize}
% \item Do you care about the entire probability vector or just about a single class? (the latter $\rightarrow$ binary approaches)
% \item Do you have a large calibration set? (yes $\rightarrow$ non-parametric approaches)
% \item Do you have a small calibration set? (yes $\rightarrow$ consider regularisation)
% \item Are you only interested in certain probability values? (yes $\rightarrow$ binning approaches)
% \end{itemize}


==> mlj_files/05_advanced_topics.tex <==
% \section{Advanced topics}
% \label{sec:out:conc}

% Now that we are nearing the end of this survey we will briefly discuss some more advanced topics related to post-hoc calibration.
% Section~\ref{sec:hyp} gives an introduction to statistical tests for calibration.
% Section~\ref{sec:costs} provides an alternative, cost-based view of the problem of classifier calibration, and discusses the need of calibration from the point of decision theory.
% In Section~\ref{sec:regcal} we consider what it means to calibrate in regression.
% Finally, section~\ref{sec:conclusion} concludes the paper.

\section{Hypothesis tests for calibration}
\label{sec:hyp}
%----------------------------------------------------%

Even if a classifier is perfectly calibrated, it almost always slightly deviates from calibration on any finite dataset due to sampling effects.
Here we consider a method of testing whether the dataset provides sufficient evidence that the classifier is uncalibrated. 

\newtext{A common way to test for calibration is to apply goodness-of-fit tests that were originally proposed for logistic regression models, but can be extended to any model that predicts probabilities. For example, one could apply the Pearson chi-squared goodness-of-fit test, which works by grouping instances sharing the same value of the independent variable $X$ and then applying a chi-squared test under the null hypothesis that the observed number of positives in the target variable is equal to the predicted number of positives for each unique value of $X$.}

\newtext{The issue with this approach is that the higher the number of unique values of $X$ or the higher the number of combinations of values of multiple independent variables, the lower the probability that each group of instances will be well-represented enough for the calculation of the Pearson chi-squared statistic to be reliable. A possible solution to this problem is to group instances into $M$ bins based on percentiles of the predicted probabilities for the positive class (equal-frequency binning) and then apply the Hosmer-Lemeshow (HL) test, which involves calculating the statistic $H$ given by Equation (\ref{eq:hosmer-lemeshow}) \cite{Hosmer2003applied}.} 

\newtext{
\begin{equation}
\label{eq:hosmer-lemeshow}
H = \sum_{m=1}^{M} \left(\frac{\left(O_{m+} - E_{m+}\right)^2}{E_{m+}}+\frac{\left(O_{m-} - E_{m-}\right)^2}{E_{m-}} \right),
\end{equation}
}
\newtext{
\noindent where $O_{m+}$ and $O_{m-}$ are the observed counts of positives and negatives in bin $\mathbb{B}_{m}$ and $E_{m+}$ and $E_{m-}$ are the expected counts of positives and negatives in bin $\mathbb{B}_{m}$, calculated as the sums of positive and negative probabilities in the bin, respectively.
}

\newtext{The HL test was later extended to evaluate the goodness-of-fit of multinomial logistic regression models, by binning instances based on the percentiles of $\sum_{j=2}^K s_{ij} = 1 - s_{i1}$, i.e. the complement of the probabilities assigned to the reference class \cite{fagerland2008multinomial}. Then, similarly to the binary case, once the instances are binned, we calculate $O_{mj}$ and $E_{mj}$, respectively the observed and expected counts for each class $j$ and bin $m$. Finally we calculate the $C$ statistic, given by Equation (\ref{eq:hosmer-lemeshow:C}), which is expected to follow a chi-squared distribution with $(M-2)(K-1)$ degrees of freedom.}

\newtext{
\begin{equation}
\label{eq:hosmer-lemeshow:C}
C = \sum_{m=1}^{M}\sum_{j=1}^{K} \left(\frac{\left(O_{mj} - E_{mj}\right)^2}{E_{mj}}+\frac{\left(O_{mj} - E_{mj}\right)^2}{E_{mj}} \right).
\end{equation}
}

\newtext{Table \ref{tab:hosmer:lemeshow} shows $M=5$ bins based on the toy example of Table \ref{tab:evaluation:toy}. By applying Equation (\ref{eq:hosmer-lemeshow:C}) to these values, we get $C = 25.3$. Finally, to complete the HL test under the null hypothesis that the observed and expected proportions are the same, we compare $C$ to a chi-squared distribution with $(M-2)(K-1) = 6$ degrees of freedom, obtaining a p-value of $0.0003$, rejecting the null hypothesis with $\alpha=0.05$.}

\begin{table}[ht]
    \centering
    \small

    \begin{tabular}{llrrrrrr}
    \toprule
    $\mathbb{B}_{m}$ &    $\mathsf{s}(\mathbb{B}_{m})$ &  $O_{m1}$ &       $E_{m1}$ &  $O_{m2}$ &       $E_{m2}$ &  $O_{m3}$ &     $E_{m3}$ \\
    \midrule
    $\mathbb{B}_{1}$ &  $[0.0, 0.2]$ &  $3.0$ &  $5.9$ &  $1.0$ &  $0.7$ &  $3.0$ &  $0.4$ \\
    $\mathbb{B}_{2}$ &  $(0.2, 0.56]$&  $2.0$ &  $3.1$ &  $2.0$ &  $0.6$ &  $1.0$ &  $1.3$ \\
    $\mathbb{B}_{3}$ &  $(0.56, 0.7]$&  $3.0$ &  $2.47$ &  $3.0$ &  $1.77$ &  $1.0$ &  $2.77$ \\
    $\mathbb{B}_{4}$ &  $(0.7, 0.9]$ &  $2.0$ &  $1.1$ &  $3.0$ &  $3.1$ &  $2.0$ &  $2.8$ \\
    $\mathbb{B}_{5}$ &  $(0.9, 1.0]$ &  $0.0$ &  $0.0$ &  $1.0$ &  $1.2$ &  $3.0$ &  $2.8$ \\
    \bottomrule
    \end{tabular}
    \caption{\newtext{Instances grouped into 5 bins using equal-frequency binning on the complement of the probabilities predicted for class 1. Column $\mathsf{s}(\mathbb{B}_{m})$ shows the probability intervals corresponding to each bin. The probabilities were obtained by considering the multiclass toy problem in Table \ref{tab:evaluation:toy}.}}
        \label{tab:hosmer:lemeshow}
\end{table}

\newtext{This example is of course simply illustrative, as the HL test is not recommended for such small samples, as experiments have shown that it has satisfactory power for samples of over 400 instances \cite{fagerland2008multinomial}. There are several other goodness-of-fit tests, most of them using some sort of binning to calculate a statistic that is assumed to follow a chi-squared distribution. Additionally, as the multiclass HL test, they usually test for classwise calibration. Testing for multiclass calibration is a more complex task and has recently been investigated by \citet{widmann2019calibration}, by using kernel-based measures. These measures were later adapted for regression calibration \cite{widmann2022calibration}. For  details on how these measures can be interpreted as test statistics, we refer the reader to their original papers.}

\newtext{Another approach, proposed by \citet{vaicenavicius2019evaluating}, is to test the classifier's probabilities according to an arbitrary measure of calibration.}
Given a classifier $\mathsf{f}$, we can check if its predictions for a test set $\{(\boldsymbol{x}_1, y_1), \dots, (\boldsymbol{x}_N, y_N)\}$ are calibrated according to a chosen calibration measure $\phi(\mathsf{f}(\mathbf{X}_{\text{test}}),\mathbf{\dot{Y}}_{\text{test}})$, such as ECE, log-loss or Brier score. We discuss a simple resampling-based hypothesis test under the null hypothesis that the classifier's outputs are calibrated \cite{vaicenavicius2019evaluating}. Algorithm \ref{alg:test:steps} details the steps of the hypothesis test procedure.

\begin{algorithm}[H]
		\caption{Hypothesis test for calibration}
		\label{alg:test:steps}
		\begin{algorithmic}[1]
			\Require Test predictions $\mathsf{f}(\mathbf{X}_{\text{test}})$; test set labels $\mathbf{\dot{Y}}_{\text{test}}$, Calibration measure $\phi$; Number of resampled label sets $L$; Significance level $\alpha$;
			
			\For { l=1:L}
			\State Sample $\boldsymbol{y}_l$, $l \in \{1, \ldots, L\}$, such that each $y_{l,i} \sim \mathsf{Cat}(\mathsf{f}(\mathbf{\hat{x}}_i))$;
			\State $\phi_s \leftarrow \phi\left(\mathsf{f}(\mathbf{X}_{\text{test}}),\mathbf{\dot{Y}}_l\right)$;
			\EndFor
		
			\State $\text{p-value} \leftarrow \text{proportion of $\phi_l$ among $\phi_1,\dots,\phi_L$ with}\ \phi_l > \phi\left(\mathsf{f}(\mathbf{X}_{\text{test}}),\mathbf{\dot{Y}}_{\text{test}}\right)$;
			
			\If {$\text{p-value} < \alpha$}
			\State Reject the null hypothesis and conclude that the classifier is not calibrated;
			\Else
			\State Accept the null hypothesis, i.e. there is not enough evidence that the classifier is not calibrated.
			\EndIf
		\end{algorithmic}
\end{algorithm}

Let us return to our toy example (Table \ref{tab:evaluation:toy}). If we follow Algorithm \ref{alg:test:steps} and choose $\mathsf{ECE}_{\text{classwise}}$ as the calibration measure and $L=1,000$, we obtain a distribution such as the one in Figure \ref{fig:eval:loss-distribution}. 

% First, we generate $S$ bootstrapped label sets $\boldsymbol{y}_s$, $s \in \{1, \ldots, S\}$, such that each $y_{s,i}$ is sampled from $\boldsymbol{\hat{p}}(\boldsymbol{\hat{x}}_i)$. Then we calculate $\phi(\boldsymbol{\hat{p}}(X_{\text{test}}), \boldsymbol{y}_s)$ for each label set $\boldsymbol{y}_s$, which gives us a distribution such as the one in Figure \ref{fig:eval:loss-distribution:a}.

% \begin{figure}
%         \centering
%         \includegraphics[width=0.7\textwidth]{figures/evaluation/loss-distribution.png}
%         \caption{Distribution of $\text{classwise-ECE}$ values calculated for every bootstrapped label set $\boldsymbol{y}_s$ with $s \in \{1, \ldots, S\}$, following the procedure described in Algorithm \ref{alg:test:steps}.}
%         \label{fig:eval:loss-distribution}
%     \end{figure}

\begin{figure}[!t]
    \centering
%    \begin{subfigure}{0.45\linewidth}
%    \includegraphics[width=\linewidth]{figures/evaluation/loss-distribution.png}
%    \caption{Distribution of loss values.}
%    \label{fig:eval:loss-distribution:a}
%    \end{subfigure}
%    \begin{subfigure}{0.45\linewidth}
%    \includegraphics[width=\linewidth]{figures/evaluation/loss-distribution-p-value.png}
%    \caption{Red bars represent $\phi_l >  0.1787$.}
%    \label{fig:eval:loss-distribution:b}
%    \end{subfigure}    
    \includegraphics[width=0.6\linewidth]{loss-distribution-p-value.png}
    \caption{Distribution of $\mathsf{ECE}_{\text{classwise}}$ values $\phi_1,\dots,\phi_L$ calculated for every resampled label set $\mathbf{\dot{Y}}_l$ with $l \in \{1, \ldots, L\}$, following the procedure described in Algorithm \ref{alg:test:steps}. The red bars represent the region where $\phi_l >  0.1787$.}\label{fig:eval:loss-distribution}
\end{figure}


Recall that in our example $\mathsf{ECE}_{\text{classwise}} = 0.1787$. The p-value for this test is then $\mathsf{P}\Big(\phi_l >  0.1787\Big) \approx 0.016$, which means we can reject the null hypothesis that the classifier is calibrated according to $\mathsf{ECE}_{\text{classwise}}$. Note that we keep the scores fixed and only resample the labels to perform this test. This means that instances will stay in the same bins and small bins will have low weights for all $L$ resampled $\mathsf{ECE}_{\text{classwise}}$ values.




% Now let the value of the arbitrary loss measure for the test set be $\phi(\boldsymbol{\hat{p}}(X_{\text{test}}), \boldsymbol{y}_{\text{test}}) = 0.32$. We calculate the p-value for the test as $P\Big(\phi(\boldsymbol{\hat{p}}(X_{\text{test}}), \boldsymbol{y}_s) > 0.32\Big) \approx 0.26$, which is equivalent to the red area in Figure \ref{fig:eval:loss-distribution:b}. Thus, we cannot reject the null hypothesis in this example, and this classifier would be considered calibrated.


% \subsection{A cost-based view of classifier calibration}
% \label{sec:costs}
%So far we have framed calibration as aiming to get as close as possible to the Bayes-optimal classifier, predicting the `true' $\mathsf{P}(y|x)$.
%That is, we want the probabilities estimated by a predictive model to match the observed frequencies as closely as possible. 
% One of the scenarios where calibrated probabilities are particularly required is cost-sensitive decision making, where the aim is to minimise the expected cost of misclassifications, given the cost matrix specifying the cost of predicting class $i$ for an instance of class $j$ for any classes $i$ and $j$.
% In Section~\ref{sec:2:1} \todo[inline]{Fix reference to sec:2:1. A closer look at calibration, and why it matters}, we saw that in binary classification the optimal threshold for the Bayes-optimal model $\mathsf{P}(+|\mathbf{x})$ is equal to $c=\frac{\mathsf{C}(+|-)}{\mathsf{C}(+|-)+\mathsf{C}(-|+)}$, where $\mathsf{C}(+|-)$ and $\mathsf{C}(-|+)$ are the costs of a false positive and a false negative, respectively.
% We will refer to $c \in [0, 1]$ as the cost proportion.
%It is also possible to justify the need of calibration from a decision-theoretic point of view.
% Let us now investigate what the optimal threshold is for non-optimal classifiers. 
%In the context of binary classification, we need to decide which class to predict for any score $s$, and our aim is to minimise some given objective on the dataset.
% Among all the possible values of predicted positive class probability $s$, the optimal threshold $s_{\text{dec}}$ is such that the expected misclassification cost is the same regardless of which class is predicted:
%
%When the evaluation metric is accuracy, an intuitive location for the decision boundary is where both classes are equally likely on the particular score.
%This condition explicitly suggests the calibrated probability of $0.5$.
%
%Now we move to a more comprehensive setting.
%Let $c_{FP}$ denote the instance-wise cost for making a false positive prediction, and $c_{FN}$ the instance-wise cost for a false negative prediction.
%Denoting the Recall that the decision boundary $s_{\text{dec}}$ is where it makes no difference to predict either class, which suggests:
%
% \begin{align}
% \label{eq:samecost}
%     P(Y=+ \mid s_{\text{dec}}) \mathsf{C}(-|+) = P(Y=- \mid s_{\text{dec}})  \mathsf{C}(+|-)
% \end{align}
% but additionally, we also need to require that scores higher than $s_{\text{dec}}$ would be more likely positives and scores lower than $s_{\text{dec}}$ would be less likely positives (known as the requirement of being classification-calibrated at $s_{\text{dec}}$ \citep{nguyen2009surrogate}):
% \begin{align*}
%     \label{eq:dec}
%     P(Y=+ \mid s') &> P(Y=+ \mid s_{\text{dec}}) \quad \forall s' > s_{\text{dec}} \\
%     P(Y=+ \mid s') &< P(Y=+ \mid s_{\text{dec}}) \quad \forall s' < s_{\text{dec}} \nonumber
% \end{align*}
% The requirement (\ref{eq:samecost}) that the expected misclassification cost is the same regardless of which class is predicted can be rewritten as
% \begin{align*}
%     P(Y=+ \mid s_{\text{dec}}) \mathsf{C}(-|+) = \Big(1 - P(Y=+ \mid s_{\text{dec}}) \Big) \mathsf{C}(+|-)
% \end{align*}
% leading to
% \begin{align*}
%     \quad P(Y=+ \mid s_{\text{dec}}) = \frac{\mathsf{C}(+|-)}{\mathsf{C}(+|-) + \mathsf{C}(-|+)}=c
% \end{align*}
%
%Since both costs can be assumed to be positive, we can normalise it as the relative misclassification cost:
%
%\begin{align*}
%    c = \frac{c_{FP}}{c_{FP} + c_{FN}}
%\end{align*}
%
% The corresponding decision threshold $s_{\text{dec}}$ for a given $c$ is then such that:
%
% \begin{align*}
%    P(Y=+ \mid s_{\text{dec}}) = c
% \end{align*}
% If the scoring classifier is perfectly calibrated, then $P(Y=+ \mid s_{\text{dec}})=s_{\text{dec}}$. From this we can conclude that for calibrated classifiers the optimal 
% decision threshold is $s_{\text{dec}}=c$, which is the same optimal threshold as for the Bayes-optimal classifier.

%Next, we will continue on binary classification and cover the definitions of classification-calibrated and ranking-calibrated, which are both weaker concepts than class probability calibration.
%While the decision boundary only suggests that it makes no difference to predict either class given the particular score, it can help us to determine the predictions for other scores when the following conditions are met (referred to as being classification-calibrated on $s_{\text{dec}}$ by \citet{nguyen2009surrogate}):
%
%\begin{align}
%    \label{eq:dec}
%    P(Y=+ \mid s') &> P(Y=+ \mid s_{\text{dec}}) \quad \forall s' > s_{\text{dec}} \\
%    P(Y=+ \mid s') &< P(Y=+ \mid s_{\text{dec}}) \quad \forall s' < s_{\text{dec}} \nonumber
%\end{align}
%
%That is, given any other score $s'$, the probability of $P(Y=+ \mid s')$ will be larger than $P(Y=+ \mid s_{\text{dec}})$ is $s' > s_{\text{dec}}$, and vice versa.
%In this case, we can simply predict positives for every score that is larger than $s'$, and predict negative otherwise. 
%Therefore, if we have a cost proportion $c$, and the two conditions in Equation~(\ref{eq:dec}) are met, then the optimal threshold $s_{dec}$ is the score that has a calibrated probability of $c$.


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.35\textwidth]{figures/conclusion/rel.png}\hfill
%     \includegraphics[width=0.5\textwidth]{figures/conclusion/brier_curve.png}
%     \caption{({Left}) The reliability diagrams of the same logistic classifier that are respectively uncalibrated and perfectly post-calibrated. ({Right}): The corresponding Brier curves. The area under the blue curve is the refinement loss of both classifiers, and the area between the red and blue curves is the calibration loss of the uncalibrated model.}
%     \label{fig:brier_curve}
% \end{figure}


% At first sight, calculating misclassification cost based on costs of false positives and false negatives is quite a different way of evaluating a classifier than proper scoring rules.
% Interestingly though, connections can be made between them.
% Suppose we consider different cost scenarios with different values of the cost proportion $c$, but only such that the cost of a false positive and a false negative add up to $2$, that is $\mathsf{C}(+|-)+\mathsf{C}(-|+)=2$.
% Here requiring the sum to be equal to $2$ ensures that the error rate is among the considered scenarios, as then $\mathsf{C}(+|-)=\mathsf{C}(-|+)=1$.
% Let us always pick the decision threshold assuming that the scoring classifier is perfectly calibrated, i.e. $s_{\text{dec}}=c$, even if actually the classifier is not calibrated.
% Then the \emph{Brier curve} is the result of plotting average misclassification cost per instance denoted as $L(c)$ against the cost proportion $c$ 
%  \cite{hernandez-orallo2011}, where $L(c)$ is defined as: 
% \begin{align*}
% L(c)=\frac{1}{n}\sum_{i=1}^n \mathsf{C}(+|-)\mathsf{I}(\hat{y}_i=+,y_i=-)+\mathsf{C}(-|+)\mathsf{I}(\hat{y}_i=-,y_i=+)
% \end{align*}
% and $\mathsf{C}(+|-)=2c$, $\mathsf{C}(-|+)=2(1-c)$. 
% Denote $\pi$ as the marginal probability for the positive class, $\mathit{fpr}(s_{dec})$ and $\mathit{tpr}(s_{dec})$ as the false positive rate and true positive rate at threshold $s_{dec}$. 
% The normalised optimal cost can then be derived as \cite{hernandez-orallo2012}:
% %
% \begin{align*}
%     L_c(s_{dec}) = 2c(1-\pi)\mathit{fpr}(s_{dec}) + 2(1-c)\pi(1 - \mathit{tpr}(s_{dec}))
% \end{align*}
% %
% Denote $\hat{Y}$ as the predicted label, here $(1-\pi)\mathit{fpr}(s_{dec})$ is the probability of false positive $P(Y=-, \hat{Y}=+)$, and $\pi(1 - \mathit{tpr}(s_{dec}))$ is the probability of false negative $P(Y=+, \hat{Y}=-)$. 
% A factor of $2$ is added to mimic the common definition of error rate, which corresponds to the case of $c = 0.5$ (i.e. a false positive has the same cost as a false negative).
% 
% While the above threshold $s_{\text{dec}}$ and cost are only optimised for the specific cost proportion $c$, it would be desirable if the classifier can provide scores that can be optimised with any potential cost proportion $c \in [0, 1]$.
% In this case, we want the conditions in Equation~(\ref{eq:dec}) to be met with any $s_{dec} $ (hence $c$), leading to the following definition.
% %
% \textit{Ranking calibration}: Denote a scoring binary classifier as $\mathsf{f}: \mathbb{X} \rightarrow \mathbb{R}$, $s_1, s_2 \in \mathbb{R}$ are two independent model output values, the classifier is ranking-calibrated if the following condition is met:
% %
% \begin{align}
%     P(Y=+ \mid s_1) \geq P(Y=+ \mid s_2)  \quad \forall s_1 \geq s_2
% \end{align}
% %
% With a ranking-calibrated classifier, we can simply find the $s_{\text{dec}}$ with any given cost proportion $c$.
% 
% This procedure can be further simplified by assuming $s$ are probability-calibrated scores, which is a sufficient condition to be ranking-calibrated:
% %
% \begin{align*}
%     P(Y=+ \mid s) = s  \quad \forall s \in [0, 1]
% \end{align*}
% %
% With calibrated scores, given any cost proportion $c$, we always have $s_{\text{dec}}=c$, and the optimal cost is hence:
% %
% \begin{align*}
%     L_c(c) = 2c(1-\pi)\mathit{fpr}(c) + 2(1-c)\pi(1 - \mathit{tpr}(c))
% \end{align*}
% 
% 
% Since the cost now only depends on $c$, it is possible to plot $L(c)$ as a scalar function of $c$, and such a visualisation is known as cost curves.
% The Brier curve plots $L(c)$ against $c$ \cite{hernandez-orallo2011}. 
% Brier curves are a particular kind of cost curve \cite{drummond2006}.
% These Brier curves have several useful properties:
% (1) The area under the Brier curve (i.e., the expected loss over uniform $c$) is equal to the Brier score, making a connection between the cost perspective and the proper scoring rule perspective; 
% (2) Among all possible score transformations, a perfectly calibrated classifier has the lowest possible Brier curve (lower envelope);
% (3) The areas between and under the Brier curves before and after perfectly calibrating are corresponding to the decomposition of Brier score into refinement loss and calibration loss. 

% Example Brier curves are given in Figure~\ref{fig:brier_curve}.
% We again consider a synthetic dataset where we can have as many data points as necessary to ensure a classifier can be nearly calibrated everywhere.
% As indicated by the left figure, we have a logistic classifier trained on the synthetic dataset, resulting in uncalibrated probabilities as depicted by the red reliability diagram.
% With unlimited data points, we then calibrate the classifier to be close to perfectly calibrated, and the corresponding blue reliability diagram follows the ascending diagonal.
% For the right figure, we see that the blue curve has a smaller area under it, which indicates a smaller Brier score.
% Since the blue curve is from a perfectly calibrated model, this area is also equivalent to the refinement loss of the model as calculated by the Brier score.
% The area between the two curves is therefore the calibration loss of the uncalibrated model.
% \citet{flach2015lmce} demonstrates that this construction carries over to other proper scoring rules. 



% \subsection{Beyond the calibration of label probabilities}
% \label{sec:beyond}
% 
% While we have been mainly addressing calibration of label probabilities in the classification context, the notion of calibration can be generalised to various tasks beyond standard probabilistic classification.
% 
% \subsubsection*{Probability calibration for optimal decisions with F-score}
% 
% When we discussed the cost-sensitive view of calibration in the previous section, we saw that the decision boundary under a standard accuracy setting (equal misclassification cost) is the calibrated probability of $0.5$.
% Furthermore, if we have a classifier that is calibrated for a specific probability value of $p$, it will be the corresponding decision boundary if we assume the negatives are $\frac{p}{1-p}$ times more important than positives.
% This assumption leads to a modified version of the accuracy measure, known as the weighted accuracy:
% %
% \begin{align*}
%     \mathit{acc}_{p}(t) = 2p(1 - \pi)\mathit{tnr}(t) + 2(1-p)\pi \mathit{tpr}(t)
% \end{align*}
% 
% By varying the value of $p$, we provide a cost-sensitive trade-off between true positives and true negatives, which further implies a trade-off between precision and recall.  
% In the extreme case, if we only care about the positives, that is, we can have $p$ getting close to $0$, and it means negatives are $\frac{p}{1-p} \rightarrow 0$ times more important than positives.
% With this setting, we can see the decision boundary will be the calibrated probability of $0$ and we will have a weighted accuracy of $1$.
% As a result, this decision boundary will lead to a recall of $1$ and a precision of $\pi$, which corresponds to a always-positive classifier.
% 
% Since the results above indicate a specific trade-off between precision and recall, it is more interpretable to use the $F_{\beta}$ score as a evaluation metric, as it includes both the precision and recall terms:
% %
% \begin{align*}
%     F_{\beta}(t) &= \frac{1}{\fracii{\frac{1}{1+\beta^2}}{\text{prec(t)}} + \fracii{\frac{\beta^2}{1+\beta^2}}{\text{rec(t)}}} \\
%     &= \frac{(1+\beta^2)\text{TP}(t)}{(1+\beta^2)\text{TP}(t) + \text{FP}(t) + \beta^2 \text{FN}(t)}
% \end{align*}
% %
% While $F_{\beta}$ is the standard form of the F-score, it is often more convenient to have a $[0, 1]$ weight $d = \frac{1}{1 + \beta^2}$, leading to the following re-parameterised version:
% %
% \begin{align*}
%     F_{d}(t) &= \frac{1}{d\frac{1}{\text{prec}(t)} + (1-d)\frac{1}{\text{rec}(t)}} \\
%     &= \frac{\text{TP}(t)}{\text{TP}(t) + d \text{FP}(t) + (1-d)\text{FN}(t) }
% \end{align*}
% 
% \begin{figure}[!b]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/conclusion/fig2-left.pdf}
%     \includegraphics[width=0.45\textwidth]{figures/conclusion/fig2-right.png}
%     \caption{({Left}): precision-recall curve, ({Right}) precision-recall-gain curve.}
%     \label{fig:pr_prg}
% \end{figure}
% 
% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/conclusion/PRG2.png}
%     \includegraphics[width=0.45\textwidth]{figures/conclusion/PRG3.png}
%     \caption{({Left}) Calibration for weighted accuracy with ROC curve, ({Right}) Calibration for $F_{\beta}$-score with precision-recall-gain curve.}
%     \label{fig:prg}
% \end{figure}
% 
% The question is now: how to calibrate a probabilistic classifier so that instances with a score value of $d$ will be on the $F_{d}$ decision boundary? 
% \citet{flach2015} address this problem by means of a non-linear transformation of the measures involved.
% We have seen that the conventional ROC curve can be used for calibrating probabilities by constructing the ROC convex hull, which is equivalent to isotonic regression.
% However, the traditional precision-recall curve is not sufficiently similar to a ROC curve to allow a similar calibration property.
% In contrast, the precision-recall-gain curve proposed by \citet{flach2015} can be seen as a proper generalisation of ROC curve obtained by replacing weighted accuracy with F-score.
% Figure~\ref{fig:pr_prg} gives a comparison between the precision-recall curve and the precision-recall-gain curve.
% Figure~\ref{fig:prg} exemplifies the calibration procedure for both the ROC curve and the precision-recall-gain curve.
% As indicated by the figures, unlike the traditional precision-recall curve, precision-recall-gain curve can be used together with the convex hull method to achieve calibration on any given $F_{\beta}$ score, as with the ROC curve with weighted accuracy.  

% \subsection{Calibration for regression}
% \label{sec:regcal}

% While in this survey we have focused on the cases where the target variable is discrete, the notion of calibration is also applicable to the continuous regression case.
% As in the classification scenario, there are multiple definitions of calibration for regression models.

% We first introduce the concept of quantile calibration.
% We denote a quantile regression model as $g: \mathbb{X} \times [0, 1] \rightarrow \mathbb{R}$, which takes a feature vector $\mathbf{x}$ and a value $\tau \in [0, 1]$, and outputs the estimated $\tau$-quantile value $\hat{y}$ so that $P(Y \leq \hat{y} \mid \mathbf{X}=\mathbf{x}) = \tau$. 
% The quantile regression model is defined as \emph{quantile-calibrated}, if and only if
% for $\forall \tau \in [0, 1]$, the following is satisfied: 
% %
% \begin{align*}
%     P\Big(Y \leq g(\mathbf{X}, \tau) \Big) = \tau \qquad \text{for } \forall \tau \in [0, 1]
% \end{align*}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.95\textwidth]{figures/conclusion/quantile_example.png}
%     \caption{An example of quantile calibration, calibrating the quantiles corresponding to $\tau=0.05,0.75,0.9$ (left plot) using a calibration map (middle plot) into quantiles corresponding to $\tau=0.1,0.5,0.8$ (right plot). }
%     \label{fig:quanitle}
% \end{figure}

% Following this definition, we can investigate how to calibrate a quantile regression model within a post-hoc setting.
% Since all possible quantiles are in the interval of $[0, 1]$, \citet{kuleshov2018} propose to adopt existing binary calibrators to adjust the quantiles.
% This procedure is demonstrated in Figure~\ref{fig:quanitle}.

% \subsubsection*{Distribution calibration for regression}

% Unlike calibration as defined for classifiers, quantile calibration for regression is defined globally across all predictions, and has no requirements on the individual prediction produced by the regression model.   
%
% To mimic the same level of calibration as in classification, \citet{pmlr-v97-song19a} introduce a stronger definition known as distribution calibration for regression. 
% If we denote a regression model (or conditional density estimator) as $$f: \mathbb{X} \rightarrow \{s \mid s:\mathbb{R} \rightarrow [0, \infty), \int s(y)dy = 1 \}$$ then this model is defined as \emph{distribution-calibrated}, if and only if
% for $\forall s :\mathbb{R} \rightarrow [0, \infty), \int s(y)dy = 1$, the following holds: 
%
% \begin{align*}
%     P\Big(Y=y \mid f(\mathbf{X}) = s) \Big) = s(y) \qquad \text{for } \forall s :\mathbb{R} \rightarrow [0, \infty), \int s(y)dy = 1
% \end{align*}
%
% Being distribution-calibrated is a sufficient but not necessary condition for being quantile-calibrated \citep[][Theorem 1]{pmlr-v97-song19a}.

% Figure~\ref{fig:dist} gives an illustration of the differences between quantile calibration and distribution calibration.
% Quantile-calibrated regression considers the global quantiles, and distribution-calibrated regression further models local distributions.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.65\textwidth]{figures/conclusion/regression_example.png}
%     \caption{The difference between distribution calibration and quantile calibration.}
%     \label{fig:dist}
% \end{figure}

% Alternative concepts of regression calibration also exist, including conformal prediction \cite{romano2019conformalized} and threshold calibration \cite{sahoo3reliable}. 
%\todo{This citation is incomplete (missing year)}




% \newtext{Will work on this in a few hours \begin{itemize}
%         \item There are various ways to visualise and quantify calibration
%         \item ECE measures aim at producing an aggregate measure of the visual information provided in reliability diagrams
%         \begin{itemize}
%             \item Thus, their optimisation is not guaranteed to produce desirable classifiers
%         \end{itemize}
%         \item Proper scoring rules measure different aspects of probability correctness
%         \begin{itemize}
%             \item They have been used as training losses in classifier training for a while
%             \item But they cannot tell ``where'' the model is more miscalibrated
%         \end{itemize}
%         \item Finally, the hypothesis test for calibration can help determine if a particular loss value means that the classifier is calibrated or not
%     \end{itemize}}


==> mlj_files/06_conclusion.tex <==
\section{Concluding remarks}
\label{sec:conclusion}

In this survey we have given a detailed overview of the principles and practice of classifier calibration.
We discussed the motivation, definition, evaluation and related approaches for the calibration of probabilistic classifiers, and touched upon topics beyond the standard classification setting.
With the recent proliferation of predictive machine learning, it is becoming more and more important that models are carefully evaluated and if possibly improved on multiple criteria to ensure the overall system robustness.
Classifier calibration relates to the criterion of uncertainty quantification, investigating the statistical relationships between model predictions and observed target variables.
There are other levels of uncertainty in the overall modelling procedure, including uncertainty pertaining to model parameters when the training set is limited, uncertainty brought about by model mismatch, or uncertainty regarding whether the model should abstain when there might be novel target values that were not seen in the training set -- see \cite{hullermeier2021aleatoric} for a recent survey on uncertainty in machine learning. 
% With all of these interesting challenges in mind, we hope this paper can provide a useful reference for researchers and practitioner that are interested in bring predictive machine learning to the next steps.

As we hopefully have made clear in this survey, calibration research has a rich history which predates the birth of machine learning as an academic field by decades. It is important to take full advantage of that history, which perhaps isn't always fully acknowledged in recent literature on classifier calibration (e.g., of deep neural networks, which are often over-confident). Recent proposals such as confidence calibration, temperature scaling and expected calibration error have value but are far from the only options and may not be suitable for a particular application. As is often the case in machine learning, the space of options and things to consider is large, and navigating this space requires the right set of concepts and tools, many of which we have discussed in detail in this survey. 

It is perhaps useful to point out that, naturally, there are also concepts that are less than helpful when thinking about classifier calibration. One of the most prominent of these is the concept of a decision boundary, which is like describing Mount Everest with a single contour line, halfway up. To faithfully characterise the mountain -- which is what is needed for optimal decision making -- one needs many contour lines at different elevations. The only case in which the decision boundary is useful is when the class prior (and misclassification costs, if any) won't change after training, in which case only the decision threshold needs calibrating. In all other cases context change is expected and needs to be anticipated with a proper calibration analysis. 

\newtext{If a trained classifier $f$ is going to be used for a task for which it is good enough to be accurate, precise or to perform well according to any contingency matrix-based measure, then there is no particular need to consider calibration in the model's development pipeline. However, if calibrated probabilities are important for any decisions supported by $f$, the following steps can be taken to implement what was discussed in this paper:}
\newtext{
    \begin{enumerate}
        \item If possible, any classifiers considered for a task should be trained using a proper scoring rule as loss function;
        \begin{itemize}
            \item The resulting models are likely to produce better probabilities than if a non-proper loss function is used, as probability refinement and calibration will be encouraged during training (recall Section \ref{sec:psr});
            \item An alternative is to use a method that encourages calibration during training time, as discussed in Section \ref{sec:cal:training};
        \end{itemize}
        \item With the trained classifiers and, preferably a held-out calibration dataset, the calibration of the probabilities produced by the models can be evaluated using classwise reliability diagrams, to understand the miscalibration patterns, and/or ECE measures (recall Section \ref{sec:metrics});
        \item To help define which models are uncalibrated, a hypothesis test for calibration can be applied (recall Section \ref{sec:hyp});
        \item If any models produce uncalibrated probabilities, post-hoc calibrators should be used to fix them;
        \begin{itemize}
            \item The resulting calibrators should also be evaluated using reliability diagrams, ECE measures and hypothesis tests to find out which ones work best for the particular miscalibration patterns found during step 2.
        \end{itemize}
    \end{enumerate}
}

\newtext{
In order to help with the aforementioned steps, we have developed an open-source Python library called PyCalib \cite{pycalib} \footnote{The documentation of the library can be found at https://classifier-calibration.github.io/PyCalib/}. This library provides tools to measure the calibration quality of a classifier, multiple visualisation functions to better understand how calibrated is a model, and some calibration methods and pipelines to directly train arbitrary calibrated classifiers.
}

\newtext{We close this survey with some open problems. First, although binning is such an important concept in calibration, there is no standard method to decide which type of binning, e.g. equal frequency or equal width, or what number of bins to use. Recent work \cite{kangsepp2022usefulness} has investigated cross-validation to tune the number of bins used to evaluate a model on a calibration set. Second, a recurrent topic of interest is the fact that post-hoc calibration does not improve robustness against out-of-distribution inputs and what can be done to improve calibration in this context \cite{ovadia2019can}. Finally, and somewhat related to the previous point, even though calibrated probabilities provide estimations of the uncertainty regarding an instance's class given its feature values (aleatoric or first-order uncertainty), classifiers could also be made to predict their uncertainty about the predicted probabilities, which comes from not knowing the true probabilities (epistemic uncertainty). This type of prediction, a distribution of distributions, also called second-order uncertainty \cite{hullermeier2022quantifying,bengs2022pitfalls}, has been recently treated using inference based on Bayesian methods and credal sets, which are convex sets of probability distributions \cite{shaker2021ensemble}.}

% Ensure that after lessons learned we add some discussion of current open problems: second-level uncertainty, aleatoric/epistemic uncertainty, out of distribution, better metrics, better binning

%----------------------------------------------------%
% \subsection{Concluding remarks}

% \paragraph{{The myth of the decision boundary}}
%  \begin{itemize}
%     \item \highlighted{red}{Resist} thinking in terms of decision boundaries.
%     \begin{itemize}
%         \item {That is like describing Mount Everest with a single contour line, halfway up.}
%         \item {To faithfully characterise the mountain you need many contour lines at different elevations.}
%     \end{itemize}
%     \item[]
%     \item The \highlighted{red}{only case} in which the decision boundary is useful is when the class prior (and misclassification costs, if any) won't change after training. 
%         \bb{In that case you don't need to calibrate the entire probability range, only the decision threshold.}
% \end{itemize}

% \paragraph{{The long history of classifier calibration}}
%\begin{itemize}
%\item Contrary what recent machine learning literature may lead you to believe, \highlighted{red}{calibration research predates machine learning} and has been studied for three-quarters of a century.
%\item{Make sure you take full advantage of that history, and don't just follow the citations in the latest NeurIPS paper on DNN calibration.}
%\item[]
%\item Recent proposals such as confidence calibration, temperature scaling and expected calibration error have their value, but are far from the only options and may not be suitable for your particular application. 
%\item{Which leads me to\ldots}
% \end{itemize}

% \paragraph{{Calibration is an art as well as a science}}
% Many practical questions don't have \textit{a priori} answers:
%\begin{itemize}
%    \item Which calibration method? 
%    \item How many bins? 
%    \item What evaluation metric? 
%    \item Do I use a validation set? How large? 
%    \item \ldots
% \end{itemize}

%\begin{description}
%    \item[]
%    \item[We hope this tutorial has given you the tools to navigate this space!]
%\end{description}

==> mlj_files/07_declarations.tex <==
\subsection*{Declarations}

\paragraph{Funding} 
The work of PF, RSR and MPN was supported by the SPHERE Next Steps Project funded by the UK Engineering and Physical Sciences Research Council (EPSRC) [grant EP/R005273/1]. The work of RSR was funded by the UKRI Turing AI Fellowship [grant EP/V024817/1].
The work of PF and HS was supported by The Alan Turing Institute under EPSRC [grant EP/N510129/1].
The work of MK was supported by Estonian Research Council [grant PRG1604].

\paragraph{Conflicts of interest/Competing interests} Not applicable.
\paragraph{Ethics approval} Not applicable.
\paragraph{Consent to participate} Not applicable.
\paragraph{Consent for publication} Not applicable.
\paragraph{Availability of data and material} The availability of data and material used in this survey can be found at \href{https://github.com/classifier-calibration/additional_material}{https://github.com/classifier-calibration/additional\_material}. Further information is available at \href{ https://classifier-calibration.github.io/survey/}{ https://classifier-calibration.github.io/survey/}.
\paragraph{Code availability} The code to generate measurements, visualisation and results is part of \href{https://pypi.org/project/pycalib/}{PyCalib}. Further information can be found in the documentation of the library
\url{https://classifier-calibration.github.io/PyCalib/}.
\paragraph{Authors' contributions}
TSF: conceptualisation, formal analysis, methodology, software, writing (original draft, and review and editing). 
HS: conceptualisation, formal analysis, methodology, software,  writing (original draft, and review and editing). 
MPN: formal analysis, methodology, software, visualisation, writing (original draft, and review and editing). 
RSR: formal analysis, writing (review and editing). 
MK: conceptualisation, formal analysis, methodology, writing (review and editing). 
PF: conceptualisation, formal analysis, methodology, supervision, writing (original draft, and review and editing).
\footnote{The categories follow the CRediT taxonomy: http://credit.niso.org/}


==> mlj_files/compiled/01_intro.tex <==
\section{Introduction and motivation}
\label{sec:intro}


A $K$-class probabilistic classifier is \emph{well-calibrated} if among test instances receiving a predicted $K$-dimensional probability vector $\mathbf{s}$, the class distribution is (approximately) distributed as $\mathbf{s}$.  
This property is of fundamental importance when using a classifier for cost-sensitive classification, for human decision making, or within an autonomous system.
It means that the classifier correctly quantifies the level of uncertainty or confidence associated with its predictions. 
In a binary setting, scores given by a sufficiently calibrated classifier can be simply thresholded to minimise expected misclassification cost. Thresholds can also be derived to optimally adapt to a change in class prior, or to a combination of both. In contrast, for a poorly calibrated classifier the optimal thresholds cannot be obtained without optimisation.

Many machine learning algorithms are known to produce over-confident models, unless dedicated procedures are applied during training. 
%(e.g., Laplace smoothing in decision trees \cite{ferri2003improving}).
The goal of \emph{(post-hoc) calibration methods} is to use hold-out validation data to learn a \emph{calibration map} for a previously trained model that transforms the model's predictions to be better calibrated.
Many calibration methods for binary classifiers have been introduced, including
logistic calibration (also known as `Platt scaling'), 
various binning methods including isotonic calibration (also known as the ROC convex hull method), 
as well as more recent methods including beta calibration and Bayesian methods. 

When we have more than two classes, calibration is generally more involved, as is often the case with multiclass classification. 
Multiclass calibration has mostly been approached by decomposing the problem into $K$ one-vs-rest binary calibration tasks, one for each class. The predictions of these $K$ calibration models form unnormalised probability vectors, which, after normalisation, may not be calibrated in a multiclass sense. 
Native multiclass calibration methods were introduced recently focusing on neural networks. These methods constitute various multiclass extensions of Platt scaling, adding a calibration layer between the logits of the neural network and the softmax layer. 

The literature on post-hoc classifier calibration in machine learning is now sufficiently rich that it is no longer straightforward to obtain or maintain a good overview of the area, which was the main motivation for writing this survey. It grew out of a tutorial we presented at the 2020 European Conference on Machine Learning and Principles and Practice of Knowledge Discovery in Databases (see \url{https://classifier-calibration.github.io}). Our aim then and now is to provide both introductory material and up-to-date technical details of the main concepts and methods. \newtext{Our focus is on the classical setup where the classifier is deployed in the same setting where it was calibrated, except for potential changes in class prior or misclassification costs. We do not cover methods to achieve robustness under conditions of other distributional shifts or out-of-distribution inputs \cite{ovadia2019can}.} We try to do justice to historical developments and pay attention to important topics that are not as widely known as they deserve to be, such as proper scoring rules. 

We also try to identify and clarify possible sources for confusion. 
The multiclass setting in particular introduces numerous subtleties that have not always been recognised or correctly dealt with in previous work. 
For example, some authors use the weaker notion of \emph{confidence calibration}, which requires only that the classifier's predicted probability for what it considers the most likely class is calibrated. 
While this is perfectly valid in its own right, it isn't always appreciated by subsequent authors that this is a much weaker notion of calibration than the one defined informally in the first sentence of this survey. 
One can also observe variations in the evaluation metric used and in the way calibrated probabilities are visualised. 
Our main aim in this survey is hence to provide a unified perspective on the different methods and metrics for binary and multiclass calibration, giving each variation its proper place. 

For the purpose of this survey we have developed a Python library which includes most of the functionalities presented in the following sections.
PyCalib~\footnote{https://classifier-calibration.github.io/PyCalib/} implements several calibration metrics (eg. confidence and classwise ECE, and their MCE counterparts), common calibration methods (eg. Isotonic Calibration, Platt's Scaling, Binning calibration), a method to combine arbitrary classifiers and calibrators into a unified training and deployment pipeline, a one-vs-the-rest implementation to adapt any binary calibration method to the multiclass setting, and multiple visualisation tools to inspect visually the calibration quality as well as tools to get better insights about the learned calibration maps.
As an illustration of the library's capabilities, most of the figures and results reported in this paper have been generated using PyCalib.

%Given the lack of a unified code distribution for calibration, we have created a Python library called .
%which includes most of the functionalities presented in this paper to assess calibration.
%This library implements several calibration metrics (eg. confidence-ECE, classwise-ECE, confidence-MCE), common calibration methods (eg. Isotonic Calibration, Platt's Scaling, Binning calibration), a one-vs-the-rest implementation to adapt any binary calibration method for the multiclass setting, and multiple visualisation tools to assess calibration (eg. binary and multiclass reliability diagrams, calibration maps for two and three classes, and other functions to explore three class classification problems). Most of the reliability diagrams and other common calibration metrics in this survey have been generated using this library.

The survey is structured as follows. 
The next section will cover important notions and intuitions related to calibration. \newtext{It aims to be at a more introductory level}, leaving technical detail for later sections. 
Section \ref{sec:psr} discusses proper scoring rules, an important general framework for evaluation of probability estimates. In Section \ref{sec:metrics} we present systematic overview of visualisation approaches and evaluation metrics for classifier calibration. 
Section \ref{sec:calibrators} is devoted to a comprehensive account of post-hoc calibration methods for both the binary and multiclass scenarios. 
Section \ref{sec:hyp} covers hypothesis tests for calibration, and Section \ref{sec:conclusion} concludes with a summary and outlook. 

==> mlj_files/compiled/02_highlevel_intro.tex <==
\section{A brief introduction to classifier calibration}
\label{sec:intro:high:level}

\newtext{
The origins of classifier calibration can be traced back to weather forecasting and meteorology. 
Here is what the UK Met Office website used to say about what their forecast probabilities mean: 

\begin{quote}
    ``[S]uppose the Met Office says that the probability of rain tomorrow in your region is 80\%. They aren't saying that it will rain in 80\% of the land area of your region, and not rain in the other 20\%. Nor are they saying it will rain for 80\% of the time. What they are saying is there is an 80\% chance of rain occurring at any one place in the region, such as in your garden.
[...]
[A] forecast of 80\% chance of rain in your region should broadly mean that, on about 80\% of days when the weather conditions are like tomorrow's, you will experience rain where you are. 
%But there is still some expert judgement involved, and different forecasting organisations with different experts and different technology might well give different probabilities.
[...]
If it doesn't rain in your garden tomorrow, then the 80\% forecast wasn't wrong, because it didn't say rain was certain. But if you look at a long run of days, on which the Met Office said the probability of rain was 80\%, you'd expect it to have rained on about 80\% of them. '' %
%(\url{https://www.metoffice.gov.uk/about-us/what/accuracy-and-trust})
(\url{https://web.archive.org/web/20210928235732/https://www.metoffice.gov.uk/about-us/what/accuracy-and-trust/probability})
%\todo[inline]{The link is broken now. I found an archived version from Sept. 28, 2021 in the Internet Archive.}
\end{quote}
\noindent
Note the phrase ``a long run of days'': determining the degree to which a forecaster is well-calibrated cannot be done on a per-forecast basis, but rather requires looking at a sufficiently large and diverse set of forecasts. 

\begin{table}[!t]
        \centering
        \includegraphics[width=\linewidth]{hallenbeck1920_tab1}
        \caption{Reproduced from \citet{hallenbeck1920}.}
        \label{tab:eval:hallenbeck1920}
\end{table}

\begin{figure}[!b]
    \centering
%    \includegraphics[width=0.6\linewidth]{Hallenbeck.pdf}\\
    \begin{subfigure}[b]{0.45\linewidth}
    \includegraphics[width=\linewidth]{Hallenbeck.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{0.40\linewidth}
    \includegraphics[width=\linewidth]{hallenbeck_alt.pdf}
    \end{subfigure}
    \caption{Two different graphical representations of the forecasts in Table~\ref{tab:eval:hallenbeck1920}.
\textbf{(Left)} The bottom graph gives a histogram of the probability forecasts. 
The top graph compares the forecast probabilities with the proportion of actual rain events in that bin. 
The red bars indicate to what extent these proportions are higher or lower than predicted. 
\textbf{(Right)} A simplified visualisation, only showing the proportion of rain events in a bin (y-axis) against the average prediction in the bin (x-axis).
    }\label{fig:hallenbeck-rel}
\end{figure}


Table~\ref{tab:eval:hallenbeck1920}, reproduced from \citet{hallenbeck1920}, groups 123 weather forecasts in 10 equal-width bins, and compares each bin with the actual empirical percentage of rain events. 
Figure~\ref{fig:hallenbeck-rel} shows two possibilities of displaying this information graphically, comparing the predicted probabilities on the $x$-axis to empirical probabilities on the $y$-axis. 
A variety of such graphical representations can be found in the literature; they are generally known as \emph{reliability diagrams}, `reliability' being one of many terms used to denote goodness of calibration \cite{murphy1977reliability}.
We can see that most of the forecasts are slight under-estimates: for example, of the 15 forecasts in the 40-49\% bin, $8/15=53\%$ were actual rain events. 
In the left graph this is shown by the vertical red line, which indicates how much the top of the blue bar extends above the diagonal (meaning that the actual proportion of rain events was higher than estimated). 
On the right graph this can be seen directly from how much the respective point is higher than the diagonal.
Similarly, we see that two of the bins (20-29\% and 30-39\%) are very slight over-estimates: on the left graph the top of the blue bar is below the diagonal, which means that the actual proportion of rain events was lower than estimated. 

\begin{figure}[!t]
    \centering
    \begin{subfigure}{0.45\linewidth}
    \includegraphics[width=\linewidth]{Hallenbeck2.pdf}
    \end{subfigure}
    \begin{subfigure}{0.45\linewidth}
    \includegraphics[width=\linewidth]{Hallenbeck3.pdf}
    \end{subfigure}
    \caption{Dividing the forecasts in Table~\ref{tab:eval:hallenbeck1920} in five (left figure) and two (right figure) equal-width bins.}\label{fig:hallenbeck2-rel}
\end{figure}

The choice of ten equal-width bins is somewhat arbitrary, and it is informative to consider different choices. 
Merging pairs of adjacent bins results in five equal-width bins, as depicted in Figure~\ref{fig:hallenbeck2-rel} (left). 
We see that all but the right-most bin averages are now slightly off-centre (we assumed that within each original bin all forecast probabilities are the same and equal to the bin centre: e.g., 25\% in the 20-29\% bin). Again, the pattern is that the higher forecast probabilities are about 10\% too low. 
Figure~\ref{fig:hallenbeck2-rel} (right) shows what we get with only two bins. 
We have lost a bit too much information here, so bins shouldn't be taken too wide. 
On the other hand they shouldn't be taken too narrow either, in order to be able to measure the true proportion of rain events with sufficient resolution. 

Taking the forecast event as a binary variable means that the calibration concept is directly applicable to binary classification. Here is an example from the typical machine learning task of learning a classifier for distinguishing `junk' or `spam' emails from regular ones: 

\begin{quote}
    A prediction `70\% chance of spam' should be spam 70\% of the time.
\end{quote}
\noindent
And a generalisation to categorical variables with more than two values is equally straightforward, as this example from Fisher's famous Iris dataset shows: 

\begin{quote}
    A prediction `70\% chance of setosa, 10\% chance of versicolor and 20\% chance of virginica' should be setosa/versicolor/virginica 70/10/20\% of the time.
\end{quote}
\noindent
So, to sum up: \emph{A predicted probability (vector) should match empirical (observed) probabilities.}
\newtext{
In the language of predictive machine learning, given an instance space $\mathbb{X}$, a binary target space $\mathbb{Y} = \{+, -\}$, and a binary probabilistic classifier $\mathsf{f}:\mathbb{X}\rightarrow [0, 1]$, the binary classifier is \emph{calibrated} if $\forall s \in[0,1]$:
\begin{align*} 
\mathsf{P}(Y=+ \: | \: \mathsf{f}(\mathbf{X}) = s)=s
\end{align*}}




% \subsection{A closer look at calibration, and why it matters}
% \label{sec:2:1}

% % \paragraph{Why are we interested in calibration?}
% In general, to calibrate means \emph{to employ a known scale with known properties}. 
% % \bb{E.g., additive scale with a well-defined zero, so that ratios are meaningful.}
% For example, we can calibrate a thermometer to Celsius or Fahrenheit scales; 
% or a weighing device to kilograms or pounds. 
% If a measuring device is calibrated to one scale but we need the measurement in another, there are usually simple conversion formulas: 
% for example, $\text{F}=\text{C}\cdot 9/5+32$ for Celsius to Fahrenheit, and $\text{Lb}=2.2\cdot \text{Kg}$ for kilograms to pounds. 
% Notice that the temperature conversion shifts the zero point 
% (0 degrees Celsius is 32 degrees Fahrenheit, and 0 degrees Fahrenheit is $-17.8$ degrees Celsius) 
% as it is essentially arbitrarily chosen for either scale. 

% The weight conversion, in contrast, has an absolute zero which is the same for all scales. 
% Such scales are called \textit{ratio scales}, because the ratio of two measurements is meaningful: e.g., if one object is twice as heavy as another in kilograms then it will be so regardless of the scale. Such ratios are not meaningful for Celsius and Fahrenheit, but temperature \textit{differences} are.  
% For example, we could say that this person's change from morning to evening body temperature today is twice that of yesterday, without specifying the temperature scale. 
% It follows that ratios of differences (or intervals) are meaningful in this case, which is why Celsius and Fahrenheit are called \textit{interval scales}. 

% For classifiers we want to use the probability scale. Probabilities have an absolute zero like any other ratio scale, and so it is meaningful to say that one event is twice as probable as another. Probabilities also have a fixed maximum, so that taking the complement with respect to the maximum gives another ratio scale: for example, the probability of this event \textbf{not} happening might be twice the probability of another event \textbf{not} happening. This essentially fixes the scale: we don't have pounds vs.\ kilograms dilemmas for probabilities. 

% % Q: Is the probability scale additive?
% Are probabilities additive? In certain situations it is indeed valid to sum probabilities, for example to obtain the probability of any one of a number of mutually exclusive events happening, as might occur when joining classes in a multiclass classification setting. 
% But multiplication and division of probabilities are more common basic operations, for example to obtain the joint probability of independent events, or to derive a conditional probability from joint and marginal probabilities. This makes the probability scale \textit{multiplicative} for typical usage. We could obtain an additive scale by taking logarithms, giving log-likelihoods, logits as differences of log-likelihoods, etc. A couple of observations are worth making: 
% \begin{itemize}
% \item Such transformations are fundamentally different from scale conversions such as Celsius to Fahrenheit, because probabilities and log-likelihoods measure different things -- physicists might say they represent different \textit{dimensions}. Nevertheless, the transformations are invertible and hence the dimensions convey the same information. 
% \item While some ratios or products of probabilities again yield probabilities, in other cases they may derive another dimension, such as \textit{odds}, which are not expressed on a probability scale.
% \end{itemize}

\subsection{Why calibration matters}
\label{sec:int:why}

What are the benefits of using well-defined calibrated scales in general, and well-calibrated probabilities in particular? One obvious benefit of calibrated scales is that we can easily combine measurements that are expressed on the same scale without comparing apples and oranges. Another is that we can use standardised decision rules, e.g., defining a fever as a body temperature exceeding 100 degrees Fahrenheit. These benefits
% \footnote{As for combining multiple probability estimates as might happen in ensemble methods in machine learning, note that the argument of probabilities being multiplicative leads to favouring the \textit{geometric mean} (or the arithmetic mean on log-probabilities). Using the arithmetic mean directly on probabilities means that the members of the ensemble are treated as classifiers scoring on some arbitrary but fixed and additive scale, disregarding their probabilistic nature.}
directly carry over to the class probability scenario, justifying decision rules such as predicting the class whose estimated probability exceeds $0.5$ in binary classification, or the class with the highest predicted probability for multiclass classification. Importantly, there is a further benefit to using calibrated probabilities as it means we can adjust these decision rules in a straightforward way to account for different class priors or misclassification costs, as we will briefly discuss presently.

% %Q: What issues might arise when applying MAP decisions to poorly calibrated classifiers such as naive Bayes? 

% % PF: UNTIL HERE (27 JAN 9.30 GMT)

% % \paragraph{Optimal decisions}
% Denote the cost of predicting class $j$ for an instance of true class $i$ as ${\mathsf{C}(\hat{Y}=j|Y=i)}$. 
% % Since we don't know the true class of an unlabelled instance, we need to base our prediction on an assessment of the expected cost over all possible true classes. 
% The expected cost of predicting class $j$ for instance $\mathbf{x}$ is then
% %
% \begin{align}\label{eq::expected-cost}
% \mathsf{C}(\hat{Y}=j|\mathbf{X}=\mathbf{x}) &= \sum_i \mathsf{P}(Y=i|\mathbf{X}=\mathbf{x})\mathsf{C}(\hat{Y}=j|Y=i)
% \end{align}
% %
% where $\mathsf{P}(Y=i|\mathbf{X}=\mathbf{x})$ is the (true) probability of instance $\mathbf{x}$ having true class $i$
% (as would be given by the Bayes-optimal classifier). 
% %
% The optimal decision is to predict the class with lowest expected cost:
% \begin{align*}
% \hat{Y}^* = \argmin_j \mathsf{C}(\hat{Y}=j|\mathbf{X}=\mathbf{x}) = \argmin_j \sum_i \mathsf{P}(Y=i|\mathbf{X}=\mathbf{x})\mathsf{C}(\hat{Y}=j|Y=i)
% \end{align*}
% %
% % In the special case that all misclassifications have equal cost we can assume without loss of generality that $C(\hat{Y}=j|Y=i)=1$ for $i\neq j$ and $C(\hat{Y}=j|Y=i)=0$ for $i=j$, which gives
% % \begin{align*}
% % C(\hat{Y}=j|X=x) &= \sum_{i\neq j} P(Y=i|X=x) = 1-P(Y=j|X=x) \\
% % %\end{align*}
% % %and so
% % %\begin{align*}
% % \hat{Y}^* &= \arg\min_j [1-P(Y=j|X=x)] = \argmax_j P(Y=j|X=x)
% % \end{align*}
% In binary classification (with a positive, $+$, and and negative class, $-$) we have one predicted probability and four cost parameters, and we can rewrite Equation~(\ref{eq::expected-cost}) as
% %
% \begin{align*}
% \mathsf{C}(\hat{Y}=+|\mathbf{X}=\mathbf{x}) &= \mathsf{P}(+|\mathbf{x})\mathsf{C}(+|+) + \big(1-\mathsf{P}(+|\mathbf{x})\big)\mathsf{C}(+|-) \\
% \mathsf{C}(\hat{Y}=-|\mathbf{X}=\mathbf{x}) &= \mathsf{P}(+|\mathbf{x})\mathsf{C}(-|+) + \big(1-\mathsf{P}(+|\mathbf{x})\big)\mathsf{C}(-|-)
% \end{align*}
% %
% where $\mathsf{P}(+|\mathbf{x})$ is shorthand for $\mathsf{P}(Y=+|\mathbf{X}=\mathbf{x})$ and $\mathsf{C}(j|i)$ for $\mathsf{C}(\hat{Y}=j|Y=i)$.
% %
% On the optimal decision boundary these two expected costs are equal, 
% which gives
% \begin{align*}
% \mathsf{P}(+|\mathbf{x})\mathsf{C}(+|+) + (1-\mathsf{P}(+|\mathbf{x}))\mathsf{C}(+|-) = \mathsf{P}(+|\mathbf{x})\mathsf{C}(-|+) + (1-\mathsf{P}(+|\mathbf{x}))\mathsf{C}(-|-)
% \end{align*}
% which can be rearranged to give the posterior odds
% \begin{align*}
% \frac{\mathsf{P}(+|\mathbf{x})}{1-\mathsf{P}(+|\mathbf{x})} = \frac{\mathsf{C}(+|-)-\mathsf{C}(-|-)}{\mathsf{C}(-|+)-\mathsf{C}(+|+)}
% \end{align*}
% as well as the posterior probability
% \begin{align*}%\label{eq::cost-threshold}
% \mathsf{P}(+|\mathbf{x})  = \frac{{\mathsf{C}(+|-)-\mathsf{C}(-|-)}}{{\mathsf{C}(+|-)-\mathsf{C}(-|-)}+{\mathsf{C}(-|+)-\mathsf{C}(+|+)}} \triangleq c
% \end{align*}
% %
% $c$ thus gives the optimal threshold on the hypothetical Bayes-optimal probabilities. 
% It is also the best thing to do in practice, as long as the probabilities are well-calibrated (this is discussed in more detail in Section~\ref{sec:out:conc}). 

% Under reasonable assumptions (e.g., changing the prediction from correct to incorrect cannot decrease the incurred cost) we can set the cost of true positives and true negatives to zero \cite{elkan2001}; 

Let
$c = \frac{\mathsf{C}(+|-)}{\mathsf{C}(+|-) + \mathsf{C}(-|+)}$ be the cost of a false positive in proportion to the combined cost of one false positive and one false negative. 
With these cost parameters the Bayes-optimal decision rule is to set the decision threshold to $c$.
For instance, if false positives are 4 times as costly as false negatives then we set the decision threshold to $4/(4+1)=0.8$ in order to only make positive predictions if we are sufficiently certain.
%
Similar reasoning applies to changes in class priors: 
\begin{itemize}
    \item if we trained on balanced classes but want to deploy with 4 times as many positives compared to negatives, we lower the decision threshold to $0.2$; 
    \item more generally, if we trained for class ratio $r$ and deploy for class ratio $r'$ we set the decision threshold to $r/(r+r')$. 
\end{itemize}
Cost and class prior changes can be combined in the obvious way; see  \citet{flach2014classification} for details.

In summary, an important reason to be interested in calibrating our classifiers is that default decision rules such as predicting the class with the highest predicted probability are fully justified from a decision-theoretic point of view, and can easily be adapted to changes in class and cost distributions. In contrast, poorly calibrated classifiers such as naive Bayes will often perform sub-optimally with default decision rules. It is possible to learn a better decision rule for a given cost and class skew using, e.g., ROC analysis \cite{lachiche2003improving} but this would have to be repeated each time the skew changes. The great advantage of post-calibration is that it only needs to be done once -- in a sense, it optimises all possible decision rules in one go.

%\todo{mention fairness and explainability?}

%\subsection{Challenges in evaluating calibration}
%Impact of binning for reliability diagrams}



\subsection{Common forms of miscalibration, and how to fix them}

There are many reasons why a probabilistic classifier might produce miscalibrated scores, and hence many ways in which miscalibration manifests itself, but two main types stand out: underconfidence and overconfidence. In this section we look at some examples and introduce two mitigation techniques. 

 
Figure~\ref{fig:under-over}, taken from \citet{niculescu-mizil2005}, shows two typical examples. In both cases the points in the reliability diagram are far from the diagonal, although the effect is smaller in the figure on the right. 

\begin{figure}[!t]
    \centering
    \begin{subfigure}{0.4\linewidth}
        \includegraphics[width=\linewidth]{caruana_fig_1.pdf}
        \caption{Underconfidence}
    \end{subfigure}%\hfill
    \hspace{1cm}
    \begin{subfigure}{0.4\linewidth}
        \includegraphics[width=\linewidth]{caruana_fig_2.pdf}
        \caption{Overconfidence}
    \end{subfigure}
    \caption{Examples of under- and overconfident classifiers. The axes are the same as for the previous figures: x-axis shows predicted probabilities and y-axis shows empirical probabilities. The dots represent the reliability diagram, and the lines show the best-fit logistic curve and beta curve.
    %To correct the underconfident scores on the left we would have to pull the points away from the midpoint on the $x$-axis, whereas to deal with the overconfidence on the right we would push them toward the midpoint. 
    Note that the logistic sigmoid is a good fit for underconfident scores but not for overconfidence.
    The figure has been adapted from \citet{niculescu-mizil2005}, and the beta curves have been added.}
    \label{fig:under-over}
\end{figure}


% \begin{figure}[!t]
%     \centering
%     \begin{subfigure}{0.3\linewidth}
%         \includegraphics[width=\linewidth]{Underconfidence.pdf}
%         \caption{Underconfidence, logistic curve}
%     \end{subfigure}\hfill
%     \begin{subfigure}{0.3\linewidth}
%         \includegraphics[width=\linewidth]{Overconfidence.pdf}
%         \caption{Overconfidence, logistic curve}
%     \end{subfigure}
%     \begin{subfigure}{0.35\linewidth}
%         \includegraphics[width=\linewidth]{betafig.pdf}
%         \caption{Overconfidence, beta curve}
%     \end{subfigure}
%     \caption{Examples of under- and overconfident classifiers. The axes are the same as for the previous figures: x-axis shows predicted probabilities and y-axis shows empirical probabilities. The dots represent the reliability diagram, and the line shows the best-fit logistic curve (a,b) or beta curve (c).
%     %To correct the underconfident scores on the left we would have to pull the points away from the midpoint on the $x$-axis, whereas to deal with the overconfidence on the right we would push them toward the midpoint. 
%     Note that the logistic sigmoid is a good fit for underconfident scores but not for overconfidence.
%     Figures (a,b) are reproduced from \citet{niculescu-mizil2005}.}
%     \label{fig:under-over}
% \end{figure}

What do we see in the left figure? It is quite natural to give precedence to vertical information in such graphs, so you might be inclined to say ``The points on the left are too low, and the points on the right are too high''. But keeping in mind that the predicted probabilities on the $x$-axis are under our control but not the empirical probabilities on the $y$-axis, a more `actionable' way to express this is

\begin{quote}
    The lower points are too far to the right, and the higher points are too far to the left. In other words, the points have a tendency to sit too close to the midpoint on the $x$-axis. 
\end{quote}
\noindent
This is the typical pattern displayed by an \textit{underconfident} classifier, which thinks it's {worse} at separating classes than it actually is. 

Hence, to mitigate this, we need to {pull predicted probabilities away from the centre}. As the left plot in Figure \ref{fig:under-over} shows, this can be neatly modelled by a sigmoidal logistic curve, which can be defined in parametric form as
%
\begin{align*}
    \mathsf{c}(s; w, m) &= \frac{1}{1+\exp(-w(s-m))}%\\
    % w &= (\mu_{\textit{pos}}-\mu_{\textit{neg}})/\sigma^2, 
    % m = (\mu_{\textit{pos}}+\mu_{\textit{neg}})/2
\end{align*}
%
Here, $s$ is the uncalibrated score produced by the classifier and $\mathsf{c}$ gives the logistically calibrated score. 
$m$ and $w$ are the two parameters of the logistic family, which determine the point where $\mathsf{c}(s)=0.5$ and the slope at that point, respectively. They can be estimated from the points in the reliability diagram in order to find the best fit. In this case they can be obtained analytically as the mean of the classwise average scores, and the difference between those two means in proportion to the score variance \cite{flach2012machine}.
%(which is assumed to be the same for both classes). 

The fitted logistic curve thus establishes a \textit{calibration map} which transforms uncalibrated scores $s$ into calibrated scores $\mathsf{c}(s)$. 
Even though the calibration map doesn't map to empirical probabilities, plotting it over the reliability diagram allows us to see clearly that if we project each point in the reliability diagram vertically onto the calibration map, and replace its $x$-value with the corresponding $y$-value of the projection, we end up with points on or very close to the diagonal, and hence near-perfectly calibrated scores (Figure~\ref{fig:under-cal}).

\begin{figure}[!t]
    \centering
        \includegraphics[width=0.5\linewidth]{caruana_fig_3.pdf}
    \caption{Graphical illustration of how a well-fitted calibration map leads to near-perfect calibration. From left to right, the dotted arrows show (1) using a point's uncalibrated score $s$ on the $x$-axis as input to the calibration map, (2) mapping the resulting output $\mathsf{c}(s)$ back to the diagonal, and (3) combine with the empirical probability of the point we started from. The closer the original point is to the fitted calibration map, the closer the calibrated point (in red) will be to the diagonal. }
    \label{fig:under-cal}
\end{figure}

The logistic curve is widely used as a `squashing function', compressing values on a possibly unbounded scale into the $[0,1]$ interval. 
Following \citet{platt2000} it is often used as a way to convert scores from a Support Vector Machine into probabilities. 
Technically this isn't calibration as SVM scores are not probabilities but (signed) geometric distances from the decision boundary -- this is also called \textit{scaling} to emphasise the difference \newtext{(hence the popular name `Platt scaling`)}. 
The parametric form of the logistic map can be derived from first principles by assuming that within each class the uncalibrated scores are normally distributed with the same variance. % (Figure~\ref{fig:logistic}). 
\label{page:platt}

% \begin{figure}[!b]
%     \centering
%     \includegraphics[width=0.6\textwidth]{Logistic.pdf}\vfill
%     \caption{Assuming normally distributed scores within each class (left) leads to a logistic calibration map (right).}\label{fig:logistic}
% \end{figure}

The other common form of miscalibration is overconfidence, as exemplified in Figure~\ref{fig:under-over}(b,c). 
% Here, we see that
%
% \begin{quote}
%     The lower points are too far to the left, and the higher points are too far to the right. In other words, the points have a tendency to be too far from the midpoint on the $x$-axis. 
% \end{quote}
% \noindent
An \textit{overconfident} classifier thinks it's {better} at separating classes than it actually is. 
Hence we need to {make predicted probabilities less extreme by pushing them toward the centre}. 
The paper we took this figure from \cite{niculescu-mizil2005} also fitted a logistic curve to this reliability diagram Figure~\ref{fig:under-over}(b), because they were investigating the effect of Platt scaling in a wide range of scenarios. But we see clearly that the fit is rather poor, and using this logistic curve as a calibration map is likely to make matters worse. In this particular case we would be looking for something that can produce an inverse sigmoidal curve. What would be a principled way to achieve this? 

%\begin{figure}[!b]
%    \centering
%    \includegraphics[width=0.9\textwidth]{Beta.pdf}
%    \caption{An example of Beta calibration where overconfident scores (left) lead to an inverse-sigmoidal calibration map (right).}\label{fig:beta}
%\end{figure}

One approach that works well is to model the classwise scores with Beta distributions \cite{pmlr-v54-kull17a,kull2017beyond}.
These assume random variables bounded in $[0,1]$ which is exactly what we need for post-hoc calibration. 
Beta distributions can easily model the skewed distributions resulting from overconfident classifiers, as demonstrated in Figure~\ref{fig:under-over}(b).%Figure~\ref{fig:beta}. 
Mathematically, these curves have three parameters: 
%
    \begin{align*}
        \mathsf{c}(s; a, b, c) &= \frac{1}{1+\exp(-a \ln s + b \ln (1-s) - c)}
        % a &= \alpha_{\textit{pos}}-\alpha_{\textit{neg}}, 
        % b = \beta_{\textit{neg}}-\beta_{\textit{pos}}
    \end{align*}
%
This additional degree of freedom allows Beta calibration to produce both sigmoidal and inverse-sigmoidal calibration maps. 
It can even fit the identity map ($a=b=1$, $c=0$), which means that Beta calibration can recognise that scores are already calibrated. 
In contrast, applying logistic calibration to a calibrated classifier will decalibrate it. 
While Beta calibration can achieve many shapes of calibration maps, it is still a limited parametric family.
Methods to fit richer calibration map families will be discussed in Section~\ref{sec:calibrators}.

%PF: UNTIL HERE (28 JAN 18.00 GMT)

% So far we have seen two calibration techniques: 
% \begin{itemize}
%     \item logistic calibration, which -- although technically a scaling technique, mapping real-valued scores into probabilities -- can adjust for underconfident scores; 
%     \item Beta calibration, which assumes a classifier already scores on a probability scale, and which can adjust for both over- and underconfident scores. 
% \end{itemize}
% We will now take a first look at 
%%% A third calibration technique
%%% % quite different from these two because it 
%%% derives a calibration map from the \textit{ranks} of a set of scores, and hence works for classifiers scoring on arbitrary scales. It is also different from logistic and Beta calibration because it doesn't attempt to model the classwise score distributions, and is hence \textit{non-parametric}. 
%%% %
%%% The technique in question is called \textit{isotonic regression}, belying its origin as an alternative to linear regression which learns a piecewise constant, monotonically increasing or decreasing function. There are several algorithms for isotonic regression, one of which is called \textit{pooled adjacent violators}, which in turn is also used for constructing the convex hull of an ROC curve \cite{zadrozny2001obtaining,fawcett2007}. Figure~\ref{fig:isotonic} demonstrates this graphically. 
%%% 
%%% \begin{figure}[!t]
%%%     \centering
%%%     \begin{subfigure}{0.44\linewidth}
%%%     \includegraphics[width=\linewidth]{ROCCH.pdf}
%%%     \caption{ROC curve and convex hull.}
%%%     \end{subfigure}
%%%     \begin{subfigure}{0.55\linewidth}
%%%     \includegraphics[width=\linewidth]{ROCcal2.pdf}
%%%     \caption{Isotonic calibration map.}
%%%     \end{subfigure}
%%%     \caption{An example of isotonic calibration which derives a piece-wise constant calibration map from the ROC convex hull (Source: \cite{flach2016roc}).}\label{fig:isotonic}
%%% \end{figure}
%%% 
%%% The technique starts from a list of test instances, ranked on their scores; this might give a list of class labels like that depicted at the top of the right figure in Figure~\ref{fig:isotonic}. We then proceed to segment this ranking such that, in each adjacent pair of segments, the right neighbour has a larger proportion of positives than the left neighbour. This defines a unique set of segments, which is depicted on the right of the right figure. Each segment defines an interval on the original classifier scores, as well as an empirical probability of positives in that segment which is taken as the calibrated score for all instances whose score falls in that interval. The calibration map is thus piece-wise constant and increasing. 
%%% 
%%% As a non-parametric method, isotonic regression avoids problems of misspecification which can plague parametric models. For example, a perfectly calibrated classifier has classwise scores which are far from normally distributed, so applying logistic calibration will make matters worse. The downside is that isotonic regression tends to need more labelled data to reliably estimate the segment boundaries and the empirical probabilities within each segment, and is more liable to overfitting if data is not plentiful. 
%%% 

%----------------------------------------------------%
\subsection{Multiclass calibration}
%----------------------------------------------------%

The examples we have seen so far all relate to binary classification. Is it straightforward to generalise calibration concepts and methods to more than two classes? 
The answer to this question is somewhat involved. Some ideas do generalise quite easily: for example, we can model per-class scores by multivariate distributions such as Dirichlet distributions \cite{kull2019}. Some other ideas don't generalise easily at all: for example, a multiclass generalisation of isotonic regression is not straightforward because rankings are inherently bipartite. Such approaches therefore need to be approximated by considering classes in a pairwise or one-versus-rest manner. 

This helps to explain why there is divergence even at a definitional level. 
There are at least three different ways of \emph{defining} what it means to be calibrated in a multiclass setting. 
They are equivalent for binary classification but increasingly stronger for more than two classes,%
\footnote{In rare cases it is possible for a multiclass classifier to be classwise calibrated but not confidence calibrated.
% Example due to Meelis
Here is an example with 40 instances in four groups:
10 instances with predicted probabilities (0.3,0.3,0.4) and actual class distribution (4,2,4);
another 10 with probabilities (0.4,0.3,0.3) and classes (3,4,3);
another 10 with probabilities (0.4,0.6,0.0) and classes (5,5,0);
and the remaining 10 instances with probabilities (0.3,0.6,0.1) and classes (2,7,1).
This classifier is classwise-calibrated but not confidence-calibrated. There are 20 instances with confidence level 0.6 and accuracy 0.6 (5+7=12 out of 20), but the remaining 20 instances have confidence 0.4 and accuracy 0.35 (4+3=7 out of 20). The key idea of this construction is that classwise calibration considers the instances with 0.4 predicted for class 1 as a single group, but confidence calibration looks among them only at those instances for which 0.4 is the highest probability -- e.g., it does consider (0.4,0.3,0.3) but not (0.4,0.6,0.0).}
and can be summarised as follows: 
    \begin{itemize}
        \item {Confidence calibration}: only consider the highest predicted probability. 
        \item {Classwise calibration}: only consider marginal probabilities.
        \item {Multiclass calibration}: consider the entire vector of predicted probabilities.
    \end{itemize}
We will use this terminology throughout the paper to avoid confusion. 

%\renewcommand{\vph}{\hat{\mathbf{p}}}

\textit{Confidence calibration} was proposed by \citet{guo2017}, although not under that name. It requires that among all instances where the probability of \emph{the most likely class} is predicted to be $\alpha$, the expected accuracy is $\alpha$. 
Let $\mathbb{X}$ denote the instance space and $\mathbb{P}_{\mathbb{Y}}$ the probability $K$-simplex, then a probabilistic classifier $\mathsf{f}:\mathbb{X}\rightarrow\mathbb{P}_{\mathbb{Y}}$ is \emph{confidence-calibrated}, if for any confidence level $\alpha\in[0,1]$, 
the actual proportion of the predicted class, among all possible instances $\mathbf{x}$ being predicted this class with confidence $\alpha$, is equal to $\alpha$:  
\begin{align*} 
\mathsf{P}(Y=\hat{Y} \: | \: S_{\hat{Y}}=\alpha)=\alpha\qquad\text{where }\ \hat{Y}=\argmax_j S_j.
%P\Big(Y=\argmax\big(\vph(X)\big) \: \Big| \: \max\big(\vph(X)\big)=c\Big)=c.
\end{align*}
Here, $S_j$ denotes the $j$-th dimension of $\mathsf{f}(\mathbf{X})$.

\textit{Classwise calibration}, proposed by \citet{zadrozny2002}, requires that all \emph{one-vs-rest} probability estimators obtained from the original multiclass model are calibrated. 
Formally, a probabilistic classifier $\mathsf{f}:\mathbb{X}\rightarrow\mathbb{P}_{\mathbb{Y}}$ is \emph{classwise-calibrated}, if for any class $i \in \{1, \dots, K\}$ and any predicted probability value $s \in [0, 1]$ for this class, 
the actual proportion of class $i$, among all possible instances on the random variable $\mathbf{X}$ getting the same prediction on class i, is equal to $s$:  
\begin{align*} 
\mathsf{P}(Y=i\mid S_i=s)=s
\end{align*}

\textit{Multiclass calibration}, also called \textit{calibration in the strong sense} \cite{widmann2019calibration}, is the {strongest form of calibration} for more than two classes, subsuming the previous two definitions. 
A probabilistic classifier $\mathsf{f}:\mathbb{X}\rightarrow\mathbb{P}_{\mathbb{Y}}$ is \emph{multiclass-calibrated} if for any prediction vector $\mathbf{s}=[s_1,\dots,s_K]\in\mathbb{P}_{\mathbb{Y}}$, the proportions of classes among all possible instances on the random variable $\mathbf{X}$ getting the same prediction $\mathsf{f}(\mathbf{X})=\mathbf{s}$ are equal to the prediction vector $\mathbf{s}$:  
\begin{align*} %\label{eq:calib}
\mathsf{P}(Y=i\mid \mathsf{f}(\mathbf{X})=\mathbf{s})=s_i\qquad\text{for }\ i=1,\dots,K.
\end{align*}
%
%Here $\mathbf{s}=[s_1, \dots, s_K]$ denotes the $K$-dimensional probability vector instance.

For practical purposes, the conditions in these definitions need to be relaxed. This is where {binning} comes in. 
Once we define the bins, we can draw a {reliability diagram} as in the two-class case. For classwise calibration, we can show per-class reliability diagrams or a single averaged one. 
One way to assess the degree of calibration is by means of the {gaps} in the reliability diagram. 
These topics will be explored in Section \ref{sec:metrics}. 
We will first take a closer look at the important concept of \emph{proper scoring rules} in the next section. Proper scoring rules are instance-wise evaluation measures for probability estimates that avoid the need for score binning. As a result they cannot measure the degree of calibration directly, but through decomposition results, we will show how the scores can be decomposed into various components, including the calibration loss. 

}


==> mlj_files/compiled/03_evaluation.tex <==
\section{From proper scoring rules to calibration}
\label{sec:psr}




%----------------------------------------------------%
% \subsection{Proper scoring rules}
% \label{sec:met:psr}
%----------------------------------------------------%

% {\color{red}(TODO: Mention this \cite{savage1971}.)}
    
As early as 1950 researchers were interested in scoring functions that would evaluate probabilistic forecasts without influencing the forecaster into making undesirable predictions \cite{brier1950}, thus keeping the forecaster ``honest'' while encouraging useful forecasts. In the late 1960s the term \emph{proper scoring rule} was already in use for score functions whose computation was based on a forecaster's probabilities and the actual occurrence or not of the corresponding events \cite{winkler1969scoring}. Informally, a scoring rule is said to be proper if optimal values are obtained by the forecaster predicting the true probabilities of the events. %At the same time, proper scoring rules were shown to be useful not only to evaluate predicted probabilities but also to help in training better forecasters \cite{winkler1969scoring}.
% In addition to machine learning evaluation and to the seminal works in meteorology, 
Proper scoring rules and their ability to induce useful and accurate forecasts also lend themselves to game-theoretic interpretations, as discussed in the seminal work of \citet{savage1971}.

Before diving into details, let us introduce the notation. In a multiclass classification task with $K$ classes, let the true class of an instance be a vector $\dot{\mathbf{y}}=[y_1,\ldots,y_K]$, where $y_j = 1$ when the true class is $j$, otherwise $y_j = 0$. Additionally, let $\mathbf{s}=[s_1,\ldots,s_K]$ be a class probability vector obtained from a classification model for an instance, i.e. $s_j \geq 0$, $j=1,\ldots,K$ and $\sum^K_{j=1} s_j = 1$. A scoring rule $\phi(\mathbf{s}, \dot{\mathbf{y}})$ is a non-negative measure of how well the estimated probability vector $\mathbf{s}$ matches the true class vector $\mathbf{\dot{y}}$. We assume that lower values of $\phi(\mathbf{s}, \dot{\mathbf{y}})$ are better.% 
\footnote{Some authors \cite{winkler1969scoring,gneiting2007} use scoring rules in the opposite way, i.e. higher is better, sometimes calling them utility or payoff functions, in the sense that a forecaster is rewarded for giving better predictions. If a scoring rule was proposed as a payoff function, we can typically negate its values such that lower values are better.} 

Popular scoring rules include Brier score $\phi_{\text{BS}}$ and log-loss $\phi_{\text{LL}}$, which are defined as follows:
%
\begin{equation}
    \label{eq:evaluation:brier}
    \phi_{\text{BS}}(\mathbf{s}, \mathbf{\dot{y}})  = \sum_{j=1}^{K} (s_j - y_j)^2.
\end{equation}

  \begin{equation}
    \label{eq:evaluation:logloss}
    \phi_{\text{LL}}(\mathbf{s}, \mathbf{\dot{y}}) = - \sum_{j=1}^{K} y_j \log s_j.
\end{equation}
%
Our Brier score definition ranges between $0$ and $2$, agreeing with Brier's original definition \cite{brier1950}, although it is now common for half this quantity to be called Brier score. While scoring rules evaluate the loss incurred by the class probability estimates for a single instance, we are usually interested in evaluating the performance of a model on test data. Thus, given a test dataset, we can calculate the empirical loss as the average instance-wise loss across the data. % Going back to our example from Table \ref{tab:evaluation:toy}, we have 



% \begin{align*}
%     \bar{\phi}_{\text{BS}} &= \frac{1}{30}\sum_{i=1}^{30} \sum_{j=1}^{3} (p_{ij} - y_{ij})^2, \\ &= \frac{1}{30}\left[(1 -1)^2 + (0 - 0)^2 + (0 - 0)^2 + \ldots  + (0.3 - 0)^2 + (0.7 - 1)^2\right], \\ &= XXX,
% \end{align*}

% \noindent and

% \begin{align*}
%     \bar{\phi}_{\text{LL}} &= -\frac{1}{30}\sum_{i=1}^{30} \sum_{j=1}^{3} y_{ij} \log p_{ij}, \\ &= -\frac{1}{30}\left(1\log 1 + 0\log 0 + 0\log 0 + \ldots + 0\log 0 + 0\log 0.3 + 1\log 0.7\right), \\ &= XXX.
% \end{align*}

Suppose the class labels $\mathbf{\dot{y}}$ are drawn from the true distribution $\mathbf{q}$ over classes. A scoring rule $\phi$ is proper if its expected value on probability vector $\mathbf{s}$ and $\mathbf{\dot{y}}$ is higher than (i.e., worse) or the same as its expected value on $\mathbf{q}$ and $\mathbf{\dot{y}}$, that is if

% In this section we cover loss measures ($\breve{\phi}$) that prefer Bayes-optimal classifiers over other classifiers, i.e. for any given $P(\mathbf{X}, Y)$, $\mathbf{x} \in \mathcal{X}$, the following is satisfied:

\begin{align*}
\mathsf{E}_{\mathbf{\dot{y}} \sim \mathbf{q}} \Big[ \phi\big(\mathbf{s}, \mathbf{\dot{y}}\big)  \Big] \geq \mathsf{E}_{\mathbf{\dot{y}} \sim \mathbf{q}} \Big[ \phi\big(\mathbf{q}, \mathbf{\dot{y}}\big)  \Big], 
\end{align*}
and it is strictly proper if and only if both sides of the expression being equal implies $\mathbf{s} = \mathbf{q}$. % and $P(Y \mid \mathbf{X}=\mathbf{x})$ is a vector with elements $P(Y=j \mid \mathbf{X}=\mathbf{x})$.
Both Brier score and log-loss are strictly proper scoring rules.
     
%  Proper scoring rules are calculated as expectations over probability distributions, while ECE measures are averages across bins. If proper scoring rules are approximated empirically, they can be interpreted as putting each item in its separate bin, which would look like the example in Figure \ref{fig:rel4}, then computing the average of some loss for each predicted probability and its corresponding observed label. Instead of the absolute difference, as in ECE, this loss can be the quadratic error or the Kullback–Leibler divergence, which have better mathematical properties. The best-known proper scoring rules include Brier score and log-loss, which are given by Equations (\ref{eq:evaluation:brier}) and (\ref{eq:evaluation:logloss}), respectively, where $\mathbb{I}(\cdot)$ is an indicator function, such that $\mathbb{I}(y_n=j) = 1$, if $y_n=j$, otherwise $\mathbb{I}(y_n=j) = 0$.
    
    % \begin{figure}
    %     \centering
    %     \includegraphics[width=0.7\textwidth]{figures/evaluation/Forecaster4.png}
    %     \caption{Binary reliability diagram with one bin per instance.}
    %     \label{fig:eval:forecaster4}
    % \end{figure}
    


    % \begin{equation}
    %     \label{eq:evaluation:brier}
    %     \breve{\phi}_{\text{BS}}\Big(\mathbf{Q}, \mathbf{y}\Big)  = \frac{1}{N}\sum_{n=1}^{N}\sum_{j=1}^{K} \Big(\mathbb{I}(y_n=j) - q_{n,j} \Big)^2.
    % \end{equation}
    
    %   \begin{equation}
    %     \label{eq:evaluation:logloss}
    %     \breve{\phi}_{\text{LL}}\Big(\mathbf{Q}, \mathbf{y}\Big) = -\frac{1}{N}\sum_{n=1}^{N} \sum_{j=1}^{K} \mathbb{I}(y_n=j) \cdot \text{log} (q_{n,j}).
    % \end{equation}
    
% TSF proposed text
%    Among proper scoring rules, log-loss in particular is frequently used as the training loss of machine learning methods such as neural networks, often under the name of cross-entropy. At the instance level, log-loss only depends on the predicted class probability for the true class (as all other classes $y_j$ are zero) and it might not be obvious why it is a proper scoring function. However, properness is defined as an expectation over a population. For instance, suppose that, for a population of instances, the true probability is $[0.8, 0.2, 0.0]$. In this case, the expected log-loss will be $-(0.8 \log(s_1) + 0.2 \log(s_2))$, which can only be minimised by predicting the probability vector $[0.8, 0.2, 0.0]$, satisfying the properness condition.
    
% MPN merged TSF and MK and PF feedback
Among proper scoring rules, log-loss in particular is frequently used as the training loss of machine learning methods such as neural networks, often under the name of cross-entropy. \newtext{It is also the loss function used by most of the calibration methods discussed in Section \ref{sec:calibrators}, including Platt scaling, temperature scaling and its variations (vector and matrix), beta calibration and Dirichlet calibration. A notable exception is isotonic calibration, which optimised Brier score.}

At the instance level, log-loss only depends on the predicted class probability for the true class (as all other classes $y_j$ are zero) and it might not be obvious why it is a proper scoring function.
For example, one could argue that it does not matter whether the model predicts $[0.8, 0.2, 0.0]$ or $[0.8, 0.1, 0.1]$ on an instance of class $1$, as log-loss would be $-\ln(0.8)$ in both cases.
However, one needs to keep in mind that properness is defined as an expectation over a population. 
For instance, suppose that, for a population of instances, the true probability is $[0.8, 0.2, 0.0]$.
In this case, the expected log-loss will be $-(0.8 \log(s_1) + 0.2 \log(s_2))$, which can only be minimised by predicting the probability vector $[0.8, 0.2, 0.0]$, satisfying the properness condition.
Note that log-loss can be dominated by cases where the true class is predicted with low probability: in the extreme case of a single instance with zero probability for the true class the loss is infinite. 

    %, as it only penalises the probability given to the true class, which can be useful if one is only interested in maximising the probability given to the true class of an instance.
   %Log-loss only depends on the predicted class probability for the true class (as all other $y_j$ are zero) and it might not be obvious why it is a proper scoring function. %, i.e. why this loss has a unique minimum achieved by the Bayes-optimal model. 
   %For example, one could argue that it does not matter whether the model would predict $[0.7,0.1,0.1,0.1]$ or $[0.7,0.3,0.0,0.0]$ on an instance of class $1$, as log-loss would be $-\ln(0.7)$ in both cases. However, one needs to keep in mind that at the time of making the prediction the model does not know the true class of the instance and has no way of knowing which of the values in the predicted probability vector will be `probed' by the loss and will thus eventually matter. Therefore, the model should only predict $[0.7,0.3,0.0,0.0]$ when it is absolutely sure that the instance cannot belong to classes 3 and 4, because otherwise the evaluation on test set might catch it with an infinite loss of $-\ln(0)$ with a predicted probability $0$ for the true class $3$ or $4$.

    % We can easily see that Brier score and log-loss are not minimised by constantly predicting the class distribution, as in ECE. In fact, if a classifier predicts $0.5$ positive probability for two different instances, one positive and another negative, Equations (\ref{eq:evaluation:brier}) and (\ref{eq:evaluation:logloss}) result in $\breve{\phi}_{\text{BS}}\Big(\mathbf{Q}, \mathbf{y}\Big) = 0.5$ and $\breve{\phi}_{\text{LL}}\Big(\mathbf{Q}, \mathbf{y}\Big) = 0.6931$, respectively.
        
    
  
    
    


\subsection{Decompositions of proper scoring rules}\label{sec:decomp}

When proposing the forecast evaluation that would later be known as Brier score, Brier mentioned that it could not be ``gamed'', i.e. in order to obtain low scores, the forecaster has to produce honest, useful and correct predictions. Later research focused on why this was true for Brier score and other proper scoring rules.

\citet{sanders1963} showed that Brier score corresponds to the sum of two aspects of probability evaluation: validity and sharpness, terms introduced by \citet{miller1962statistical} and \citet{bross1953design}, respectively. Validity, later known as reliability \cite{murphy1977reliability}, is now often called \emph{calibration loss} \cite{kull2015novel}. It refers to the fit between the forecasts and the frequency of occurrence of the event, which means that it is a joint property of the predictions and the events. Sharpness, which is now commonly called \emph{refinement loss} and was also known as resolution \cite{murphy1977reliability}, is the loss due to predicting the same probability for instances from different classes.
% and is a property of predicted probabilities only. 
\citet{degroot1983} %comparison}
showed that these two terms make up proper scoring rules in general, and that probabilistic predictions should minimise refinement loss subject to calibration.

We now formally introduce such proper scoring rule decompositions. Let $\mathbf{X}$ and $\mathbf{\dot{Y}}=[Y_1,\ldots,Y_K]$ be multivariate random variables, respectively corresponding to the features and the class of a randomly picked instance, where $Y_j=1$ if the instance is of class $j$, otherwise $Y_j= 0$, for $j=1,2,\ldots,k$. Given a scoring classifier, class probability estimator or probability forecaster $\mathsf{f}$, we denote by $\mathbf{S}=[S_1,S_2,...,S_k]=\mathsf{f}(\mathbf{X})$ the vector output of $\mathsf{f}$ for random feature $\mathbf{X}$, where $\mathbf{S}$ is a random vector due to its dependence on $\mathbf{X}$. The expected value of proper scoring rule $\phi$ with respect to $\mathbf{S}$ and $\mathbf{\dot{Y}}$ is then $\mathsf{E} \Big[ \phi\big(\mathbf{S}, \mathbf{\dot{Y}}\big)  \Big]$.

\begin{table}[h]
\centering
\begin{tabular}{cccccc}
\hline
\textbf{$i$} & \textbf{$X^{(i)}$} & \textbf{$Y^{(i)}$} & $Q^{(i)}$         & $S^{(i)}$       & $C^{(i)}$          \\ \hline
$1$          & $(3,1,3)$          & $(1,0,0)$          & $(0.75,0.25,0.0)$ & $(0.9,0.1,0.0)$ & $(0.75,0.25,0.0)$  \\
$2$          & $(3,1,3)$          & $(1,0,0)$          & $(0.75,0.25,0.0)$ & $(0.9,0.1,0.0)$ & $(0.75,0.25,0.0)$  \\
$3$          & $(3,1,3)$          & $(1,0,0)$          & $(0.75,0.25,0.0)$ & $(0.9,0.1,0.0)$ & $(0.75,0.25,0.0)$  \\
$4$          & $(3,1,3)$          & $(0,1,0)$          & $(0.75,0.25,0.0)$ & $(0.9,0.1,0.0)$ & $(0.75,0.25,0.0)$  \\
$5$          & $(2,2,2)$          & $(1,0,0)$          & $(0.50,0.50,0.0)$ & $(0.6,0.2,0.2)$ & $(0.17,0.50,0.33)$ \\
$6$          & $(2,2,2)$          & $(0,1,0)$          & $(0.50,0.50,0.0)$ & $(0.6,0.2,0.2)$ & $(0.17,0.50,0.33)$ \\
$7$          & $(0,2,2)$          & $(0,1,0)$          & $(0.0,0.50,0.50)$ & $(0.6,0.2,0.2)$ & $(0.17,0.50,0.33)$ \\
$8$          & $(0,2,2)$          & $(0,1,0)$          & $(0.0,0.50,0.50)$ & $(0.6,0.2,0.2)$ & $(0.17,0.50,0.33)$ \\
$9$          & $(0,2,2)$          & $(0,0,1)$          & $(0.0,0.50,0.50)$ & $(0.6,0.2,0.2)$ & $(0.17,0.50,0.33)$ \\
$10$         & $(0,2,2)$          & $(0,0,1)$          & $(0.0,0.50,0.50)$ & $(0.6,0.2,0.2)$ & $(0.17,0.50,0.33)$ \\ \hline
\end{tabular}
        \caption{Example dataset with three classes and three features. Column $Q^{(i)}$ shows class posteriors given by the optimal model with $Q_1 = 0.25X_1$, $Q_2 = 0.25X_2$ and $Q_3 = 1 - (Q_1 + Q_2)$. Column $S^{(i)}$ corresponds to estimated class posteriors $S=f(X)$, which are given by $S_1 = 0.3X_3$, $S_2 = 0.1X_2$ and $S_3 = 1 - (S_1 + S_2)$. Finally, column $C$ represents calibrated probabilities.
        %calculated with $X|Y_1 \sim \mathcal{N}(4.375,1)$, $X|Y_2 \sim \mathcal{N}(1.875,2)$ and $X|Y_3 \sim \mathcal{N}(0,1)$. The class posteriors $S=f(X)$ are estimated by a trained model $f$ with $X|Y_1 \sim \mathcal{N}(4.5,1)$, $X|Y_2 \sim \mathcal{N}(3,1)$ and $X|Y_3 \sim \mathcal{N}(0.5,1)$. For the optimal model, the class priors are $\pi_1 = 4/10$,  $\pi_2 = 4/10$ and  $\pi_3 = 2/10$, while for model $f$, $\pi_1 = \pi_2 = \pi_3 = 1/3$, i.e. the classes are considered equally probable. Column $C$ represents calibrated probabilities.
        }
        \label{tab:evaluation:toy:psr}
\end{table}

Consider a classification test set of $10$ instances belonging to three classes ($K=3$) and described by $3$ features, as shown in column $\mathbf{X}^{(i)}$ of Table \ref{tab:evaluation:toy:psr}. Suppose instances  $1$, $2$, $3$ and $5$ belong to class $1$, i.e. $Y_1=1$, instances $4$, $6$, $7$, $8$ belong to class $2$ and the rest belong to class $3$. Note that in this example, the optimal class posteriors $\mathbf{Q}^{(i)}$ are given, however this is not generally the case. Additionally, the sample is representative by design, with average $\mathbf{Y}^{(i)}$, among instances with the same feature values, exactly agreeing with $\mathbf{Q}^{(i)}$. Given columns $\mathbf{S}^{(i)}$ and $\mathbf{Y}^{(i)}$ from Table \ref{tab:evaluation:toy:psr}, and using Equations (\ref{eq:evaluation:brier}) and (\ref{eq:evaluation:logloss}), by averaging over the 10 instances, we get a mean Brier score of $0.71$ and mean log-loss of $1.12$.

% \begin{align*}
%     \bar{\phi}_{\text{BS}} &= \frac{1}{10}\sum_{i=1}^{10} \sum_{j=1}^{3} (p_{ij} - y_{ij})^2, \\ &= \frac{1}{10}\left[(1 -0.9)^2 + (0 - 0.1)^2 + (0 - 0)^2 + \ldots  + (0.3 - 0)^2 + (0.7 - 1)^2\right], \\ &= XXX,
% \end{align*}

% \noindent and

% \begin{align*}
%     \bar{\phi}_{\text{LL}} &= -\frac{1}{10}\sum_{i=1}^{10} \sum_{j=1}^{3} y_{ij} \log p_{ij}, \\ &= -\frac{1}{30}\left(1\log 1 + 0\log 0 + 0\log 0 + \ldots + 0\log 0 + 0\log 0.3 + 1\log 0.7\right), \\ &= XXX.
% \end{align*}


% \todo[inline]{Meelis Kull: I think it is better to first state that suppose Q is given. Because then C can be calculated from it. Otherwise it is not clear how the expectation of E[Y|S] has been obtained. Note that by a lucky chance (well,.. by our design) the average Y exactly agrees with Q, i.e. Y are a representative sample.  This makes average[Y|S]=average[Q|S], which does not have to be the case in general. So somehow we need to be a bit careful to distinguish what is a coincidence here and what is exactly equal always. One possibility is to make the data generating process to pick lines from this table uniformly randomly, but not sure it is the best way to explain.}
Now let $\mathbf{C}=[C_1,C_2,\ldots,C_K]$ be yet another random vector, where $C_j=\mathsf{E}[Y_j| \mathbf{S}]$, i.e. $C_j$ represents the actual proportion of class $j$ given all instances which received the same estimate $\mathbf{S}$ from model $\mathsf{f}$. The decomposition of proper scoring rule $\phi$ into calibration loss and refinement loss is then the sum of expected loss between $\mathbf{S}$ and $\mathbf{C}$ and expected loss between $\mathbf{C}$ and $\mathbf{Y}$ \cite{brocker2007,kull2015novel}:
\begin{align*}
    \mathsf{E} \Big[ \mathsf{d}\big(\mathbf{S}, \mathbf{\dot{Y}}\big)  \Big] = \mathsf{E} \Big[ \mathsf{d}\big(\mathbf{S}, \mathbf{C}\big)\Big] + \mathsf{E} \Big[ \mathsf{d}\big(\mathbf{C}, \mathbf{\dot{Y}}\big)  \Big],
\end{align*}

\noindent where $\mathsf{d}: \mathbb{P}_{\mathbb{Y}} \times \mathbb{P}_{\mathbb{Y}} \rightarrow \mathbb{R}$ is the divergence associated to proper scoring rule $\phi$. For log-loss and Brier score, $\mathsf{d}$ has been shown to correspond to the Kullback-Leibler divergence and the mean squared difference, respectively \cite{kull2015novel}.

The definition above is given based on expected population loss. In practice, we would be calculating these quantities on test data, as we generally do not have access to the whole population. Thus, we actually calculate an empirical loss. But assuming that test data is representative of the whole population and that there is a uniform distribution over the test instances and zero probability elsewhere, empirical loss can be interpreted as a special case of expected loss and all decompositions derived for expected loss also apply to empirical loss \cite{kull2015novel}. 

In our example in Table \ref{tab:evaluation:toy:psr}, the first four instances share the same model scores $\mathbf{S}=[0.9,0.1,0.0]$, with the first three instances belonging to class $1$ and the fourth to class $2$. Thus, for these instances, $\mathbf{C}=[0.75,0.25,0.0]$. The other six instances also share a score vector, with $1$ instance from class $1$, three from class $2$ and 2 instances from class $3$. As a result, they share the same calibrated probabilities $\mathbf{C}=[1/6, 3/6, 2/6]$. Given these values and considering Brier score, calibration loss is $0.19$ and refinement loss is $0.52$, which sum up to the Brier score of $0.71$, as expected. For log-loss the decomposition is $1.12 = 0.29 + 0.83$.

% {\color{red}(TODO: Calculate using toy example.)}

It is easy to see that a function that maps $\mathbf{S}$ to $\mathbf{C}$, known as a calibrator in Section \ref{sec:calibrators}, could potentially reduce calibration loss to $0$, consequently decreasing proper scoring rule loss. Refinement loss, on the other hand, is only zero if there are no ties between instances of different classes, i.e. they do not share the same value for $\mathbf{S}$. If that is the case, it is possible to map $\mathbf{S}$ to $\mathbf{C}$ such that it is perfectly confident and correct, i.e. $C_j = Y_j$.

Now suppose we knew the optimal model that outputs the true posterior class probabilities $\mathbf{Q}=[Q_1,Q_2,\ldots,Q_K]$, where $Q_j=\mathsf{E}[Y_j|\mathbf{X}]$, i.e. $Q_j$ is the true proportion of class $j$ among instances with feature values $\mathbf{X}$. Then the expected loss according to proper scoring rule $\phi$ can be decomposed into the sum of expected divergences between $\mathbf{S}$ and $\mathbf{Q}$ and $\mathbf{Q}$ and $\mathbf{Y}$:

\begin{align*}
    \mathsf{E} \Big[ \mathsf{d}\big(\mathbf{S}, \mathbf{\dot{Y}}\big)  \Big] = \mathsf{E} \Big[ \mathsf{d}\big(\mathbf{S}, \mathbf{Q}\big)\Big] + \mathsf{E} \Big[ \mathsf{d}\big(\mathbf{Q}, \mathbf{\dot{Y}}\big)  \Big],
\end{align*}
The first term in the sum is called epistemic loss \cite{senge2014reliable} and is the loss due to our model $\mathsf{f}(\mathbf{X})$ not being optimal. The second term is called irreducible or aleatoric loss \cite{senge2014reliable} and is the loss of the optimal model. Going back to the example in Table \ref{tab:evaluation:toy:psr}, for Brier score, epistemic loss is $0.26$ and irreducible loss is $0.45$. For log-loss the decomposition is $1.12 = 0.48 + 0.64$. The irreducible loss is only zero if the attributes of every instance $\mathbf{X}$ carry enough information to uniquely define the label $\mathbf{\dot{Y}}$. It is thus not possible to come up with a procedure to reduce the overall loss based on it. Additionally it would be unrealistic to do so based on epistemic loss. We are then naturally drawn to calibration loss as it is simple to interpret (we want our predicted probabilities of occurrence of an event to match the actual frequencies of occurrence) and also because we can easily estimate it with enough data. Thus, as discussed in the following section, visualisation and estimation of miscalibration have received considerable attention in the literature of probability evaluation and machine learning.


% {\color{red}(TODO: Connect to reliability diagrams (depends on the section's position).)}


% {\color{red}(TODO: Epistemic-irreducible.)}
%Other decompositions and why they're important


%  Let us once again return to our example from Table \ref{tab:evaluation:toy}. As mentioned before, a model that always outputs the class proportion will have a perfect ECE of 0, and that is what happens if we take class 1 as the positive class and constantly predict class probabilities equal to the class proportions. But while this gives $\text{binary-ECE}=0$ for class 1, the resulting log-loss is $0.6365$.
% % 
%  On the other hand, a different model which always outputs $0.9$ probability to the instances' true classes gets the reliability diagram shown in Figure \ref{fig:eval:reliability0.9}, with $\text{binary-ECE}=0.1$ for class 1, and $0.1054$ log-loss.
% %
% From the first to the second model, ECE increases (0 to 0.1), but log-loss decreases (0.6365 to 0.1054). This happens because proper scoring rules do not measure only calibration. In fact, they can be decomposed into terms with distinct interpretations \cite{kull2015}. 




%     \begin{figure}
%         \centering
%         \includegraphics[width=0.7\textwidth]{figures/evaluation/reliability-0.9-v2.pdf}
%         \caption{Binary reliability diagram of a model that always outputs $0.9$ probability for the true class of the instances in Table \ref{tab:evaluation:toy}.}
%         \label{fig:eval:reliability0.9}
%     \end{figure}



% An intuitive way to decompose proper scoring rules is into refinement (RL) and calibration losses (CL): $\mathsf{E}\left[\breve{\phi}\right] = \text{RL} + \text{CL}$. Refinement loss is the loss due to producing the same probability for instances from different classes (the second model reduces this loss), while calibration loss is the loss due to the difference between
% the probabilities predicted by the model and the observed class proportions among instances with the same output (the second model increases this loss).

% Since we don't usually know the real score distribution, we would need to once again rely on binning if we wanted to actually estimate refinement and calibration losses. Additionally, the terms are calculated (estimated) differently, depending on the proper scoring rule. Finally, the loss of the optimal classifier is not necessarily 0. This is due to irreducible loss, which is only 0 if the attributes provide enough information to uniquely determine the instances' right label Y, with probability 1 \cite{kull2015}.


%\subsection{Calibration metrics}
%    \subsubsection{First attempts to evaluate calibration}
%    \subsubsection{Binary}
%    \subsubsection{ECE}


\newpage

\section{Evaluation and visualisation of classifier calibration}
\label{sec:metrics}

In this section we present a range of approaches to evaluate and visualise calibration, and discuss the advantages and disadvantages of each.
In Section \ref{sec:met:1st} we explore the first steps towards measuring miscalibration, starting from the early work on weather forecast calibration, and discuss various approaches to visually inspect miscalibration.
Some of those early approaches have been later adapted and proposed as new calibration metrics which are discussed in the following sections.
We start with binary calibration in Section \ref{sec:met:bin} which will serve as a building block for the two multiclass calibration measures discussed in Sections \ref{sec:met:clw:ece} and \ref{sec:met:con:ece}.
% We finish this section discussing hypothesis tests for calibration in Section \ref{sec:met:hyp}.



%----------------------------------------------------%
%\subsection{First attempts to evaluate calibration}
\subsection{Visualising calibration}
\label{sec:met:1st}
%----------------------------------------------------%

% Calibration metrics and proper scoring rules can provide evidence of the quality of a model's calibration.
Several visualisation techniques have been proposed for easier inspection of the reliability of predictions at different score ranges.
In this section we summarise a range of approaches that have been proposed in the literature, from simple tabular inspection to the more recent reliability diagrams (see \citet{brocker2007} for an extended discussion of reliability diagrams).

Starting from the binary case, the basic idea has been to show the relation between a particular predicted score $\hat{s} \in [0, 1]$ for the positive class of a probabilistic classifier and the respective observed proportion of positives, which we denote by $\mathsf{\bar{y}}(\hat{s})$.
In order to compute a observed proportion of positives we require multiple samples with the same score $\hat{s}$. However, given that the scores are continuous variables, the probability of getting multiple samples with the same score is almost zero.
For that reason, the score space is commonly discretised into $M$ bins $\{\mathbb{B}_1, \dots, \mathbb{B}_M\}$, thus increasing the probability of having multiple samples per estimation range (perhaps by forcing each bin to have a minimum number of samples).
Then, we can obtain $M$ observed proportions of positives $\mathsf{\bar{y}}(\mathbb{B}_m)$ instead of one per score value $\hat{s}$.
% If we have an indicator variable for every bin with the indices of the scores that fall into it $\mathbb{I}_m \in \{i; \hat{s}_i \in \mathbb{B}_m\}$ we can compute the \emph{observed proportion of positives} in each bin as
% %
% \begin{equation}
%     \mathsf{\bar{y}}(\mathbb{B}_m) = \frac{\sum_{i \in \mathbb{I}_m} y_i}{\text{count}(\mathbb{I}_m)}.
% \end{equation}
% %
% Some of the first uses of \emph{observed proportion of positives} appeared in the context of weather forecast evaluation in the form of tabular data \cite{hallenbeck1920, brier1950}.
%\citet{hallenbeck1920} showed ten equally distributed bin boundaries with their respective number of forecasts, number of rains and percentage (See Figure \ref{tab:eval:hallenbeck1920:1}). 
See Table \ref{tab:eval:hallenbeck1920} for an early use of observed proportions of positives using equal-width bins of predicted probabilities. 

\begin{figure}
    % \begin{subfigure}{0.48\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{figures/evaluation/hallenbeck1920_tab1}
    %     \caption{Hallenbeck 1920}
    %     \label{tab:eval:hallenbeck1920:1}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}{0.48\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{figures/evaluation/brier1950_tab2}
    %     \caption{Brier 1950}
    %     \label{tab:eval:brier1950:2}
    % \end{subfigure}
    
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{sanders1963_fig1}
        \caption{\citep[Fig.~1]{sanders1963}}
        \label{fig:eval:sanders1963:1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{lichtenstein1976_fig6.jpg}
        \caption{\citep[Fig.~2]{lichtenstein1977calibration}}
        \label{fig:eval:lichtenstein1977:6}
    \end{subfigure}
    
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{brocker_2007_fig1}
        \caption{\citep[Fig.~1]{brocker2007}}
        \label{fig:eval:brocker2007:1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{brocker_2007_fig4}
        \caption{\citep[Fig.~4]{brocker2007}}
        \label{fig:eval:brocker2007:4}
    \end{subfigure}
    \caption{Different graphical representations of calibration-related information found in the literature.}
    \label{fig:eval:rd}
\end{figure}
    
Later work showed line plots instead of tabular data, with markers at the centre of each bin~\cite{sanders1963, lichtenstein1977calibration, lichtenstein1982, murphy1977reliability}; occasionally including the number of samples in each bin next to the markers (See Figure \ref{fig:eval:sanders1963:1}). Other authors showed the markers with size relative to the sample size~\cite{hagedorn2005}, or as a separate histogram next to the reliability diagram~\cite{niculescu-mizil2005}.
Line plots facilitate visual inspection of the discrepancy of the observed proportions of positives against a perfectly calibrated model, which corresponds to the diagonal.
However, positioning the markers at the centre of the bins can be misleading, as even perfectly calibrated scores may result in a \emph{visually} non-calibrated reliability diagram with a deviation of up to half the bin width from the diagonal~\cite{brocker2007} (See Figure \ref{fig:mean:vs:centre} for an example).
This may happen in cases in which the scores are not evenly distributed in each bin.
%
\begin{figure}
    \centering
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=1.0\linewidth]{rd_mean_score_vs_bin_centre_not_calibrated.pdf}
        \caption{Not calibrated example. $4$ samples with score $0$ from which $25\%$ are positive, and $4$ samples with score $1$ from which $75\%$ are positive.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=1.0\linewidth]{rd_mean_score_vs_bin_centre_calibrated.pdf}
        \caption{Calibrated example. $1$ sample with score $0$ from negative class, and $1$ sample with score $1$ from positive class.}
    \end{subfigure}
    \caption{
Simple example showing the maximum discrepancy in calibration error when using the centre of the bin for the marker instead of the average score of the bin. Both examples show only two bins $[0, 0.5)$ and $[0.5, 1]$.
\textbf{(a)} shows a model not calibrated, but using the centre of the bin (green dashed line) visually seems calibrated. The gap between the centre of the bin and the average score is maximum, which corresponds to half of the bin size with respect to the average score (red line).
\textbf{(b)} shows a calibrated model which seems uncalibrated if using the centre of the bin. The gap is again half of the bin size.
}
    \label{fig:mean:vs:centre}
\end{figure}
%
In order to alleviate this problem, later work centred the markers on the average predicted scores $\mathsf{\bar{s}}(\mathbb{B}_m)$ in each bin instead. % where
% %
% \begin{equation}
%     \mathsf{\bar{s}}(\mathbb{B}_m) = \frac{\sum_{i \in \mathbb{I}_m}\hat{s_i}}{\text{count}(\mathbb{I}_m)}.
% \end{equation}
% %

There are two main methods to group the predicted scores into bins to build reliability diagrams. The first one, commonly called \emph{width binning}, distributes scores into a number of  bins of the same width, choosing bin edges accordingly (e.g., 10 bins $[0, 0.1], (0.1, 0.2], \ldots, $ $(0.9, 1.0]$). Another method, called \emph{frequency binning} (also equal size or equal mass binning) groups the scores by keeping the same number of samples in each bin. Frequency binning can and will normally result in bins with different widths, but it ensures that all bins have the same ``weight'' when assessing the model's miscalibration.

Bin estimations have varying reliability, e.g., depending on the number of samples in the bin. 
One way to show this visually is by incorporating confidence intervals.
%If previous work showed the counts in text form (eg. in a table or next to the markers \cite{brier1950, sanders1963, murphy1977reliability}), later work also incorporated in the visualisation confidence intervals in the reliability diagram.
One of the simplest methods is to assume that each bin is sampled from a binomial distribution, and compute the corresponding confidence intervals of the observed proportion of positives (see Figure~\ref{fig:eval:pycalib:lines}).
However, making the assumption of fixed bins, score averages and proportion of positives is unrealistic; unless the score distribution is uniform (see \cite{brocker2007} for a detailed discussion).
More accurate intervals can be obtained by using the \emph{consistency resampling} method proposed by \citet{brocker2007}, which consists on sampling the scores with replacement several times in order to obtain multiple surrogate forecasts and observations and their respective quantiles.

More recently, binary reliability diagrams have been extended to the multiclass setting.
One method to show multiclass scores in a binary fashion consists in plotting only the \emph{confidence} of the model for each sample (the highest score among all possible classes). 
% and consider a positive prediction if the predicted class is correct, and negative otherwise.
%.showing only the highest score per sample and its corresponding class as the positive; which could still be  a wrong or right prediction.
This approach was already used for binary classification by
\citet{lichtenstein1977calibration}, reproduced here as Figure \ref{fig:eval:lichtenstein1977:6}. 
The figure shows a binary reliability diagram with scores in the range $[0.5,1]$
(with $K$ classes the confidence is never lower than $1/K$).
% and refers back to the work of \citet{Hazard1973}. {\color{red}(TODO: I can not find the pdf of Hazard1973, may need to check it.)}
% The specific score of the winning class is commonly referred as the \emph{confidence} value of the prediction.
%
Another example of the use of confidences in multiclass problems is the recent work of \citet{guo2017}, which shows the confidence for multiclass problems in the form of bar plots and the ECE and MCE metrics discussed below. 
% (which in this work we refer as confidence ECE and MCE).
%In this case, bins with probabilities lower than $1/K$ are always empty, where $K$ is the number of classes.
% \citet{guo2017} also show the deviations from the diagonal as red bars, which is a good way to highlight the mis-calibration but could be somewhat misleading as the area of such bars is not informative.
% Showing bars instead of lines is helpful to visually inspect the miscalibration, however, it is difficult to compare multiple models.
%
Finally, instead of collapsing all classes into a single diagram one could construct one reliability diagram per class as line plots or bars in a one-vs-rest manner \cite{kull2019} (see Figure \ref{fig:eval:pycalib:ter}).

\begin{figure}
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{pycalib_rd_bars.pdf}
        \caption{Reliability diagram with bars for each bin and red error gaps with regards to a perfectly calibrated model, and a histogram of the scores at the bottom.}
        \label{fig:eval:pycalib:bars}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{pycalib_rd_lines.pdf}
        \caption{Comparison of multiple calibration methods, with Clopper–Pearson binomial confidence intervals of 95\% in each observed proportion of positives.}
        \label{fig:eval:pycalib:lines}
    \end{subfigure}
    
    \begin{subfigure}{1.0\linewidth}
        \centering
        \includegraphics[width=\linewidth]{pycalib_rd_ternary.pdf}
        \caption{Multiple classes can be shown as one-vs-rest reliability diagrams.}
        \label{fig:eval:pycalib:ter}
    \end{subfigure}
    \caption{Examples of reliability diagrams using the Python library PyCalib}
    \label{fig:eval:pycal}
\end{figure}

%It is often also useful to show the number of samples in each bin in the form of a histogram next (or below) the reliability diagram in the form of a small histogram at the bottom of the reliability diagram, sharing the x-axis (as seen in {\color{red}[add references]}).\todo{MPN: fix}
%
%{\color{blue}
%MPN: We possibly need to reference the reliability diagram analysis of \cite{vaicenavicius2019evaluating} and their proposed one. And mention \cite{brocker2007} as the original idea? \cite{brocker2007} indicates that \cite{wilks2011statistical} has a great explanation of reliability diagrams.
%}
%

% All the following text in blue are notes
%\cite{Hallenbeck1920} shows a table with 10 bins and the number of rains, forecasts and actual percentage \ref{tab:eval:hallenbeck1920:1}
%
%\cite{brier1950} already used reliability diagrams in form of a table as it was enough to show 5 bins with their corresponding observed proportion of rain cases \ref{tab:eval:brier1950:2}
%
%\cite{sanders1963} is one of the first articles that show a reliability diagram depicting forecast probabilities agains observed relative frequencty of occurrence. However, the forecast probabilities always fall into a one decimal point, including zero and one (11 bins). Other figures show what it seems to be 21 bins but the first and last bins are empty.
%{\color{red} Need to understand what is the range of every bin, given that the boundaries may contain a smaller bin width.}. 
%The author also included the number of forecasts in every bin. Find out what are the numbers on the right y-axis in \ref{fig:eval:sanders1963:1}. Altough a reliability diagram is first presented, the rest of the article chooses to show departure from expectancy vs observed departure of relative frequency of occurrence \ref{fig:eval:sanders1963:2}.

%----------------------------------------------------%
% \subsection{Expected/Maximum calibration error}
%----------------------------------------------------%
    % \begin{itemize}
    %     \item As seen in the previous Section, each notion of calibration is related to a reliability diagram
    %     \begin{itemize}
    %         \item This can be used to visualise miscalibration on binned scores
    %     \end{itemize}
    %     \item We will now see how these bins can be used to measure miscalibration
    % \end{itemize}


    % \begin{itemize}
    %     \item We start by introducing a toy example:
    % \end{itemize}
    
    \begin{table}[!b]
        \begin{tabular}{lrrrr}
            \toprule
            {id} &  $\hat{s}_1$ &  $\hat{s}_2$ &  $\hat{s}_3$ &  $y$ \\
            \midrule
            1  &     1.0 &     0.0 &     0.0 &    1 \\
            2  &     0.9 &     0.1 &     0.0 &    1 \\
            3  &     0.8 &     0.1 &     0.1 &    1 \\
            4  &     0.7 &     0.1 &     0.2 &    1 \\
            5  &     0.6 &     0.3 &     0.1 &    1 \\
            6  &     0.4 &     0.1 &     0.5 &    1 \\
            7  &     1/3 &     1/3 &     1/3 &    1 \\
            8  &     1/3 &     1/3 &     1/3 &    1 \\
            9  &     0.2 &     0.4 &     0.4 &    1 \\
            10 &     0.1 &     0.5 &     0.4 &    1 \\
            \bottomrule
        \end{tabular}
        \hfill
        \begin{tabular}{lrrrr}
            \toprule
            {id} &  $\hat{s}_1$ &  $\hat{s}_2$ &  $\hat{s}_3$ &  $y$ \\
            \midrule
            11 &          0.8 &          0.2 &          0.0 &    2 \\
            12 &          0.7 &          0.0 &          0.3 &    2 \\
            13 &          0.5 &          0.2 &          0.3 &    2 \\
            14 &          0.4 &          0.4 &          0.2 &    2 \\
            15 &          0.4 &          0.2 &          0.4 &    2 \\
            16 &          0.3 &          0.4 &          0.3 &    2 \\
            17 &          0.2 &          0.3 &          0.5 &    2 \\
            18 &          0.1 &          0.6 &          0.3 &    2 \\
            19 &          0.1 &          0.3 &          0.6 &    2 \\
            20 &          0.0 &          0.2 &          0.8 &    2 \\
            \bottomrule
        \end{tabular}
        \hfill
        \begin{tabular}{lrrrr}
            \toprule
            {id} &  $\hat{s}_1$ &  $\hat{s}_2$ &  $\hat{s}_3$ &  $y$ \\
            \midrule
            21 &          0.8 &          0.2 &          0.0 &    3 \\
            22 &          0.8 &          0.1 &          0.1 &    3 \\
            23 &          0.8 &          0.0 &          0.2 &    3 \\
            24 &          0.6 &          0.0 &          0.4 &    3 \\
            25 &          0.3 &          0.0 &          0.7 &    3 \\
            26 &          0.2 &          0.6 &          0.2 &    3 \\
            27 &          0.2 &          0.4 &          0.4 &    3 \\
            28 &          0.0 &          0.4 &          0.6 &    3 \\
            29 &          0.0 &          0.3 &          0.7 &    3 \\
            30 &          0.0 &          0.3 &          0.7 &    3 \\
            \bottomrule
        \end{tabular}
        \caption{Class probabilities given by a classifier to 30 instances belonging to three different classes.}
        \label{tab:evaluation:toy}
    \end{table}

%----------------------------------------------------%
\subsection{Evaluating calibration error: the binary case}
\label{sec:met:bin}
%----------------------------------------------------%

% We define the binary \textit{estimated calibration error} \citep{roelofs2021mitigating}, also commonly called \textit{expected calibration error}, or binary-ECE \citep{naeini2015}, as the average gap across all bins in a reliability diagram, weighted by the number of instances in each bin, as given by Equation (\ref{eq:binaryECE}).


% In the past, most of the research on the calibration of probabilities has focused on binary classification problems. However, more recently multiclass calibration has got some attention and new metrics and visualisation tools have been proposed.
We now proceed with discussing how to measure calibration error. 
We will use the three-class toy problem in Table \ref{tab:evaluation:toy} throughout. 
In this section we convert it to a binary classification problem by taking class 1 as positive and classes 2 and 3 as negative. 
We then apply equal-width binning to the class 1 probabilities. 
% in order to separate class 1 probabilities and their corresponding labels into 5 bins, corresponding to intervals $[0, 0.2]$, $(0.2, 0.4]$, $(0.4, 0.6]$, $(0.6, 0.8]$, and $(0.8, 1.0]$. 
Table \ref{tab:evaluation:binary:bins} shows the resulting bins $\mathbb{B}_m$, $m \in \{1, \ldots, 5\}$, from which we calculate the number of instances in the bin denoted as $|\mathbb{B}_{m}|$, the average probability $\Bar{\mathsf{s}}(\mathbb{B}_{m})$, the proportion of positives $\Bar{\mathsf{y}}(\mathbb{B}_{m})$, and the absolute gap between them $|\Bar{\mathsf{y}}(\mathbb{B}_m) - \Bar{\mathsf{s}}(\mathbb{B}_m)|$. 


        \begin{table}[!b]
            \centering
            \small
            \begin{tabular}{lrllllc}
                \toprule
                 $\mathbb{B}_m$ &  $|\mathbb{B}_{m}|$ &  $\mathsf{s}(\mathbb{B}_{m})$ & $\Bar{\mathsf{s}}(\mathbb{B}_{m})$ & $\mathsf{y}(\mathbb{B}_{m})$                             & $\Bar{\mathsf{y}}(\mathbb{B}_{m})$ & $|\Bar{\mathsf{y}}(\mathbb{B}_m) - \Bar{\mathsf{s}}(\mathbb{B}_m)|$ \\
                \midrule
                 %$\mathbb{B}_1$ &         11 &  0.0, 0.0, 0.0, 0.0, 0.1, 0.1, 0.1,  \ldots &           0.10 &  0 (9), 1 (2) &             0.18 & 0.08\\
                 $\mathbb{B}_1$ &         11 &  $0.0^{(4)}$, $0.1^{(3)}$,  $0.2^{(4)}$ &           0.10 &  $0^{(9)}$, $1^{(2)}$ &             $0.18$ & 0.08\\
                 $\mathbb{B}_2$ &          7 &              $0.3^{(2)}$, $1/3^{(2)}$, $0.4^{(3)}$ &            0.35 &              $0^{(4)}$, $1^{(3)}$ &              0.43 & 0.08\\
                 %$\mathbb{B}_3$ &          3 &                                    0.5, 0.6, 0.6 &            0.57 &                          0 (2), 1 (1) &              $0.\arc{33}$ & 0.24\\
                 $\mathbb{B}_3$ &          3 &                                    0.5, 0.6, 0.6 &            0.57 &                          0, 0, 1 &              $0.33$ & 0.24\\
                 $\mathbb{B}_4$ &          7 &                $0.7^{(2)}$, $0.8^{(5)}$ &            0.77 &              $0^{(5)}$, $1^{(2)}$ &              0.29 & 0.48 \\
                 %$\mathbb{B}_5$ &          2 &                                         0.9, 1.0 &            0.95 &                             1 (2) &              1.00 & 0.05\\
                 $\mathbb{B}_5$ &          2 &                                         0.9, 1.0 &            0.95 &                             1, 1 &              1.00 & 0.05\\
                \bottomrule
            \end{tabular}
            
        \caption{Positive probabilities and corresponding instance labels separated into 5 bins. The probabilities were obtained by taking class 1 as the positive class in the multiclass problem in Table \ref{tab:evaluation:toy}. To reduce the width of the table, a number followed by a superscript parenthesis $X^{(Y)}$ indicates a list of number $X$ repeated $Y$ times.}
        \label{tab:evaluation:binary:bins}
    \end{table}
    
The values of $\Bar{\mathsf{p}}(\mathbb{B}_{m})$, $\Bar{\mathsf{y}}(\mathbb{B}_{m})$ and $|\Bar{\mathsf{y}}(\mathbb{B}_m) - \Bar{\mathsf{s}}(\mathbb{B}_m)|$ in Table \ref{tab:evaluation:binary:bins} can be used to draw the reliability diagram shown in Figure \ref{fig:eval:rel_diagram}, where we can see the red bars representing the calibration error at each bin.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.7\textwidth]{binary-reliability-v2.pdf}
    \caption{Reliability diagram corresponding to the 5 bins presented in Table \ref{tab:evaluation:binary:bins}.}
    \label{fig:eval:rel_diagram}
\end{figure}

Given the information about the bins in Table \ref{tab:evaluation:binary:bins} we could calculate an average of the bin-wise calibration error, which leads us to  binary estimated calibration error, as defined in  Definition \ref{def:binary:ece}.
%
\begin{definition}[Binary-ECE]
\label{def:binary:ece}
Binary \textit{estimated calibration error} \citep{roelofs2021mitigating}, or binary-ECE \citep{naeini2015}, is the average gap across all bins in a reliability diagram, weighted by the number of instances in each bin:
$$\mathsf{ECE}_{\text{binary}}  = \sum_{m=1}^M \frac{|\mathbb{B}_{m}|}{N} |\Bar{\mathsf{y}}(\mathbb{B}_{m}) - \Bar{\mathsf{s}}(\mathbb{B}_{m})|,$$
where $M$ and $N$ are the number of bins and instances, respectively. 
% $\mathbb{B}_{m}$ is the $m$-th probability bin, $|\mathbb{B}_{m}|$ denotes the size of the bin, and $\Bar{\mathsf{s}}(\mathbb{B}_{m})$ and $\Bar{\mathsf{y}}(\mathbb{B}_{m})$ are the average predicted probability and the proportion of positives in bin $\mathbb{B}_{m}$. 
Binary-ECE is also commonly called binary \textit{expected calibration error}, however this quantity is empirically estimated on a validation or test sample, which is why we prefer to call it binary \textit{estimated calibration error}.
\end{definition}
%
Binary-ECE aggregates part of the visual information about calibration error in Figure  \ref{fig:eval:rel_diagram} by taking the weighted mean of the sizes of these gaps. In this example, $\mathsf{ECE}_{\text{binary}} =0.1873$. 

Binary-ECE ranges from $0$ to $1$, with particular values including $\mathsf{ECE}_{\text{binary}} =\pi_1$ (proportion of positives) for a classifier that randomly outputs probability $1$ for one of the classes, $\mathsf{ECE}_{\text{binary}} =0$ for a perfect classifier that always predicts probability $1$ for the correct class or for a classifier that constantly outputs positive probability equal to $\pi_1$, and $\mathsf{ECE}_{\text{binary}} =1$ for a classifier that always assigns probability $1$ to the wrong class.

% \begin{equation}
% \label{eq:binaryECE}
%     \text{binary-ECE}  = \sum_{i=1}^M \frac{|B_{i}|}{N} |\Bar{y}(B_{i}) - \Bar{p}(B_{i})|,
% \end{equation}

% \noindent where $M$ and $N$ are the number of bins and instances, respectively, $B_{i}$ is the $i$-th probability bin, $|B_{i}|$ denotes the size of the bin, and $\Bar{p}(B_{i})$ and $\Bar{y}(B_{i})$ are the average predicted probability and the proportion of positives in bin $B_{i}$.

Instead of measuring how miscalibrated the model is on average, one might be interested in the worst case, in other words ``how maximally miscalibrated is the model''? In this case, one might use the binary maximum calibration error \citep{naeini2015}.
%
\begin{definition}[Binary-MCE]
\label{def:binary:mce}
Binary maximum calibration error (binary-MCE) is the maximum gap across all bins in a reliability diagram: $$\mathsf{MCE}_{\text{binary}} = \max_{m \in \{1, \ldots, M\}} |\Bar{\mathsf{y}}(\mathbb{B}_m) - \Bar{\mathsf{s}}(\mathbb{B}_m)|.$$
\end{definition}
%
In our example, Table \ref{tab:evaluation:binary:bins} and Figure \ref{fig:eval:rel_diagram} show that the fourth bin has the largest gap, with its size corresponding to $\mathsf{MCE}_{\text{binary}} = 0.48$. 

Binary-MCE can be very sensitive to bins with few instances, where the values of $\Bar{\mathsf{y}}(\mathbb{B}_m)$ and $\Bar{\mathsf{s}}(\mathbb{B}_m)$ are calculated based on very little information. In extreme cases with only a single instance in a bin, $\Bar{\mathsf{y}}(\mathbb{B}_m)$ will be the instance's actual label (1 or 0), potentially resulting in a large gap that would have a small weight in binary-ECE, while being the whole value of binary-MCE, meaning that the model would be evaluated based on its performance for a single instance.

% We can similarly define the maximum calibration error (binary-MCE) as the maximum gap across all bins in a reliability diagram, or

% \begin{equation}
% \label{eq:binaryMCE}
%     \text{binary-MCE} = \max_{i \in \{1, \ldots, M\}} |\Bar{y}(B_i) - \Bar{p}(B_i)|.
% \end{equation}


%----------------------------------------------------%
\subsection{Classwise calibration error}
\label{sec:met:clw:ece}
%----------------------------------------------------%

We now proceed to settings with more than two classes and start by defining the estimated calibration error corresponding to a single class $j$ in a multiclass task.

\begin{definition}[Class-$j$-ECE]
\label{def:class:j:ece}
Given a multiclass task with $K$ classes, class-$j$-ECE corresponds to the binary-ECE calculated by taking class $j$ as positive and the other $K-1$ classes together as a new negative class:
$$\mathsf{ECE}_{j}  = \sum_{m=1}^M \frac{|\mathbb{B}_{m,j}|}{N} |\Bar{\mathsf{y}}_j(\mathbb{B}_{m,j}) - \Bar{\mathsf{s}}_j(\mathbb{B}_{m,j})|,$$
where $\mathbb{B}_{m,j}$ is the $m$-th bin of class $j$.
\end{definition}

Once again we turn to our example in Table \ref{tab:evaluation:toy}. Following Definition \ref{def:class:j:ece}, we have already calculated class-$1$-ECE ($0.1873$) in our binary-ECE example. Now we need to calculate class-$2$-ECE and class-$3$-ECE. Tables \ref{tab:evaluation:binary2:bins} and \ref{tab:evaluation:binary3:bins} show the binary bins for classes $2$ and $3$, respectively, while the binary reliability diagrams of the three classes can be seen in Figure \ref{fig:eval:clas_rel_diagram}.

%\begin{table}[!b]
%    \centering
%    \small
%    \begin{tabular}{lrllllc}
%        \toprule
%         $\mathbb{B}_{m,2}$ &  $|\mathbb{B}_{m,2}|$ &                                              & $\Bar{\mathsf{s}}(\mathbb{B}_{m,2})$ &                                          & $\Bar{\mathsf{y}}(\mathbb{B}_{m,2})$ & $|\Bar{\mathsf{y}}(\mathbb{B}_m) - \Bar{\mathsf{s}}(\mathbb{B}_m)|$  \\
%        \midrule
%         $\mathbb{B}_{1,2}$ &         15 &  0.0$\times$(5), 0.1$\times$(5), 0.2$\times$(5) &           0.10 &  0$\times$(10), 1$\times$(5) &             0.33 & 0.23\\
%         $\mathbb{B}_{2,2}$ &         12 &  0.3$\times$(5), 1/3$\times$(2),  0.4$\times$(5) &           0.35 &           0$\times$(8), 1$\times$(4) &             0.33 & 0.02\\
%         $\mathbb{B}_{3,2}$ &          3 &                                    0.5, 0.6, 0.6 &            0.57 &                                      0, 0, 1 &              0.33 & 0.24\\
%         $\mathbb{B}_{4,2}$ &          0 &                                                  &             &                                              &             \\
%         $\mathbb{B}_{5,2}$ &          0 &                                                  &             &                                              &             \\
%        \bottomrule
%    \end{tabular}
%    \caption{Positive probabilities and corresponding instance labels separated into 5 bins. The probabilities were obtained by taking class 2 as the positive class in the multiclass problem in Table \ref{tab:evaluation:toy}.}
%        \label{tab:evaluation:binary2:bins}
%\end{table}

\begin{table}[!b]
    \setlength{\tabcolsep}{5pt}
    \centering
    \small
    \begin{tabular}{lrllllc}
        \toprule
         $\mathbb{B}_{m,2}$ &
         $|\mathbb{B}_{m,2}|$ &
         $\mathsf{s}(\mathbb{B}_{m,2})$&
         $\Bar{\mathsf{s}}(\mathbb{B}_{m,2})$&
         $\mathsf{y}(\mathbb{B}_{m,2})$ &
         $\Bar{\mathsf{y}}(\mathbb{B}_{m,2})$ &
         {\footnotesize $|\Bar{\mathsf{y}}(\mathbb{B}_m) - \Bar{\mathsf{s}}(\mathbb{B}_m)|$}  \\
        \midrule
         $\mathbb{B}_{1,2}$ &         15 &  $0^{(5)}$, $0.1^{(5)}$, $0.2^{(5)}$ &           0.10 &  $0^{(10)}$, $1^{(5)}$ &             0.33 & 0.23\\
         $\mathbb{B}_{2,2}$ &         12 &  $0.3^{(5)}$, $1/3^{(2)}$,  $0.4^{(5)}$ &           0.35 &           $0^{(8)}$, $1^{(4)}$ &             0.33 & 0.02\\
         $\mathbb{B}_{3,2}$ &          3 &                                    0.5, 0.6, 0.6 &            0.57 &                                      0, 0, 1 &              0.33 & 0.24\\
         $\mathbb{B}_{4,2}$ &          0 &                                                  &             &                                              &             \\
         $\mathbb{B}_{5,2}$ &          0 &                                                  &             &                                              &             \\
        \bottomrule
    \end{tabular}
    \caption{Positive probabilities and corresponding instance labels separated into 5 bins. The probabilities were obtained by taking class 2 as the positive class in the multiclass problem in Table \ref{tab:evaluation:toy}.}
        \label{tab:evaluation:binary2:bins}
\end{table}

\begin{table}[ht]
    \setlength{\tabcolsep}{5pt}
    \centering
    \small
    \begin{tabular}{lrllllc}
        \toprule
         $\mathbb{B}_{m,3}$ & 
         $|\mathbb{B}_{m,3}|$ &
         $\mathsf{s}(\mathbb{B}_{m,3})$ &
         $\Bar{\mathsf{s}}(\mathbb{B}_{m,3})$ &
         $\mathsf{y}(\mathbb{B}_{m,3})$ &
         $\Bar{\mathsf{y}}(\mathbb{B}_{m,3})$ &
         {\footnotesize
         $|\Bar{y}(\mathbb{B}_m) - \Bar{p}(\mathbb{B}_m)|$}\\
        \midrule
         $\mathbb{B}_{1,3}$ &         11 &  $0.0^{(4)}$, $0.1^{(3)}$, $0.2^{(4)}$ &           0.10 &  $0^{(7)}$, $1^{(4)}$ &             0.36 & 0.26\\
         $\mathbb{B}_{2,3}$ &         11 &  $0.3^{(4)}$, $1/3^{(2)}$, $0.4^{(5)}$ &           0.35 &  $0^{(9)}$, $1^{(2)}$ &             0.18 & 0.17\\
         $\mathbb{B}_{3,3}$ &          4 &                               0.5, 0.5, 0.6, 0.6 &            0.55 &                       0, 0, 0, 1 &              0.25 & 0.3\\
         $\mathbb{B}_{4,3}$ &          4 &                               0.7, 0.7, 0.7, 0.8 &            0.72 &                       0, 1, 1, 1 &              0.75 & 0.03\\
         $\mathbb{B}_{5,3}$ &          0 &                                                  &             &                                  &             \\
        \bottomrule
    \end{tabular}
    \caption{Positive probabilities and corresponding instance labels separated into 5 bins. The probabilities were obtained by taking class 3 as the positive class in the multiclass problem in Table \ref{tab:evaluation:toy}.}
        \label{tab:evaluation:binary3:bins}
\end{table}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth,trim=0 0 0 0, clip]{classwise-reliability-v2.pdf}
    \caption{Binary reliability diagram of each class in our running example. Note the empty bins in the second and third reliability diagrams, showing that the classifier never outputs high probabilities for these classes.}
    \label{fig:eval:clas_rel_diagram}
\end{figure}

\noindent From the values in Tables \ref{tab:evaluation:binary2:bins} and \ref{tab:evaluation:binary3:bins} and following Definition \ref{def:class:j:ece}, we get $\text{class-$2$-ECE} = 0.147$ and $\text{class-$3$-ECE} = 0.2017$. 

We can now define classwise-ECE \cite{kull2019}. 
%
\begin{definition}[Classwise-ECE]
\label{def:classwise:ece}
The estimated classwise calibration error (classwise-ECE) is the average class-$j$-ECE across all classes:
$$\mathsf{ECE}_{\text{classwise}}  = \frac{1}{K}\sum_{j=1}^K \mathsf{ECE}_{j}.$$
\end{definition}
%
According to Definition \ref{def:classwise:ece}, in our example $\text{classwise-ECE} = (0.1873 + 0.147 + 0.2017)/3 = 0.1787$.

% Confidence-ECE only cares about the calibration error associated with the winning class. In order to measure miscalibration for all classes, we can take the average binary-ECE across all classes, which gives the expected classwise calibration error (classwise-ECE) \cite{kull2019}. Formally, classwise-ECE is defined as the average gap across all classwise reliability diagrams, weighted by the number of instances in each bin, as shown in Equation (\ref{eq:classwiseECE}).

% \begin{equation}
%     \label{eq:classwiseECE}
%     \text{classwise-ECE}  = \frac{1}{K}\sum_{j=1}^K \sum_{i=1}^M \frac{|B_{i,j}|}{N} |\Bar{y}_j(B_{i,j}) - \Bar{p}_j(B_{i,j})|,
% \end{equation}

% \noindent where $B_{i,j}$ is the $i$-th bin of the $j$-th class, $|B_{i,j}|$ denotes the size of the bin, and  $\Bar{p}_j(B_{i,j})$ and $\Bar{y}_j(B_{i,j})$ denote the average prediction of class $j$ probability and the actual proportion of class $j$ in the bin $B_{i,j}$. The contribution of a single class $j$ to classwise-ECE is called class-$j$-ECE.

\begin{definition}[Classwise-MCE]
\label{def:classwise:mce}
The maximum classwise calibration error (classwise-MCE) \cite{kull2019} is defined as the maximum gap across all bins and all classwise-reliability diagrams:
$$
    \mathsf{MCE}_{\text{classwise}}  = \max_{j \in \{1, \ldots, K\}\, m \in \{1, \ldots, M\}}  |\Bar{\mathsf{y}}_j(B_{m,j}) - \Bar{\mathsf{s}}_j(B_{m,j})|.
$$
\end{definition}
%
% Equation (\ref{eq:classwiseMCE}) presents the maximum classwise calibration error (classwise-MCE), which is defined as the maximum gap across all bins and all classwise-reliability diagrams.
%
% \begin{equation}
%     \label{eq:classwiseMCE}
%     \text{classwise-MCE}  = \max_{j \in \{1, \ldots, K\}\, i \in \{1, \ldots, M\}}  |\Bar{y}_j(B_{i,j}) - \Bar{p}_j(B_{i,j})|.
% \end{equation}
%
In our running example, $\mathsf{MCE}_{\text{classwise}} = 0.48$. 

Note that this is not the only way to define classwise-MCE. For example, one could be interested in the average maximum gap across classes, i.e. an average class-$j$-MCE, which in our example would be $(0.48 + 0.24 + 0.3)/3 = 0.34$. As another variation, one could take the maximum class-$j$-ECE, which would then indicate the most miscalibrated class on average. In our example, this variation corresponds to class-$3$-ECE ($0.2017$).





% \begin{figure}
%     \centering
%     \includegraphics[width=0.7\textwidth]{figures/evaluation/perfect-reliability.png}
%     \caption{Reliability diagram of a classifier that predicts the  overall class distribution ($0.5$ in this case). The corresponding binary-ECE here is zero.}
%     \label{fig:eval:optim_ece}
% \end{figure}

Although classwise-ECE and MCE measure calibration error over all classes, they do not take into account the miscalibration that arises from every possible relationship between classes. For a true multiclass-ECE, we could bin the probability vectors in simplex space and then calculate the gaps between the average probability vector and the vector of class proportions in each bin. Although this seems like the right thing to do when evaluating multiclass calibration, it might not be efficiently computable with large numbers of classes, as the number of bins can be prohibitively high and most bins would likely be empty.

Similarly to binary-ECE, a value of $\text{classwise-ECE} = 0$ can be obtained by a classifier that constantly outputs the class proportions. For example, if a classifier always predicts $1/3$ setosa, $1/3$ versicolor and $1/3$ virginica for Fisher's Iris dataset, the resulting classwise-ECE will be $0$.
% Another limitation of all ECE/MCE measures is that optimising them can be as simple as predicting the overall class distribution, regardless of the given instance, as shown in Figure \ref{fig:eval:optim_ece}.



%----------------------------------------------------%
\subsection{Confidence calibration error}
\label{sec:met:con:ece}
%----------------------------------------------------%

As already mentioned, some calibration measures only consider a model's confidence, defined as
the maximum value in the predicted probability vector, i.e. the probability given to the winning class. Prediction confidence is not a new idea and has been around since at least the 1970s. \citet{lichtenstein1977calibration} called it the half-range method in the binary case (referred to as ``two alternatives'' in the paper) and it was also mentioned as one of the variations of the multiclass task, which the authors called ``three or more alternatives''. 
More recently it has been popularised by \citet{guo2017}.
    
    To calculate confidence-ECE, we first bin the confidence values and, for each instance of each bin, we produce a binary value indicating if the classifier predicted correctly or not.
    Recalling the example from Table \ref{tab:evaluation:toy}, the resulting confidence bins are presented in Table \ref{tab:evaluation:confidence:bins}, where $\Bar{\mathsf{p}}(\mathbb{B}_{m})$ and $\mathsf{acc}(\mathbb{B}_{m})$ are respectively the average confidence and prediction accuracy in bin $\mathbb{B}_{m}$, with the corresponding reliability diagram in Figure \ref{fig:eval:rel_diagram2}.
    Note that bin $\mathbb{B}_1$ is empty, which demonstrates that confidence-ECE and confidence reliability diagrams are different from binary-ECE even on two-class problems. 
        
        \begin{table}[ht]
        \centering
        \small
        \begin{tabular}{lrllllc}
            \toprule
             $\mathbb{B}_m$ &
             $|\mathbb{B}_{m}|$ &
             $\mathsf{s}(\mathbb{B}_{m})$ &
             $\Bar{\mathsf{s}}(\mathbb{B}_{m})$ &
             $\mathsf{y}(\mathbb{B}_{m})$ &
             $\mathsf{acc}(\mathbb{B}_{m})$ &
             $|\mathsf{acc}(\mathbb{B}_m) - \Bar{\mathsf{p}}(\mathbb{B}_m)|$ \\
            \midrule
             $\mathbb{B}_1$ &          0 &                                                  &             &                                  &             \\
             $\mathbb{B}_2$ &          7 &              $1/3^{(2)}$, $0.4^{(5)}$ &            0.38 &              $0^{(4)}$, $1^{(3)}$ &              0.43 & 0.05\\
             $\mathbb{B}_3$ &         10 &  $0.5^{(4)}$, $0.6^{(6)}$ &           0.56 &     $0^{(7)}$, $1^{(3)}$ &             0.30 & 0.26\\
             $\mathbb{B}_4$ &         11 &  $0.7^{(5)}$, $0.8^{(6)}$ &           0.75 &  $0^{(6)}$, $1^{(5)}$ &             0.45 & 0.3\\
             $\mathbb{B}_5$ &          2 &                                         0.9, 1.0 &            0.95 &                             1, 1 &              1.00 & 0.05\\
            \bottomrule
        \end{tabular}\caption{Confidence bins corresponding to the toy example from Table \ref{tab:evaluation:toy}. The binary values in the fifth column indicate if the classifier correctly classified each instance. }
        \label{tab:evaluation:confidence:bins}
        \end{table}
        
   

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.7\textwidth]{confidence-reliability-v2.pdf}
    \caption{Confidence reliability diagram corresponding to the bins in Table \ref{tab:evaluation:confidence:bins}.}
    \label{fig:eval:rel_diagram2}
\end{figure}

\begin{definition}[Confidence-ECE]
    \label{def:confidence:ece}
    Confidence-ECE is the average difference between accuracy and average confidence across all bins in a confidence reliability diagram, weighted by the number of instances in each bin: $$\mathsf{ECE}_{\text{confidence}}  = \sum_{m=1}^M \frac{|\mathbb{B}_{m}|}{N} |\mathsf{acc}(\mathbb{B}_{m}) - \Bar{\mathsf{p}}(\mathbb{B}_{m})|.$$
    \end{definition}
    %
    We then calculate confidence-ECE as the weighted mean of the gaps between average confidence and prediction accuracy at each bin, thus $\mathsf{ECE}_{\text{confidence}}=0.2117$, while the maximum confidence calibration error (confidence-MCE) corresponds to the largest gap, i.e. $\mathsf{MCE}_{\text{confidence}}=0.3$. As with binary-ECE and for the same reasons, confidence-MCE is very sensitive to small bins, but in this particular example, its value corresponds to the gap of the largest bin.
    


%\todo{TSF: please add concluding paragraph}

As we show in Section \ref{sec:calibrators}, there is a wide range of post-hoc calibration techniques in the literature, each one capable of handling different miscalibration patterns. Thus, it can be useful to first analyse a model's reliability diagram, as it allows us to diagnose model miscalibration, i.e. in what probability ranges it is underconfident or overconfident, and this can help choose an appropriate calibration method. In addition, any of the ECE measures discussed in this Section  can be used to decide if a classifier actually needs to be calibrated, by testing the hypothesis that the model is already calibrated, as shown in Section \ref{sec:hyp}. \newtext{Finally, it is important to consider that all ECE/MCE measures can provide very different values given different number of bins, as shown in Figs. \ref{fig:hallenbeck-rel} and \ref{fig:hallenbeck2-rel}, and they can be minimised by predicting the overall class distribution, regardless of the given instance. Thus, it is good practice to use them together with the proper scoring rules presented in Section \ref{sec:psr}, to get a full evaluation of the probabilities produced by a model.}





%----------------------------------------------------%




==> mlj_files/compiled/04_calibrators.tex <==
\section{Calibration methods}
\label{sec:calibrators}

In this section we provide a systematic review of standard approaches to calibrating classifiers through the construction of calibration maps.
In particular, we focus on post-hoc calibration methods for classification, which can be used to adjust probability outputs separately from the initial training process.
For each method, we cover the mathematical formulation, the objective function for learning the map, and the predictive function to calculate the class probabilities for a new instance.
We include a few test cases to empirically analyse each method, and discuss their advantages and disadvantages.
General guidance on each method's implementation is also discussed, addressing issues such as overfitting and computational effort.
At the end of the section, we briefly describe some related work to classifier calibration, such as methods that can improve the calibration level during training time, methods that are designed for getting well-calibrated probability for other predictive tasks, and approaches that are designed for specific tasks in areas such as computer vision and natural language processing. 

\subsection{Preliminaries}

We denote a calibration map as a function $\mathsf{g}: \mathbb{S}_{\mathbb{Y}} \rightarrow \mathbb{P}_{\mathbb{Y}}$. 
Here $\mathbb{Y} =\{1, \dots, K\}$ is the discrete space with $K$ classes of the target variable.
$\mathbb{P}_{\mathbb{Y}}$ denotes the probability vector space on $\mathbb{Y}$, that is: $\mathbb{P}_{\mathbb{Y}} = \{ [s_1, \dots, s_K] \mid s_j \geq 0, \sum_{j=1}^{K} s_j = 1\}$.  
$\mathbb{S}_{\mathbb{Y}}$ represents the original output space of the (uncalibrated) classifier, which can take various forms depending on the formalisation of the classifier.
For instance, for a typical probabilistic classifier, we have $\mathbb{S}_{\mathbb{Y}} = \mathbb{P}_{\mathbb{Y}}$.
A one-vs-rest SVM might produce $K$-dimensional vectors in $\mathbb{S}_{\mathbb{Y}} = \mathbb{R}^{K}$.
Deep neural networks can also provide unnormalised vector outputs before the softmax is performed at the final layer. 
Calibration maps that work with such vector spaces are referred to as scaling approaches.
The name suggests these approaches are used to scale the vector output into a probability output, which is quite useful for models like SVMs, as the hinge loss does not optimise probability estimates by default.
However, other than the name and historical motivation, in modern applications, probability calibrators and scaling approaches can be used interchangeably, as the probability space and vector space can be transformed into each other by using the link function (e.g. softmax) and inverse link function (e.g. logit transform ). 

In general, to obtain a calibration map, we will have a calibration set with uncalibrated probabilities and labels, denoted as $\mathbb{C} = \{(\mathbf{s}_1, y_1), \dots, (\mathbf{s}_N, y_N)\}$, and an objective function $\mathsf{L}(\mathbb{C})$ to optimise.
Typically, the objective function is constructed using proper scoring rules, that is, $\mathsf{L}(\mathbb{C}) = \sum_{i=1}^{N} \phi(\mathbf{s}_i, y_i)$, and it can be optimised via various gradient descent algorithms.


\newtext{
\textbf{Training Schemes}: While the above notation suggested that the calibration map can be obtained by fitting a calibrator on a given hold-out calibration set, in practice a small training set and calibration set might lead to over-fitting thus limiting the performance of the calibrated model.
A typical solution here is to introduce multi-fold dataset splits as introduced in \cite{platt99probabilisticoutputs}.
The author proposes to divide the training sets into three different folds and fit the model and calibration map in cross-validation.
Two folds are used to train the uncalibrated model, and the model predictions on the last fold are collected and used to fit the calibration map.
This training process thus ends up with three pairs of models and calibration maps.
At test time each instance will be predicted with all three pairs, and resulting probabilities are averaged to give the final estimate.
Alternatively, people have also used applied label smoothing \cite{muller2019does} to reduce the level of overfitting and over-confidence.
The idea is to have a weighted average between the original probability vector (either from the uncalibrated model or after a calibration method has been applied) and a uniform probability vector.
Therefore, the final probability vector will be pushed somewhat towards the uniform probability vector, which avoids overly high confidence for unsuitable cases.}


\subsection{Two-Class Test Cases}

We designed some test cases to illustrate each calibration map's characteristics empirically.
These test cases are designed with a known distribution and allow us to directly sample the instances.
For ease of understanding, we consider a scenario with a univariate feature ($ \mathbf{x} \in \mathbb{R}$), so that we can inspect the fitted functions and reliability diagrams by means of $x$-$y$ plots.

% \subsubsection*{Binary Test Cases}
Figure~\ref{fig:test_dataset} depicts the probability density functions for the synthetic two-class dataset, as well as the posterior class probabilities when predicting any new instances.
%The density functions are constructed with a mixture of Gaussian distributions, and the class prior is set to be equal to construct the joint dataset distribution.
The generative model is equally likely to produce a positive and a negative, and the distribution of the feature values are mixtures of two normal distributions within each class. 
% is a mixture of Gaussian distributions N(-4,960) and N(64,1280) for positives and a mixture of Gaussian distributions N(4,980) and N(-72,1024) for negatives. 
Denoting the mixture components as $H=1$ and $H=2$, our generative model can be formally written down as:
%
\begin{align*}
    Y &\sim \text{Bernoulli}(0.5) \\
    H &\sim \text{Bernoulli}(0.5) \\
    X \mid Y=1, H=1 &\sim \text{Gaussian}(-4, 960) \\
    X \mid Y=1, H=2 & \sim \text{Gaussian}(64, 1280) \\
    X \mid Y=2, H=1 & \sim \text{Gaussian}(4, 980) \\
    X \mid Y=2, H=2 & \sim \text{Gaussian}(-72, 1024) \\
\end{align*}


\begin{figure}[!tbp]
    \centering
    %\includegraphics[width=0.6\textwidth]{figures/calibrators/data_distribution.png}
    %\includegraphics[width=0.273\textwidth]{figures/calibrators/data_prediction.png}
    \includegraphics[width=0.61\textwidth, valign=t]{data_distribution.png}
    \includegraphics[width=0.33\textwidth, valign=t]{data_prediction.png}
    \caption{The synthetic dataset used in the test cases. The left two figures shows the data distribution for each class respectively. The figure on the right gives the Bayes-optimal posterior probability for class 1.}
    \label{fig:test_dataset}
\end{figure}

%\todo[inline]{MPN: I have modified the images in Figure \ref{fig:test_dataset}. Should I put the previous figures back?}

\noindent
This generative assumption allows us to approximate the `true' reliability diagram closely for every test case and provides better insights into each calibration map. Specifically, we generate a large number of random samples and use small bin sizes to approximate a smooth reliability diagram.

We consider three cases for binary classification, each of which may occur in practice. 
The first two cases are hypothetical over/under-confident scenarios using a logistic regression model of the form 
    $\hat{\mathsf{f}}(x) = (1 + \exp(-a\cdot x))^{-1}$.
Such a model puts the decision boundary at $x=0$, which is nearly Bayes-optimal for the synthetic data. 
The model confidence can be moderated with the parameter $a$, and we will use the following two cases: 
%
\begin{align*}
    \hat{\mathsf{f}}_{\text{under}}(x) = \frac{1}{1 + \exp(-0.01\cdot x)} \\
    \hat{\mathsf{f}}_{\text{over}}(x) = \frac{1}{1 + \exp(-0.05\cdot x)}
\end{align*}
%
The third case is obtained with an MLP classifier as implemented by the scikit-learn Python package.
The model is specified with a two layer structure with 128 hidden units per layer.
The activation is selected as the ReLU function.
The remaining settings are left at their default values.
$10,000$ instances are sampled to train the model.

The smoothed reliability diagrams for these three cases are shown in Figure~\ref{fig:binary_test_cases}.
In the under-confident case the output probabilities barely reach the outside of the interval $[0.1, 0.9]$.
The reliability diagram shows a higher slope compared with the perfectly calibrated  one (the diagonal).
In contrast, the over-confident case has a shallower slope around the middle compared with the diagonal.
It further causes the reliability diagram to have sharp transitions while approaching the extremes. 
For the MLP case, we can observe both under-confident and over-confident regions throughout the reliability diagram.
%As we have seen with the previous two test cases, before the 0.5 on the horizontal axis, if the reliability diagram falls below the diagonal, it indicates under-confident, and vice versa.
%After the 0.5 on the horizontal axis, having the reliability diagram above the diagonal becomes the sign of under-confident, and vice verse.
This specific MLP classifier tends to be under-confident around $s \in [0, 0.1]$ and $s \in [0.65, 1]$, and mostly over-confident elsewhere.

\begin{figure}[!tbp]
    \centering
    %\includegraphics[width=0.28\textwidth]{figures/calibrators/test_case_1.png}
    %\includegraphics[width=0.28\textwidth]{figures/calibrators/test_case_2.png}
    \includegraphics[width=0.3\textwidth, valign=t]{test_case_1.png}
    \includegraphics[width=0.3\textwidth, valign=t]{test_case_2.png}
    %\includegraphics[width=0.28\textwidth]{figures/calibrators/test_case_3.png}
    \includegraphics[width=0.3\textwidth, valign=t]{test_case_3.png}
    \caption{The reliability diagrams of the three uncalibrated classifiers. The left figure shows the $\hat{\mathsf{f}}_{\text{under}}$ case, where the classifier predicts a probability closer to 0.5 compared with the Bayes-optimal case (Fig.~\ref{fig:test_dataset}, right), resulting in a reliability diagram with steeper slope. The middle figure shows the $\hat{\mathsf{f}}_{\text{over}}$  case, where the predicted probabilities are pushed towards $0$ and $1$ respectively, resulting in a shallower reliability curve. The right figure is obtained with a MLP classifier ($\hat{\mathsf{f}}_{\text{MLP}}$), where the reliability diagram shows over-confident and under-confident predictions around different regions. 
    }
    \label{fig:binary_test_cases}
\end{figure}

%\todo[inline]{MPN: Decide if should increase the font size of all figures (I have changed Fig. 12 Test Case 1, 2 and 3 as an example).}

\subsection{Calibration for Binary Classification}

We start with methods that can learn calibration maps for binary problems.
In binary classification, probability estimates are scalars, so the calibration maps are functions mapping from $[0, 1]$ to $[0, 1]$.
Here we describe four widely applied methods in detail: empirical binning, isotonic regression, logistic calibration and Beta calibration.  
Other approaches will be be briefly mentioned at the end of this section.

\subsubsection*{Empirical Binning}

Empirical binning \newtext{\cite{zadrozny2001obtaining,naeini2015}} is one of the simplest methods to build a calibration map.
It directly connects to the previously introduced ECE measure, which evaluates the calibration level by calculating the empirical frequencies within a set of score intervals. 
Therefore, binning approaches can directly optimise a variant of ECE depending on how the binning scheme is selected.

\begin{figure}[!tbp]
    \centering
    \begin{subfigure}{\textwidth}
    \centering
    %\includegraphics[width=0.28\textwidth]{figures/calibrators/Case1_EMP10_prediction.png}
    \includegraphics[width=0.28\textwidth]{Case1_EMP10_calibration.png}
    \includegraphics[width=0.28\textwidth]{Case1_EMP10_reliability.png}
    \caption{Test case 1: under-confidence}
    \end{subfigure}
    
    
    \begin{subfigure}{\textwidth}
    \centering
    %\includegraphics[width=0.28\textwidth]{figures/calibrators/Case2_EMP10_prediction.png}
    \includegraphics[width=0.28\textwidth]{Case2_EMP10_calibration.png}
    \includegraphics[width=0.28\textwidth]{Case2_EMP10_reliability.png}
    \caption{Test case 2: over-confidence}
    \end{subfigure}
    
    \begin{subfigure}{\textwidth}
    \centering
    % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case3_EMP10_prediction.png}
    \includegraphics[width=0.28\textwidth]{Case3_EMP10_calibration.png}
    \includegraphics[width=0.28\textwidth]{Case3_EMP10_reliability.png}
    \caption{Test case 3: MLP classifier}
    \end{subfigure}
    
    \caption{Examples of empirical binning calibration with 10 equal-width bins. As the binning approach can only give discrete outputs, we can observe the probabilities after calibration are no longer continuous and are only presented with 10 values or less (the under-confidence case has fewer values as there are no observations in bins closer to the extremes. The reliability diagrams show that the calibration method works well with all three test case, with most points being close to the calibrated diagonal.  }
    \label{fig:test_emp10}
\end{figure}

% \begin{figure}[!tbp]
%     \centering
%     \begin{subfigure}{\textwidth}
%     \centering
%     %\includegraphics[width=0.28\textwidth]{figures/calibrators/Case1_EMP32_prediction.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/Case1_EMP32_calibration.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/Case1_EMP32_reliability.png}
%     \caption{Test case 1: under-confidence}
%     \end{subfigure}
    
    
%     \begin{subfigure}{\textwidth}
%     \centering
%     %\includegraphics[width=0.28\textwidth]{figures/calibrators/Case2_EMP32_prediction.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/Case2_EMP32_calibration.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/Case2_EMP32_reliability.png}
%     \caption{Test case 2: over-confidence}
%     \end{subfigure}
    
%     \begin{subfigure}{\textwidth}
%     \centering
%     % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case3_EMP32_prediction.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/Case3_EMP32_calibration.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/Case3_EMP32_reliability.png}
%     \caption{Test case 3: MLP classifier}
%     \end{subfigure}
    
%     \caption{Examples of empirical binning calibration with 32 equal-width bins. With a higher number of bins, the discrete probabilities appear to be denser, and the predictions fits the ground-truth better. On the other hand, as we have less samples within each bin, some bins might have a poorer estimates than the 10-bins case. This is more observable with the over-confidence case, where we have less observations around the middle region.}
%     \label{fig:test_emp32}
% \end{figure}

For a typical setting, the empirical binning approach comes with the following parameters. 
(1) Bins: $\{\mathbb{B}_1, \dots, \mathbb{B}_M \}$, where each bin $\mathbb{B}_m \subset [0, 1]$ is an interval of probability range, and $\cup_{m=1}^{M} \mathbb{B}_m = [0, 1]$.
(2) Probability estimates in the bins:  $\mathbf{a}=\{a_1,\dots,a_{M}\}$, where $a_m \in [0, 1]$ specifies the calibrated probability value in each bin.
We usually assume that these bins do not overlap with each other. 
To make a prediction based on an uncalibrated probability $s$, empirical binning uses the following functional form:
%
\begin{align}
% \mathsf{c}(p; B_1, \dots, B_M, \mathbf{a}) = \sum_{j=1}^{M} \mathbb{I}(p\in \mathbb{B}_j) \cdot a_j
\mathsf{g}(s; \mathbb{B}_1, \dots, \mathbb{B}_M, \mathbf{a}) = a_m \quad \quad \quad \text{if}\ s \in \mathbb{B}_m
\end{align}
%
Here $ s \in \mathbb{B}_m$ means that the uncalibrated probability $s$ falls within $\mathbb{B}_m$.

Fitting a binning calibration map can be done by optimising $\mathbf{a}$ using ECE as a loss function: 
%
\begin{align}
%\mathbb{L}(\mathbf{a}) = \sum_{j=1}^{M} \Big | \frac{\sum_{i=1}^{N} \mathbb{I}(p_i \in B_j) \cdot y_i}{|B_j|} - a_j \Big|
\mathbf{a}^* &
= \arg\min_{\mathbf{a}} \mathsf{L}(\mathbf{a}) \\
\mathsf{L}(\mathbf{a}) &= \mathsf{ECE}(\mathbf{a}) 
                       = \sum_{m=1}^{M} \Big | \bar{\mathsf{y}}(\mathbb{B}_m) - a_m \Big|
\end{align}
%
Here $\bar{\mathsf{y}}(\mathbb{B}_m)$ represents the empirical frequency within $\mathbb{B}_m$ as defined in the previous section.  
The equation hence indicates that we want to assign each $a_m$ according to the empirical frequency of the labels within each bin $\mathbb{B}_m$.

We empirically analyse the binning approach with a simple setting of $M=10$ equal-width bins.  
The results with the three test cases are shown in Figure~\ref{fig:test_emp10}.
The binning approach performs well on most points, as the reliability diagram are close to the diagonal  after calibration.
However, it should be noted that the output probabilities can only take $M$ different values.
Therefore, while the final probabilities are calibrated,  we can no longer distinguish instances that receive different predictions from the uncalibrated model.
In other words, binning approaches can reduce the calibration loss at the cost of a higher grouping loss \cite{kull2015novel}.
% According to the data points pictured at the bottom of the figure, we can see this poor performance is mainly caused by the lower amounts of data points around these regions.
% As the test case 2 is designed to be an over-confident example, predictions are more pushed towards either $0$ or $1$ depending on their actual classes, causing the regions around $0.2$ and $0.8$to be emptier than the rest, further causing the bin estimates to be worse for these regions. 

While here we illustrated the binning approach with equal-width bins, it is possible to use other binning schemes such as equal-frequency binning.
For example, \cite{naeini2015} propose a Bayesian binning approach.

To summarise, the main advantages of binning approaches are as follows:
(1) They can be used to directly minimise a specific variant of ECE, hence are useful when calibration loss is of primary concern.
(2) Training is reasonably fast and straightforward. 
(3) Given its non-parametric nature, it does not have any constraint on the form of the calibration maps and therefore can capture arbitrary shapes according to the given bins.
In addition, other binning strategies can also be applied to deal with different datasets and uncalibrated models. %such as equal-frequency binning and Bayesian binning \cite{naeini2015}.



\subsubsection*{Isotonic Calibration}

Calibration by means of isotonic regression is another widely used non-parametric approach \newtext{\cite{barlow1972isotonic,niculescu-mizil2005,naeini2016}}.
The isotonic approach was originally proposed to solve univariate regression tasks where the function were required to be monotonic.
In the case of probability calibration, if we assume the uncalibrated model has a monotonic reliability diagram, then isotonic regression is a suitable approach to achieve a better level of calibration. 

Isotonic regression achieves a monotonic fit by estimating a set of non-decreasing constant segments, corresponding to a set of bins of varying width.  
Isotonic regression can therefore be described with the following parameters:
(1) Bin boundaries: $\mathbf{b}=(b_1,\dots,b_M)$, $b_j \in [0, 1], b_j < b_{j+1}$, and  (2) Edge values:  $\mathbf{v}=(v_1,\dots,v_{M})$, $ v_j \in [0, 1], v_j \leq v_{j+1}$.
As indicated by the parameters, isotonic regression is quite close to an empirical binning approach.
The main difference is that instead of having a pre-defined set of bin edges, isotonic regression learns these bin boundaries from the data.
As a result, isotonic regression can have an variable number of bins depending on the training set.
To calibrate a probability $s$, isotonic regression uses the following predictive function: 
%
\begin{align}
%c(p; \mathbf{b}, \mathbf{v}) = & \frac{1}{\sum_{j=1}^{M-1} \mathbb{I}(p\geq b_j)\cdot\mathbb{I}(p\leq b_{j+1})} \\ \nonumber
%&\sum_{j=1}^{M-1} \mathbb{I}(p\geq b_j)\cdot\mathbb{I}(p<b_{j+1}) \cdot \Big(v_j + \frac{p-b_j}{b_{j+1}-b_j}(v_{j+1} - v_j)\Big) 
\mathsf{g}(s; \mathbf{b}, \mathbf{v}) = \sum_{m=1}^{M-1} \mathsf{I}(s\geq b_m)\cdot\mathsf{I}(s<b_{m+1}) \cdot m_j 
\end{align}
%

\begin{figure}[!tbp]
    \centering
    \begin{subfigure}{\textwidth}
    \centering
    %\includegraphics[width=0.28\textwidth]{figures/calibrators/Case1_ISO_L_prediction.png}
    \includegraphics[width=0.28\textwidth]{Case1_ISO_L_calibration.png}
    \includegraphics[width=0.28\textwidth]{Case1_ISO_L_reliability.png}
    \caption{Test case 1: under-confidence}
    \end{subfigure}
    
    
    \begin{subfigure}{\textwidth}
    \centering
    % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case2_ISO_L_prediction.png}
    \includegraphics[width=0.28\textwidth]{Case2_ISO_L_calibration.png}
    \includegraphics[width=0.28\textwidth]{Case2_ISO_L_reliability.png}
    \caption{Test case 2: over-confidence}
    \end{subfigure}
    
    \begin{subfigure}{\textwidth}
    \centering
    % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case3_ISO_L_prediction.png}
    \includegraphics[width=0.28\textwidth]{Case3_ISO_L_calibration.png}
    \includegraphics[width=0.28\textwidth]{Case3_ISO_L_reliability.png}
    \caption{Test case 3: MLP classifier}
    \end{subfigure}
    
    \caption{Examples of isotonic calibration trained with 10,000 samples. Compared with empirical binning, we can see the isotonic approach can provide a larger variety of outputs in the continuous interval of $[0, 1]$, and different bins can be automatically learnt according to the observations. The calibration method works reasonably well on all three test cases. The over-confidence case still has some errors around around the middle-left and middle-right boundaries, due to the lack of training points within these areas. }
    \label{fig:test_iso_L}
\end{figure}


% \begin{figure}[!tbp]
%     \centering
%     \begin{subfigure}{\textwidth}
%     \centering
%     % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case1_ISO_S_prediction.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/Case1_ISO_S_calibration.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/Case1_ISO_S_reliability.png}
%     \caption{Test case 1: under-confidence}
%     \end{subfigure}
    
    
%     \begin{subfigure}{\textwidth}
%     \centering
%     % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case2_ISO_S_prediction.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/Case2_ISO_S_calibration.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/Case2_ISO_S_reliability.png}
%     \caption{Test case 2: over-confidence}
%     \end{subfigure}
    
%     \begin{subfigure}{\textwidth}
%     \centering
%     % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case3_ISO_S_prediction.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/Case3_ISO_S_calibration.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/Case3_ISO_S_reliability.png}
%     \caption{Test case 3: MLP classifier}
%     \end{subfigure}
    
%     \caption{Examples of isotonic calibration trained with 1,000 samples. We can see from the reliability diagram that the calibration performance is significantly worse than the previous example with 10,000 samples. Being a non-parametric approach, the isotonic calibration is more suitable on larger datasets.}
%     \label{fig:test_iso_S}
% \end{figure}

The three test cases on istonic regression are shown in Figure~\ref{fig:test_iso_L}.
To compare with the empirical binning approach again, while in the empirical case we have a constant prediction within each bin, we can see the prediction of the isotonic approach depends on the two values on the bin edges.
In the case where the two bin edges do not share the same value, isotonic regression performs linear interpolation to calculate the predicted value. 
This behaviour is due to the way that the isotonic approach is estimated. 
To ensure the estimated function is monotonically increasing, the learning algorithm starts with the first bin edge as the minimal feature value ($0$ in the case of an isotonic calibration) and extends the following bin edges until it sees a higher target value (this is also referred to as `pooling adjacent violators' \cite{fawcett2007}).
It can be proven that, with monotonic sets of $\mathbf{b}$ and $\mathbf{s}$, the learning algorithm is equivalent to optimising the following loss \cite{ayer1955empirical}: 
%
\begin{align}
\mathsf{L}(\mathbf{b}, \mathbf{v}) = \frac{1}{N} \sum_{i=1}^{N}\Big( \mathsf{g}(s_i; \mathbf{b}, \mathbf{v}) - y_i\Big)^2
\end{align}
%
Therefore, when used as a probability calibration map, isotonic regression minimises the Brier score on the training set.
Instead of applying isotonic regression directly, \cite{naeini2016} also consider building an ensemble calibration map by combining a set of near-isotonic functions.  
Recently, \cite{allikivi2019} propose a Bayesian approach to improve isotonic regression, with demonstrated improvements on binary tasks.

Isotonic regression is a compelling approach for probability calibration, with the following advantages:
(1) When the monotonic assumption is suitable, isotonic regression can find the optimal bin edges for Brier score on the training sets, which is also known to give the convex hull in ROC analysis.
(2) The non-parametric nature avoids catastrophic model misfit.
On the other hand, isotonic regression has some drawbacks also:
(1) By predicting constant values within bins, it inevitably increases grouping loss. 
(2) When the uncalibrated model has a non-monotonic reliability diagram, isotonic regression can only give sub-optimal results (i.e. large grouping loss).
(3) While it performs well on large datasets, isotonic regression's training time and memory consumption are also high on large datasets.
(4) Isotonic regression can result in the first and last bins having full confidence (0 and 1), which can be problematic for certain datasets and evaluation metrics (e.g. log-loss). 
It is therefore common to clip the outputs from isotonic regression with a small $\epsilon$ (i.e., $0$ to $\epsilon$ and $1$ to $1 - \epsilon$).

\subsubsection*{Platt Scaling}

Platt scaling is probably one of the most widely known approaches for probability calibration, partly due to the popularity of SVMs around the year 2000 \newtext{\cite{platt2000}}.
As SVMs are optimised with hinge loss, they can only output scores on the samples based on the estimated margins.
Given that the margins are real scalars by definition, John Platt proposed to transform the scores into probability estimates with logistic regression.
Platt scaling hence has the same parameters as a univariate logistic regression model: 
a shape parameter $w \in \mathbb{R}$, and  
a location parameter $b \in \mathbb{R}$.
The predictive function is then: 
%
\begin{align}
\mathsf{g}(s; w, b) = \frac{1}{1+\exp(-w \cdot s-b)}
\end{align}
%
The parameters can be estimated by optimising the log-likelihood on the training set, so Platt scaling can be seen as optimising log-loss in the calibration context:
%
\begin{align}
\mathsf{L}(w, b) = \frac{1}{N} \sum_{i=1}^{N} \ln \Big(\sum_{j=1}^{2} - \mathsf{I}(y_i=j) \cdot \mathsf{g}(s; w, b)\Big) 
\end{align}
%

\begin{figure}[!tbp]
    \centering
    \begin{subfigure}{\textwidth}
    \centering
    % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case1_PLATT_prediction.png}
    \includegraphics[width=0.28\textwidth]{Case1_PLATT_calibration.png}
    \includegraphics[width=0.28\textwidth]{Case1_PLATT_reliability.png}
    \caption{Test case 1: under-confidence}
    \end{subfigure}
    
    
    \begin{subfigure}{\textwidth}
    \centering
    % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case2_PLATT_prediction.png}
    \includegraphics[width=0.28\textwidth]{Case2_PLATT_calibration.png}
    \includegraphics[width=0.28\textwidth]{Case2_PLATT_reliability.png}
    \caption{Test case 2: over-confidence}
    \end{subfigure}
    
    \begin{subfigure}{\textwidth}
    \centering
    % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case3_PLATT_prediction.png}
    \includegraphics[width=0.28\textwidth]{Case3_PLATT_calibration.png}
    \includegraphics[width=0.28\textwidth]{Case3_PLATT_reliability.png}
    \caption{Test case 3: MLP classifier}
    \end{subfigure}
    
    \caption{Examples of the Platt scaling approach. While it improves the under-confidence case well, it fails to do much with the over-confidence case. This is due to the fact that the sigmoid shape can not push the probabilities towards the middle hence can not fix over-confidence. Such result can also be observed with the MLP test case, where Platt scaling actually makes the level of calibration worse around several regions.}
    \label{fig:test_platt}
\end{figure}


% In addition, as ordinary logistic regression with log-loss can easily overfit to small datasets, 
Platt also included a technique to prevent overfitting and improve the generalisation of calibration, \newtext{which is introduced as one of the training schemes at the beginning of this section.}
The test results are shown in Figure~\ref{fig:test_platt}.

In general, Platt scaling is a practical calibration approach with the following advantages:
(1) As it is based on logistic regression, implementation is straightforward.
(2) The standard logistic regression has a convex loss.
The overall training process can, therefore be quite fast.
On the negative side, Platt scaling has two main drawbacks:
(1) The calibration map is restricted to a sigmoid shape, which effectively pushes probabilities away from the centre and may lead to over-confidence.
(2) By definition, the logistic regression model considers the input space to be a real scalar space. 
While such an assumption is suitable for the margins obtained from an SVM, it is less appropriate for probabilistic classifiers, as the input is bounded by the interval $[0, 1]$. 
Hence, certain transformations are required when applying Platt scaling to calibrate probabilistic classifiers, such as the logit transform.

\subsubsection*{Beta Calibration}

Beta calibration is specifically designed for probabilistic classifiers \newtext{and alleviates both drawbacks of Platt scaling \cite{pmlr-v54-kull17a,kull2017beyond}}.
While the latter can be derived from first principles by assuming that within each class the scores are normally distributed with the same variance, Beta calibration instead assumes two Beta distributions.
This gives a richer family of calibration functions with three parameters: two shape parameters $a, b \in \mathbb{R}$, and a location parameter $c \in \mathbb{R}$. 
The calibration function is then given as:
%
\begin{align}
\mathsf{g}(s; a, b, c) = \frac{1}{1+\exp \big(-a \cdot \ln s + b \cdot \ln(1-s) - c \big)}
\end{align}
%
In comparison with Platt scaling, Beta calibration is a bivariate logistic regression model, where the two features are $\ln s$ and $\ln(1-s)$ respectively.
Similar cross-validation training is also adopted as proposed in \cite{pmlr-v54-kull17a}. 

Given its close relationship to logistic regression, Beta calibration also optimises the log-loss and the objective function can be given with the log-likelihood:
%
\begin{align}
\mathsf{L}(a, b, c) = \frac{1}{N} \sum_{i=1}^{N} \ln \Big(\sum_{j=1}^{2} - \mathsf{I}(y_i=j) \cdot \mathsf{g}(s; a, b, c)\Big)
\end{align}

\begin{figure}[!htbp]
    \centering
    \begin{subfigure}{\textwidth}
    \centering
    % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case1_BETA_prediction.png}
    \includegraphics[width=0.28\textwidth]{Case1_BETA_calibration.png}
    \includegraphics[width=0.28\textwidth]{Case1_BETA_reliability.png}
    \caption{Test case 1: under-confidence}
    \end{subfigure}
    
    
    \begin{subfigure}{\textwidth}
    \centering
    % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case2_BETA_prediction.png}
    \includegraphics[width=0.28\textwidth]{Case2_BETA_calibration.png}
    \includegraphics[width=0.28\textwidth]{Case2_BETA_reliability.png}
    \caption{Test case 2: over-confidence}
    \end{subfigure}
    
    \begin{subfigure}{\textwidth}
    \centering
    % \includegraphics[width=0.28\textwidth]{figures/calibrators/Case3_BETA_prediction.png}
    \includegraphics[width=0.28\textwidth]{Case3_BETA_calibration.png}
    \includegraphics[width=0.28\textwidth]{Case3_BETA_reliability.png}
    \caption{Test case 3: MLP classifier}
    \end{subfigure}
    
    \caption{Examples of Beta calibration. The Beta approach deals with the under-confident case fairly well, as the reliability diagram follows the diagonal closely after calibration. Regarding the over-confident case, Beta calibration manages to put more corrections than the Platt scaling around the $[0, 0.5]$ region, as it pushes the reliability diagram towards the diagonal. However, it doesn't help much in $[0.5, 1.0]$ region. On the MLP case, Beta provides some improvements around the $[0.6, 1.0]$ region, and matches the reliability diagram to the diagonal. Here we can see that the reliability diagrams after calibration are almost identical for the over-confidence and under-confidence test cases. This observation is because the Beta calibration method fits the map on the logarithm of the uncalibrated probabilities, and therefore reverts the sigmoid functions of the pseudo-models in both test cases. The calibration method then finds similar solutions as the pre-sigmoid parts are both linear models on the feature. This result suggests that the Beta calibration method can effectively fix the over/under-confidence caused by a sub-optimal linear-sigmoid operation. }
    \label{fig:test_beta}
    % \todo{Hao: add two sentences why the top two reliability diagrams are the same in Fig. \ref{fig:test_beta}.}
\end{figure}

Figure~\ref{fig:test_beta} demonstrates Beta calibration on the three test cases.
The advantages of Beta calibration include:
(1) Compared with Platt scaling, it allows a richer family of calibration maps including inverse sigmoids and the identity map. 
The latter is particularly useful to prevent over-calibration and apply unnecessary adjustments to already calibrated probabilities.
(2) Like with Platt scaling, implementation is straightforward. 
(3) With the Beta assumption, the calibration map supports any two-class probabilistic classifiers, and the calibration map is  learnt from a set of functions that map from $[0, 1]$ to $[0, 1]$. 
However, Beta calibration's main drawback is that it can only model specific calibration maps, so if the original classifier is severely uncalibrated and requires a complicated calibration map, it might be preferable to choose non-parametric methods instead. %and it can obtain ill-posed results (e.g. non-monotonic calibration map) around the boundaries if no constraint is applied to the parameters.
% \todo{Hao: please reformulate last two sentences as they are cryptic to me (PF) how about now.}

\subsection{Calibration for Multi-class Classification}

We now proceed with calibration maps that can work natively with a multi-class classification task, without the need for binarisation.
%
% % \subsubsection*{Uncalibrated Classifier for a 3-class Problem}
% In this section, we only focus on the test case with the MLP classifier, since both the concepts of over-confident and under-confident are considered in a two-class setting.
%
We define a three-class test case for the purpose of examining multi-class calibration with a multi-layer perceptron (MLP).
% In this case we only consider the MLP classifier, as the concepts of under-confidence and over-confidence can be examined with two-class calibration methods.
We modify the previous synthetic dataset to add an additional class, such that all classes are equi-probable and the distribution of the feature for the instances of class 3 is Gaussian also:
\begin{align*}
    Y &\sim \text{Categorical}([\frac{1}{3}, \frac{1}{3}, \frac{1}{3}]) \\
    H &\sim \text{Categorical}(0.5) \\
    X \mid Y=1, H=1 &\sim \text{Gaussian}(-4, 960) \\
    X \mid Y=1, H=2 & \sim \text{Gaussian}(64, 1280) \\
    X \mid Y=2, H=1 & \sim \text{Gaussian}(4, 980) \\
    X \mid Y=2, H=2 & \sim \text{Gaussian}(-72, 1024) \\
    X \mid Y=3 &\sim \text{Gaussian}(0, 8) \\
\end{align*}

% On the visualisation side, because the calibration map is no longer a $1D$ function, we consider to visualise them in a class-wise simplex.
We visualise the calibration maps in the probability simplex (one for each class). 
An example can be seen in the top row of Figure~\ref{fig:TS}, where the heat maps indicate the change of probability for each class after calibration.
For the figure on the left, each point within the simplex represents an uncalibrated probability vector, a positive value (i.e., red colour) on that point indicates that the calibration map increases the probability value of class 1 in the vector and a negative value (i.e., blue colour) shows that the probability value on class 1 is reduced.
The white line indicates where the probability values for class 1 remain (almost) unchanged.
Class 2 and class 3 calibration maps are also depicted.
% Regarding the reliability diagram, we select the class-wise reliability diagram, and examples can be seen at the bottom of Figure~\ref{fig:TS}.
The bottom row of each figure shows the class-wise reliability diagrams. 

\subsubsection*{Temperature Scaling}

\begin{figure}[!tbp]
    \centering
    %\includegraphics[width=0.85\textwidth]{figures/calibrators/TS_prediction.png}
    \includegraphics[width=0.95\textwidth]{TS_calibration.png}
    \includegraphics[width=0.85\textwidth]{TS_reliability.png}
    \caption{MLP classifier with Temperature scaling (top: class-wise calibration map, bottom: class-wise reliability diagram). While Temperature scaling manages to improve the reliability diagram around the $[0.1, 0.4]$ region for classes 1 and 2, we can see it actually makes things worse elsewhere. As the calibration maps show, Temperature scaling applies the same calibration map to all three classes despite them having different class-wise reliability diagrams, which is the main reason for the sub-optimal results.}
    \label{fig:TS}
\end{figure}

Temperature scaling has become one of the default approaches to provide better-calibrated probabilities, \newtext{particularly in deep learning research \cite{hinton2015distilling,guo2017}}.  
Instead of simply applying the softmax operation at the last layer to obtain a probability vector on the classes, Temperature scaling assumes a single temperature parameter $t \in \mathbb{R}$ and applies a linear operation before the softmax.
Denoting $\mathbf{z} = [z_1, \dots, z_K] \in \mathbb{R}^K$ as the $K$-dimensional real vector before softmax, the probability output after Temperature scaling is given as:
%
\begin{align}
\mathsf{c}_{j}(\mathbf{z}; t) = \frac{\exp\big(-z_j / t\big)}{\sum_{j=1}^{K}\exp\big(-z_j / t\big)}
\end{align}
%
Therefore, conventional softmax can be seen as the case of scaling with a fixed temperature of $t=1$.

If we want to apply Temperature scaling to a generic probabilistic model where $z$ is not accessible, we can also use the $\mathsf{logit}$ transform on the uncalibrated probability vector to obtain a real vector:
%
\begin{align*}
    z_j &= \mathsf{logit}_j (\mathbf{s}) \\
        &= \ln\frac{s_j}{s_K}
\end{align*}
%
Here, $K$ is selected as the reference class to compute the probability ratio with other classes.
The parameter is also normally estimated with the log-loss, and the objective function is given as:
%
\begin{align}
\mathsf{L}(t) = \frac{1}{N} \sum_{i=1}^{N} \ln \Big(\sum_{j=1}^{K} - \mathsf{I}(y_i=j) \cdot \mathsf{g}_{j}(\mathbf{z}_i; t)\Big)   
\end{align}

Figure~\ref{fig:TS} gives the results on the MLP test case.
The most distinctive characteristic of Temperature scaling is that it only has a single parameter, which can be seen as both an advantage and a disadvantage.
On the positive side, a single parameter restricts the space of calibration maps and can prevent overfitting for small datasets with many classes. 
On the negative side, Temperature scaling can be sub-optimal when the function space of the calibration maps does not include the right reliability diagram.  

\subsubsection*{Vector Scaling}

\begin{figure}[!tbp]
    \centering
    % \includegraphics[width=0.85\textwidth]{figures/calibrators/VS_prediction.png}
    \includegraphics[width=0.95\textwidth]{VS_calibration.png}
    \includegraphics[width=0.85\textwidth]{VS_reliability.png}
    \caption{Class-wise calibration maps and reliability diagrams for the MLP classifier with Vector scaling. The most obvious change from Temperature scaling is that now the calibration maps are different for each class. However, the calibration maps still have a circular shape as Vector scaling only adjusts one dimension of the logit vector for each class. As a result, the reliability diagram is close to the ones of Temperature scaling. Some minor improvements can be seen with class 3, where Vector scaling does not make it quite as bad as for Temperature scaling. }
    \label{fig:VS}
\end{figure}

Where Temperature scaling only has a single parameter across all classes, it is natural to extend the parameters to support a richer form of calibration maps.
Vector scaling \newtext{\cite{guo2017}} allows a different temperature for each class, denoted as $\mathbf{w} \in \mathbb{R}^{K}$, as well as adding a set of intercept parameters $\mathbf{b} \in \mathbb{R}^{K}$ for the $K$ classes.
The predictive function is given as ($\mathbf{z}$ can also be obtained with the logit transform for generic probability classifier, as in Temperature scaling):
%
\begin{align}
\mathsf{c}_{j}(\mathbf{z}; \mathbf{w}) = \frac{\exp\big(-w_j \cdot z_j -b_j\big)}{\sum_{j=1}^{K}\exp\big(-w_j \cdot z_j - b_j\big)}
\end{align}
%
And the objective function to optimise log-likelihood is similar to the one for Temperature scaling, but with more parameters:
%
\begin{align}
\mathsf{L}(\mathbf{w}, \mathbf{b})= \frac{1}{N} \sum_{i=1}^{N} \ln \Big(\sum_{j=1}^{K} - \mathsf{I}(y_i=j) \cdot \mathsf{g}_{j}(\mathbf{z}_i; \mathbf{w}, \mathbf{b})\Big)
\end{align}

The test result is given in Figure~\ref{fig:VS}.
Vector scaling can be seen as a middle point between the quite restrictive Temperature scaling and the general approach of Matrix scaling discussed below. 
Hence it balances the risk of overfitting and the richness of available calibration maps. 

\subsubsection*{Matrix Scaling}

Matrix scaling \newtext{\cite{guo2017}} removes all the parameter constraints on Temperature scaling and Vector scaling.
Similar to a fully connected layer, it has a matrix parameter $(\mathbf{w}_1, \cdots, \mathbf{w}_K), \mathbf{w}_j \in \mathbb{R}^K$ together with the intercept parameter $\mathbf{b} \in \mathbb{R}^{K}$.
The predictive function is ($\mathbf{z}$ can also be obtained with the logit transform, as in Temperature scaling):
%
\begin{align}
\mathsf{c}_{j}(\mathbf{z}; \mathbf{w}_1, \dots, \mathbf{w}_{K}, \mathbf{b}) = \frac{\exp\big(-\mathbf{w}_j^T \mathbf{z} - b_j\big)}{\sum_{j=1}^{K}\exp\big(-\mathbf{w}_j^T \mathbf{z} - b_j\big)}
\end{align}
%
and the objective function is:
%
\begin{align}
\mathsf{L}(\mathbf{w}_1, \dots, \mathbf{w}_K, \mathbf{b})= \frac{1}{N} \sum_{i=1}^{N} \ln \Big(\sum_{j=1}^{K} - \mathsf{I}(y_i=j) \cdot \mathsf{g}_{j}(\mathbf{z}_i; \mathbf{w}_1, \dots, \mathbf{w}_K, \mathbf{b})\Big)
\end{align}

As indicated in Figure~\ref{fig:MS}, Matrix scaling can support a broader family of calibration maps than Vector scaling and Temperature scaling, but may be vulnerable to overfitting as it can be seen as another fully connected layer.  

\begin{figure}[!tbp]
    \centering
    % \includegraphics[width=0.85\textwidth]{figures/calibrators/MS_prediction.png}
    \includegraphics[width=0.95\textwidth]{MS_calibration.png}
    \includegraphics[width=0.85\textwidth]{MS_reliability.png}
    \caption{Class-wise calibration maps and reliability diagrams for the MLP classifier with Matrix scaling. As Matrix scaling is capable of providing fully linear adjustments on the logits for each class, we can see the class-wise calibration map no longer has the circular shape. While there are still minor improvements on the reliability diagram of class 1 and class 2, class 3 has gained a significant improvement.}
    \label{fig:MS}
\end{figure}

\subsubsection*{Dirichlet Calibration}

Dirichlet calibration is the multi-class extension of Beta calibration \cite{kull2019}.
Assuming Dirichlet distributions for the predicted probability vectors within each class, Dirichlet calibration is determined by a set of coefficient vectors $(\mathbf{w}_1, \cdots, \mathbf{w}_K), \mathbf{w}_j \in \mathbb{R}^K$, and a set of intercepts $\mathbf{b} \in \mathbb{R}^{K}$. 
The calibrated probability on the $j\text{-th}$ class is obtained as:
%
\begin{align}
\mathsf{g}_{j}(\mathbf{s}; \mathbf{w}_1, \dots, \mathbf{w}_{K}, \mathbf{b}) = \frac{\exp(-b_j - \mathbf{w}_j^T \ln \mathbf{s})}{\sum_{j=1}^{K}\exp(-b_j-\mathbf{w}_j^T \ln \mathbf{s})}
\end{align}
%
This function can be seen as a $K$-dimensional logistic regression on the log-probabilities (i.e., the sufficient statistics of the Dirichlet distribution). 
Therefore, to apply Dirichlet calibration to a deep neural network, one can first obtain a probability vector using the softmax function, then apply Dirichlet calibration as with other probabilistic classifiers.
%
The objective function is:
%
\begin{align}
\mathsf{L}(\mathbf{w}_1, \dots, \mathbf{w}_K, \mathbf{b})= \frac{1}{N} \sum_{i=1}^{N} \ln \Big(\sum_{j=1}^{K} - \mathsf{I}(y_i=j) \cdot \mathsf{g}_{j}(\mathbf{s}_i; \mathbf{w}_1, \dots, \mathbf{w}_K, \mathbf{b})\Big)
\end{align}

The test results are given in Figure~\ref{fig:Dcal}.
Similar to Beta calibration, one of the advantages of Dirichlet calibration is that it also supports the identity map, so it can also prevent over-adjusting calibrated results.
% Following the derivation, the Dirichlet can also be written with an interpretable canonical parameter form.
As the number of parameters is similar to that of Matrix scaling, the Dirichlet calibration can also overfit on small datasets.
The authors propose the ODIR (Off-Diagonal and Intercept Regularisation) approach to address this issue further and report various performance improvements in their experiments.



\begin{figure}[!tbp]
    \centering
    % \includegraphics[width=0.85\textwidth]{figures/calibrators/DIR_prediction.png}
    \includegraphics[width=0.95\textwidth]{DIR_calibration.png}
    \includegraphics[width=0.85\textwidth]{DIR_reliability.png}
    \caption{Class-wise calibration maps and reliability diagrams for the MLP classifier with Dirichlet calibration. The overall results on the class-wise reliability diagrams are close to those obtained with Matrix scaling. 
    % This is understandable considering the similarity on their mathematical forms. 
    The major differences are seen in the calibration maps, where we can clearly observe a local region for the changes on class 3. Importantly, this region for the Dirichlet calibration approach doesn't cover the area where the predicted probability of class 3 is close to 1. This is more reasonable compared with Matrix scaling, as both the Bayes-optimal predictions and the MLP predictions for class 3 are capped around 0.8.}
    \label{fig:Dcal}
\end{figure}

% \begin{figure}[!tbp]
%     \centering
%     \includegraphics[width=0.85\textwidth]{figures/calibrators/all_prediction.png}
%     \includegraphics[width=0.85\textwidth]{figures/calibrators/all_reliability.png}
%     \caption{A comparison of all calibrators on the binary synthetic dataset.}
%    \label{fig:all}
%\end{figure}

%\begin{figure}[!tbp]
%    \centering
%    \includegraphics[width=0.85\textwidth]{figures/calibrators/all3_prediction.png}
%    \includegraphics[width=0.85\textwidth]{figures/calibrators/all3_reliability.png}
%    \caption{A comparison of all calibrators on the ternary synthetic dataset.}
%    \label{fig:all_3}
%\end{figure}

% \subsection{Calibration methods by extension}

% At the end of this section we briefly mention related approaches that can improve the level of probability calibration in a classification setting, as well as specific applications in areas such as computer vision and natural language processing.
% While we have demonstrated generic post-hoc calibrators that can work with any probabilistic classifier without extensive training setup and specific domain knowledge (i.e. DNN architecture), in this section we will address some methods that come with such additional requirements.
% The methods covered in this section can be described with the following categories: (1) methods that can improve calibration during training time, (2) methods that require a composite training scheme, and (3) methods that work on uncertainty quantification tasks related to classifier probability calibration. 

% \subsubsection{Binary probability calibration, class-wise calibration and confidence calibration}
% Being one of most basic and interpretable definition of calibration, 
\newtext{
\subsection{Extended methods for post-hoc classifier calibration}
\label{sec:cal:extension}
%While some standard binary and multi-class post-hoc calibration methods are introduced above, the research area has recently drawn more attention as the industry is adopting ML systems into production.
In this section we discuss more recent work extending the standard calibration methods discussed above. 

\citet{leathart2017} aim to build calibration maps locally instead of a global calibration map and proposes using modified logistic model trees to build an ensemble calibration method. A decision tree is learnt to separate the original feature space into multiple regions, where a local calibrator can then be estimated using the corresponding outputs and labels.
\citet{kumar2019} propose a combined approach of scaling and binning methods to achieve better calibration with smaller calibration sets. Instead of calculating the label frequency in binning methods, the authors show that using the average value of a pre-fit continuous calibration map gives better calibration. The authors also indicate that a debiased estimator can provide better calibration error in sample complexity.
\citet{wang2019calibrating} discuss how to build flexible univariate non-decreasing calibration maps from shape-restricted polynomial regression models. The resulting method provides a useful alternative when methods like Plat scaling and Beta calibration cannot approximate the actual reliability diagram.
\citet{wenger2020} investigate non-parametric post-hoc approaches that can support richer forms of calibration map for a multi-class setting.
The idea is to employ the framework of Gaussian processes and model the calibration map as latent distribution of functions.
The family of calibration maps can thus be richer with the selection of suitable kernels.
\citet{zhang2020mix} propose an approach to build an ensemble of base calibrators, which can improve the capacity of the calibration maps while preserving the accuracy.
The authors also adapt kernel density estimation as an alternative approach to evaluating calibration error. 
\citet{ma2021meta} consider the confidence calibration setting and propose to improve a calibration map with a ranking model. The authors demonstrate that the ranking model can be used to maintain the performance of the uncalibrated classifier in terms of precision and false positive rate.
\citet{patel2021multiclass} tackle the issue of applying class-wise binning calibrators to a multi-class setting. An iterative update method is provided to adjust the bin edges to better calibration, and a sample-sharing approach among similar classes is also introduced for better sample efficiency. 

\subsection{Methods that can improve calibration during training time}
\label{sec:cal:training}

%So far, we have been mainly focusing on post-hoc calibration approaches.
While post-hoc calibration can be applied to most existing classifiers, it is of practical interest to train well-calibrated models in the first place.
Here we briefly mention some training-time calibration methods.

\citet{kumar2018} consider a regularisation approach with kernel mean embedding.
The idea is to add a differentiable regularisation term concerning the goodness of calibration, where the kernel mean of the scores is calculated as an approximation of the calibration error. 
The overall objective function allows the model to achieve better calibration during the training phase.
\citet{thulasidasan2019mixup} show that the Mixup strategy can improve the calibration level when introduced during the training phase.
Vicinal points are created by combining existing data points and labels, and then added to the training set.
The authors suggest that the improvement in calibration is due to the augmentation effect and label smoothing effect, both from the mixup process and act as a form of regularisation.
\citet{kristiadi2020being} consider a Bayesian approach where a Gaussian approximation distribution is fitted to the last layer's weights of a ReLu network.
The authors demonstrated that the method could reduce the over-confidence problem in a classification setting, particularly on data points not commonly seen in the original training set.
\citet{wen2020batchensemble} propose an efficient ensemble approach that can train multiple deep networks with lower computational and memory costs.
The authors show that the obtained ensemble achieves better calibration on out-of-distribution samples at test time.

Other than deep networks, some recent work achieves better calibration on Bayesian nonparametric methods.
\citet{milios2018} propose an alternative approach to train Gaussian Processes for classification tasks.
While the traditional GP classifier relies on sigmoid or probit link functions and requires suitable approximated inference schemes to ensure good performance, the authors propose a modified Dirichlet link function to ensure the level of calibration as well as scalability.
\citet{tran2019calibrating} demonstrate that convolution Gaussian process classifiers can be miscalibrated, and propose a solution to mitigate the issue.

% \subsubsection{Methods that require a composite fitting procedure}

% While we have introduced some general calibration methods in detail, some recent work has introduced methods that can improve calibration in a certain sense (i.e. from a binary, class-wise or confidence perspective), with the cost of a more composite fitting procedure.
% Given the diversity of these fitting procedures, here we provide a brief introduction to some of the methods so the readers can further refer to the papers for implementation details. 


\subsection{Methods for probability calibration for other predictive settings}
\label{sec:cal:other}

% Although we have discussed probability calibration in a classification setting, 
The concept of calibration can be naturally generalised to predictive settings other than classification.
The most straightforward extension is the calibration of regression outputs.
As in the classification scenario, there are multiple definitions of calibration for regression models.
The standard definition of calibration comes from the field of quantile regression \cite{koenker2001quantile}, where being calibrated means that the predicted quantile matches the marginal distribution of the target variable.
As in the case of classification, there are methods designed for training calibrated quantile regression as well as post-hoc approaches that calibrate pre-trained models.
\citet{fasiolo2020fast} provide an approach to train generalised additive regression models with calibrated quantiles.
\citet{cui2020calibrated} propose an approach to train deep regression models with better-calibrated quantiles, where the model parameter is first fit with log-loss and then updated with a loss based on the maximal mean discrepancy \cite{gretton2012kernel}.
For the post-hoc setting, \citet{kuleshov2018} point out that deep regression models' quantiles can be calibrated with binary calibrators such as isotonic regression and yield better performance on downstream tasks such as reinforcement learning.
\citet{chung2021beyond} introduce some modified loss functions to train quantile calibrators with specific emphases, such as balancing between calibration and sharpness. 

Regarding the definition of calibration, \citet{pmlr-v97-song19a} propose a stronger notion of calibration in regression, where the local conditional distribution is required to be calibrated instead of the global quantile. 
The authors 
% refer to this definition as distribution-calibrated for regression models and 
show that being distribution-calibrated in this sense implies being quantile-calibrated.
A post-hoc approach based on the Gaussian process is also introduced, where the GP models a distribution of Beta calibrators conditioning on the original regression outputs.
\citet{kuleshov2022calibrated} consider achieving post-hoc distribution calibration by learning a lower dimensional representation of the (uncalibrated) local distributions, and the post-hoc calibrators can then be built with density estimators on these representations and the target values, which avoids the costs of distributional kernels and sparse variational inference.
\citet{sahoo3reliable} propose the definition of threshold calibration for regression models, which is a stronger notion of calibration than being quantile-calibrated and weaker than the distribution-calibrated definition.
Instead of asking for calibration on a marginal quantile or local distribution level, the proposed definition requires the model to be calibrated on a group of distributions that satisfy a given threshold condition, which ensures optimal decision-making when a threshold is put on the regression outputs.

Calibration of structured outputs, such as sequential outputs, is also of interest for application domains such as natural language processing and time-series modelling. 
\citet{kuleshov2015calibrated} propose approaches to simplify the structured output to a two-class problem and employ a well-calibrated binary classifier to improve the calibration level.
On the information-retrieval side, the traditional precision-recall curve is not sufficiently similar to a ROC curve to allow a similar calibration property.
In contrast, the precision-recall-gain curve proposed by \citet{flach2015} can be seen as a proper generalisation of ROC curve obtained by replacing weighted accuracy with F-score.


Conformal prediction \cite{vovk2005algorithmic,romano2019conformalized,angelopoulos2021gentle} is another area closely related to the topic of probability calibration.
For classification, conformal prediction aims to predict a set of labels that has a probability of $1 - \alpha$ that includes the true label, where $\alpha$ is a user-defined significance level.
Therefore, we can see the conformal prediction for classifiers as an alternative definition of calibration to label probability calibration. That is, instead of requiring the probability to be accurate on the label distributions, conformal prediction wants to ensure the calibration on a variable set of labels that are exactly calibrated on the given significance level.
One of the approaches to construct a conformal classifier is to use a Venn predictor \cite{vovk2003self,vovk2012venn,johansson2018}.
The framework makes use of the Venn taxonomy to define subsets of the original label space, and requires a classifier to make predictions about each element in the subset.
The final conformal prediction can then be calculated using these predictions.

\subsection{Methods designed for other research fields and applications}
\label{sec:cal:app}

The notion of calibration can also be generalised to other areas where uncertainty quantification is of interest. rRecent work has started to explore other topics in statistics, machine learning and artificial intelligence related to calibration.
Here we briefly introduce some of them. 
A comprehensive analysis of these works is left as future work.
\citet{pleiss2017fairness} draw a link between the level of calibration and the evaluation of classifier fairness.
\citet{CobbGal2018Loss} propose an approach to modify the lower bound of approximate Bayesian inference so that the final objective function can be calibrated according to a given decision loss. 
\citet{liu2018generalized} adopt calibrated deep models to improve zero-shot learning.
\citet{menon2018loss} consider the calibration problem for an anomaly detection setup.
\citet{ghandeharioun2019characterizing} consider uncertainty and calibration as a tool to improve explainability for computer vision tasks. 
And \citet{liu2019accurate} adopt a calibration procedure to achieve better posterior distributions for a Bayesian non-parametric ensemble model.
\citet{ding2021local} consider the problem of improving calibration for semantic segmentation.
\citet{guillory2021predicting,jiang2021assessing} show that calibrated classifier can be used to estimate the model performance on OOD test sets. 
}


% \cite{kuleshov2018} focus on the calibration of quantile regression approaches, and propose to use binary post-hoc calibrators to improve various deep regression models.

%\cite{song2019} proposes a stronger definition of calibration for regression tasks, which requires the output to be calibrated on a distribution level instead of a quantile level, a GP-based approach is also given to improve such calibration.

% \cite{widmann2019} gives a statistical test framework for calibration in a multi-class setting.

% {\color{red}
% I will add some citations here that may be useful as well

% \cite{Krishnan2020}
% \begin{itemize}
%     \item Uncertainty under distribution shift between training and test
%     \item Propose a new differentiable accuracy versus uncertainty calibration (AvUC) loss function
%     \item Can be applied as a post-hoc calibration method
%     \item Intended to deal with out-of-distribution in the training data manifold
%     \item Categorise calibration methods into: (1) post-processing calibration (eg. Temperature scaling and dirichlet calibration), (2) training with data augmentation, (3) probabilistic methods with respect to the model parameters.
%     \item Contribution: (1) differentiable proxy for Accuracy versus Uncertainty measure (not sure if this measure is also a contribution), (2) evaluation of results under distribution shift, (3) propose post-hoc calibration with Temperature scaling, (4) comparison with stae-of-the-art methods (need to see this yet).
%     \item Evaluation metrics: conf-ECE, expected uncertainty calibration error (UCE) [41], NLL, Brier score, conditional probabilities $p(accurate|certain)$ and $p(uncertain|inaccurate)$ [39], AUROC, and AUPR (not gain curves).
%     \item Accuracy vs uncertainty (AvU) uses a confusion matrix to compute the "accuracy" of "certainty". Basically, constructing a confusion matrix of correctly predicted vs certain predictions if a threshold is well defined, and then computing the Accuracy on that confusion matrix.
%     \item Accuracy vs uncertainty calibration (AvUC) loss: In order to make the previous metric differentiable, a surrogate function is defined by defining a fixed threshold to determine what is considered certain, and an hyperbolic tangent of the certainty is used to approximate a similar behaviour than AvU in ideal conditions.
%     \item AvUC loss is used as an additional term to the original loss, and intended to be used as a regularization factor.
%     \item In the example with loss-calibrated evidence lower bound (ELBO), the first epochs are trained ONLY with ELBO, later the AvUC term is introduced with an scaling hyperparameter Beta. The required uncertainty "threshold is obtained from the average of predictive uncertainty mean for accurate and inaccurate predictions on the training data from initial epochs".
%     \item Question: The method is trying to calibrate the probabilistic outputs, but uses a fixed threshold to define what is certain, and what is not... This is very simplistic in my view, and it should show signs of poor classwise calibration.
%     \item Experiments compare several sota networks with Temperature scaling, deep-ensembles, Monte Carlo dropout, Mean-field stochastic variational inference, Temperature scaling on SVI, and Radial Bayesian neural network.
%     \item All methods evaluated in 16 types of image corruption at 5 level of intensities (80 variations).
% \end{itemize}
% }

% \subsection{The toy dataset (feature space, generative view)}
% For better illustration, we adopt a dataset and a set of visualisations.
% \begin{figure}
%     \centering
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/toy.png}\hfill
%     \includegraphics[width=0.62\textwidth]{figures/calibrators/toy_conditional.png}
% \end{figure}

% \subsection{The toy dataset (feature space, discriminative view)}

% As we know the data distribution, we can calculate the Bayes-optimal scoring model, that is: 
% \begin{align*}
% s(x) = P(Y=1 | X=x)
% \end{align*}

% \subsection{The distribution of predictions}
% We can further calculate the distribution of $s(x)$.
% \begin{figure}
%     \centering
%     \includegraphics[width=0.33\textwidth]{figures/calibrators/bayes_opt.png}
%     \caption{Distribution of scores }
% \end{figure}

% \begin{figure}
% \centering
% \includegraphics[width=0.62\textwidth]{figures/calibrators/bo_conditional.png}
% \caption{Probability distribution of scores per class}
% \end{figure}


% \subsection{Reliability diagram}
% As well as $P\Big(Y=1 | s(x)\Big)$ (reliability diagram).
% Since the model is Bayes-optimal, we have a perfect reliability diagram.
% \begin{figure}
%     \centering
%     \includegraphics[width=0.33\textwidth]{figures/calibrators/bo_score.png}
%     \includegraphics[width=0.27\textwidth]{figures/calibrators/bo_rg.png}
%     \caption{Joint probability distribution of the scores, and correspoinding reliability diagram.}
% \end{figure}

% \subsection{With a classifier}
% Now if we train a neural network with some samples.
% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/mlp.png}
% \includegraphics[width=0.28\textwidth]{figures/calibrators/mlp_rel.png}
% \caption{Neural network's predicted scores in the input space, and corresponding reliability diagram.}
% \end{figure}

% \subsection{Post-hoc calibrators}
% This is where we need post-hoc calibrators.

% \subsection{Post-hoc calibrators (scaling view)}

% \begin{itemize}
%     \item It is also common to re-scale a real vector output into calibrated probability vector space.  (e.g. SVM margins, final layer of a neural network) 
    
%     \item Since a real vector and a probability vector can be transformed into each other through link function and inverse link function (e.g. soft-max and logit transform), for later slides we will use the probability vector view by default. 

% \end{itemize}



% \begin{figure}
%     \centering
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/mlp_map.png}
%     \includegraphics[width=0.28\textwidth]{figures/calibrators/mlp_map_sca.png}
%     \caption{Example of original and scaled scores.}
% \end{figure}

% \section{Scaling v.s. Probability calibrator}

% \subsection{Scaling v.s. Probability calibrator}{
% \textbf{Scaling}: designed to re-scale a function output into probability vector space and match with target observations. (e.g. SVM margins, final layer of a neural network, latent functions modelled by a Gaussian process)

%   \begin{figure}
%       \centering
%       \includegraphics[width=0.28\textwidth]{figures/calibrators/svm_margin.png}
%       \includegraphics[width=0.1\textwidth]{figures/calibrators/right_arrow.png}
%       \includegraphics[width=0.28\textwidth]{figures/calibrators/svm_after.png}
%   \end{figure}

%}

% \subsection{Scaling v.s. Probability calibrator}{
% \textbf{Probability calibrator}: designed to match a probability output with target observations.

 %   \begin{figure}
   %    \centering
  %     \includegraphics[width=0.65\textwidth]{figures/calibrators/p_x_g_y_model.png} 
    %   \includegraphics[width=0.05\textwidth]{figures/calibrators/down_arrow.png}
   %    \includegraphics[width=0.65\textwidth]{figures/calibrators/p_x_g_y_hat.png}
  % \end{figure}

%}

% \subsection{Scaling v.s. Probability calibrator}{
% \textbf{Probability calibrator}: designed to match a probability output with target observations.

%    \begin{figure}
%        \centering
%        \includegraphics[width=0.65\textwidth]{figures/calibrators/simplex_model.png} 
%        \includegraphics[width=0.05\textwidth]{figures/calibrators/down_arrow.png}
%        \includegraphics[width=0.65\textwidth]{figures/calibrators/simplex_hat.png}
%    \end{figure}

% }

%\section{Categories of Calibrators}

%\subsection{Categories of Calibrators}{
%     Scaling approaches v.s. probability calibrator 
%     Parametric approaches v.s. non-parametric approaches 
%     Generative approaches v.s. discriminative approaches 
%}

%\subsection{Scaling approaches v.s. probability calibrator}{
%    \textbf{Scaling approaches}: designed to re-scale a function output into probability vector space and match with target observations.
    
%    \begin{figure}
%        \centering
%        \includegraphics[width=0.5\textwidth]{figures/calibrators/f_x.png} 
%        \includegraphics[width=0.15\textwidth]{figures/calibrators/down_arrow.png}
%        \includegraphics[width=0.5\textwidth]{figures/calibrators/p_x.png}
%    \end{figure}
%}

%\subsection{Scaling approaches v.s. probability calibrator}{
%    \textbf{Probability calibrator}: designed to match a probability output with target observations.
    
%    \begin{figure}
%        \centering
%        \includegraphics[width=0.5\textwidth]{figures/calibrators/p_x.png} 
%        \includegraphics[width=0.15\textwidth]{figures/calibrators/down_arrow.png}
%        \includegraphics[width=0.5\textwidth]{figures/calibrators/p_hat_x.png}
%    \end{figure}
%}

%\subsection{Scaling approaches v.s. probability calibrator}{
%The differences between scaling approaches and probability calibrators mainly come from their motivations.
%For instance, some scaling approaches are proposed for non-probabilistic models such as SVM.
%In practice, the application of both types are exchangeable. 
%We can re-scale a function value into probability estimation, and apply probability calibrators.
%We can also use inverse link function to turn a probability estimation into a real number, and apply scaling approaches.
%}

% \subsection{Parametric approaches v.s. non-parametric approaches}{}

% \subsection{Generative approaches v.s. discriminative approaches}{}

% \section{Calibrators}

% \subsection{Binary approaches}

% \begin{itemize}
%     \item \cite{naeini2016}
%     \item \cite{platt2000}
%     \item \cite{kull2017}
% \end{itemize}

% \subsubsection{Empirical Binning}

% While being simple and effective, binning approaches can only give discrete outputs.

% you can trust the probabilities, but it doesn't give many.

% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/emp_map_1000_10.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/emp_rel_1000_10.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/emp_1000_10.png}
% \caption{Empirical binning with 10 bins}
% \end{figure}

% A suitable number of bins / binning algorithm is important to get good results. 

% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/emp_map_1000_100.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/emp_rel_1000_100.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/emp_1000_100.png}
% \caption{Empirical binning with 100 bins}
% \end{figure}

% \textbf{Parameters:} 
% \hspace{24pt}Bins: $\{\mathbb{B}_1, \dots, \mathbb{B}_M \}, \mathbb{B}_j \subset [0, 1]$  
% \hspace{24pt}Bin averages:  $\mathbf{a}=(a_1,\dots,a_{M})$, $a_j \in \{0, 1\}$
% \vspace{12pt}
% \textbf{Predictive Function:} 
% \hspace{24pt}$c(p; \mathbb{B}_1, \dots, \mathbb{B}_M, \mathbf{a}) = \sum_{j=1}^{M} \mathbb{I}(p\in \mathbb{B}_j) \cdot a_j$ 
% \vspace{12pt}
% \textbf{Objective Function:} 
% \hspace{24pt} $\mathbb{L}(\mathbf{a}) = \sum_{j=1}^{M} \Big | \frac{\sum_{i=1}^{N} \mathbb{I}(p_i \in B_j) \cdot y_i}{|\mathbb{B}_j|} - a_j \Big|$ 


% \subsubsection{Isotonic Regression}

% With the ROC-convex hull method, isotonic regression can give good calibration performance with automatic binning and interpolation.
% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/iso_map_100.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/iso_rel_100.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/iso_100.png}
% \caption{Isotonic regression with 100 data points}
% \end{figure}

% More data points are beneficial for isotonic regression, but the monotonicity assumption might not be suitable for certain datasets / base models.
% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/iso_map_10000.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/iso_rel_10000.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/iso_10000.png}
% \caption{Isotonic regression with 10,000 data points}
% \end{figure}

% \textbf{Parameters:} 
% \hspace{24pt}Bin edges: $\mathbf{b}=(b_1,\dots,b_M)$, $b_j \in \{0, 1\}, b_j < b_{j+1}$  
% \hspace{24pt}Edge values:  $\mathbf{v}=(v_1,\dots,v_{M})$, $ v_j \in [0, 1], v_j \leq v_{j+1}$
% \vspace{12pt}
% \textbf{Predictive Function:} 
% \hspace{24pt}$c(p; \mathbf{b}, \mathbf{v}) = \frac{1}{\sum_{j=1}^{M-1} \mathbb{I}(p\geq b_j)\cdot\mathbb{I}(p\leq b_{j+1})}\sum_{j=1}^{M-1} \mathbb{I}(p\geq b_j)\cdot\mathbb{I}(p<b_{j+1}) \cdot \Big(v_j + \frac{p-b_j}{b_{j+1}-b_j}(v_{j+1} - v_j)\Big) $ 
% \vspace{12pt}
% \textbf{Objective Function:} 
% \hspace{24pt} $\mathbb{L}(\mathbf{b}, \mathbf{v}) = \frac{1}{N} \sum_{i=1}^{N}\Big( c(p_i; \mathbf{b}, \mathbf{v}) - y_i\Big)^2$ 

% \subsubsection{Platt Scaling}

% The ONE that allows SVMs to output probabilities.

% \begin{figure}
%        \centering
%        \includegraphics[width=0.4\textwidth]{figures/calibrators/svm_margin.png}\hfill
%        \includegraphics[width=0.1\textwidth]{figures/calibrators/right_arrow.png}\hfill
%        \includegraphics[width=0.4\textwidth]{figures/calibrators/svm_after.png}
%    \end{figure}

% We can also use it to calibrate from the final layer of the MLP classifier.
% \begin{figure}
%        \centering
%        \includegraphics[width=0.28\textwidth]{figures/calibrators/platt_map.png}\hfill
%        \includegraphics[width=0.28\textwidth]{figures/calibrators/platt_rel.png}\hfill
%        \includegraphics[width=0.28\textwidth]{figures/calibrators/platt.png}
% \end{figure}

% \textbf{Parameters:} 
% \hspace{24pt}Slope: $w \in \mathbb{R}$  
% \hspace{24pt}Intercept: $b \in \mathbb{R}$ 
% \vspace{12pt}
% \textbf{Predictive Function:} 
% \hspace{24pt}$c(p; w, b) = \frac{1}{1+\exp(-w \cdot p-b)}$ 
% \vspace{12pt}
% \textbf{Objective Function:} 
% \hspace{24pt} $\mathbb{L}(w, b) = \frac{1}{N} \sum_{i=1}^{N} \ln \Big(\sum_{j=1}^{2} - \mathbb{I}(y_i=j) \cdot c(p; w, b)\Big) $ 

% \subsubsection{Beta Calibration}

% While Platt scaling can be derived with conditional Gaussian distribution with shared variance, probabilities are on a finite support hence Gaussian is less suitable.

% With a Beta assumption, we can get calibration maps that get beyond sigmoid.
% \begin{figure}
% \centering
% \includegraphics[width=0.45\textwidth]{figures/calibrators/beta_list.png}
%\end{figure}

% As well as a identity map if the original model is already calibrated, or no better calibration map can be modelled.
% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/beta_3_map.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/beta_3_rel.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/beta_3.png}
% \end{figure}

% \textbf{Parameters:} 
% \hspace{24pt}Slope 1: $a \in \mathbb{R}$ 
% \hspace{24pt}Slope 2: $b \in \mathbb{R}$ 
% \hspace{24pt}Intercept: $c \in \mathbb{R}$ 
% \vspace{12pt}
% \textbf{Predictive Function:} 
% \hspace{24pt}$c(p; a, b, c) = \frac{1}{1+\exp\big(-a \cdot \ln p - b \cdot \ln (1-p) - c \big)}$ 
% \vspace{12pt}
% \textbf{Objective Function:} 
% \hspace{24pt} $\mathbb{L}(a, b, c) = \frac{1}{N} \sum_{i=1}^{N} \ln \Big(\sum_{j=1}^{2} - % \mathbb{I}(y_i=j) \cdot c(p; a, b, c)\Big) $ 

% \subsection{Multi-class approaches}


% \begin{table}[htpb!]
%     \centering
%     \begin{tabularx}{\linewidth}{L|l|l}
%         \toprule
%         \textbf{Calibration method} & \textbf{Details} & \textbf{} \\
%         \midrule
%         Platt's scaling \cite{platt1999}       &  Multiclass & Scaling \\
%         \midrule
%         Isotonic regression \cite{chakravarti1989}   &  & Non-parametric\\
%         \midrule
%         Nearly-Isotonic regression \cite{chakravarti1989}   &  & Non-parametric\\
%         \midrule
%         Size binning     & & \\
%         \midrule
%         Width binning     & & \\
%         \midrule
%         Binning averaging \cite{zadrozny2001}     & & \\
%         \midrule
%         Similarity binning averaging \cite{bella2009} & & \\
%         \midrule
%         Bayesian binning into quantiles \cite{naeini2015} & & \\
%         \midrule
%         Probability Calibration Trees \cite{leathart2017} & & \\
%         \midrule
%         Calibration of nested dichotomies \cite{leathart2018} & & \\
%         \midrule
%         Temporal probability calibration \cite{leathart2020} & & \\
%         \midrule
%         Venn predictors for probability estimation trees \cite{johansson2018} & &  \\
%         \midrule
%         Ensemble of Near Isotonic Regression \cite{Naeini2017} & Binary & \\
%         \midrule
%         Temperature scaling \cite{guo2017}  & Multiclass & \\
%         \midrule
%         Vector scaling \cite{guo2017}       & Multiclass & \\
%         \midrule
%         Matrix scaling \cite{guo2017}       & Multiclass &  \\
%         \midrule
%         Dirichlet calibration \cite{kull2019} & Multiclass & \\
%         \midrule
%         Accuracy versus uncertainty calibration (AvUC) loss \cite{Krishnan2020}   & Multiclass confidence & %  \\
%         \midrule
%         \cite{milios2018}   & &  \\
%         \midrule
%         \cite{allikivi2019} & &  \\
%         \midrule
%         \cite{Kumar2018}    & &  \\
%         \midrule
%         \cite{Wenger2020}   & &  \\
%         \midrule
%         \cite{Kuleshov2018} & &  \\
%         \midrule
%         \cite{song2019}     & &  \\
%         \midrule
%         \cite{widmann2019}  & &  \\
%          \bottomrule
%     \end{tabularx}
%     \caption{Caption}
% \end{table}

% \subsubsection{Start with adding one more class}

% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/ternary_1.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/ternary_2.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/ternary_3.png}
% \end{figure}


% \subsubsection{Temperature Scaling}

% \textbf{Parameters:} 
% \hspace{24pt}Temperature: $t \in \mathbb{R}$  
% \vspace{12pt}
% \textbf{Predictive Function:} 
% \hspace{24pt}$c_{j}(\mathbf{p}; t) = \frac{\exp\big(-t \cdot \text{logit}_j (p)\big)}{\sum_{j=1}^{K}\exp\big(-t \cdot \text{logit}_j (p)\big)}$ 
% \vspace{12pt}
% \textbf{Objective Function:} 
% \hspace{24pt} $\mathbb{L}(t) = \frac{1}{N} \sum_{i=1}^{N} \ln \Big(\sum_{j=1}^{K} - \mathbb{I}(y_i=j) \cdot c_{j}(\mathbf{p}_i; t)\Big)$


% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/ts_c1.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/ts_c2.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/ts_c3.png}
% \end{figure}
% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/ts_map_c1.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/ts_map_c2.png}\hfill
% \includegraphics[width=0.33\textwidth]{figures/calibrators/ts_map_c3.png}
% \end{figure}

% \subsubsection{Vector Scaling}

% \textbf{Parameters:} 
% \hspace{24pt}Vector: $\mathbf{w} \in \mathbb{R}^{K}$  
% \hspace{24pt}Intercept: $\mathbf{b} \in \mathbb{R}^{K}$ 
% \vspace{12pt}
% \textbf{Predictive Function:} 
% \hspace{24pt}$c_{j}(\mathbf{p}; \mathbf{w}) = \frac{\exp\big(-w_j \cdot \text{logit}_j (p) -b_j\big)}{\sum_{j=1}^{K}\exp\big(-w_j \cdot \text{logit}_j (p) - b_j\big)}$ 
%\vspace{12pt}
% \textbf{Objective Function:} 
% \hspace{24pt} $\mathbb{L}(\mathbf{w}, \mathbf{b})= \frac{1}{N} \sum_{i=1}^{N} \ln \Big(\sum_{j=1}^{K} - \mathbb{I}(y_i=j) \cdot c_{j}(\mathbf{p}_i; \mathbf{w}, \mathbf{b})\Big)$


% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/vs_c1.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/vs_c2.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/vs_c3.png}
% \end{figure}
% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/vs_map_c1.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/vs_map_c2.png}\hfill
% \includegraphics[width=0.33\textwidth]{figures/calibrators/vs_map_c3.png}
% \end{figure}


% \subsubsection{Matrix Scaling}

% \textbf{Parameters:} 
% \hspace{24pt}Matrix: $(\mathbf{w}_1, \cdots, \mathbf{w}_K), \mathbf{w}_j \in \mathbb{R}^K$   
% \hspace{24pt}Intercept: $\mathbf{b} \in \mathbb{R}^{K}$
% \vspace{12pt}
% \textbf{Predictive Function:} 
% \hspace{24pt}$c_{j}(\mathbf{p}; \mathbf{w}_1, \dots, \mathbf{w}_{K}, \mathbf{b}) = \frac{\exp\big(-\mathbf{w}_j^T \text{logit}( \mathbf{p}) - b_j\big)}{\sum_{j=1}^{K}\exp\big(-\mathbf{w}_j^T \text{logit}( \mathbf{p}) - b_j\big)}$ 
% \vspace{12pt}
% \textbf{Objective Function:} 
% \hspace{24pt} $\mathbb{L}(\mathbf{w}_1, \dots, \mathbf{w}_K, \mathbf{b})= \frac{1}{N} \sum_{i=1}^{N} \ln \Big(\sum_{j=1}^{K} - \mathbb{I}(y_i=j) \cdot c_{j}(\mathbf{p}_i; \mathbf{w}_1, \dots, \mathbf{w}_K, \mathbf{b})\Big)$

% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/ms_c1.png}\hfill
% \includegraphics[width=0.28\t\extwidth]{figures/calibrators/ms_c2.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/ms_c3.png}
% \end{figure}

% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/ms_map_c1.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/ms_map_c2.png}\hfill
% \includegraphics[width=0.33\textwidth]{figures/calibrators/ms_map_c3.png}
% \end{figure}

% \subsubsection{Dirichlet Calibration}

% \textbf{Parameters:} 
% \hspace{24pt}Coefficients: $(\mathbf{w}_1, \cdots, \mathbf{w}_K), \mathbf{w}_j \in \mathbb{R}^K$  
% \hspace{24pt}Intercept: $\mathbf{b} \in \mathbb{R}^{K}$ 
% \vspace{12pt}
% \textbf{Predictive Function:} 
% \hspace{24pt}$c_{j}(\mathbf{p}; \mathbf{w}_1, \dots, \mathbf{w}_{K}, \mathbf{b}) = \frac{\exp(-b_j - \mathbf{w}_j^T \ln \mathbf{p})}{\sum_{j=1}^{K}\exp(-b_j-\mathbf{w}_j^T \ln \mathbf{p})}$
% \vspace{12pt}
% \textbf{Objective Function:} 
% \hspace{24pt} $\mathbb{L}(\mathbf{w}_1, \dots, \mathbf{w}_K, \mathbf{b})= \frac{1}{N} \sum_{i=1}^{N} \ln \Big(\sum_{j=1}^{K} - \mathbb{I}(y_i=j) \cdot c_{j}(\mathbf{p}_i; \mathbf{w}_1, \dots, \mathbf{w}_K, \mathbf{b})\Big)$

% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/dir_c1.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/dir_c2.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/dir_c3.png}
% \end{figure}
% \begin{figure}
% \centering
% \includegraphics[width=0.28\textwidth]{figures/calibrators/dir_map_c1.png}\hfill
% \includegraphics[width=0.28\textwidth]{figures/calibrators/dir_map_c2.png}\hfill
% \includegraphics[width=0.33\textwidth]{figures/calibrators/dir_map_c3.png}
% \end{figure}

% \subsection{Notable Mentions}

% \begin{itemize}
% \item \cite{naeini2015}
% \item \cite{milios2018}
% \item \cite{allikivi2019}
% \item \cite{Kumar2018}
% \item \cite{Wenger2020}
% \item \cite{Kuleshov2018}
% \item \cite{song2019}
% \item \cite{widmann2019}
% \end{itemize}

% \subsection{Regularisation and Bayesian Treatments}

% \begin{itemize}
%     \item Typical approaches are generally easy to adopt: $L_{0}$, $L_{1}$, $L_2$, lasso, ridge, as well as common Bayesian inference with certain priors on the parameters. 
    
%     \item In Dirichlet calibration, the authors proposed an off-diagonal L2 regularisation approach for Dirichlet calibration, which improves the generalisation of calibration for deep nets by limiting the pair-wise interaction among different classes.
% \end{itemize}


% \subsection{Implementation}

% There are also some common practices when implementing a calibration approach:
% \begin{itemize}
% \item Have multiple inner folds to train the base model and calibrators separately
% \item Approaches including Beta, Dirichlet, and matrix scaling can be easily trained with existing logistic regression implementations.  
% \item For calibrators with a convex loss, when the number of data points and classes is manageable, explicit Newton approaches is generally better than stochastic optimisation.
% \end{itemize}

% \subsection{Wrap Up}

% \subsubsection{Lessons learned}

% To select a suitable calibrator, consider the following:
% \begin{itemize}
% \item Do you care about the entire probability vector or just about a single class? (the latter $\rightarrow$ binary approaches)
% \item Do you have a large calibration set? (yes $\rightarrow$ non-parametric approaches)
% \item Do you have a small calibration set? (yes $\rightarrow$ consider regularisation)
% \item Are you only interested in certain probability values? (yes $\rightarrow$ binning approaches)
% \end{itemize}


==> mlj_files/compiled/05_advanced_topics.tex <==
% \section{Advanced topics}
% \label{sec:out:conc}

% Now that we are nearing the end of this survey we will briefly discuss some more advanced topics related to post-hoc calibration.
% Section~\ref{sec:hyp} gives an introduction to statistical tests for calibration.
% Section~\ref{sec:costs} provides an alternative, cost-based view of the problem of classifier calibration, and discusses the need of calibration from the point of decision theory.
% In Section~\ref{sec:regcal} we consider what it means to calibrate in regression.
% Finally, section~\ref{sec:conclusion} concludes the paper.

\section{Hypothesis tests for calibration}
\label{sec:hyp}
%----------------------------------------------------%

Even if a classifier is perfectly calibrated, it almost always slightly deviates from calibration on any finite dataset due to sampling effects.
Here we consider a method of testing whether the dataset provides sufficient evidence that the classifier is uncalibrated. 

\newtext{A common way to test for calibration is to apply goodness-of-fit tests that were originally proposed for logistic regression models, but can be extended to any model that predicts probabilities. For example, one could apply the Pearson chi-squared goodness-of-fit test, which works by grouping instances sharing the same value of the independent variable $X$ and then applying a chi-squared test under the null hypothesis that the observed number of positives in the target variable is equal to the predicted number of positives for each unique value of $X$.}

\newtext{The issue with this approach is that the higher the number of unique values of $X$ or the higher the number of combinations of values of multiple independent variables, the lower the probability that each group of instances will be well-represented enough for the calculation of the Pearson chi-squared statistic to be reliable. A possible solution to this problem is to group instances into $M$ bins based on percentiles of the predicted probabilities for the positive class (equal-frequency binning) and then apply the Hosmer-Lemeshow (HL) test, which involves calculating the statistic $H$ given by Equation (\ref{eq:hosmer-lemeshow}) \cite{Hosmer2003applied}.} 

\newtext{
\begin{equation}
\label{eq:hosmer-lemeshow}
H = \sum_{m=1}^{M} \left(\frac{\left(O_{m+} - E_{m+}\right)^2}{E_{m+}}+\frac{\left(O_{m-} - E_{m-}\right)^2}{E_{m-}} \right),
\end{equation}
}
\newtext{
\noindent where $O_{m+}$ and $O_{m-}$ are the observed counts of positives and negatives in bin $\mathbb{B}_{m}$ and $E_{m+}$ and $E_{m-}$ are the expected counts of positives and negatives in bin $\mathbb{B}_{m}$, calculated as the sums of positive and negative probabilities in the bin, respectively.
}

\newtext{The HL test was later extended to evaluate the goodness-of-fit of multinomial logistic regression models, by binning instances based on the percentiles of $\sum_{j=2}^K s_{ij} = 1 - s_{i1}$, i.e. the complement of the probabilities assigned to the reference class \cite{fagerland2008multinomial}. Then, similarly to the binary case, once the instances are binned, we calculate $O_{mj}$ and $E_{mj}$, respectively the observed and expected counts for each class $j$ and bin $m$. Finally we calculate the $C$ statistic, given by Equation (\ref{eq:hosmer-lemeshow:C}), which is expected to follow a chi-squared distribution with $(M-2)(K-1)$ degrees of freedom.}

\newtext{
\begin{equation}
\label{eq:hosmer-lemeshow:C}
C = \sum_{m=1}^{M}\sum_{j=1}^{K} \left(\frac{\left(O_{mj} - E_{mj}\right)^2}{E_{mj}}+\frac{\left(O_{mj} - E_{mj}\right)^2}{E_{mj}} \right).
\end{equation}
}

\newtext{Table \ref{tab:hosmer:lemeshow} shows $M=5$ bins based on the toy example of Table \ref{tab:evaluation:toy}. By applying Equation (\ref{eq:hosmer-lemeshow:C}) to these values, we get $C = 25.3$. Finally, to complete the HL test under the null hypothesis that the observed and expected proportions are the same, we compare $C$ to a chi-squared distribution with $(M-2)(K-1) = 6$ degrees of freedom, obtaining a p-value of $0.0003$, rejecting the null hypothesis with $\alpha=0.05$.}

\begin{table}[ht]
    \centering
    \small

    \begin{tabular}{llrrrrrr}
    \toprule
    $\mathbb{B}_{m}$ &    $\mathsf{s}(\mathbb{B}_{m})$ &  $O_{m1}$ &       $E_{m1}$ &  $O_{m2}$ &       $E_{m2}$ &  $O_{m3}$ &     $E_{m3}$ \\
    \midrule
    $\mathbb{B}_{1}$ &  $[0.0, 0.2]$ &  $3.0$ &  $5.9$ &  $1.0$ &  $0.7$ &  $3.0$ &  $0.4$ \\
    $\mathbb{B}_{2}$ &  $(0.2, 0.56]$&  $2.0$ &  $3.1$ &  $2.0$ &  $0.6$ &  $1.0$ &  $1.3$ \\
    $\mathbb{B}_{3}$ &  $(0.56, 0.7]$&  $3.0$ &  $2.47$ &  $3.0$ &  $1.77$ &  $1.0$ &  $2.77$ \\
    $\mathbb{B}_{4}$ &  $(0.7, 0.9]$ &  $2.0$ &  $1.1$ &  $3.0$ &  $3.1$ &  $2.0$ &  $2.8$ \\
    $\mathbb{B}_{5}$ &  $(0.9, 1.0]$ &  $0.0$ &  $0.0$ &  $1.0$ &  $1.2$ &  $3.0$ &  $2.8$ \\
    \bottomrule
    \end{tabular}
    \caption{\newtext{Instances grouped into 5 bins using equal-frequency binning on the complement of the probabilities predicted for class 1. Column $\mathsf{s}(\mathbb{B}_{m})$ shows the probability intervals corresponding to each bin. The probabilities were obtained by considering the multiclass toy problem in Table \ref{tab:evaluation:toy}.}}
        \label{tab:hosmer:lemeshow}
\end{table}

\newtext{This example is of course simply illustrative, as the HL test is not recommended for such small samples, as experiments have shown that it has satisfactory power for samples of over 400 instances \cite{fagerland2008multinomial}. There are several other goodness-of-fit tests, most of them using some sort of binning to calculate a statistic that is assumed to follow a chi-squared distribution. Additionally, as the multiclass HL test, they usually test for classwise calibration. Testing for multiclass calibration is a more complex task and has recently been investigated by \citet{widmann2019calibration}, by using kernel-based measures. These measures were later adapted for regression calibration \cite{widmann2022calibration}. For  details on how these measures can be interpreted as test statistics, we refer the reader to their original papers.}

\newtext{Another approach, proposed by \citet{vaicenavicius2019evaluating}, is to test the classifier's probabilities according to an arbitrary measure of calibration.}
Given a classifier $\mathsf{f}$, we can check if its predictions for a test set $\{(\boldsymbol{x}_1, y_1), \dots, (\boldsymbol{x}_N, y_N)\}$ are calibrated according to a chosen calibration measure $\phi(\mathsf{f}(\mathbf{X}_{\text{test}}),\mathbf{\dot{Y}}_{\text{test}})$, such as ECE, log-loss or Brier score. We discuss a simple resampling-based hypothesis test under the null hypothesis that the classifier's outputs are calibrated \cite{vaicenavicius2019evaluating}. Algorithm \ref{alg:test:steps} details the steps of the hypothesis test procedure.

\begin{algorithm}[H]
		\caption{Hypothesis test for calibration}
		\label{alg:test:steps}
		\begin{algorithmic}[1]
			\Require Test predictions $\mathsf{f}(\mathbf{X}_{\text{test}})$; test set labels $\mathbf{\dot{Y}}_{\text{test}}$, Calibration measure $\phi$; Number of resampled label sets $L$; Significance level $\alpha$;
			
			\For { l=1:L}
			\State Sample $\boldsymbol{y}_l$, $l \in \{1, \ldots, L\}$, such that each $y_{l,i} \sim \mathsf{Cat}(\mathsf{f}(\mathbf{\hat{x}}_i))$;
			\State $\phi_s \leftarrow \phi\left(\mathsf{f}(\mathbf{X}_{\text{test}}),\mathbf{\dot{Y}}_l\right)$;
			\EndFor
		
			\State $\text{p-value} \leftarrow \text{proportion of $\phi_l$ among $\phi_1,\dots,\phi_L$ with}\ \phi_l > \phi\left(\mathsf{f}(\mathbf{X}_{\text{test}}),\mathbf{\dot{Y}}_{\text{test}}\right)$;
			
			\If {$\text{p-value} < \alpha$}
			\State Reject the null hypothesis and conclude that the classifier is not calibrated;
			\Else
			\State Accept the null hypothesis, i.e. there is not enough evidence that the classifier is not calibrated.
			\EndIf
		\end{algorithmic}
\end{algorithm}

Let us return to our toy example (Table \ref{tab:evaluation:toy}). If we follow Algorithm \ref{alg:test:steps} and choose $\mathsf{ECE}_{\text{classwise}}$ as the calibration measure and $L=1,000$, we obtain a distribution such as the one in Figure \ref{fig:eval:loss-distribution}. 

% First, we generate $S$ bootstrapped label sets $\boldsymbol{y}_s$, $s \in \{1, \ldots, S\}$, such that each $y_{s,i}$ is sampled from $\boldsymbol{\hat{p}}(\boldsymbol{\hat{x}}_i)$. Then we calculate $\phi(\boldsymbol{\hat{p}}(X_{\text{test}}), \boldsymbol{y}_s)$ for each label set $\boldsymbol{y}_s$, which gives us a distribution such as the one in Figure \ref{fig:eval:loss-distribution:a}.

% \begin{figure}
%         \centering
%         \includegraphics[width=0.7\textwidth]{figures/evaluation/loss-distribution.png}
%         \caption{Distribution of $\text{classwise-ECE}$ values calculated for every bootstrapped label set $\boldsymbol{y}_s$ with $s \in \{1, \ldots, S\}$, following the procedure described in Algorithm \ref{alg:test:steps}.}
%         \label{fig:eval:loss-distribution}
%     \end{figure}

\begin{figure}[!t]
    \centering
%    \begin{subfigure}{0.45\linewidth}
%    \includegraphics[width=\linewidth]{figures/evaluation/loss-distribution.png}
%    \caption{Distribution of loss values.}
%    \label{fig:eval:loss-distribution:a}
%    \end{subfigure}
%    \begin{subfigure}{0.45\linewidth}
%    \includegraphics[width=\linewidth]{figures/evaluation/loss-distribution-p-value.png}
%    \caption{Red bars represent $\phi_l >  0.1787$.}
%    \label{fig:eval:loss-distribution:b}
%    \end{subfigure}    
    \includegraphics[width=0.6\linewidth]{loss-distribution-p-value.png}
    \caption{Distribution of $\mathsf{ECE}_{\text{classwise}}$ values $\phi_1,\dots,\phi_L$ calculated for every resampled label set $\mathbf{\dot{Y}}_l$ with $l \in \{1, \ldots, L\}$, following the procedure described in Algorithm \ref{alg:test:steps}. The red bars represent the region where $\phi_l >  0.1787$.}\label{fig:eval:loss-distribution}
\end{figure}


Recall that in our example $\mathsf{ECE}_{\text{classwise}} = 0.1787$. The p-value for this test is then $\mathsf{P}\Big(\phi_l >  0.1787\Big) \approx 0.016$, which means we can reject the null hypothesis that the classifier is calibrated according to $\mathsf{ECE}_{\text{classwise}}$. Note that we keep the scores fixed and only resample the labels to perform this test. This means that instances will stay in the same bins and small bins will have low weights for all $L$ resampled $\mathsf{ECE}_{\text{classwise}}$ values.




% Now let the value of the arbitrary loss measure for the test set be $\phi(\boldsymbol{\hat{p}}(X_{\text{test}}), \boldsymbol{y}_{\text{test}}) = 0.32$. We calculate the p-value for the test as $P\Big(\phi(\boldsymbol{\hat{p}}(X_{\text{test}}), \boldsymbol{y}_s) > 0.32\Big) \approx 0.26$, which is equivalent to the red area in Figure \ref{fig:eval:loss-distribution:b}. Thus, we cannot reject the null hypothesis in this example, and this classifier would be considered calibrated.


% \subsection{A cost-based view of classifier calibration}
% \label{sec:costs}
%So far we have framed calibration as aiming to get as close as possible to the Bayes-optimal classifier, predicting the `true' $\mathsf{P}(y|x)$.
%That is, we want the probabilities estimated by a predictive model to match the observed frequencies as closely as possible. 
% One of the scenarios where calibrated probabilities are particularly required is cost-sensitive decision making, where the aim is to minimise the expected cost of misclassifications, given the cost matrix specifying the cost of predicting class $i$ for an instance of class $j$ for any classes $i$ and $j$.
% In Section~\ref{sec:2:1} \todo[inline]{Fix reference to sec:2:1. A closer look at calibration, and why it matters}, we saw that in binary classification the optimal threshold for the Bayes-optimal model $\mathsf{P}(+|\mathbf{x})$ is equal to $c=\frac{\mathsf{C}(+|-)}{\mathsf{C}(+|-)+\mathsf{C}(-|+)}$, where $\mathsf{C}(+|-)$ and $\mathsf{C}(-|+)$ are the costs of a false positive and a false negative, respectively.
% We will refer to $c \in [0, 1]$ as the cost proportion.
%It is also possible to justify the need of calibration from a decision-theoretic point of view.
% Let us now investigate what the optimal threshold is for non-optimal classifiers. 
%In the context of binary classification, we need to decide which class to predict for any score $s$, and our aim is to minimise some given objective on the dataset.
% Among all the possible values of predicted positive class probability $s$, the optimal threshold $s_{\text{dec}}$ is such that the expected misclassification cost is the same regardless of which class is predicted:
%
%When the evaluation metric is accuracy, an intuitive location for the decision boundary is where both classes are equally likely on the particular score.
%This condition explicitly suggests the calibrated probability of $0.5$.
%
%Now we move to a more comprehensive setting.
%Let $c_{FP}$ denote the instance-wise cost for making a false positive prediction, and $c_{FN}$ the instance-wise cost for a false negative prediction.
%Denoting the Recall that the decision boundary $s_{\text{dec}}$ is where it makes no difference to predict either class, which suggests:
%
% \begin{align}
% \label{eq:samecost}
%     P(Y=+ \mid s_{\text{dec}}) \mathsf{C}(-|+) = P(Y=- \mid s_{\text{dec}})  \mathsf{C}(+|-)
% \end{align}
% but additionally, we also need to require that scores higher than $s_{\text{dec}}$ would be more likely positives and scores lower than $s_{\text{dec}}$ would be less likely positives (known as the requirement of being classification-calibrated at $s_{\text{dec}}$ \citep{nguyen2009surrogate}):
% \begin{align*}
%     \label{eq:dec}
%     P(Y=+ \mid s') &> P(Y=+ \mid s_{\text{dec}}) \quad \forall s' > s_{\text{dec}} \\
%     P(Y=+ \mid s') &< P(Y=+ \mid s_{\text{dec}}) \quad \forall s' < s_{\text{dec}} \nonumber
% \end{align*}
% The requirement (\ref{eq:samecost}) that the expected misclassification cost is the same regardless of which class is predicted can be rewritten as
% \begin{align*}
%     P(Y=+ \mid s_{\text{dec}}) \mathsf{C}(-|+) = \Big(1 - P(Y=+ \mid s_{\text{dec}}) \Big) \mathsf{C}(+|-)
% \end{align*}
% leading to
% \begin{align*}
%     \quad P(Y=+ \mid s_{\text{dec}}) = \frac{\mathsf{C}(+|-)}{\mathsf{C}(+|-) + \mathsf{C}(-|+)}=c
% \end{align*}
%
%Since both costs can be assumed to be positive, we can normalise it as the relative misclassification cost:
%
%\begin{align*}
%    c = \frac{c_{FP}}{c_{FP} + c_{FN}}
%\end{align*}
%
% The corresponding decision threshold $s_{\text{dec}}$ for a given $c$ is then such that:
%
% \begin{align*}
%    P(Y=+ \mid s_{\text{dec}}) = c
% \end{align*}
% If the scoring classifier is perfectly calibrated, then $P(Y=+ \mid s_{\text{dec}})=s_{\text{dec}}$. From this we can conclude that for calibrated classifiers the optimal 
% decision threshold is $s_{\text{dec}}=c$, which is the same optimal threshold as for the Bayes-optimal classifier.

%Next, we will continue on binary classification and cover the definitions of classification-calibrated and ranking-calibrated, which are both weaker concepts than class probability calibration.
%While the decision boundary only suggests that it makes no difference to predict either class given the particular score, it can help us to determine the predictions for other scores when the following conditions are met (referred to as being classification-calibrated on $s_{\text{dec}}$ by \citet{nguyen2009surrogate}):
%
%\begin{align}
%    \label{eq:dec}
%    P(Y=+ \mid s') &> P(Y=+ \mid s_{\text{dec}}) \quad \forall s' > s_{\text{dec}} \\
%    P(Y=+ \mid s') &< P(Y=+ \mid s_{\text{dec}}) \quad \forall s' < s_{\text{dec}} \nonumber
%\end{align}
%
%That is, given any other score $s'$, the probability of $P(Y=+ \mid s')$ will be larger than $P(Y=+ \mid s_{\text{dec}})$ is $s' > s_{\text{dec}}$, and vice versa.
%In this case, we can simply predict positives for every score that is larger than $s'$, and predict negative otherwise. 
%Therefore, if we have a cost proportion $c$, and the two conditions in Equation~(\ref{eq:dec}) are met, then the optimal threshold $s_{dec}$ is the score that has a calibrated probability of $c$.


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.35\textwidth]{figures/conclusion/rel.png}\hfill
%     \includegraphics[width=0.5\textwidth]{figures/conclusion/brier_curve.png}
%     \caption{({Left}) The reliability diagrams of the same logistic classifier that are respectively uncalibrated and perfectly post-calibrated. ({Right}): The corresponding Brier curves. The area under the blue curve is the refinement loss of both classifiers, and the area between the red and blue curves is the calibration loss of the uncalibrated model.}
%     \label{fig:brier_curve}
% \end{figure}


% At first sight, calculating misclassification cost based on costs of false positives and false negatives is quite a different way of evaluating a classifier than proper scoring rules.
% Interestingly though, connections can be made between them.
% Suppose we consider different cost scenarios with different values of the cost proportion $c$, but only such that the cost of a false positive and a false negative add up to $2$, that is $\mathsf{C}(+|-)+\mathsf{C}(-|+)=2$.
% Here requiring the sum to be equal to $2$ ensures that the error rate is among the considered scenarios, as then $\mathsf{C}(+|-)=\mathsf{C}(-|+)=1$.
% Let us always pick the decision threshold assuming that the scoring classifier is perfectly calibrated, i.e. $s_{\text{dec}}=c$, even if actually the classifier is not calibrated.
% Then the \emph{Brier curve} is the result of plotting average misclassification cost per instance denoted as $L(c)$ against the cost proportion $c$ 
%  \cite{hernandez-orallo2011}, where $L(c)$ is defined as: 
% \begin{align*}
% L(c)=\frac{1}{n}\sum_{i=1}^n \mathsf{C}(+|-)\mathsf{I}(\hat{y}_i=+,y_i=-)+\mathsf{C}(-|+)\mathsf{I}(\hat{y}_i=-,y_i=+)
% \end{align*}
% and $\mathsf{C}(+|-)=2c$, $\mathsf{C}(-|+)=2(1-c)$. 
% Denote $\pi$ as the marginal probability for the positive class, $\mathit{fpr}(s_{dec})$ and $\mathit{tpr}(s_{dec})$ as the false positive rate and true positive rate at threshold $s_{dec}$. 
% The normalised optimal cost can then be derived as \cite{hernandez-orallo2012}:
% %
% \begin{align*}
%     L_c(s_{dec}) = 2c(1-\pi)\mathit{fpr}(s_{dec}) + 2(1-c)\pi(1 - \mathit{tpr}(s_{dec}))
% \end{align*}
% %
% Denote $\hat{Y}$ as the predicted label, here $(1-\pi)\mathit{fpr}(s_{dec})$ is the probability of false positive $P(Y=-, \hat{Y}=+)$, and $\pi(1 - \mathit{tpr}(s_{dec}))$ is the probability of false negative $P(Y=+, \hat{Y}=-)$. 
% A factor of $2$ is added to mimic the common definition of error rate, which corresponds to the case of $c = 0.5$ (i.e. a false positive has the same cost as a false negative).
% 
% While the above threshold $s_{\text{dec}}$ and cost are only optimised for the specific cost proportion $c$, it would be desirable if the classifier can provide scores that can be optimised with any potential cost proportion $c \in [0, 1]$.
% In this case, we want the conditions in Equation~(\ref{eq:dec}) to be met with any $s_{dec} $ (hence $c$), leading to the following definition.
% %
% \textit{Ranking calibration}: Denote a scoring binary classifier as $\mathsf{f}: \mathbb{X} \rightarrow \mathbb{R}$, $s_1, s_2 \in \mathbb{R}$ are two independent model output values, the classifier is ranking-calibrated if the following condition is met:
% %
% \begin{align}
%     P(Y=+ \mid s_1) \geq P(Y=+ \mid s_2)  \quad \forall s_1 \geq s_2
% \end{align}
% %
% With a ranking-calibrated classifier, we can simply find the $s_{\text{dec}}$ with any given cost proportion $c$.
% 
% This procedure can be further simplified by assuming $s$ are probability-calibrated scores, which is a sufficient condition to be ranking-calibrated:
% %
% \begin{align*}
%     P(Y=+ \mid s) = s  \quad \forall s \in [0, 1]
% \end{align*}
% %
% With calibrated scores, given any cost proportion $c$, we always have $s_{\text{dec}}=c$, and the optimal cost is hence:
% %
% \begin{align*}
%     L_c(c) = 2c(1-\pi)\mathit{fpr}(c) + 2(1-c)\pi(1 - \mathit{tpr}(c))
% \end{align*}
% 
% 
% Since the cost now only depends on $c$, it is possible to plot $L(c)$ as a scalar function of $c$, and such a visualisation is known as cost curves.
% The Brier curve plots $L(c)$ against $c$ \cite{hernandez-orallo2011}. 
% Brier curves are a particular kind of cost curve \cite{drummond2006}.
% These Brier curves have several useful properties:
% (1) The area under the Brier curve (i.e., the expected loss over uniform $c$) is equal to the Brier score, making a connection between the cost perspective and the proper scoring rule perspective; 
% (2) Among all possible score transformations, a perfectly calibrated classifier has the lowest possible Brier curve (lower envelope);
% (3) The areas between and under the Brier curves before and after perfectly calibrating are corresponding to the decomposition of Brier score into refinement loss and calibration loss. 

% Example Brier curves are given in Figure~\ref{fig:brier_curve}.
% We again consider a synthetic dataset where we can have as many data points as necessary to ensure a classifier can be nearly calibrated everywhere.
% As indicated by the left figure, we have a logistic classifier trained on the synthetic dataset, resulting in uncalibrated probabilities as depicted by the red reliability diagram.
% With unlimited data points, we then calibrate the classifier to be close to perfectly calibrated, and the corresponding blue reliability diagram follows the ascending diagonal.
% For the right figure, we see that the blue curve has a smaller area under it, which indicates a smaller Brier score.
% Since the blue curve is from a perfectly calibrated model, this area is also equivalent to the refinement loss of the model as calculated by the Brier score.
% The area between the two curves is therefore the calibration loss of the uncalibrated model.
% \citet{flach2015lmce} demonstrates that this construction carries over to other proper scoring rules. 



% \subsection{Beyond the calibration of label probabilities}
% \label{sec:beyond}
% 
% While we have been mainly addressing calibration of label probabilities in the classification context, the notion of calibration can be generalised to various tasks beyond standard probabilistic classification.
% 
% \subsubsection*{Probability calibration for optimal decisions with F-score}
% 
% When we discussed the cost-sensitive view of calibration in the previous section, we saw that the decision boundary under a standard accuracy setting (equal misclassification cost) is the calibrated probability of $0.5$.
% Furthermore, if we have a classifier that is calibrated for a specific probability value of $p$, it will be the corresponding decision boundary if we assume the negatives are $\frac{p}{1-p}$ times more important than positives.
% This assumption leads to a modified version of the accuracy measure, known as the weighted accuracy:
% %
% \begin{align*}
%     \mathit{acc}_{p}(t) = 2p(1 - \pi)\mathit{tnr}(t) + 2(1-p)\pi \mathit{tpr}(t)
% \end{align*}
% 
% By varying the value of $p$, we provide a cost-sensitive trade-off between true positives and true negatives, which further implies a trade-off between precision and recall.  
% In the extreme case, if we only care about the positives, that is, we can have $p$ getting close to $0$, and it means negatives are $\frac{p}{1-p} \rightarrow 0$ times more important than positives.
% With this setting, we can see the decision boundary will be the calibrated probability of $0$ and we will have a weighted accuracy of $1$.
% As a result, this decision boundary will lead to a recall of $1$ and a precision of $\pi$, which corresponds to a always-positive classifier.
% 
% Since the results above indicate a specific trade-off between precision and recall, it is more interpretable to use the $F_{\beta}$ score as a evaluation metric, as it includes both the precision and recall terms:
% %
% \begin{align*}
%     F_{\beta}(t) &= \frac{1}{\fracii{\frac{1}{1+\beta^2}}{\text{prec(t)}} + \fracii{\frac{\beta^2}{1+\beta^2}}{\text{rec(t)}}} \\
%     &= \frac{(1+\beta^2)\text{TP}(t)}{(1+\beta^2)\text{TP}(t) + \text{FP}(t) + \beta^2 \text{FN}(t)}
% \end{align*}
% %
% While $F_{\beta}$ is the standard form of the F-score, it is often more convenient to have a $[0, 1]$ weight $d = \frac{1}{1 + \beta^2}$, leading to the following re-parameterised version:
% %
% \begin{align*}
%     F_{d}(t) &= \frac{1}{d\frac{1}{\text{prec}(t)} + (1-d)\frac{1}{\text{rec}(t)}} \\
%     &= \frac{\text{TP}(t)}{\text{TP}(t) + d \text{FP}(t) + (1-d)\text{FN}(t) }
% \end{align*}
% 
% \begin{figure}[!b]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/conclusion/fig2-left.pdf}
%     \includegraphics[width=0.45\textwidth]{figures/conclusion/fig2-right.png}
%     \caption{({Left}): precision-recall curve, ({Right}) precision-recall-gain curve.}
%     \label{fig:pr_prg}
% \end{figure}
% 
% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/conclusion/PRG2.png}
%     \includegraphics[width=0.45\textwidth]{figures/conclusion/PRG3.png}
%     \caption{({Left}) Calibration for weighted accuracy with ROC curve, ({Right}) Calibration for $F_{\beta}$-score with precision-recall-gain curve.}
%     \label{fig:prg}
% \end{figure}
% 
% The question is now: how to calibrate a probabilistic classifier so that instances with a score value of $d$ will be on the $F_{d}$ decision boundary? 
% \citet{flach2015} address this problem by means of a non-linear transformation of the measures involved.
% We have seen that the conventional ROC curve can be used for calibrating probabilities by constructing the ROC convex hull, which is equivalent to isotonic regression.
% However, the traditional precision-recall curve is not sufficiently similar to a ROC curve to allow a similar calibration property.
% In contrast, the precision-recall-gain curve proposed by \citet{flach2015} can be seen as a proper generalisation of ROC curve obtained by replacing weighted accuracy with F-score.
% Figure~\ref{fig:pr_prg} gives a comparison between the precision-recall curve and the precision-recall-gain curve.
% Figure~\ref{fig:prg} exemplifies the calibration procedure for both the ROC curve and the precision-recall-gain curve.
% As indicated by the figures, unlike the traditional precision-recall curve, precision-recall-gain curve can be used together with the convex hull method to achieve calibration on any given $F_{\beta}$ score, as with the ROC curve with weighted accuracy.  

% \subsection{Calibration for regression}
% \label{sec:regcal}

% While in this survey we have focused on the cases where the target variable is discrete, the notion of calibration is also applicable to the continuous regression case.
% As in the classification scenario, there are multiple definitions of calibration for regression models.

% We first introduce the concept of quantile calibration.
% We denote a quantile regression model as $g: \mathbb{X} \times [0, 1] \rightarrow \mathbb{R}$, which takes a feature vector $\mathbf{x}$ and a value $\tau \in [0, 1]$, and outputs the estimated $\tau$-quantile value $\hat{y}$ so that $P(Y \leq \hat{y} \mid \mathbf{X}=\mathbf{x}) = \tau$. 
% The quantile regression model is defined as \emph{quantile-calibrated}, if and only if
% for $\forall \tau \in [0, 1]$, the following is satisfied: 
% %
% \begin{align*}
%     P\Big(Y \leq g(\mathbf{X}, \tau) \Big) = \tau \qquad \text{for } \forall \tau \in [0, 1]
% \end{align*}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.95\textwidth]{figures/conclusion/quantile_example.png}
%     \caption{An example of quantile calibration, calibrating the quantiles corresponding to $\tau=0.05,0.75,0.9$ (left plot) using a calibration map (middle plot) into quantiles corresponding to $\tau=0.1,0.5,0.8$ (right plot). }
%     \label{fig:quanitle}
% \end{figure}

% Following this definition, we can investigate how to calibrate a quantile regression model within a post-hoc setting.
% Since all possible quantiles are in the interval of $[0, 1]$, \citet{kuleshov2018} propose to adopt existing binary calibrators to adjust the quantiles.
% This procedure is demonstrated in Figure~\ref{fig:quanitle}.

% \subsubsection*{Distribution calibration for regression}

% Unlike calibration as defined for classifiers, quantile calibration for regression is defined globally across all predictions, and has no requirements on the individual prediction produced by the regression model.   
%
% To mimic the same level of calibration as in classification, \citet{pmlr-v97-song19a} introduce a stronger definition known as distribution calibration for regression. 
% If we denote a regression model (or conditional density estimator) as $$f: \mathbb{X} \rightarrow \{s \mid s:\mathbb{R} \rightarrow [0, \infty), \int s(y)dy = 1 \}$$ then this model is defined as \emph{distribution-calibrated}, if and only if
% for $\forall s :\mathbb{R} \rightarrow [0, \infty), \int s(y)dy = 1$, the following holds: 
%
% \begin{align*}
%     P\Big(Y=y \mid f(\mathbf{X}) = s) \Big) = s(y) \qquad \text{for } \forall s :\mathbb{R} \rightarrow [0, \infty), \int s(y)dy = 1
% \end{align*}
%
% Being distribution-calibrated is a sufficient but not necessary condition for being quantile-calibrated \citep[][Theorem 1]{pmlr-v97-song19a}.

% Figure~\ref{fig:dist} gives an illustration of the differences between quantile calibration and distribution calibration.
% Quantile-calibrated regression considers the global quantiles, and distribution-calibrated regression further models local distributions.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.65\textwidth]{figures/conclusion/regression_example.png}
%     \caption{The difference between distribution calibration and quantile calibration.}
%     \label{fig:dist}
% \end{figure}

% Alternative concepts of regression calibration also exist, including conformal prediction \cite{romano2019conformalized} and threshold calibration \cite{sahoo3reliable}. 
%\todo{This citation is incomplete (missing year)}




% \newtext{Will work on this in a few hours \begin{itemize}
%         \item There are various ways to visualise and quantify calibration
%         \item ECE measures aim at producing an aggregate measure of the visual information provided in reliability diagrams
%         \begin{itemize}
%             \item Thus, their optimisation is not guaranteed to produce desirable classifiers
%         \end{itemize}
%         \item Proper scoring rules measure different aspects of probability correctness
%         \begin{itemize}
%             \item They have been used as training losses in classifier training for a while
%             \item But they cannot tell ``where'' the model is more miscalibrated
%         \end{itemize}
%         \item Finally, the hypothesis test for calibration can help determine if a particular loss value means that the classifier is calibrated or not
%     \end{itemize}}


==> mlj_files/compiled/06_conclusion.tex <==
\section{Concluding remarks}
\label{sec:conclusion}

In this survey we have given a detailed overview of the principles and practice of classifier calibration.
We discussed the motivation, definition, evaluation and related approaches for the calibration of probabilistic classifiers, and touched upon topics beyond the standard classification setting.
With the recent proliferation of predictive machine learning, it is becoming more and more important that models are carefully evaluated and if possibly improved on multiple criteria to ensure the overall system robustness.
Classifier calibration relates to the criterion of uncertainty quantification, investigating the statistical relationships between model predictions and observed target variables.
There are other levels of uncertainty in the overall modelling procedure, including uncertainty pertaining to model parameters when the training set is limited, uncertainty brought about by model mismatch, or uncertainty regarding whether the model should abstain when there might be novel target values that were not seen in the training set -- see \cite{hullermeier2021aleatoric} for a recent survey on uncertainty in machine learning. 
% With all of these interesting challenges in mind, we hope this paper can provide a useful reference for researchers and practitioner that are interested in bring predictive machine learning to the next steps.

As we hopefully have made clear in this survey, calibration research has a rich history which predates the birth of machine learning as an academic field by decades. It is important to take full advantage of that history, which perhaps isn't always fully acknowledged in recent literature on classifier calibration (e.g., of deep neural networks, which are often over-confident). Recent proposals such as confidence calibration, temperature scaling and expected calibration error have value but are far from the only options and may not be suitable for a particular application. As is often the case in machine learning, the space of options and things to consider is large, and navigating this space requires the right set of concepts and tools, many of which we have discussed in detail in this survey. 

It is perhaps useful to point out that, naturally, there are also concepts that are less than helpful when thinking about classifier calibration. One of the most prominent of these is the concept of a decision boundary, which is like describing Mount Everest with a single contour line, halfway up. To faithfully characterise the mountain -- which is what is needed for optimal decision making -- one needs many contour lines at different elevations. The only case in which the decision boundary is useful is when the class prior (and misclassification costs, if any) won't change after training, in which case only the decision threshold needs calibrating. In all other cases context change is expected and needs to be anticipated with a proper calibration analysis. 

\newtext{If a trained classifier $f$ is going to be used for a task for which it is good enough to be accurate, precise or to perform well according to any contingency matrix-based measure, then there is no particular need to consider calibration in the model's development pipeline. However, if calibrated probabilities are important for any decisions supported by $f$, the following steps can be taken to implement what was discussed in this paper:}
\newtext{
    \begin{enumerate}
        \item If possible, any classifiers considered for a task should be trained using a proper scoring rule as loss function;
        \begin{itemize}
            \item The resulting models are likely to produce better probabilities than if a non-proper loss function is used, as probability refinement and calibration will be encouraged during training (recall Section \ref{sec:psr});
            \item An alternative is to use a method that encourages calibration during training time, as discussed in Section \ref{sec:cal:training};
        \end{itemize}
        \item With the trained classifiers and, preferably a held-out calibration dataset, the calibration of the probabilities produced by the models can be evaluated using classwise reliability diagrams, to understand the miscalibration patterns, and/or ECE measures (recall Section \ref{sec:metrics});
        \item To help define which models are uncalibrated, a hypothesis test for calibration can be applied (recall Section \ref{sec:hyp});
        \item If any models produce uncalibrated probabilities, post-hoc calibrators should be used to fix them;
        \begin{itemize}
            \item The resulting calibrators should also be evaluated using reliability diagrams, ECE measures and hypothesis tests to find out which ones work best for the particular miscalibration patterns found during step 2.
        \end{itemize}
    \end{enumerate}
}

\newtext{
In order to help with the aforementioned steps, we have developed an open-source Python library called PyCalib \cite{pycalib} \footnote{The documentation of the library can be found at https://classifier-calibration.github.io/PyCalib/}. This library provides tools to measure the calibration quality of a classifier, multiple visualisation functions to better understand how calibrated is a model, and some calibration methods and pipelines to directly train arbitrary calibrated classifiers.
}

\newtext{We close this survey with some open problems. First, although binning is such an important concept in calibration, there is no standard method to decide which type of binning, e.g. equal frequency or equal width, or what number of bins to use. Recent work \cite{kangsepp2022usefulness} has investigated cross-validation to tune the number of bins used to evaluate a model on a calibration set. Second, a recurrent topic of interest is the fact that post-hoc calibration does not improve robustness against out-of-distribution inputs and what can be done to improve calibration in this context \cite{ovadia2019can}. Finally, and somewhat related to the previous point, even though calibrated probabilities provide estimations of the uncertainty regarding an instance's class given its feature values (aleatoric or first-order uncertainty), classifiers could also be made to predict their uncertainty about the predicted probabilities, which comes from not knowing the true probabilities (epistemic uncertainty). This type of prediction, a distribution of distributions, also called second-order uncertainty \cite{hullermeier2022quantifying,bengs2022pitfalls}, has been recently treated using inference based on Bayesian methods and credal sets, which are convex sets of probability distributions \cite{shaker2021ensemble}.}

% Ensure that after lessons learned we add some discussion of current open problems: second-level uncertainty, aleatoric/epistemic uncertainty, out of distribution, better metrics, better binning

%----------------------------------------------------%
% \subsection{Concluding remarks}

% \paragraph{{The myth of the decision boundary}}
%  \begin{itemize}
%     \item \highlighted{red}{Resist} thinking in terms of decision boundaries.
%     \begin{itemize}
%         \item {That is like describing Mount Everest with a single contour line, halfway up.}
%         \item {To faithfully characterise the mountain you need many contour lines at different elevations.}
%     \end{itemize}
%     \item[]
%     \item The \highlighted{red}{only case} in which the decision boundary is useful is when the class prior (and misclassification costs, if any) won't change after training. 
%         \bb{In that case you don't need to calibrate the entire probability range, only the decision threshold.}
% \end{itemize}

% \paragraph{{The long history of classifier calibration}}
%\begin{itemize}
%\item Contrary what recent machine learning literature may lead you to believe, \highlighted{red}{calibration research predates machine learning} and has been studied for three-quarters of a century.
%\item{Make sure you take full advantage of that history, and don't just follow the citations in the latest NeurIPS paper on DNN calibration.}
%\item[]
%\item Recent proposals such as confidence calibration, temperature scaling and expected calibration error have their value, but are far from the only options and may not be suitable for your particular application. 
%\item{Which leads me to\ldots}
% \end{itemize}

% \paragraph{{Calibration is an art as well as a science}}
% Many practical questions don't have \textit{a priori} answers:
%\begin{itemize}
%    \item Which calibration method? 
%    \item How many bins? 
%    \item What evaluation metric? 
%    \item Do I use a validation set? How large? 
%    \item \ldots
% \end{itemize}

%\begin{description}
%    \item[]
%    \item[We hope this tutorial has given you the tools to navigate this space!]
%\end{description}

==> mlj_files/compiled/07_declarations.tex <==
\subsection*{Declarations}

\paragraph{Funding} 
The work of PF, RSR and MPN was supported by the SPHERE Next Steps Project funded by the UK Engineering and Physical Sciences Research Council (EPSRC) [grant EP/R005273/1]. The work of RSR was funded by the UKRI Turing AI Fellowship [grant EP/V024817/1].
The work of PF and HS was supported by The Alan Turing Institute under EPSRC [grant EP/N510129/1].
The work of MK was supported by Estonian Research Council [grant PRG1604].

\paragraph{Conflicts of interest/Competing interests} Not applicable.
\paragraph{Ethics approval} Not applicable.
\paragraph{Consent to participate} Not applicable.
\paragraph{Consent for publication} Not applicable.
\paragraph{Availability of data and material} The availability of data and material used in this survey can be found at \href{https://github.com/classifier-calibration/additional_material}{https://github.com/classifier-calibration/additional\_material}. Further information is available at \href{ https://classifier-calibration.github.io/survey/}{ https://classifier-calibration.github.io/survey/}.
\paragraph{Code availability} The code to generate measurements, visualisation and results is part of \href{https://pypi.org/project/pycalib/}{PyCalib}. Further information can be found in the documentation of the library
\url{https://classifier-calibration.github.io/PyCalib/}.
\paragraph{Authors' contributions}
TSF: conceptualisation, formal analysis, methodology, software, writing (original draft, and review and editing). 
HS: conceptualisation, formal analysis, methodology, software,  writing (original draft, and review and editing). 
MPN: formal analysis, methodology, software, visualisation, writing (original draft, and review and editing). 
RSR: formal analysis, writing (review and editing). 
MK: conceptualisation, formal analysis, methodology, writing (review and editing). 
PF: conceptualisation, formal analysis, methodology, supervision, writing (original draft, and review and editing).
\footnote{The categories follow the CRediT taxonomy: http://credit.niso.org/}


==> mlj_files/compiled/definitions.tex <==
\newcommand{\bb}[1]{
    \begin{itemize}
        \item {#1}
    \end{itemize}
}

% MPN: I am currently ignoring the color
\newcommand{\highlighted}[2]{\textcolor{red}{\textbf{#2}}}
%\setbeamercolor{emph}{fg=ecmlred}
\renewcommand{\cite}[1]{\citep{#1}}

\newcolumntype{L}{>{\raggedright\arraybackslash}X}

% MPN: Allows to align figures
\usepackage[export]{adjustbox}% http://ctan.org/pkg/adjustbox

% MPN: Review modifications
\newcommand{\newtext}[1]{{
\leavevmode\color{red}{#1}}}
\newcommand{\done}{\textcolor{green}{\checkmark}}
% Opinion of a reviewer that does not need response
\newcommand{\opinion}[1]{{\fontfamily{qhv}\selectfont
\leavevmode\color{gray}{#1}}}
% Suggestion of a reviewer that requires changes
\newcommand{\suggestion}[1]{{\fontfamily{qhv}\selectfont
\leavevmode\color{black}{#1}}}
% Our response to a suggestion
\newcommand{\response}[1]{{\fontfamily{cmr}\selectfont
\leavevmode\color{green!60!blue}{#1}}}


==> mlj_files/compiled/notations.tex <==
\newcommand{\va}{\mathbf{a}}
\newcommand{\vb}{\mathbf{b}}
\newcommand{\vc}{\mathbf{c}}
\newcommand{\vp}{\mathbf{p}}
\newcommand{\vq}{\mathbf{q}}
\newcommand{\vs}{\mathbf{s}}
\newcommand{\vu}{\mathbf{u}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\vw}{\mathbf{w}}
\newcommand{\vx}{\mathbf{x}}
\newcommand{\vz}{\mathbf{z}}
\newcommand{\vX}{\mathbf{X}}
\newcommand{\MI}{\mathbf{I}}
\newcommand{\vzero}{\mathbf{0}}
\newcommand{\valpha}{\boldsymbol{\alpha}}
\newcommand{\vmu}{\boldsymbol{\mu}}
\newcommand{\vmuh}{\hat{\boldsymbol{\mu}}}
\newcommand{\vpi}{\boldsymbol{\pi}}
\newcommand{\softmax}{\boldsymbol{\sigma}}
\newcommand{\logistic}{\sigma_1}
\newcommand{\vln}{\mathbf{ln}}
\newcommand{\vexp}{\mathbf{exp}}
\newcommand{\Dir}{\mathsf{Dir}}
\newcommand{\sR}{\mathbb{R}}
\newcommand{\ODIR}{ODIR} %{ODir}

\newcommand{\eE}{\mathbb{E}}

\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}

\newcommand{\ph}{\hat{p}}
\newcommand{\vph}{\mathbf{\hat{p}}}
\newcommand{\yh}{\hat{y}}
\newcommand{\vsh}{\mathbf{\hat{s}}}
\newcommand{\sh}{\hat{s}}
\newcommand{\Ph}{\hat{P}}
\newcommand{\vPh}{\mathbf{\hat{P}}}
\newcommand{\qh}{\hat{q}}
\newcommand{\vqh}{\mathbf{\hat{q}}}
\newcommand{\muh}{\hat{\mu}}
\newcommand{\vy}{\mathbf{y}}
\newcommand{\Mph}{\mathbf{\hat{P}}}
\newcommand{\My}{\mathbf{Y}}
\newcommand{\MD}{\mathbf{D}}
\newcommand{\MW}{\mathbf{W}}
\newcommand{\MA}{\mathbf{A}}
\newcommand{\Mp}{\mathbf{P}}

\newcommand{\TO}[1]{{\color{red}[TO \uppercase{#1}]}}
\newcommand{\TODO}{\TO{DO}}

\newcommand{\Sk}{\Delta_{k}} %{\Delta_{k-1}}
\newcommand{\sX}{\mathcal{X}}

%\newtheorem{proposition}{Proposition}

\newcommand{\Fb}{\ensuremath{F_{\beta}}}
\newcommand{\pre}{\ensuremath{\mathit{prec}}}
\newcommand{\rec}{\ensuremath{\mathit{rec}}}
% MPN: I have modified the previous definition as it was raising some errors/warnings.
%      I am still not sure what is the best solution but based on the discussion [1] I decided
%      to go for the current version which does not through errors. I finally opted for adding 
%      an invisible delimiter on left and right with dot (.) as indicated in [2].
%      [1] https://tex.stackexchange.com/questions/68261/on-using-the-slash-to-denote-division-in-math-mode
%      [2] https://tex.stackexchange.com/questions/34902/what-does-right-do
% \newcommand{\fracii}[2]{\ensuremath{\left #1 \middle/ #2 \right}}
\newcommand{\fracii}[2]{\left. #1 \middle/ #2 \right.}


% For repeated decimal arc symbol above several characters/digits
\makeatletter
\DeclareFontFamily{U}{tipa}{}
\DeclareFontShape{U}{tipa}{m}{n}{<->tipa10}{}
\newcommand{\arc@char}{{\usefont{U}{tipa}{m}{n}\symbol{62}}}%

\newcommand{\arc}[1]{\mathpalette\arc@arc{#1}}

\newcommand{\arc@arc}[2]{%
  \sbox0{$\m@th#1#2$}%
  \vbox{
    \hbox{\resizebox{\wd0}{\height}{\arc@char}}
    \nointerlineskip
    \box0
  }%
}
\makeatother

==> mlj_files/definitions.tex <==
\newcommand{\bb}[1]{
    \begin{itemize}
        \item {#1}
    \end{itemize}
}

% MPN: I am currently ignoring the color
\newcommand{\highlighted}[2]{\textcolor{red}{\textbf{#2}}}
%\setbeamercolor{emph}{fg=ecmlred}
\renewcommand{\cite}[1]{\citep{#1}}

\newcolumntype{L}{>{\raggedright\arraybackslash}X}

% MPN: Allows to align figures
\usepackage[export]{adjustbox}% http://ctan.org/pkg/adjustbox

% MPN: Review modifications
\newcommand{\newtext}[1]{{
\leavevmode\color{red}{#1}}}
\newcommand{\done}{\textcolor{green}{\checkmark}}
% Opinion of a reviewer that does not need response
\newcommand{\opinion}[1]{{\fontfamily{qhv}\selectfont
\leavevmode\color{gray}{#1}}}
% Suggestion of a reviewer that requires changes
\newcommand{\suggestion}[1]{{\fontfamily{qhv}\selectfont
\leavevmode\color{black}{#1}}}
% Our response to a suggestion
\newcommand{\response}[1]{{\fontfamily{cmr}\selectfont
\leavevmode\color{green!60!blue}{#1}}}


==> mlj_files/notations.tex <==
\newcommand{\va}{\mathbf{a}}
\newcommand{\vb}{\mathbf{b}}
\newcommand{\vc}{\mathbf{c}}
\newcommand{\vp}{\mathbf{p}}
\newcommand{\vq}{\mathbf{q}}
\newcommand{\vs}{\mathbf{s}}
\newcommand{\vu}{\mathbf{u}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\vw}{\mathbf{w}}
\newcommand{\vx}{\mathbf{x}}
\newcommand{\vz}{\mathbf{z}}
\newcommand{\vX}{\mathbf{X}}
\newcommand{\MI}{\mathbf{I}}
\newcommand{\vzero}{\mathbf{0}}
\newcommand{\valpha}{\boldsymbol{\alpha}}
\newcommand{\vmu}{\boldsymbol{\mu}}
\newcommand{\vmuh}{\hat{\boldsymbol{\mu}}}
\newcommand{\vpi}{\boldsymbol{\pi}}
\newcommand{\softmax}{\boldsymbol{\sigma}}
\newcommand{\logistic}{\sigma_1}
\newcommand{\vln}{\mathbf{ln}}
\newcommand{\vexp}{\mathbf{exp}}
\newcommand{\Dir}{\mathsf{Dir}}
\newcommand{\sR}{\mathbb{R}}
\newcommand{\ODIR}{ODIR} %{ODir}

\newcommand{\eE}{\mathbb{E}}

\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}

\newcommand{\ph}{\hat{p}}
\newcommand{\vph}{\mathbf{\hat{p}}}
\newcommand{\yh}{\hat{y}}
\newcommand{\vsh}{\mathbf{\hat{s}}}
\newcommand{\sh}{\hat{s}}
\newcommand{\Ph}{\hat{P}}
\newcommand{\vPh}{\mathbf{\hat{P}}}
\newcommand{\qh}{\hat{q}}
\newcommand{\vqh}{\mathbf{\hat{q}}}
\newcommand{\muh}{\hat{\mu}}
\newcommand{\vy}{\mathbf{y}}
\newcommand{\Mph}{\mathbf{\hat{P}}}
\newcommand{\My}{\mathbf{Y}}
\newcommand{\MD}{\mathbf{D}}
\newcommand{\MW}{\mathbf{W}}
\newcommand{\MA}{\mathbf{A}}
\newcommand{\Mp}{\mathbf{P}}

\newcommand{\TO}[1]{{\color{red}[TO \uppercase{#1}]}}
\newcommand{\TODO}{\TO{DO}}

\newcommand{\Sk}{\Delta_{k}} %{\Delta_{k-1}}
\newcommand{\sX}{\mathcal{X}}

%\newtheorem{proposition}{Proposition}

\newcommand{\Fb}{\ensuremath{F_{\beta}}}
\newcommand{\pre}{\ensuremath{\mathit{prec}}}
\newcommand{\rec}{\ensuremath{\mathit{rec}}}
% MPN: I have modified the previous definition as it was raising some errors/warnings.
%      I am still not sure what is the best solution but based on the discussion [1] I decided
%      to go for the current version which does not through errors. I finally opted for adding 
%      an invisible delimiter on left and right with dot (.) as indicated in [2].
%      [1] https://tex.stackexchange.com/questions/68261/on-using-the-slash-to-denote-division-in-math-mode
%      [2] https://tex.stackexchange.com/questions/34902/what-does-right-do
% \newcommand{\fracii}[2]{\ensuremath{\left #1 \middle/ #2 \right}}
\newcommand{\fracii}[2]{\left. #1 \middle/ #2 \right.}


% For repeated decimal arc symbol above several characters/digits
\makeatletter
\DeclareFontFamily{U}{tipa}{}
\DeclareFontShape{U}{tipa}{m}{n}{<->tipa10}{}
\newcommand{\arc@char}{{\usefont{U}{tipa}{m}{n}\symbol{62}}}%

\newcommand{\arc}[1]{\mathpalette\arc@arc{#1}}

\newcommand{\arc@arc}[2]{%
  \sbox0{$\m@th#1#2$}%
  \vbox{
    \hbox{\resizebox{\wd0}{\height}{\arc@char}}
    \nointerlineskip
    \box0
  }%
}
\makeatother

==> notations.tex <==
\newcommand{\va}{\mathbf{a}}
\newcommand{\vb}{\mathbf{b}}
\newcommand{\vc}{\mathbf{c}}
\newcommand{\vp}{\mathbf{p}}
\newcommand{\vq}{\mathbf{q}}
\newcommand{\vs}{\mathbf{s}}
\newcommand{\vu}{\mathbf{u}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\vw}{\mathbf{w}}
\newcommand{\vx}{\mathbf{x}}
\newcommand{\vz}{\mathbf{z}}
\newcommand{\vX}{\mathbf{X}}
\newcommand{\MI}{\mathbf{I}}
\newcommand{\vzero}{\mathbf{0}}
\newcommand{\valpha}{\boldsymbol{\alpha}}
\newcommand{\vmu}{\boldsymbol{\mu}}
\newcommand{\vmuh}{\hat{\boldsymbol{\mu}}}
\newcommand{\vpi}{\boldsymbol{\pi}}
\newcommand{\softmax}{\boldsymbol{\sigma}}
\newcommand{\logistic}{\sigma_1}
\newcommand{\vln}{\mathbf{ln}}
\newcommand{\vexp}{\mathbf{exp}}
\newcommand{\Dir}{\mathsf{Dir}}
\newcommand{\sR}{\mathbb{R}}
\newcommand{\ODIR}{ODIR} %{ODir}

\newcommand{\eE}{\mathbb{E}}

\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}

\newcommand{\ph}{\hat{p}}
\newcommand{\vph}{\mathbf{\hat{p}}}
\newcommand{\yh}{\hat{y}}
\newcommand{\vsh}{\mathbf{\hat{s}}}
\newcommand{\sh}{\hat{s}}
\newcommand{\Ph}{\hat{P}}
\newcommand{\vPh}{\mathbf{\hat{P}}}
\newcommand{\qh}{\hat{q}}
\newcommand{\vqh}{\mathbf{\hat{q}}}
\newcommand{\muh}{\hat{\mu}}
\newcommand{\vy}{\mathbf{y}}
\newcommand{\Mph}{\mathbf{\hat{P}}}
\newcommand{\My}{\mathbf{Y}}
\newcommand{\MD}{\mathbf{D}}
\newcommand{\MW}{\mathbf{W}}
\newcommand{\MA}{\mathbf{A}}
\newcommand{\Mp}{\mathbf{P}}

\newcommand{\TO}[1]{{\color{red}[TO \uppercase{#1}]}}
\newcommand{\TODO}{\TO{DO}}

\newcommand{\Sk}{\Delta_{k}} %{\Delta_{k-1}}
\newcommand{\sX}{\mathcal{X}}

%\newtheorem{proposition}{Proposition}

\newcommand{\Fb}{\ensuremath{F_{\beta}}}
\newcommand{\pre}{\ensuremath{\mathit{prec}}}
\newcommand{\rec}{\ensuremath{\mathit{rec}}}
% MPN: I have modified the previous definition as it was raising some errors/warnings.
%      I am still not sure what is the best solution but based on the discussion [1] I decided
%      to go for the current version which does not through errors. I finally opted for adding 
%      an invisible delimiter on left and right with dot (.) as indicated in [2].
%      [1] https://tex.stackexchange.com/questions/68261/on-using-the-slash-to-denote-division-in-math-mode
%      [2] https://tex.stackexchange.com/questions/34902/what-does-right-do
% \newcommand{\fracii}[2]{\ensuremath{\left #1 \middle/ #2 \right}}
\newcommand{\fracii}[2]{\left. #1 \middle/ #2 \right.}


% For repeated decimal arc symbol above several characters/digits
\makeatletter
\DeclareFontFamily{U}{tipa}{}
\DeclareFontShape{U}{tipa}{m}{n}{<->tipa10}{}
\newcommand{\arc@char}{{\usefont{U}{tipa}{m}{n}\symbol{62}}}%

\newcommand{\arc}[1]{\mathpalette\arc@arc{#1}}

\newcommand{\arc@arc}[2]{%
  \sbox0{$\m@th#1#2$}%
  \vbox{
    \hbox{\resizebox{\wd0}{\height}{\arc@char}}
    \nointerlineskip
    \box0
  }%
}
\makeatother

==> sections/02_old_highlevel_intro_2023_01_17_with_old_comments.tex <==
\section{A brief introduction to classifier calibration}
\label{sec:intro:high:level}
The origins of classifier calibration can be traced back to weather forecasting and meteorology. 
Here is what the UK Met Office website has to say about what their forecast probabilities mean: 

\begin{quote}
    ``[S]uppose the Met Office says that the probability of rain tomorrow in your region is 80\%. They aren't saying that it will rain in 80\% of the land area of your region, and not rain in the other 20\%. Nor are they saying it will rain for 80\% of the time. What they are saying is there is an 80\% chance of rain occurring at any one place in the region, such as in your garden.
[...]
[A] forecast of 80\% chance of rain in your region should broadly mean that, on about 80\% of days when the weather conditions are like tomorrow's, you will experience rain where you are. 
%But there is still some expert judgement involved, and different forecasting organisations with different experts and different technology might well give different probabilities.
[...]
If it doesn't rain in your garden tomorrow, then the 80\% forecast wasn't wrong, because it didn't say rain was certain. But if you look at a long run of days, on which the Met Office said the probability of rain was 80\%, you'd expect it to have rained on about 80\% of them. '' (\url{https://www.metoffice.gov.uk/about-us/what/accuracy-and-trust/probability})
\end{quote}
\noindent
Note the phrase ``a long run of days'': \emph{determining the degree to which a forecaster is well-calibrated cannot be done on a per-forecast basis, but rather requires looking at a sufficiently large and diverse set of forecasts}. 

\begin{table}[!t]
        \centering
        \includegraphics[width=\linewidth]{figures/evaluation/hallenbeck1920_tab1}
        \caption{Reproduced from \citet{hallenbeck1920}.}
        \label{tab:eval:hallenbeck1920}
\end{table}

\begin{figure}[!b]
    \centering
    \includegraphics[width=0.6\linewidth]{figures/intro/Hallenbeck.pdf}\\
    \caption{Graphical representation of the forecasts in Table~\ref{tab:eval:hallenbeck1920}.
The bottom graph gives a histogram of the probability forecasts. 
The top graph compares the forecast probabilities with the proportion of actual rain events in that bin. 
The red bars indicate to what extent these proportions are higher or lower than predicted. 
    }\label{fig:hallenbeck-rel}
\end{figure}


Table~\ref{tab:eval:hallenbeck1920}, reproduced from \citet{hallenbeck1920}, groups 123 weather forecasts in 10 equal-width bins, and compares each bin with the actual percentage of rain events. 
Figure~\ref{fig:hallenbeck-rel} displays this information graphically. 
We can see that most of the forecasts are slight under-estimates: for example, of the 15 forecasts in the 40-49\% bin, $8/15=53\%$ were actual rain events. 
In the graph this is shown by the vertical red line, which indicates how much the top of the blue bar extends above the diagonal (meaning that the actual proportion of rain events was higher than estimated). 
Similarly, we see that two of the bins (20-29\% and 30-39\%) are very slight over-estimates: the top of the blue bar is below the diagonal, which means that the actual proportion of rain events was lower than estimated. 

\begin{figure}[!t]
    \centering
    \begin{subfigure}{0.45\linewidth}
    \includegraphics[width=\linewidth]{figures/intro/Hallenbeck2.pdf}
    \end{subfigure}
    \begin{subfigure}{0.45\linewidth}
    \includegraphics[width=\linewidth]{figures/intro/Hallenbeck3.pdf}
    \end{subfigure}
    \caption{Dividing the forecasts in Table~\ref{tab:eval:hallenbeck1920} in five (left figure) and two (right figure) equal-width bins.}\label{fig:hallenbeck2-rel}
\end{figure}

The choice of ten equal-width bins is somewhat arbitrary, \newtext{and it is informative to consider different choices}. 
Merging pairs of adjacent bins results in five equal-width bins, as depicted in Figure~\ref{fig:hallenbeck2-rel} (left). 
We see that all but the right-most bin averages are now slightly off-centre (we assumed that within each original bin all forecast probabilities are the same and equal to the bin centre: e.g., 25\% in the 20-29\% bin). Again, the pattern is that the higher forecast probabilities are about 10\% too low. 
Figure~\ref{fig:hallenbeck2-rel} (right) shows what we get with only two bins. 
We have lost a bit too much information here, so bins shouldn't be taken too wide. 
On the other hand they shouldn't be taken too narrow either, in order to be able to measure the true proportion of rain events with sufficient resolution. 

Taking the forecast event as a binary variable means that the calibration concept is directly applicable to binary classification. Here is an example from the typical machine learning task of learning a classifier for distinguishing `junk' or `spam' emails from regular ones: 

\begin{quote}
    A prediction `70\% chance of spam' should be spam 70\% of the time.
\end{quote}
\noindent
And a generalisation to categorical variables with more than two values is equally straightforward, as this example from Fisher's famous Iris dataset shows: 

\begin{quote}
    A prediction `70\% chance of setosa, 10\% chance of versicolor and 20\% chance of virginica' should be setosa/versicolor/virginica 70/10/20\% of the time.
\end{quote}
\noindent
So, to sum up: \emph{A predicted probability (vector) should match empirical (observed) probabilities.}




% \subsection{A closer look at calibration, and why it matters}
% \label{sec:2:1}

% % \paragraph{Why are we interested in calibration?}
% In general, to calibrate means \emph{to employ a known scale with known properties}. 
% % \bb{E.g., additive scale with a well-defined zero, so that ratios are meaningful.}
% For example, we can calibrate a thermometer to Celsius or Fahrenheit scales; 
% or a weighing device to kilograms or pounds. 
% If a measuring device is calibrated to one scale but we need the measurement in another, there are usually simple conversion formulas: 
% for example, $\text{F}=\text{C}\cdot 9/5+32$ for Celsius to Fahrenheit, and $\text{Lb}=2.2\cdot \text{Kg}$ for kilograms to pounds. 
% Notice that the temperature conversion shifts the zero point 
% (0 degrees Celsius is 32 degrees Fahrenheit, and 0 degrees Fahrenheit is $-17.8$ degrees Celsius) 
% as it is essentially arbitrarily chosen for either scale. 

% The weight conversion, in contrast, has an absolute zero which is the same for all scales. 
% Such scales are called \textit{ratio scales}, because the ratio of two measurements is meaningful: e.g., if one object is twice as heavy as another in kilograms then it will be so regardless of the scale. Such ratios are not meaningful for Celsius and Fahrenheit, but temperature \textit{differences} are.  
% For example, we could say that this person's change from morning to evening body temperature today is twice that of yesterday, without specifying the temperature scale. 
% It follows that ratios of differences (or intervals) are meaningful in this case, which is why Celsius and Fahrenheit are called \textit{interval scales}. 

% For classifiers we want to use the probability scale. Probabilities have an absolute zero like any other ratio scale, and so it is meaningful to say that one event is twice as probable as another. Probabilities also have a fixed maximum, so that taking the complement with respect to the maximum gives another ratio scale: for example, the probability of this event \textbf{not} happening might be twice the probability of another event \textbf{not} happening. This essentially fixes the scale: we don't have pounds vs.\ kilograms dilemmas for probabilities. 

% % Q: Is the probability scale additive?
% Are probabilities additive? In certain situations it is indeed valid to sum probabilities, for example to obtain the probability of any one of a number of mutually exclusive events happening, as might occur when joining classes in a multiclass classification setting. 
% But multiplication and division of probabilities are more common basic operations, for example to obtain the joint probability of independent events, or to derive a conditional probability from joint and marginal probabilities. This makes the probability scale \textit{multiplicative} for typical usage. We could obtain an additive scale by taking logarithms, giving log-likelihoods, logits as differences of log-likelihoods, etc. A couple of observations are worth making: 
% \begin{itemize}
% \item Such transformations are fundamentally different from scale conversions such as Celsius to Fahrenheit, because probabilities and log-likelihoods measure different things -- physicists might say they represent different \textit{dimensions}. Nevertheless, the transformations are invertible and hence the dimensions convey the same information. 
% \item While some ratios or products of probabilities again yield probabilities, in other cases they may derive another dimension, such as \textit{odds}, which are not expressed on a probability scale.
% \end{itemize}

What are the benefits of using well-defined calibrated scales \newtext{in general, and well-calibrated probabilities in particular}? One obvious benefit \newtext{of calibrated scales} is that we can easily combine measurements that are expressed on the same scale without comparing apples and oranges. Another is that we can use standardised decision rules, e.g., defining a fever as a body temperature exceeding 100 degrees Fahrenheit. These benefits
% \footnote{As for combining multiple probability estimates as might happen in ensemble methods in machine learning, note that the argument of probabilities being multiplicative leads to favouring the \textit{geometric mean} (or the arithmetic mean on log-probabilities). Using the arithmetic mean directly on probabilities means that the members of the ensemble are treated as classifiers scoring on some arbitrary but fixed and additive scale, disregarding their probabilistic nature.}
directly carry over to the \newtext{class probability} scenario, justifying decision rules such as predicting the class whose estimated probability exceeds $0.5$ in binary classification, or maximum posterior probability for multiclass classification. Importantly, there is a further benefit to using calibrated probabilities as it means we can adjust these decision rules in a straightforward way to account for different class priors or misclassification costs, as we will briefly discuss presently.

% %Q: What issues might arise when applying MAP decisions to poorly calibrated classifiers such as naive Bayes? 

% % PF: UNTIL HERE (27 JAN 9.30 GMT)

% % \paragraph{Optimal decisions}
% Denote the cost of predicting class $j$ for an instance of true class $i$ as ${\mathsf{C}(\hat{Y}=j|Y=i)}$. 
% % Since we don't know the true class of an unlabelled instance, we need to base our prediction on an assessment of the expected cost over all possible true classes. 
% The expected cost of predicting class $j$ for instance $\mathbf{x}$ is then
% %
% \begin{align}\label{eq::expected-cost}
% \mathsf{C}(\hat{Y}=j|\mathbf{X}=\mathbf{x}) &= \sum_i \mathsf{P}(Y=i|\mathbf{X}=\mathbf{x})\mathsf{C}(\hat{Y}=j|Y=i)
% \end{align}
% %
% where $\mathsf{P}(Y=i|\mathbf{X}=\mathbf{x})$ is the (true) probability of instance $\mathbf{x}$ having true class $i$
% (as would be given by the Bayes-optimal classifier). 
% %
% The optimal decision is to predict the class with lowest expected cost:
% \begin{align*}
% \hat{Y}^* = \argmin_j \mathsf{C}(\hat{Y}=j|\mathbf{X}=\mathbf{x}) = \argmin_j \sum_i \mathsf{P}(Y=i|\mathbf{X}=\mathbf{x})\mathsf{C}(\hat{Y}=j|Y=i)
% \end{align*}
% %
% % In the special case that all misclassifications have equal cost we can assume without loss of generality that $C(\hat{Y}=j|Y=i)=1$ for $i\neq j$ and $C(\hat{Y}=j|Y=i)=0$ for $i=j$, which gives
% % \begin{align*}
% % C(\hat{Y}=j|X=x) &= \sum_{i\neq j} P(Y=i|X=x) = 1-P(Y=j|X=x) \\
% % %\end{align*}
% % %and so
% % %\begin{align*}
% % \hat{Y}^* &= \arg\min_j [1-P(Y=j|X=x)] = \argmax_j P(Y=j|X=x)
% % \end{align*}
% In binary classification (with a positive, $+$, and and negative class, $-$) we have one predicted probability and four cost parameters, and we can rewrite Equation~(\ref{eq::expected-cost}) as
% %
% \begin{align*}
% \mathsf{C}(\hat{Y}=+|\mathbf{X}=\mathbf{x}) &= \mathsf{P}(+|\mathbf{x})\mathsf{C}(+|+) + \big(1-\mathsf{P}(+|\mathbf{x})\big)\mathsf{C}(+|-) \\
% \mathsf{C}(\hat{Y}=-|\mathbf{X}=\mathbf{x}) &= \mathsf{P}(+|\mathbf{x})\mathsf{C}(-|+) + \big(1-\mathsf{P}(+|\mathbf{x})\big)\mathsf{C}(-|-)
% \end{align*}
% %
% where $\mathsf{P}(+|\mathbf{x})$ is shorthand for $\mathsf{P}(Y=+|\mathbf{X}=\mathbf{x})$ and $\mathsf{C}(j|i)$ for $\mathsf{C}(\hat{Y}=j|Y=i)$.
% %
% On the optimal decision boundary these two expected costs are equal, 
% which gives
% \begin{align*}
% \mathsf{P}(+|\mathbf{x})\mathsf{C}(+|+) + (1-\mathsf{P}(+|\mathbf{x}))\mathsf{C}(+|-) = \mathsf{P}(+|\mathbf{x})\mathsf{C}(-|+) + (1-\mathsf{P}(+|\mathbf{x}))\mathsf{C}(-|-)
% \end{align*}
% which can be rearranged to give the posterior odds
% \begin{align*}
% \frac{\mathsf{P}(+|\mathbf{x})}{1-\mathsf{P}(+|\mathbf{x})} = \frac{\mathsf{C}(+|-)-\mathsf{C}(-|-)}{\mathsf{C}(-|+)-\mathsf{C}(+|+)}
% \end{align*}
% as well as the posterior probability
% \begin{align*}%\label{eq::cost-threshold}
% \mathsf{P}(+|\mathbf{x})  = \frac{{\mathsf{C}(+|-)-\mathsf{C}(-|-)}}{{\mathsf{C}(+|-)-\mathsf{C}(-|-)}+{\mathsf{C}(-|+)-\mathsf{C}(+|+)}} \triangleq c
% \end{align*}
% %
% $c$ thus gives the optimal threshold on the hypothetical Bayes-optimal probabilities. 
% It is also the best thing to do in practice, as long as the probabilities are well-calibrated (this is discussed in more detail in Section~\ref{sec:out:conc}). 

% Under reasonable assumptions (e.g., changing the prediction from correct to incorrect cannot decrease the incurred cost) we can set the cost of true positives and true negatives to zero \cite{elkan2001}; 

Let
$c = \frac{\mathsf{C}(+|-)}{\mathsf{C}(+|-) + \mathsf{C}(-|+)}$ be the cost of a false positive in proportion to the combined cost of one false positive and one false negative. 
\newtext{With these cost parameters the Bayes-optimal decision rule is to set the decision threshold to $c$.}
{For instance, if false positives are 4 times as costly as false negatives then we set the decision threshold to $4/(4+1)=0.8$ in order to only make positive predictions if we are sufficiently certain.}
%
Similar reasoning applies to changes in class priors: 
\begin{itemize}
    \item if we trained on balanced classes but want to deploy with 4 times as many positives compared to negatives, we lower the decision threshold to $0.2$; 
    \item more generally, if we trained for class ratio $r$ and deploy for class ratio $r'$ we set the decision threshold to $r/(r+r')$. 
\end{itemize}
Cost and class prior changes can be combined in the obvious way; see  \citet{flach2014classification} for details.

In summary, an important reason to be interested in calibrating our classifiers is that default decision rules such as maximum posterior probability are fully justified from a decision-theoretic point of view, and can easily be adapted to changes in class and cost distributions. In contrast, poorly calibrated classifiers such as naive Bayes will often perform sub-optimally with default decision rules. It is possible to learn a better decision rule for a given cost and class skew using, e.g., ROC analysis \cite{lachiche2003improving} but this would have to be repeated each time the skew changes. The great advantage of post-calibration is that it only needs to be done once -- in a sense, it optimises all possible decision rules in one go. 


\subsection{Common forms of miscalibration, and how to fix them}

There are many reasons why a probabilistic classifier might produce miscalibrated scores, and hence many ways in which miscalibration manifests itself, but two main types stand out: underconfidence and overconfidence. In this section we look at some examples and introduce three mitigation techniques. 

A good starting point for calibration analysis are diagrams such as Figure~\ref{fig:hallenbeck-rel}, which compare predicted probabilities on the $x$-axis to empirical probabilities on the $y$-axis. 
A variety of such graphical representations can be found in the literature; they are generally known as \emph{reliability diagrams}, `reliability' being one of many terms used to denote goodness of calibration \cite{murphy1977reliability};
Section~\ref{sec:met:1st} discusses reliability diagrams in more detail. 
Figure~\ref{fig:under-over}, taken from \citet{niculescu-mizil2005}, shows two typical examples. In both cases the points in the diagram are far from the diagonal, although the effect is smaller in the figure on the right. 

\begin{figure}[!t]
    \centering
    \begin{subfigure}{0.4\linewidth}
        \includegraphics[width=\linewidth]{figures/intro/Underconfidence.pdf}
        \caption{Underconfidence}
    \end{subfigure}\hfill
    \begin{subfigure}{0.4\linewidth}
        \includegraphics[width=\linewidth]{figures/intro/Overconfidence.pdf}
        \caption{Overconfidence}
    \end{subfigure}
    \caption{Examples of under- and overconfident classifiers. The dots represent the reliability diagram, and the line shows the best-fit logistic curve. 
    %To correct the underconfident scores on the left we would have to pull the points away from the midpoint on the $x$-axis, whereas to deal with the overconfidence on the right we would push them toward the midpoint. 
    Note that the logistic sigmoid is a good fit for underconfident scores but not for overconfidence.
    Figures reproduced from \citet{niculescu-mizil2005}.}
    \label{fig:under-over}
\end{figure}

What do we see in the left figure? It is quite natural to give precedence to vertical information in such graphs, so you might be inclined to say ``The points on the left are too low, and the points on the right are too high''. But keeping in mind that the predicted probabilities on the $x$-axis are under our control but not the empirical probabilities on the $y$-axis, a more `actionable' way to express this is

\begin{quote}
    The lower points are too far to the right, and the higher points are too far to the left. In other words, the points have a tendency to sit too close to the midpoint on the $x$-axis. 
\end{quote}
\noindent
This is the typical pattern displayed by an \textit{underconfident} classifier, which thinks it's {worse} at separating classes than it actually is. 

Hence, to mitigate this, we need to {pull predicted probabilities away from the centre}. As the left plot in Figure \ref{fig:under-over} shows, this can be neatly modelled by a sigmoidal logistic curve, which can be defined in parametric form as
%
\begin{align*}
    \mathsf{c}(s; w, m) &= \frac{1}{1+\exp(-w(s-m))}%\\
    % w &= (\mu_{\textit{pos}}-\mu_{\textit{neg}})/\sigma^2, 
    % m = (\mu_{\textit{pos}}+\mu_{\textit{neg}})/2
\end{align*}
%
Here, $s$ is the uncalibrated score produced by the classifier and $\mathsf{c}$ gives the logistically calibrated score. 
$m$ and $w$ are the two parameters of the logistic family, which determine the point where $\mathsf{c}(s)=0.5$ and the slope at that point, respectively. They can be estimated from the points in the reliability diagram in order to find the best fit. In this case they can be obtained analytically as the mean of the classwise average scores, and the difference between those two means in proportion to the score variance \cite{flach2012machine}.
%(which is assumed to be the same for both classes). 

The fitted logistic curve thus establishes a \textit{calibration map} which transforms uncalibrated scores $s$ into calibrated scores $\mathsf{c}(s)$. 
Even though the calibration map doesn't map to empirical probabilities, plotting it over the reliability diagram allows us to see clearly that if we project each point in the reliability diagram vertically onto the calibration map, and replace its $x$-value with the corresponding $y$-value of the projection, we end up with points on or very close to the diagonal, and hence near-perfectly calibrated scores (Figure~\ref{fig:under-cal}).

\begin{figure}[!t]
    \centering
        \includegraphics[width=0.4\linewidth]{figures/intro/Underconfidence-calibrated.pdf}
    \caption{Graphical illustration of how a well-fitted calibration map leads to near-perfect calibration. From left to right, the dotted arrows show (1) using a point's uncalibrated score $s$ on the $x$-axis as input to the calibration map, (2) mapping the resulting output $\mathsf{c}(s)$ back to the diagonal, and (3) combine with the empirical probability of the point we started from. The closer the original point is to the fitted calibration map, the closer the calibrated point (in blue) will be to the diagonal. }
    \label{fig:under-cal}
\end{figure}

The logistic curve is widely used as a `squashing function', compressing values on a possibly unbounded scale into the $[0,1]$ interval. 
Following \citet{platt2000} it is often used as a way to convert scores from a Support Vector Machine into probabilities. 
Technically this isn't calibration as SVM scores are not probabilities but (signed) geometric distances from the decision boundary -- this is also called \textit{scaling} to emphasise the difference. 
The parametric form of the logistic map can be derived from first principles by assuming that within each class the uncalibrated scores are normally distributed with the same variance (Figure~\ref{fig:logistic}). 

\begin{figure}[!b]
    \centering
    \includegraphics[width=0.6\textwidth]{figures/intro/Logistic.pdf}\vfill
    \caption{Assuming normally distributed scores within each class (left) leads to a logistic calibration map (right).}\label{fig:logistic}
\end{figure}

The other common form of miscalibration is overconfidence, as exemplified on the right-hand side of Figure~\ref{fig:under-over}. 
% Here, we see that
%
% \begin{quote}
%     The lower points are too far to the left, and the higher points are too far to the right. In other words, the points have a tendency to be too far from the midpoint on the $x$-axis. 
% \end{quote}
% \noindent
An \textit{overconfident} classifier thinks it's {better} at separating classes than it actually is. 
Hence we need to {make predicted probabilities less extreme by pushing them toward the centre}. 
The paper we took this figure from \cite{niculescu-mizil2005} also fitted a logistic curve to this reliability diagram, because they were investigating the effect of Platt scaling in a wide range of scenarios. But we see clearly that the fit is rather poor, and using this logistic curve as a calibration map is likely to make matters worse. In this particular case we would be looking for something that can produce an inverse sigmoidal curve. What would be a principled way to achieve this? 

\begin{figure}[!b]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/intro/Beta.pdf}
    \caption{An example of Beta calibration where overconfident scores (left) lead to an inverse-sigmoidal calibration map (right).}\label{fig:beta}
\end{figure}

One approach that works well is to model the classwise scores with Beta distributions \cite{pmlr-v54-kull17a,kull2017beyond}.
These assume random variables bounded in $[0,1]$ which is exactly what we need for post-hoc calibration. 
Beta distributions can easily model the skewed distributions resulting from overconfident classifiers, as demonstrated in Figure~\ref{fig:beta}. 
Mathematically, these curves have three parameters: 
%
    \begin{align*}
        \mathsf{c}(s; a, b, c) &= \frac{1}{1+\exp(-a \ln s + b \ln (1-s) - c)}
        % a &= \alpha_{\textit{pos}}-\alpha_{\textit{neg}}, 
        % b = \beta_{\textit{neg}}-\beta_{\textit{pos}}
    \end{align*}
%
This additional degree of freedom allows Beta calibration to produce both sigmoidal and inverse-sigmoidal calibration maps. 
It can even fit the identity map ($a=b=1$, $c=0$), which means that Beta calibration can recognise that scores are already calibrated. 
In contrast, applying logistic calibration to a calibrated classifier will decalibrate it. 

%PF: UNTIL HERE (28 JAN 18.00 GMT)

% So far we have seen two calibration techniques: 
% \begin{itemize}
%     \item logistic calibration, which -- although technically a scaling technique, mapping real-valued scores into probabilities -- can adjust for underconfident scores; 
%     \item Beta calibration, which assumes a classifier already scores on a probability scale, and which can adjust for both over- and underconfident scores. 
% \end{itemize}
% We will now take a first look at 
A third calibration technique
% quite different from these two because it 
derives a calibration map from the \textit{ranks} of a set of scores, and hence works for classifiers scoring on arbitrary scales. It is also different from logistic and Beta calibration because it doesn't attempt to model the classwise score distributions, and is hence \textit{non-parametric}. 
%
The technique in question is called \textit{isotonic regression}, belying its origin as an alternative to linear regression which learns a piecewise constant, monotonically increasing or decreasing function. There are several algorithms for isotonic regression, one of which is called \textit{pooled adjacent violators}, which in turn is also used for constructing the convex hull of an ROC curve \cite{zadrozny2001obtaining,fawcett2007}. Figure~\ref{fig:isotonic} demonstrates this graphically. 

\begin{figure}[!t]
    \centering
    \begin{subfigure}{0.44\linewidth}
    \includegraphics[width=\linewidth]{figures/intro/ROCCH.pdf}
    \caption{ROC curve and convex hull.}
    \end{subfigure}
    \begin{subfigure}{0.55\linewidth}
    \includegraphics[width=\linewidth]{figures/intro/ROCcal2.pdf}
    \caption{Isotonic calibration map.}
    \end{subfigure}
    \caption{An example of isotonic calibration which derives a piece-wise constant calibration map from the ROC convex hull (Source: \cite{flach2016roc}).}\label{fig:isotonic}
\end{figure}

The technique starts from a list of test instances, ranked on their scores; this might give a list of class labels like that depicted at the top of the right figure in Figure~\ref{fig:isotonic}. We then proceed to segment this ranking such that, in each adjacent pair of segments, the right neighbour has a larger proportion of positives than the left neighbour. This defines a unique set of segments, which is depicted on the right of the right figure. Each segment defines an interval on the original classifier scores, as well as an empirical probability of positives in that segment which is taken as the calibrated score for all instances whose score falls in that interval. The calibration map is thus piece-wise constant and increasing. 

As a non-parametric method, isotonic regression avoids problems of misspecification which can plague parametric models. For example, a perfectly calibrated classifier has classwise scores which are far from normally distributed, so applying logistic calibration will make matters worse. The downside is that isotonic regression tends to need more labelled data to reliably estimate the segment boundaries and the empirical probabilities within each segment, and is more liable to overfitting if data is not plentiful. 


%----------------------------------------------------%
\subsection{Multiclass calibration}
%----------------------------------------------------%

The examples we have seen so far all relate to binary classification. Is it straightforward to generalise calibration concepts and methods to more than two classes? 
The answer to this question is somewhat involved. Some ideas do generalise quite easily: for example, we can model per-class scores by multivariate distributions such as Dirichlet distributions \cite{kull2019}. Some other ideas don't generalise easily at all: for example, a multiclass generalisation of isotonic regression is not straightforward because rankings are inherently bipartite. Such approaches therefore need to be approximated by considering classes in a pairwise or one-versus-rest manner. 

This helps to explain why there is divergence even at a definitional level. 
There are at least three different ways of \emph{defining} what it means to be calibrated in a multiclass setting. 
They are equivalent for binary classification but increasingly stronger for more than two classes,%
\footnote{In rare cases it is possible for a multiclass classifier to be classwise calibrated but not confidence calibrated.
% Example due to Meelis
Here is an example with 40 instances in four groups:
10 instances with predicted probabilities (0.3,0.3,0.4) and actual class distribution (4,2,4);
another 10 with probabilities (0.4,0.3,0.3) and classes (3,4,3);
another 10 with probabilities (0.4,0.6,0.0) and classes (5,5,0);
and the remaining 10 instances with probabilities (0.3,0.6,0.1) and classes (2,7,1).
This classifier is classwise-calibrated but not confidence-calibrated. There are 20 instances with confidence level 0.6 and accuracy 0.6 (5+7=12 out of 20), but the remaining 20 instances have confidence 0.4 and accuracy 0.35 (4+3=7 out of 20). The key idea of this construction is that classwise calibration considers the instances with 0.4 predicted for class 1 as a single group, but confidence calibration looks among them only at those instances for which 0.4 is the highest probability -- e.g., it does consider (0.4,0.3,0.3) but not (0.4,0.6,0.0).}
and can be summarised as follows: 
    \begin{itemize}
        \item {Confidence calibration}: only consider the highest predicted probability. 
        \item {Classwise calibration}: only consider marginal probabilities.
        \item {Multiclass calibration}: consider the entire vector of predicted probabilities.
    \end{itemize}
We will use this terminology throughout the paper to avoid confusion. 

%\renewcommand{\vph}{\hat{\mathbf{p}}}

\textit{Confidence calibration} was proposed by \citet{guo2017}, although not under that name. It requires that among all instances where the probability of \emph{the most likely class} is predicted to be $\alpha$, the expected accuracy is $\alpha$. 
Let $\mathbb{X}$ denote the instance space and $\mathbb{P}_{\mathbb{Y}}$ the probability $K$-simplex, then a probabilistic classifier $\mathsf{f}:\mathbb{X}\rightarrow\mathbb{P}_{\mathbb{Y}}$ is \emph{confidence-calibrated}, if for any confidence level $\alpha\in[0,1]$, 
the actual proportion of the predicted class, among all possible instances $\mathbf{x}$ being predicted this class with confidence $\alpha$, is equal to $\alpha$:  
\begin{align*} 
\mathsf{P}(Y=\hat{Y} \: | \: S_{\hat{Y}}=\alpha)=\alpha\qquad\text{where }\ \hat{Y}=\argmax_j S_j.
%P\Big(Y=\argmax\big(\vph(X)\big) \: \Big| \: \max\big(\vph(X)\big)=c\Big)=c.
\end{align*}
Here, $S_j$ denotes the $j$-th dimension of $\mathsf{f}(\mathbf{X})$.

\textit{Classwise calibration}, proposed by \citet{zadrozny2002}, requires that all \emph{one-vs-rest} probability estimators obtained from the original multiclass model are calibrated. 
Formally, a probabilistic classifier $\mathsf{f}:\mathbb{X}\rightarrow\mathbb{P}_{\mathbb{Y}}$ is \emph{classwise-calibrated}, if for any class $i \in \{1, \dots, K\}$ and any predicted probability value $s \in [0, 1]$ for this class, 
the actual proportion of class $i$, among all possible instances on the random variable $\mathbf{X}$ getting the same prediction on class i, is equal to $s$:  
\begin{align*} 
\mathsf{P}(Y=i\mid S_i=s)=s
\end{align*}

\textit{Multiclass calibration} is the {strongest form of calibration} for more than two classes, subsuming the previous two definitions. 
A probabilistic classifier $\mathsf{f}:\mathbb{X}\rightarrow\mathbb{P}_{\mathbb{Y}}$ is \emph{multiclass-calibrated} if for any prediction vector $\mathbf{s}=[s_1,\dots,s_K]\in\mathbb{P}_{\mathbb{Y}}$, the proportions of classes among all possible instances on the random variable $\mathbf{X}$ getting the same prediction $\mathsf{f}(\mathbf{X})=\mathbf{s}$ are equal to the prediction vector $\mathbf{s}$:  
\begin{align*} %\label{eq:calib}
\mathsf{P}(Y=i\mid \mathsf{f}(\mathbf{X})=\mathbf{s})=s_i\qquad\text{for }\ i=1,\dots,K.
\end{align*}
%
%Here $\mathbf{s}=[s_1, \dots, s_K]$ denotes the $K$-dimensional probability vector instance.

For practical purposes, the conditions in these definitions need to be relaxed. This is where {binning} comes in. 
Once we define the bins, we can draw a {reliability diagram} as in the two-class case. For classwise calibration, we can show per-class reliability diagrams or a single averaged one. 
One way to assess the degree of calibration is by means of the {gaps} in the reliability diagram. 
These topics will be explored in Section \ref{sec:metrics}. 
We will first take a closer look at the important concept of \emph{proper scoring rules} in the next section. Proper scoring rules are instance-wise evaluation measures for probability estimates that avoid the need for score binning. As a result they cannot measure the degree of calibration directly, but through decomposition results, we will show how the scores can be decomposed into various components, including the calibration loss. 

==> sections/A_response_letter.tex <==
\section{Response Letter}

\response{Dear editor and reviewers, first of all we would like to thank you for your comments and suggestions. We have carefully considered them and improved the survey accordingly. We have used \newtext{a red font} in the survey to clearly indicate the most significant changes. Below, you can find your original response, suggested changes, and how we have addressed each of your suggestions.

In this response letter, we have used three types of text including colour and format to differentiate easily the original reviewers comments and our responses in the following manner:
}

% MPN: Feel free to change the formats, those are currently defined in the definitions.tex file
\begin{itemize}
    \item \opinion{Original text from the reviewers that did not require a change of the manuscript.}
    \item \suggestion{Original text from the reviewers that clearly indicated a suggestion or comment to improve the survey.}
    \item \response{Our responses indicating the changes that we have implemented.}
\end{itemize}


\subsection{Editor}

\opinion{
All reviewers are quite in favour of the paper and emphasise the timeliness of the topic. Besides, they acknowledge the expertise of the authors on the topic and highlight some additional strengths of the paper, for example that it is accompanied by a software library.}
\suggestion{That said, they also have a couple of suggestions to further improve the paper. For example, the style of presentation is criticised for being somehow in-between a tutorial introduction (more like a textbook) and a survey paper. Moreover, suggestions are made for reorganisation of the paper, for shortening some parts and expanding others, and also for adding additional material. The authors are kindly invited to revise the paper according to the comments and suggestions of the reviewers.
}

\response{We have adapted the style of the presentation to be more in line with a survey paper; in particular, Section 2 has been significantly rewritten and is now shorter and more in line with the rest of the survey. We have also reorganised some sections of the paper and added additional material as suggested. The point-wise list of responses can be found in the following sections.}

\subsection{Reviewer 1}

\opinion{
This paper presents a survey on classifier calibration. The papers most of the typical topics in this area, including reliability maps, calibration definitions for binary and multi-class problems, and methods to recalibrate, on a validation dataset, probabilistic models that are not calibrated.

Overall the paper is very well structured, and very useful readers that are new to the field. On the other hand, the material is a bit lengthy for readers that have already expertise on classifier calibration.

The authors have an extensive expertise on the topic, and they manage to explain the concepts in an accessible way. In addition, the software package that comes with this paper is really excellent.

I would recommend to accept this paper after a revision. Below I am giving some specific comments per section.
}

\suggestion{
Section 2:

Especially the first part of this section is very introductory (but this might be appreciated by people that are new to the field). Also, Section 2.1, the discussion about the cost functions is quite long. In fact, the only thing you want to say here is that the Bayes-optimal decision changes when the cost changes, so it is important to have calibrated probabilities.
}

\response{Section 2 has been significantly rewritten to bring it more in line with the rest of the paper, and is now considerably shorter (7 rather than 11 pages).}


% \suggestion{
% In Section 2.2 the space between two lines suddenly becomes smaller. Looks a bit weird.
% }

% \todo[inline]{MPN: I am not sure what this means. Maybe LaTeX adjusted the spacing to fit the content? I propose the following sentence:}
% \response{The problem with the spacing has been fixed.}

\suggestion{
Figure 5: mapping the resulting output back to the x-axis -\textgreater  probably you mean mapping back to the diagonal line.
}

\response{This has been corrected (Figure 5 is now Figure 4).}

\suggestion{
In Figure 4 and 5 I would suggest to add names for the horizontal and vertical axis.
}
%\todo[inline]{PF: to add names to the axes of figures 3 and 4.}

\response{Done.}

\suggestion{
Logistic scaling: you refer to Platt (2000), but you don't mention here that this is Platt scaling. It would be useful to say that at this stage already.
}

% \todo[inline]{MPN: Not sure if the reviewer refers to the paragraph "The logistic curve is [...]. Following J. Platt (2000) [...]." in page \pageref{page:platt}}
\response{Done.}

% \suggestion{
% P12: classifier scores (which/that) are far…
% }

% \todo[inline]{MPN: I can not find this sentence}

\suggestion{
Multi-class calibration: it is an added value that the different notions of calibration are formally introduced for the multi-class case. I would argue that a formal definition would also be useful for the binary case.
}
%\todo[inline]{MPN: Find a place in Section 2 to add the formal definition for the binary case. (HS: check the new text above section 2.1).}

\response{We have added a formal definition of binary calibration before Section~\ref{sec:int:why}.}

\suggestion{
Concerning the strongest notion, no reference is given. In
Widmann et al. Calibration tests in multi-class classification: A unifying framework Advances in Neural Information Processing Systems 32 (NeurIPS 2019)
This is called "calibration in the strong sense". I would recommend to add this reference.
}
\response{Done.}

\suggestion{
Section 3:

It is useful to have a section about proper scoring rules in a survey about classifier calibration, but this section is a bit disconnected from the rest of the paper. Are proper scoring rules used in Sections 4 and 5? I would suggest to place Section 3 after Section 4. Perhaps also mention why this topic is covered.
}

% \todo[inline]{TF: Answer how the changes that have been made to Chapter 3 are better than the change of order. Another option is to change the order, but this may create some inconsistencies.}

\response{We have modified Chapter 3 to better introduce the importance of proper scoring rules.}

\suggestion{
Section 4.2:

Maximum calibration error -\textgreater  perhaps add a few references, see for example in the paper of Widmann et al.
}

\response{We have added an appropriate reference for MCE.}

\suggestion{
Section 5:

Very nice overview of calibration techniques. 
Please add for all calibration methods at least one reference, for example, a reference to the paper where the method was proposed for the first time.
}

\response{We have added the appropriate references the first time we mentioned each calibration method.}

\suggestion{
Section 6:

Calibration tests, as discussed in Section 6.1 are very important, because calibration metrics as such don't give enough insight whether a model is calibrated or not. So, this is a very important section of the paper. However, for me, Section 6.1 is very incomplete. I am aware of at least two other types of statistical tests.

-       The Hosmer-Lemeshov is used in statistics to test whether a logistic regression model is calibrated (binary and multi-class classification). As far as I know, this test can be used as well for other types of probabilistic classifiers. In fact, there is quite a lot of literature about this test. An advantage over the test of Vaicenaivicius is that resampling is not needed.

-       The above paper of Widmann et al. presents a kernel-based test that can be used in combination with many calibration metrics. This test has as main advantage that binning can be avoided.
}

\response{Following this and other reviewers' suggestions, we have repurposed Section~\ref{sec:hyp} which is now entirely for hypothesis tests (previously Section 6.1).  We have now included the definition of the Hosmer-Lemeshov test and its extension to evaluate the goodness-of-fit of multinomial logistic regression. We have also mentioned the kernel-based measure by Widmann et al. (2019).}

\subsection{Reviewer 2}

\opinion{
First of all, I would like to congratulate the author to a very interesting paper. I think it is in many ways the perfect introduction to the problem with classifier calibration, its importance and the existing techniques.

Consequently, I think publishing this paper will benefit many researchers and practitioners in machine learning. 

Having said that, I'm not sure that it is, in its current form, a very good fit for the Machine Learning journal, and it is not, in my opinion, a typical survey paper.
}

\suggestion{
First of all, the paper is quite long! One reason is that it starts from the absolute basics, but it is also very very detailed. The authors say that it has originated from a tutorial, and this is obvious. There is a lot of reasoning, really trying to lead the reader one step at the time by using many examples and even phrases as "let's play around with". In my opinion, this part of the paper is very pedagogical, but it might actually be a better fit for a textbook than for a survey paper.
}

% \todo[inline]{MPN: We made the paper still longer from 47 to 52 pages (without references). I propose the following response.}

\response{We have removed or compressed the most introductory material from Section 2. We have had to add material in response to the reviewer's comments but have tried to be as concise as possible in this revision.}

\opinion{
The section about multiclass is probably the most important one, introducing and summarizing the concepts in a very good way. As the authors say, the understanding in the machine learning field of calibration for multiclass is generally much weaker than for the binary case.    
}

\suggestion{
While I find the sections about proper scoring rules and evaluations and visualizations very well written and interesting, they are again rather long and potentially too detailed. To be clear, I think they definitely add value to the paper, but I would not consider these sections mandatory in a survey about calibration and calibration techniques. Of course, evaluation and the metrics must be covered but, if needed, these sections could probably be reduced.
}
\response{In our opinion, evaluation is equally important as calibration, and indeed another reviewer asked for more material on hypothesis tests for calibration, so we decided to keep these sections equally detailed.}

\opinion{
I find Chapter 5.1-5.4 to be another really strong part of the paper, and I like the fact that examples are used to illustrate the different techniques. Again, however, techniques that most readers probably are familiar with (Platt scaling and Isotonic regression) are described in great detail, while to be honest,} \suggestion{the less well-known techniques for multiclass, are more summarized.}

\suggestion{
The section 5.5 (Related work) is not as strong though. It is a very quick walkthrough of a number of recent papers, and the criteria for inclusion are not obvious. The papers are also more or less just mentioned, rather than described in terms of approach and main contributions. I think for a survey paper rather than just a tutorial paper, improving this section - or maybe rather integrate parts of it in the presentation of the techniques - is necessary. Actually, discussing recent papers in a survey as "related work", while presenting basic approaches in great detail is somewhat unorthodox.
}

\response{We have expanded the previous Section 5.5 and reorganised in order to include multiple subsections of more specific topics, such as non-post-hoc calibration methods and non-classification settings.}

% \todo[inline]{HS: check response after final changes made.}

\suggestion{
I am not convinced about the heading "Advanced topics" for chapter 6.2, and I think this is a questionable section altogether. Parts of it could be merged with earlier sections, and parts of it may not be necessary to include at all.
}

\response{We have merged the topics in this section to the new Section 5.7, where we discuss calibration methods for general predictive settings.}

% \todo[inline]{HS: check response after final changes made.}

\suggestion{
I think the section 6.3 should be removed; it doesn't really add anything to a paper focused on classification. 
}

\response{The regression setting is now briefly discussed in Section 5.7 with more focus on recent development.}

% \todo[inline]{HS: check response after final changes made.}

\opinion{
I would also like to mention the fact that the paper is accompanied with a software package, which is great.
}

\suggestion{
Before summing up I would like to highlight two things (on very different levels) that I am actually missing.
}

\suggestion{
1. I would argue that a survey paper about calibration has to include the "prediction with confidence" framework developed by Vovk et al., i.e., conformal prediction and - for this paper - in particular Venn prediction. These techniques have unique validity guarantees, and they have in the last few years almost exploded with a lot of papers being published. In addition, I think their approach to calibration, and how they describe it and reason about are valuable in itself. One good starting point is the paper Venn-Abers Predictors https://arxiv.org/pdf/1211.0025.pdf but there are many related papers, both earlier and later.
}

\response{We have included a discussion about Venn predictors and conformal prediction in Section 5.5.}

\suggestion{
2. I believe - from a practitioner's perspective - that it might have been interesting to reason about actual machine learning algorithms, and maybe even suggest which calibration techniques that work the best with these algorithms. After all, being overconfident or underconfident is often an inherent property of the algorithm, e.g., decision trees are generally (very) overconfident and random forests are typically underconfident, at least for higher confidence values.
}

\response{We have added a list of take-home messages at the end of Section~\ref{sec:conclusion} (\nameref{sec:conclusion}), addressing the more empirical steps that a common practitioner may need to follow.}

% \todo[inline]{TF: check response after final changes made.}

% % \suggestion{
% % So - in summary - I really liked the paper, and I think a lot can be learned from it. I think, however, that it may be too long in its current format so I would suggest trying to shorten it - but keeping it pedagogical. So, I don't suggest removing, for instance, a lot of examples but rather thinking carefully about what parts that really are needed for the overall story.
% % }

% % \suggestion{
% % For a survey paper (in contrast to a tutorial paper) I think the current state-of-the-art must be better described. What is now covered in "related work" is an embryo of this, but it would need to be expanded, and preferably structured - maybe even using some kind of taxonomy. I would appreciate a processed overview of the state-of-the-art, and the most important open questions.
% % }

% % \suggestion{
% % The other alternative is, of course, to make it a more outright tutorial paper.
% % }

% % \suggestion{
% % Finally, in my opinion, Venn prediction must be covered.
% % }

% \response{We have extended Section 5.5 to include a discussion about Veen predictors.}



\subsection{Reviewer 3}

\opinion{
This survey paper gives an overview of the area of classifier
calibration, mostly in the context of binary and multi-class
classification. The authors cover proper scoring rules, visualization
of classifier calibration through reliability diagrams, metrics to
assess classifier calibration, and techniques for post-training
calibration of classifiers.

The topic is timely as classifier calibration has received a
resurgence of attention lately, with a number of workshops dedicated
to the topic and the more general issue of uncertainty estimation. The
paper is generally well written, with many toy examples that aid in
the understanding of the concepts presented. If anything, the
explanations are a bit basic, so the paper reads more like a textbook
chapter than than a survey.

Before offering my suggestions to improve the paper I do want to
acknowledge that this type of paper is hard to write and easy to
criticize. That being said, I would like to suggest some suggestions
that I feel would significantly improve the paper:
}

\suggestion{\textbf{1.}
Cover more recent developments in the area. The most recent
technique covered in the survey is from 2019. The most recent one in
the context of binary classification is from 2017. I realize
that part of the authors' motivation is to cover classifier
calibration from a historical perspective, but showing how this
perspective is relevant to current research would improve the paper.
}

\response{In sections 5.5, 5.6 and 5.7 we added discussion on more recently published methods on the general topic of calibration, up to the end of 2022.}

% \todo[inline]{HS: check response after final changes made.}

\suggestion{\textbf{2.}
One more recent topic that I wish the authors would have dedicated
more attention to is that of out of distribution prediction, and the
distinction between aleatoric and epistemic uncertainty. One reason
this topic is important to cover is that out of distribution
prediction is a failure mode for the post-training calibration techniques
presented in this survey. For instance, temperature scaling works well
if the test data comes from the same distribution as the training
data, it still tends to lead to over-confident predictions in regions
of the space where the model has seen little/no data during training/calibration.
}

%\todo[inline]{MK to add to intro that this is out of scope.}
% \todo[inline]{MPN: We should make sure that in some part of the survey we indicate that classifier calibration does not deal with out of distribution. I propose a response like the following, but we need to be sure it is true.}
% \todo[inline]{HS: In Section 5.5, we have discussed method that can both improve IID calibration, as well as improve uncertainty estimates on OOD data points.}

\response{We agree that achieving robustness of calibrated classifiers under conditions of distributional shift and out-of-distribution inputs is a very important challenge. It is a very active field of research now and the problem is definitely not solved yet. However, we see this field as out-of-scope of our paper. We have now explicitly stated in the introduction that we focus on the setup where the classifier is deployed in the same setting where it was calibrated, except for potential changes in class prior or misclassification costs.}

% \response{As you indicated, classifier calibration is not intended to be used on out of distribution data. We have clarified that in Section \textcolor{red}{X} and discussed the out of distribution and epistemic uncertainty in Section 5.}

\suggestion{\textbf{3.}
While I understand that the paper is focused on post-training
calibration, I thing it would be useful to also discuss techniques
that aim to train well calibrated classifiers directly, such as deep
ensembles and mix-up.
}

% \todo[inline]{Check if we have mentioned non-post-hoc calibration methods and respond.}
% \todo[inline]{HS: 5.5.1 is now totally on this topic. Revisit after restructuring.}
\response{Section~\ref{sec:cal:training} is now on the topic of training models with a better level of calibration.}

\suggestion{\textbf{4.}
I really noticed the absence of any real case study. Ideally the
authors would show how to apply the presented techniques to a real
application where classifier calibration is critical.
}

% \todo[inline]{Check if we have mentioned real applications of calibration and its importance. Probably in Section 6.2 A cost-based view, or somewhere in the introduction.}
% \todo[inline]{HS: Sec 5.5.4 is about appications. Revisit after restructuring.}
\response{In Section~\ref{sec:cal:app} we have added discussion on links to other research fields and applications}

\suggestion{\textbf{5.}
It would be great if the authors could discuss the current state of
the research in the field and open problems.
}

\response{A new paragraph covering open problems was added at the end of Section~\ref{sec:conclusion}.}

% \todo[inline]{TF/HS: Ensure that after lessons learned we add some discussion of current open problems: second-level uncertainty, aleatoric/epistemic uncertainty, out of distribution, better metrics, better binning}

\suggestion{\textbf{6.}
While I like that the authors discussed proper scoring rules and their
decompositions, that section seemed too disconnected from the rest of
the paper. I think it would be hard for reader unfamiliar with calibration (which
seems to be the target audience of this tutorial paper) to understand
what is the relevance of proper scoring rules for calibration. A more
concrete discussion of how proper scoring rules are applicable to
calibration, and a more consistent use of them throughout the paper
would help. Alternatively, maybe moving the section later in the
paper, after the calibration metrics and visualizations have been
introduced, might help highlight the connection. Also, the explanation of
the decomposition also seemed confusing to me
}

\response{We have kept the order of the Sections but we have clarified in the text some of the calibration methods that rely on proper scoring rules.}

\suggestion{\textbf{7.}
In section 4 the authors present a number of metrics to measure
calibration. It would be good if they can contrast the different
metrics: when should one metric or another be used? why should one
even use these calibration metrics rather than a proper scoring rule
like brier score or log-likelihood? At a minimum, the authors should
emphasize that the calibration metrics can be easily minimized by
reducing resolution, and should always be used in conjunction with
other metrics.
}

\response{We have extended the Section~\ref{sec:metrics} about calibration measures clearly indicating that the number of bins is important, and that complementary metrics should be used in conjunction.}

\suggestion{\textbf{8.}
When discussing Platt scaling, the authors describe a cross-validation
scheme for calibrating the models. These scheme is not particular to
Platt scaling, it can be used with any post-training calibration
technique. Maybe the authors should discuss the training schemes in a
general context, or at least mention that the same approach is
applicable to all techniques if there is not enough data to have a
separate calibration set.
}

% \todo[inline]{This is true and we did not address it.}
% \todo[inline]{HS: 5.1 covers that now, please write response. MPN: I propose the following response:}
\response{We have now clearly defined in Section 5.1 two common training schemes that can be used in post-hoc calibration.}


\suggestion{\textbf{9.}
In section 6.1 the authors should explain the algorithm, and the
intuition behind it.
}

\response{We have extended Section 6.1 which now includes the formulation and a step by step example that can provide the intuition behind the algorithm.}

\suggestion{\textbf{10.}
Section 6.3 should be significantly expanded, or removed from the
paper. As it is, it is confusing and incomplete. When most readers
think about regression they only think about learning a function
f:X-\textgreater R, not about quantile or distribution regressions. The different
types or regression should be better explained and differentiated. How
would on e even train a quantile or distribution regression model?
Also, calibration procedures are not explained at all in the paper, just
"demonstrated" in a figure. Are there any techniques for distribution
calibration? If so they should be described too.
}

% \todo[inline]{HS: please respond to this. MPN: I propose something like this:}

\response{We have removed Section 6.3 Calibration for regression, and created a new Section \ref{sec:cal:other} that provides a general overview of calibration methods for other predictive settings.}

\suggestion{
Typos: Beta calibration, last paragraph: can only model-specific --\textgreater 
can only model specific 

equation 12, (s;a,b,c) --\textgreater  g(s;a,b,c)
}

\response{We have revised the survey and fixed the typos.}

==> sections/A_reviewers_comments.tex <==
\section{Review: 06/06/2022}


The reports from the reviewers of your manuscript, "Classifier Calibration -- How to assess and improve predicted class probabilities: a survey", which you submitted to Machine Learning, have now been received.

Based on the advice received, your manuscript requires major revisions in order to be acceptable for publication.
It is the policy of Machine Learning not to accept manuscripts requiring major revisions.
Instead, authors choosing to revise their manuscript according to the reviewers' comments must resubmit a revised manuscript, which usually will be reassessed by the same action editor.

When preparing your revised manuscript, you should carefully consider the reviewers' comments, and submit a point wise list of responses to the comments.
Your list of responses should be uploaded as a separate file in addition to your revised manuscript.

Your revision is due by 03 Dec 2022.

Please make sure to submit your editable source files (i. e. Word, TeX).

COMMENTS FOR THE AUTHOR:

Editor: All reviewers are quite in favour of the paper and emphasise the timeliness of the topic. Besides, they acknowledge the expertise of the authors on the topic and highlight some additional strengths of the paper, for example that it is accompanied by a software library. That said, they also have a couple of suggestions to further improve the paper. For example, the style of presentation is criticised for being somehow in-between a tutorial introduction (more like a textbook) and a survey paper. Moreover, suggestions are made for reorganisation of the paper, for shortening some parts and expanding others, and also for adding additional material. The authors are kindly invited to revise the paper according to the comments and suggestions of the reviewers.


\subsection{Reviewer 1}

This paper presents a survey on classifier calibration. The papers most of the typical topics in this area, including reliability maps, calibration definitions for binary and multi-class problems, and methods to recalibrate, on a validation dataset, probabilistic models that are not calibrated.

Overall the paper is very well structured, and very useful readers that are new to the field. On the other hand, the material is a bit lengthy for readers that have already expertise on classifier calibration.

The authors have an extensive expertise on the topic, and they manage to explain the concepts in an accessible way. In addition, the software package that comes with this paper is really excellent.

I would recommend to accept this paper after a revision. Below I am giving some specific comments per section.

Section 2:

Especially the first part of this section is very introductory (but this might be appreciated by people that are new to the field). Also, Section 2.1, the discussion about the cost functions is quite long. In fact, the only thing you want to say here is that the Bayes-optimal decision changes when the cost changes, so it is important to have calibrated probabilities.

In Section 2.2 the space between two lines suddenly becomes smaller. Looks a bit weird.

Figure 5: mapping the resulting output back to the x-axis -> probably you mean mapping back to the diagonal line.

In Figure 4 and 5 I would suggest to add names for the horizontal and vertical axis.

Logistic scaling: you refer to Platt (2000), but you don't mention here that this is Platt scaling. It would be useful to say that at this stage already.

P12: classifier scores (which/that) are far…

Multi-class calibration: it is an added value that the different notions of calibration are formally introduced for the multi-class case. I would argue that a formal definition would also be useful for the binary case.

Concerning the strongest notion, no reference is given. In
Widmann et al. Calibration tests in multi-class classification: A unifying framework Advances in Neural Information Processing Systems 32 (NeurIPS 2019)
This is called "calibration in the strong sense". I would recommend to add this reference.

Section 3:

It is useful to have a section about proper scoring rules in a survey about classifier calibration, but this section is a bit disconnected from the rest of the paper. Are proper scoring rules used in Sections 4 and 5? I would suggest to place Section 3 after Section 4. Perhaps also mention why this topic is covered.

Section 4.2:

Maximum calibration error -> perhaps add a few references, see for example in the paper of Widmann et al.

Section 5:

Very nice overview of calibration techniques. 
Please add for all calibration methods at least one reference, for example, a reference to the paper where the method was proposed for the first time.

Section 6:

Calibration tests, as discussed in Section 6.1 are very important, because calibration metrics as such don't give enough insight whether a model is calibrated or not. So, this is a very important section of the paper. However, for me, Section 6.1 is very incomplete. I am aware of at least two other types of statistical tests.

-       The Hosmer-Lemeshov is used in statistics to test whether a logistic regression model is calibrated (binary and multi-class classification). As far as I know, this test can be used as well for other types of probabilistic classifiers. In fact, there is quite a lot of literature about this test. An advantage over the test of Vaicenaivicius is that resampling is not needed.

-       The above paper of Widmann et al. presents a kernel-based test that can be used in combination with many calibration metrics. This test has as main advantage that binning can be avoided.
 

\subsection{Reviewer 2}

First of all, I would like to congratulate the author to a very interesting paper. I think it is in many ways the perfect introduction to the problem with classifier calibration, its importance and the existing techniques.

Consequently, I think publishing this paper will benefit many researchers and practitioners in machine learning. 

Having said that, I'm not sure that it is, in its current form, a very good fit for the Machine Learning journal, and it is not, in my opinion, a typical survey paper.

First of all, the paper is quite long! One reason is that it starts from the absolute basics, but it is also very very detailed. The authors say that it has originated from a tutorial, and this is obvious. There is a lot of reasoning, really trying to lead the reader one step at the time by using many examples and even phrases as "let's play around with". In my opinion, this part of the paper is very pedagogical, but it might actually be a better fit for a textbook than for a survey paper.

The section about multiclass is probably the most important one, introducing and summarizing the concepts in a very good way. As the authors say, the understanding in the machine learning field of calibration for multiclass is generally much weaker than for the binary case.    

While I find the sections about proper scoring rules and evaluations and visualizations very well written and interesting, they are again rather long and potentially too detailed. To be clear, I think they definitely add value to the paper, but I would not consider these sections mandatory in a survey about calibration and calibration techniques. Of course, evaluation and the metrics must be covered but, if needed, these sections could probably be reduced.

I find Chapter 5.1-5.4 to be another really strong part of the paper, and I like the fact that examples are used to illustrate the different techniques. Again, however, techniques that most readers probably are familiar with (Platt scaling and Isotonic regression) are described in great detail, while to be honest, the less well-known techniques for multiclass, are more summarized.     

The section 5.5 (Related work) is not as strong though. It is a very quick walkthrough of a number of recent papers, and the criteria for inclusion are not obvious. The papers are also more or less just mentioned, rather than described in terms of approach and main contributions. I think for a survey paper rather than just a tutorial paper, improving this section - or maybe rather integrate parts of it in the presentation of the techniques - is necessary. Actually, discussing recent papers in a survey as "related work", while presenting basic approaches in great detail is somewhat unorthodox.

I am not convinced about the heading "Advanced topics" for chapter 6.2, and I think this is a questionable section altogether. Parts of it could be merged with earlier sections, and parts of it may not be necessary to include at all.

I think the section 6.3 should be removed; it doesn't really add anything to a paper focused on classification. 

I would also like to mention the fact that the paper is accompanied with a software package, which is great.

Before summing up I would like to highlight two things (on very different levels) that I am actually missing.

\begin{enumerate}
\item  I would argue that a survey paper about calibration has to include the "prediction with confidence" framework developed by Vovk et al., i.e., conformal prediction and - for this paper - in particular Venn prediction. These techniques have unique validity guarantees, and they have in the last few years almost exploded with a lot of papers being published. In addition, I think their approach to calibration, and how they describe it and reason about are valuable in itself. One good starting point is the paper Venn-Abers Predictors https://arxiv.org/pdf/1211.0025.pdf but there are many related papers, both earlier and later.

\item I believe - from a practitioner's perspective - that it might have been interesting to reason about actual machine learning algorithms, and maybe even suggest which calibration techniques that work the best with these algorithms. After all, being overconfident or underconfident is often an inherent property of the algorithm, e.g., decision trees are generally (very) overconfident and random forests are typically underconfident, at least for higher confidence values.
\end{enumerate}

So - in summary - I really liked the paper, and I think a lot can be learned from it. I think, however, that it may be too long in its current format so I would suggest trying to shorten it - but keeping it pedagogical. So, I don't suggest removing, for instance, a lot of examples but rather thinking carefully about what parts that really are needed for the overall story.

For a survey paper (in contrast to a tutorial paper) I think the current state-of-the-art must be better described. What is now covered in "related work" is an embryo of this, but it would need to be expanded, and preferably structured - maybe even using some kind of taxonomy. I would appreciate a processed overview of the state-of-the-art, and the most important open questions.

The other alternative is, of course, to make it a more outright tutorial paper.

Finally, in my opinion, Venn prediction must be covered.



\subsection{Reviewer 3}

This survey paper gives an overview of the area of classifier
calibration, mostly in the context of binary and multi-class
classification. The authors cover proper scoring rules, visualization
of classifier calibration through reliability diagrams, metrics to
assess classifier calibration, and techniques for post-training
calibration of classifiers.

The topic is timely as classifier calibration has received a
resurgence of attention lately, with a number of workshops dedicated
to the topic and the more general issue of uncertainty estimation. The
paper is generally well written, with many toy examples that aid in
the understanding of the concepts presented. If anything, the
explanations are a bit basic, so the paper reads more like a textbook
chapter than than a survey.


Before offering my suggestions to improve the paper I do want to
acknowledge that this type of paper is hard to write and easy to
criticize. That being said, I would like to suggest some suggestions
that I feel would significantly improve the paper:

\begin{enumerate}
\item Cover more recent developments in the area. The most recent
technique covered in the survey is from 2019. The most recent one in
the context of binary classification is from 2017. I realize
that part of the authors' motivation is to cover classifier
calibration from a historical perspective, but showing how this
perspective is relevant to current research would improve the paper.

\item One more recent topic that I wish the authors would have dedicated
more attention to is that of out of distribution prediction, and the
distinction between aleatoric and epistemic uncertainty. One reason
this topic is important to cover is that out of distribution
prediction is a failure mode for the post-training calibration techniques
presented in this survey. For instance, temperature scaling works well
if the test data comes from the same distribution as the training
data, it still tends to lead to over-confident predictions in regions
of the space where the model has seen little/no data during training/calibration.

\item While I understand that the paper is focused on post-training
calibration, I thing it would be useful to also discuss techniques
that aim to train well calibrated classifiers directly, such as deep
ensembles and mix-up.

\item I really noticed the absence of any real case study. Ideally the
authors would show how to apply the presented techniques to a real
application where classifier calibration is critical.

\item It would be great if the authors could discuss the current state of
the research in the field and open problems.

\item While I like that the authors discussed proper scoring rules and their
decompositions, that section seemed too disconnected from the rest of
the paper. I think it would be hard for reader unfamiliar with calibration (which
seems to be the target audience of this tutorial paper) to understand
what is the relevance of proper scoring rules for calibration. A more
concrete discussion of how proper scoring rules are applicable to
calibration, and a more consistent use of them throughout the paper
would help. Alternatively, maybe moving the section later in the
paper, after the calibration metrics and visualizations have been
introduced, might help highlight the connection. Also, the explanation of
the decomposition also seemed confusing to me.

\item In section 4 the authors present a number of metrics to measure
calibration. It would be good if they can contrast the different
metrics: when should one metric or another be used? why should one
even use these calibration metrics rather than a proper scoring rule
like brier score or log-likelihood? At a minimum, the authors should
emphasize that the calibration metrics can be easily minimized by
reducing resolution, and should always be used in conjunction with
other metrics.

\item When discussing Platt scaling, the authors describe a cross-validation
scheme for calibrating the models. These scheme is not particular to
Platt scaling, it can be used with any post-training calibration
technique. Maybe the authors should discuss the training schemes in a
general context, or at least mention that the same approach is
applicable to all techniques if there is not enough data to have a
separate calibration set.

\item In section 6.1 the authors should explain the algorithm, and the
intuition behind it.

\item Section 6.3 should be significantly expanded, or removed from the
paper. As it is, it is confusing and incomplete. When most readers
think about regression they only think about learning a function
f:X->R, not about quantile or distribution regressions. The different
types or regression should be better explained and differentiated. How
would on e even train a quantile or distribution regression model?
Also, calibration procedures are not explained at all in the paper, just
"demonstrated" in a figure. Are there any techniques for distribution
calibration? If so they should be described too.
\end{enumerate}

Typos: Beta calibration, last paragraph: can only model-specific -->
can only model specific 

equation 12, (s;a,b,c) --> g(s;a,b,c)


==> sections/A_todos.tex <==
\section{TODOs}

\newtext{MPN: I have added a new command in the definitions.tex called \textbackslash newtext\{\#text\} to modify the submitted version and keep easy track of the modifications in red. This paragraph is an example.}

%\begin{itemize}

    %\item PF-Intro: Finalise running example and figures.
    %\item PF-Intro: Deal with comments.
    %\item PF-Intro: Discuss the relationship between the different definitions of calibration.
    %\item PF-Intro: forward reference to $c$ optimal threshold discussion in S.5
    % \item HS-Intro: Develop argument why $c$ is optimal threshold even if probabilities are not Bayes-optimal (Done)
    %\item MPN-Intro: Change figures to the final reliability diagrams.
    % \item Eval: Add Definitions for each metric
    % \item Eval: Discuss different binning strategies
    %  \item TSF-Eval: Decide if Multiclass calibration subsection should be moved to evaluation section
    %  \item TSF-Eval: Table 2: add gap between p and y? They could show MCE on every row, and ECE in a final row (weighted average difference) (check if doable)
    %\item MPN-Vis: Think about PyCalib moved to an appendix
    % \item PF-Vis: Remove subfigures that are already in other sections, and refer to them. -- done, not really needed
    %\item All-All: Adjust all tables only with horizontal lines (use Table 7 as a reference)
    %\item MPN-Eval: Add text about Vaicenavicius et al 19. Changed to add text about Brocker et al. 2007
    %\item MPN-Vis: Add math's notations and explanation for reliability diagrams.
    %\item MPN-Vis: Reliability diagrams section finalise draft.
    %\item MPN-Vis: Move section to the end of Eval? Moved to the begining.
    % \item RSR-Vis: Look at the reliability diagram text.
    % \item MPN-Eval: Rephrase visualisation section now that we have a final ordering.
    %\item MPN-Eval: Think about the ordering of the subsections in Eval.
    %\item MPN-all: Fix issue making multiple citations in only one command cite.
    % \item Eval: Raul's paper already had reliability diagrams for the confidence only in binary case. Maybe we need to refer to that when talking for the first time conf-ECE
    % \item Eval: Add some text about why would be useful to use expected instead of maximum calibration error.
    % \item Eval: Reference to Dirichlet Cal paper when talking about classwise-MCE.
    % \item Eval: Mention the issues that could arise from MCE.
    % \item Eval: Mention that classwise-MCE could be also defined as expected maximum, or maximum expectation.
    % \item Eval: The end of the MCE/ECE part talks about optimization. Given that the section is not about optimization we could rephrase just to describe that they can have a minimumm value by predicting the prior probability.
    % \item TSF-RSR-Eval: Proper scoring rules requires an introduction about why are we covering proper scoring rules.
    % \item MPN-TSF-Eval: Log-loss (aka cross entropy).
    % \item TSF-Eval: Discuss the proper losses which can be computed as instance level but they may be proper only when the number of samples goes to infinity.
    % \item TSF-Eval: Expand proper scoring rules section.
    % \item Vis: Add visualisations section Evaluation: Reliability diagrams
    % \item Vis: Add literature review of uses of reliability diagram
    %\item Cal: Need the definition of the true calibration map somewhere.
    %\item Cal: Clarify what it is referred as "new feature values" 
    %\item Cal: Clarify how equation 9 is introduced in the text. 
    %\item Cal: Explain in the text what are the figures 16 and 17 showing.
    %\item Cal: For all calibration methods (eg. isotonic regression), before talking about the parameters maybe explain shortly in words what the method consist on.
    %\item Cal: Make reference to word that "can prove that , the learning algorithm is equivalent to optimise the loss" in equation 11.
    %\item Cal: Temperature scaling is known by deep practitioners with a different equation (no logits involved). Think about explaining the known version of the function first, and then maybe introduce the logits if necessary.
    %\item Cal: explain the rest implementation for Platt scaling
    % \item HS-All: unify notations (done, need others checking)
    %\item HS-cal: add a notation table. (done, need to decide what to do with it.)
    % \item HS-Cal: response to Meelis's comments (mainly figures and structure, also change to Miquel's style. For MPN and MK to check HS response. Style done.)
    %\item MPN-Cal: Check responses to my comments in HS section
    % \item MK-Cal: Check responses to HS comments in Calibration Methods section (Done)
    % \item HS-Cal: consider other ways of giving a unified comparison. (Probably Github online page, not easy with a single picture in paper) 
    % \item HS-Adv: move calibration tests. (Done)
    % \item HS-Cal: Check again for quality control (e.g. Figure layout)
    % \item HS-Cal: figures that compare different calibration approaches (Done, but all the lines are not distinguishable)
    % \item HS-Conclusion: expand regression calibration (Done)
    % \item HS-S5: add reference for classification-calibrated (Done).
    % \item MK-S5: read and comment Advanced Topics section
    % \item PF-S5: read and comment Advanced Topics section
    % \item HS-S5: Think about citing Peter's JMLR paper -> reference added but some further text needed? (The cost sensitive part texts explain some idea, to discuss if Peter wants to cover anything else.)
    %\item All-Conclusion: PF has written first draft, please check; MK checked - ok.
    % \item HS-References: Clean again the bibtex. (Done)
    % \item HS-add references and related work -- is this done? (Done)
    %\item MPN-Overall: Refactor all section numbers in text files (need to coordinate with everybody not to create file conflicts).
    %\item HS: fix incomplete citation at the end of Section \ref{sec:calibrators}
    %\item MK: decide what to do with comment in Section \ref{sec:decomp}
    %\item All: write abstract (PF: done, please check) and titlepage
    %\item All: complete Contribution table in Section \ref{sec:contribution}, then compile into text
    %\item MPN: Add list of authors based on the contribution table. 
    %\item TSF: Add section for contributions based on the table. Instructions indicate the following: These contributions should be listed at the separate title page
    %\item MPN: Adapt text about PyCalib to fit the end of the introduction section.
    %\item MPN\&TSF: Prepare all the submission requirements.
    %\item MPN\&TSF: Related papers for the submission: Mention Eyke concept of uncertainty as related, and Raul's found paper of 1957 (or around)
    %\item MPN: Name your figure files with "Fig" and the figure number, e.g., Fig1.eps.
    %\item TSF: Check PyCalib text (previous to last paragraph of the introduction section)
    %\item MPN: Remind Telmo to prepare a TODO list with the necessary changes.
%\end{itemize}

\subsection{List}
\begin{enumerate}
    \item \done TSF: Connect Section 3 with the rest of the paper
        \newtext{\begin{itemize}
            \item Added new text to the first paragraph of page 16 
            \item Added new text to the last paragraph of Section 4 
        \end{itemize}}
    \item \done TSF: Discuss more hypothesis tests on Section 6 \newtext{\begin{itemize}
            \item Added new text about goodness-of-fit tests to Section 6.1 (including an example of the multinomial HL test)  
        \end{itemize}}
    \item \done TSF: Add a new Section with take-home messages  
    \newtext{\begin{itemize}
            \item Added a new Section 7
            \item Maybe a good place to add some text about pycalib?
        \end{itemize}}
    \item \done PF: Compress Section 2
        \newtext{\begin{itemize}
            \item PF: Removed the more tutorial parts from the first half of S.2, now 9pp.
        \end{itemize}}
    \item \done HS: Add references for the calibrators 
    \item HS: Improve (and rename) Section 5.5 (perhaps include conformal predictions and Venn predictors here?) (initially done)
    \item HS: Add additional introduction to more recent calibration methods. Improve the related work section. 
    
    \item HS: move compressed version of Cal for regression to 5
    \item \done TSF: add reference about hyp tests for calibration for regression
    \item \done TSF: rename section 6
    
    \item \done MPN: Improve positions of figures starting from Fig. 20; they're all bundled up at the end
    \item \done HS: Decide if we want to change the font and size of the figures in the calibrator's section (MPN: I changed Fig.12 (a) and (b) as an example). Decided, we will change them in the final version.
    \item MPN/HS: Increase size of fonts in figures.
\end{enumerate}

\subsection{E-mail: Peter considerations after a discussion with Eyke}

Thanks Telmo. I saw Eyke a few days ago and we briefly discussed the paper. I got the impression that we shouldn't feel obliged to follow all recommendations from the reviewers, so I suggest we prioritise a few that we really need to follow up. Here is my suggestion: 

Section 2: I can compress and perhaps move the most introductory material to an online location. 

Section 3: Needs better connection with the rest as suggested by Telmo. 

Section 5.5 needs improving. 

Conformal prediction and Venn predictors need to be covered somewhere. 

We need to cover more hypothesis tests. Perhaps that should be the real focus of Section 6. The main points of 6.2 and 6.3 could perhaps be stated elsewhere: e.g., that once you consider calibration for regression you realise that the main goal of calibration is to estimate the distribution of Y|X, which could be said in the conclusions. 


\subsection{E-mail: Telmo's considerations after reading the responses}

I was checking the comments to try to come up with the beginnings of a plan for changes and rebuttal. Sorry for the long email.

First of all, it seems clear that the referees thought the paper’s writing style is closer to a textbook or “tutorial paper” than a survey and this could be expected, but I’m not sure if we would want to change the way we wrote it, to decrease the tutorialness of the paper in order to increase its surveyness. And making it more of a survey without reducing a bit of the pedagogical content would make the paper even longer.

They had some reservations about the proper scoring rules section and felt it was a bit disconnected from the rest of the paper and comment 3.7 said

“when should one metric or another be used? why should one even use these calibration metrics rather than a proper scoring rule like brier score or log-likelihood? … emphasize that the calibration metrics can be easily minimized by reducing resolution, and should always be used in conjunction with other metrics”.

Some comments also mentioned having Section 3 later in the paper. I think we could keep the proper scoring rules section where it is, but try to connect the calibration metrics section back to them, with the motivation to use more than one metric. We can also connect Section 3 more with the calibration methods, by mentioning in Section 3 which algorithms discussed later use each proper scoring rule as its loss function. This is mentioned in each algorithm’s Section, but we can reinforce it.

Reviewers also thought Section 6.3 should be better explained or removed altogether. Even though it’s a short part of the paper, I think removing it would give us some space to discuss some of the suggestions.

Section 5.5 was also mentioned as a point of improvement. Perhaps we could rename it to Recent Advances and focus on better explaining more recent papers in more detail as the other parts of Section 5 do?

Finally, some of the topics they asked us to discuss, such as conformal predictions, calibration during training and the change to Section 5.5 mentioned above, would increase the length of the paper even more, definitely taking us into short textbook territory, unless we can decide on some cuts to our current sections. What do you think?

==> sections/OLD_01_intro.tex <==
\section{Introduction}
\label{sec:intro}

% adapted from Neurips 2019

A $K$-class probabilistic classifier is \emph{well-calibrated} if among test instances receiving a predicted $K$-dimensional probability vector $\mathbf{s}$, the class distribution is (approximately) distributed as $\mathbf{s}$. % \citep{isotonic}. 
This property is of fundamental importance when using a classifier for cost-sensitive classification, for human decision making, or within an autonomous system.
It means that the classifier correctly quantifies the level of uncertainty or confidence associated with its predictions. 
%Due to overfitting, 
Many machine learning algorithms are known to produce over-confident models, unless dedicated procedures are applied during training. 
%(e.g., Laplace smoothing in decision trees \cite{ferri2003improving}).
The goal of \emph{(post-hoc) calibration methods} is to use hold-out validation data to learn a \emph{calibration map} for a previously trained model that transforms the model's predictions to be better calibrated.

%%% A probabilistic classifier is \emph{well-calibrated} if among test instances receiving a predicted probability vector $p$, the class distribution is (approximately) distributed as $p$ \citep{isotonic}. 
%%% %In this sense, perfect calibration can be crudely approximated by a constant classifier predicting the overall class distribution for every instance.
%%% %
%%% % Calibration is closely related to optimal decision making and cost-sensitive classification, where we wish to determine the predicted class that minimises expected misclassification cost. 
%%% In a binary setting, scores given by a sufficiently calibrated classifier can be simply thresholded to minimise expected misclassification cost \citep{isotonic}. Thresholds can also be derived to optimally adapt to a change in class prior, or to a combination of both. In contrast, for a poorly calibrated classifier the optimal thresholds cannot be obtained without optimisation; for example, by means of ROC analysis \citep{provost2001robust}.

Meteorologists were among the first to think about probability calibration. 
\citet{brier1950} introduced an evaluation measure for probabilistic forecasts, which we now call Brier score.  \citet{murphy1977reliability} proposed reliability diagrams, which allow us to visualise calibration errors.  \citet{degroot1983} investigated proper scoring rules for forecaster evaluation and the decomposition of these loss measures into calibration and refinement losses. 
Since then, many calibration methods for binary classifiers have been introduced, including: 
\begin{itemize}
\item logistic calibration, also known as `Platt scaling' \citep{platt2000}; 
\item binning calibration \citep{zadrozny2001obtaining} with either equal-width or equal-frequency bins;
\item isotonic calibration \citep{barlow1972isotonic}, also known as the ROC convex hull method and pooled adjacent violators \citep{fawcett2007}; and
\item beta calibration \citep{kull2017beyond,pmlr-v54-kull17a}. 
\end{itemize}
%
Recent extensions of the above approaches were introduced by the following authors: 
\citet{naeini2015} perform Bayesian averaging of multiple calibration maps obtained with equal-frequency binning; 
\citet{naeini2016} use near-isotonic regression to allow for some non-monotonic segments in the calibration maps; and \citet{allikivi2019} introduce a non-parametric Bayesian isotonic calibration method.

When we have more than two classes, calibration is generally more involved, as is often the case with multiclass classification more generally. 
Multiclass calibration has mostly been approached by decomposing the problem into $K$ one-vs-rest binary calibration tasks \citep{fawcett2007}, one for each class. The predictions of these $K$ calibration models form unnormalised probability vectors, which, after normalisation, may not be calibrated in a multiclass sense. 
%
Native multiclass calibration methods were introduced recently with a focus on neural networks, including: matrix scaling, vector scaling and temperature scaling \citep{guo2017}, which can all be seen as multiclass extensions of Platt scaling and have been proposed as a calibration layer which should be applied to the logits of a neural network, before the softmax layer. 

An alternative to \emph{post-hoc} calibration is to modify the classifier learning algorithm itself, which has been pursued by several authors. 
MMCE \citep{kumar2018} trains neural networks by optimising the combination of log-loss with a kernel-based measure of calibration loss.
SWAG \citep{maddox2019} models the posterior distribution over the weights of the neural network and then samples from this distribution to perform Bayesian model averaging. 
%\cite{kumar2018trainable} argued that while trying to avoid neural network overconfidence, temperature scaling could penalise legitimately confident predictions. Therefore, they proposed a kernel based measure of calibration that can be trained alongside the negative likelihood loss and preserves high confidence predictions. 
%
\citet{milios2018} proposed a method to transform the classification task into regression and to learn a Gaussian Process model.
%\cite{milios2018dirichlet} showed Gaussian Processes can yield more calibrated results using a Dirichlet-based transform on the labels to form a regression task;  
%
Calibration methods have been proposed for regression tasks as well, adding confidence assessments to the scalar values predicted in regression. For example, the method proposed by \citet{kuleshov2018} adopts isotonic regression to calibrate the predicted quantiles.
The theory of calibration functions and empirical calibration evaluation in classification was studied by \citet{vaicenavicius2019evaluating}, also proposing a statistical test of calibration.
%and finally, \cite{vaicenavicius2019evaluating} studied the theory of calibration functions and empirical calibration evaluation, proposing a statistical test of calibration.
%a statistical test for calibration was provided in \cite{vaicenavicius2019evaluating}, which is done by approximating the distribution of probabilistic outputs under the hypothesis that the probabilities are calibrated.

% While there are several calibration methods tailored for deep neural networks, we propose a general-purpose, natively multiclass calibration method called \emph{Dirichlet calibration}, applicable for calibrating any probabilistic classifier.
%Similar to how Platt scaling was originally proposed for the continuous scores produced by SVMs and later used to calibrate probabilistic models, matrix, vector and temperature scaling could be applied to the probability estimates from non-neural network models, but some of their underlying assumptions would not be appropriate, as shown later in this paper. \cite{pmlr-v54-kull17a} proposed beta calibration as a parametric model with the correct support for probabilistic outputs. The multivariate extension of the beta distribution is the Dirichlet distribution, therefore we propose Dirichlet calibration as a natural extension of beta calibration to the multiclass scenario.
%
%While we are not the first to address multiclass calibration, 
As we will see later, the multiclass setting introduces numerous subtleties that have not always been recognised or correctly dealt with in previous work. 
For example, some authors use the weaker notion of \emph{confidence calibration}, which requires only that the classifier's predicted probability for what it considers the most likely class is calibrated. 
There are also variations in the evaluation metric used and in the way calibrated probabilities are visualised. 
Our main aim in this survey is hence to provide a unified perspective on the different methods for binary and multiclass calibration, as well as discuss empirical aspects such as evaluation metrics. 

% Consequently, Section~\ref{sec:temp:eval} is concerned with clarifying such fundamental issues. 
%
% \cite{song2019distribution} further generalises the concept by performing calibration on regression outputs at the level of conditional distribution. 
%\cite{kumar2018trainable} proposes a training measure based on kernel mean embedding that improves calibration on the obtained neural networks.
%A statically test for calibration is provided in \cite{vaicenavicius2019evaluating}, which is done by approximating the distribution of probabilistic outputs under the hypothesis of being calibrated.
%
% We then propose the approach of Dirichlet calibration in Section~\ref{sec:dirichlet}, present and discuss experimental results in Section~\ref{sec:experiments}, and conclude in Section~\ref{sec:discussion}.

The paper is structured as follows. 
The next section will cover important notions and intuitions related to calibration by way of introduction, leaving technical detail for later sections.  
% and how it can help with optimal decision making; exemplify what are some possible sources of miscalibration by means of simple examples; define the binary and multiclass scenarios together with corresponding visualisations; demonstrate how to obtain calibrated probabilities with simple techniques, such as binning methods; and propose different notions of multiclass calibration from the weakest to the strongest (confidence-calibrated, classwise-calibrated and multiclass-calibrated).
Section \ref{sec:psr} discusses proper scoring rules, an important framework for evaluation of probability estimates. 
Section \ref{sec:metrics} gives a systematic overview of visualisation approaches and evaluation metrics for calibration. 
In Section \ref{sec:calibrators} is devoted to a comprehensive account of post-hoc calibration methods for both the binary and multiclass scenarios. 
Section \ref{sec:out:conc} covers advanced topics including a cost-based view of classifier calibration and a hypothesis test for calibration, and Section \ref{sec:conclusion} concludes with a summary and outlook. 

==> sections/OLD_02_highlevel_intro.tex <==
\section{A high-level introduction to classifier calibration}
\label{sec:intro:high:level}
As already mentioned, weather forecasters started thinking about calibration a long time ago \cite{brier1950}. 
It is therefore appropriate to start with some simplified weather forecasting examples. 
%
\begin{quote}
    A forecast `70\% chance of rain' should be followed by rain 70\% of the time.
\end{quote}
%
%this is worth reading https://www.metoffice.gov.uk/about-us/what/accuracy-and-trust/probability#:~:text=In%20weather%20forecasting%2C%20suppose%20the,in%20your%20region%20is%2080%25.&text=So%20a%20forecast%20of%2080,experience%20rain%20where%20you%20are.%
%
This effectively says that the uncertainty in the forecast should be borne out by the data. Note that in weather forecasting there can be many sources of uncertainty: e.g., spatial uncertainty (does a rain forecast for Bristol mean that it will rain everywhere in Bristol?), temporal uncertainty (does a rain forecast for 4--5pm mean that it will rain the entire hour?), and even uncertainty regarding the proper definition of rain. We will not consider any of those issues here, and simply assume that `rain' is a binary, observable variable, much like a coin coming up either heads or tails.

This is in accordance with the account found on the UK Met Office website: 
\begin{quote}
    ``[S]uppose the Met Office says that the probability of rain tomorrow in your region is 80\%. They aren't saying that it will rain in 80\% of the land area of your region, and not rain in the other 20\%. Nor are they saying it will rain for 80\% of the time. What they are saying is there is an 80\% chance of rain occurring at any one place in the region, such as in your garden.
...
[A] forecast of 80\% chance of rain in your region should broadly mean that, on about 80\% of days when the weather conditions are like tomorrow's, you will experience rain where you are. 
%But there is still some expert judgement involved, and different forecasting organisations with different experts and different technology might well give different probabilities.
...
If it doesn't rain in your garden tomorrow, then the 80\% forecast wasn't wrong, because it didn't say rain was certain. But if you look at a long run of days, on which the Met Office said the probability of rain was 80\%, you'd expect it to have rained on about 80\% of them. '' (\url{https://www.metoffice.gov.uk/about-us/what/accuracy-and-trust/probability})
\end{quote}

Taking the forecast event as a binary variable means that the calibration concept is directly applicable to binary classification. Here is an example from the typical machine learning task of learning a classifier for distinguishing `junk' or `spam' emails from regular ones: 
%
\begin{quote}
    A prediction `70\% chance of spam' should be spam 70\% of the time.
\end{quote}
%
And a generalisation to categorical variables with more than two values is equally straightforward, as this example from Fisher's famous Iris dataset shows: 
%
\begin{quote}
    A prediction `70\% chance of setosa, 10\% chance of versicolor and 20\% chance of virginica' should be setosa/versicolor/virginica 70/10/20\% of the time.
\end{quote}
%
So, in general: \emph{A predicted probability (vector) should match empirical (observed) probabilities.}

But what does `$x\%$ of the time' mean? Clearly we can't say much about the degree of calibration of a single forecast. How do we aggregate forecasts in a reasonable way? As we will see, this question lies at the heart of both methods and metrics for calibration. 

\input{sections/02_1_alternative}

\subsection{A toy example}
\label{sec:int:toy}

Let's consider a small toy example, with eight forecasts using four different probabilities: 
\begin{itemize}
\item {Two forecasts of `10\% chance of rain' were both followed by `no rain'.}
\item {Two forecasts of `40\% chance of rain' were once followed by `no rain', and once by `rain'.}
\item {Three forecasts of `70\% chance of rain' were once followed by `no rain', and twice by `rain'.}
\item {One forecast of `90\% chance of rain' was followed by `rain'.}
\end{itemize}
Writing `rain' as $y=1$ and `no rain' as $y=0$, we can calculate the proportion of `rain' events as an average $\bar{y}$. 
This allows us to look at the relation between the empirical and predicted probability in each group: 
\begin{itemize}
    \item `10\%' chance of rain' was a slight over-estimate  ($\bar{y} = 0/2 =   0\%$);
    \item `40\%' chance of rain' was a slight under-estimate ($\bar{y} = 1/2 =  50\%$); 
    \item `70\%' chance of rain' was a slight over-estimate  ($\bar{y} = 2/3 =  67\%$); 
    \item `90\%' chance of rain' was a slight under-estimate ($\bar{y} = 1/1 = 100\%$).
\end{itemize}
While this forecaster didn't get it completely right (which would be hard anyway on such a small sample) the deviations from the empirical probabilities are pretty small. Figure~\ref{fig:rel1} gives a graphical representation of this called a \emph{reliability diagram}.
    
\begin{figure}[!t]
    \centering
    \begin{subfigure}{.33\linewidth}
     \begin{tabular}{l|rr}
            \toprule
            id &  $\hat{p}$ &  $y$ \\
            \midrule
            0  &     0.1 &    0 \\
            1  &     0.1 &    0 \\
            \midrule
            2  &     0.4 &    0 \\
            3  &     0.4 &    1 \\
            \midrule
            4  &     0.7 &    0 \\
            5  &     0.7 &    1 \\
            6  &     0.7 &    1
            \\
            \midrule
            7  &     0.9 &    1 \\
            \bottomrule
        \end{tabular}
    \end{subfigure}
    % \includegraphics[width=0.9\textwidth]{figures/intro/Forecaster1.png}\\
    \begin{subfigure}{.55\linewidth}
    \includegraphics[width=1\linewidth]{figures/intro/Forecaster1-fixed-gaps-v2.pdf}
    \end{subfigure}
    \caption{An example of a reliability diagram.}\label{fig:rel1}
\end{figure}

% MPN commented to solve compilation timeout
\begin{table}[htb]
    \centering
    \begin{tabular}{c|c|c|c|c}
         \toprule
         \textbf{Forecasted probability} & \textbf{No. of forecasts} & \textbf{No. of rains} & \textbf{Actual percentage} & \textbf{Difference} \\
         \midrule
         90\% & 1 & 1 & 100\% & -10\% \\
         70\% & 3 & 2 & 67\% & +3\% \\
         40\% & 2 & 1 & 50\% & -10\% \\
         10\% & 2 & 0 & 0\% & +10\% \\
         \bottomrule
    \end{tabular}
    \caption{Toy example described in Section \ref{sec:int:toy} without binning and assuming the model forecasts the exact probabilities shown.}
    \label{tab:int:toy:1}
\end{table}

Reliability diagrams plot the predicted probability, which we will denote as $\hat{p}$, against the empirical probability $\bar{y}$ in the four groups of predictions. This gives four points, here marked by the small red crosses. Ideally we would want the predicted and empirical probabilities to match, in which case they lie on the ascending diagonal (dashed line). 
The blue bars are essentially histogram bars, the width of which indicate bin boundaries on the predicted probabilities (these are fairly arbitrary in this example, but as we will see there are different ways of binning predicted probabilities, particularly if there are many predicted values). 
The narrow red bars, finally, indicate where miscalibration occurs. These may give the false impression that to calibrate corresponds to moving the red crosses vertically, but in fact this needs to be done by horizontal movement as the empirical probability is not directly under control of the forecaster. So, for example, in the second group we can calibrate by adjusting $\hat{p}$ from $0.4$ to $0.5$, moving the cross laterally until it hits the diagonal. Hence, under-estimates correspond to points above the diagonal. 

Let's make the example a bit more interesting by changing the numbers slightly. 
In Figure~\ref{fig:rel2} the groups remain the same but the predicted probabilities are now all distinct. The bin boundaries cut half-way between one group's highest prediction and the next group's lowest. We now need to average over the predicted probabilities in each bin to get the $x$-location of the points in the reliability diagram. The resulting diagram is a bit different but not much, and we still have the same pattern of alternating over- and under-estimates. 

\begin{figure}[!b]
    \centering
    \begin{subfigure}{.33\linewidth}
        \begin{tabular}{l|rr}
            \toprule
            id &  $\hat{p}$ &  $y$ \\
            \midrule
            0  &     0.1 &    0 \\
            1  &     \highlighted{red}{0.2} &    0 \\
            \midrule
            2  &     \highlighted{red}{0.3} &    0 \\
            3  &     0.4 &    1 \\
            \midrule
            4  &     \highlighted{red}{0.6} &    0 \\
            5  &     0.7 &    1 \\
            6  &     \highlighted{red}{0.8} &    1
            \\
            \midrule
            7  &     0.9 &    1 \\
            \bottomrule
        \end{tabular}
    \end{subfigure}
    % \includegraphics[width=0.9\textwidth]{figures/intro/Forecaster1.png}\\
    \begin{subfigure}{.55\linewidth}
    \includegraphics[width=1\linewidth]{figures/intro/Forecaster2-fixed-gaps-v2.pdf}\\
    \end{subfigure}
    \caption{Changing the numbers slightly.}\label{fig:rel2}
\end{figure}

% MPN commented to solve compilation timeout
\begin{table}[htb]
    \centering
    \begin{tabular}{c|c|c|c|c}
         \toprule
         \textbf{Forecasted probability} & \textbf{No. of forecasts} & \textbf{No. of rains} & \textbf{Actual percentage} & \textbf{Difference} \\
         \midrule
         80\% to 100\%& 1 & 1 & 100\% & -10\% \\
         50\% to 80\% & 3 & 2 & 67\%  & +3\% \\
         30\% to 50\% & 2 & 1 & 50\%  & -10\% \\
         0\% to 30\%  & 2 & 0 & 0\%   & +10\% \\
         \bottomrule
    \end{tabular}
    \caption{Changes on the predicted probabilities and binning the scores.}
    \label{tab:int:toy:2}
\end{table}

% \paragraph{Or should we group forecasts differently?}

However, with the modified numbers in Figure~\ref{fig:rel2} the binning into four groups has become less obvious. 
Figure~\ref{fig:rel3} explores a coarser grouping into two bins, which could be justified by the observation that the single bin boundary occurs where the neighbouring predictions are furthest apart. It turns out that under this binning the predictions are perfectly calibrated, as in the first bin the average $\hat{p}$ is $0.25$ and in the second bin it is $0.75$, matching the empirical probabilities in both cases. 
We could even take this a step further and put all predictions in one bin, with an average prediction of $0.5$, matching the prior probability. It seems that with fewer bins it is easier to ensure calibrated predictions. 
On the other hand, too many bins lead to an exaggerated view of miscalibration that is hard to correct (Figure~\ref{fig:rel4}). 
There clearly is a trade-off here, which needs to be decided empirically or heuristically, 
%as there is no general algorithm to decide the optimal binning. 

\begin{figure}[!t]
    \centering
    \begin{subfigure}{.33\linewidth}
     \begin{tabular}{l|rr}
            \toprule
            id &  $\hat{p}$ &  $y$ \\
            \midrule
            0  &     0.1 &    0 \\
            1  &     0.2 &    0 \\
            2  &     0.3 &    0 \\
            3  &     0.4 &    1 \\
            \midrule
            4  &     0.6 &    0 \\
            5  &     0.7 &    1 \\
            6  &     0.8 &    1 \\
            7  &     0.9 &    1 \\
            \bottomrule
        \end{tabular}
    \end{subfigure}
    \begin{subfigure}{.55\linewidth}
    \includegraphics[width=1.0\textwidth]{figures/intro/Forecaster3-fixed-gaps-v2.pdf}\\
    \end{subfigure}
    \caption{A coarser binning of forecasts suggests perfect calibration.}\label{fig:rel3}
\end{figure}

% MPN: commented to solve compilation timeout
\begin{table}[htb]
    \centering
    \begin{tabular}{c|c|c|c|c}
         \toprule
         \textbf{Forecasted probability} & \textbf{No. of forecasts} & \textbf{No. of rains} & \textbf{Actual percentage} & \textbf{Difference} \\
         \midrule
         50\% to 100\% & 4 & 3 & 75\%  & 0\% \\
         0\% to 50\%   & 4 & 1 & 25\%  & 0\% \\
         \bottomrule
    \end{tabular}
    \caption{Applying a coarse binning.}
    \label{tab:int:toy:3}
\end{table}


% % \paragraph{Or not at all?}

\begin{figure}[!b]
    \centering
    \begin{subfigure}{.33\linewidth}
     \begin{tabular}{l|rr}
            \toprule
            id &  $\hat{p}$ &  $y$ \\
            \midrule
            0  &     0.1 &    0 \\
            \midrule
            1  &     {0.2} &    0 \\
            \midrule
            2  &     {0.3} &    0 \\
            \midrule
            3  &     0.4 &    1 \\
            \midrule
            4  &     {0.6} &    0 \\
            \midrule
            5  &     0.7 &    1 \\
            \midrule
            6  &     {0.8} &    1 \\
            \midrule
            7  &     0.9 &    1 \\
            \bottomrule
        \end{tabular}
    \end{subfigure}
    % \includegraphics[width=0.9\textwidth]{figures/intro/Forecaster1.png}\\
    \begin{subfigure}{.55\linewidth}
    \includegraphics[width=1.0\textwidth]{figures/intro/Forecaster4-fixed-gaps-v2.pdf}\\
    \end{subfigure}
    \caption{A less useful reliability diagram where forecasts are not grouped at all.}\label{fig:rel4}
\end{figure}

% MPN: Commented to solve compilation timeout
\begin{table}[htbp]
    \centering
    \begin{tabular}{c|c|c|c|c}
         \toprule
         \textbf{Forecasted probability} & \textbf{No. of forecasts} & \textbf{No. of rains} & \textbf{Actual percentage} & \textbf{Difference} \\
         \midrule
         90\%  & 1 & 1 & 100\% & -10\% \\
         80\%  & 1 & 1 & 100\% & -20\% \\
         70\%  & 1 & 1 & 100\% & -30\% \\
         60\%  & 1 & 0 & 0\%   &  60\% \\
         40\%  & 1 & 1 & 100\% & -60\% \\
         30\%  & 1 & 1 & 0\%   &  30\% \\
         20\%  & 1 & 0 & 0\%   &  20\% \\
         10\%  & 1 & 0 & 0\%   &  10\% \\
         \bottomrule
    \end{tabular}
    \caption{Forecasts not grouped.}
    \label{tab:int:toy:4}
\end{table}

It is clear, then, that {binning or pooling predictions is a fundamental notion} for calibration. 
In particular, we usually need bins to \emph{evaluate} the degree of calibration, as discussed in the next section. 
In order to decide whether a weather forecaster is well-calibrated, we need to look at a good number of forecasts, say over one year. 
We also need to make sure that there is a good spread of predicted probability values. 
But adjusting forecasts in groups also gives rise to practical calibration \emph{methods}, such as empirical binning and isotonic regression, as we will see later. 


\subsection{A closer look at calibration, and why it matters}

% \paragraph{Why are we interested in calibration?}
In general, to calibrate means \emph{to employ a known scale with known properties}. 
% \bb{E.g., additive scale with a well-defined zero, so that ratios are meaningful.}
For example, we can calibrate a thermometer to Celsius or Fahrenheit scales; 
or a weighing device to kilograms or pounds. 
If a measuring device is calibrated to one scale but we need the measurement in another, there are usually simple conversion formulas: 
for example, $F=C\cdot 9/5+32$ for Celsius to Fahrenheit, and $Lb=2.2\cdot Kg$ for kilograms to pounds. 
Notice that the temperature conversion shifts the zero point (0 degrees Celsius is 32 degrees Fahrenheit) as it is essentially arbitrarily chosen. The weight conversion, in contrast, has an absolute zero which is the same for all scales. 
Such scales are called \textit{ratio scales}, because the ratio of two measurements is meaningful: e.g., if one object is twice as heavy as another in kilograms then it will be so regardless of the scale. Such ratios are not meaningful for Celsius and Fahrenheit, but temperature \textit{differences} are.  
For example, we could say that this person's change from morning to evening body temperature today is twice that of yesterday, without specifying the temperature scale. 
It follows that ratios of differences (or intervals) are meaningful in this case, which is why Celsius and Fahrenheit are called \textit{interval scales}. 

For classifiers we want to use the probability scale. Probabilities have an absolute zero like any other ratio scale, and so it is meaningful to say that one event is twice as probable as another. Probabilities also have a fixed maximum, so that taking the complement with respect to the maximum gives another ratio scale: for example, the probability of this event \textbf{not} happening might be twice the probability of another event \textbf{not} happening. This essentially fixes the scale: we don't have pounds vs.\ kilograms dilemmas for probabilities. 

% Q: Is the probability scale additive?
Are probabilities additive? In certain situations it is indeed valid to sum probabilities, for example to obtain the probability of one of a number of mutually exclusive events happening, as might occur when joining classes in a multiclass classification setting. 
But multiplication and division of probabilities are more common basic operations, for example to obtain the joint probability of independent events, or to derive a conditional probability from joint and marginal probabilities. This makes the probability scale \textit{multiplicative}. We could obtain an additive scale by taking logarithms, giving log-likelihoods, logits as differences of log-likelihoods, etc. A couple of observations are worth noting: 
\begin{itemize}
\item Such transformations are fundamentally different from scale conversions such as Celsius to Fahrenheit, because probabilities and log-likelihoods measure different things -- physicists might say they represent different \textit{dimensions}. Nevertheless, the transformations are invertible and hence the dimensions convey the same information. 
\item While some ratios or products of probabilities again yield probabilities, in other cases they may derive another dimension, such as \textit{odds}, which are not expressed on a probability scale.
\end{itemize}

What are the benefits of using well-defined calibrated scales? One obvious benefit is that we can easily combine measurements that are expressed on the same scale without comparing apples and oranges. Another is that we can use standardised decision rules, e.g., defining a fever as a body temperature exceeding 100 degrees Fahrenheit. These benefits% 
\footnote{As for combining multiple probability estimates as might happen in ensemble methods in machine learning, note that the argument of probabilities being multiplicative leads to favouring the \textit{geometric mean} (or the arithmetic mean on log-probabilities). Using the arithmetic mean in this case means that the members of the ensemble are treated as classifiers scoring on some arbitrary but fixed and additive scale, disregarding their probabilistic nature.}
directly carry over to the classification scenario, justifying decision rules such as predicting the class whose estimated probability exceeds $0.5$ in binary classification, or maximum posterior probability for multiclass classification. Importantly, there is an additional benefit to using calibrated probabilities as it means we can adjust these decision rules in a straightforward way to account for different class priors or misclassification costs, as we will show presently.

%Q: What issues might arise when applying MAP decisions to poorly calibrated classifiers such as naive Bayes? 

% PF: UNTIL HERE (27 JAN 9.30 GMT)

% \paragraph{Optimal decisions}
Denote the cost of predicting class $j$ for an instance of true class $i$ as $C(\hat{Y}=j|Y=i)$. 
% Since we don't know the true class of an unlabelled instance, we need to base our prediction on an assessment of the expected cost over all possible true classes. 
The expected cost of predicting class $j$ for instance $x$ is
%
\begin{align}\label{eq::expected-cost}
C(\hat{Y}=j|X=x) &= \sum_i P(Y=i|X=x)C(\hat{Y}=j|Y=i)
\end{align}
%
where $P(Y=i|X=x)$ is the (true) probability of instance $x$ having true class $i$
(as would be given by the Bayes-optimal classifier). 
%
The optimal decision is then to predict the class with lowest expected cost:
\begin{align*}
\hat{Y}^* = \argmin_j C(\hat{Y}=j|X=x) = \argmin_j \sum_i P(Y=i|X=x)C(\hat{Y}=j|Y=i)
\end{align*}
%
% In the special case that all misclassifications have equal cost we can assume without loss of generality that $C(\hat{Y}=j|Y=i)=1$ for $i\neq j$ and $C(\hat{Y}=j|Y=i)=0$ for $i=j$, which gives
% \begin{align*}
% C(\hat{Y}=j|X=x) &= \sum_{i\neq j} P(Y=i|X=x) = 1-P(Y=j|X=x) \\
% %\end{align*}
% %and so
% %\begin{align*}
% \hat{Y}^* &= \arg\min_j [1-P(Y=j|X=x)] = \argmax_j P(Y=j|X=x)
% \end{align*}

In binary classification we have one predicted probability and four cost parameters, and we can rewrite Equation~(\ref{eq::expected-cost}) as
%
\begin{align*}
C(\hat{Y}=+|X=x) &= P(+|x)C(+|+) + \big(1-P(+|x)\big)C(+|-) \\
C(\hat{Y}=-|X=x) &= P(+|x)C(-|+) + \big(1-P(+|x)\big)C(-|-)
\end{align*}
%
where $P(+|x)$ is shorthand for $P(Y=+|X=x)$ and $C(j|i)$ for $C(\hat{Y}=j|Y=i)$.
%
On the optimal decision boundary these two expected costs are equal, 
which gives
\begin{align*}
P(+|x)C(+|+) + (1-P(+|x))C(+|-) = P(+|x)C(-|+) + (1-P(+|x))C(-|-)
\end{align*}
which can be rearranged to give the posterior odds
\begin{align*}
\frac{P(+|x)}{1-P(+|x)} = \frac{C(+|-)-C(-|-)}{C(-|+)-C(+|+)}
\end{align*}
as well as the posterior probability
\begin{align*}%\label{eq::cost-threshold}
P(+|x)  = \frac{{C(+|-)-C(-|-)}}{{C(+|-)-C(-|-)}+{C(-|+)-C(+|+)}} \triangleq c
\end{align*}
%
$c$ thus gives the optimal threshold on the hypothetical Bayes-optimal probabilities. 
It is also the best thing to do in practice, as long as the probabilities are well-calibrated (see Section~\ref{sec:out:conc} for details). 

Under reasonable assumptions (e.g., changing the prediction from correct to incorrect cannot decrease the incurred cost) we can set the cost of true positives and true negatives to zero \cite{elkan2001}; 
$c = \frac{C(+|-)}{C(+|-) + C(-|+)}$ is then the cost of a false positive in proportion to the combined cost of one false positive and one false negative. 
{For instance, if false positives are 4 times as costly as false negatives then we set the decision threshold to $4/(4+1)=0.8$ in order to only make positive predictions if we're pretty certain.}

Similar reasoning applies to changes in class priors \cite{flach2014classification}: 
\begin{itemize}
    \item if we trained on balanced classes but want to deploy with 4 times as many positives compared to negatives, we lower the decision threshold to $0.2$; 
    \item more generally, if we trained for class ratio $r$ and deploy for class ratio $r'$ we set the decision threshold to $r/(r+r')$. 
\end{itemize}
Cost and class prior changes can be combined in the obvious way.

In summary, an important reason we should be interested in calibrating our classifiers is that default decision rules such as maximum posterior probability are fully justified from a decision-theoretic point of view, and can easily be adapted to changes in class and cost distributions. In contrast, poorly calibrated classifiers such as naive Bayes will often perform sub-optimally with default decision rules. It is possible to learn a better decision rule for a given cost and class skew using, e.g., ROC analysis \cite{lachiche2003improving} but this would have to be repeated each time the skew changes. The great advantage of post-calibration is that it only needs to be done once -- in a sense, it optimises all possible decision rules in one go. 


\subsection{Common forms of miscalibration, and how to fix them}

There are many reasons why a probabilistic classifier might produce miscalibrated scores, and hence many ways in which miscalibration manifests itself, but two main types stand out: underconfidence and overconfidence. In this section we look at some examples and introduce three mitigation techniques. 

\begin{figure}[!t]
    \centering
    \begin{subfigure}{0.45\linewidth}
        \includegraphics[width=\linewidth]{figures/intro/Underconfidence.pdf}
        \caption{Underconfidence}
    \end{subfigure}\hfill
    \begin{subfigure}{0.45\linewidth}
        \includegraphics[width=\linewidth]{figures/intro/Overconfidence.pdf}
        \caption{Overconfidence}
    \end{subfigure}
    \caption{Examples of under- and overconfident classifiers. The dots represent the reliability diagram, and the line shows the best-fit logistic curve. 
    To correct the underconfident scores on the left we would have to pull the points away from the midpoint on the $x$-axis,
    whereas to deal with the overconfidence on the right we would push them toward the midpoint. 
    Note that the logistic sigmoid is a good fit for underconfident scores but not for overconfidence.
    Figures reproduced from \citet{niculescu-mizil2005}.}
    \label{fig:under-over}
\end{figure}

The starting point for any calibration analysis is the reliability diagram. Figure~\ref{fig:under-over} shows two typical examples. In both cases the points in the diagram are far from the diagonal, although the effect is smaller in the right figure. 
What do we see in the left figure? It is quite natural to give precedence to vertical information in such graphs, so you might say ``The points on the left are too low, and the points on the right are too high''. But keeping in mind the earlier point that the predicted probabilities on the $x$-axis are under our control but not the empirical probabilities on the $y$-axis, a better way to express this is
%
\begin{quote}
    The lower points are too far to the right, and the higher points are too far to the left. In other words, the points have a tendency to sit too close to the midpoint on the $x$-axis. 
\end{quote}
%
This is the typical pattern displayed by an \textit{underconfident} classifier: it thinks it's {worse} at separating classes than it actually is. 

Hence, to mitigate this, we need to {pull predicted probabilities away from the centre}. As the left figure shows, this can be neatly modelled by a sigmoidal logistic curve, which is defined as
%
\begin{align*}
    p(s; w, m) &= \frac{1}{1+\exp(-w(s-m))}%\\
    % w &= (\mu_{\textit{pos}}-\mu_{\textit{neg}})/\sigma^2, 
    % m = (\mu_{\textit{pos}}+\mu_{\textit{neg}})/2
\end{align*}
%
Here, $s$ is the uncalibrated score produced by the classifier and $p$ is the logistically calibrated score. 
$m$ and $w$ are the two parameters of the logistic curve, which determine the point where $p(s)=0.5$ and the slope at that point, respectively. They can be estimated from the points in the reliability diagram in order to find the best fit. In this case they can be obtained analytically as the mean of the classwise average scores, and the difference between those two means in proportion to the score variance \cite{flach2012machine}.
%(which is assumed to be the same for both classes). 

The fitted logistic curve thus establishes a \textit{calibration map} which transforms uncalibrated scores $s$ into calibrated scores $p$. 
Even though the calibration map doesn't map to empirical probabilities, plotting it over the reliability diagram allows us to see clearly that if we project each point in the reliability diagram vertically onto the calibration map, and replace its $x$-value with the corresponding $y$-value of the projection, we end up with points on or very close to the diagonal, and hence near-perfectly calibrated scores. 

The logistic curve is widely used as a `squashing function', compressing values on a possibly unbounded scale into the $[0,1]$ interval. 
Following \citet{platt2000} it is often used as a way to convert scores from a Support Vector Machine into probabilities. 
Technically this isn't calibration as SVM scores are not probabilities but (signed) geometric distances from the decision boundary -- this is also called \textit{scaling} to emphasise the difference. 
The parametric form of the logistic map can be derived from first principles by assuming that within each class the uncalibrated scores are normally distributed with the same variance (Figure~\ref{fig:logistic}). 

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/intro/Logistic.pdf}\vfill
    \caption{Assuming normally distributed scores within each class (left) leads to a logistic calibration map (right).}\label{fig:logistic}
\end{figure}

The other common form of miscalibration is overconfidence, as exemplified on the right-hand side of Figure~\ref{fig:under-over}. 
Here, we see that
%
\begin{quote}
    The lower points are too far to the left, and the higher points are too far to the right. In other words, the points have a tendency to be too far from the midpoint on the $x$-axis. 
\end{quote}
%
An \textit{overconfident} classifier thinks it's {better} at separating classes than it actually is. 
Hence we need to {make predicted probabilities less extreme by pushing them toward the centre}. 
The paper we took this figure from \cite{niculescu-mizil2005} also fitted a logistic curve to this reliability diagram, because they were investigating the effect of Platt scaling in a wide range of scenarios. But we see clearly that the fit is rather poor, and using this logistic curve as a calibration map is likely to make matters worse. In this particular case we would be looking for something that can produce an inverse sigmoidal curve. What would be a principled way to achieve this? 

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/intro/Beta.pdf}
    \caption{An example of Beta calibration where overconfident scores (left) lead to an inverse-sigmoidal calibration map (right).}\label{fig:beta}
\end{figure}

One approach that works well is to model the classwise scores with Beta distributions \cite{kull2017,kull2017ejs}.
These assume random variables bounded in $[0,1]$ which is exactly what we need for post-hoc calibration. 
They can easily model the skewed distributions resulting from overconfident classifiers, as demonstrated in Figure~\ref{fig:beta}. 
Mathematically, these curves have three parameters: 
%
    \begin{align*}
        p(s; a, b, c) &= \frac{1}{1+\exp(-a \ln s + b \ln (1-s) - c)}
        % a &= \alpha_{\textit{pos}}-\alpha_{\textit{neg}}, 
        % b = \beta_{\textit{neg}}-\beta_{\textit{pos}}
    \end{align*}
%
This additional degree of freedom means that Beta calibration can produce both sigmoidal and inverse-sigmoidal calibration maps. 
It can even fit the identity map ($a=b=1$, $c=0$), which means that it can recognise that scores are already calibrated. 
In contrast, applying logistic calibration to a calibrated classifier will decalibrate it. 

%PF: UNTIL HERE (28 JAN 18.00 GMT)

So far we have seen two calibration techniques: 
\begin{itemize}
    \item logistic calibration, which -- although technically a scaling technique, mapping real-valued scores into probabilities -- can adjust for underconfident scores; 
    \item Beta calibration, which assumes a classifier already scores on a probability scale, and which can adjust for both over- and underconfident scores. 
\end{itemize}
We will now take a first look at a third calibration technique, quite different from these two because it derives a calibration map from the \textit{ranks} of a set of scores, and hence works for classifiers scoring on arbitrary scales. It is also different from logistic and Beta calibration because it doesn't attempt to model the classwise score distributions, and is hence \textit{non-parametric}. 

The technique in question is called \textit{isotonic regression}, belying its origin as an alternative to linear regression which learns a piecewise constant, monotonically increasing or decreasing function. There are several algorithms for isotonic regression, one of which is called \textit{pooled adjacent violators}, which in turn is also used for constructing the convex hull of an ROC curve \cite{zadrozny2001,fawcett2007}. Figure~\ref{fig:isotonic} gives an example. 

\begin{figure}[!t]
    \centering
    \begin{subfigure}{0.44\linewidth}
    \includegraphics[width=\linewidth]{figures/intro/ROCCH.pdf}
    \caption{ROC curve and convex hull.}
    \end{subfigure}
    \begin{subfigure}{0.55\linewidth}
    \includegraphics[width=\linewidth]{figures/intro/ROCcal2.pdf}
    \caption{Isotonic calibration map.}
    \end{subfigure}
    \caption{An example of isotonic calibration which derives a piece-wise constant calibration map from the ROC convex hull (Source: \cite{flach2016roc}).}\label{fig:isotonic}
\end{figure}

The technique starts from a list of test instances, ranked on their scores; this might give a list of class labels like that depicted at the top of the right figure in Figure~\ref{fig:isotonic}. We then proceed to segment this ranking such that, in each adjacent pair of segments, the right neighbour has a larger proportion of positives than the left neighbour. This defines a unique set of segments, which is depicted on the right of the right figure. Each segment defines an interval on the original classifier scores, as well as an empirical probability of positives in that segment which is taken as the calibrated score for all instances whose score falls in that interval. The calibration map is thus piece-wise constant and increasing. 

As a non-parametric method, isotonic regression avoids problems of misspecification which can plague parametric models. For example, a perfectly calibrated classifier has classwise scores which are far from normally distributed, so applying logistic calibration will make matters worse. The downside is that isotonic regression tends to need more labelled data to reliably estimate the segment boundaries and the empirical probabilities within each segment, and is more liable to overfitting if the data is not plentiful. 


%----------------------------------------------------%
\subsection{Multiclass calibration}
%----------------------------------------------------%

The examples we have seen so far all relate to binary classification. Is it straightforward to generalise calibration concepts and methods to more than two classes? 
The answer to this question is quite involved. Some ideas do generalise quite easily: for example, we can model per-class scores by multivariate distributions such as Dirichlet distributions \cite{kull2019}. Some other ideas don't generalise easily at all: for example, a multiclass generalisation of isotonic regression is not straightforward because rankings are inherently bipartite. Such approaches therefore need to be approximated by considering classes in a pairwise or one-versus-rest manner. 

This helps to explain why there is divergence even at a definitional level. 
There are at least three different ways of \emph{defining} what it means to be calibrated in a multiclass setting. 
They are equivalent for binary classification but increasingly stronger for more than two classes,%
\footnote{In rare cases it is possible for a multiclass classifier to be classwise calibrated but not confidence calibrated.}
and can be summarised as follows: 
    \begin{itemize}
        \item {Confidence calibration}: only consider the highest predicted probability. 
        \item {Classwise calibration}: only consider marginal probabilities.
        \item {Multiclass calibration}: consider the entire vector of predicted probabilities.
    \end{itemize}
We will use this terminology throughout the paper to avoid confusion. 

%\renewcommand{\vph}{\hat{\mathbf{p}}}

\textit{Confidence calibration} was proposed by \citet{guo2017}, although not under that name. It requires that among all instances where the probability of \emph{the most likely class} is predicted to be $c$, the expected accuracy is $c$. 
Formally, a probabilistic classifier $\vph:\sX\to\Sk$ is \emph{confidence-calibrated}, if for any confidence level $c\in[0,1]$, 
the actual proportion of the predicted class, among all possible instances $\vx$ being predicted this class with confidence $c$, is equal to $c$:  
\begin{align*} 
P(Y=i \: | \: \ph_i(\vx)=c)=c\qquad\text{where }\ i=\argmax_j \ph_j(\vx).
%P\Big(Y=\argmax\big(\vph(X)\big) \: \Big| \: \max\big(\vph(X)\big)=c\Big)=c.
\end{align*}

\textit{Classwise calibration}, proposed by \citet{zadrozny2002}, requires that all \emph{one-vs-rest} probability estimators obtained from the original multiclass model are calibrated. 
Formally, a probabilistic classifier $\vph:\sX\to\Sk$ is \emph{classwise-calibrated}, if for any class $i$ and any predicted probability $q_i$ for this class, 
the actual proportion of class $i$, among all possible instances $\vx$ getting the same prediction $\ph_i(\vx)=q_i$, is equal to $q_i$:  
\begin{align*} 
P(Y=i\mid \ph_i(\vx)=q_i)=q_i\qquad\text{for }\ i=1,\dots,k.
\end{align*}

\textit{Multiclass calibration} is the {strongest form of calibration} for more than two classes, subsuming the previous two definitions. 
A probabilistic classifier $\vph:\sX\to\Sk$ is \emph{multiclass-calibrated} if for any prediction vector $\vq=(q_1,\dots,q_k)\in\Sk$, the proportions of classes among all possible instances $\vx$ getting the same prediction $\vph(\vx)=\vq$ are equal to the prediction vector $\vq$:  
\begin{align*} %\label{eq:calib}
P(Y=i\mid \vph(\vx)=\vq)=q_i\qquad\text{for }\ i=1,\dots,k.
\end{align*}

For practical purposes, the conditions in these definitions need to be relaxed. This is where \emph{binning} comes in. 
Once we have the bins, we can draw a \emph{reliability diagram} as in the two-class case. For classwise calibration, we can show per-class reliability diagrams or a single averaged one. 
One way to assess the degree of calibration is by means of the \emph{gaps} in the reliability diagram. 
This leads us to evaluation metrics for calibration, which is the topic of the next section. 

==> sections/b_contribution.tex <==
\subsection*{Author contributions}\label{sec:contribution}

 \begin{table}[h!]
     \centering
     \begin{tabular}{l|c|c|c|c|c|c}
 \toprule
 Role                         & TS & HS & MP & RS & MK & PF \\
 \midrule
 Conceptualisation            & X  &  X &    &    & X  & X  \\
 Data curation:               &    &    &    &    &    &    \\
 Formal Analysis:             &    &    &    &  X &    &    \\
 Funding acquisition:         &    &    &    &    &    &    \\
 Investigation:               & X  &  X &    &    & X  & X  \\
 Methodology:                 & X  &  X &    &    & X  & X  \\
 Project administration:      &    &    &    &    &    &    \\
 Resources:                   &    &    &    &    &    &    \\
 Software:                    & X  &  X & X  &    &    &    \\
 Supervision:                 &    &    &    &    &    & X  \\
 Validation:                  &    &    &    &    &    &    \\
 Visualisation:               &    &    & X  &    &    &    \\
 Writing - original draft:    & X  & X  & X  &    &    & X  \\
 Writing - review \& editing: & X  & X  & X  & X  & X  & X  \\
 \bottomrule
     \end{tabular}
     \caption{Caption}
     \label{tab:my_label}
 \end{table}

% These contributions should be listed at the separate title page
Conceptualisation: TSF, HS, MK and PF; Formal Analysis: TSF, HS, MPN, RS, MK and PF; Methodology: TSF, HS, MK and PF; Software: TSF, HS and MPN; Supervision: PF; Visualisation: MPN; Writing - original draft preparation: TSF, HS, MPN and PF; Writing - review and editing: TSF, HS, MPN, RS, MK and PF. \footnote{The categories follow the CRediT taxonomy: http://credit.niso.org/}

==> sections/notation_list.tex <==
Feature / Label random variable: $(\mathbf{X}, Y)$

Feature vector / Label instance: $(\mathbf{x}, y)$

Feature space: $\mathbb{X}$

Probability simplex: $\mathbb{P}$

Probability measure: $\mathsf{P}$

Probability vector: $\mathbf{s} = [s_1, ..., s_K]$

Cost of predicting class $j$ for an instance of true class $i$: $\mathsf{c}(\hat{Y}=j|Y=i)$

Cost parameter (the cost of a false positive in proportion to the combined cost of one false positive and one false negative): $c$

Class ratio: $r$

Calibrated binary score (calibration map function): $\mathsf{g}(s; w, m)$

Uncalibrated score: $s$, $\mathbf{s}=[s_1, ..., s_K]$

Confidence level: $\alpha$

Uncalibrated model output on class $i$: $s_i$

Probability on class $i$: $q_i$

Probability vector: $\mathbf{s}=[s_1, ..., s_K]$, $\mathbf{q}=[q_1,...,q_K]$

Instance one-hot vector: $\dot{\mathbf{y}}=[y_1,\ldots,y_K]$

Scoring rule: $\phi(\mathbf{p}, \dot{\mathbf{y}})$

Expectation: $\mathbb{E}$ (Decomposition uses $E$)

Random probability vector: $\mathbf{S}=[S_1,S_2,...,S_K]$, $\mathbf{C}=[C_1,C_2,\ldots,C_K]$ (calibrated), $\mathbf{Q}=[Q_1,Q_2,\ldots,Q_K]$ (Bayes optimal).

(Check) Predicted score / corresponding TP rate on $i_{th}$ instance: $\hat{p}_i$, $\bar{y}_i$

Bin: $\mathbb{B}_j$

Set of each bin: $\mathbb{I}_j \in \{i; \mathsf{s}_i \in \mathbb{B}_j\}$

Set size: $\text{count}(\mathbb{I}_j)$, $|\mathbb{B}_{j}|$

(Check) Average predicted scores: $\hat{p}_j$, $\Bar{p}(\mathbb{B}_{j})$

(Check) The proportion of positives in bin: $\Bar{y}(\mathbb{B}_{j})$

Accuracy in each bin: $\mathsf{acc}(\mathbb{B}_{j})$

ECE: $\mathsf{ECE}$

A classifier: $\mathsf{f}$

Test set: $\{(\mathbf{x}_1, y_1), \dots, (\mathbf{x}_N, y_N)\}$

(Check) Calibration measure: $\phi(\boldsymbol{\hat{p}}(X_{\text{test}}),\boldsymbol{y}_{\text{test}})$

Calibrator: $\mathsf{g}: \mathbb{S}_{\mathbb{Y}} \rightarrow \mathbb{P}_{\mathbb{Y}}$

Probability vector space: $\mathbb{P}_{\mathbb{Y}}$

Score space: $\mathbb{S}_{\mathbb{Y}}$

Calibration set: $\mathbb{C} = \{(\mathbf{s}_1, y_1), \dots, (\mathbf{s}_N, y_N)\}$

Loss function: $L(\mathbb{C})$

Bins: $\{\mathbb{B}_1, \dots, \mathbb{B}_M \}, \mathbb{B}_j \subset [0, 1], \cup_{j=1}^{M} \mathbb{B}_j = [0, 1]$

Probability estimates in the Bins: $\mathbf{a}=(a_1,\dots,a_{M})$, $a_j \in \{0, 1\}$

Bin boundaries: $\mathbf{b}=(b_1,\dots,b_M)$, $b_j \in [0, 1], b_j < b_{j+1}$

Edge values:  $\mathbf{v}=(v_1,\dots,v_{M})$, $ v_j \in [0, 1], v_j \leq v_{j+1}$

Logits: $\mathbf{z} = [z_1, \dots, z_K] \in \mathbb{R}^K$

Sudo-logits: $z_j = \text{logit}_j (\mathbf{s})$

Log probability: $\mathsf{ln} \mathbf{s}$

Costs: $c_{FP}$, $c_{FN}$

Decision boundary:  $s_{\text{dec}}$

TPr, FPr: $tpr(s_{dec})$, $fpr(s_{dec})$ 

Weighted accuracy: $\textbf{acc}_{p}(t)$

F beta: $F_{\beta}$

F d: $F_{d}(t)$

A quantile regression model: $\mathsf{q}: \mathbb{X} \times [0, 1] \rightarrow \mathbb{R}$

A regression model (or conditional density estimator): $$f: \mathbb{X} \rightarrow \{s \mid s:\mathbb{R} \rightarrow [0, \infty), \int s(y)dy = 1 \}$$




















